ACID: A Low Dimensional Characterization of Markov-Modulated and Self-Exciting Counting Processes

The conditional intensity (CI) of a counting process $Y_t$ is based on the minimal knowledge $\mathcal{F}_t^Y$, i.e., on the observation of $Y_t$ alone. Prominently, the mutual information rate of a signal and its Poisson channel output is a difference functional between the CI and the intensity that has full knowledge about the input. While the CI of Markov-modulated Poisson processes evolves according to Snyder's filter, self-exciting processes, e.g., Hawkes processes, specify the CI via the history of $Y_t$. The emergence of the CI as a self-contained stochastic process prompts us to bring its statistical ensemble into focus. We investigate the asymptotic conditional intensity distribution (ACID) and emphasize its rich information content. We assume the case in which the CI is determined from a sufficient statistic that progresses as a Markov process. We present a simulation-free method to compute the ACID when the dimension of the sufficient statistic is low. The method is made possible by introducing a backward recurrence time parametrization, which has the advantage to align all probability inflow in a boundary condition for the master equation. Case studies illustrate the usage of ACID for three primary examples: 1) the Poisson channels with binary Markovian input (as an example of a Markov-modulated Poisson process), 2) the standard Hawkes process with exponential kernel (as an example of a self-exciting counting process) and 3) the Gamma filter (as an example of an approximate filter to a Markov-modulated Poisson process).

==> Fig7_part1_extra.tex <==
\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0	0\\
0.291772771818225	0\\
0.291772771818225	1\\
2.04024525635636	1\\
2.04024525635636	2\\
2.11387038806217	2\\
2.11387038806217	3\\
4.14697535341548	3\\
4.14697535341548	4\\
4.50260182890084	4\\
4.50260182890084	5\\
5.98732507038431	5\\
5.98732507038431	6\\
6.01983002336989	6\\
6.01983002336989	7\\
6.09621611079786	7\\
6.09621611079786	8\\
6.75107071564799	8\\
6.75107071564799	9\\
6.81640322368433	9\\
6.81640322368433	10\\
6.96142514683589	10\\
6.96142514683589	11\\
9.20641957008332	11\\
9.20641957008332	12\\
9.7579261277762	12\\
9.7579261277762	13\\
11.8110975031566	13\\
11.8110975031566	14\\
};

==> fig7_part1_extra_220209.tex <==

\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0	0\\
1.90043034201646	0\\
1.90043034201646	1\\
2.42249692675537	1\\
2.42249692675537	2\\
2.44746720640466	2\\
2.44746720640466	3\\
3.33405639303388	3\\
3.33405639303388	4\\
3.54127961580251	4\\
3.54127961580251	5\\
3.67643269587083	5\\
3.67643269587083	6\\
3.92083834639183	6\\
3.92083834639183	7\\
3.98052546735389	7\\
3.98052546735389	8\\
4.1847409678019	8\\
4.1847409678019	9\\
4.22781596843031	9\\
4.22781596843031	10\\
4.23637321351316	10\\
4.23637321351316	11\\
4.30473748442818	11\\
4.30473748442818	12\\
4.35455634422505	12\\
4.35455634422505	13\\
4.61101340486059	13\\
4.61101340486059	14\\
4.76038901173518	14\\
4.76038901173518	15\\
5.23603543745627	15\\
5.23603543745627	16\\
5.87015830519904	16\\
5.87015830519904	17\\
6.81758578961062	17\\
6.81758578961062	18\\
6.8422516438123	18\\
6.8422516438123	19\\
7.79262935686131	19\\
7.79262935686131	20\\
8.4268748386327	20\\
8.4268748386327	21\\
13.7211042601068	21\\
13.7211042601068	22\\
};

==> fig7_part1a_220209.tex <==
\pgfplotsset{my plot options/.style={color=blue, line width=0.5pt, opacity = 0.07, forget plot}}
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0452573690506952	0\\
0.0452573690506952	1\\
0.611269842056881	1\\
0.611269842056881	2\\
1.35494031819486	2\\
1.35494031819486	3\\
1.50087249969834	3\\
1.50087249969834	4\\
1.5122283890939	4\\
1.5122283890939	5\\
1.54657188721032	5\\
1.54657188721032	6\\
3.17502464585893	6\\
3.17502464585893	7\\
3.44289432420551	7\\
3.44289432420551	8\\
3.79655486125036	8\\
3.79655486125036	9\\
4.62289651376888	9\\
4.62289651376888	10\\
4.80864958079705	10\\
4.80864958079705	11\\
5.45369715152413	11\\
5.45369715152413	12\\
5.53556193807393	12\\
5.53556193807393	13\\
5.57817856628142	13\\
5.57817856628142	14\\
5.63054160493678	14\\
5.63054160493678	15\\
5.65397628455759	15\\
5.65397628455759	16\\
6.64615556338759	16\\
6.64615556338759	17\\
7.88618987639998	17\\
7.88618987639998	18\\
8.65478828846046	18\\
8.65478828846046	19\\
8.75676593490012	19\\
8.75676593490012	20\\
8.78100553101916	20\\
8.78100553101916	21\\
9.00250917044776	21\\
9.00250917044776	22\\
9.11518437151272	22\\
9.11518437151272	23\\
9.44225177237919	23\\
9.44225177237919	24\\
11.1611525737742	24\\
11.1611525737742	25\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.276010595235483	0\\
0.276010595235483	1\\
0.700132621952875	1\\
0.700132621952875	2\\
5.4033078161168	2\\
5.4033078161168	3\\
5.69036603549682	3\\
5.69036603549682	4\\
6.22769928129811	4\\
6.22769928129811	5\\
6.71064957171485	5\\
6.71064957171485	6\\
7.02960500702054	6\\
7.02960500702054	7\\
7.98793779339422	7\\
7.98793779339422	8\\
9.26790280455273	8\\
9.26790280455273	9\\
11.2666501609013	9\\
11.2666501609013	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.147960800593616	0\\
0.147960800593616	1\\
0.224557579591881	1\\
0.224557579591881	2\\
0.230891597566512	2\\
0.230891597566512	3\\
0.375955169481472	3\\
0.375955169481472	4\\
0.58621670912693	4\\
0.58621670912693	5\\
0.676239928179093	5\\
0.676239928179093	6\\
0.677137954537102	7\\
0.772189769408882	7\\
0.772189769408882	8\\
1.03750651701775	8\\
1.03750651701775	9\\
1.10154436280887	9\\
1.10154436280887	10\\
1.17979226461912	10\\
1.17979226461912	11\\
1.66992852745244	11\\
1.66992852745244	12\\
2.23162505338838	12\\
2.23162505338838	13\\
2.35888762813799	13\\
2.35888762813799	14\\
3.69655124884855	14\\
3.69655124884855	15\\
3.80203671487252	15\\
3.80203671487252	16\\
4.00965391225757	16\\
4.00965391225757	17\\
4.37102249080878	17\\
4.37102249080878	18\\
4.37590467304761	18\\
4.37590467304761	19\\
4.52118176898995	19\\
4.52118176898995	20\\
4.52208026546527	21\\
5.04079843967735	21\\
5.04079843967735	22\\
5.0766443190731	22\\
5.0766443190731	23\\
5.18418494013163	23\\
5.18418494013163	24\\
5.38506129673003	24\\
5.38506129673003	25\\
6.14324981581439	25\\
6.14324981581439	26\\
6.35769986782694	26\\
6.35769986782694	27\\
6.71788751350718	27\\
6.71788751350718	28\\
6.84400411850593	28\\
6.84400411850593	29\\
7.08054259174423	29\\
7.08054259174423	30\\
7.49611249620668	30\\
7.49611249620668	31\\
7.66726437980641	31\\
7.66726437980641	32\\
7.85008281584987	32\\
7.85008281584987	33\\
7.93972639340177	33\\
7.93972639340177	34\\
8.10462875206915	34\\
8.10462875206915	35\\
8.1405067350402	35\\
8.1405067350402	36\\
8.91458887350367	36\\
8.91458887350367	37\\
9.10701776061943	37\\
9.10701776061943	38\\
9.92249490040169	38\\
9.92249490040169	39\\
9.99450326298255	39\\
9.99450326298255	40\\
10.0833461584613	40\\
10.0833461584613	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.12748400092072	0\\
1.12748400092072	1\\
2.93878254892194	1\\
2.93878254892194	2\\
3.13401562061622	2\\
3.13401562061622	3\\
4.03852376066396	3\\
4.03852376066396	4\\
4.05733162799972	4\\
4.05733162799972	5\\
4.21265487977711	5\\
4.21265487977711	6\\
4.27533339621404	6\\
4.27533339621404	7\\
4.72980480060398	7\\
4.72980480060398	8\\
5.34081662190795	8\\
5.34081662190795	9\\
5.3895641113503	9\\
5.3895641113503	10\\
6.03979077058731	10\\
6.03979077058731	11\\
8.1557456757026	11\\
8.1557456757026	12\\
9.18318295881253	12\\
9.18318295881253	13\\
10.9793541566022	13\\
10.9793541566022	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0589919225862214	0\\
0.0589919225862214	1\\
0.510117557554244	1\\
0.510117557554244	2\\
2.05168469112281	2\\
2.05168469112281	3\\
2.40915016902006	3\\
2.40915016902006	4\\
2.6551013825727	4\\
2.6551013825727	5\\
2.93611465691293	5\\
2.93611465691293	6\\
2.96502557118292	6\\
2.96502557118292	7\\
3.79538546308399	7\\
3.79538546308399	8\\
3.84697674620941	8\\
3.84697674620941	9\\
3.91132264733447	9\\
3.91132264733447	10\\
4.68404302713068	10\\
4.68404302713068	11\\
4.70468660611756	11\\
4.70468660611756	12\\
8.66212135657463	12\\
8.66212135657463	13\\
9.6512216891761	13\\
9.6512216891761	14\\
11.8490440293767	14\\
11.8490440293767	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0159766958999867	0\\
0.0159766958999867	1\\
0.230199774590449	1\\
0.230199774590449	2\\
9.85183519556326	2\\
9.85183519556326	3\\
10.2350288392394	3\\
10.2350288392394	4\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.263069073906673	0\\
0.263069073906673	1\\
0.465233706798822	1\\
0.465233706798822	2\\
0.572530202636917	2\\
0.572530202636917	3\\
0.645653660541424	3\\
0.645653660541424	4\\
1.30455066933138	4\\
1.30455066933138	5\\
1.72004060014349	5\\
1.72004060014349	6\\
1.80967263978748	6\\
1.80967263978748	7\\
2.48098509315513	7\\
2.48098509315513	8\\
2.92521903089631	8\\
2.92521903089631	9\\
4.45603712046829	9\\
4.45603712046829	10\\
4.75339993470385	10\\
4.75339993470385	11\\
6.75384205712717	11\\
6.75384205712717	12\\
7.29616036610939	12\\
7.29616036610939	13\\
7.81582227113681	13\\
7.81582227113681	14\\
10.4048864589255	14\\
10.4048864589255	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0971502704178135	0\\
0.0971502704178135	1\\
0.489648740873342	1\\
0.489648740873342	2\\
0.979512600226535	2\\
0.979512600226535	3\\
0.982338457423211	4\\
1.11277701957543	4\\
1.11277701957543	5\\
1.41266640454833	5\\
1.41266640454833	6\\
1.66227056831571	6\\
1.66227056831571	7\\
1.73316756453576	7\\
1.73316756453576	8\\
1.9574233082651	8\\
1.9574233082651	9\\
2.07755480451317	9\\
2.07755480451317	10\\
3.08355210084613	10\\
3.08355210084613	11\\
3.20210313399285	11\\
3.20210313399285	12\\
3.93602116917454	12\\
3.93602116917454	13\\
3.94991097419327	13\\
3.94991097419327	14\\
3.97493402294538	14\\
3.97493402294538	15\\
4.02586909563665	15\\
4.02586909563665	16\\
4.26723997361677	16\\
4.26723997361677	17\\
4.56096217135318	17\\
4.56096217135318	18\\
4.9762729274023	18\\
4.9762729274023	19\\
5.0368594525352	19\\
5.0368594525352	20\\
5.05529542228926	20\\
5.05529542228926	21\\
5.10613531969191	21\\
5.10613531969191	22\\
5.19657499125825	22\\
5.19657499125825	23\\
5.24089398908762	23\\
5.24089398908762	24\\
5.58644426184203	24\\
5.58644426184203	25\\
5.68505332963358	25\\
5.68505332963358	26\\
6.2369755361516	26\\
6.2369755361516	27\\
8.38177612442632	27\\
8.38177612442632	28\\
8.62509420375818	28\\
8.62509420375818	29\\
8.70821187789009	29\\
8.70821187789009	30\\
8.80813911404407	30\\
8.80813911404407	31\\
9.62539179609364	31\\
9.62539179609364	32\\
10.4481903615418	32\\
10.4481903615418	33\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.09860725842557	0\\
1.09860725842557	1\\
1.30403772978855	1\\
1.30403772978855	2\\
1.51772304652946	2\\
1.51772304652946	3\\
1.67698610232242	3\\
1.67698610232242	4\\
1.68164296616995	4\\
1.68164296616995	5\\
2.02700203308983	5\\
2.02700203308983	6\\
2.32561856118334	6\\
2.32561856118334	7\\
3.37921043511462	7\\
3.37921043511462	8\\
3.95527514625177	8\\
3.95527514625177	9\\
4.07633052990888	9\\
4.07633052990888	10\\
5.01883932293248	10\\
5.01883932293248	11\\
5.63436585089346	11\\
5.63436585089346	12\\
8.0126944727181	12\\
8.0126944727181	13\\
8.05164624520756	13\\
8.05164624520756	14\\
8.12787167632712	14\\
8.12787167632712	15\\
8.93925641125197	15\\
8.93925641125197	16\\
9.13862880302217	16\\
9.13862880302217	17\\
9.35615938233846	17\\
9.35615938233846	18\\
9.67477590065129	18\\
9.67477590065129	19\\
9.92442822188594	19\\
9.92442822188594	20\\
10.3548727279195	20\\
10.3548727279195	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.38164013166098	0\\
1.38164013166098	1\\
2.25045987380717	1\\
2.25045987380717	2\\
2.29140940717371	2\\
2.29140940717371	3\\
2.55638467349224	3\\
2.55638467349224	4\\
2.79742636426787	4\\
2.79742636426787	5\\
6.46752749074375	5\\
6.46752749074375	6\\
7.08614247637898	6\\
7.08614247637898	7\\
7.7571496595264	7\\
7.7571496595264	8\\
9.02404670810322	8\\
9.02404670810322	9\\
10.5020968440501	9\\
10.5020968440501	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.162602980586243	0\\
0.162602980586243	1\\
0.456108065317025	1\\
0.456108065317025	2\\
0.595548994542348	2\\
0.595548994542348	3\\
0.663563011816272	3\\
0.663563011816272	4\\
1.01500151421254	4\\
1.01500151421254	5\\
1.24243428287841	5\\
1.24243428287841	6\\
1.42324697770664	6\\
1.42324697770664	7\\
1.60573714040205	7\\
1.60573714040205	8\\
1.964297936454	8\\
1.964297936454	9\\
2.19328245245405	9\\
2.19328245245405	10\\
2.2540693870664	10\\
2.2540693870664	11\\
2.41939725014328	11\\
2.41939725014328	12\\
2.53650714266857	12\\
2.53650714266857	13\\
2.63765642761285	13\\
2.63765642761285	14\\
2.80420655724464	14\\
2.80420655724464	15\\
2.86730211303837	15\\
2.86730211303837	16\\
3.04359951060074	16\\
3.04359951060074	17\\
3.14713969785396	17\\
3.14713969785396	18\\
3.26810870775699	18\\
3.26810870775699	19\\
3.29839263489123	19\\
3.29839263489123	20\\
3.38961180363891	20\\
3.38961180363891	21\\
3.43985672887376	21\\
3.43985672887376	22\\
3.49027418823409	22\\
3.49027418823409	23\\
3.75253451654152	23\\
3.75253451654152	24\\
4.65763177077751	24\\
4.65763177077751	25\\
4.66919187684248	25\\
4.66919187684248	26\\
4.76066374357404	26\\
4.76066374357404	27\\
4.83408144934105	27\\
4.83408144934105	28\\
4.84054402706021	28\\
4.84054402706021	29\\
6.88474085954908	29\\
6.88474085954908	30\\
8.06945343421191	30\\
8.06945343421191	31\\
10.2652013146921	31\\
10.2652013146921	32\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.943994652805149	0\\
0.943994652805149	1\\
4.73054539757505	1\\
4.73054539757505	2\\
8.92120612806476	2\\
8.92120612806476	3\\
9.14804459594393	3\\
9.14804459594393	4\\
9.60528258230927	4\\
9.60528258230927	5\\
12.3621478093898	5\\
12.3621478093898	6\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.488867247330557	0\\
0.488867247330557	1\\
1.84467682445619	1\\
1.84467682445619	2\\
3.31469044421154	2\\
3.31469044421154	3\\
3.94328310151085	3\\
3.94328310151085	4\\
4.04904492246411	4\\
4.04904492246411	5\\
4.63190502707214	5\\
4.63190502707214	6\\
4.9604878301856	6\\
4.9604878301856	7\\
5.26098634504486	7\\
5.26098634504486	8\\
6.46863383252266	8\\
6.46863383252266	9\\
6.72719812735314	9\\
6.72719812735314	10\\
6.97651273518681	10\\
6.97651273518681	11\\
7.08727180870882	11\\
7.08727180870882	12\\
7.64242866565008	12\\
7.64242866565008	13\\
7.83228848395026	13\\
7.83228848395026	14\\
8.22552954141582	14\\
8.22552954141582	15\\
8.57691034015941	15\\
8.57691034015941	16\\
9.08814724726911	16\\
9.08814724726911	17\\
9.19758449595325	17\\
9.19758449595325	18\\
9.30035900869147	18\\
9.30035900869147	19\\
9.38185816500084	19\\
9.38185816500084	20\\
11.9408958478914	20\\
11.9408958478914	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.286094078264689	0\\
0.286094078264689	1\\
0.287375523961643	2\\
0.663784444352796	2\\
0.663784444352796	3\\
0.713902880143714	3\\
0.713902880143714	4\\
1.2036271308125	4\\
1.2036271308125	5\\
1.3046266762992	5\\
1.3046266762992	6\\
2.4193499699426	6\\
2.4193499699426	7\\
2.53751970322503	7\\
2.53751970322503	8\\
3.83598108713487	8\\
3.83598108713487	9\\
4.04024930228212	9\\
4.04024930228212	10\\
4.39546688706119	10\\
4.39546688706119	11\\
5.61896452634281	11\\
5.61896452634281	12\\
5.89181880594886	12\\
5.89181880594886	13\\
5.96112562468264	13\\
5.96112562468264	14\\
6.28348790986015	14\\
6.28348790986015	15\\
6.64356719817092	15\\
6.64356719817092	16\\
6.66859178675603	16\\
6.66859178675603	17\\
7.21367699180062	17\\
7.21367699180062	18\\
8.54816284592183	18\\
8.54816284592183	19\\
8.71017939028797	19\\
8.71017939028797	20\\
9.81858185729183	20\\
9.81858185729183	21\\
9.85862417185028	21\\
9.85862417185028	22\\
11.0937635851885	22\\
11.0937635851885	23\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.27918690641456	0\\
2.27918690641456	1\\
2.99652646095181	1\\
2.99652646095181	2\\
3.10176123843243	2\\
3.10176123843243	3\\
3.44486811612519	3\\
3.44486811612519	4\\
4.79147982967798	4\\
4.79147982967798	5\\
5.33065058018349	5\\
5.33065058018349	6\\
6.2055253857337	6\\
6.2055253857337	7\\
6.33517115901952	7\\
6.33517115901952	8\\
6.36558463791218	8\\
6.36558463791218	9\\
7.16208897315066	9\\
7.16208897315066	10\\
7.8011517462627	10\\
7.8011517462627	11\\
8.0551727536688	11\\
8.0551727536688	12\\
8.41086213736947	12\\
8.41086213736947	13\\
9.49509567950285	13\\
9.49509567950285	14\\
10.1828004915093	14\\
10.1828004915093	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.232861427522646	0\\
0.232861427522646	1\\
1.7452134135586	1\\
1.7452134135586	2\\
1.74833080450761	3\\
1.88582156995665	3\\
1.88582156995665	4\\
2.01941541249585	4\\
2.01941541249585	5\\
2.85400446431505	5\\
2.85400446431505	6\\
3.39735347423587	6\\
3.39735347423587	7\\
5.44814001342588	7\\
5.44814001342588	8\\
5.58987072055508	8\\
5.58987072055508	9\\
8.45049611036342	9\\
8.45049611036342	10\\
8.87911120718748	10\\
8.87911120718748	11\\
9.36475572204539	11\\
9.36475572204539	12\\
9.59014664064929	12\\
9.59014664064929	13\\
9.80577288760457	13\\
9.80577288760457	14\\
9.87975943500636	14\\
9.87975943500636	15\\
10.0886456528266	15\\
10.0886456528266	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.484583677174037	0\\
0.484583677174037	1\\
0.951677350594085	1\\
0.951677350594085	2\\
1.12217828563816	2\\
1.12217828563816	3\\
1.32518028133394	3\\
1.32518028133394	4\\
1.40059308130069	4\\
1.40059308130069	5\\
4.45830235485048	5\\
4.45830235485048	6\\
5.28816403851998	6\\
5.28816403851998	7\\
6.31812282080317	7\\
6.31812282080317	8\\
6.38855752976135	8\\
6.38855752976135	9\\
6.755284339671	9\\
6.755284339671	10\\
7.03215063355839	10\\
7.03215063355839	11\\
7.11538937003886	11\\
7.11538937003886	12\\
8.37314795956635	12\\
8.37314795956635	13\\
8.50134313482577	13\\
8.50134313482577	14\\
9.50084885446906	14\\
9.50084885446906	15\\
10.3534895060606	15\\
10.3534895060606	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.00497996730149453	0\\
0.00497996730149453	1\\
0.157455933976067	1\\
0.157455933976067	2\\
0.180083154192928	2\\
0.180083154192928	3\\
0.373030968402112	3\\
0.373030968402112	4\\
0.425609216529047	4\\
0.425609216529047	5\\
0.453953180120301	5\\
0.453953180120301	6\\
0.667491296996687	6\\
0.667491296996687	7\\
0.850474317460744	7\\
0.850474317460744	8\\
0.946813480682849	8\\
0.946813480682849	9\\
1.25885161760857	9\\
1.25885161760857	10\\
1.43619995275107	10\\
1.43619995275107	11\\
1.80931070904277	11\\
1.80931070904277	12\\
2.14490998067387	12\\
2.14490998067387	13\\
2.21947182302898	13\\
2.21947182302898	14\\
2.41950134966228	14\\
2.41950134966228	15\\
2.44757214262302	15\\
2.44757214262302	16\\
2.54056083005172	16\\
2.54056083005172	17\\
2.61671801991055	17\\
2.61671801991055	18\\
2.69524490783429	18\\
2.69524490783429	19\\
2.78531494347995	19\\
2.78531494347995	20\\
2.84036863402661	20\\
2.84036863402661	21\\
2.87786257459244	21\\
2.87786257459244	22\\
3.14036199334242	22\\
3.14036199334242	23\\
3.34059940672606	23\\
3.34059940672606	24\\
3.76503468078488	24\\
3.76503468078488	25\\
3.86320666794414	25\\
3.86320666794414	26\\
4.26584564245	26\\
4.26584564245	27\\
4.37646969172843	27\\
4.37646969172843	28\\
4.59775010730721	28\\
4.59775010730721	29\\
4.61344893383954	29\\
4.61344893383954	30\\
4.68443488848526	30\\
4.68443488848526	31\\
4.81007401531647	31\\
4.81007401531647	32\\
5.09474118692504	32\\
5.09474118692504	33\\
6.21979890123535	33\\
6.21979890123535	34\\
7.07795966852949	34\\
7.07795966852949	35\\
9.51094320698083	35\\
9.51094320698083	36\\
10.7894936056746	36\\
10.7894936056746	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.26408364369349	0\\
3.26408364369349	1\\
3.3373225746628	1\\
3.3373225746628	2\\
3.83612108331682	2\\
3.83612108331682	3\\
3.89433515071907	3\\
3.89433515071907	4\\
4.04645436376439	4\\
4.04645436376439	5\\
4.487665282958	5\\
4.487665282958	6\\
4.57159202329381	6\\
4.57159202329381	7\\
5.00053810553859	7\\
5.00053810553859	8\\
5.2637573992552	8\\
5.2637573992552	9\\
5.58080329511407	9\\
5.58080329511407	10\\
5.82080505526079	10\\
5.82080505526079	11\\
5.96459317472194	11\\
5.96459317472194	12\\
5.97045690585944	12\\
5.97045690585944	13\\
9.68776101090717	13\\
9.68776101090717	14\\
9.76378855168567	14\\
9.76378855168567	15\\
10.2714844135497	15\\
10.2714844135497	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.559505935726925	0\\
0.559505935726925	1\\
0.691503096514516	1\\
0.691503096514516	2\\
0.804444141670189	2\\
0.804444141670189	3\\
2.24748836247225	3\\
2.24748836247225	4\\
3.17150154599373	4\\
3.17150154599373	5\\
3.87875237630978	5\\
3.87875237630978	6\\
4.23623127379395	6\\
4.23623127379395	7\\
4.30154828338979	7\\
4.30154828338979	8\\
4.95231059804389	8\\
4.95231059804389	9\\
5.11315114795703	9\\
5.11315114795703	10\\
6.4100007027028	10\\
6.4100007027028	11\\
7.80118043524299	11\\
7.80118043524299	12\\
7.87405260374884	12\\
7.87405260374884	13\\
7.99912642249156	13\\
7.99912642249156	14\\
8.16822673624484	14\\
8.16822673624484	15\\
8.43821085872193	15\\
8.43821085872193	16\\
8.44862103101497	16\\
8.44862103101497	17\\
13.8659622510915	17\\
13.8659622510915	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.042023899312742	0\\
0.042023899312742	1\\
0.252552300067121	1\\
0.252552300067121	2\\
0.511385045905909	2\\
0.511385045905909	3\\
2.4712262282434	3\\
2.4712262282434	4\\
2.69958264714124	4\\
2.69958264714124	5\\
3.3627195412831	5\\
3.3627195412831	6\\
3.49583767877085	6\\
3.49583767877085	7\\
4.56361171754093	7\\
4.56361171754093	8\\
5.74193091950356	8\\
5.74193091950356	9\\
9.46202153948131	9\\
9.46202153948131	10\\
10.6435353870466	10\\
10.6435353870466	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.542837981123309	0\\
0.542837981123309	1\\
0.670161464490057	1\\
0.670161464490057	2\\
1.34811517676293	2\\
1.34811517676293	3\\
1.71312826502223	3\\
1.71312826502223	4\\
2.30503075826202	4\\
2.30503075826202	5\\
2.5276830569545	5\\
2.5276830569545	6\\
2.8914370685785	6\\
2.8914370685785	7\\
3.08861877782944	7\\
3.08861877782944	8\\
3.17399439109445	8\\
3.17399439109445	9\\
5.29777747871456	9\\
5.29777747871456	10\\
9.30811813781175	10\\
9.30811813781175	11\\
9.33525633149366	11\\
9.33525633149366	12\\
11.5870144962514	12\\
11.5870144962514	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.40794636033976	0\\
2.40794636033976	1\\
2.48109491387824	1\\
2.48109491387824	2\\
3.76918369136011	2\\
3.76918369136011	3\\
3.77642887458164	3\\
3.77642887458164	4\\
5.30944643488859	4\\
5.30944643488859	5\\
5.62596592820633	5\\
5.62596592820633	6\\
5.69101441116495	6\\
5.69101441116495	7\\
6.17129727174968	7\\
6.17129727174968	8\\
6.18912729372505	8\\
6.18912729372505	9\\
6.32354583970699	9\\
6.32354583970699	10\\
6.41062552344409	10\\
6.41062552344409	11\\
6.87943704251158	11\\
6.87943704251158	12\\
9.74711166989263	12\\
9.74711166989263	13\\
15.3934356425578	13\\
15.3934356425578	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.243347306902397	0\\
0.243347306902397	1\\
1.85822491116419	1\\
1.85822491116419	2\\
2.32811898203932	2\\
2.32811898203932	3\\
2.33087121102056	4\\
2.66041013286878	4\\
2.66041013286878	5\\
2.72003186414151	5\\
2.72003186414151	6\\
2.74066320167128	6\\
2.74066320167128	7\\
3.36432185576577	7\\
3.36432185576577	8\\
6.20373483256774	8\\
6.20373483256774	9\\
7.23239313219419	9\\
7.23239313219419	10\\
7.57414336121985	10\\
7.57414336121985	11\\
8.27003817785076	11\\
8.27003817785076	12\\
8.65772499396766	12\\
8.65772499396766	13\\
8.80279237091178	13\\
8.80279237091178	14\\
9.2252828763916	14\\
9.2252828763916	15\\
9.72628062322007	15\\
9.72628062322007	16\\
10.1453223306588	16\\
10.1453223306588	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.309402879099199	0\\
0.309402879099199	1\\
0.332780773169901	1\\
0.332780773169901	2\\
0.610133714768537	2\\
0.610133714768537	3\\
1.77992443457538	3\\
1.77992443457538	4\\
2.19528269484848	4\\
2.19528269484848	5\\
2.56841318298002	5\\
2.56841318298002	6\\
2.66512033106055	6\\
2.66512033106055	7\\
2.77979093605583	7\\
2.77979093605583	8\\
2.78640633392664	8\\
2.78640633392664	9\\
2.8492965515975	9\\
2.8492965515975	10\\
2.89004067302578	10\\
2.89004067302578	11\\
2.99003201280873	11\\
2.99003201280873	12\\
3.05655635836167	12\\
3.05655635836167	13\\
3.23979573716159	13\\
3.23979573716159	14\\
4.72042550563641	14\\
4.72042550563641	15\\
5.09599684650708	15\\
5.09599684650708	16\\
5.52760950409442	16\\
5.52760950409442	17\\
6.92879211698937	17\\
6.92879211698937	18\\
7.19935058588753	18\\
7.19935058588753	19\\
7.29938865708996	19\\
7.29938865708996	20\\
8.20732244219992	20\\
8.20732244219992	21\\
8.3178185971983	21\\
8.3178185971983	22\\
8.58861876076183	22\\
8.58861876076183	23\\
8.61151672345972	23\\
8.61151672345972	24\\
9.08450895998281	24\\
9.08450895998281	25\\
10.1324658864529	25\\
10.1324658864529	26\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.238727645452407	0\\
0.238727645452407	1\\
0.899336351452295	1\\
0.899336351452295	2\\
1.21448476936993	2\\
1.21448476936993	3\\
1.232431919906	3\\
1.232431919906	4\\
2.09608680219589	4\\
2.09608680219589	5\\
2.70528393757982	5\\
2.70528393757982	6\\
3.01178000918595	6\\
3.01178000918595	7\\
3.76393831308214	7\\
3.76393831308214	8\\
4.28541762471245	8\\
4.28541762471245	9\\
4.3390632720226	9\\
4.3390632720226	10\\
5.17425384854391	10\\
5.17425384854391	11\\
8.58089991594752	11\\
8.58089991594752	12\\
8.72131171688078	12\\
8.72131171688078	13\\
9.23631221055129	13\\
9.23631221055129	14\\
9.28717511320446	14\\
9.28717511320446	15\\
9.64565894427824	15\\
9.64565894427824	16\\
10.2083880247089	16\\
10.2083880247089	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.221954734460516	0\\
0.221954734460516	1\\
0.332289692579284	1\\
0.332289692579284	2\\
0.79395294729412	2\\
0.79395294729412	3\\
0.923072834330119	3\\
0.923072834330119	4\\
1.06309547214955	4\\
1.06309547214955	5\\
1.28318211600655	5\\
1.28318211600655	6\\
1.38479734297015	6\\
1.38479734297015	7\\
1.90168468460888	7\\
1.90168468460888	8\\
1.99302086231178	8\\
1.99302086231178	9\\
4.59745447219814	9\\
4.59745447219814	10\\
5.46842621701105	10\\
5.46842621701105	11\\
7.79933266545196	11\\
7.79933266545196	12\\
9.89892159290414	12\\
9.89892159290414	13\\
10.0287250366057	13\\
10.0287250366057	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.00908908489284066	0\\
0.00908908489284066	1\\
0.432982235412403	1\\
0.432982235412403	2\\
2.27373692503157	2\\
2.27373692503157	3\\
2.89614525981628	3\\
2.89614525981628	4\\
2.94965565277224	4\\
2.94965565277224	5\\
3.22966722788281	5\\
3.22966722788281	6\\
3.29767588745292	6\\
3.29767588745292	7\\
4.75066601360433	7\\
4.75066601360433	8\\
4.82441932356064	8\\
4.82441932356064	9\\
5.02057433099848	9\\
5.02057433099848	10\\
5.15758711707264	10\\
5.15758711707264	11\\
5.39122016809963	11\\
5.39122016809963	12\\
10.1899591115013	12\\
10.1899591115013	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.15356853676014	0\\
1.15356853676014	1\\
2.80672743360305	1\\
2.80672743360305	2\\
6.10110236722447	2\\
6.10110236722447	3\\
7.18651304739305	3\\
7.18651304739305	4\\
10.7926477025462	4\\
10.7926477025462	5\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0360616676475303	0\\
0.0360616676475303	1\\
0.11165993832887	1\\
0.11165993832887	2\\
0.164136896662143	2\\
0.164136896662143	3\\
0.433640700123178	3\\
0.433640700123178	4\\
0.515749254508471	4\\
0.515749254508471	5\\
1.07594143499251	5\\
1.07594143499251	6\\
1.09865976386208	6\\
1.09865976386208	7\\
1.42100168321315	7\\
1.42100168321315	8\\
1.48252195489215	8\\
1.48252195489215	9\\
1.76575563836852	9\\
1.76575563836852	10\\
1.88504209329928	10\\
1.88504209329928	11\\
1.92445815194792	11\\
1.92445815194792	12\\
2.09733416989485	12\\
2.09733416989485	13\\
2.21514383610336	13\\
2.21514383610336	14\\
2.22884890052546	14\\
2.22884890052546	15\\
2.71739086863657	15\\
2.71739086863657	16\\
4.66558127348142	16\\
4.66558127348142	17\\
4.75867685610814	17\\
4.75867685610814	18\\
4.93151298066648	18\\
4.93151298066648	19\\
4.98999285972753	19\\
4.98999285972753	20\\
5.17748746124607	20\\
5.17748746124607	21\\
5.62381707341203	21\\
5.62381707341203	22\\
5.82706501635539	22\\
5.82706501635539	23\\
5.96417427540974	23\\
5.96417427540974	24\\
6.71049977586296	24\\
6.71049977586296	25\\
7.14270762891729	25\\
7.14270762891729	26\\
7.2864354815876	26\\
7.2864354815876	27\\
7.34855822444135	27\\
7.34855822444135	28\\
7.90978308029077	28\\
7.90978308029077	29\\
8.16283549076098	29\\
8.16283549076098	30\\
8.48528236855923	30\\
8.48528236855923	31\\
8.73453952437367	31\\
8.73453952437367	32\\
9.03198490501754	32\\
9.03198490501754	33\\
11.0318639636842	33\\
11.0318639636842	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.222629121867534	0\\
0.222629121867534	1\\
0.582921611974101	1\\
0.582921611974101	2\\
1.38346982715295	2\\
1.38346982715295	3\\
2.15142836734157	3\\
2.15142836734157	4\\
2.89358395434154	4\\
2.89358395434154	5\\
3.31200467740344	5\\
3.31200467740344	6\\
5.42864805283271	6\\
5.42864805283271	7\\
5.69429356835555	7\\
5.69429356835555	8\\
5.85664295934485	8\\
5.85664295934485	9\\
5.98833748622687	9\\
5.98833748622687	10\\
6.15301937827759	10\\
6.15301937827759	11\\
6.17376633136443	11\\
6.17376633136443	12\\
6.40842488087237	12\\
6.40842488087237	13\\
6.40857607642445	14\\
6.45291936206846	14\\
6.45291936206846	15\\
6.66616647578243	15\\
6.66616647578243	16\\
6.73650367104915	16\\
6.73650367104915	17\\
7.3578072890891	17\\
7.3578072890891	18\\
7.37815635222417	18\\
7.37815635222417	19\\
7.54132868477566	19\\
7.54132868477566	20\\
7.54786236010634	20\\
7.54786236010634	21\\
7.83189249304164	21\\
7.83189249304164	22\\
8.03140032133395	22\\
8.03140032133395	23\\
8.04269475353622	23\\
8.04269475353622	24\\
8.06703877196443	24\\
8.06703877196443	25\\
8.09373050831981	25\\
8.09373050831981	26\\
8.10628785481573	26\\
8.10628785481573	27\\
8.69490348722388	27\\
8.69490348722388	28\\
8.85322318120797	28\\
8.85322318120797	29\\
8.95749712662104	29\\
8.95749712662104	30\\
9.42242548883596	30\\
9.42242548883596	31\\
9.55349053772078	31\\
9.55349053772078	32\\
9.68487640070571	32\\
9.68487640070571	33\\
10.0272583940221	33\\
10.0272583940221	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.04939706235753	0\\
1.04939706235753	1\\
1.44731174883159	1\\
1.44731174883159	2\\
1.64885107530647	2\\
1.64885107530647	3\\
1.65106335356723	4\\
1.67540081329687	4\\
1.67540081329687	5\\
1.83842186519236	5\\
1.83842186519236	6\\
1.97135035778398	6\\
1.97135035778398	7\\
2.11557616001947	7\\
2.11557616001947	8\\
2.21737334600964	8\\
2.21737334600964	9\\
3.27370924883481	9\\
3.27370924883481	10\\
5.32929936031083	10\\
5.32929936031083	11\\
5.84924186627141	11\\
5.84924186627141	12\\
6.37186419573909	12\\
6.37186419573909	13\\
6.39143143479942	13\\
6.39143143479942	14\\
7.00451948666539	14\\
7.00451948666539	15\\
7.04361238749259	15\\
7.04361238749259	16\\
7.86922426049843	16\\
7.86922426049843	17\\
7.91990690524221	17\\
7.91990690524221	18\\
7.93610216790174	18\\
7.93610216790174	19\\
8.031446705843	19\\
8.031446705843	20\\
8.28174240006552	20\\
8.28174240006552	21\\
8.33308863533653	21\\
8.33308863533653	22\\
8.45011859626106	22\\
8.45011859626106	23\\
8.77734059661726	23\\
8.77734059661726	24\\
8.90701901503818	24\\
8.90701901503818	25\\
8.94232966604643	25\\
8.94232966604643	26\\
9.05990486575757	26\\
9.05990486575757	27\\
9.36893008455478	27\\
9.36893008455478	28\\
9.53189278010844	28\\
9.53189278010844	29\\
9.53290910094842	30\\
9.68087132365903	30\\
9.68087132365903	31\\
10.1657561257724	31\\
10.1657561257724	32\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.2761348278451	0\\
1.2761348278451	1\\
1.71705035218863	1\\
1.71705035218863	2\\
2.07862767378539	2\\
2.07862767378539	3\\
2.25895613784548	3\\
2.25895613784548	4\\
2.32147847062355	4\\
2.32147847062355	5\\
4.28288438913908	5\\
4.28288438913908	6\\
4.55975097199889	6\\
4.55975097199889	7\\
5.50487373024603	7\\
5.50487373024603	8\\
5.95540294411692	8\\
5.95540294411692	9\\
6.59822769509174	9\\
6.59822769509174	10\\
6.99999527830223	10\\
6.99999527830223	11\\
7.24494403207127	11\\
7.24494403207127	12\\
7.61986516506195	12\\
7.61986516506195	13\\
8.27851396890059	13\\
8.27851396890059	14\\
8.32975292185854	14\\
8.32975292185854	15\\
8.91675201938987	15\\
8.91675201938987	16\\
9.14034170187083	16\\
9.14034170187083	17\\
9.70725050671855	17\\
9.70725050671855	18\\
9.7761462563047	18\\
9.7761462563047	19\\
10.0107545417492	19\\
10.0107545417492	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0390285366672849	0\\
0.0390285366672849	1\\
0.61783156572606	1\\
0.61783156572606	2\\
0.655559064776256	2\\
0.655559064776256	3\\
0.795251009022515	3\\
0.795251009022515	4\\
0.968609477688258	4\\
0.968609477688258	5\\
1.94493559787531	5\\
1.94493559787531	6\\
2.35195089011742	6\\
2.35195089011742	7\\
2.36234710947402	7\\
2.36234710947402	8\\
5.05235485693807	8\\
5.05235485693807	9\\
5.65127825369205	9\\
5.65127825369205	10\\
6.73175085475233	10\\
6.73175085475233	11\\
6.73934688808202	11\\
6.73934688808202	12\\
6.89906915876067	12\\
6.89906915876067	13\\
6.97086352335347	13\\
6.97086352335347	14\\
7.26595383387918	14\\
7.26595383387918	15\\
8.12455724234804	15\\
8.12455724234804	16\\
9.15383313650598	16\\
9.15383313650598	17\\
9.64437657043124	17\\
9.64437657043124	18\\
10.22196304456	18\\
10.22196304456	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.27549531199503	0\\
0.27549531199503	1\\
0.576645766802685	1\\
0.576645766802685	2\\
0.869401266528698	2\\
0.869401266528698	3\\
2.00997398768509	3\\
2.00997398768509	4\\
2.73115897833218	4\\
2.73115897833218	5\\
3.42637847731388	5\\
3.42637847731388	6\\
4.05716206592557	6\\
4.05716206592557	7\\
4.07300306128057	7\\
4.07300306128057	8\\
4.49432199626182	8\\
4.49432199626182	9\\
4.63974336845077	9\\
4.63974336845077	10\\
4.7862758501274	10\\
4.7862758501274	11\\
4.8382313340666	11\\
4.8382313340666	12\\
5.30502297266199	12\\
5.30502297266199	13\\
5.45178470420306	13\\
5.45178470420306	14\\
5.4633617024577	14\\
5.4633617024577	15\\
5.81966667510977	15\\
5.81966667510977	16\\
5.90542325417894	16\\
5.90542325417894	17\\
5.96021198520241	17\\
5.96021198520241	18\\
6.01075380323478	18\\
6.01075380323478	19\\
6.15585319210226	19\\
6.15585319210226	20\\
6.55431361365085	20\\
6.55431361365085	21\\
7.08706302462672	21\\
7.08706302462672	22\\
7.60738508354481	22\\
7.60738508354481	23\\
7.80728575198584	23\\
7.80728575198584	24\\
8.01228126324732	24\\
8.01228126324732	25\\
8.17549666409747	25\\
8.17549666409747	26\\
8.19530993789754	26\\
8.19530993789754	27\\
8.21437810825184	27\\
8.21437810825184	28\\
8.27648304319657	28\\
8.27648304319657	29\\
8.64061840143468	29\\
8.64061840143468	30\\
8.65396005122733	30\\
8.65396005122733	31\\
8.68565410896741	31\\
8.68565410896741	32\\
9.48863613426094	32\\
9.48863613426094	33\\
9.8105087134284	33\\
9.8105087134284	34\\
10.7358424452994	34\\
10.7358424452994	35\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.19370915822461	0\\
1.19370915822461	1\\
1.39658574795169	1\\
1.39658574795169	2\\
1.40224004201904	2\\
1.40224004201904	3\\
1.82362323150032	3\\
1.82362323150032	4\\
3.02385442469619	4\\
3.02385442469619	5\\
3.03453371827421	5\\
3.03453371827421	6\\
3.03594653178493	7\\
3.15881000908162	7\\
3.15881000908162	8\\
3.29566195806084	8\\
3.29566195806084	9\\
3.43293648326935	9\\
3.43293648326935	10\\
3.48173340234825	10\\
3.48173340234825	11\\
3.93961349988072	11\\
3.93961349988072	12\\
4.34530659760264	12\\
4.34530659760264	13\\
4.4192011348785	13\\
4.4192011348785	14\\
4.68388986310855	14\\
4.68388986310855	15\\
5.11730409047654	15\\
5.11730409047654	16\\
5.42586481017425	16\\
5.42586481017425	17\\
6.05929093754716	17\\
6.05929093754716	18\\
6.30516947965137	18\\
6.30516947965137	19\\
6.93589039581887	19\\
6.93589039581887	20\\
7.63595557120188	20\\
7.63595557120188	21\\
7.81997925952239	21\\
7.81997925952239	22\\
8.22754166323261	22\\
8.22754166323261	23\\
8.23151329501813	23\\
8.23151329501813	24\\
8.7906745795827	24\\
8.7906745795827	25\\
8.85722699912121	25\\
8.85722699912121	26\\
9.35212013613707	26\\
9.35212013613707	27\\
9.38161139692332	27\\
9.38161139692332	28\\
9.66757602941508	28\\
9.66757602941508	29\\
9.86984734174825	29\\
9.86984734174825	30\\
10.2947521693357	30\\
10.2947521693357	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.38211952126406	0\\
1.38211952126406	1\\
1.65852575358657	1\\
1.65852575358657	2\\
2.26132885600107	2\\
2.26132885600107	3\\
2.65231482900235	3\\
2.65231482900235	4\\
3.76962390632821	4\\
3.76962390632821	5\\
5.79751166197116	5\\
5.79751166197116	6\\
7.31248579738226	6\\
7.31248579738226	7\\
7.31631546321552	7\\
7.31631546321552	8\\
7.46533224548504	8\\
7.46533224548504	9\\
9.49407691235326	9\\
9.49407691235326	10\\
11.0047767130864	10\\
11.0047767130864	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.51846915347128	0\\
1.51846915347128	1\\
1.98942288362201	1\\
1.98942288362201	2\\
2.57211606757734	2\\
2.57211606757734	3\\
3.74950047607178	3\\
3.74950047607178	4\\
5.51276722743708	4\\
5.51276722743708	5\\
5.51412064332486	6\\
6.08084161251581	6\\
6.08084161251581	7\\
6.38807761895619	7\\
6.38807761895619	8\\
6.75960255127051	8\\
6.75960255127051	9\\
7.07609528128905	9\\
7.07609528128905	10\\
7.69188529643925	10\\
7.69188529643925	11\\
7.72171221475413	11\\
7.72171221475413	12\\
7.86233871972975	12\\
7.86233871972975	13\\
8.01597540819469	13\\
8.01597540819469	14\\
8.08817129194459	14\\
8.08817129194459	15\\
8.08872780126354	16\\
8.23524078927116	16\\
8.23524078927116	17\\
8.30869603449761	17\\
8.30869603449761	18\\
8.57249252033747	18\\
8.57249252033747	19\\
8.83688901539049	19\\
8.83688901539049	20\\
9.02607717915651	20\\
9.02607717915651	21\\
9.34359687355264	21\\
9.34359687355264	22\\
9.41124249121695	22\\
9.41124249121695	23\\
9.4894425893665	23\\
9.4894425893665	24\\
9.60914713660405	24\\
9.60914713660405	25\\
9.67127096283695	25\\
9.67127096283695	26\\
9.70040074514923	26\\
9.70040074514923	27\\
9.73517835173771	27\\
9.73517835173771	28\\
9.89826640202467	28\\
9.89826640202467	29\\
10.3581963340448	29\\
10.3581963340448	30\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.129204305678213	0\\
0.129204305678213	1\\
2.34208891181064	1\\
2.34208891181064	2\\
2.58965013391185	2\\
2.58965013391185	3\\
5.31405584545128	3\\
5.31405584545128	4\\
5.56407664788476	4\\
5.56407664788476	5\\
6.64267460221668	5\\
6.64267460221668	6\\
7.76257068710275	6\\
7.76257068710275	7\\
7.8358013546461	7\\
7.8358013546461	8\\
8.89157638362843	8\\
8.89157638362843	9\\
8.99277883329633	9\\
8.99277883329633	10\\
9.1613911823378	10\\
9.1613911823378	11\\
11.2021299682763	11\\
11.2021299682763	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.446821716180423	0\\
0.446821716180423	1\\
1.39013461390621	1\\
1.39013461390621	2\\
1.85807530981	2\\
1.85807530981	3\\
2.16271426797994	3\\
2.16271426797994	4\\
3.91953785066129	4\\
3.91953785066129	5\\
5.8042225502736	5\\
5.8042225502736	6\\
5.81732718882729	6\\
5.81732718882729	7\\
8.02080775752888	7\\
8.02080775752888	8\\
10.6257001818862	8\\
10.6257001818862	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.167457863820268	0\\
0.167457863820268	1\\
0.268474789288909	1\\
0.268474789288909	2\\
0.40065271175618	2\\
0.40065271175618	3\\
0.718148579129426	3\\
0.718148579129426	4\\
0.745853597085869	4\\
0.745853597085869	5\\
1.25825104809542	5\\
1.25825104809542	6\\
1.34792354716415	6\\
1.34792354716415	7\\
1.36205385960707	7\\
1.36205385960707	8\\
1.51199043467287	8\\
1.51199043467287	9\\
1.68413549474611	9\\
1.68413549474611	10\\
1.78633368092751	10\\
1.78633368092751	11\\
1.92529943934647	11\\
1.92529943934647	12\\
1.94181448536028	12\\
1.94181448536028	13\\
1.98103758065167	13\\
1.98103758065167	14\\
1.99285486920268	14\\
1.99285486920268	15\\
2.08704878553149	15\\
2.08704878553149	16\\
2.20045212092698	16\\
2.20045212092698	17\\
2.37275579071189	17\\
2.37275579071189	18\\
2.47345886108574	18\\
2.47345886108574	19\\
2.48728552112377	19\\
2.48728552112377	20\\
2.83821741361527	20\\
2.83821741361527	21\\
2.98274892174867	21\\
2.98274892174867	22\\
3.16995344981355	22\\
3.16995344981355	23\\
3.50938890324478	23\\
3.50938890324478	24\\
4.28740040146202	24\\
4.28740040146202	25\\
4.61165115264925	25\\
4.61165115264925	26\\
4.80095781143391	26\\
4.80095781143391	27\\
4.90224141908817	27\\
4.90224141908817	28\\
5.00842262151338	28\\
5.00842262151338	29\\
5.22232187314518	29\\
5.22232187314518	30\\
5.73842723141598	30\\
5.73842723141598	31\\
6.92565934448617	31\\
6.92565934448617	32\\
8.49510251931881	32\\
8.49510251931881	33\\
8.63840357915407	33\\
8.63840357915407	34\\
8.83235742148842	34\\
8.83235742148842	35\\
9.14631042569592	35\\
9.14631042569592	36\\
9.30655723755481	36\\
9.30655723755481	37\\
9.34824192067744	37\\
9.34824192067744	38\\
10.8890188930796	38\\
10.8890188930796	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.45088377908307	0\\
2.45088377908307	1\\
4.65818538561582	1\\
4.65818538561582	2\\
6.8263822073045	2\\
6.8263822073045	3\\
7.05963617585216	3\\
7.05963617585216	4\\
7.34093277295838	4\\
7.34093277295838	5\\
7.39318385023007	5\\
7.39318385023007	6\\
7.40591418262904	6\\
7.40591418262904	7\\
7.55756534756026	7\\
7.55756534756026	8\\
10.9675319816561	8\\
10.9675319816561	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.660280824193052	0\\
0.660280824193052	1\\
0.66655441354844	1\\
0.66655441354844	2\\
0.71812540216559	2\\
0.71812540216559	3\\
0.823320902826929	3\\
0.823320902826929	4\\
0.932520490643093	4\\
0.932520490643093	5\\
1.49675815977968	5\\
1.49675815977968	6\\
1.57297511218766	6\\
1.57297511218766	7\\
1.57403180693782	8\\
1.98170452460914	8\\
1.98170452460914	9\\
2.72855465454682	9\\
2.72855465454682	10\\
2.93740192540128	10\\
2.93740192540128	11\\
3.01306580290807	11\\
3.01306580290807	12\\
3.31042815395078	12\\
3.31042815395078	13\\
3.31475022843002	13\\
3.31475022843002	14\\
3.37928757540514	14\\
3.37928757540514	15\\
3.42186178990851	15\\
3.42186178990851	16\\
3.49159846913254	16\\
3.49159846913254	17\\
3.57195948380275	17\\
3.57195948380275	18\\
3.77300217479493	18\\
3.77300217479493	19\\
4.05956925562259	19\\
4.05956925562259	20\\
4.15964551681289	20\\
4.15964551681289	21\\
4.37968950999536	21\\
4.37968950999536	22\\
4.63656609604709	22\\
4.63656609604709	23\\
5.12592648887791	23\\
5.12592648887791	24\\
5.44737681436705	24\\
5.44737681436705	25\\
6.13696247328716	25\\
6.13696247328716	26\\
6.4863016147315	26\\
6.4863016147315	27\\
6.54804357012495	27\\
6.54804357012495	28\\
6.843963517172	28\\
6.843963517172	29\\
6.93331599956644	29\\
6.93331599956644	30\\
6.96762579564646	30\\
6.96762579564646	31\\
7.02497813525388	31\\
7.02497813525388	32\\
7.15681327452113	32\\
7.15681327452113	33\\
7.16046855403469	33\\
7.16046855403469	34\\
7.21806020555695	34\\
7.21806020555695	35\\
7.42784928769473	35\\
7.42784928769473	36\\
7.43312484671237	36\\
7.43312484671237	37\\
7.50042314082468	37\\
7.50042314082468	38\\
7.50245792685201	39\\
7.55589491425941	39\\
7.55589491425941	40\\
7.59408429839107	40\\
7.59408429839107	41\\
7.60328453795784	41\\
7.60328453795784	42\\
7.86113132294984	42\\
7.86113132294984	43\\
7.9340712202203	43\\
7.9340712202203	44\\
10.589512954776	44\\
10.589512954776	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0571746206038473	0\\
0.0571746206038473	1\\
0.665375083575634	1\\
0.665375083575634	2\\
0.711770320744755	2\\
0.711770320744755	3\\
4.14870055650536	3\\
4.14870055650536	4\\
4.70671724793928	4\\
4.70671724793928	5\\
5.17522781136987	5\\
5.17522781136987	6\\
5.26890782449193	6\\
5.26890782449193	7\\
8.18424033015532	7\\
8.18424033015532	8\\
9.48866637689712	8\\
9.48866637689712	9\\
10.2010084302616	9\\
10.2010084302616	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.11827997678255	0\\
1.11827997678255	1\\
1.15387553971896	1\\
1.15387553971896	2\\
1.35242477173806	2\\
1.35242477173806	3\\
1.81756278941881	3\\
1.81756278941881	4\\
1.82824034259044	4\\
1.82824034259044	5\\
1.86045900204996	5\\
1.86045900204996	6\\
2.09495415353673	6\\
2.09495415353673	7\\
3.55802136450716	7\\
3.55802136450716	8\\
4.14462815838619	8\\
4.14462815838619	9\\
4.32082278890916	9\\
4.32082278890916	10\\
5.36363309482111	10\\
5.36363309482111	11\\
6.23844083463264	11\\
6.23844083463264	12\\
7.43033227140674	12\\
7.43033227140674	13\\
8.90100942317546	13\\
8.90100942317546	14\\
12.0725494887183	14\\
12.0725494887183	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.263812821829234	0\\
0.263812821829234	1\\
1.35881094583892	1\\
1.35881094583892	2\\
3.16713972391137	2\\
3.16713972391137	3\\
3.20014465889135	3\\
3.20014465889135	4\\
4.85345893567269	4\\
4.85345893567269	5\\
5.26460577599336	5\\
5.26460577599336	6\\
6.14119432941241	6\\
6.14119432941241	7\\
6.29365956468889	7\\
6.29365956468889	8\\
6.34214401726442	8\\
6.34214401726442	9\\
6.76353492998127	9\\
6.76353492998127	10\\
6.80188525018552	10\\
6.80188525018552	11\\
6.99665955806821	11\\
6.99665955806821	12\\
8.14989532745123	12\\
8.14989532745123	13\\
8.28392719438916	13\\
8.28392719438916	14\\
8.37761682052532	14\\
8.37761682052532	15\\
8.68071246477142	15\\
8.68071246477142	16\\
8.82755154695055	16\\
8.82755154695055	17\\
8.89043113516222	17\\
8.89043113516222	18\\
8.99922909010888	18\\
8.99922909010888	19\\
9.20782014088337	19\\
9.20782014088337	20\\
9.24439964447035	20\\
9.24439964447035	21\\
11.5758986247816	21\\
11.5758986247816	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.08239747267513	0\\
1.08239747267513	1\\
2.43072506075288	1\\
2.43072506075288	2\\
4.28262570166427	2\\
4.28262570166427	3\\
5.44074850994788	3\\
5.44074850994788	4\\
6.22544375440843	4\\
6.22544375440843	5\\
6.5406901983513	5\\
6.5406901983513	6\\
8.13797556852394	6\\
8.13797556852394	7\\
8.38849593375199	7\\
8.38849593375199	8\\
8.64874605050856	8\\
8.64874605050856	9\\
9.12772471791734	9\\
9.12772471791734	10\\
9.26223879208475	10\\
9.26223879208475	11\\
9.37731981400794	11\\
9.37731981400794	12\\
9.45048013708603	12\\
9.45048013708603	13\\
9.54805141515689	13\\
9.54805141515689	14\\
9.70402053256116	14\\
9.70402053256116	15\\
10.3547625991521	15\\
10.3547625991521	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.192195066242125	0\\
0.192195066242125	1\\
0.504703992136037	1\\
0.504703992136037	2\\
0.680264778821762	2\\
0.680264778821762	3\\
1.06626987620236	3\\
1.06626987620236	4\\
1.08279559987896	4\\
1.08279559987896	5\\
1.25244445971921	5\\
1.25244445971921	6\\
1.61096782442999	6\\
1.61096782442999	7\\
1.78996646058514	7\\
1.78996646058514	8\\
1.79470536504779	8\\
1.79470536504779	9\\
2.05529604318805	9\\
2.05529604318805	10\\
2.3164884119767	10\\
2.3164884119767	11\\
2.98204902409957	11\\
2.98204902409957	12\\
4.35158924988392	12\\
4.35158924988392	13\\
4.57245443387201	13\\
4.57245443387201	14\\
4.99852191751289	14\\
4.99852191751289	15\\
5.05209783361707	15\\
5.05209783361707	16\\
5.25465335549381	16\\
5.25465335549381	17\\
5.34511708663987	17\\
5.34511708663987	18\\
5.49472235396394	18\\
5.49472235396394	19\\
5.56364218655594	19\\
5.56364218655594	20\\
5.93877062082031	20\\
5.93877062082031	21\\
6.49455433664195	21\\
6.49455433664195	22\\
6.55824072213082	22\\
6.55824072213082	23\\
6.77802388978368	23\\
6.77802388978368	24\\
7.66049665440509	24\\
7.66049665440509	25\\
7.89431202479909	25\\
7.89431202479909	26\\
8.06549351425659	26\\
8.06549351425659	27\\
8.26686912055472	27\\
8.26686912055472	28\\
8.41871332006368	28\\
8.41871332006368	29\\
9.17558956549975	29\\
9.17558956549975	30\\
10.1570934396891	30\\
10.1570934396891	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.267771000318106	0\\
0.267771000318106	1\\
0.6870716682688	1\\
0.6870716682688	2\\
0.874902471070534	2\\
0.874902471070534	3\\
1.13677533990991	3\\
1.13677533990991	4\\
1.20996984108691	4\\
1.20996984108691	5\\
1.22462019109422	5\\
1.22462019109422	6\\
1.2526037469281	6\\
1.2526037469281	7\\
1.37197424098691	7\\
1.37197424098691	8\\
1.40761351793646	8\\
1.40761351793646	9\\
1.79642167361282	9\\
1.79642167361282	10\\
2.1067756199098	10\\
2.1067756199098	11\\
2.14278828889597	11\\
2.14278828889597	12\\
2.31026483834518	12\\
2.31026483834518	13\\
2.33265003826862	13\\
2.33265003826862	14\\
2.51226179298527	14\\
2.51226179298527	15\\
2.62427078192959	15\\
2.62427078192959	16\\
2.85871157986339	16\\
2.85871157986339	17\\
3.2654278824552	17\\
3.2654278824552	18\\
3.69741738838714	18\\
3.69741738838714	19\\
3.84368546578546	19\\
3.84368546578546	20\\
3.941371092834	20\\
3.941371092834	21\\
3.94245014196581	22\\
4.10029585678372	22\\
4.10029585678372	23\\
4.14522491410209	23\\
4.14522491410209	24\\
4.21372965832202	24\\
4.21372965832202	25\\
4.41661560576041	25\\
4.41661560576041	26\\
4.75121001250083	26\\
4.75121001250083	27\\
5.05058471310955	27\\
5.05058471310955	28\\
5.11333959755316	28\\
5.11333959755316	29\\
5.41620699716832	29\\
5.41620699716832	30\\
5.86172109548463	30\\
5.86172109548463	31\\
6.60847346207822	31\\
6.60847346207822	32\\
7.96336976182315	32\\
7.96336976182315	33\\
8.11413949247569	33\\
8.11413949247569	34\\
8.413502669189	34\\
8.413502669189	35\\
9.48380232314006	35\\
9.48380232314006	36\\
9.59807611462381	36\\
9.59807611462381	37\\
9.82814899148341	37\\
9.82814899148341	38\\
9.97790018353545	38\\
9.97790018353545	39\\
10.7038594136508	39\\
10.7038594136508	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0363499955150743	0\\
0.0363499955150743	1\\
0.0584146149908769	1\\
0.0584146149908769	2\\
0.249433809084476	2\\
0.249433809084476	3\\
0.514841721151722	3\\
0.514841721151722	4\\
0.53431309625006	4\\
0.53431309625006	5\\
1.58165484172749	5\\
1.58165484172749	6\\
1.6282867956628	6\\
1.6282867956628	7\\
1.87404981270168	7\\
1.87404981270168	8\\
2.00195823255591	8\\
2.00195823255591	9\\
2.0250043457796	9\\
2.0250043457796	10\\
2.22702007614979	10\\
2.22702007614979	11\\
3.20273094103521	11\\
3.20273094103521	12\\
5.82247390467294	12\\
5.82247390467294	13\\
5.92066156771469	13\\
5.92066156771469	14\\
6.28908709834141	14\\
6.28908709834141	15\\
10.7201936272166	15\\
10.7201936272166	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.80948217474553	0\\
1.80948217474553	1\\
1.83078501893327	1\\
1.83078501893327	2\\
2.30889190421615	2\\
2.30889190421615	3\\
2.36431378672417	3\\
2.36431378672417	4\\
3.38809339381477	4\\
3.38809339381477	5\\
3.38929570165959	6\\
3.97782558677858	6\\
3.97782558677858	7\\
4.12073734787966	7\\
4.12073734787966	8\\
4.30699818623303	8\\
4.30699818623303	9\\
4.42151667018672	9\\
4.42151667018672	10\\
4.51857805178877	10\\
4.51857805178877	11\\
4.62010101696506	11\\
4.62010101696506	12\\
6.02898585917592	12\\
6.02898585917592	13\\
6.83804826945965	13\\
6.83804826945965	14\\
8.51418583449879	14\\
8.51418583449879	15\\
8.57669032285893	15\\
8.57669032285893	16\\
9.06059783139334	16\\
9.06059783139334	17\\
9.23211985954878	17\\
9.23211985954878	18\\
9.48029035924417	18\\
9.48029035924417	19\\
11.0064381902609	19\\
11.0064381902609	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.512943435366561	0\\
0.512943435366561	1\\
0.851415441406196	1\\
0.851415441406196	2\\
0.900933435979786	2\\
0.900933435979786	3\\
1.51444089719177	3\\
1.51444089719177	4\\
1.7710071181537	4\\
1.7710071181537	5\\
2.95124282042734	5\\
2.95124282042734	6\\
3.19658775585578	6\\
3.19658775585578	7\\
3.48925423694032	7\\
3.48925423694032	8\\
3.53570672822476	8\\
3.53570672822476	9\\
3.63499013144424	9\\
3.63499013144424	10\\
4.13516836523145	10\\
4.13516836523145	11\\
4.71299267614418	11\\
4.71299267614418	12\\
8.8862380331331	12\\
8.8862380331331	13\\
10.3931072734913	13\\
10.3931072734913	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0504576805115544	0\\
0.0504576805115544	1\\
2.50930669705121	1\\
2.50930669705121	2\\
3.80528652044235	2\\
3.80528652044235	3\\
3.80595703323548	4\\
3.98039216667074	4\\
3.98039216667074	5\\
5.72442220134922	5\\
5.72442220134922	6\\
8.97689355652479	6\\
8.97689355652479	7\\
9.3924729118457	7\\
9.3924729118457	8\\
9.40395815846619	8\\
9.40395815846619	9\\
9.60841449104421	9\\
9.60841449104421	10\\
9.61273602019708	10\\
9.61273602019708	11\\
9.61445206975674	12\\
9.84699069841968	12\\
9.84699069841968	13\\
9.90480309011331	13\\
9.90480309011331	14\\
10.3268845462989	14\\
10.3268845462989	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.16238180844779	0\\
0.16238180844779	1\\
0.168591542674317	1\\
0.168591542674317	2\\
1.87420800955669	2\\
1.87420800955669	3\\
2.27291624524585	3\\
2.27291624524585	4\\
2.48277628237541	4\\
2.48277628237541	5\\
2.65237156438312	5\\
2.65237156438312	6\\
4.05790106526501	6\\
4.05790106526501	7\\
4.31062834718725	7\\
4.31062834718725	8\\
4.69978131950846	8\\
4.69978131950846	9\\
4.8011529329216	9\\
4.8011529329216	10\\
4.82189290338697	10\\
4.82189290338697	11\\
4.8514689198391	11\\
4.8514689198391	12\\
4.9795783114029	12\\
4.9795783114029	13\\
5.23543602133795	13\\
5.23543602133795	14\\
5.91911954857361	14\\
5.91911954857361	15\\
5.94466977058284	15\\
5.94466977058284	16\\
7.41391244436149	16\\
7.41391244436149	17\\
7.62695719279091	17\\
7.62695719279091	18\\
7.68185823276028	18\\
7.68185823276028	19\\
7.80558365368139	19\\
7.80558365368139	20\\
7.84023902229451	20\\
7.84023902229451	21\\
8.73334662097089	21\\
8.73334662097089	22\\
8.80380796811533	22\\
8.80380796811533	23\\
9.12187583847632	23\\
9.12187583847632	24\\
9.34170548915984	24\\
9.34170548915984	25\\
11.9019830504223	25\\
11.9019830504223	26\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.428690797665833	0\\
0.428690797665833	1\\
0.544610750967887	1\\
0.544610750967887	2\\
0.944989617270849	2\\
0.944989617270849	3\\
6.04167662945995	3\\
6.04167662945995	4\\
6.30578846917474	4\\
6.30578846917474	5\\
6.9019112698906	5\\
6.9019112698906	6\\
7.13211778279154	6\\
7.13211778279154	7\\
7.43840129841865	7\\
7.43840129841865	8\\
7.57881952735397	8\\
7.57881952735397	9\\
7.90421064586894	9\\
7.90421064586894	10\\
8.03592028746434	10\\
8.03592028746434	11\\
8.58086826341407	11\\
8.58086826341407	12\\
8.77595514091102	12\\
8.77595514091102	13\\
8.87913479256259	13\\
8.87913479256259	14\\
8.9100567170683	14\\
8.9100567170683	15\\
9.34297887044028	15\\
9.34297887044028	16\\
9.39458268657242	16\\
9.39458268657242	17\\
9.57310432123628	17\\
9.57310432123628	18\\
9.57776032471089	18\\
9.57776032471089	19\\
9.78240315469186	19\\
9.78240315469186	20\\
10.2948120169506	20\\
10.2948120169506	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0764784478304037	0\\
0.0764784478304037	1\\
0.815304406238695	1\\
0.815304406238695	2\\
1.09478581255396	2\\
1.09478581255396	3\\
3.33676283817723	3\\
3.33676283817723	4\\
3.72733463552741	4\\
3.72733463552741	5\\
3.98893816127584	5\\
3.98893816127584	6\\
5.25705095040942	6\\
5.25705095040942	7\\
5.65864507725259	7\\
5.65864507725259	8\\
5.67611126719404	8\\
5.67611126719404	9\\
6.0647542333892	9\\
6.0647542333892	10\\
6.30926785039777	10\\
6.30926785039777	11\\
6.32381807064815	11\\
6.32381807064815	12\\
6.34551555982525	12\\
6.34551555982525	13\\
7.50041662181275	13\\
7.50041662181275	14\\
8.16870773575209	14\\
8.16870773575209	15\\
8.46345142112484	15\\
8.46345142112484	16\\
8.97981871264616	16\\
8.97981871264616	17\\
9.0704164134839	17\\
9.0704164134839	18\\
9.15471033345331	18\\
9.15471033345331	19\\
9.29798366053185	19\\
9.29798366053185	20\\
9.45003758189328	20\\
9.45003758189328	21\\
9.50664226907255	21\\
9.50664226907255	22\\
9.52827555392602	22\\
9.52827555392602	23\\
9.56535280266521	23\\
9.56535280266521	24\\
9.58415423292988	24\\
9.58415423292988	25\\
9.6836871682385	25\\
9.6836871682385	26\\
10.1672612324568	26\\
10.1672612324568	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.129495332541898	0\\
0.129495332541898	1\\
0.203138452539573	1\\
0.203138452539573	2\\
0.479565861252309	2\\
0.479565861252309	3\\
3.11590362149817	3\\
3.11590362149817	4\\
4.66694972727981	4\\
4.66694972727981	5\\
5.45908761337822	5\\
5.45908761337822	6\\
5.51284401146855	6\\
5.51284401146855	7\\
5.57026880833995	7\\
5.57026880833995	8\\
9.43900476741694	8\\
9.43900476741694	9\\
10.8277040688717	9\\
10.8277040688717	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.363463705151915	0\\
0.363463705151915	1\\
0.767763124827312	1\\
0.767763124827312	2\\
0.877999183524942	2\\
0.877999183524942	3\\
0.912722297975733	3\\
0.912722297975733	4\\
1.24997926920444	4\\
1.24997926920444	5\\
1.61318751781061	5\\
1.61318751781061	6\\
1.90236510085469	6\\
1.90236510085469	7\\
1.96574652994392	7\\
1.96574652994392	8\\
2.41121459954573	8\\
2.41121459954573	9\\
2.66258218499581	9\\
2.66258218499581	10\\
3.12038551978475	10\\
3.12038551978475	11\\
3.25114055516009	11\\
3.25114055516009	12\\
3.87086718832111	12\\
3.87086718832111	13\\
4.9432167552154	13\\
4.9432167552154	14\\
5.07994623065498	14\\
5.07994623065498	15\\
5.14977485304566	15\\
5.14977485304566	16\\
5.56996047805659	16\\
5.56996047805659	17\\
5.8121878600232	17\\
5.8121878600232	18\\
6.0916879985772	18\\
6.0916879985772	19\\
6.44404669592306	19\\
6.44404669592306	20\\
6.71740397834728	20\\
6.71740397834728	21\\
6.78483197747243	21\\
6.78483197747243	22\\
6.96430554976218	22\\
6.96430554976218	23\\
7.1974930671913	23\\
7.1974930671913	24\\
7.52090171525452	24\\
7.52090171525452	25\\
7.52603444320268	25\\
7.52603444320268	26\\
7.67738663915686	26\\
7.67738663915686	27\\
7.75308395260119	27\\
7.75308395260119	28\\
7.95495598978759	28\\
7.95495598978759	29\\
8.36004610395347	29\\
8.36004610395347	30\\
8.93077936267247	30\\
8.93077936267247	31\\
8.94010442385444	31\\
8.94010442385444	32\\
8.97071930995804	32\\
8.97071930995804	33\\
9.00136743850322	33\\
9.00136743850322	34\\
9.12875874397579	34\\
9.12875874397579	35\\
9.18341148785802	35\\
9.18341148785802	36\\
9.28741238190646	36\\
9.28741238190646	37\\
9.31448585607404	37\\
9.31448585607404	38\\
9.49450803729341	38\\
9.49450803729341	39\\
9.53609693399203	39\\
9.53609693399203	40\\
9.83124663332963	40\\
9.83124663332963	41\\
9.95204231950682	41\\
9.95204231950682	42\\
11.0326416327438	42\\
11.0326416327438	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.64296846817211	0\\
1.64296846817211	1\\
2.93518500953621	1\\
2.93518500953621	2\\
3.35636251727419	2\\
3.35636251727419	3\\
3.40043831142822	3\\
3.40043831142822	4\\
3.43871420344038	4\\
3.43871420344038	5\\
3.62163697902069	5\\
3.62163697902069	6\\
3.66351066239929	6\\
3.66351066239929	7\\
3.80961099641067	7\\
3.80961099641067	8\\
4.46693884148329	8\\
4.46693884148329	9\\
5.41452838654362	9\\
5.41452838654362	10\\
5.44578656676664	10\\
5.44578656676664	11\\
6.84433224427159	11\\
6.84433224427159	12\\
7.45243829492406	12\\
7.45243829492406	13\\
7.45543240729041	14\\
8.19610741626443	14\\
8.19610741626443	15\\
10.8537297087562	15\\
10.8537297087562	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.38997747562273	0\\
1.38997747562273	1\\
1.55020048029113	1\\
1.55020048029113	2\\
1.58833849707224	2\\
1.58833849707224	3\\
2.20374522946535	3\\
2.20374522946535	4\\
2.58503495101812	4\\
2.58503495101812	5\\
2.59013772344527	5\\
2.59013772344527	6\\
2.77034679592779	6\\
2.77034679592779	7\\
3.35322362591663	7\\
3.35322362591663	8\\
3.40971694959571	8\\
3.40971694959571	9\\
3.61175201901818	9\\
3.61175201901818	10\\
4.38079995959989	10\\
4.38079995959989	11\\
4.74778837346629	11\\
4.74778837346629	12\\
5.31619497225821	12\\
5.31619497225821	13\\
5.63838928312441	13\\
5.63838928312441	14\\
5.83837081798914	14\\
5.83837081798914	15\\
6.16594498336504	15\\
6.16594498336504	16\\
6.19811683076099	16\\
6.19811683076099	17\\
6.50993965055379	17\\
6.50993965055379	18\\
7.18792976667282	18\\
7.18792976667282	19\\
7.2146439947761	19\\
7.2146439947761	20\\
7.93160330703159	20\\
7.93160330703159	21\\
8.07604676590638	21\\
8.07604676590638	22\\
8.3171461919281	22\\
8.3171461919281	23\\
8.32554647816271	23\\
8.32554647816271	24\\
8.41182957030143	24\\
8.41182957030143	25\\
8.91384762047595	25\\
8.91384762047595	26\\
9.10055434246235	26\\
9.10055434246235	27\\
9.20054579883784	27\\
9.20054579883784	28\\
9.3024253111206	28\\
9.3024253111206	29\\
9.86358691196525	29\\
9.86358691196525	30\\
9.96782008788326	30\\
9.96782008788326	31\\
10.3632072011509	31\\
10.3632072011509	32\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.261963939185559	0\\
0.261963939185559	1\\
0.969948542623191	1\\
0.969948542623191	2\\
1.03318857567759	2\\
1.03318857567759	3\\
3.13286203883	3\\
3.13286203883	4\\
3.28316679848644	4\\
3.28316679848644	5\\
3.72958530585524	5\\
3.72958530585524	6\\
6.05978042605409	6\\
6.05978042605409	7\\
7.33299924792601	7\\
7.33299924792601	8\\
7.58532227851125	8\\
7.58532227851125	9\\
7.84661953325707	9\\
7.84661953325707	10\\
8.10246762000572	10\\
8.10246762000572	11\\
8.56989677502673	11\\
8.56989677502673	12\\
8.66358254159951	12\\
8.66358254159951	13\\
8.94960863333852	13\\
8.94960863333852	14\\
10.7469695623949	14\\
10.7469695623949	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.706160086189332	0\\
0.706160086189332	1\\
0.854687497790465	1\\
0.854687497790465	2\\
1.57125568793141	2\\
1.57125568793141	3\\
1.73861625761369	3\\
1.73861625761369	4\\
2.00584259499156	4\\
2.00584259499156	5\\
2.15670754700154	5\\
2.15670754700154	6\\
2.804829619682	6\\
2.804829619682	7\\
2.88885831036592	7\\
2.88885831036592	8\\
4.08804866858052	8\\
4.08804866858052	9\\
5.2396755642039	9\\
5.2396755642039	10\\
6.3328822087069	10\\
6.3328822087069	11\\
6.81342800723975	11\\
6.81342800723975	12\\
6.86264671207363	12\\
6.86264671207363	13\\
9.54222888655578	13\\
9.54222888655578	14\\
9.80435715688543	14\\
9.80435715688543	15\\
11.5997285119939	15\\
11.5997285119939	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.322153722221721	0\\
0.322153722221721	1\\
0.773248904686678	1\\
0.773248904686678	2\\
1.61432635160453	2\\
1.61432635160453	3\\
2.88531331942173	3\\
2.88531331942173	4\\
3.58722444865157	4\\
3.58722444865157	5\\
3.80749717640877	5\\
3.80749717640877	6\\
3.88304778537605	6\\
3.88304778537605	7\\
4.17156264195924	7\\
4.17156264195924	8\\
4.26434243618156	8\\
4.26434243618156	9\\
4.38083733271567	9\\
4.38083733271567	10\\
5.27359148398592	10\\
5.27359148398592	11\\
5.5426250631017	11\\
5.5426250631017	12\\
5.61800376558803	12\\
5.61800376558803	13\\
5.70891749478123	13\\
5.70891749478123	14\\
6.03371415466478	14\\
6.03371415466478	15\\
6.37722580333348	15\\
6.37722580333348	16\\
7.53089784489871	16\\
7.53089784489871	17\\
7.538954881755	17\\
7.538954881755	18\\
7.67913804443819	18\\
7.67913804443819	19\\
7.71138970989048	19\\
7.71138970989048	20\\
8.60679991889155	20\\
8.60679991889155	21\\
8.6484858538109	21\\
8.6484858538109	22\\
8.69036694039922	22\\
8.69036694039922	23\\
8.97748014527988	23\\
8.97748014527988	24\\
8.99331205624579	24\\
8.99331205624579	25\\
9.7944218382778	25\\
9.7944218382778	26\\
11.1554861114292	26\\
11.1554861114292	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.55798615446812	0\\
3.55798615446812	1\\
5.96082689443795	1\\
5.96082689443795	2\\
8.94165952008568	2\\
8.94165952008568	3\\
9.06960898318492	3\\
9.06960898318492	4\\
9.40511810726739	4\\
9.40511810726739	5\\
9.87949755403794	5\\
9.87949755403794	6\\
9.94727723855617	6\\
9.94727723855617	7\\
10.1315781235707	7\\
10.1315781235707	8\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.517751902871447	0\\
0.517751902871447	1\\
0.631778989069357	1\\
0.631778989069357	2\\
1.15159017492516	2\\
1.15159017492516	3\\
1.23639005065534	3\\
1.23639005065534	4\\
1.28727272930661	4\\
1.28727272930661	5\\
1.36482601708267	5\\
1.36482601708267	6\\
2.64602794808867	6\\
2.64602794808867	7\\
2.86991634770072	7\\
2.86991634770072	8\\
5.98452783333168	8\\
5.98452783333168	9\\
7.53805012651125	9\\
7.53805012651125	10\\
7.76561218564524	10\\
7.76561218564524	11\\
7.9587960958735	11\\
7.9587960958735	12\\
7.97134723522963	12\\
7.97134723522963	13\\
10.4999600852621	13\\
10.4999600852621	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.670880428394529	0\\
0.670880428394529	1\\
1.32344440588681	1\\
1.32344440588681	2\\
1.54914624348024	2\\
1.54914624348024	3\\
2.57712441736165	3\\
2.57712441736165	4\\
2.84047829498572	4\\
2.84047829498572	5\\
2.89954790069434	5\\
2.89954790069434	6\\
2.93805475601831	6\\
2.93805475601831	7\\
3.30312080788584	7\\
3.30312080788584	8\\
4.00661488915821	8\\
4.00661488915821	9\\
5.38942234894871	9\\
5.38942234894871	10\\
5.59200072645722	10\\
5.59200072645722	11\\
5.62566190628443	11\\
5.62566190628443	12\\
5.64136356153666	12\\
5.64136356153666	13\\
9.66172845019535	13\\
9.66172845019535	14\\
12.5444860104328	14\\
12.5444860104328	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.651065050128871	0\\
0.651065050128871	1\\
1.3385265149653	1\\
1.3385265149653	2\\
1.72406322344652	2\\
1.72406322344652	3\\
2.00276429105475	3\\
2.00276429105475	4\\
2.2329408468189	4\\
2.2329408468189	5\\
2.27369773435384	5\\
2.27369773435384	6\\
2.51027102057376	6\\
2.51027102057376	7\\
2.58250146997599	7\\
2.58250146997599	8\\
2.87201191182728	8\\
2.87201191182728	9\\
3.22724940297648	9\\
3.22724940297648	10\\
3.3218643404472	10\\
3.3218643404472	11\\
3.87760976912474	11\\
3.87760976912474	12\\
3.99545715226722	12\\
3.99545715226722	13\\
4.30495560523989	13\\
4.30495560523989	14\\
5.0365198870488	14\\
5.0365198870488	15\\
5.29765450833246	15\\
5.29765450833246	16\\
5.82393343178271	16\\
5.82393343178271	17\\
6.62354444737289	17\\
6.62354444737289	18\\
6.66185898347329	18\\
6.66185898347329	19\\
7.10437710109535	19\\
7.10437710109535	20\\
7.23397349099431	20\\
7.23397349099431	21\\
8.42946409269999	21\\
8.42946409269999	22\\
10.9519851640284	22\\
10.9519851640284	23\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.203268965700659	0\\
0.203268965700659	1\\
0.477320617453032	1\\
0.477320617453032	2\\
0.494447698404024	2\\
0.494447698404024	3\\
0.54395980085318	3\\
0.54395980085318	4\\
0.822328617337867	4\\
0.822328617337867	5\\
1.0026002666113	5\\
1.0026002666113	6\\
1.01797949728433	6\\
1.01797949728433	7\\
1.03344291602487	7\\
1.03344291602487	8\\
1.08634380553299	8\\
1.08634380553299	9\\
1.11628854495826	9\\
1.11628854495826	10\\
1.49574509076182	10\\
1.49574509076182	11\\
1.59909529349227	11\\
1.59909529349227	12\\
1.84488485301386	12\\
1.84488485301386	13\\
1.88564902379045	13\\
1.88564902379045	14\\
2.02970261959792	14\\
2.02970261959792	15\\
2.03380502934154	15\\
2.03380502934154	16\\
2.12045871031611	16\\
2.12045871031611	17\\
2.21919537228516	17\\
2.21919537228516	18\\
2.25048486572199	18\\
2.25048486572199	19\\
2.55150247639879	19\\
2.55150247639879	20\\
2.73331820236962	20\\
2.73331820236962	21\\
2.77555440173589	21\\
2.77555440173589	22\\
3.06093328719032	22\\
3.06093328719032	23\\
3.3355646862957	23\\
3.3355646862957	24\\
3.33627369171167	25\\
3.34779071301524	25\\
3.34779071301524	26\\
3.42820602581936	26\\
3.42820602581936	27\\
3.44527947383122	27\\
3.44527947383122	28\\
3.51517493496105	28\\
3.51517493496105	29\\
3.71290049255292	29\\
3.71290049255292	30\\
4.11461839137871	30\\
4.11461839137871	31\\
4.20123854562016	31\\
4.20123854562016	32\\
4.26695580606827	32\\
4.26695580606827	33\\
4.86600100683741	33\\
4.86600100683741	34\\
5.35651152571887	34\\
5.35651152571887	35\\
5.85714263731354	35\\
5.85714263731354	36\\
6.50145633813218	36\\
6.50145633813218	37\\
6.81401291497968	37\\
6.81401291497968	38\\
7.21063585846057	38\\
7.21063585846057	39\\
7.90311765085063	39\\
7.90311765085063	40\\
8.13088168381613	40\\
8.13088168381613	41\\
8.26987538162497	41\\
8.26987538162497	42\\
8.5282875054928	42\\
8.5282875054928	43\\
8.68868782078068	43\\
8.68868782078068	44\\
8.82942965511143	44\\
8.82942965511143	45\\
9.11251713736738	45\\
9.11251713736738	46\\
9.40974889378224	46\\
9.40974889378224	47\\
9.59233916603838	47\\
9.59233916603838	48\\
10.0478578820847	48\\
10.0478578820847	49\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.95660263663915	0\\
1.95660263663915	1\\
3.703808032608	1\\
3.703808032608	2\\
3.82491016383392	2\\
3.82491016383392	3\\
4.56257074478924	3\\
4.56257074478924	4\\
7.34995574188079	4\\
7.34995574188079	5\\
7.4532695211995	5\\
7.4532695211995	6\\
7.49172433977675	6\\
7.49172433977675	7\\
7.91469331623888	7\\
7.91469331623888	8\\
9.49494130275249	8\\
9.49494130275249	9\\
13.8727099970351	9\\
13.8727099970351	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.225729462492847	0\\
0.225729462492847	1\\
0.349457433651299	1\\
0.349457433651299	2\\
0.601303370678984	2\\
0.601303370678984	3\\
0.625968250392077	3\\
0.625968250392077	4\\
1.42806669674275	4\\
1.42806669674275	5\\
1.67627681042499	5\\
1.67627681042499	6\\
1.80682047029735	6\\
1.80682047029735	7\\
4.38177800878419	7\\
4.38177800878419	8\\
4.63506271982198	8\\
4.63506271982198	9\\
4.64048010683615	9\\
4.64048010683615	10\\
4.71173386804567	10\\
4.71173386804567	11\\
5.84285752165825	11\\
5.84285752165825	12\\
5.92416762250058	12\\
5.92416762250058	13\\
6.47384736083566	13\\
6.47384736083566	14\\
7.1686514661604	14\\
7.1686514661604	15\\
8.32695315284241	15\\
8.32695315284241	16\\
8.43694751458208	16\\
8.43694751458208	17\\
8.48754766647204	17\\
8.48754766647204	18\\
8.81781152243142	18\\
8.81781152243142	19\\
9.22304229880112	19\\
9.22304229880112	20\\
9.4921133591908	20\\
9.4921133591908	21\\
11.3976801187903	21\\
11.3976801187903	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.285133006594936	0\\
0.285133006594936	1\\
0.37392025750362	1\\
0.37392025750362	2\\
0.599880441242572	2\\
0.599880441242572	3\\
0.814777322196743	3\\
0.814777322196743	4\\
0.937508348074481	4\\
0.937508348074481	5\\
2.3670008077024	5\\
2.3670008077024	6\\
3.5766155945264	6\\
3.5766155945264	7\\
5.28725855521375	7\\
5.28725855521375	8\\
5.52532016297894	8\\
5.52532016297894	9\\
6.47697504031317	9\\
6.47697504031317	10\\
6.49640152949379	10\\
6.49640152949379	11\\
7.44311459420302	11\\
7.44311459420302	12\\
8.03214999397893	12\\
8.03214999397893	13\\
8.4033553399445	13\\
8.4033553399445	14\\
8.97339633545079	14\\
8.97339633545079	15\\
9.34750363008556	15\\
9.34750363008556	16\\
9.73359723684735	16\\
9.73359723684735	17\\
12.292989680232	17\\
12.292989680232	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.573613123009263	0\\
0.573613123009263	1\\
1.05406339744932	1\\
1.05406339744932	2\\
1.19330832507541	2\\
1.19330832507541	3\\
1.66445879067816	3\\
1.66445879067816	4\\
1.68918144482488	4\\
1.68918144482488	5\\
2.07385698903632	5\\
2.07385698903632	6\\
2.0957244484212	6\\
2.0957244484212	7\\
2.2293773455635	7\\
2.2293773455635	8\\
2.61698797968526	8\\
2.61698797968526	9\\
3.52643716187442	9\\
3.52643716187442	10\\
3.716379034187	10\\
3.716379034187	11\\
5.21626485725698	11\\
5.21626485725698	12\\
5.4821769065356	12\\
5.4821769065356	13\\
6.57982570322374	13\\
6.57982570322374	14\\
6.75214994085295	14\\
6.75214994085295	15\\
6.98307264663988	15\\
6.98307264663988	16\\
6.99708794905413	16\\
6.99708794905413	17\\
7.23898424901443	17\\
7.23898424901443	18\\
7.82033808642714	18\\
7.82033808642714	19\\
8.05028281011423	19\\
8.05028281011423	20\\
8.96581180834828	20\\
8.96581180834828	21\\
9.04200367853034	21\\
9.04200367853034	22\\
9.07657365186567	22\\
9.07657365186567	23\\
9.29392938653938	23\\
9.29392938653938	24\\
9.341766235769	24\\
9.341766235769	25\\
9.45749071309546	25\\
9.45749071309546	26\\
9.56801918989986	26\\
9.56801918989986	27\\
9.68596215655318	27\\
9.68596215655318	28\\
9.85114032043525	28\\
9.85114032043525	29\\
9.89428090886142	29\\
9.89428090886142	30\\
10.1674454441261	30\\
10.1674454441261	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.202234516268991	0\\
0.202234516268991	1\\
0.795047768253294	1\\
0.795047768253294	2\\
0.934288560556105	2\\
0.934288560556105	3\\
1.82368667737192	3\\
1.82368667737192	4\\
1.94609416812642	4\\
1.94609416812642	5\\
1.95592303400981	5\\
1.95592303400981	6\\
2.0025257506915	6\\
2.0025257506915	7\\
3.08772662301012	7\\
3.08772662301012	8\\
3.2934233440054	8\\
3.2934233440054	9\\
3.36958057550393	9\\
3.36958057550393	10\\
3.48261824016622	10\\
3.48261824016622	11\\
4.02227471603508	11\\
4.02227471603508	12\\
4.24063649926962	12\\
4.24063649926962	13\\
8.86271699011814	13\\
8.86271699011814	14\\
9.71009098164887	14\\
9.71009098164887	15\\
9.74287814293268	15\\
9.74287814293268	16\\
9.80159265306765	16\\
9.80159265306765	17\\
9.89328586524542	17\\
9.89328586524542	18\\
9.92930043280572	18\\
9.92930043280572	19\\
9.93681476023323	19\\
9.93681476023323	20\\
10.1745117455632	20\\
10.1745117455632	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.418732916877087	0\\
0.418732916877087	1\\
1.29442764066659	1\\
1.29442764066659	2\\
3.08997901221368	2\\
3.08997901221368	3\\
3.22866409722053	3\\
3.22866409722053	4\\
3.68737510442231	4\\
3.68737510442231	5\\
3.78197130043255	5\\
3.78197130043255	6\\
4.13112008030134	6\\
4.13112008030134	7\\
4.5826942926494	7\\
4.5826942926494	8\\
8.31761814039515	8\\
8.31761814039515	9\\
8.3661320053933	9\\
8.3661320053933	10\\
8.80523308918912	10\\
8.80523308918912	11\\
9.67960094634029	11\\
9.67960094634029	12\\
12.0040468525298	12\\
12.0040468525298	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
4.22542215707887	0\\
4.22542215707887	1\\
4.34935038879406	1\\
4.34935038879406	2\\
6.83107224274331	2\\
6.83107224274331	3\\
9.22706909043675	3\\
9.22706909043675	4\\
9.42837675301717	4\\
9.42837675301717	5\\
13.1451167187751	5\\
13.1451167187751	6\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0690451968691956	0\\
0.0690451968691956	1\\
0.17824278705274	1\\
0.17824278705274	2\\
0.193287917082118	2\\
0.193287917082118	3\\
0.547367949654976	3\\
0.547367949654976	4\\
1.00726873188087	4\\
1.00726873188087	5\\
1.52068682650493	5\\
1.52068682650493	6\\
2.13300975301772	6\\
2.13300975301772	7\\
5.69402574195719	7\\
5.69402574195719	8\\
5.83207339522523	8\\
5.83207339522523	9\\
5.90331780908443	9\\
5.90331780908443	10\\
5.92105175805796	10\\
5.92105175805796	11\\
8.57286478134551	11\\
8.57286478134551	12\\
9.12548838148815	12\\
9.12548838148815	13\\
9.87890168697091	13\\
9.87890168697091	14\\
11.6991231043178	14\\
11.6991231043178	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.701893323800594	0\\
0.701893323800594	1\\
0.816905865577539	1\\
0.816905865577539	2\\
0.964364200800453	2\\
0.964364200800453	3\\
1.09166870216227	3\\
1.09166870216227	4\\
1.66677998007291	4\\
1.66677998007291	5\\
2.32221443826874	5\\
2.32221443826874	6\\
3.59024557546909	6\\
3.59024557546909	7\\
3.97419085548652	7\\
3.97419085548652	8\\
4.226318130489	8\\
4.226318130489	9\\
4.23907601126134	9\\
4.23907601126134	10\\
4.29618017229971	10\\
4.29618017229971	11\\
4.52976183085465	11\\
4.52976183085465	12\\
4.5539188233105	12\\
4.5539188233105	13\\
4.65743002779363	13\\
4.65743002779363	14\\
5.40771814702601	14\\
5.40771814702601	15\\
5.99059789137237	15\\
5.99059789137237	16\\
8.00740331905888	16\\
8.00740331905888	17\\
9.04404785497188	17\\
9.04404785497188	18\\
10.9045834375805	18\\
10.9045834375805	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.241970716981562	0\\
0.241970716981562	1\\
0.419392749609379	1\\
0.419392749609379	2\\
0.472985132688429	2\\
0.472985132688429	3\\
2.01232588870072	3\\
2.01232588870072	4\\
2.56139051799822	4\\
2.56139051799822	5\\
3.46146480417444	5\\
3.46146480417444	6\\
3.90633719736872	6\\
3.90633719736872	7\\
3.94205952014878	7\\
3.94205952014878	8\\
3.97380743872409	8\\
3.97380743872409	9\\
4.08628029984673	9\\
4.08628029984673	10\\
4.40517687478307	10\\
4.40517687478307	11\\
4.56297984480919	11\\
4.56297984480919	12\\
4.58462980614527	12\\
4.58462980614527	13\\
4.70902516571629	13\\
4.70902516571629	14\\
5.63182453303077	14\\
5.63182453303077	15\\
6.5364944023999	15\\
6.5364944023999	16\\
7.62979626934588	16\\
7.62979626934588	17\\
10.6189088626102	17\\
10.6189088626102	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.618267195792384	0\\
0.618267195792384	1\\
1.17975511994756	1\\
1.17975511994756	2\\
1.38232800947027	2\\
1.38232800947027	3\\
1.4699970468141	3\\
1.4699970468141	4\\
1.67662726670363	4\\
1.67662726670363	5\\
1.88124089220939	5\\
1.88124089220939	6\\
1.91544524904959	6\\
1.91544524904959	7\\
1.94502074958746	7\\
1.94502074958746	8\\
2.24338467508771	8\\
2.24338467508771	9\\
2.33062359328316	9\\
2.33062359328316	10\\
2.64021147153478	10\\
2.64021147153478	11\\
2.79279144183147	11\\
2.79279144183147	12\\
2.95648733834523	12\\
2.95648733834523	13\\
3.12095258289861	13\\
3.12095258289861	14\\
3.13690707340896	14\\
3.13690707340896	15\\
3.67036472549593	15\\
3.67036472549593	16\\
3.75092812192578	16\\
3.75092812192578	17\\
4.21655254063458	17\\
4.21655254063458	18\\
4.224848261955	18\\
4.224848261955	19\\
5.39757067736292	19\\
5.39757067736292	20\\
5.9384794322219	20\\
5.9384794322219	21\\
5.95082714913815	21\\
5.95082714913815	22\\
7.5103652592322	22\\
7.5103652592322	23\\
7.67082094255916	23\\
7.67082094255916	24\\
7.75415613109001	24\\
7.75415613109001	25\\
7.78597406715829	25\\
7.78597406715829	26\\
11.1952545598077	26\\
11.1952545598077	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.611224722738829	0\\
0.611224722738829	1\\
0.769717428036486	1\\
0.769717428036486	2\\
0.816975871086498	2\\
0.816975871086498	3\\
0.96113682265144	3\\
0.96113682265144	4\\
1.00183613009736	4\\
1.00183613009736	5\\
1.44091050477769	5\\
1.44091050477769	6\\
3.17116908429839	6\\
3.17116908429839	7\\
3.4166301359773	7\\
3.4166301359773	8\\
4.01901878213728	8\\
4.01901878213728	9\\
4.1098432664202	9\\
4.1098432664202	10\\
4.13766099085272	10\\
4.13766099085272	11\\
5.64667907846013	11\\
5.64667907846013	12\\
5.90133999263228	12\\
5.90133999263228	13\\
6.04467530399966	13\\
6.04467530399966	14\\
6.24572835739717	14\\
6.24572835739717	15\\
6.46424900098701	15\\
6.46424900098701	16\\
6.5796830977691	16\\
6.5796830977691	17\\
6.70109776079336	17\\
6.70109776079336	18\\
7.33163372501048	18\\
7.33163372501048	19\\
8.12928540514507	19\\
8.12928540514507	20\\
8.1586097024684	20\\
8.1586097024684	21\\
10.0495104837533	21\\
10.0495104837533	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.524599729147818	0\\
0.524599729147818	1\\
1.35943817597277	1\\
1.35943817597277	2\\
2.19772790991068	2\\
2.19772790991068	3\\
2.62092075177748	3\\
2.62092075177748	4\\
5.91538075424351	4\\
5.91538075424351	5\\
6.55666046875826	5\\
6.55666046875826	6\\
6.67101584332353	6\\
6.67101584332353	7\\
7.19110599249168	7\\
7.19110599249168	8\\
7.29965577284522	8\\
7.29965577284522	9\\
7.76277956123876	9\\
7.76277956123876	10\\
7.8423885353429	10\\
7.8423885353429	11\\
8.12303340987365	11\\
8.12303340987365	12\\
8.48764282303783	12\\
8.48764282303783	13\\
12.7626369671693	13\\
12.7626369671693	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.58075678590297	0\\
1.58075678590297	1\\
1.94246549003163	1\\
1.94246549003163	2\\
2.03951497364353	2\\
2.03951497364353	3\\
2.09126692078943	3\\
2.09126692078943	4\\
2.11412123493383	4\\
2.11412123493383	5\\
2.18392710295685	5\\
2.18392710295685	6\\
2.36429901535411	6\\
2.36429901535411	7\\
2.51118503625662	7\\
2.51118503625662	8\\
3.19649542628853	8\\
3.19649542628853	9\\
3.31458195390753	9\\
3.31458195390753	10\\
4.11791387442784	10\\
4.11791387442784	11\\
4.18151307838908	11\\
4.18151307838908	12\\
4.51619216227301	12\\
4.51619216227301	13\\
4.76999884623185	13\\
4.76999884623185	14\\
5.99355357484709	14\\
5.99355357484709	15\\
6.16801827762938	15\\
6.16801827762938	16\\
6.25529133621082	16\\
6.25529133621082	17\\
6.33161602852886	17\\
6.33161602852886	18\\
6.58228581873779	18\\
6.58228581873779	19\\
6.70853612325967	19\\
6.70853612325967	20\\
6.72002006573996	20\\
6.72002006573996	21\\
6.87450487741296	21\\
6.87450487741296	22\\
7.23874294577538	22\\
7.23874294577538	23\\
7.30246687861203	23\\
7.30246687861203	24\\
7.68462262597652	24\\
7.68462262597652	25\\
8.90304140232167	25\\
8.90304140232167	26\\
8.93091422239534	26\\
8.93091422239534	27\\
9.04996579968119	27\\
9.04996579968119	28\\
10.3121542707133	28\\
10.3121542707133	29\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.37188781813856	0\\
1.37188781813856	1\\
3.09219170801967	1\\
3.09219170801967	2\\
4.96862928285465	2\\
4.96862928285465	3\\
7.33090341235169	3\\
7.33090341235169	4\\
7.48540298071888	4\\
7.48540298071888	5\\
7.49012279678696	5\\
7.49012279678696	6\\
7.53652242125794	6\\
7.53652242125794	7\\
7.55488723727228	7\\
7.55488723727228	8\\
10.9436629288184	8\\
10.9436629288184	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.151966071781235	0\\
0.151966071781235	1\\
1.67710241517837	1\\
1.67710241517837	2\\
1.7623253879174	2\\
1.7623253879174	3\\
4.6118098514298	3\\
4.6118098514298	4\\
5.33897859840662	4\\
5.33897859840662	5\\
5.53504319044576	5\\
5.53504319044576	6\\
6.45628690440148	6\\
6.45628690440148	7\\
8.15536899943535	7\\
8.15536899943535	8\\
8.62372726386685	8\\
8.62372726386685	9\\
8.90336575674946	9\\
8.90336575674946	10\\
8.95459102651032	10\\
8.95459102651032	11\\
9.23978473060495	11\\
9.23978473060495	12\\
9.47494478973985	12\\
9.47494478973985	13\\
9.54444978332178	13\\
9.54444978332178	14\\
9.57426140889784	14\\
9.57426140889784	15\\
10.2164751098918	15\\
10.2164751098918	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.80353005695015	0\\
1.80353005695015	1\\
2.06929180715767	1\\
2.06929180715767	2\\
2.63958010080202	2\\
2.63958010080202	3\\
3.38283478719855	3\\
3.38283478719855	4\\
4.52209932670052	4\\
4.52209932670052	5\\
4.86645024463097	5\\
4.86645024463097	6\\
4.9009654009096	6\\
4.9009654009096	7\\
5.13238010942793	7\\
5.13238010942793	8\\
5.9986913056029	8\\
5.9986913056029	9\\
6.38652630382514	9\\
6.38652630382514	10\\
6.71422953800408	10\\
6.71422953800408	11\\
7.17754354542048	11\\
7.17754354542048	12\\
7.42713334837553	12\\
7.42713334837553	13\\
7.45255409405846	13\\
7.45255409405846	14\\
8.5617430450324	14\\
8.5617430450324	15\\
8.66734766270438	15\\
8.66734766270438	16\\
8.72205988167862	16\\
8.72205988167862	17\\
8.77562991482028	17\\
8.77562991482028	18\\
9.01974897775226	18\\
9.01974897775226	19\\
9.24478246973761	19\\
9.24478246973761	20\\
9.33675307831528	20\\
9.33675307831528	21\\
9.35778915297507	21\\
9.35778915297507	22\\
9.56928231447662	22\\
9.56928231447662	23\\
9.79877026857552	23\\
9.79877026857552	24\\
9.96456564638646	24\\
9.96456564638646	25\\
10.2167141417496	25\\
10.2167141417496	26\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.28295066920428	0\\
1.28295066920428	1\\
1.30295358848746	1\\
1.30295358848746	2\\
1.37575457462958	2\\
1.37575457462958	3\\
1.39178283916599	3\\
1.39178283916599	4\\
1.65226955675303	4\\
1.65226955675303	5\\
1.85112639796447	5\\
1.85112639796447	6\\
2.12398595865236	6\\
2.12398595865236	7\\
3.2639968617289	7\\
3.2639968617289	8\\
4.01144518679825	8\\
4.01144518679825	9\\
4.13927493156734	9\\
4.13927493156734	10\\
4.75879162723915	10\\
4.75879162723915	11\\
4.98912312081835	11\\
4.98912312081835	12\\
5.89030036497916	12\\
5.89030036497916	13\\
6.7019187748923	13\\
6.7019187748923	14\\
7.02718369075133	14\\
7.02718369075133	15\\
10.454826226415	15\\
10.454826226415	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.17882598584282	0\\
2.17882598584282	1\\
2.51013751198123	1\\
2.51013751198123	2\\
3.35689993663743	2\\
3.35689993663743	3\\
5.16540892008532	3\\
5.16540892008532	4\\
6.72142897881467	4\\
6.72142897881467	5\\
6.73788681902047	5\\
6.73788681902047	6\\
6.93626762231121	6\\
6.93626762231121	7\\
6.98478720066282	7\\
6.98478720066282	8\\
7.59986408090156	8\\
7.59986408090156	9\\
7.63190408966843	9\\
7.63190408966843	10\\
7.99107701646198	10\\
7.99107701646198	11\\
11.469888334771	11\\
11.469888334771	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.111695721762953	0\\
0.111695721762953	1\\
0.128992078669892	1\\
0.128992078669892	2\\
0.184177631970567	2\\
0.184177631970567	3\\
3.89531963056811	3\\
3.89531963056811	4\\
4.34259393996367	4\\
4.34259393996367	5\\
4.34308925368684	6\\
4.84665828166116	6\\
4.84665828166116	7\\
5.03565053068199	7\\
5.03565053068199	8\\
5.08736066962168	8\\
5.08736066962168	9\\
5.24524530894687	9\\
5.24524530894687	10\\
6.27450088623272	10\\
6.27450088623272	11\\
6.92171668599546	11\\
6.92171668599546	12\\
7.07655730509914	12\\
7.07655730509914	13\\
7.16400713741533	13\\
7.16400713741533	14\\
7.57449541905332	14\\
7.57449541905332	15\\
7.62941848368038	15\\
7.62941848368038	16\\
7.63745642670737	16\\
7.63745642670737	17\\
7.8450085740055	17\\
7.8450085740055	18\\
7.99041316649775	18\\
7.99041316649775	19\\
8.11925890472246	19\\
8.11925890472246	20\\
8.23950876692045	20\\
8.23950876692045	21\\
8.35120910718821	21\\
8.35120910718821	22\\
11.5432950048148	22\\
11.5432950048148	23\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0177019847877915	0\\
0.0177019847877915	1\\
0.363693312009406	1\\
0.363693312009406	2\\
0.602056885945533	2\\
0.602056885945533	3\\
0.753131659468036	3\\
0.753131659468036	4\\
0.78749581732508	4\\
0.78749581732508	5\\
0.976904289757673	5\\
0.976904289757673	6\\
1.09680779660224	6\\
1.09680779660224	7\\
1.25035237777828	7\\
1.25035237777828	8\\
1.32877265536053	8\\
1.32877265536053	9\\
1.34128290018825	9\\
1.34128290018825	10\\
1.44792729889614	10\\
1.44792729889614	11\\
1.93379347277116	11\\
1.93379347277116	12\\
2.58582174288223	12\\
2.58582174288223	13\\
2.77464366863635	13\\
2.77464366863635	14\\
2.8994757685063	14\\
2.8994757685063	15\\
2.98256317299881	15\\
2.98256317299881	16\\
3.15776434226147	16\\
3.15776434226147	17\\
3.56468880428302	17\\
3.56468880428302	18\\
4.83388779771385	18\\
4.83388779771385	19\\
6.88346699796091	19\\
6.88346699796091	20\\
7.03683911765425	20\\
7.03683911765425	21\\
7.57045431507319	21\\
7.57045431507319	22\\
10.2042582605847	22\\
10.2042582605847	23\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.980488632152827	0\\
0.980488632152827	1\\
2.2807086103548	1\\
2.2807086103548	2\\
3.41085183708728	2\\
3.41085183708728	3\\
3.77001272964656	3\\
3.77001272964656	4\\
3.92069162261616	4\\
3.92069162261616	5\\
4.07930391179843	5\\
4.07930391179843	6\\
4.13735294848236	6\\
4.13735294848236	7\\
5.04644028575607	7\\
5.04644028575607	8\\
5.42948078853264	8\\
5.42948078853264	9\\
5.49992212492843	9\\
5.49992212492843	10\\
6.71323279131868	10\\
6.71323279131868	11\\
7.87268697355168	11\\
7.87268697355168	12\\
7.87458649897273	13\\
9.01720382578979	13\\
9.01720382578979	14\\
9.16023661009041	14\\
9.16023661009041	15\\
13.0569502121661	15\\
13.0569502121661	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.30396206200267	0\\
0.30396206200267	1\\
0.51902284819527	1\\
0.51902284819527	2\\
0.580863332118502	2\\
0.580863332118502	3\\
0.948043918846739	3\\
0.948043918846739	4\\
1.1645146126941	4\\
1.1645146126941	5\\
3.34763826666095	5\\
3.34763826666095	6\\
6.1662500068301	6\\
6.1662500068301	7\\
7.80445503902437	7\\
7.80445503902437	8\\
9.26112577000689	8\\
9.26112577000689	9\\
9.53751235452796	9\\
9.53751235452796	10\\
10.2691842481559	10\\
10.2691842481559	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.67812122198984	0\\
2.67812122198984	1\\
3.66687868994735	1\\
3.66687868994735	2\\
4.75335598161674	2\\
4.75335598161674	3\\
4.92928711139323	3\\
4.92928711139323	4\\
6.64367858125098	4\\
6.64367858125098	5\\
9.77240690664343	5\\
9.77240690664343	6\\
10.0734609966656	6\\
10.0734609966656	7\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.6147866037583	0\\
1.6147866037583	1\\
1.7696770232832	1\\
1.7696770232832	2\\
3.38015236660706	2\\
3.38015236660706	3\\
3.4920677938512	3\\
3.4920677938512	4\\
3.88680873454663	4\\
3.88680873454663	5\\
4.25107446859219	5\\
4.25107446859219	6\\
4.51662278455367	6\\
4.51662278455367	7\\
4.6019208734196	7\\
4.6019208734196	8\\
4.69386330402677	8\\
4.69386330402677	9\\
4.85526747225579	9\\
4.85526747225579	10\\
4.8881716848695	10\\
4.8881716848695	11\\
5.13986746472458	11\\
5.13986746472458	12\\
5.57913033978112	12\\
5.57913033978112	13\\
5.66496822913134	13\\
5.66496822913134	14\\
5.67032285036257	14\\
5.67032285036257	15\\
5.79168398848548	15\\
5.79168398848548	16\\
7.65926181820143	16\\
7.65926181820143	17\\
7.89791458513396	17\\
7.89791458513396	18\\
8.57412804133548	18\\
8.57412804133548	19\\
12.686645199555	19\\
12.686645199555	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0481727590252241	0\\
0.0481727590252241	1\\
0.0686652880852989	1\\
0.0686652880852989	2\\
0.566434557897505	2\\
0.566434557897505	3\\
1.56600362843935	3\\
1.56600362843935	4\\
1.74206251908696	4\\
1.74206251908696	5\\
1.74856321111291	5\\
1.74856321111291	6\\
1.97177586643965	6\\
1.97177586643965	7\\
2.16096601756978	7\\
2.16096601756978	8\\
2.30409548797642	8\\
2.30409548797642	9\\
2.49795379218721	9\\
2.49795379218721	10\\
2.62586310248905	10\\
2.62586310248905	11\\
3.48149019849433	11\\
3.48149019849433	12\\
5.46006161934136	12\\
5.46006161934136	13\\
5.63656973183504	13\\
5.63656973183504	14\\
5.91751733766154	14\\
5.91751733766154	15\\
5.97414934720728	15\\
5.97414934720728	16\\
9.38746241015493	16\\
9.38746241015493	17\\
9.94749738386131	17\\
9.94749738386131	18\\
10.7959267209003	18\\
10.7959267209003	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0187815427547839	0\\
0.0187815427547839	1\\
1.17263717546488	1\\
1.17263717546488	2\\
3.12365544107182	2\\
3.12365544107182	3\\
3.26365109432083	3\\
3.26365109432083	4\\
4.21909174903787	4\\
4.21909174903787	5\\
4.30667398063471	5\\
4.30667398063471	6\\
6.4656805015088	6\\
6.4656805015088	7\\
6.57952305459802	7\\
6.57952305459802	8\\
6.72627354138982	8\\
6.72627354138982	9\\
6.74914726235771	9\\
6.74914726235771	10\\
6.8407413740111	10\\
6.8407413740111	11\\
7.68469030102168	11\\
7.68469030102168	12\\
7.74813106177294	12\\
7.74813106177294	13\\
8.68832377977213	13\\
8.68832377977213	14\\
9.22658378503885	14\\
9.22658378503885	15\\
11.1081857227689	15\\
11.1081857227689	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.241728726158737	0\\
0.241728726158737	1\\
0.486183533748473	1\\
0.486183533748473	2\\
0.530947042332381	2\\
0.530947042332381	3\\
0.733768207713457	3\\
0.733768207713457	4\\
2.75977646581417	4\\
2.75977646581417	5\\
6.74705473485604	5\\
6.74705473485604	6\\
6.98288901720928	6\\
6.98288901720928	7\\
7.2854430890909	7\\
7.2854430890909	8\\
7.33071141633732	8\\
7.33071141633732	9\\
7.76863069327772	9\\
7.76863069327772	10\\
8.10443103616015	10\\
8.10443103616015	11\\
9.12245308561093	11\\
9.12245308561093	12\\
12.0913271989418	12\\
12.0913271989418	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.203594211942779	0\\
0.203594211942779	1\\
0.266976121836453	1\\
0.266976121836453	2\\
1.43586234271751	2\\
1.43586234271751	3\\
2.10089930597173	3\\
2.10089930597173	4\\
2.90241085353091	4\\
2.90241085353091	5\\
3.57255804219624	5\\
3.57255804219624	6\\
3.59945927884397	6\\
3.59945927884397	7\\
3.68813581323744	7\\
3.68813581323744	8\\
3.69166658739269	8\\
3.69166658739269	9\\
3.93266106331464	9\\
3.93266106331464	10\\
4.17146195715777	10\\
4.17146195715777	11\\
4.55402460937196	11\\
4.55402460937196	12\\
4.80650912382896	12\\
4.80650912382896	13\\
4.93804735784854	13\\
4.93804735784854	14\\
5.56167110537038	14\\
5.56167110537038	15\\
7.07858634617868	15\\
7.07858634617868	16\\
7.59244101622268	16\\
7.59244101622268	17\\
10.9841958799294	17\\
10.9841958799294	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.344694288518895	0\\
0.344694288518895	1\\
0.757342944414811	1\\
0.757342944414811	2\\
7.40130200667622	2\\
7.40130200667622	3\\
13.6421447746621	3\\
13.6421447746621	4\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.516574884480463	0\\
0.516574884480463	1\\
0.632100179746956	1\\
0.632100179746956	2\\
1.06962807988355	2\\
1.06962807988355	3\\
1.07543882740856	3\\
1.07543882740856	4\\
1.20240875260934	4\\
1.20240875260934	5\\
1.85225998048788	5\\
1.85225998048788	6\\
5.12736259906934	6\\
5.12736259906934	7\\
5.84095393401714	7\\
5.84095393401714	8\\
5.92084151359242	8\\
5.92084151359242	9\\
5.92267547065092	10\\
6.75226706536699	10\\
6.75226706536699	11\\
7.40343134591207	11\\
7.40343134591207	12\\
8.08600798658836	12\\
8.08600798658836	13\\
8.55303362777762	13\\
8.55303362777762	14\\
9.15609356411406	14\\
9.15609356411406	15\\
9.93593504716475	15\\
9.93593504716475	16\\
10.0605229324352	16\\
10.0605229324352	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.591810954453216	0\\
0.591810954453216	1\\
2.44722389247089	1\\
2.44722389247089	2\\
2.6522296607257	2\\
2.6522296607257	3\\
4.63086891595317	3\\
4.63086891595317	4\\
5.55705489275282	4\\
5.55705489275282	5\\
5.82277414319854	5\\
5.82277414319854	6\\
6.09782726784542	6\\
6.09782726784542	7\\
6.27005045890638	7\\
6.27005045890638	8\\
6.35103912387203	8\\
6.35103912387203	9\\
6.39823157305104	9\\
6.39823157305104	10\\
6.51482485827059	10\\
6.51482485827059	11\\
6.59830771200484	11\\
6.59830771200484	12\\
6.95171978618288	12\\
6.95171978618288	13\\
7.00712484060556	13\\
7.00712484060556	14\\
7.03149436605025	14\\
7.03149436605025	15\\
7.05724831162668	15\\
7.05724831162668	16\\
7.1568979017224	16\\
7.1568979017224	17\\
7.43182028709825	17\\
7.43182028709825	18\\
7.45318860360107	18\\
7.45318860360107	19\\
7.45454196563755	20\\
8.24859752224869	20\\
8.24859752224869	21\\
8.36542504484017	21\\
8.36542504484017	22\\
8.59929713123556	22\\
8.59929713123556	23\\
8.66651465078127	23\\
8.66651465078127	24\\
8.95159279091164	24\\
8.95159279091164	25\\
9.057918427878	25\\
9.057918427878	26\\
9.07989611826134	26\\
9.07989611826134	27\\
9.1451373779036	27\\
9.1451373779036	28\\
9.55385382987364	28\\
9.55385382987364	29\\
9.59182353174972	29\\
9.59182353174972	30\\
9.60447468278195	30\\
9.60447468278195	31\\
9.84200219627841	31\\
9.84200219627841	32\\
11.0886421541626	32\\
11.0886421541626	33\\
};


==> fig7_part1b_220209.tex <==

\addplot [color=blue,
%line width=1.0pt,
forget plot]
  table[row sep=crcr]{%
-0.025578987642584	1.42529773991451\\
0.0271883912521851	1.36590736550217\\
0.0799557701469524	1.31172289793476\\
0.132723149041722	1.26228800962812\\
0.185490527936491	1.21718637272729\\
0.238257906831258	1.17603815290092\\
0.291025285726027	1.13849681047463\\
0.37017635406818	1.08826373018664\\
0.449327422410331	1.04448855120732\\
0.528478490752484	1.00634105390702\\
0.607629559094637	0.97309775064231\\
0.686780627436789	0.94412816442674\\
0.765931695778942	0.918882871598324\\
0.871466453568479	0.890197310670082\\
0.977001211358015	0.866320251221772\\
1.08253596914755	0.846445654056868\\
1.21445441638447	0.82621975039716\\
1.3463728636214	0.810139055877663\\
1.5046750003057	0.795130429324107\\
1.68936082643739	0.78211981286649\\
1.90043034201646	0.771564889591062\\
1.90043034201646	1.86009875466243\\
1.95263700049035	1.76358535767595\\
2.00484365896424	1.67544603419795\\
2.05705031743814	1.59495420005136\\
2.10925697591203	1.52144631380239\\
2.16146363438592	1.45431640679902\\
2.2188909587072	1.38718105837171\\
2.27631828302848	1.32642472320589\\
2.33374560734976	1.27144128528157\\
2.39117293167104	1.22168222002973\\
2.42249692675537	1.19656342068203\\
2.42249692675537	2.2850972857534\\
2.44746720640466	2.21978662374247\\
2.44746720640466	3.30832048881384\\
2.50066255760242	3.08213484641942\\
2.55385790880017	2.87592915573524\\
2.60705325999792	2.6879385015964\\
2.66024861119567	2.51655387139396\\
2.71344396239343	2.36030838353084\\
2.76663931359118	2.21786473237761\\
2.81983466478893	2.08800374226927\\
2.87303001598668	1.9696139325769\\
2.92622536718444	1.86168200454138\\
2.97942071838219	1.76328416844605\\
3.03261606957994	1.67357823689765\\
3.08581142077769	1.59179641654166\\
3.13900677197545	1.51723873651655\\
3.1922021231732	1.44926705740095\\
3.24539747437095	1.38729960937631\\
3.29859282556871	1.33080601285716\\
3.33405639303387	1.29594406350903\\
3.33405639303387	2.3844779285804\\
3.38378996649834	2.24890669413217\\
3.43352353996282	2.12456495744775\\
3.48325711342729	2.01052256825935\\
3.53299068689176	1.90592642155436\\
3.5412796158025	1.88935619712947\\
3.5412796158025	2.97789006220084\\
3.5899347246271	2.79700455348919\\
3.6385898334517	2.63079061774191\\
3.67643269587083	2.51089114032105\\
3.67643269587083	3.59942500539242\\
3.72531382597503	3.36709751056562\\
3.77419495607923	3.15369790471727\\
3.82307608618343	2.95768411904726\\
3.87195721628763	2.77763971821556\\
3.92083834639183	2.61226366489339\\
3.92083834639183	3.70079752996476\\
3.96978178558072	3.45991732758952\\
3.98052546735389	3.40972907079995\\
3.98052546735389	4.49826293587133\\
4.02953718746141	4.19192442905006\\
4.07854890756894	3.91060741796377\\
4.12756062767646	3.6522681659131\\
4.17657234778398	3.41502986705451\\
4.1847409678019	3.37741849062154\\
4.1847409678019	4.46595235569291\\
4.22781596843031	4.19767710696878\\
4.22781596843031	5.28621097204016\\
4.23637321351316	5.21919187059628\\
4.23637321351316	6.30772573566765\\
4.28491184586282	5.85779285671461\\
4.30473748442818	5.68466326906937\\
4.30473748442818	6.77319713414074\\
4.35306177843114	6.28766059582283\\
4.35455634422504	6.27328465301127\\
4.35455634422504	7.36181851808264\\
4.4032831857458	6.8245959115899\\
4.45201002726655	6.33100883923431\\
4.5007368687873	5.87751303497708\\
4.54946371030806	5.46085211333379\\
4.59819055182881	5.0780341864756\\
4.61101340486059	4.98256753192234\\
4.61101340486059	6.07110139699371\\
4.65881359906046	5.64660211928465\\
4.70661379326032	5.25595367038716\\
4.75441398746019	4.89645668502214\\
4.76038901173518	4.85358395354785\\
4.76038901173518	5.94211781861922\\
4.80795365430729	5.52986201373868\\
4.85551829687939	5.15032531295371\\
4.9030829394515	4.80091093106408\\
4.95064758202361	4.47922817938607\\
4.99821222459572	4.18307610869131\\
5.04577686716783	3.91042845034069\\
5.09334150973994	3.65941975258051\\
5.14090615231205	3.42833261714566\\
5.18847079488416	3.21558594884293\\
5.23603543745626	3.01972413771814\\
5.23603543745626	4.10825800278951\\
5.28676526687569	3.82457064526061\\
5.33749509629511	3.56483165281395\\
5.38822492571453	3.32701934850521\\
5.43895475513395	3.10928272164027\\
5.48968458455338	2.90992702044419\\
5.5404144139728	2.72740056097061\\
5.59114424339222	2.56028264957868\\
5.64187407281164	2.40727252497239\\
5.69260390223106	2.26717923373247\\
5.74333373165049	2.13891236053744\\
5.79406356106991	2.0214735409222\\
5.84479339048933	1.91394869051401\\
5.87015830519904	1.8636396342871\\
5.87015830519904	2.95217349935847\\
5.91752967941962	2.77789970780222\\
5.9649010536402	2.61740341589664\\
6.01227242786078	2.46959542087105\\
6.05964380208136	2.33347262866138\\
6.10701517630194	2.20811124644555\\
6.15438655052251	2.09266051335411\\
6.20175792474309	1.98633692680968\\
6.24912929896367	1.88841892531274\\
6.29650067318425	1.79824199158838\\
6.34387204740483	1.71519414286179\\
6.40071769646952	1.6241567431317\\
6.45756334553422	1.54168610552861\\
6.51440899459891	1.46697608429748\\
6.57125464366361	1.39929639326346\\
6.6281002927283	1.33798546732638\\
6.684945941793	1.28244399569978\\
6.74179159085769	1.23212906368239\\
6.79863723992239	1.18654884569798\\
6.81758578961062	1.17232934346202\\
6.81758578961062	2.26086320853339\\
6.8422516438123	2.19734907949578\\
6.8422516438123	3.28588294456715\\
6.88977052946476	3.08462783100788\\
6.93728941511721	2.8993307958328\\
6.98480830076965	2.72872647856879\\
7.0323271864221	2.5716498526982\\
7.07984607207456	2.42702826990025\\
7.12736495772701	2.29387413512645\\
7.17488384337946	2.17127816248985\\
7.22240272903191	2.05840316591356\\
7.26992161468436	1.95447834213597\\
7.31744050033681	1.85879400703257\\
7.36495938598926	1.77069674930929\\
7.41247827164171	1.68958496847312\\
7.46950093442465	1.60069490486378\\
7.52652359720759	1.52019431309804\\
7.58354625999053	1.4472913922146\\
7.64056892277347	1.38126907167312\\
7.69759158555641	1.32147795827383\\
7.75461424833935	1.26732994874906\\
7.79262935686131	1.23410119947816\\
7.79262935686131	2.32263506454953\\
7.84336899540302	2.18966212235371\\
7.89410863394474	2.06791658763339\\
7.94484827248645	1.95645048799255\\
7.99558791102816	1.85439589192308\\
8.04632754956987	1.76095815065052\\
8.09706718811158	1.67540971059619\\
8.14780682665329	1.59708444827655\\
8.198546465195	1.52537248352832\\
8.25562855855443	1.45190808715149\\
8.31271065191385	1.38538415709352\\
8.36979274527328	1.32514500059576\\
8.4268748386327	1.27059687073633\\
8.4268748386327	2.3591307358077\\
8.47981713284744	2.21743755257515\\
8.53275942706219	2.088203894723\\
8.58570172127692	1.97033415716168\\
8.63864401549166	1.86282907478857\\
8.69158630970641	1.76477725101119\\
8.74452860392115	1.67534743119388\\
8.79747089813589	1.5937814555246\\
8.85041319235063	1.51938783155808\\
8.90335548656537	1.45153587194551\\
8.95629778078011	1.38965034765195\\
9.00924007499485	1.3332066113331\\
9.06218236920959	1.28172614952885\\
9.11512466342433	1.23477252596628\\
9.16806695763907	1.1919476815809\\
9.22100925185381	1.15288855988844\\
9.27395154606855	1.11726402909838\\
9.32689384028329	1.08477207487563\\
9.37983613449803	1.05513723995151\\
9.43277842871277	1.02810828887768\\
9.53866301714226	0.98097161347496\\
9.64454760557174	0.941760217185605\\
9.75043219400122	0.909141590907348\\
9.8563167824307	0.882007265660953\\
9.96220137086018	0.859435143821845\\
10.0151436650749	0.849614890993715\\
};
\addplot [color=red, dashed,
%line width=1.0pt,
forget plot]
  table[row sep=crcr]{%
-0.025578987642584	1.40246483376747\\
0.0271883912521851	1.3482788084557\\
0.0799557701469524	1.29924628275398\\
0.132723149041722	1.25504624572232\\
0.185490527936491	1.21514474409276\\
0.238257906831258	1.17903281518511\\
0.291025285726027	1.14660626259592\\
0.37017635406818	1.10378652887061\\
0.449327422410331	1.06716912796858\\
0.528478490752484	1.03588401623812\\
0.607629559094637	1.00919745316538\\
0.686780627436789	0.986433614716409\\
0.765931695778942	0.967075807813723\\
0.871466453568479	0.945674969636187\\
0.977001211358015	0.92864975616177\\
1.10891965859494	0.911902678678201\\
1.26722179527924	0.897059059026075\\
1.42552393196355	0.886495314643067\\
1.61020975809524	0.877858287298746\\
1.8476629631217	0.870774714037637\\
1.90043034201646	0.869620607252823\\
1.90043034201646	1.73781847817045\\
1.9787403297273	1.63634965049487\\
2.05182965159075	1.54815852915242\\
2.11969830760681	1.47256820172365\\
2.18234629777547	1.408447514342\\
2.24499428794414	1.34976906947882\\
2.30764227811281	1.29639024331351\\
2.37029026828148	1.24806441594557\\
2.42249692675537	1.21143487190123\\
2.42249692675537	2.18867912973402\\
2.44746720640466	2.13311933832279\\
2.44746720640466	3.12043253147227\\
2.50952844946871	2.89335294993555\\
2.56272380066646	2.71234101406642\\
2.61591915186421	2.54413020389973\\
2.66911450306197	2.38860925176493\\
2.72230985425972	2.2454275866799\\
2.77550520545747	2.1140226650915\\
2.82870055665522	1.99389510216361\\
2.88189590785298	1.88430622479683\\
2.93509125905073	1.78453556554018\\
2.98828661024848	1.69385344790517\\
3.04148196144623	1.61153472790433\\
3.09467731264399	1.53689216196485\\
3.14787266384174	1.4692809593095\\
3.20106801503949	1.40811251777546\\
3.25426336623724	1.35279877687352\\
3.307458717435	1.30285553038754\\
3.33405639303387	1.27972028764586\\
3.33405639303387	2.30784472264997\\
3.38378996649834	2.18549360405635\\
3.45010139778431	2.03502747347166\\
3.50397943570415	1.92330619953146\\
3.5412796158025	1.85149854233963\\
3.5412796158025	2.9115278198889\\
3.59128625542778	2.73523757539145\\
3.64534748745511	2.55828479692522\\
3.67643269587083	2.46316158535424\\
3.67643269587083	3.55221375020413\\
3.72042571296461	3.34740495243255\\
3.77419495607923	3.11427155256451\\
3.82552014268864	2.90845903035119\\
3.87440127279284	2.72801814935172\\
3.92083834639183	2.57009615849102\\
3.92083834639183	3.69614407546868\\
3.97037865679034	3.44603658321921\\
3.98052546735389	3.39724216449024\\
3.98052546735389	4.53332856451765\\
4.02545287745246	4.24188351574164\\
4.06833813254654	3.98230568883471\\
4.11939200765854	3.69508849025168\\
4.16840372776606	3.44222763487089\\
4.1847409678019	3.36270421734607\\
4.1847409678019	4.52580016606695\\
4.22781596843031	4.23933184293756\\
4.22781596843031	5.40825248890259\\
4.23637321351316	5.33575800386436\\
4.23637321351316	6.50628655381164\\
4.28491184586282	6.01576448688568\\
4.30473748442818	5.82645652856257\\
4.30473748442818	7.01048623548394\\
4.35306177843114	6.47508409490327\\
4.35455634422504	6.45921293356304\\
4.35455634422504	7.65238065688625\\
4.39558947392673	7.15265433857733\\
4.44944545666019	6.54590395325705\\
4.5007368687873	6.01485588455061\\
4.54946371030806	5.55301606945879\\
4.59562598122245	5.15202165788111\\
4.61101340486059	5.0258097467564\\
4.61101340486059	6.24304074155269\\
4.65433233085422	5.81548710145268\\
4.70362628112283	5.36501992304711\\
4.74993271925396	4.97725752642647\\
4.76038901173518	4.89426005764853\\
4.76038901173518	6.11574252910148\\
4.80795365430729	5.65418718963435\\
4.85551829687939	5.23082238147531\\
4.9030829394515	4.84339839864803\\
4.95064758202361	4.4892517987246\\
4.99821222459572	4.16599216431677\\
5.04577686716783	3.87089648125506\\
5.09334150973994	3.60161677090597\\
5.14090615231205	3.35589963123832\\
5.18847079488416	3.13173973627821\\
5.23603543745626	2.92729887413525\\
5.23603543745626	4.12288214902003\\
5.28676526687569	3.81770700707876\\
5.33115386761768	3.57266074881556\\
5.37554246835968	3.34690392274435\\
5.4262722977791	3.11080972109396\\
5.47700212719852	2.89651163982888\\
5.52139072794051	2.72557446508336\\
5.56577932868251	2.5685770361815\\
5.6101679294245	2.42458140906736\\
5.6545565301665	2.29248306196593\\
5.69894513090849	2.17127797000389\\
5.74333373165049	2.06011062773186\\
5.79406356106991	1.94426645238354\\
5.84479339048933	1.83934324810642\\
5.87015830519904	1.79066790013262\\
5.87015830519904	2.91197420911231\\
5.91752967941962	2.73698686773194\\
5.9649010536402	2.57514190299796\\
6.01227242786078	2.42583647460696\\
6.05964380208136	2.28869572652507\\
6.10701517630194	2.16275411847468\\
6.15438655052251	2.04721666433894\\
6.20175792474309	1.94167446025704\\
6.24912929896367	1.84505475950115\\
6.29650067318425	1.75679702799113\\
6.34387204740483	1.6762119964719\\
6.39124342162541	1.60262209435072\\
6.43861479584599	1.53548637156504\\
6.48598617006657	1.4741794408191\\
6.54283181913126	1.40771678140459\\
6.59967746819596	1.34819213558298\\
6.65652311726065	1.29493855957946\\
6.71336876632535	1.24734306377129\\
6.77021441539004	1.20477731103983\\
6.81758578961062	1.17279557960359\\
6.81758578961062	2.18000873885863\\
6.8422516438123	2.12396704061418\\
6.8422516438123	3.13877425896271\\
6.89927430659525	2.92377042258789\\
6.95629696937819	2.72451002157598\\
7.01331963216112	2.54105577924997\\
7.06083851781358	2.40001033538667\\
7.10835740346603	2.26930883228442\\
7.15587628911848	2.14847105045364\\
7.20339517477093	2.03710476984946\\
7.25091406042338	1.93457166772615\\
7.29843294607583	1.84039080452548\\
7.34595183172828	1.75394434031225\\
7.39347071738073	1.6746848791446\\
7.44098960303318	1.60209480996957\\
7.48850848868563	1.5356256826037\\
7.53602737433808	1.47485434635915\\
7.59305003712102	1.40875255179061\\
7.65007269990396	1.34949360607751\\
7.7070953626869	1.29636522479296\\
7.76411802546984	1.24880220507176\\
7.79262935686131	1.22690858174737\\
7.79262935686131	2.24475586785121\\
7.84971145022074	2.11094818332578\\
7.90679354358016	1.9876632003168\\
7.95753318212187	1.88675570692997\\
8.00827282066358	1.7937292268806\\
8.0590124592053	1.70816938376499\\
8.10975209774701	1.62975664414427\\
8.16049173628872	1.55802040340335\\
8.21123137483043	1.49249754278358\\
8.26197101337214	1.43271982626196\\
8.31905310673157	1.37179094368543\\
8.37613520009099	1.31698905592539\\
8.4268748386327	1.27296518861459\\
8.4268748386327	2.29359822041823\\
8.47981713284744	2.16639668733114\\
8.53275942706219	2.04797970889219\\
8.58570172127692	1.93810871505248\\
8.63864401549166	1.83677192861978\\
8.69158630970641	1.74373740546942\\
8.74452860392115	1.65867411606534\\
8.79747089813589	1.58115160453629\\
8.85041319235063	1.51056683853187\\
8.90335548656537	1.44650975699933\\
8.95629778078011	1.38840840800225\\
9.00924007499485	1.33578996109787\\
9.06218236920959	1.28817433764259\\
9.11512466342433	1.24509171789274\\
9.16806695763907	1.20617810708561\\
9.22100925185381	1.17100268989817\\
9.27395154606855	1.13928406103412\\
9.32689384028329	1.11068734299063\\
9.37983613449803	1.08505403904236\\
9.43277842871277	1.06195969728532\\
9.48572072292751	1.04108051247425\\
9.591605311357	1.00563254913293\\
9.69748989978648	0.976795328251036\\
9.80337448821596	0.953730088239428\\
9.90925907664544	0.934937063986698\\
10.0151436650749	0.919943668455284\\
};

==> fig7_part1c_220209.tex <==
\pgfplotsset{my plot options/.style={color=red, line width=0.5pt, opacity = 0.07, forget plot}}
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0552014411519011	0\\
0.0552014411519011	1\\
0.641129787086722	1\\
0.641129787086722	2\\
0.730811042603747	2\\
0.730811042603747	3\\
0.803361385610252	3\\
0.803361385610252	4\\
1.11642619765648	4\\
1.11642619765648	5\\
1.19012140034457	5\\
1.19012140034457	6\\
1.48762321497222	6\\
1.48762321497222	7\\
1.7594533091669	7\\
1.7594533091669	8\\
2.16542060510017	8\\
2.16542060510017	9\\
2.19132464055584	9\\
2.19132464055584	10\\
2.23753154641486	10\\
2.23753154641486	11\\
2.55083292058145	11\\
2.55083292058145	12\\
2.59285357283553	12\\
2.59285357283553	13\\
2.67166970354059	13\\
2.67166970354059	14\\
2.75115591927027	14\\
2.75115591927027	15\\
4.37858382600226	15\\
4.37858382600226	16\\
6.39803418052517	16\\
6.39803418052517	17\\
6.82807669398506	17\\
6.82807669398506	18\\
7.83351348227965	18\\
7.83351348227965	19\\
9.19484018857953	19\\
9.19484018857953	20\\
11.1660725439894	20\\
11.1660725439894	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0523081136738135	0\\
0.0523081136738135	1\\
1.00953324845823	1\\
1.00953324845823	2\\
1.48423849970277	2\\
1.48423849970277	3\\
3.07494553618184	3\\
3.07494553618184	4\\
3.54932041418036	4\\
3.54932041418036	5\\
4.82313997153194	5\\
4.82313997153194	6\\
4.86896507579868	6\\
4.86896507579868	7\\
5.15343602211519	7\\
5.15343602211519	8\\
5.21471407965828	8\\
5.21471407965828	9\\
6.53901094692752	9\\
6.53901094692752	10\\
9.38382225092466	10\\
9.38382225092466	11\\
9.478171901595	11\\
9.478171901595	12\\
9.59082183763682	12\\
9.59082183763682	13\\
9.86850234387708	13\\
9.86850234387708	14\\
9.89492037159717	14\\
9.89492037159717	15\\
10.9883265947253	15\\
10.9883265947253	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.496603112529591	0\\
0.496603112529591	1\\
1.24210236256199	1\\
1.24210236256199	2\\
1.88283383047363	2\\
1.88283383047363	3\\
1.99357941758366	3\\
1.99357941758366	4\\
2.15705194357483	4\\
2.15705194357483	5\\
2.28268437809553	5\\
2.28268437809553	6\\
3.30418758723502	6\\
3.30418758723502	7\\
3.41946422714483	7\\
3.41946422714483	8\\
4.01866204079632	8\\
4.01866204079632	9\\
6.85471619982468	9\\
6.85471619982468	10\\
10.7467656077099	10\\
10.7467656077099	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.49527647914121	0\\
1.49527647914121	1\\
1.53503916493639	1\\
1.53503916493639	2\\
1.83751980149212	2\\
1.83751980149212	3\\
1.99612396129453	3\\
1.99612396129453	4\\
6.61438757715195	4\\
6.61438757715195	5\\
7.61957799397872	5\\
7.61957799397872	6\\
8.67174117889904	6\\
8.67174117889904	7\\
8.85767135813828	7\\
8.85767135813828	8\\
9.11634083090208	8\\
9.11634083090208	9\\
9.17668106054603	9\\
9.17668106054603	10\\
9.62944485292957	10\\
9.62944485292957	11\\
11.598038742324	11\\
11.598038742324	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.02841790652971	0\\
1.02841790652971	1\\
1.04092531261983	1\\
1.04092531261983	2\\
1.40495617954746	2\\
1.40495617954746	3\\
1.5226739645443	3\\
1.5226739645443	4\\
1.6408775407112	4\\
1.6408775407112	5\\
1.8395537745213	5\\
1.8395537745213	6\\
1.86334711594494	6\\
1.86334711594494	7\\
1.88982987971651	7\\
1.88982987971651	8\\
1.90173576039291	8\\
1.90173576039291	9\\
2.40549814728696	9\\
2.40549814728696	10\\
2.48312792311848	10\\
2.48312792311848	11\\
2.63109249608193	11\\
2.63109249608193	12\\
3.48535461408293	12\\
3.48535461408293	13\\
3.60901217408879	13\\
3.60901217408879	14\\
4.47681193195562	14\\
4.47681193195562	15\\
4.64438473702584	15\\
4.64438473702584	16\\
5.09930155860014	16\\
5.09930155860014	17\\
5.11978869681404	17\\
5.11978869681404	18\\
5.15836545749274	18\\
5.15836545749274	19\\
5.20845543435352	19\\
5.20845543435352	20\\
5.28053471386847	20\\
5.28053471386847	21\\
5.41446908915096	21\\
5.41446908915096	22\\
5.50158796805439	22\\
5.50158796805439	23\\
5.74038041364772	23\\
5.74038041364772	24\\
5.88278910966908	24\\
5.88278910966908	25\\
5.93144554020717	25\\
5.93144554020717	26\\
6.02301537347186	26\\
6.02301537347186	27\\
7.15432563681613	27\\
7.15432563681613	28\\
7.64460292358927	28\\
7.64460292358927	29\\
9.01617597732508	29\\
9.01617597732508	30\\
10.7087621031215	30\\
10.7087621031215	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.674870040725345	0\\
0.674870040725345	1\\
1.52564549307209	1\\
1.52564549307209	2\\
1.57398170981203	2\\
1.57398170981203	3\\
1.75667291922014	3\\
1.75667291922014	4\\
1.76144214519272	4\\
1.76144214519272	5\\
1.96462560455144	5\\
1.96462560455144	6\\
2.22201810122501	6\\
2.22201810122501	7\\
2.27646697134248	7\\
2.27646697134248	8\\
4.12220503767739	8\\
4.12220503767739	9\\
4.4955603258744	9\\
4.4955603258744	10\\
5.98460818259591	10\\
5.98460818259591	11\\
6.80689003138882	11\\
6.80689003138882	12\\
6.82758582991775	12\\
6.82758582991775	13\\
6.85130784156673	13\\
6.85130784156673	14\\
7.57572715480644	14\\
7.57572715480644	15\\
8.58707775682117	15\\
8.58707775682117	16\\
11.8139135660601	16\\
11.8139135660601	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.35143980524168	0\\
1.35143980524168	1\\
1.53061167626013	1\\
1.53061167626013	2\\
1.67233281708138	2\\
1.67233281708138	3\\
1.90087640622773	3\\
1.90087640622773	4\\
2.95421679944866	4\\
2.95421679944866	5\\
2.95842797472795	5\\
2.95842797472795	6\\
3.64177193937889	6\\
3.64177193937889	7\\
6.25722255204578	7\\
6.25722255204578	8\\
7.09403542228484	8\\
7.09403542228484	9\\
7.18080875734919	9\\
7.18080875734919	10\\
7.88657441275049	10\\
7.88657441275049	11\\
7.94731506415882	11\\
7.94731506415882	12\\
8.02314570843491	12\\
8.02314570843491	13\\
8.05409199876305	13\\
8.05409199876305	14\\
8.06148671751164	14\\
8.06148671751164	15\\
8.36372102481699	15\\
8.36372102481699	16\\
8.56207183679642	16\\
8.56207183679642	17\\
9.1644501754399	17\\
9.1644501754399	18\\
9.42674603676507	18\\
9.42674603676507	19\\
10.1987064948783	19\\
10.1987064948783	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.699372072302253	0\\
0.699372072302253	1\\
0.885761184392159	1\\
0.885761184392159	2\\
0.934593913614599	2\\
0.934593913614599	3\\
1.13785223310591	3\\
1.13785223310591	4\\
1.48065070403173	4\\
1.48065070403173	5\\
1.5659342269148	5\\
1.5659342269148	6\\
1.67758759594319	6\\
1.67758759594319	7\\
3.85572356526928	7\\
3.85572356526928	8\\
4.58025236047971	8\\
4.58025236047971	9\\
5.23631666902705	9\\
5.23631666902705	10\\
5.542782291523	10\\
5.542782291523	11\\
7.00010202841927	11\\
7.00010202841927	12\\
7.35881097468306	12\\
7.35881097468306	13\\
7.53044905150027	13\\
7.53044905150027	14\\
7.54741639799749	14\\
7.54741639799749	15\\
7.55282130016676	15\\
7.55282130016676	16\\
7.64097318318482	16\\
7.64097318318482	17\\
7.75542007060473	17\\
7.75542007060473	18\\
7.85757048133112	18\\
7.85757048133112	19\\
7.94018217138176	19\\
7.94018217138176	20\\
8.09877192367075	20\\
8.09877192367075	21\\
8.19706714280281	21\\
8.19706714280281	22\\
8.24382047795451	22\\
8.24382047795451	23\\
8.26203818839953	23\\
8.26203818839953	24\\
8.32907672152809	24\\
8.32907672152809	25\\
8.39014891324639	25\\
8.39014891324639	26\\
8.51652063386062	26\\
8.51652063386062	27\\
8.5450076718493	27\\
8.5450076718493	28\\
8.62531098473094	28\\
8.62531098473094	29\\
8.80152772798056	29\\
8.80152772798056	30\\
9.11606128148292	30\\
9.11606128148292	31\\
9.24808587749062	31\\
9.24808587749062	32\\
9.44618115714407	32\\
9.44618115714407	33\\
9.50387968371319	33\\
9.50387968371319	34\\
9.53335090382558	34\\
9.53335090382558	35\\
9.60390123743199	35\\
9.60390123743199	36\\
9.61932064133981	36\\
9.61932064133981	37\\
9.69679728840085	37\\
9.69679728840085	38\\
9.9013155698368	38\\
9.9013155698368	39\\
10.0154181000033	39\\
10.0154181000033	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.922439341997105	0\\
0.922439341997105	1\\
1.34860749687313	1\\
1.34860749687313	2\\
2.14839691025239	2\\
2.14839691025239	3\\
4.10258445234396	3\\
4.10258445234396	4\\
4.84869395225525	4\\
4.84869395225525	5\\
5.40434002255333	5\\
5.40434002255333	6\\
5.42202785689418	6\\
5.42202785689418	7\\
5.6016641706932	7\\
5.6016641706932	8\\
6.4446795867014	8\\
6.4446795867014	9\\
6.49891338257965	9\\
6.49891338257965	10\\
6.51055663950077	10\\
6.51055663950077	11\\
6.85215412164938	11\\
6.85215412164938	12\\
7.19485572311364	12\\
7.19485572311364	13\\
7.85075162263801	13\\
7.85075162263801	14\\
8.75092115064929	14\\
8.75092115064929	15\\
10.239145200537	15\\
10.239145200537	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.49709300068103	0\\
1.49709300068103	1\\
1.64973862644223	1\\
1.64973862644223	2\\
1.84688681611538	2\\
1.84688681611538	3\\
1.98237476525678	3\\
1.98237476525678	4\\
2.70853282753443	4\\
2.70853282753443	5\\
2.8816918023452	5\\
2.8816918023452	6\\
3.01014245865161	6\\
3.01014245865161	7\\
3.06015127432951	7\\
3.06015127432951	8\\
3.18078396978999	8\\
3.18078396978999	9\\
3.47877532699535	9\\
3.47877532699535	10\\
3.61865975594164	10\\
3.61865975594164	11\\
5.02964453787262	11\\
5.02964453787262	12\\
5.61284562513431	12\\
5.61284562513431	13\\
5.80380088854866	13\\
5.80380088854866	14\\
5.85582324880444	14\\
5.85582324880444	15\\
5.8785833846927	15\\
5.8785833846927	16\\
6.02505727781357	16\\
6.02505727781357	17\\
6.04828564621022	17\\
6.04828564621022	18\\
6.74045082206279	18\\
6.74045082206279	19\\
6.98102819608881	19\\
6.98102819608881	20\\
7.00037553173689	20\\
7.00037553173689	21\\
7.08582040627455	21\\
7.08582040627455	22\\
7.13974813634071	22\\
7.13974813634071	23\\
7.17665838131057	23\\
7.17665838131057	24\\
7.23742342190017	24\\
7.23742342190017	25\\
7.39540785408613	25\\
7.39540785408613	26\\
7.4358137002679	26\\
7.4358137002679	27\\
7.4444090249801	27\\
7.4444090249801	28\\
7.48698639667617	28\\
7.48698639667617	29\\
7.53564774772364	29\\
7.53564774772364	30\\
7.6139882384385	30\\
7.6139882384385	31\\
7.66488476247755	31\\
7.66488476247755	32\\
7.85487460920019	32\\
7.85487460920019	33\\
8.04381280267077	33\\
8.04381280267077	34\\
8.34956780380966	34\\
8.34956780380966	35\\
8.35582739664513	35\\
8.35582739664513	36\\
8.58296390631356	36\\
8.58296390631356	37\\
8.75685305771406	37\\
8.75685305771406	38\\
8.78410577632965	38\\
8.78410577632965	39\\
8.96983433265147	39\\
8.96983433265147	40\\
9.28289594575097	40\\
9.28289594575097	41\\
9.48188733747866	41\\
9.48188733747866	42\\
10.2336207950042	42\\
10.2336207950042	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.511215450893705	0\\
0.511215450893705	1\\
0.875952064368914	1\\
0.875952064368914	2\\
3.56789092803792	2\\
3.56789092803792	3\\
3.99775991565908	3\\
3.99775991565908	4\\
4.34111496517132	4\\
4.34111496517132	5\\
4.8235293832213	5\\
4.8235293832213	6\\
5.19695085688093	6\\
5.19695085688093	7\\
5.19783874069638	8\\
5.50561704194216	8\\
5.50561704194216	9\\
5.54332115600618	9\\
5.54332115600618	10\\
5.5933294705417	10\\
5.5933294705417	11\\
5.64031912359663	11\\
5.64031912359663	12\\
5.70420672068118	12\\
5.70420672068118	13\\
5.77478081954338	13\\
5.77478081954338	14\\
6.00712379819591	14\\
6.00712379819591	15\\
6.24774996488953	15\\
6.24774996488953	16\\
6.50174026065084	16\\
6.50174026065084	17\\
6.76695682864022	17\\
6.76695682864022	18\\
7.21607126107621	18\\
7.21607126107621	19\\
7.28980256946964	19\\
7.28980256946964	20\\
7.38657587963919	20\\
7.38657587963919	21\\
7.50142354792348	21\\
7.50142354792348	22\\
7.65287974948937	22\\
7.65287974948937	23\\
8.09294547245113	23\\
8.09294547245113	24\\
8.58786485839526	24\\
8.58786485839526	25\\
8.93699510454286	25\\
8.93699510454286	26\\
9.52639691325721	26\\
9.52639691325721	27\\
9.98372288381844	27\\
9.98372288381844	28\\
10.3211108826203	28\\
10.3211108826203	29\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.245632008275917	0\\
0.245632008275917	1\\
1.39264366160901	1\\
1.39264366160901	2\\
2.16738784240795	2\\
2.16738784240795	3\\
3.63632413519367	3\\
3.63632413519367	4\\
3.86541609651771	4\\
3.86541609651771	5\\
4.1248685701029	5\\
4.1248685701029	6\\
4.1406400822537	6\\
4.1406400822537	7\\
4.18864376098339	7\\
4.18864376098339	8\\
5.58873684299815	8\\
5.58873684299815	9\\
8.66152522725587	9\\
8.66152522725587	10\\
9.98063419215243	10\\
9.98063419215243	11\\
10.4998617253929	11\\
10.4998617253929	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.18412090357767	0\\
2.18412090357767	1\\
2.89101539338363	1\\
2.89101539338363	2\\
3.96697023137662	2\\
3.96697023137662	3\\
4.23749722172049	3\\
4.23749722172049	4\\
4.51933520841484	4\\
4.51933520841484	5\\
4.6599200044553	5\\
4.6599200044553	6\\
4.6772470107132	6\\
4.6772470107132	7\\
4.79457222849494	7\\
4.79457222849494	8\\
4.8650939851938	8\\
4.8650939851938	9\\
5.0176654505925	9\\
5.0176654505925	10\\
5.3163636647099	10\\
5.3163636647099	11\\
5.41297655961205	11\\
5.41297655961205	12\\
5.8192486094948	12\\
5.8192486094948	13\\
5.8423381017578	13\\
5.8423381017578	14\\
5.88657177701519	14\\
5.88657177701519	15\\
5.90568341409636	15\\
5.90568341409636	16\\
6.01166989196486	16\\
6.01166989196486	17\\
6.99202040706295	17\\
6.99202040706295	18\\
7.02509789834038	18\\
7.02509789834038	19\\
7.16070684805872	19\\
7.16070684805872	20\\
7.38675058109212	20\\
7.38675058109212	21\\
7.59241712605539	21\\
7.59241712605539	22\\
8.06003961649721	22\\
8.06003961649721	23\\
8.11404365665356	23\\
8.11404365665356	24\\
8.1925074837138	24\\
8.1925074837138	25\\
8.2895676077579	25\\
8.2895676077579	26\\
8.46639336822629	26\\
8.46639336822629	27\\
8.66274536081232	27\\
8.66274536081232	28\\
8.71571956136833	28\\
8.71571956136833	29\\
8.78651718694535	29\\
8.78651718694535	30\\
9.0720137318035	30\\
9.0720137318035	31\\
9.1915420208858	31\\
9.1915420208858	32\\
9.30081531082077	32\\
9.30081531082077	33\\
9.37190610556996	33\\
9.37190610556996	34\\
9.41704733176411	34\\
9.41704733176411	35\\
9.4766399413927	35\\
9.4766399413927	36\\
9.56758906646516	36\\
9.56758906646516	37\\
9.62119406670434	37\\
9.62119406670434	38\\
9.72138671213578	38\\
9.72138671213578	39\\
10.253022868118	39\\
10.253022868118	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.636058905557448	0\\
0.636058905557448	1\\
2.8911340394808	1\\
2.8911340394808	2\\
3.32317470085616	2\\
3.32317470085616	3\\
4.26187594666464	3\\
4.26187594666464	4\\
4.64398547525586	4\\
4.64398547525586	5\\
5.13298244060929	5\\
5.13298244060929	6\\
5.1629526028806	6\\
5.1629526028806	7\\
6.22400590880886	7\\
6.22400590880886	8\\
6.77254132524492	8\\
6.77254132524492	9\\
7.01047462774731	9\\
7.01047462774731	10\\
9.40648321080967	10\\
9.40648321080967	11\\
9.56248098681333	11\\
9.56248098681333	12\\
12.895834687588	12\\
12.895834687588	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.53541912156529	0\\
0.53541912156529	1\\
0.604773585987914	1\\
0.604773585987914	2\\
0.621508732711703	2\\
0.621508732711703	3\\
0.894229434116209	3\\
0.894229434116209	4\\
1.17775882233511	4\\
1.17775882233511	5\\
4.66318769537759	5\\
4.66318769537759	6\\
4.75748007741775	6\\
4.75748007741775	7\\
5.09958930919697	7\\
5.09958930919697	8\\
7.40649334228171	8\\
7.40649334228171	9\\
7.47487619861438	9\\
7.47487619861438	10\\
7.5501417885537	10\\
7.5501417885537	11\\
7.63991850594469	11\\
7.63991850594469	12\\
7.66757565212487	12\\
7.66757565212487	13\\
7.79066656846617	13\\
7.79066656846617	14\\
7.9833398477707	14\\
7.9833398477707	15\\
8.05562222203964	15\\
8.05562222203964	16\\
8.06084698798518	16\\
8.06084698798518	17\\
8.18917766825882	17\\
8.18917766825882	18\\
8.37243051583506	18\\
8.37243051583506	19\\
8.63187624167536	19\\
8.63187624167536	20\\
10.3309931425367	20\\
10.3309931425367	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.210556530578694	0\\
0.210556530578694	1\\
0.256240263212989	1\\
0.256240263212989	2\\
0.555985218205031	2\\
0.555985218205031	3\\
0.911457089144488	3\\
0.911457089144488	4\\
1.46804676822728	4\\
1.46804676822728	5\\
2.10435332813422	5\\
2.10435332813422	6\\
2.36056967764529	6\\
2.36056967764529	7\\
2.37554977423862	7\\
2.37554977423862	8\\
2.92501413406949	8\\
2.92501413406949	9\\
2.9287195616959	10\\
3.25932481859121	10\\
3.25932481859121	11\\
3.95123535107913	11\\
3.95123535107913	12\\
5.29175362856895	12\\
5.29175362856895	13\\
7.58356220062788	13\\
7.58356220062788	14\\
12.0983209112321	14\\
12.0983209112321	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
4.5287038131988	0\\
4.5287038131988	1\\
4.56819408393678	1\\
4.56819408393678	2\\
4.62484210698481	2\\
4.62484210698481	3\\
5.00093021009582	3\\
5.00093021009582	4\\
5.79597714814779	4\\
5.79597714814779	5\\
6.52658662563204	5\\
6.52658662563204	6\\
6.86828302526893	6\\
6.86828302526893	7\\
7.2406270019946	7\\
7.2406270019946	8\\
7.49128706725827	8\\
7.49128706725827	9\\
7.54025959052063	9\\
7.54025959052063	10\\
7.84083219281727	10\\
7.84083219281727	11\\
8.18850087305362	11\\
8.18850087305362	12\\
8.25394834398694	12\\
8.25394834398694	13\\
8.31564995428198	13\\
8.31564995428198	14\\
8.44095561509405	14\\
8.44095561509405	15\\
8.5919549386282	15\\
8.5919549386282	16\\
8.93800669912489	16\\
8.93800669912489	17\\
9.26001907551187	17\\
9.26001907551187	18\\
9.4328614727193	18\\
9.4328614727193	19\\
9.53294325494875	19\\
9.53294325494875	20\\
9.57978848061582	20\\
9.57978848061582	21\\
11.9612929335053	21\\
11.9612929335053	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0591672431911086	0\\
0.0591672431911086	1\\
0.248644842319081	1\\
0.248644842319081	2\\
0.402155218867634	2\\
0.402155218867634	3\\
0.486814577156217	3\\
0.486814577156217	4\\
0.502670684803153	4\\
0.502670684803153	5\\
0.705870728210456	5\\
0.705870728210456	6\\
2.38296432481038	6\\
2.38296432481038	7\\
2.49255897625792	7\\
2.49255897625792	8\\
3.114330813787	8\\
3.114330813787	9\\
3.14528885707134	9\\
3.14528885707134	10\\
3.17166846852756	10\\
3.17166846852756	11\\
3.2853323680763	11\\
3.2853323680763	12\\
3.46978747213065	12\\
3.46978747213065	13\\
3.57894765336631	13\\
3.57894765336631	14\\
3.81748671512491	14\\
3.81748671512491	15\\
3.87586554155227	15\\
3.87586554155227	16\\
4.00852229263803	16\\
4.00852229263803	17\\
4.16295719311328	17\\
4.16295719311328	18\\
5.74944476594318	18\\
5.74944476594318	19\\
5.83944280968251	19\\
5.83944280968251	20\\
6.43584853146406	20\\
6.43584853146406	21\\
6.73211451361088	21\\
6.73211451361088	22\\
7.02695238249754	22\\
7.02695238249754	23\\
8.0090134812835	23\\
8.0090134812835	24\\
8.40099753268894	24\\
8.40099753268894	25\\
9.05415445355235	25\\
9.05415445355235	26\\
11.5057042123089	26\\
11.5057042123089	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.01233796506821	0\\
1.01233796506821	1\\
1.19675642334672	1\\
1.19675642334672	2\\
1.30139750981619	2\\
1.30139750981619	3\\
1.39060882195051	3\\
1.39060882195051	4\\
2.94356205319397	4\\
2.94356205319397	5\\
4.03315360697617	5\\
4.03315360697617	6\\
4.03455752963759	7\\
4.56036387305106	7\\
4.56036387305106	8\\
4.61620786921354	8\\
4.61620786921354	9\\
4.62710093961987	9\\
4.62710093961987	10\\
5.33381600511572	10\\
5.33381600511572	11\\
5.6501179902505	11\\
5.6501179902505	12\\
6.40498396033763	12\\
6.40498396033763	13\\
6.76812586208639	13\\
6.76812586208639	14\\
6.9256262506124	14\\
6.9256262506124	15\\
7.34183732939353	15\\
7.34183732939353	16\\
7.57852300284821	16\\
7.57852300284821	17\\
7.69787524572019	17\\
7.69787524572019	18\\
7.78772498174377	18\\
7.78772498174377	19\\
7.8805595107174	19\\
7.8805595107174	20\\
7.91265560357981	20\\
7.91265560357981	21\\
8.05377980970394	21\\
8.05377980970394	22\\
8.15889379445812	22\\
8.15889379445812	23\\
8.23501025696114	23\\
8.23501025696114	24\\
8.63359410563125	24\\
8.63359410563125	25\\
8.9858940261414	25\\
8.9858940261414	26\\
11.7617757099113	26\\
11.7617757099113	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.987523853445769	0\\
0.987523853445769	1\\
1.42905155048325	1\\
1.42905155048325	2\\
1.72582104194234	2\\
1.72582104194234	3\\
1.8281527782816	3\\
1.8281527782816	4\\
1.84933129927101	4\\
1.84933129927101	5\\
1.93651104412412	5\\
1.93651104412412	6\\
1.96228485546946	6\\
1.96228485546946	7\\
2.04896920745183	7\\
2.04896920745183	8\\
2.09663638340236	8\\
2.09663638340236	9\\
2.11597683949331	9\\
2.11597683949331	10\\
2.11956417827679	11\\
2.13465356974961	11\\
2.13465356974961	12\\
2.6643634024309	12\\
2.6643634024309	13\\
2.76591875301774	13\\
2.76591875301774	14\\
4.33961271961552	14\\
4.33961271961552	15\\
7.89637048294966	15\\
7.89637048294966	16\\
7.90189194422939	16\\
7.90189194422939	17\\
9.29431299031524	17\\
9.29431299031524	18\\
9.45512221702318	18\\
9.45512221702318	19\\
9.48799987860126	19\\
9.48799987860126	20\\
9.93309591995565	20\\
9.93309591995565	21\\
10.1613637939538	21\\
10.1613637939538	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0484546296577832	0\\
0.0484546296577832	1\\
0.141522700751626	1\\
0.141522700751626	2\\
0.231948538249661	2\\
0.231948538249661	3\\
0.867341682080852	3\\
0.867341682080852	4\\
0.969318265937027	4\\
0.969318265937027	5\\
1.05832523977521	5\\
1.05832523977521	6\\
3.28925262102355	6\\
3.28925262102355	7\\
3.46747710582011	7\\
3.46747710582011	8\\
4.46493895345818	8\\
4.46493895345818	9\\
4.81092067737402	9\\
4.81092067737402	10\\
4.8328426693432	10\\
4.8328426693432	11\\
7.94012468156878	11\\
7.94012468156878	12\\
8.10485855474683	12\\
8.10485855474683	13\\
8.55334847692155	13\\
8.55334847692155	14\\
8.68412605732606	14\\
8.68412605732606	15\\
8.76926711532754	15\\
8.76926711532754	16\\
9.22308563826531	16\\
9.22308563826531	17\\
9.22429241745804	18\\
9.27737273402784	18\\
9.27737273402784	19\\
9.3492518461881	19\\
9.3492518461881	20\\
9.45517757374979	20\\
9.45517757374979	21\\
9.79010506380795	21\\
9.79010506380795	22\\
9.86140558034887	22\\
9.86140558034887	23\\
10.1233305750804	23\\
10.1233305750804	24\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.598427273805932	0\\
0.598427273805932	1\\
0.638105140341018	1\\
0.638105140341018	2\\
1.83154891220704	2\\
1.83154891220704	3\\
2.18241804656098	3\\
2.18241804656098	4\\
2.63429853719804	4\\
2.63429853719804	5\\
2.6387196024115	5\\
2.6387196024115	6\\
2.73767199416604	6\\
2.73767199416604	7\\
2.8836013039735	7\\
2.8836013039735	8\\
2.97875763237778	8\\
2.97875763237778	9\\
3.06286802382258	9\\
3.06286802382258	10\\
3.06743947469202	10\\
3.06743947469202	11\\
3.37051958842223	11\\
3.37051958842223	12\\
3.46131543849657	12\\
3.46131543849657	13\\
4.0837186999665	13\\
4.0837186999665	14\\
4.20142726971949	14\\
4.20142726971949	15\\
4.46658273173936	15\\
4.46658273173936	16\\
6.41318163394754	16\\
6.41318163394754	17\\
7.26563992540232	17\\
7.26563992540232	18\\
10.7838858638366	18\\
10.7838858638366	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.88029539306493	0\\
1.88029539306493	1\\
2.0928986588266	1\\
2.0928986588266	2\\
2.1479233732631	2\\
2.1479233732631	3\\
2.25117806147327	3\\
2.25117806147327	4\\
2.48206560638461	4\\
2.48206560638461	5\\
2.59257874451621	5\\
2.59257874451621	6\\
2.77665601534105	6\\
2.77665601534105	7\\
2.98441609458127	7\\
2.98441609458127	8\\
3.05825025544669	8\\
3.05825025544669	9\\
3.23438971026269	9\\
3.23438971026269	10\\
3.36187642657487	10\\
3.36187642657487	11\\
3.37438856404177	11\\
3.37438856404177	12\\
3.4385931496753	12\\
3.4385931496753	13\\
3.80838614652814	13\\
3.80838614652814	14\\
6.43404989922112	14\\
6.43404989922112	15\\
8.06350138445322	15\\
8.06350138445322	16\\
8.18596009093553	16\\
8.18596009093553	17\\
11.0912577421606	17\\
11.0912577421606	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.959411435407326	0\\
0.959411435407326	1\\
1.88505229632526	1\\
1.88505229632526	2\\
2.12244333932413	2\\
2.12244333932413	3\\
2.40827962370804	3\\
2.40827962370804	4\\
3.01489826829668	4\\
3.01489826829668	5\\
3.65836438801071	5\\
3.65836438801071	6\\
4.47373265227306	6\\
4.47373265227306	7\\
6.26407625196321	7\\
6.26407625196321	8\\
6.45948504095118	8\\
6.45948504095118	9\\
6.46124392376196	10\\
6.61211765135187	10\\
6.61211765135187	11\\
8.32606596114752	11\\
8.32606596114752	12\\
9.21899380404222	12\\
9.21899380404222	13\\
10.9246535699788	13\\
10.9246535699788	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.208764030044957	0\\
0.208764030044957	1\\
0.652338694664301	1\\
0.652338694664301	2\\
0.748722587493027	2\\
0.748722587493027	3\\
0.749107928816859	4\\
0.915070872587894	4\\
0.915070872587894	5\\
1.12751183045061	5\\
1.12751183045061	6\\
3.31590055517694	6\\
3.31590055517694	7\\
3.37780098418073	7\\
3.37780098418073	8\\
3.41406503903047	8\\
3.41406503903047	9\\
3.87127927242868	9\\
3.87127927242868	10\\
5.16479738966482	10\\
5.16479738966482	11\\
7.21435748408776	11\\
7.21435748408776	12\\
7.25139405589815	12\\
7.25139405589815	13\\
7.28055379032588	13\\
7.28055379032588	14\\
7.81603600246594	14\\
7.81603600246594	15\\
8.28404160598628	15\\
8.28404160598628	16\\
8.52388566893945	16\\
8.52388566893945	17\\
8.93178723723074	17\\
8.93178723723074	18\\
9.15388240584168	18\\
9.15388240584168	19\\
9.60566282471682	19\\
9.60566282471682	20\\
9.68994927958034	20\\
9.68994927958034	21\\
10.1438223686977	21\\
10.1438223686977	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.895417077775601	0\\
0.895417077775601	1\\
1.56607543981311	1\\
1.56607543981311	2\\
4.00846922345836	2\\
4.00846922345836	3\\
4.25946443802879	3\\
4.25946443802879	4\\
5.50842843913005	4\\
5.50842843913005	5\\
7.10339611047124	5\\
7.10339611047124	6\\
8.32408023626608	6\\
8.32408023626608	7\\
8.33028273522922	7\\
8.33028273522922	8\\
8.34081426398183	8\\
8.34081426398183	9\\
10.0432055997276	9\\
10.0432055997276	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.185496607725621	0\\
0.185496607725621	1\\
0.443091585317159	1\\
0.443091585317159	2\\
1.67807066738682	2\\
1.67807066738682	3\\
1.90955752563107	3\\
1.90955752563107	4\\
2.31520605212249	4\\
2.31520605212249	5\\
2.65908303132784	5\\
2.65908303132784	6\\
4.419320186127	6\\
4.419320186127	7\\
5.1090711634967	7\\
5.1090711634967	8\\
6.7871356407595	8\\
6.7871356407595	9\\
7.81669086635442	9\\
7.81669086635442	10\\
7.83637435093526	10\\
7.83637435093526	11\\
8.84552420859077	11\\
8.84552420859077	12\\
9.00870766645182	12\\
9.00870766645182	13\\
9.09324889757006	13\\
9.09324889757006	14\\
9.23455145255727	14\\
9.23455145255727	15\\
9.67883240384135	15\\
9.67883240384135	16\\
9.77759844516033	16\\
9.77759844516033	17\\
10.61532767499	17\\
10.61532767499	18\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0334293371990491	0\\
0.0334293371990491	1\\
0.163271932800964	1\\
0.163271932800964	2\\
0.164274658244139	3\\
0.534245965791314	3\\
0.534245965791314	4\\
1.46384200480771	4\\
1.46384200480771	5\\
1.58789301383646	5\\
1.58789301383646	6\\
1.86415009329153	6\\
1.86415009329153	7\\
2.76796147967766	7\\
2.76796147967766	8\\
4.66123691384811	8\\
4.66123691384811	9\\
5.11217401582062	9\\
5.11217401582062	10\\
6.1700990037742	10\\
6.1700990037742	11\\
6.61962471073373	11\\
6.61962471073373	12\\
6.90386362340526	12\\
6.90386362340526	13\\
7.35211906804092	13\\
7.35211906804092	14\\
7.38312540152898	14\\
7.38312540152898	15\\
7.86720684108924	15\\
7.86720684108924	16\\
8.45295377135283	16\\
8.45295377135283	17\\
8.63722578304434	17\\
8.63722578304434	18\\
9.37241633443034	18\\
9.37241633443034	19\\
9.68822782528975	19\\
9.68822782528975	20\\
9.77224050263683	20\\
9.77224050263683	21\\
9.83755599668136	21\\
9.83755599668136	22\\
9.99095899228391	22\\
9.99095899228391	23\\
10.1007866552649	23\\
10.1007866552649	24\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.608891532572979	0\\
0.608891532572979	1\\
2.22369909359658	1\\
2.22369909359658	2\\
3.5628306495239	2\\
3.5628306495239	3\\
3.69400710296271	3\\
3.69400710296271	4\\
3.79423230435215	4\\
3.79423230435215	5\\
3.83359127103434	5\\
3.83359127103434	6\\
3.84630623506678	6\\
3.84630623506678	7\\
3.88391653873819	7\\
3.88391653873819	8\\
4.01074854578671	8\\
4.01074854578671	9\\
4.12769850358962	9\\
4.12769850358962	10\\
4.16476032039759	10\\
4.16476032039759	11\\
4.3304729489685	11\\
4.3304729489685	12\\
4.67096234111341	12\\
4.67096234111341	13\\
5.30944246137546	13\\
5.30944246137546	14\\
5.79217012239037	14\\
5.79217012239037	15\\
6.39481531119374	15\\
6.39481531119374	16\\
7.14349675022872	16\\
7.14349675022872	17\\
8.39267885156962	17\\
8.39267885156962	18\\
12.6372837252606	18\\
12.6372837252606	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.823996035368939	0\\
0.823996035368939	1\\
5.63243494257412	1\\
5.63243494257412	2\\
7.73786662008614	2\\
7.73786662008614	3\\
7.91034522777463	3\\
7.91034522777463	4\\
8.21527372700019	4\\
8.21527372700019	5\\
8.35159882573162	5\\
8.35159882573162	6\\
8.86440884901316	6\\
8.86440884901316	7\\
9.0360127846077	7\\
9.0360127846077	8\\
9.27871536054391	8\\
9.27871536054391	9\\
10.2491382637335	9\\
10.2491382637335	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0121415652061536	0\\
0.0121415652061536	1\\
0.216251344814534	1\\
0.216251344814534	2\\
1.01351273292393	2\\
1.01351273292393	3\\
2.38585088823712	3\\
2.38585088823712	4\\
2.50397769220832	4\\
2.50397769220832	5\\
2.72658060076508	5\\
2.72658060076508	6\\
2.84805806778641	6\\
2.84805806778641	7\\
3.488687843475	7\\
3.488687843475	8\\
3.68885039480093	8\\
3.68885039480093	9\\
4.15680657632834	9\\
4.15680657632834	10\\
4.23880491320266	10\\
4.23880491320266	11\\
4.58509243266172	11\\
4.58509243266172	12\\
4.65964755342616	12\\
4.65964755342616	13\\
4.67514216463744	13\\
4.67514216463744	14\\
5.40803465144333	14\\
5.40803465144333	15\\
5.87922255445954	15\\
5.87922255445954	16\\
6.90758213924761	16\\
6.90758213924761	17\\
6.93430501728295	17\\
6.93430501728295	18\\
7.14261375601837	18\\
7.14261375601837	19\\
10.1770126841025	19\\
10.1770126841025	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.373282235871297	0\\
0.373282235871297	1\\
0.521664647604208	1\\
0.521664647604208	2\\
1.09627153301933	2\\
1.09627153301933	3\\
2.20845554217672	3\\
2.20845554217672	4\\
2.25437603509594	4\\
2.25437603509594	5\\
2.26354015701828	5\\
2.26354015701828	6\\
2.69674954622293	6\\
2.69674954622293	7\\
2.70618319502959	7\\
2.70618319502959	8\\
2.86744822801069	8\\
2.86744822801069	9\\
2.88667974887759	9\\
2.88667974887759	10\\
3.28538342984406	10\\
3.28538342984406	11\\
3.30843890929639	11\\
3.30843890929639	12\\
3.77629558725934	12\\
3.77629558725934	13\\
3.98428033985832	13\\
3.98428033985832	14\\
4.0815282110035	14\\
4.0815282110035	15\\
4.46303202376857	15\\
4.46303202376857	16\\
4.70511785280804	16\\
4.70511785280804	17\\
4.78484653832319	17\\
4.78484653832319	18\\
5.24178557716203	18\\
5.24178557716203	19\\
5.6158423434345	19\\
5.6158423434345	20\\
6.74533881257759	20\\
6.74533881257759	21\\
7.67310807636105	21\\
7.67310807636105	22\\
7.87749833033842	22\\
7.87749833033842	23\\
7.96293958770554	23\\
7.96293958770554	24\\
8.03674604126443	24\\
8.03674604126443	25\\
9.0826864884871	25\\
9.0826864884871	26\\
9.10939574110881	26\\
9.10939574110881	27\\
9.22550713558447	27\\
9.22550713558447	28\\
9.48830213684258	28\\
9.48830213684258	29\\
9.96408009481666	29\\
9.96408009481666	30\\
10.9598558945831	30\\
10.9598558945831	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.33813729440249	0\\
2.33813729440249	1\\
2.5696313629394	1\\
2.5696313629394	2\\
2.83019433956714	2\\
2.83019433956714	3\\
3.91822742482441	3\\
3.91822742482441	4\\
4.47076182371499	4\\
4.47076182371499	5\\
4.63422101219301	5\\
4.63422101219301	6\\
5.71795573931405	6\\
5.71795573931405	7\\
5.89306901822593	7\\
5.89306901822593	8\\
6.7693625796766	8\\
6.7693625796766	9\\
7.46684532373632	9\\
7.46684532373632	10\\
7.8201911844284	10\\
7.8201911844284	11\\
8.04868919290918	11\\
8.04868919290918	12\\
8.38143469504978	12\\
8.38143469504978	13\\
8.91999608905833	13\\
8.91999608905833	14\\
9.05976343965153	14\\
9.05976343965153	15\\
9.12541477001934	15\\
9.12541477001934	16\\
9.63997895644646	16\\
9.63997895644646	17\\
9.8826040039711	17\\
9.8826040039711	18\\
9.89386561267219	18\\
9.89386561267219	19\\
10.3469876090198	19\\
10.3469876090198	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.2673857258609	0\\
2.2673857258609	1\\
2.35149236061577	1\\
2.35149236061577	2\\
2.85822294647119	2\\
2.85822294647119	3\\
3.26618662359611	3\\
3.26618662359611	4\\
4.34232517193484	4\\
4.34232517193484	5\\
6.20738959208409	5\\
6.20738959208409	6\\
6.24150992351093	6\\
6.24150992351093	7\\
6.25519083422991	7\\
6.25519083422991	8\\
6.40490908715521	8\\
6.40490908715521	9\\
6.60444033210427	9\\
6.60444033210427	10\\
6.78696675592183	10\\
6.78696675592183	11\\
6.98006344902439	11\\
6.98006344902439	12\\
7.99862768240798	12\\
7.99862768240798	13\\
8.06343365564778	13\\
8.06343365564778	14\\
8.42607751279214	14\\
8.42607751279214	15\\
9.12022340012093	15\\
9.12022340012093	16\\
9.21253577278675	16\\
9.21253577278675	17\\
9.31141104627832	17\\
9.31141104627832	18\\
9.63159359441606	18\\
9.63159359441606	19\\
10.6878624794617	19\\
10.6878624794617	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0198601116091481	0\\
0.0198601116091481	1\\
0.0817011389185538	1\\
0.0817011389185538	2\\
0.168571239111991	2\\
0.168571239111991	3\\
0.261341654028165	3\\
0.261341654028165	4\\
0.374272765327667	4\\
0.374272765327667	5\\
0.581030442096989	5\\
0.581030442096989	6\\
1.09930499680056	6\\
1.09930499680056	7\\
2.61057174374925	7\\
2.61057174374925	8\\
5.20847668541746	8\\
5.20847668541746	9\\
5.34149031045321	9\\
5.34149031045321	10\\
5.67828366159475	10\\
5.67828366159475	11\\
5.70804996232322	11\\
5.70804996232322	12\\
6.14904072429114	12\\
6.14904072429114	13\\
6.37338123076206	13\\
6.37338123076206	14\\
6.6478737058522	14\\
6.6478737058522	15\\
6.80318255556205	15\\
6.80318255556205	16\\
7.44013948539484	16\\
7.44013948539484	17\\
7.75395130034494	17\\
7.75395130034494	18\\
7.99431674149773	18\\
7.99431674149773	19\\
9.42702180666132	19\\
9.42702180666132	20\\
9.86988550317198	20\\
9.86988550317198	21\\
10.5357967347897	21\\
10.5357967347897	22\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.61099987496833	0\\
1.61099987496833	1\\
2.48506892394102	1\\
2.48506892394102	2\\
2.7126732143052	2\\
2.7126732143052	3\\
3.01021790913166	3\\
3.01021790913166	4\\
3.14111082577092	4\\
3.14111082577092	5\\
3.51110251950053	5\\
3.51110251950053	6\\
3.54208509881943	6\\
3.54208509881943	7\\
3.59152157762382	7\\
3.59152157762382	8\\
3.59744157574348	8\\
3.59744157574348	9\\
3.64429392057788	9\\
3.64429392057788	10\\
3.8439429222281	10\\
3.8439429222281	11\\
3.87331778528821	11\\
3.87331778528821	12\\
3.8775588189963	12\\
3.8775588189963	13\\
4.05139911805385	13\\
4.05139911805385	14\\
4.18753448096268	14\\
4.18753448096268	15\\
4.29650899231142	15\\
4.29650899231142	16\\
4.44120883324337	16\\
4.44120883324337	17\\
4.75573109765359	17\\
4.75573109765359	18\\
4.77641110073697	18\\
4.77641110073697	19\\
4.79408170093272	19\\
4.79408170093272	20\\
4.83963117540783	20\\
4.83963117540783	21\\
4.86883219761549	21\\
4.86883219761549	22\\
4.93801454717746	22\\
4.93801454717746	23\\
4.97144726378171	23\\
4.97144726378171	24\\
5.01725488659828	24\\
5.01725488659828	25\\
5.24682090345041	25\\
5.24682090345041	26\\
5.26551608417471	26\\
5.26551608417471	27\\
5.27690497666256	27\\
5.27690497666256	28\\
5.3370525872572	28\\
5.3370525872572	29\\
5.41018600275617	29\\
5.41018600275617	30\\
5.57906120294333	30\\
5.57906120294333	31\\
6.21709941737931	31\\
6.21709941737931	32\\
6.7717341189667	32\\
6.7717341189667	33\\
6.93398695685057	33\\
6.93398695685057	34\\
7.06878124528994	34\\
7.06878124528994	35\\
7.20551128338262	35\\
7.20551128338262	36\\
7.24929311630522	36\\
7.24929311630522	37\\
7.73877589741065	37\\
7.73877589741065	38\\
7.87555357345637	38\\
7.87555357345637	39\\
7.88651700516675	39\\
7.88651700516675	40\\
7.89344308090051	40\\
7.89344308090051	41\\
8.0120599511653	41\\
8.0120599511653	42\\
8.14454961841322	42\\
8.14454961841322	43\\
8.65469403482506	43\\
8.65469403482506	44\\
9.34567042184948	44\\
9.34567042184948	45\\
9.42597572436094	45\\
9.42597572436094	46\\
10.182333452947	46\\
10.182333452947	47\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.65268074304267	0\\
3.65268074304267	1\\
3.88901241460533	1\\
3.88901241460533	2\\
5.59020242663688	2\\
5.59020242663688	3\\
6.5352843013183	3\\
6.5352843013183	4\\
7.07792061040775	4\\
7.07792061040775	5\\
7.93563810341947	5\\
7.93563810341947	6\\
8.00987452144641	6\\
8.00987452144641	7\\
9.96398114682045	7\\
9.96398114682045	8\\
10.4086309635678	8\\
10.4086309635678	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.05982456234745	0\\
1.05982456234745	1\\
1.62986379320227	1\\
1.62986379320227	2\\
1.99380447814152	2\\
1.99380447814152	3\\
2.39499272344351	3\\
2.39499272344351	4\\
2.47781101607012	4\\
2.47781101607012	5\\
5.07805523942512	5\\
5.07805523942512	6\\
6.57465680435746	6\\
6.57465680435746	7\\
8.8172192206883	7\\
8.8172192206883	8\\
9.17577682031326	8\\
9.17577682031326	9\\
9.2825104718798	9\\
9.2825104718798	10\\
9.30586963517969	10\\
9.30586963517969	11\\
9.31728505350225	11\\
9.31728505350225	12\\
9.33391223439852	12\\
9.33391223439852	13\\
9.61415204029871	13\\
9.61415204029871	14\\
9.63399876717513	14\\
9.63399876717513	15\\
10.8699066070632	15\\
10.8699066070632	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.66463752389706	0\\
1.66463752389706	1\\
2.94736136588761	1\\
2.94736136588761	2\\
3.91486473461745	2\\
3.91486473461745	3\\
3.92405468938567	3\\
3.92405468938567	4\\
5.17115543023066	4\\
5.17115543023066	5\\
5.25391550410906	5\\
5.25391550410906	6\\
5.59369825237716	6\\
5.59369825237716	7\\
5.59405677940283	8\\
5.59996943703111	8\\
5.59996943703111	9\\
5.6646717699285	9\\
5.6646717699285	10\\
5.72141155138076	10\\
5.72141155138076	11\\
6.13066117932172	11\\
6.13066117932172	12\\
6.60657619793438	12\\
6.60657619793438	13\\
9.46832812081661	13\\
9.46832812081661	14\\
9.50859202664192	14\\
9.50859202664192	15\\
11.9637982326723	15\\
11.9637982326723	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.75966347760385	0\\
1.75966347760385	1\\
1.88043403178503	1\\
1.88043403178503	2\\
2.43971876889291	2\\
2.43971876889291	3\\
3.04002235162658	3\\
3.04002235162658	4\\
4.14378824148086	4\\
4.14378824148086	5\\
5.45658957628896	5\\
5.45658957628896	6\\
6.04432035138437	6\\
6.04432035138437	7\\
6.65743997648742	7\\
6.65743997648742	8\\
6.72237946695015	8\\
6.72237946695015	9\\
6.81442979880124	9\\
6.81442979880124	10\\
6.97790425109621	10\\
6.97790425109621	11\\
7.26395035632135	11\\
7.26395035632135	12\\
7.56665138456619	12\\
7.56665138456619	13\\
7.82378358469683	13\\
7.82378358469683	14\\
7.84510847426384	14\\
7.84510847426384	15\\
8.20590667550848	15\\
8.20590667550848	16\\
8.70802014077596	16\\
8.70802014077596	17\\
8.87915038705058	17\\
8.87915038705058	18\\
10.1004168564402	18\\
10.1004168564402	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.802882306235247	0\\
0.802882306235247	1\\
1.95022291742877	1\\
1.95022291742877	2\\
1.95317711354829	3\\
2.50867870510842	3\\
2.50867870510842	4\\
2.5581939719096	4\\
2.5581939719096	5\\
2.93154558270806	5\\
2.93154558270806	6\\
3.19135350712457	6\\
3.19135350712457	7\\
3.67395829538213	7\\
3.67395829538213	8\\
3.86406961616886	8\\
3.86406961616886	9\\
3.87741057657617	9\\
3.87741057657617	10\\
4.03191788168402	10\\
4.03191788168402	11\\
4.06223322377689	11\\
4.06223322377689	12\\
4.12243129150662	12\\
4.12243129150662	13\\
4.18205014850846	13\\
4.18205014850846	14\\
4.2146753159704	14\\
4.2146753159704	15\\
4.32856320888516	15\\
4.32856320888516	16\\
4.33897597465783	16\\
4.33897597465783	17\\
4.4593536929607	17\\
4.4593536929607	18\\
4.47848098603284	18\\
4.47848098603284	19\\
4.4946955942118	19\\
4.4946955942118	20\\
4.60858627413251	20\\
4.60858627413251	21\\
4.81180199568006	21\\
4.81180199568006	22\\
5.04529336600145	22\\
5.04529336600145	23\\
5.12010953256016	23\\
5.12010953256016	24\\
5.25541548001017	24\\
5.25541548001017	25\\
5.39840677858091	25\\
5.39840677858091	26\\
5.46620769501722	26\\
5.46620769501722	27\\
5.54455884721685	27\\
5.54455884721685	28\\
5.57330030231591	28\\
5.57330030231591	29\\
5.60019903290362	29\\
5.60019903290362	30\\
5.612732208982	30\\
5.612732208982	31\\
5.62160885730046	31\\
5.62160885730046	32\\
5.6317909593583	32\\
5.6317909593583	33\\
5.71588231189909	33\\
5.71588231189909	34\\
5.747312128911	34\\
5.747312128911	35\\
5.78611283785087	35\\
5.78611283785087	36\\
5.92005072618856	36\\
5.92005072618856	37\\
6.11301787906298	37\\
6.11301787906298	38\\
6.31347676444571	38\\
6.31347676444571	39\\
6.54385268426562	39\\
6.54385268426562	40\\
6.59972192653831	40\\
6.59972192653831	41\\
6.77238633594301	41\\
6.77238633594301	42\\
6.9855698662405	42\\
6.9855698662405	43\\
7.03699553759036	43\\
7.03699553759036	44\\
7.24684538108124	44\\
7.24684538108124	45\\
7.31018698857778	45\\
7.31018698857778	46\\
7.38641795470331	46\\
7.38641795470331	47\\
7.94311520190707	47\\
7.94311520190707	48\\
7.97616060536325	48\\
7.97616060536325	49\\
8.40821577296121	49\\
8.40821577296121	50\\
9.72948587686744	50\\
9.72948587686744	51\\
13.2732171141859	51\\
13.2732171141859	52\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.240495918688939	0\\
0.240495918688939	1\\
0.295075818530883	1\\
0.295075818530883	2\\
0.658185150128563	2\\
0.658185150128563	3\\
0.859298523257767	3\\
0.859298523257767	4\\
0.878408798936199	4\\
0.878408798936199	5\\
0.942022197013415	5\\
0.942022197013415	6\\
1.20983875794135	6\\
1.20983875794135	7\\
1.7709516975981	7\\
1.7709516975981	8\\
1.8499073483894	8\\
1.8499073483894	9\\
2.41062901504254	9\\
2.41062901504254	10\\
2.65035730735789	10\\
2.65035730735789	11\\
3.07143596379811	11\\
3.07143596379811	12\\
4.40139640548128	12\\
4.40139640548128	13\\
4.45248975378456	13\\
4.45248975378456	14\\
4.48313496025532	14\\
4.48313496025532	15\\
4.65968572365616	15\\
4.65968572365616	16\\
4.839360824866	16\\
4.839360824866	17\\
4.92405826749826	17\\
4.92405826749826	18\\
5.00119162843466	18\\
5.00119162843466	19\\
5.04163503413378	19\\
5.04163503413378	20\\
6.92087557363422	20\\
6.92087557363422	21\\
7.42362281373524	21\\
7.42362281373524	22\\
9.29935021928897	22\\
9.29935021928897	23\\
11.1250699207783	23\\
11.1250699207783	24\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.65074568290526	0\\
1.65074568290526	1\\
2.09509199886653	1\\
2.09509199886653	2\\
6.77059234003944	2\\
6.77059234003944	3\\
7.92549893572122	3\\
7.92549893572122	4\\
8.24405558620337	4\\
8.24405558620337	5\\
8.41524800751711	5\\
8.41524800751711	6\\
8.68457747650699	6\\
8.68457747650699	7\\
8.81617025014891	7\\
8.81617025014891	8\\
9.26334725558174	8\\
9.26334725558174	9\\
9.39058102237706	9\\
9.39058102237706	10\\
9.49066264911621	10\\
9.49066264911621	11\\
10.0369212141329	11\\
10.0369212141329	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.79612470825485	0\\
3.79612470825485	1\\
3.90965557924743	1\\
3.90965557924743	2\\
3.94303029549701	2\\
3.94303029549701	3\\
4.12299888321962	3\\
4.12299888321962	4\\
4.40658359442575	4\\
4.40658359442575	5\\
6.61461580711504	5\\
6.61461580711504	6\\
6.61673708111012	7\\
7.32937658790826	7\\
7.32937658790826	8\\
7.42023299029577	8\\
7.42023299029577	9\\
7.44084146671697	9\\
7.44084146671697	10\\
7.53978423423207	10\\
7.53978423423207	11\\
7.66339438619937	11\\
7.66339438619937	12\\
7.70832572691562	12\\
7.70832572691562	13\\
7.71468422239511	13\\
7.71468422239511	14\\
7.72457557199636	14\\
7.72457557199636	15\\
10.4807822493448	15\\
10.4807822493448	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.00849151233674483	0\\
0.00849151233674483	1\\
0.199474246715845	1\\
0.199474246715845	2\\
2.22383651003061	2\\
2.22383651003061	3\\
2.87578044339178	3\\
2.87578044339178	4\\
4.41887235974975	4\\
4.41887235974975	5\\
5.82476046957459	5\\
5.82476046957459	6\\
6.24208472137468	6\\
6.24208472137468	7\\
7.36591114688347	7\\
7.36591114688347	8\\
9.37275830519668	8\\
9.37275830519668	9\\
9.39130155407896	9\\
9.39130155407896	10\\
10.7358898936678	10\\
10.7358898936678	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
6.47568824023215	0\\
6.47568824023215	1\\
7.5311840843385	1\\
7.5311840843385	2\\
8.39015297150397	2\\
8.39015297150397	3\\
8.61271022814241	3\\
8.61271022814241	4\\
8.71429012613661	4\\
8.71429012613661	5\\
9.12411562880098	5\\
9.12411562880098	6\\
9.48718480982542	6\\
9.48718480982542	7\\
9.77984579851976	7\\
9.77984579851976	8\\
9.83231969659476	8\\
9.83231969659476	9\\
9.99457090717643	9\\
9.99457090717643	10\\
10.0387619373265	10\\
10.0387619373265	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.369813910037625	0\\
0.369813910037625	1\\
0.480981049796167	1\\
0.480981049796167	2\\
0.616926800102863	2\\
0.616926800102863	3\\
0.711202761790332	3\\
0.711202761790332	4\\
0.933217446783843	4\\
0.933217446783843	5\\
2.25131927662921	5\\
2.25131927662921	6\\
2.64725741871117	6\\
2.64725741871117	7\\
4.73317920619934	7\\
4.73317920619934	8\\
5.03486085210117	8\\
5.03486085210117	9\\
5.17380742298183	9\\
5.17380742298183	10\\
5.56877173083704	10\\
5.56877173083704	11\\
6.04404572612503	11\\
6.04404572612503	12\\
7.87392266584745	12\\
7.87392266584745	13\\
8.17006226271298	13\\
8.17006226271298	14\\
8.17057525082723	15\\
8.45739849056644	15\\
8.45739849056644	16\\
9.61385484050161	16\\
9.61385484050161	17\\
9.91372274600745	17\\
9.91372274600745	18\\
10.2159681370426	18\\
10.2159681370426	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.151736794255623	0\\
0.151736794255623	1\\
1.55939154469493	1\\
1.55939154469493	2\\
1.83711082591768	2\\
1.83711082591768	3\\
1.98733198296756	3\\
1.98733198296756	4\\
2.02240241409731	4\\
2.02240241409731	5\\
2.28458073474555	5\\
2.28458073474555	6\\
2.87759152413614	6\\
2.87759152413614	7\\
2.90817569067608	7\\
2.90817569067608	8\\
2.94967234648491	8\\
2.94967234648491	9\\
4.36779149612711	9\\
4.36779149612711	10\\
4.7112025332128	10\\
4.7112025332128	11\\
4.74646131493082	11\\
4.74646131493082	12\\
5.52921746732263	12\\
5.52921746732263	13\\
5.58892562007884	13\\
5.58892562007884	14\\
5.63965601291801	14\\
5.63965601291801	15\\
5.64269181109466	16\\
11.9932000629947	16\\
11.9932000629947	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.861349211215156	0\\
0.861349211215156	1\\
1.70745519578741	1\\
1.70745519578741	2\\
2.53712762635551	2\\
2.53712762635551	3\\
2.7798811148541	3\\
2.7798811148541	4\\
2.83602907171221	4\\
2.83602907171221	5\\
2.89759896999137	5\\
2.89759896999137	6\\
3.49568619796977	6\\
3.49568619796977	7\\
3.5173320966921	7\\
3.5173320966921	8\\
3.64348109258277	8\\
3.64348109258277	9\\
3.95779681989604	9\\
3.95779681989604	10\\
4.03549201917964	10\\
4.03549201917964	11\\
4.07096024454253	11\\
4.07096024454253	12\\
4.14889460465748	12\\
4.14889460465748	13\\
4.19431998848973	13\\
4.19431998848973	14\\
4.20182156447065	14\\
4.20182156447065	15\\
4.34658754325489	15\\
4.34658754325489	16\\
4.42407407545368	16\\
4.42407407545368	17\\
4.49600887637844	17\\
4.49600887637844	18\\
4.52819323035898	18\\
4.52819323035898	19\\
4.54077974878096	19\\
4.54077974878096	20\\
4.58166156525815	20\\
4.58166156525815	21\\
4.59561247469262	21\\
4.59561247469262	22\\
5.09716955440968	22\\
5.09716955440968	23\\
5.46575031587781	23\\
5.46575031587781	24\\
5.76208594161248	24\\
5.76208594161248	25\\
6.79038919595363	25\\
6.79038919595363	26\\
8.2131390224466	26\\
8.2131390224466	27\\
8.66437602829834	27\\
8.66437602829834	28\\
9.03625437525464	28\\
9.03625437525464	29\\
9.81089962249598	29\\
9.81089962249598	30\\
10.7091384983361	30\\
10.7091384983361	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.350547926060486	0\\
0.350547926060486	1\\
0.94753935331801	1\\
0.94753935331801	2\\
2.22029483708389	2\\
2.22029483708389	3\\
4.98814505904412	3\\
4.98814505904412	4\\
7.26339788651606	4\\
7.26339788651606	5\\
7.30034080730047	5\\
7.30034080730047	6\\
7.32979248229368	6\\
7.32979248229368	7\\
8.10033620432572	7\\
8.10033620432572	8\\
8.10090975151818	9\\
8.19722222237467	9\\
8.19722222237467	10\\
8.20300398448711	10\\
8.20300398448711	11\\
8.22093598885951	11\\
8.22093598885951	12\\
12.1559848390801	12\\
12.1559848390801	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.57372697807847	0\\
1.57372697807847	1\\
1.6215125444195	1\\
1.6215125444195	2\\
1.64664827385884	2\\
1.64664827385884	3\\
1.66949603686702	3\\
1.66949603686702	4\\
1.81784279938968	4\\
1.81784279938968	5\\
6.07983799366968	5\\
6.07983799366968	6\\
6.31210789897795	6\\
6.31210789897795	7\\
6.43744003537308	7\\
6.43744003537308	8\\
6.64519109399676	8\\
6.64519109399676	9\\
6.90443883593069	9\\
6.90443883593069	10\\
7.34605777848079	10\\
7.34605777848079	11\\
7.43806098408016	11\\
7.43806098408016	12\\
8.18249714935448	12\\
8.18249714935448	13\\
8.29274141524275	13\\
8.29274141524275	14\\
9.38017986425297	14\\
9.38017986425297	15\\
9.78541170765322	15\\
9.78541170765322	16\\
10.1601947698987	16\\
10.1601947698987	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.38016908012677	0\\
1.38016908012677	1\\
1.63624167392887	1\\
1.63624167392887	2\\
2.25373905492216	2\\
2.25373905492216	3\\
2.4404453499256	3\\
2.4404453499256	4\\
4.12081128471009	4\\
4.12081128471009	5\\
4.2823897035713	5\\
4.2823897035713	6\\
4.34792510532856	6\\
4.34792510532856	7\\
4.55875968525573	7\\
4.55875968525573	8\\
4.56567956565773	8\\
4.56567956565773	9\\
4.70979268547464	9\\
4.70979268547464	10\\
4.77396650983434	10\\
4.77396650983434	11\\
4.77962853581138	11\\
4.77962853581138	12\\
5.03063797291833	12\\
5.03063797291833	13\\
5.15583750415787	13\\
5.15583750415787	14\\
5.30180457131138	14\\
5.30180457131138	15\\
5.3232313131567	15\\
5.3232313131567	16\\
5.70425808544814	16\\
5.70425808544814	17\\
5.77471692525368	17\\
5.77471692525368	18\\
5.78190671140478	18\\
5.78190671140478	19\\
5.80002911414826	19\\
5.80002911414826	20\\
6.02362119193703	20\\
6.02362119193703	21\\
6.12805000748688	21\\
6.12805000748688	22\\
6.39825303370725	22\\
6.39825303370725	23\\
6.67238867223671	23\\
6.67238867223671	24\\
6.85893034827279	24\\
6.85893034827279	25\\
6.89174061455992	25\\
6.89174061455992	26\\
6.93081729492595	26\\
6.93081729492595	27\\
7.03502559205442	27\\
7.03502559205442	28\\
7.06636941646967	28\\
7.06636941646967	29\\
7.12808503646221	29\\
7.12808503646221	30\\
7.18416467235817	30\\
7.18416467235817	31\\
7.31164283560509	31\\
7.31164283560509	32\\
7.65595632126412	32\\
7.65595632126412	33\\
7.7338610303989	33\\
7.7338610303989	34\\
7.92350544247613	34\\
7.92350544247613	35\\
8.07990428410221	35\\
8.07990428410221	36\\
8.13229577339065	36\\
8.13229577339065	37\\
8.16235349129913	37\\
8.16235349129913	38\\
8.2184996475598	38\\
8.2184996475598	39\\
8.4664490808025	39\\
8.4664490808025	40\\
8.53133915315978	40\\
8.53133915315978	41\\
8.54777133140556	41\\
8.54777133140556	42\\
8.63456454753101	42\\
8.63456454753101	43\\
8.88970223871591	43\\
8.88970223871591	44\\
8.90732281682065	44\\
8.90732281682065	45\\
8.95245466295723	45\\
8.95245466295723	46\\
8.95894119007939	46\\
8.95894119007939	47\\
9.1612546976066	47\\
9.1612546976066	48\\
9.24089893696733	48\\
9.24089893696733	49\\
9.49294801673896	49\\
9.49294801673896	50\\
9.61702810919365	50\\
9.61702810919365	51\\
16.2160699309231	51\\
16.2160699309231	52\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
4.66581351362453	0\\
4.66581351362453	1\\
4.89898698130776	1\\
4.89898698130776	2\\
5.19167634014164	2\\
5.19167634014164	3\\
5.37175048966089	3\\
5.37175048966089	4\\
5.51436033237628	4\\
5.51436033237628	5\\
6.11314077818323	5\\
6.11314077818323	6\\
6.11981916104368	6\\
6.11981916104368	7\\
6.23632910570346	7\\
6.23632910570346	8\\
6.49177234828163	8\\
6.49177234828163	9\\
6.5164717811952	9\\
6.5164717811952	10\\
6.96859464765076	10\\
6.96859464765076	11\\
7.60562072259572	11\\
7.60562072259572	12\\
7.78696731974892	12\\
7.78696731974892	13\\
8.18533246245373	13\\
8.18533246245373	14\\
8.2072579827614	14\\
8.2072579827614	15\\
8.22354355640629	15\\
8.22354355640629	16\\
8.75503454153673	16\\
8.75503454153673	17\\
9.69798805416045	17\\
9.69798805416045	18\\
10.1790607680364	18\\
10.1790607680364	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.984376482355007	0\\
0.984376482355007	1\\
3.28164050464314	1\\
3.28164050464314	2\\
3.45148150043893	2\\
3.45148150043893	3\\
4.58232944470512	3\\
4.58232944470512	4\\
5.14799874172008	4\\
5.14799874172008	5\\
5.6557016155263	5\\
5.6557016155263	6\\
5.81761588309027	6\\
5.81761588309027	7\\
6.05465423910265	7\\
6.05465423910265	8\\
6.11896337906108	8\\
6.11896337906108	9\\
6.61486188953682	9\\
6.61486188953682	10\\
6.6893470982857	10\\
6.6893470982857	11\\
7.36802140138793	11\\
7.36802140138793	12\\
7.37916746399208	12\\
7.37916746399208	13\\
7.49580097418247	13\\
7.49580097418247	14\\
7.58805198304495	14\\
7.58805198304495	15\\
7.64263961558508	15\\
7.64263961558508	16\\
7.6681108073522	16\\
7.6681108073522	17\\
7.68076054617898	17\\
7.68076054617898	18\\
8.13475749985131	18\\
8.13475749985131	19\\
8.17390225935543	19\\
8.17390225935543	20\\
8.30209635633657	20\\
8.30209635633657	21\\
8.42388808667933	21\\
8.42388808667933	22\\
8.45533874512352	22\\
8.45533874512352	23\\
8.68035702747767	23\\
8.68035702747767	24\\
9.06957097773265	24\\
9.06957097773265	25\\
10.796521522665	25\\
10.796521522665	26\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0503445460185503	0\\
0.0503445460185503	1\\
0.721415594896321	1\\
0.721415594896321	2\\
0.785738472742295	2\\
0.785738472742295	3\\
0.797854329318241	3\\
0.797854329318241	4\\
0.862858914842981	4\\
0.862858914842981	5\\
1.15388000671329	5\\
1.15388000671329	6\\
1.18987915525144	6\\
1.18987915525144	7\\
1.57166189551155	7\\
1.57166189551155	8\\
1.76792931473017	8\\
1.76792931473017	9\\
2.10602242906052	9\\
2.10602242906052	10\\
2.22681482053373	10\\
2.22681482053373	11\\
2.57102237743422	11\\
2.57102237743422	12\\
2.710870225416	12\\
2.710870225416	13\\
2.81765400318009	13\\
2.81765400318009	14\\
2.92996678296697	14\\
2.92996678296697	15\\
3.00460238186251	15\\
3.00460238186251	16\\
3.7450780846505	16\\
3.7450780846505	17\\
3.76514879127176	17\\
3.76514879127176	18\\
3.96835251675233	18\\
3.96835251675233	19\\
4.30825513153645	19\\
4.30825513153645	20\\
4.43479546346839	20\\
4.43479546346839	21\\
4.55614049486542	21\\
4.55614049486542	22\\
5.44447966409265	22\\
5.44447966409265	23\\
6.29771166618744	23\\
6.29771166618744	24\\
6.79398334213963	24\\
6.79398334213963	25\\
7.44056927472199	25\\
7.44056927472199	26\\
8.04158616762683	26\\
8.04158616762683	27\\
8.2573803727463	27\\
8.2573803727463	28\\
8.66340183179495	28\\
8.66340183179495	29\\
8.90235054209501	29\\
8.90235054209501	30\\
9.09065218201403	30\\
9.09065218201403	31\\
9.38397070273052	31\\
9.38397070273052	32\\
9.96053592447581	32\\
9.96053592447581	33\\
10.0392680019539	33\\
10.0392680019539	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.228096183615474	0\\
0.228096183615474	1\\
1.18013237820549	1\\
1.18013237820549	2\\
1.34199831798384	2\\
1.34199831798384	3\\
1.88017902457864	3\\
1.88017902457864	4\\
3.38243809700025	4\\
3.38243809700025	5\\
3.86472301632471	5\\
3.86472301632471	6\\
4.34101628325791	6\\
4.34101628325791	7\\
4.50519920169548	7\\
4.50519920169548	8\\
6.64636157661993	8\\
6.64636157661993	9\\
6.75634722010225	9\\
6.75634722010225	10\\
7.1552438825729	10\\
7.1552438825729	11\\
8.79510565425704	11\\
8.79510565425704	12\\
8.83898148868688	12\\
8.83898148868688	13\\
8.89175954214802	13\\
8.89175954214802	14\\
8.98256107474942	14\\
8.98256107474942	15\\
10.5359656522204	15\\
10.5359656522204	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.69052312938828	0\\
2.69052312938828	1\\
2.7707202256235	1\\
2.7707202256235	2\\
3.43463816337183	2\\
3.43463816337183	3\\
3.87949095762489	3\\
3.87949095762489	4\\
5.81534176912505	4\\
5.81534176912505	5\\
8.32113212280007	5\\
8.32113212280007	6\\
9.07468234184783	6\\
9.07468234184783	7\\
9.17538534180793	7\\
9.17538534180793	8\\
9.73956360679943	8\\
9.73956360679943	9\\
9.97097294752166	9\\
9.97097294752166	10\\
10.9496165648524	10\\
10.9496165648524	11\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.03748809801337	0\\
1.03748809801337	1\\
1.46515064876445	1\\
1.46515064876445	2\\
2.11011787173251	2\\
2.11011787173251	3\\
2.66179798105541	3\\
2.66179798105541	4\\
3.43140305239014	4\\
3.43140305239014	5\\
7.34342071437272	5\\
7.34342071437272	6\\
8.89235350483266	6\\
8.89235350483266	7\\
9.22521716806614	7\\
9.22521716806614	8\\
9.22811922749727	9\\
10.0516810738808	9\\
10.0516810738808	10\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.257408227793874	0\\
0.257408227793874	1\\
0.415191820756576	1\\
0.415191820756576	2\\
0.570543942043081	2\\
0.570543942043081	3\\
0.640795333728221	3\\
0.640795333728221	4\\
0.767481122553725	4\\
0.767481122553725	5\\
0.844647105869619	5\\
0.844647105869619	6\\
0.8775848215666	6\\
0.8775848215666	7\\
1.26046767930757	7\\
1.26046767930757	8\\
1.29675565889847	8\\
1.29675565889847	9\\
1.52686099378704	9\\
1.52686099378704	10\\
1.68089634993503	10\\
1.68089634993503	11\\
1.81661350882185	11\\
1.81661350882185	12\\
1.89473799410691	12\\
1.89473799410691	13\\
2.65224938138848	13\\
2.65224938138848	14\\
4.44783061416943	14\\
4.44783061416943	15\\
4.52107815114854	15\\
4.52107815114854	16\\
4.82382109333099	16\\
4.82382109333099	17\\
4.96473595011381	17\\
4.96473595011381	18\\
5.10769479972483	18\\
5.10769479972483	19\\
5.32240449644738	19\\
5.32240449644738	20\\
5.4330492828844	20\\
5.4330492828844	21\\
5.54644865870504	21\\
5.54644865870504	22\\
5.88105725278653	22\\
5.88105725278653	23\\
6.35710623580399	23\\
6.35710623580399	24\\
7.73806996804375	24\\
7.73806996804375	25\\
8.05786343472372	25\\
8.05786343472372	26\\
8.14112044035107	26\\
8.14112044035107	27\\
8.4736463789351	27\\
8.4736463789351	28\\
8.56859102003533	28\\
8.56859102003533	29\\
8.56978784146094	30\\
8.67276299302538	30\\
8.67276299302538	31\\
8.72695567188466	31\\
8.72695567188466	32\\
8.96140000197936	32\\
8.96140000197936	33\\
9.21945802884971	33\\
9.21945802884971	34\\
9.25324481741515	34\\
9.25324481741515	35\\
9.28502753933368	35\\
9.28502753933368	36\\
9.43017029223145	36\\
9.43017029223145	37\\
9.89951314977574	37\\
9.89951314977574	38\\
10.0464781563802	38\\
10.0464781563802	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.266684155279602	0\\
0.266684155279602	1\\
0.678843863895143	1\\
0.678843863895143	2\\
0.7559711106334	2\\
0.7559711106334	3\\
1.54922592752941	3\\
1.54922592752941	4\\
2.14143791727808	4\\
2.14143791727808	5\\
2.19590614847768	5\\
2.19590614847768	6\\
2.35446065941422	6\\
2.35446065941422	7\\
2.41269865140747	7\\
2.41269865140747	8\\
2.58221398339638	8\\
2.58221398339638	9\\
2.61308852903293	9\\
2.61308852903293	10\\
2.64488236793954	10\\
2.64488236793954	11\\
2.74247591011792	11\\
2.74247591011792	12\\
2.74397952197154	13\\
2.8842526641944	13\\
2.8842526641944	14\\
3.01241210758352	14\\
3.01241210758352	15\\
3.08861655953175	15\\
3.08861655953175	16\\
3.11165346774795	16\\
3.11165346774795	17\\
3.46399623498044	17\\
3.46399623498044	18\\
3.71445291209747	18\\
3.71445291209747	19\\
4.13168000031582	19\\
4.13168000031582	20\\
4.14575124086022	20\\
4.14575124086022	21\\
4.15916262586177	21\\
4.15916262586177	22\\
5.91419426872131	22\\
5.91419426872131	23\\
7.89734088021519	23\\
7.89734088021519	24\\
8.06987045376318	24\\
8.06987045376318	25\\
9.76721808182989	25\\
9.76721808182989	26\\
11.4890125175012	26\\
11.4890125175012	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.864813476967857	0\\
0.864813476967857	1\\
2.70197386856792	1\\
2.70197386856792	2\\
3.89567696370159	2\\
3.89567696370159	3\\
4.19588107568802	3\\
4.19588107568802	4\\
4.34248708674367	4\\
4.34248708674367	5\\
4.41390757690013	5\\
4.41390757690013	6\\
4.93011673997655	6\\
4.93011673997655	7\\
4.99784864630609	7\\
4.99784864630609	8\\
5.3157632967026	8\\
5.3157632967026	9\\
6.58405322662636	9\\
6.58405322662636	10\\
6.76041501987883	10\\
6.76041501987883	11\\
7.19080974307583	11\\
7.19080974307583	12\\
7.48245982721309	12\\
7.48245982721309	13\\
8.27809133068709	13\\
8.27809133068709	14\\
8.47649937164409	14\\
8.47649937164409	15\\
8.78923701938551	15\\
8.78923701938551	16\\
9.13574286244206	16\\
9.13574286244206	17\\
9.30185705895086	17\\
9.30185705895086	18\\
9.39496174611932	18\\
9.39496174611932	19\\
12.8065769240892	19\\
12.8065769240892	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0498432881683755	0\\
0.0498432881683755	1\\
0.452631387964374	1\\
0.452631387964374	2\\
0.869641683277504	2\\
0.869641683277504	3\\
1.18335491757574	3\\
1.18335491757574	4\\
1.53596699546574	4\\
1.53596699546574	5\\
1.73655307832151	5\\
1.73655307832151	6\\
2.94961645459887	6\\
2.94961645459887	7\\
2.95868290209037	7\\
2.95868290209037	8\\
3.64091059326638	8\\
3.64091059326638	9\\
4.01993688234015	9\\
4.01993688234015	10\\
4.3802873273962	10\\
4.3802873273962	11\\
4.39947262877835	11\\
4.39947262877835	12\\
4.67357597835276	12\\
4.67357597835276	13\\
5.44206654299428	13\\
5.44206654299428	14\\
6.52878781276856	14\\
6.52878781276856	15\\
6.65557978242609	15\\
6.65557978242609	16\\
7.80659084247048	16\\
7.80659084247048	17\\
8.15243513300631	17\\
8.15243513300631	18\\
8.48809948421782	18\\
8.48809948421782	19\\
8.83355537746771	19\\
8.83355537746771	20\\
9.83566918474001	20\\
9.83566918474001	21\\
9.95886299452343	21\\
9.95886299452343	22\\
9.97469059131535	22\\
9.97469059131535	23\\
10.1251764466913	23\\
10.1251764466913	24\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.41175660039123	0\\
1.41175660039123	1\\
1.53110842089393	1\\
1.53110842089393	2\\
1.60649498442268	2\\
1.60649498442268	3\\
1.65221317178313	3\\
1.65221317178313	4\\
1.88745107251101	4\\
1.88745107251101	5\\
2.56359074660656	5\\
2.56359074660656	6\\
2.60993947532473	6\\
2.60993947532473	7\\
3.94548661618203	7\\
3.94548661618203	8\\
4.63126685164449	8\\
4.63126685164449	9\\
4.6833668778159	9\\
4.6833668778159	10\\
5.90992042075612	10\\
5.90992042075612	11\\
6.22276724096033	11\\
6.22276724096033	12\\
6.27696808069368	12\\
6.27696808069368	13\\
6.36182586990723	13\\
6.36182586990723	14\\
6.71742203756506	14\\
6.71742203756506	15\\
6.72293628280407	15\\
6.72293628280407	16\\
6.85773137269914	16\\
6.85773137269914	17\\
7.66220630177868	17\\
7.66220630177868	18\\
8.76188021234221	18\\
8.76188021234221	19\\
9.41522387919038	19\\
9.41522387919038	20\\
11.4666565720083	20\\
11.4666565720083	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.44116613451498	0\\
0.44116613451498	1\\
0.491999754388249	1\\
0.491999754388249	2\\
0.628168006571828	2\\
0.628168006571828	3\\
3.33635777626306	3\\
3.33635777626306	4\\
5.40116459696756	4\\
5.40116459696756	5\\
5.85560944202209	5\\
5.85560944202209	6\\
6.8614722709371	6\\
6.8614722709371	7\\
6.95547870560664	7\\
6.95547870560664	8\\
7.20256787978771	8\\
7.20256787978771	9\\
8.46707203213695	9\\
8.46707203213695	10\\
9.41961196791167	10\\
9.41961196791167	11\\
10.1965504747128	11\\
10.1965504747128	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.25309718951064	0\\
2.25309718951064	1\\
4.65160075892645	1\\
4.65160075892645	2\\
5.21888648808354	2\\
5.21888648808354	3\\
5.23661476142442	3\\
5.23661476142442	4\\
5.32687901630145	4\\
5.32687901630145	5\\
5.44957571421675	5\\
5.44957571421675	6\\
5.89987321341516	6\\
5.89987321341516	7\\
6.13736245682359	7\\
6.13736245682359	8\\
6.15008502298029	8\\
6.15008502298029	9\\
6.33439258018366	9\\
6.33439258018366	10\\
6.9878278468946	10\\
6.9878278468946	11\\
7.34876641313971	11\\
7.34876641313971	12\\
7.71293263082697	12\\
7.71293263082697	13\\
7.90564657523004	13\\
7.90564657523004	14\\
7.9346974000968	14\\
7.9346974000968	15\\
8.45626587114108	15\\
8.45626587114108	16\\
8.50237438310935	16\\
8.50237438310935	17\\
8.57859488786361	17\\
8.57859488786361	18\\
8.71991295473952	18\\
8.71991295473952	19\\
8.75023708666638	19\\
8.75023708666638	20\\
8.95206476830067	20\\
8.95206476830067	21\\
9.07743039689651	21\\
9.07743039689651	22\\
9.11038620196051	22\\
9.11038620196051	23\\
9.16771473402888	23\\
9.16771473402888	24\\
9.31612754693236	24\\
9.31612754693236	25\\
9.39399468903685	25\\
9.39399468903685	26\\
9.40481635113354	26\\
9.40481635113354	27\\
10.1373594367954	27\\
10.1373594367954	28\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.142566891077548	0\\
0.142566891077548	1\\
1.25294316928822	1\\
1.25294316928822	2\\
1.83627673429801	2\\
1.83627673429801	3\\
2.73557203386557	3\\
2.73557203386557	4\\
5.02047534064891	4\\
5.02047534064891	5\\
5.65771398522408	5\\
5.65771398522408	6\\
7.04563554912176	6\\
7.04563554912176	7\\
7.15235215104482	7\\
7.15235215104482	8\\
7.2109511381172	8\\
7.2109511381172	9\\
7.49104995074928	9\\
7.49104995074928	10\\
9.94512182057685	10\\
9.94512182057685	11\\
14.2498132220533	11\\
14.2498132220533	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.72441205912031	0\\
3.72441205912031	1\\
4.27634477520901	1\\
4.27634477520901	2\\
4.68983787376694	2\\
4.68983787376694	3\\
4.80493214178715	3\\
4.80493214178715	4\\
8.06668314072856	4\\
8.06668314072856	5\\
9.45939594850261	5\\
9.45939594850261	6\\
9.66574870235878	6\\
9.66574870235878	7\\
10.1522120706309	7\\
10.1522120706309	8\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.687298251900195	0\\
0.687298251900195	1\\
0.711920011285819	1\\
0.711920011285819	2\\
1.09188489920682	2\\
1.09188489920682	3\\
2.28504076988918	3\\
2.28504076988918	4\\
2.34374594973601	4\\
2.34374594973601	5\\
2.40634087448903	5\\
2.40634087448903	6\\
2.44053424214815	6\\
2.44053424214815	7\\
2.59767586523582	7\\
2.59767586523582	8\\
2.66212127563525	8\\
2.66212127563525	9\\
3.18327007348818	9\\
3.18327007348818	10\\
3.29648934903729	10\\
3.29648934903729	11\\
3.56445299892439	11\\
3.56445299892439	12\\
3.87179483046263	12\\
3.87179483046263	13\\
4.04192862504356	13\\
4.04192862504356	14\\
4.16010141556277	14\\
4.16010141556277	15\\
4.23155870811919	15\\
4.23155870811919	16\\
4.34948487557858	16\\
4.34948487557858	17\\
4.54671613233319	17\\
4.54671613233319	18\\
4.80495695620108	18\\
4.80495695620108	19\\
4.86520785026211	19\\
4.86520785026211	20\\
5.09603099231696	20\\
5.09603099231696	21\\
5.1388927758799	21\\
5.1388927758799	22\\
5.18901999518896	22\\
5.18901999518896	23\\
5.22983399259662	23\\
5.22983399259662	24\\
5.66525285260644	24\\
5.66525285260644	25\\
5.83562658989246	25\\
5.83562658989246	26\\
6.02015682096464	26\\
6.02015682096464	27\\
6.11450607832171	27\\
6.11450607832171	28\\
6.94027010033778	28\\
6.94027010033778	29\\
7.12158200695355	29\\
7.12158200695355	30\\
7.73793259134444	30\\
7.73793259134444	31\\
7.75454133726435	31\\
7.75454133726435	32\\
7.81184732503957	32\\
7.81184732503957	33\\
8.09162472896944	33\\
8.09162472896944	34\\
8.38345997787243	34\\
8.38345997787243	35\\
8.65174311057233	35\\
8.65174311057233	36\\
8.70179023752472	36\\
8.70179023752472	37\\
8.7430456815582	37\\
8.7430456815582	38\\
8.85701711196598	38\\
8.85701711196598	39\\
9.13631652855125	39\\
9.13631652855125	40\\
10.6784906377583	40\\
10.6784906377583	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
3.19354417841247	0\\
3.19354417841247	1\\
3.64114214010698	1\\
3.64114214010698	2\\
3.85379866185679	2\\
3.85379866185679	3\\
4.01876915928446	3\\
4.01876915928446	4\\
4.16872976296784	4\\
4.16872976296784	5\\
4.62151703411065	5\\
4.62151703411065	6\\
4.66317669289238	6\\
4.66317669289238	7\\
4.73095822038759	7\\
4.73095822038759	8\\
4.81798761294876	8\\
4.81798761294876	9\\
5.32229596611167	9\\
5.32229596611167	10\\
5.34498169316885	10\\
5.34498169316885	11\\
7.34770039063741	11\\
7.34770039063741	12\\
7.42712660747738	12\\
7.42712660747738	13\\
7.54363206037119	13\\
7.54363206037119	14\\
7.79260709027814	14\\
7.79260709027814	15\\
9.47052035142874	15\\
9.47052035142874	16\\
10.2618906648488	16\\
10.2618906648488	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.362490800842721	0\\
0.362490800842721	1\\
0.66304051561093	1\\
0.66304051561093	2\\
0.763519294073426	2\\
0.763519294073426	3\\
0.820120427148133	3\\
0.820120427148133	4\\
1.15522356535714	4\\
1.15522356535714	5\\
2.25411125211873	5\\
2.25411125211873	6\\
2.48642257991645	6\\
2.48642257991645	7\\
3.60107041408268	7\\
3.60107041408268	8\\
3.72855300617416	8\\
3.72855300617416	9\\
3.87439413808676	9\\
3.87439413808676	10\\
4.14460477079505	10\\
4.14460477079505	11\\
4.63158628536694	11\\
4.63158628536694	12\\
4.96391055629237	12\\
4.96391055629237	13\\
5.36237162095151	13\\
5.36237162095151	14\\
5.48118140029743	14\\
5.48118140029743	15\\
5.50622092190108	15\\
5.50622092190108	16\\
5.52341311521994	16\\
5.52341311521994	17\\
5.61771918314312	17\\
5.61771918314312	18\\
5.79962433783722	18\\
5.79962433783722	19\\
6.0897927336156	19\\
6.0897927336156	20\\
9.2225568722728	20\\
9.2225568722728	21\\
9.82863926760847	21\\
9.82863926760847	22\\
11.5516334184715	22\\
11.5516334184715	23\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.55342115803808	0\\
1.55342115803808	1\\
1.72176386746263	1\\
1.72176386746263	2\\
2.64806474061615	2\\
2.64806474061615	3\\
3.19306290738058	3\\
3.19306290738058	4\\
3.36214629054955	4\\
3.36214629054955	5\\
3.37878456302283	5\\
3.37878456302283	6\\
3.4751878633722	6\\
3.4751878633722	7\\
3.87806522345641	7\\
3.87806522345641	8\\
4.07603501429874	8\\
4.07603501429874	9\\
4.31019233330894	9\\
4.31019233330894	10\\
7.60058803365285	10\\
7.60058803365285	11\\
8.18534678346622	11\\
8.18534678346622	12\\
8.28246148915435	12\\
8.28246148915435	13\\
8.83405591353668	13\\
8.83405591353668	14\\
9.34112249081028	14\\
9.34112249081028	15\\
10.9295814364697	15\\
10.9295814364697	16\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0314382708144052	0\\
0.0314382708144052	1\\
0.177108041793595	1\\
0.177108041793595	2\\
0.181505422734393	2\\
0.181505422734393	3\\
0.477622919724414	3\\
0.477622919724414	4\\
0.6743238288594	4\\
0.6743238288594	5\\
0.745984869326435	5\\
0.745984869326435	6\\
0.771064594357949	6\\
0.771064594357949	7\\
0.82822601948164	7\\
0.82822601948164	8\\
0.95795871233868	8\\
0.95795871233868	9\\
1.02778730867982	9\\
1.02778730867982	10\\
1.1782949736228	10\\
1.1782949736228	11\\
1.8919391697492	11\\
1.8919391697492	12\\
2.01940944685705	12\\
2.01940944685705	13\\
2.11230074009136	13\\
2.11230074009136	14\\
2.22882569370467	14\\
2.22882569370467	15\\
2.40227477228826	15\\
2.40227477228826	16\\
3.06585721358975	16\\
3.06585721358975	17\\
4.63197122310601	17\\
4.63197122310601	18\\
4.99600101026246	18\\
4.99600101026246	19\\
5.03700072902366	19\\
5.03700072902366	20\\
5.27746530590849	20\\
5.27746530590849	21\\
6.56088918094243	21\\
6.56088918094243	22\\
9.31737413461046	22\\
9.31737413461046	23\\
9.72750842466092	23\\
9.72750842466092	24\\
9.75302629240455	24\\
9.75302629240455	25\\
9.91681950381196	25\\
9.91681950381196	26\\
10.1254074921137	26\\
10.1254074921137	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.50504958090977	0\\
0.50504958090977	1\\
0.626772665821598	1\\
0.626772665821598	2\\
0.839082382750295	2\\
0.839082382750295	3\\
0.84686433603904	3\\
0.84686433603904	4\\
1.76014895458909	4\\
1.76014895458909	5\\
4.00181027674765	5\\
4.00181027674765	6\\
4.85483031950322	6\\
4.85483031950322	7\\
6.95473812335598	7\\
6.95473812335598	8\\
7.11470891487381	8\\
7.11470891487381	9\\
7.48333666837262	9\\
7.48333666837262	10\\
7.68718074381317	10\\
7.68718074381317	11\\
8.52357707100751	11\\
8.52357707100751	12\\
8.69669588331957	12\\
8.69669588331957	13\\
9.05805309947675	13\\
9.05805309947675	14\\
9.06973539730091	14\\
9.06973539730091	15\\
9.65312262298992	15\\
9.65312262298992	16\\
9.7803201337754	16\\
9.7803201337754	17\\
9.86463381014973	17\\
9.86463381014973	18\\
9.87436194892689	18\\
9.87436194892689	19\\
10.1746071447009	19\\
10.1746071447009	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.842051887028248	0\\
0.842051887028248	1\\
0.950807923425124	1\\
0.950807923425124	2\\
0.961859219426834	2\\
0.961859219426834	3\\
1.13596111927942	3\\
1.13596111927942	4\\
1.14173188989237	4\\
1.14173188989237	5\\
1.18899936650475	5\\
1.18899936650475	6\\
1.21686363578814	6\\
1.21686363578814	7\\
1.22086515831827	7\\
1.22086515831827	8\\
1.51339395840677	8\\
1.51339395840677	9\\
1.53456264718686	9\\
1.53456264718686	10\\
1.57496952488999	10\\
1.57496952488999	11\\
1.64295843947255	11\\
1.64295843947255	12\\
1.74162739618592	12\\
1.74162739618592	13\\
1.76767399662025	13\\
1.76767399662025	14\\
1.8894140567407	14\\
1.8894140567407	15\\
2.00790973562599	15\\
2.00790973562599	16\\
2.15582718871509	16\\
2.15582718871509	17\\
2.18378016459889	17\\
2.18378016459889	18\\
2.32112230483874	18\\
2.32112230483874	19\\
2.44990477650221	19\\
2.44990477650221	20\\
2.54723404602105	20\\
2.54723404602105	21\\
2.61037881568929	21\\
2.61037881568929	22\\
2.61460361225359	22\\
2.61460361225359	23\\
3.02850750900122	23\\
3.02850750900122	24\\
3.12178074939492	24\\
3.12178074939492	25\\
3.36001707623856	25\\
3.36001707623856	26\\
3.50783832906596	26\\
3.50783832906596	27\\
3.7375397469394	27\\
3.7375397469394	28\\
4.00244188135388	28\\
4.00244188135388	29\\
4.07711346944437	29\\
4.07711346944437	30\\
4.20595303119092	30\\
4.20595303119092	31\\
4.32538666667564	31\\
4.32538666667564	32\\
4.33209291591422	32\\
4.33209291591422	33\\
4.50026426034282	33\\
4.50026426034282	34\\
4.76931096626289	34\\
4.76931096626289	35\\
4.81070125446782	35\\
4.81070125446782	36\\
4.92336340847931	36\\
4.92336340847931	37\\
5.50978781279592	37\\
5.50978781279592	38\\
6.05965350679575	38\\
6.05965350679575	39\\
6.98808593363766	39\\
6.98808593363766	40\\
7.38263617858199	40\\
7.38263617858199	41\\
7.52199031125961	41\\
7.52199031125961	42\\
7.71784220379863	42\\
7.71784220379863	43\\
7.72270418404094	43\\
7.72270418404094	44\\
7.79926450336259	44\\
7.79926450336259	45\\
8.50054809289528	45\\
8.50054809289528	46\\
8.7545028164912	46\\
8.7545028164912	47\\
10.730074883028	47\\
10.730074883028	48\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.151716602181875	0\\
0.151716602181875	1\\
0.489144111137092	1\\
0.489144111137092	2\\
2.6700681399813	2\\
2.6700681399813	3\\
4.11462260491589	3\\
4.11462260491589	4\\
4.14168367115879	4\\
4.14168367115879	5\\
4.65669007344029	5\\
4.65669007344029	6\\
5.2249505649525	6\\
5.2249505649525	7\\
6.98655318842068	7\\
6.98655318842068	8\\
7.13277843924942	8\\
7.13277843924942	9\\
7.29354064240498	9\\
7.29354064240498	10\\
7.38943324384182	10\\
7.38943324384182	11\\
7.40511128052549	11\\
7.40511128052549	12\\
8.65621721458096	12\\
8.65621721458096	13\\
9.81493288477358	13\\
9.81493288477358	14\\
10.5966159435817	14\\
10.5966159435817	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.290514005089737	0\\
0.290514005089737	1\\
0.313362785294213	1\\
0.313362785294213	2\\
0.452339848707044	2\\
0.452339848707044	3\\
0.854171535360813	3\\
0.854171535360813	4\\
1.14826673051072	4\\
1.14826673051072	5\\
1.60913397067714	5\\
1.60913397067714	6\\
2.42715419080066	6\\
2.42715419080066	7\\
4.68869644400466	7\\
4.68869644400466	8\\
5.04889798162025	8\\
5.04889798162025	9\\
5.67829715919127	9\\
5.67829715919127	10\\
5.81235212650888	10\\
5.81235212650888	11\\
5.98360652592798	11\\
5.98360652592798	12\\
6.2444523741817	12\\
6.2444523741817	13\\
6.86105602341225	13\\
6.86105602341225	14\\
7.12553448770288	14\\
7.12553448770288	15\\
7.14655009361564	15\\
7.14655009361564	16\\
7.18515679662731	16\\
7.18515679662731	17\\
7.32613796670092	17\\
7.32613796670092	18\\
7.34699871140149	18\\
7.34699871140149	19\\
7.54330517779331	19\\
7.54330517779331	20\\
8.32083122421175	20\\
8.32083122421175	21\\
8.90344374647711	21\\
8.90344374647711	22\\
8.90355764176535	23\\
8.9782462084117	23\\
8.9782462084117	24\\
9.28156571035895	24\\
9.28156571035895	25\\
9.7906272567106	25\\
9.7906272567106	26\\
10.2965455950799	26\\
10.2965455950799	27\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.29092728462539	0\\
0.29092728462539	1\\
0.440435989302593	1\\
0.440435989302593	2\\
0.717037398832112	2\\
0.717037398832112	3\\
0.723060851249173	3\\
0.723060851249173	4\\
0.874714421668983	4\\
0.874714421668983	5\\
1.21442623948445	5\\
1.21442623948445	6\\
1.88521133716597	6\\
1.88521133716597	7\\
2.09058072175482	7\\
2.09058072175482	8\\
2.20133584088411	8\\
2.20133584088411	9\\
2.87033341816377	9\\
2.87033341816377	10\\
2.87492459172682	10\\
2.87492459172682	11\\
3.0127886013352	11\\
3.0127886013352	12\\
3.22782180660036	12\\
3.22782180660036	13\\
3.39919342496545	13\\
3.39919342496545	14\\
3.42925727586886	14\\
3.42925727586886	15\\
3.43132558960836	16\\
3.447077782813	16\\
3.447077782813	17\\
3.45632535325132	17\\
3.45632535325132	18\\
4.51616407306989	18\\
4.51616407306989	19\\
5.50224475612191	19\\
5.50224475612191	20\\
5.58681846111935	20\\
5.58681846111935	21\\
5.70454716894071	21\\
5.70454716894071	22\\
5.8398380765034	22\\
5.8398380765034	23\\
5.96229457357673	23\\
5.96229457357673	24\\
6.01369496740766	24\\
6.01369496740766	25\\
6.29350903610761	25\\
6.29350903610761	26\\
6.32249454406995	26\\
6.32249454406995	27\\
6.32811238500451	27\\
6.32811238500451	28\\
6.39308103620529	28\\
6.39308103620529	29\\
6.8011271550509	29\\
6.8011271550509	30\\
6.98262160389152	30\\
6.98262160389152	31\\
7.64697653459594	31\\
7.64697653459594	32\\
7.70919595922712	32\\
7.70919595922712	33\\
8.53792690354489	33\\
8.53792690354489	34\\
9.0893744908777	34\\
9.0893744908777	35\\
10.0922134372964	35\\
10.0922134372964	36\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.206968656219912	0\\
0.206968656219912	1\\
0.717187631591246	1\\
0.717187631591246	2\\
0.865665686056122	2\\
0.865665686056122	3\\
0.976916958065841	3\\
0.976916958065841	4\\
1.14031130441952	4\\
1.14031130441952	5\\
1.90389066169601	5\\
1.90389066169601	6\\
2.35680282038282	6\\
2.35680282038282	7\\
2.99663598257113	7\\
2.99663598257113	8\\
3.27900146379837	8\\
3.27900146379837	9\\
3.29145067504593	9\\
3.29145067504593	10\\
3.30050577132499	10\\
3.30050577132499	11\\
3.3296442562854	11\\
3.3296442562854	12\\
4.97978852239625	12\\
4.97978852239625	13\\
10.4269320062248	13\\
10.4269320062248	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.57833404732559	0\\
0.57833404732559	1\\
0.92458874074735	1\\
0.92458874074735	2\\
1.40214511009921	2\\
1.40214511009921	3\\
1.96769207325997	3\\
1.96769207325997	4\\
2.13471629391124	4\\
2.13471629391124	5\\
2.28417078692729	5\\
2.28417078692729	6\\
2.34309687258171	6\\
2.34309687258171	7\\
2.55382294011402	7\\
2.55382294011402	8\\
2.85641844850419	8\\
2.85641844850419	9\\
2.91442765190704	9\\
2.91442765190704	10\\
3.04691608181978	10\\
3.04691608181978	11\\
5.03863933192312	11\\
5.03863933192312	12\\
5.23511897257689	12\\
5.23511897257689	13\\
5.48252887314066	13\\
5.48252887314066	14\\
5.51907849344024	14\\
5.51907849344024	15\\
5.52508114252074	15\\
5.52508114252074	16\\
5.65595507639155	16\\
5.65595507639155	17\\
5.81547822757856	17\\
5.81547822757856	18\\
5.97064171387174	18\\
5.97064171387174	19\\
8.64569360605881	19\\
8.64569360605881	20\\
9.35037313476552	20\\
9.35037313476552	21\\
9.43171739901662	21\\
9.43171739901662	22\\
9.57579809618395	22\\
9.57579809618395	23\\
9.96625109406318	23\\
9.96625109406318	24\\
10.1864843750434	24\\
10.1864843750434	25\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.00612435431597191	0\\
0.00612435431597191	1\\
0.0992617024513436	1\\
0.0992617024513436	2\\
0.195991980063766	2\\
0.195991980063766	3\\
0.21412445779265	3\\
0.21412445779265	4\\
0.250786229415411	4\\
0.250786229415411	5\\
0.368818476164122	5\\
0.368818476164122	6\\
0.382526529564622	6\\
0.382526529564622	7\\
0.490484102889745	7\\
0.490484102889745	8\\
0.752574471579898	8\\
0.752574471579898	9\\
0.758083242428079	9\\
0.758083242428079	10\\
0.82102549867362	10\\
0.82102549867362	11\\
0.933453864309499	11\\
0.933453864309499	12\\
1.08619563599487	12\\
1.08619563599487	13\\
1.26240155647812	13\\
1.26240155647812	14\\
1.32810214874361	14\\
1.32810214874361	15\\
1.34341184912154	15\\
1.34341184912154	16\\
1.34374175888048	17\\
1.37461190444903	17\\
1.37461190444903	18\\
1.39323138852176	18\\
1.39323138852176	19\\
1.41343685568793	19\\
1.41343685568793	20\\
1.4139261589228	21\\
1.46251356714713	21\\
1.46251356714713	22\\
1.55358573616271	22\\
1.55358573616271	23\\
1.60430031822781	23\\
1.60430031822781	24\\
1.6908699948353	24\\
1.6908699948353	25\\
1.72328685016075	25\\
1.72328685016075	26\\
1.76745891506666	26\\
1.76745891506666	27\\
1.76927766289253	28\\
1.88361507130643	28\\
1.88361507130643	29\\
1.89305371217056	29\\
1.89305371217056	30\\
1.93823525465368	30\\
1.93823525465368	31\\
1.99396502506821	31\\
1.99396502506821	32\\
2.14735357374834	32\\
2.14735357374834	33\\
2.21962676160795	33\\
2.21962676160795	34\\
2.26395505392037	34\\
2.26395505392037	35\\
2.37685573095021	35\\
2.37685573095021	36\\
2.44504434861553	36\\
2.44504434861553	37\\
2.51251090248333	37\\
2.51251090248333	38\\
2.6290615106501	38\\
2.6290615106501	39\\
2.63354132622266	39\\
2.63354132622266	40\\
2.77714325470095	40\\
2.77714325470095	41\\
3.07739534532592	41\\
3.07739534532592	42\\
3.10333578302636	42\\
3.10333578302636	43\\
3.49916057972415	43\\
3.49916057972415	44\\
3.76962700948451	44\\
3.76962700948451	45\\
3.83262866950801	45\\
3.83262866950801	46\\
4.7100817228414	46\\
4.7100817228414	47\\
7.72951611131313	47\\
7.72951611131313	48\\
7.77966265839734	48\\
7.77966265839734	49\\
7.80476912783971	49\\
7.80476912783971	50\\
7.82208042508878	50\\
7.82208042508878	51\\
8.01297613319428	51\\
8.01297613319428	52\\
8.23352963007152	52\\
8.23352963007152	53\\
8.61160788956327	53\\
8.61160788956327	54\\
8.80400762646767	54\\
8.80400762646767	55\\
8.8308993164583	55\\
8.8308993164583	56\\
10.3042213670695	56\\
10.3042213670695	57\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.19282134439782	0\\
1.19282134439782	1\\
1.92858789029258	1\\
1.92858789029258	2\\
6.17649595874365	2\\
6.17649595874365	3\\
8.19821446581565	3\\
8.19821446581565	4\\
8.91998499569682	4\\
8.91998499569682	5\\
8.94927435763803	5\\
8.94927435763803	6\\
9.16609676267616	6\\
9.16609676267616	7\\
9.48303256715602	7\\
9.48303256715602	8\\
9.63239514497427	8\\
9.63239514497427	9\\
9.70838170109696	9\\
9.70838170109696	10\\
9.7898068429437	10\\
9.7898068429437	11\\
9.94005128266204	11\\
9.94005128266204	12\\
10.1193263299423	12\\
10.1193263299423	13\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.808734791018463	0\\
0.808734791018463	1\\
1.09061814053538	1\\
1.09061814053538	2\\
1.79926151705092	2\\
1.79926151705092	3\\
2.29338984185356	3\\
2.29338984185356	4\\
2.36330934648444	4\\
2.36330934648444	5\\
2.37512377791538	5\\
2.37512377791538	6\\
3.53685107514838	6\\
3.53685107514838	7\\
3.98926072987798	7\\
3.98926072987798	8\\
4.82516321081692	8\\
4.82516321081692	9\\
5.20594748120465	9\\
5.20594748120465	10\\
5.2582302906926	10\\
5.2582302906926	11\\
5.30540642645663	11\\
5.30540642645663	12\\
5.34074830913706	12\\
5.34074830913706	13\\
6.01974863302966	13\\
6.01974863302966	14\\
6.08696776770347	14\\
6.08696776770347	15\\
6.13627851842736	15\\
6.13627851842736	16\\
6.34551662197464	16\\
6.34551662197464	17\\
6.54282634315784	17\\
6.54282634315784	18\\
7.029156093885	18\\
7.029156093885	19\\
7.51332708640922	19\\
7.51332708640922	20\\
7.82449613186106	20\\
7.82449613186106	21\\
7.84635875295563	21\\
7.84635875295563	22\\
7.89783473635125	22\\
7.89783473635125	23\\
8.60716979999297	23\\
8.60716979999297	24\\
8.77948922080871	24\\
8.77948922080871	25\\
10.1335235787249	25\\
10.1335235787249	26\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.229570421411731	0\\
0.229570421411731	1\\
1.16258736942773	1\\
1.16258736942773	2\\
5.52877177630564	2\\
5.52877177630564	3\\
6.04173646645347	3\\
6.04173646645347	4\\
6.62093104923491	4\\
6.62093104923491	5\\
7.51578097195085	5\\
7.51578097195085	6\\
9.7302286607316	6\\
9.7302286607316	7\\
9.76340295933884	7\\
9.76340295933884	8\\
10.0007031019151	8\\
10.0007031019151	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.22840766947926	0\\
0.22840766947926	1\\
1.07650477983647	1\\
1.07650477983647	2\\
1.23683327960107	2\\
1.23683327960107	3\\
1.82563929158619	3\\
1.82563929158619	4\\
1.96402873937544	4\\
1.96402873937544	5\\
2.09935946766077	5\\
2.09935946766077	6\\
2.56300007047802	6\\
2.56300007047802	7\\
2.58419857384975	7\\
2.58419857384975	8\\
2.68979706121517	8\\
2.68979706121517	9\\
2.86250850619891	9\\
2.86250850619891	10\\
3.4703426068285	10\\
3.4703426068285	11\\
3.84986076640507	11\\
3.84986076640507	12\\
3.96911355023397	12\\
3.96911355023397	13\\
4.03229090172663	13\\
4.03229090172663	14\\
5.25079551810575	14\\
5.25079551810575	15\\
5.85230514820112	15\\
5.85230514820112	16\\
6.15892592198662	16\\
6.15892592198662	17\\
6.38700752310834	17\\
6.38700752310834	18\\
6.45246194042845	18\\
6.45246194042845	19\\
6.50668774493055	19\\
6.50668774493055	20\\
6.88462095364101	20\\
6.88462095364101	21\\
7.30296691502677	21\\
7.30296691502677	22\\
7.35194708118385	22\\
7.35194708118385	23\\
7.55572131485746	23\\
7.55572131485746	24\\
7.74150348672139	24\\
7.74150348672139	25\\
7.75976266432183	25\\
7.75976266432183	26\\
8.09059690677778	26\\
8.09059690677778	27\\
8.25978217828352	27\\
8.25978217828352	28\\
8.50039584118252	28\\
8.50039584118252	29\\
9.10283445303577	29\\
9.10283445303577	30\\
9.1071419950745	30\\
9.1071419950745	31\\
9.10834000214257	32\\
9.33242973537925	32\\
9.33242973537925	33\\
9.36441526558647	33\\
9.36441526558647	34\\
9.36531878237744	35\\
9.73699876865069	35\\
9.73699876865069	36\\
11.3970364162469	36\\
11.3970364162469	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.49651830344502	0\\
1.49651830344502	1\\
2.2258968578456	1\\
2.2258968578456	2\\
3.61623285326043	2\\
3.61623285326043	3\\
3.74683638383492	3\\
3.74683638383492	4\\
3.87305500375632	4\\
3.87305500375632	5\\
4.41830067716806	5\\
4.41830067716806	6\\
6.14739717444336	6\\
6.14739717444336	7\\
6.88236888102735	7\\
6.88236888102735	8\\
7.83050047104163	8\\
7.83050047104163	9\\
7.91388867363137	9\\
7.91388867363137	10\\
8.36225244085742	10\\
8.36225244085742	11\\
9.76053210114838	11\\
9.76053210114838	12\\
9.95130199109481	12\\
9.95130199109481	13\\
10.0668154972627	13\\
10.0668154972627	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.176389959485428	0\\
0.176389959485428	1\\
0.24585918667727	1\\
0.24585918667727	2\\
0.877135401840558	2\\
0.877135401840558	3\\
0.908910796618247	3\\
0.908910796618247	4\\
1.33477052567475	4\\
1.33477052567475	5\\
1.36836819800286	5\\
1.36836819800286	6\\
2.08296439293744	6\\
2.08296439293744	7\\
2.19934725277975	7\\
2.19934725277975	8\\
4.52439432918571	8\\
4.52439432918571	9\\
4.54651167012679	9\\
4.54651167012679	10\\
4.83431063614634	10\\
4.83431063614634	11\\
5.97624748269729	11\\
5.97624748269729	12\\
8.52463108779187	12\\
8.52463108779187	13\\
8.97678608465296	13\\
8.97678608465296	14\\
11.8666066126576	14\\
11.8666066126576	15\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.516348706890394	0\\
0.516348706890394	1\\
2.28175002497308	1\\
2.28175002497308	2\\
2.40128332357094	2\\
2.40128332357094	3\\
3.40057665917224	3\\
3.40057665917224	4\\
4.42325383659048	4\\
4.42325383659048	5\\
5.81415045618485	5\\
5.81415045618485	6\\
6.99999789397836	6\\
6.99999789397836	7\\
9.04025309252849	7\\
9.04025309252849	8\\
10.3996187960465	8\\
10.3996187960465	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.616105819078836	0\\
0.616105819078836	1\\
1.85362630744776	1\\
1.85362630744776	2\\
2.04876632405602	2\\
2.04876632405602	3\\
2.63382364616754	3\\
2.63382364616754	4\\
5.73394217238082	4\\
5.73394217238082	5\\
6.70202282037915	5\\
6.70202282037915	6\\
6.77585333853498	6\\
6.77585333853498	7\\
9.2411613057282	7\\
9.2411613057282	8\\
10.6446111168547	8\\
10.6446111168547	9\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.347563486106651	0\\
0.347563486106651	1\\
0.973961433947906	1\\
0.973961433947906	2\\
1.47764029804309	2\\
1.47764029804309	3\\
2.15252574082035	3\\
2.15252574082035	4\\
2.41153323848906	4\\
2.41153323848906	5\\
3.65988128967295	5\\
3.65988128967295	6\\
3.86182689829824	6\\
3.86182689829824	7\\
4.2178415202799	7\\
4.2178415202799	8\\
4.44413902564294	8\\
4.44413902564294	9\\
4.89195091167661	9\\
4.89195091167661	10\\
7.38211066454001	10\\
7.38211066454001	11\\
7.59350455577778	11\\
7.59350455577778	12\\
7.68482247402984	12\\
7.68482247402984	13\\
10.3566925520512	13\\
10.3566925520512	14\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.676112612455981	0\\
0.676112612455981	1\\
0.98556190402677	1\\
0.98556190402677	2\\
2.6161637179899	2\\
2.6161637179899	3\\
2.69186874885727	3\\
2.69186874885727	4\\
3.5999137894783	4\\
3.5999137894783	5\\
3.9848380473913	5\\
3.9848380473913	6\\
4.00941045476561	6\\
4.00941045476561	7\\
4.02121241194275	7\\
4.02121241194275	8\\
4.58123281309492	8\\
4.58123281309492	9\\
4.59614133414625	9\\
4.59614133414625	10\\
4.71246151871333	10\\
4.71246151871333	11\\
6.65602369657223	11\\
6.65602369657223	12\\
6.99394289529067	12\\
6.99394289529067	13\\
8.11679313443623	13\\
8.11679313443623	14\\
8.36554128948769	14\\
8.36554128948769	15\\
8.80829315489229	15\\
8.80829315489229	16\\
9.14231112704768	16\\
9.14231112704768	17\\
9.17999419741639	17\\
9.17999419741639	18\\
9.42634645250205	18\\
9.42634645250205	19\\
9.99798388688959	19\\
9.99798388688959	20\\
10.3510543733382	20\\
10.3510543733382	21\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.0321589610849173	0\\
0.0321589610849173	1\\
0.235388346219807	1\\
0.235388346219807	2\\
0.333587778641451	2\\
0.333587778641451	3\\
0.43221658627704	3\\
0.43221658627704	4\\
0.491910054168297	4\\
0.491910054168297	5\\
1.05281333981313	5\\
1.05281333981313	6\\
1.07644118653804	6\\
1.07644118653804	7\\
1.1378819031578	7\\
1.1378819031578	8\\
1.22568669016813	8\\
1.22568669016813	9\\
1.30583420887679	9\\
1.30583420887679	10\\
1.42057300792533	10\\
1.42057300792533	11\\
1.52641422392795	11\\
1.52641422392795	12\\
1.91061831024266	12\\
1.91061831024266	13\\
1.9687806694306	13\\
1.9687806694306	14\\
1.97716780232136	14\\
1.97716780232136	15\\
2.01730280578858	15\\
2.01730280578858	16\\
3.58988629848152	16\\
3.58988629848152	17\\
4.13775552544178	17\\
4.13775552544178	18\\
5.47323932275546	18\\
5.47323932275546	19\\
5.71330275335758	19\\
5.71330275335758	20\\
5.84544234916456	20\\
5.84544234916456	21\\
6.12097819628854	21\\
6.12097819628854	22\\
6.36231687744597	22\\
6.36231687744597	23\\
6.72896843237272	23\\
6.72896843237272	24\\
8.32808318185059	24\\
8.32808318185059	25\\
8.82081350393637	25\\
8.82081350393637	26\\
9.63124993571914	26\\
9.63124993571914	27\\
12.1117128858937	27\\
12.1117128858937	28\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.299952024489034	0\\
0.299952024489034	1\\
0.346798441563948	1\\
0.346798441563948	2\\
0.749259010756425	2\\
0.749259010756425	3\\
2.45834726629849	3\\
2.45834726629849	4\\
2.52419094890921	4\\
2.52419094890921	5\\
2.8448531868691	5\\
2.8448531868691	6\\
2.97347496026456	6\\
2.97347496026456	7\\
3.2718178019649	7\\
3.2718178019649	8\\
3.48768469458991	8\\
3.48768469458991	9\\
4.18902012485014	9\\
4.18902012485014	10\\
4.25327477748676	10\\
4.25327477748676	11\\
4.48148113452177	11\\
4.48148113452177	12\\
4.60814503950841	12\\
4.60814503950841	13\\
4.63970778985344	13\\
4.63970778985344	14\\
5.297921254199	14\\
5.297921254199	15\\
5.8006532067298	15\\
5.8006532067298	16\\
5.81854997744994	16\\
5.81854997744994	17\\
5.94736793475409	17\\
5.94736793475409	18\\
5.98688680984046	18\\
5.98688680984046	19\\
8.37068450877456	19\\
8.37068450877456	20\\
8.39853043193521	20\\
8.39853043193521	21\\
8.40774728034592	21\\
8.40774728034592	22\\
8.53581386653441	22\\
8.53581386653441	23\\
8.89340742340196	23\\
8.89340742340196	24\\
8.92377526356828	24\\
8.92377526356828	25\\
8.93118819818156	25\\
8.93118819818156	26\\
9.08414292765605	26\\
9.08414292765605	27\\
9.34658980342221	27\\
9.34658980342221	28\\
9.87314041194811	28\\
9.87314041194811	29\\
13.0603885626699	29\\
13.0603885626699	30\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
1.17643628294371	0\\
1.17643628294371	1\\
1.31896836879458	1\\
1.31896836879458	2\\
1.69879010313326	2\\
1.69879010313326	3\\
1.71765698187523	3\\
1.71765698187523	4\\
1.72991617569636	4\\
1.72991617569636	5\\
1.74048264051125	5\\
1.74048264051125	6\\
1.77069033673559	6\\
1.77069033673559	7\\
2.66172977802569	7\\
2.66172977802569	8\\
2.69916495762267	8\\
2.69916495762267	9\\
4.88940420474972	9\\
4.88940420474972	10\\
7.8669671122919	10\\
7.8669671122919	11\\
8.41860799778593	11\\
8.41860799778593	12\\
9.42960757102727	12\\
9.42960757102727	13\\
9.78242282862928	13\\
9.78242282862928	14\\
9.87971733217916	14\\
9.87971733217916	15\\
9.99502611145924	15\\
9.99502611145924	16\\
10.2610529530234	16\\
10.2610529530234	17\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.32314875010163	0\\
0.32314875010163	1\\
0.96710872230808	1\\
0.96710872230808	2\\
0.989406295616064	2\\
0.989406295616064	3\\
1.30087515936739	3\\
1.30087515936739	4\\
1.30995544204051	4\\
1.30995544204051	5\\
1.70909488463446	5\\
1.70909488463446	6\\
1.97512324099153	6\\
1.97512324099153	7\\
2.22867862132201	7\\
2.22867862132201	8\\
2.35213229193958	8\\
2.35213229193958	9\\
2.80462191480346	9\\
2.80462191480346	10\\
3.32034887190387	10\\
3.32034887190387	11\\
3.47009702659671	11\\
3.47009702659671	12\\
3.48699031675831	12\\
3.48699031675831	13\\
3.50897970226675	13\\
3.50897970226675	14\\
3.55640498991431	14\\
3.55640498991431	15\\
3.78285664387066	15\\
3.78285664387066	16\\
4.40264143866071	16\\
4.40264143866071	17\\
4.42882485946577	17\\
4.42882485946577	18\\
4.58103694073247	18\\
4.58103694073247	19\\
4.61824004079294	19\\
4.61824004079294	20\\
5.48264456423173	20\\
5.48264456423173	21\\
8.03620025675123	21\\
8.03620025675123	22\\
8.54190879829694	22\\
8.54190879829694	23\\
10.5473520600583	23\\
10.5473520600583	24\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.06704636055498	0\\
2.06704636055498	1\\
2.61958309675919	1\\
2.61958309675919	2\\
3.39593541765473	2\\
3.39593541765473	3\\
5.37511882801989	3\\
5.37511882801989	4\\
7.1510229788281	4\\
7.1510229788281	5\\
7.25357340038019	5\\
7.25357340038019	6\\
8.2028394853538	6\\
8.2028394853538	7\\
8.42006855915295	7\\
8.42006855915295	8\\
9.47396884479049	8\\
9.47396884479049	9\\
9.49740690948104	9\\
9.49740690948104	10\\
9.84152695121917	10\\
9.84152695121917	11\\
10.2197496321591	11\\
10.2197496321591	12\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.90537766560112	0\\
2.90537766560112	1\\
3.73502908799611	1\\
3.73502908799611	2\\
4.8242148329821	2\\
4.8242148329821	3\\
5.6146131639365	3\\
5.6146131639365	4\\
5.87729542209727	4\\
5.87729542209727	5\\
5.95837696598402	5\\
5.95837696598402	6\\
6.06749647561867	6\\
6.06749647561867	7\\
6.31808098981254	7\\
6.31808098981254	8\\
6.70041079886744	8\\
6.70041079886744	9\\
7.23369487691879	9\\
7.23369487691879	10\\
8.06445305760043	10\\
8.06445305760043	11\\
8.08755741885422	11\\
8.08755741885422	12\\
8.5261327689442	12\\
8.5261327689442	13\\
9.33998508604688	13\\
9.33998508604688	14\\
9.53917605639866	14\\
9.53917605639866	15\\
9.68339184387342	15\\
9.68339184387342	16\\
9.71907804719496	16\\
9.71907804719496	17\\
9.76175603172607	17\\
9.76175603172607	18\\
10.2376039943511	18\\
10.2376039943511	19\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.27339231919292	0\\
0.27339231919292	1\\
3.7836443076084	1\\
3.7836443076084	2\\
5.75866833284013	2\\
5.75866833284013	3\\
6.29228134245942	3\\
6.29228134245942	4\\
9.20709023012389	4\\
9.20709023012389	5\\
11.696813867832	5\\
11.696813867832	6\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.617841554428345	0\\
0.617841554428345	1\\
2.00934689191325	1\\
2.00934689191325	2\\
2.0548651195694	2\\
2.0548651195694	3\\
2.2831933528572	3\\
2.2831933528572	4\\
2.71305553952961	4\\
2.71305553952961	5\\
2.88846368463005	5\\
2.88846368463005	6\\
3.16218967338726	6\\
3.16218967338726	7\\
3.41592175910581	7\\
3.41592175910581	8\\
3.4790692962297	8\\
3.4790692962297	9\\
3.80481651861835	9\\
3.80481651861835	10\\
3.92355749313617	10\\
3.92355749313617	11\\
3.9500001952571	11\\
3.9500001952571	12\\
4.00330367972963	12\\
4.00330367972963	13\\
4.09729734111789	13\\
4.09729734111789	14\\
4.13324606730158	14\\
4.13324606730158	15\\
4.14683435603895	15\\
4.14683435603895	16\\
4.55126704885918	16\\
4.55126704885918	17\\
4.58022512942422	17\\
4.58022512942422	18\\
4.60440164365124	18\\
4.60440164365124	19\\
4.69678912945307	19\\
4.69678912945307	20\\
4.75193370729322	20\\
4.75193370729322	21\\
5.04266423338061	21\\
5.04266423338061	22\\
5.2135828491967	22\\
5.2135828491967	23\\
5.22026956266047	23\\
5.22026956266047	24\\
5.37056882590022	24\\
5.37056882590022	25\\
5.45534158739537	25\\
5.45534158739537	26\\
6.48389602759374	26\\
6.48389602759374	27\\
6.53910337155526	27\\
6.53910337155526	28\\
6.9192631919184	28\\
6.9192631919184	29\\
7.10328519288488	29\\
7.10328519288488	30\\
7.44259454626238	30\\
7.44259454626238	31\\
7.75104573213929	31\\
7.75104573213929	32\\
7.83936020037704	32\\
7.83936020037704	33\\
7.85212515376172	33\\
7.85212515376172	34\\
8.00500831726594	34\\
8.00500831726594	35\\
8.02609233708311	35\\
8.02609233708311	36\\
8.29569397856313	36\\
8.29569397856313	37\\
8.77816758193869	37\\
8.77816758193869	38\\
9.08087028935521	38\\
9.08087028935521	39\\
9.08267914089691	40\\
9.24807790881245	40\\
9.24807790881245	41\\
9.45716036476804	41\\
9.45716036476804	42\\
9.52115435676373	42\\
9.52115435676373	43\\
9.81733034336944	43\\
9.81733034336944	44\\
10.113572894398	44\\
10.113572894398	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
0.297516491333013	0\\
0.297516491333013	1\\
0.306693112362645	1\\
0.306693112362645	2\\
0.835773555617184	2\\
0.835773555617184	3\\
0.875902157953703	3\\
0.875902157953703	4\\
1.02333900495513	4\\
1.02333900495513	5\\
1.38380917346952	5\\
1.38380917346952	6\\
1.51660587314202	6\\
1.51660587314202	7\\
1.60946580770651	7\\
1.60946580770651	8\\
1.68371617091979	8\\
1.68371617091979	9\\
1.75795167572191	9\\
1.75795167572191	10\\
3.12918030001659	10\\
3.12918030001659	11\\
3.48003346453094	11\\
3.48003346453094	12\\
4.22430118514303	12\\
4.22430118514303	13\\
7.24795053869331	13\\
7.24795053869331	14\\
7.48210751695528	14\\
7.48210751695528	15\\
7.60127512708595	15\\
7.60127512708595	16\\
7.93680305888891	16\\
7.93680305888891	17\\
7.99983167930632	17\\
7.99983167930632	18\\
8.03383731780369	18\\
8.03383731780369	19\\
8.60022151227473	19\\
8.60022151227473	20\\
8.60578310934654	20\\
8.60578310934654	21\\
8.78716898831048	21\\
8.78716898831048	22\\
8.93522818346145	22\\
8.93522818346145	23\\
9.35912926625089	23\\
9.35912926625089	24\\
9.56330412071	24\\
9.56330412071	25\\
9.62768010071707	25\\
9.62768010071707	26\\
9.8059929594891	26\\
9.8059929594891	27\\
9.87114176350187	27\\
9.87114176350187	28\\
10.0980517029691	28\\
10.0980517029691	29\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0	0\\
2.49347389102885	0\\
2.49347389102885	1\\
2.74359268186894	1\\
2.74359268186894	2\\
3.10573021975353	2\\
3.10573021975353	3\\
4.23822814536005	3\\
4.23822814536005	4\\
4.31129433701992	4\\
4.31129433701992	5\\
5.24705026148987	5\\
5.24705026148987	6\\
5.6020091017746	6\\
5.6020091017746	7\\
5.71025261724248	7\\
5.71025261724248	8\\
5.78084446175858	8\\
5.78084446175858	9\\
6.2646332938344	9\\
6.2646332938344	10\\
6.9739410705833	10\\
6.9739410705833	11\\
7.05342380585077	11\\
7.05342380585077	12\\
7.2358009874752	12\\
7.2358009874752	13\\
9.19597622041966	13\\
9.19597622041966	14\\
10.1585016387596	14\\
10.1585016387596	15\\
};

==> fig7b_part1_extra_220211.tex <==

\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-8.33926722807375	0\\
2.08990033701544	0\\
2.08990033701544	1\\
3.39445460452089	1\\
3.39445460452089	2\\
4.90239367161476	2\\
4.90239367161476	3\\
6.35433763801178	3\\
6.35433763801178	4\\
8.21856472197344	4\\
8.21856472197344	5\\
11.3084691727409	5\\
11.3084691727409	6\\
12.1487064633451	6\\
12.1487064633451	7\\
14.1750577343057	7\\
14.1750577343057	8\\
16.6264286173738	8\\
16.6264286173738	9\\
17.4152824636824	9\\
17.4152824636824	10\\
18.3189332436033	10\\
18.3189332436033	11\\
21.8497981009266	11\\
21.8497981009266	12\\
23.0511551550544	12\\
23.0511551550544	13\\
26.3804408071963	13\\
26.3804408071963	14\\
26.7890593795568	14\\
26.7890593795568	15\\
26.988313141431	15\\
26.988313141431	16\\
27.7685829354995	16\\
27.7685829354995	17\\
27.9314603857247	17\\
27.9314603857247	18\\
31.179531538202	18\\
31.179531538202	19\\
32.2384538120012	19\\
32.2384538120012	20\\
38.279483024817	20\\
38.279483024817	21\\
40.122430806354	21\\
40.122430806354	22\\
46.0282047223154	22\\
46.0282047223154	23\\
51.6820722636303	23\\
51.6820722636303	24\\
52.7518671425009	24\\
52.7518671425009	25\\
55.7531667169127	25\\
55.7531667169127	26\\
61.4259919126909	26\\
61.4259919126909	27\\
65.2238834745573	27\\
65.2238834745573	28\\
67.5465231872242	28\\
67.5465231872242	29\\
68.9833220223404	29\\
68.9833220223404	30\\
72.2114684104993	30\\
72.2114684104993	31\\
73.0024003674814	31\\
73.0024003674814	32\\
74.1049055058542	32\\
74.1049055058542	33\\
75.0552988235728	33\\
75.0552988235728	34\\
76.3552371132935	34\\
76.3552371132935	35\\
76.6356361413734	35\\
76.6356361413734	36\\
77.2086501526321	36\\
77.2086501526321	37\\
79.4918490927707	37\\
79.4918490927707	38\\
79.9556084599757	38\\
79.9556084599757	39\\
79.99303842984	39\\
79.99303842984	40\\
80.6301899791901	40\\
80.6301899791901	41\\
80.7271092099367	41\\
80.7271092099367	42\\
81.5952199509247	42\\
81.5952199509247	43\\
82.0646767252026	43\\
82.0646767252026	44\\
82.768881698244	44\\
82.768881698244	45\\
83.480019705127	45\\
83.480019705127	46\\
83.684650263151	46\\
83.684650263151	47\\
84.1547499790182	47\\
84.1547499790182	48\\
84.187095720882	48\\
84.187095720882	49\\
84.5694288397226	49\\
84.5694288397226	50\\
86.6177267497954	50\\
86.6177267497954	51\\
87.7073336993925	51\\
87.7073336993925	52\\
87.8689532003259	52\\
87.8689532003259	53\\
88.7158790665253	53\\
88.7158790665253	54\\
95.187013089865	54\\
95.187013089865	55\\
98.515327371143	55\\
98.515327371143	56\\
106.153395866096	56\\
};

==> fig7b_part1_extra_220211_0.tex <==

\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-7.70739614398602	0\\
21.8959376404813	0\\
21.8959376404813	1\\
24.857926756689	1\\
24.857926756689	2\\
29.7441244950827	2\\
29.7441244950827	3\\
36.4707503921376	3\\
36.4707503921376	4\\
40.9008133867041	4\\
40.9008133867041	5\\
43.314162541293	5\\
43.314162541293	6\\
45.1551845750471	6\\
45.1551845750471	7\\
46.2081535003217	7\\
46.2081535003217	8\\
47.5616116755034	8\\
47.5616116755034	9\\
48.0757746784737	9\\
48.0757746784737	10\\
50.4166211105765	10\\
50.4166211105765	11\\
50.5942795825371	11\\
50.5942795825371	12\\
58.5199132449301	12\\
58.5199132449301	13\\
59.3309257947062	13\\
59.3309257947062	14\\
60.8211513269597	14\\
60.8211513269597	15\\
61.7040043348388	15\\
61.7040043348388	16\\
65.2845919309203	16\\
65.2845919309203	17\\
68.936227168857	17\\
68.936227168857	18\\
69.3323714925064	18\\
69.3323714925064	19\\
69.3734724142791	19\\
69.3734724142791	20\\
70.7625137592869	20\\
70.7625137592869	21\\
71.1859865861832	21\\
71.1859865861832	22\\
71.3123730360775	22\\
71.3123730360775	23\\
71.4010257524899	23\\
71.4010257524899	24\\
73.8583806036058	24\\
73.8583806036058	25\\
80.8984458201233	25\\
80.8984458201233	26\\
85.5531194396147	26\\
85.5531194396147	27\\
85.7950259108089	27\\
85.7950259108089	28\\
90.7542865067465	28\\
90.7542865067465	29\\
92.5808050463237	29\\
92.5808050463237	30\\
92.6472804161133	30\\
92.6472804161133	31\\
93.4385282030853	31\\
93.4385282030853	32\\
93.8483868346353	32\\
93.8483868346353	33\\
95.1396814281817	33\\
95.1396814281817	34\\
95.5492670978414	34\\
95.5492670978414	35\\
95.7162666581019	35\\
95.7162666581019	36\\
102.573184175818	36\\
};

==> fig7b_part1b_220211.tex <==

\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
-0.100224851653294	0.273710617732178\\
0.629816877902954	0.270958132078619\\
1.46415028311009	0.268750654461968\\
2.08990033701544	0.267565741357387\\
2.08990033701544	0.522171797923576\\
2.22035576376598	0.507303854130427\\
2.35081119051652	0.493292028724611\\
2.49431215994213	0.478809087644464\\
2.63781312936773	0.465240802839261\\
2.78131409879333	0.452529410067854\\
2.93786061089398	0.439576220720582\\
3.09440712299464	0.427512833125974\\
3.26399917777034	0.415377490119553\\
3.39445460452089	0.40665892191231\\
3.39445460452089	0.661264978478499\\
3.50001033921747	0.642650220979618\\
3.60556607391403	0.624907623176739\\
3.7111218086106	0.607996321656231\\
3.83175693397811	0.589637154500593\\
3.95239205934563	0.572257720318049\\
4.07302718471313	0.555805735870976\\
4.19366231008064	0.540231708005408\\
4.31429743544815	0.525488784758821\\
4.4500119514866	0.509841295727696\\
4.58572646752505	0.495130026446333\\
4.7214409835635	0.481298961063359\\
4.85715549960194	0.468295435264935\\
4.90239367161476	0.464136179408072\\
4.90239367161476	0.718742235974275\\
5.00402974926254	0.698207577057644\\
5.10566582691034	0.678600123824495\\
5.20730190455814	0.65987800996561\\
5.30893798220592	0.642001259569881\\
5.41057405985372	0.624931701766755\\
5.52672957716547	0.60636535619129\\
5.64288509447724	0.588753971286906\\
5.759040611789	0.572048428616185\\
5.87519612910076	0.556202136150347\\
5.99135164641253	0.54117089832333\\
6.12202660338825	0.525182887176314\\
6.25270156036399	0.510116993213842\\
6.35433763801178	0.499002432852919\\
6.35433763801178	0.753608489419122\\
6.44754899220986	0.733293566063907\\
6.54076034640795	0.71382149257235\\
6.63397170060603	0.695157299780121\\
6.72718305480412	0.677267469365475\\
6.83903667984181	0.656776689912675\\
6.95089030487951	0.637301805301234\\
7.06274392991722	0.618792449349101\\
7.17459755495491	0.60120075293608\\
7.28645117999261	0.584481220204211\\
7.39830480503031	0.56859061089574\\
7.510158430068	0.553487828524766\\
7.64065432594532	0.536811641215905\\
7.77115022182264	0.521095982785653\\
7.90164611769995	0.506285527894377\\
8.03214201357727	0.492328137877294\\
8.16263790945459	0.479174677195672\\
8.21856472197344	0.473772009306757\\
8.21856472197344	0.72837806587296\\
8.31126185549647	0.709214005314195\\
8.40395898901949	0.690840751671715\\
8.49665612254252	0.673225672217342\\
8.58935325606554	0.656337480815779\\
8.68205038958855	0.640146182357284\\
8.80564656761926	0.619592307897136\\
8.92924274564996	0.600161460208213\\
9.05283892368065	0.581792279125509\\
9.17643510171135	0.564426757093145\\
9.30003127974206	0.548010055983895\\
9.42362745777275	0.532490333927271\\
9.54722363580345	0.517818581599442\\
9.67081981383414	0.503948467457988\\
9.79441599186484	0.490836191432706\\
9.94891121440321	0.475448692616098\\
10.1034064369416	0.46110484732354\\
10.25790165948	0.447733869997805\\
10.4123968820183	0.435269776095581\\
10.5668921045567	0.42365105645986\\
10.7213873270951	0.412820373777848\\
10.9067815941411	0.40078876599533\\
11.0921758611872	0.389729641734931\\
11.2775701282332	0.379564397686309\\
11.3084691727409	0.377951934196034\\
11.3084691727409	0.632557990762223\\
11.4177000205194	0.614701769474991\\
11.526930868298	0.597710579481713\\
11.6445640889826	0.580331755193313\\
11.7621973096672	0.563857881794448\\
11.8798305303518	0.548241836643257\\
12.0058661239424	0.532411585123555\\
12.131901717533	0.517462857037273\\
12.1487064633451	0.515533627336666\\
12.1487064633451	0.770139683902855\\
12.2500240268931	0.747354254403959\\
12.3513415904412	0.725594509547207\\
12.4526591539892	0.704814278204495\\
12.5539767175372	0.684969467638012\\
12.6552942810852	0.666017969941748\\
12.7566118446333	0.647919572694349\\
12.8579294081813	0.63063587363402\\
12.9592469717293	0.614130199174326\\
13.080828047987	0.595301182094659\\
13.2024091242446	0.57748463481397\\
13.3239902005022	0.560626115027091\\
13.4455712767599	0.544674107888625\\
13.5671523530175	0.529579868598191\\
13.6887334292751	0.515297273450159\\
13.8305780182424	0.49960198035437\\
13.9724226072096	0.484886832119599\\
14.1142671961768	0.471090620334991\\
14.1750577343057	0.465444914758535\\
14.1750577343057	0.720050971324738\\
14.2731125696284	0.700166801633657\\
14.3711674049511	0.681149529987863\\
14.4692222402738	0.66296136188889\\
14.5672770755966	0.645566150580038\\
14.6653319109193	0.628929325209114\\
14.7879004550727	0.609149541472121\\
14.9104689992261	0.59044175192966\\
15.0330375433795	0.572747858294662\\
15.1556060875329	0.556012911001403\\
15.2781746316863	0.54018493855591\\
15.4007431758397	0.525214786135066\\
15.5233117199931	0.511055962932957\\
15.6458802641465	0.497664497780633\\
15.7929625171306	0.482549256271824\\
15.9400447701147	0.468411639188375\\
16.0871270230988	0.455188415683708\\
16.2342092760829	0.442820444559402\\
16.381291529067	0.431252409754748\\
16.5528874908817	0.418698563480973\\
16.6264286173738	0.413610985595056\\
16.6264286173738	0.668217042161245\\
16.7289796173939	0.649803242856237\\
16.8394191558771	0.630909904515235\\
16.9498586943603	0.612941715668242\\
17.0602982328435	0.595853374549577\\
17.1786263097898	0.578471894680234\\
17.2969543867361	0.56200070781891\\
17.4152824636824	0.546392140616348\\
17.4152824636824	0.800998197182537\\
17.5056475416745	0.779383599710087\\
17.5960126196666	0.75863894967938\\
17.6954142054579	0.736782877362728\\
17.7948157912492	0.715892466793747\\
17.8942173770405	0.695925052364558\\
17.9936189628318	0.67683985355194\\
18.0930205486231	0.658597891628943\\
18.2014586422136	0.639615543505343\\
18.3098967358041	0.621546270221017\\
18.3189332436033	0.620080320430773\\
18.3189332436033	0.874686376996976\\
18.3895505407498	0.855391717097234\\
18.4954764864695	0.827586648192863\\
18.6014024321891	0.801088793829493\\
18.7073283779089	0.775836697232407\\
18.8132543236286	0.751771790927009\\
18.9191802693482	0.728838260902634\\
19.025106215068	0.706982917162478\\
19.1310321607877	0.686155070359462\\
19.2369581065073	0.666306414231798\\
19.342884052227	0.6473909135658\\
19.4488099979468	0.6293646974258\\
19.5547359436664	0.612185957403867\\
19.6606618893861	0.595814850653056\\
19.7665878351059	0.580213407479448\\
19.8725137808255	0.565345443278602\\
19.9784397265452	0.551176474612177\\
20.1196743208382	0.53331526776654\\
20.2609089151311	0.51656481910382\\
20.4021435094241	0.500856052455092\\
20.543378103717	0.486124187381321\\
20.6846126980099	0.472308472029226\\
20.8258472923028	0.459351932600256\\
20.9670818865958	0.44720113839989\\
21.1083164808887	0.435805981497921\\
21.2848597237549	0.42255334214056\\
21.461402966621	0.410322765455248\\
21.6379462094872	0.399035428493789\\
21.8144894523534	0.388618587247478\\
21.8497981009266	0.386633676953792\\
21.8497981009266	0.641239733519981\\
21.9579202357981	0.623143922266237\\
22.0660423706696	0.60591606793713\\
22.1741645055411	0.589514539394244\\
22.2943002109539	0.572211624749144\\
22.4144359163667	0.55582835716703\\
22.5345716217794	0.540315857557999\\
22.6667208977335	0.524202682525058\\
22.7988701736875	0.509029016892043\\
22.9310194496416	0.494740080771635\\
23.0511551550544	0.482474412989617\\
23.0511551550544	0.737080469555806\\
23.1510337246186	0.716078863628638\\
23.2509122941829	0.696009519062613\\
23.3507908637472	0.676831052772627\\
23.4506694333114	0.658503918668885\\
23.5505480028757	0.640990326112615\\
23.6504265724399	0.624254161991658\\
23.7503051420042	0.608260916255034\\
23.8501837115684	0.592977610753053\\
23.9833551376541	0.573649955184308\\
24.1165265637398	0.555457690899928\\
24.2496979898255	0.538334120034577\\
24.3828694159111	0.522216462848135\\
24.5160408419968	0.507045627557858\\
24.6492122680825	0.492765993691563\\
24.7823836941682	0.479325208167637\\
24.9155551202539	0.466673993354178\\
25.0487265463395	0.454765966403571\\
25.2151908289466	0.44085977662094\\
25.3816551115537	0.427967113773434\\
25.5481193941608	0.416014108824015\\
25.7145836767679	0.404932276543846\\
25.881047959375	0.394658123123392\\
26.0808050985035	0.383312697173722\\
26.280562237632	0.372952162371021\\
26.3804408071963	0.368114213283562\\
26.3804408071963	0.622720269849765\\
26.4907678217337	0.605170556196825\\
26.6051810219946	0.587877084806863\\
26.7236804079792	0.570889431015758\\
26.7890593795568	0.561901348730245\\
26.7890593795568	0.816507405296448\\
26.8787235724002	0.794437586806481\\
26.9703803028624	0.772788176452039\\
26.988313141431	0.768656919169729\\
26.988313141431	1.02326297573593\\
27.0663401208379	0.996801589840771\\
27.1443671002447	0.971262377832446\\
27.2223940796516	0.946613202139588\\
27.3004210590584	0.922823045178617\\
27.386250736406	0.897610341118906\\
27.4720804137535	0.873362458335166\\
27.557910091101	0.850042475754094\\
27.6437397684485	0.827614885170959\\
27.7295694457961	0.806045537182982\\
27.7685829354995	0.796516074699568\\
27.7685829354995	1.05112213126577\\
27.8451353371053	1.02419931344329\\
27.9233165132134	0.997653863878938\\
27.9314603857247	0.994942582826198\\
27.9314603857247	1.24954863939239\\
27.9964218087742	1.22086809843213\\
28.0613832318238	1.19302216271068\\
28.1263446548733	1.16598654517203\\
28.1913060779229	1.13973766551479\\
28.2562675009724	1.11425262962553\\
28.321228924022	1.08950920961074\\
28.3861903470715	1.06548582440976\\
28.4511517701211	1.04216152097194\\
28.5161131931706	1.01951595598149\\
28.5810746162201	0.997529378114152\\
28.6460360392697	0.97618261081027\\
28.743478173844	0.94532152522936\\
28.8409203084183	0.915797680304607\\
28.9383624429926	0.887553132106319\\
29.035804577567	0.860532447471286\\
29.1332467121413	0.834682595208832\\
29.2306888467156	0.809952842020991\\
29.3281309812899	0.786294652932611\\
29.4255731158642	0.763661596035917\\
29.5230152504385	0.742009251362589\\
29.6204573850129	0.721295123704408\\
29.7178995195872	0.701478559211594\\
29.8153416541615	0.682520665604997\\
29.9127837887358	0.664384235845432\\
30.0102259233101	0.647033675110748\\
30.1076680578845	0.630434930936772\\
30.2051101924588	0.614555426385536\\
30.3025523270331	0.599363996109247\\
30.4324751731322	0.580127748701656\\
30.5623980192313	0.561994763396029\\
30.6923208653304	0.544901764479576\\
30.8222437114295	0.528789105309926\\
30.9521665575286	0.513600560175988\\
31.0820894036276	0.499283128096209\\
31.179531538202	0.489086557880668\\
31.179531538202	0.743692614446871\\
31.2748345428439	0.723352064279126\\
31.3701375474858	0.703873957302577\\
31.4654405521278	0.685221725762091\\
31.5713327795077	0.665423103193021\\
31.6772250068876	0.646554994612472\\
31.7831172342675	0.628573666862764\\
31.8890094616474	0.611437442197612\\
32.0054909117654	0.593516340754775\\
32.1219723618833	0.576519530448635\\
32.2384538120012	0.560399340431061\\
32.2384538120012	0.81500539699725\\
32.3592743962575	0.785555257909564\\
32.4800949805138	0.757679069467414\\
32.6009155647701	0.73129271252192\\
32.7217361490265	0.706316563637714\\
32.8425567332828	0.682675254821419\\
32.9633773175391	0.660297446091207\\
33.0841979017954	0.639115610201472\\
33.2050184860517	0.619065828872593\\
33.325839070308	0.600087599911305\\
33.4466596545644	0.582123654639346\\
33.5674802388207	0.565119785079531\\
33.688300823077	0.549024680377855\\
33.8091214073333	0.533789771967946\\
33.9299419915896	0.519369087010602\\
34.0507625758459	0.505719109666217\\
34.1715831601022	0.492798649781463\\
34.2924037443586	0.480568718593887\\
34.4132243286149	0.468992411079554\\
34.5340449128712	0.4580347945884\\
34.7152757892557	0.442686570157406\\
34.8965066656401	0.428552175830461\\
35.0777375420246	0.415535614606242\\
35.2589684184091	0.403548481504899\\
35.4401992947936	0.392509363145265\\
35.621430171178	0.382343284807149\\
35.8026610475625	0.372981201223112\\
35.983891923947	0.36435952764171\\
36.2255330924596	0.353915177914217\\
36.4671742609722	0.344557383740394\\
36.7088154294849	0.336173107640448\\
36.9504565979975	0.328661071746708\\
37.1920977665101	0.321930534417504\\
37.4941492271509	0.314493305608721\\
37.7962006877917	0.308010302250992\\
38.0982521484325	0.302359093498794\\
38.279483024817	0.299322641892331\\
38.279483024817	0.553928698458535\\
38.4084893695246	0.537412222251234\\
38.5374957142322	0.521836532101716\\
38.6665020589398	0.507148040404758\\
38.7955084036473	0.493296211929717\\
38.9429442261703	0.478429028008733\\
39.0903800486933	0.464525659566263\\
39.2378158712162	0.451523624004267\\
39.3852516937392	0.439364489370462\\
39.5511169940775	0.426625094293641\\
39.7169822944158	0.414810969917227\\
39.8828475947542	0.403854913217543\\
40.0671423729079	0.392612246599143\\
40.122430806354	0.389419060699709\\
40.122430806354	0.644025117265898\\
40.2405462846732	0.624155624465971\\
40.3586617629924	0.605324905601393\\
40.4767772413117	0.587478653735417\\
40.5948927196309	0.570565401089326\\
40.7130081979501	0.554536370611771\\
40.8311236762694	0.539345335307843\\
40.9492391545886	0.52494848492266\\
41.0673546329078	0.511304299594499\\
41.185470111227	0.498373430113446\\
41.3035855895463	0.486118584440021\\
41.4217010678655	0.474504420156677\\
41.5988742853443	0.45821166298731\\
41.7760475028232	0.44317973237807\\
41.953220720302	0.429311058372079\\
42.1303939377809	0.416515621532682\\
42.3075671552597	0.404710368641162\\
42.4847403727386	0.393818673610966\\
42.6619135902174	0.383769840119555\\
42.8390868076962	0.374498642729435\\
43.0162600251751	0.365944903519804\\
43.2524909818135	0.355560627095258\\
43.488721938452	0.346233745207329\\
43.7249528950905	0.337856587069865\\
43.9611838517289	0.330332445636174\\
44.1974148083674	0.323574461199783\\
44.4927035041654	0.316086306121079\\
44.7879921999635	0.309538811867725\\
45.0832808957616	0.303813812779566\\
45.4376273307193	0.297884963359536\\
45.7919737656769	0.292838225168921\\
46.0282047223154	0.289898146020803\\
46.0282047223154	0.544504202587007\\
46.1412820731417	0.530447290712317\\
46.254359423968	0.517094724731976\\
46.3674367747943	0.50441121217608\\
46.4805141256206	0.492363228965047\\
46.65013015186	0.475413650783807\\
46.8197461780995	0.459721910542498\\
46.9893622043389	0.445194663364575\\
47.1589782305784	0.431745491550402\\
47.3285942568178	0.419294390507531\\
47.4982102830573	0.407767292830314\\
47.6678263092967	0.397095627697837\\
47.8374423355362	0.387215912969225\\
48.0070583617756	0.378069377549778\\
48.2332130634282	0.366921044202613\\
48.4593677650808	0.356861933976504\\
48.6855224667334	0.347785626748333\\
48.911677168386	0.339596099936472\\
49.1378318700386	0.332206712632129\\
49.4205252471043	0.323976816885306\\
49.7032186241701	0.316739437150673\\
49.9859120012358	0.310374877132574\\
50.3251440537147	0.303742231148519\\
50.6643761061936	0.298057482736283\\
51.0036081586725	0.29318516411891\\
51.3993788865645	0.288373659120367\\
51.6820722636303	0.285429979482672\\
51.6820722636303	0.540036036048875\\
51.8104476490947	0.524385580096151\\
51.9388230345592	0.509622347243095\\
52.0778963688124	0.494571786290024\\
52.2169697030656	0.48044331950436\\
52.3560430373187	0.467180453466611\\
52.5058143203606	0.453804649163871\\
52.6555856034025	0.441309250203389\\
52.7518671425009	0.433714282662677\\
52.7518671425009	0.688320339228866\\
52.8419061297332	0.671301196687409\\
52.9619581127097	0.649666014469204\\
53.0820100956862	0.629179958922492\\
53.2020620786626	0.609781995566763\\
53.3221140616391	0.591414331694537\\
53.4421660446156	0.574022244188413\\
53.5622180275921	0.55755391648357\\
53.6822700105685	0.541960284189628\\
53.802321993545	0.527194888912305\\
53.9223739765215	0.513213739839017\\
54.0424259594979	0.49997518267628\\
54.1924909382185	0.484411369944965\\
54.3425559169391	0.469873919999941\\
54.4926208956597	0.456295148875398\\
54.6426858743803	0.443611836055737\\
54.7927508531009	0.431764930131351\\
54.9428158318215	0.420699273864955\\
55.1228938062862	0.408379437678946\\
55.3029717807509	0.397027980476352\\
55.4830497552156	0.386568784535996\\
55.6631277296803	0.376931715235884\\
55.7531667169127	0.372401080503366\\
55.7531667169127	0.627007137069555\\
55.8666232208283	0.608756837594299\\
55.9800797247438	0.591423988794588\\
56.0935362286594	0.574962470016715\\
56.206992732575	0.55932847911275\\
56.3204492364905	0.544480415888273\\
56.4339057404061	0.53037877140909\\
56.5473622443216	0.516986022872743\\
56.6608187482372	0.504266533764763\\
56.7742752521528	0.492186459034087\\
56.9444600080261	0.475195378761981\\
57.1146447638995	0.459469282799162\\
57.2848295197728	0.444913993184187\\
57.4550142756461	0.431442343495874\\
57.6251990315195	0.418973656844813\\
57.7953837873928	0.407433262728318\\
57.9655685432662	0.39675204985555\\
58.1357532991395	0.386866052264665\\
58.3059380550129	0.377716066253612\\
58.532851062844	0.366566876232795\\
58.7597640706751	0.356510460384129\\
58.9866770785062	0.347439711788724\\
59.2135900863374	0.339258021480831\\
59.4405030941685	0.331878249503902\\
59.7241443539574	0.323662236079514\\
60.0077856137463	0.316440177226411\\
60.2914268735352	0.310091826586799\\
60.6317963852819	0.303479194461147\\
60.9721658970286	0.297814529580236\\
61.3125354087753	0.292961934183523\\
61.4259919126909	0.291504235698966\\
61.4259919126909	0.546110292265155\\
61.5399286595469	0.531868217755971\\
61.6538654064028	0.518345051387954\\
61.8057810688775	0.501370008569296\\
61.9576967313522	0.485527726981488\\
62.1096123938268	0.470742616358308\\
62.2615280563015	0.456944130645994\\
62.4134437187761	0.444066431398028\\
62.5653593812508	0.432048073631961\\
62.7172750437255	0.420831712649132\\
62.8691907062001	0.410363830418802\\
63.0590852842934	0.398255755760673\\
63.2489798623867	0.387149091279625\\
63.4388744404801	0.376961014365847\\
63.6287690185734	0.367615552334655\\
63.8186635966667	0.359043015896646\\
64.0465370903787	0.349686604012192\\
64.2744105840907	0.341250933530034\\
64.5022840778027	0.33364539656111\\
64.7681364871333	0.325712936164948\\
65.033988896464	0.318683509574441\\
65.2238834745573	0.31415794567242\\
65.2238834745573	0.568764002238609\\
65.3400154601906	0.553089737303821\\
65.456147445824	0.538221519711399\\
65.5722794314573	0.524117898565819\\
65.7116378142173	0.508147602481529\\
65.8509961969773	0.493157692044491\\
65.9903545797374	0.479087983272365\\
66.1297129624974	0.465881986761318\\
66.2690713452574	0.453486680882975\\
66.4316561251441	0.439983891126417\\
66.5942409050307	0.427443129274664\\
66.7568256849174	0.415795854107259\\
66.9194104648041	0.404978407732855\\
67.1052216418175	0.393556081906638\\
67.2910328188308	0.383058982630473\\
67.4768439958441	0.373412165082954\\
67.5465231872242	0.36999958166119\\
67.5465231872242	0.624605638227379\\
67.6614670940335	0.606244541380946\\
67.7764110008428	0.588818252377237\\
67.8913549076521	0.572279177888362\\
68.0062988144614	0.55658214767783\\
68.1356107096218	0.539876201628317\\
68.2649226047823	0.524124022135496\\
68.3942344999428	0.509271157290925\\
68.5235463951032	0.495266263924151\\
68.6672262786148	0.480641017741661\\
68.8109061621265	0.466940529356961\\
68.9545860456381	0.454106326114385\\
68.9833220223404	0.451638557059425\\
68.9833220223404	0.706244613625614\\
69.0801664139852	0.687195194242832\\
69.17701080563	0.668966251792114\\
69.2738551972747	0.651522447537801\\
69.3706995889195	0.634829964817769\\
69.4675439805643	0.618856443486294\\
69.564388372209	0.603570917180434\\
69.6935142277354	0.584209397962368\\
69.8226400832617	0.565951711729724\\
69.9517659387881	0.548734927095481\\
70.0808917943145	0.532499700497496\\
70.2100176498408	0.517190071650532\\
70.3391435053672	0.502753270660008\\
70.4682693608935	0.489139536132285\\
70.5973952164199	0.476301943655074\\
70.7265210719462	0.464196244056211\\
70.8879283913542	0.450030004752392\\
71.0493357107621	0.436866017337692\\
71.2107430301701	0.424633373166017\\
71.372150349578	0.41326618033024\\
71.533557668986	0.402703208731253\\
71.7272464522755	0.391009388978517\\
71.920935235565	0.380301204195916\\
72.1146240188546	0.370495578338591\\
72.2114684104993	0.365907194900231\\
72.2114684104993	0.62051325146642\\
72.3221988844768	0.603009309853235\\
72.4329293584543	0.586364684769919\\
72.5515691520016	0.569436850204028\\
72.6702089455489	0.553397823615057\\
72.7967580586661	0.53721665794788\\
72.9233071717832	0.521940123429701\\
73.0024003674814	0.512829080573098\\
73.0024003674814	0.767435137139287\\
73.101625829935	0.745228956629887\\
73.2008512923885	0.724002207128294\\
73.3000767548421	0.703711689620675\\
73.3993022172956	0.684316110439056\\
73.4985276797492	0.665775997223619\\
73.6087781935865	0.646133360531778\\
73.7190287074237	0.627450958859839\\
73.829279221261	0.609681850887881\\
73.9395297350983	0.59278139003365\\
74.0608053003193	0.575143552195399\\
74.1049055058542	0.568967092475489\\
74.1049055058542	0.823573149041678\\
74.1904409044489	0.802230472099353\\
74.2854802362207	0.779469694114013\\
74.3805195679926	0.757671364689145\\
74.4755588997645	0.736794786304145\\
74.5705982315363	0.716800982349241\\
74.6656375633082	0.697652624356138\\
74.7701808282572	0.677523298455199\\
74.8747240932062	0.658328261563639\\
74.9792673581553	0.640024149290767\\
75.0552988235728	0.627247969265795\\
75.0552988235728	0.881854025831984\\
75.1462945038532	0.856815151183568\\
75.2372901841337	0.832790932924325\\
75.3282858644141	0.809740253887369\\
75.4192815446946	0.7876236631067\\
75.510277224975	0.766403308297427\\
75.6012729052555	0.746042871071907\\
75.6922685855359	0.726507504781395\\
75.7962636487136	0.705148835526913\\
75.9002587118912	0.684776437928107\\
76.0042537750689	0.665344769270334\\
76.1082488382465	0.646810389848667\\
76.2122439014242	0.629131865857943\\
76.3162389646019	0.612269676767042\\
76.3552371132935	0.606149067105932\\
76.3552371132935	0.860755123672121\\
76.4421608119982	0.83763220561498\\
76.529084510703	0.815405195759737\\
76.6188121996886	0.793364120327666\\
76.6356361413734	0.789330578136628\\
76.6356361413734	1.04393663470283\\
76.710127962837	1.01796556061838\\
76.7903499244132	0.990962989769457\\
76.8705718859895	0.964927445583299\\
76.9507938475657	0.939824296521607\\
77.0310158091419	0.915620151284301\\
77.1169679108307	0.890648203348704\\
77.2029200125195	0.866633200198706\\
77.2086501526321	0.865065318329343\\
77.2086501526321	1.11967137489553\\
77.2771461208363	1.0934363815462\\
77.3456420890404	1.06800572335321\\
77.4141380572446	1.04335474031245\\
77.4826340254488	1.01945952846759\\
77.5511299936529	0.996296916730515\\
77.6196259618571	0.973844444412364\\
77.7109539194626	0.944974941775001\\
77.8022818770682	0.917279508851237\\
77.8936098346737	0.890710398379525\\
77.9849377922792	0.865221804891888\\
78.0762657498848	0.840769785744712\\
78.1675937074903	0.817312185361075\\
78.2589216650959	0.794808562554039\\
78.3502496227014	0.773220120805561\\
78.4415775803069	0.752509641380797\\
78.5329055379125	0.732641419162618\\
78.624233495518	0.713581201095451\\
78.7155614531236	0.695296127132707\\
78.8068894107291	0.677754673585596\\
78.921049357736	0.65682761937974\\
79.035209304743	0.636958932314172\\
79.1493692517499	0.618095086412765\\
79.2635291987568	0.600185262728004\\
79.3776891457638	0.58318121243542\\
79.4918490927707	0.567037126851872\\
79.4918490927707	0.821643183418075\\
79.5799633725396	0.799745608289754\\
79.6727152459807	0.777623776191064\\
79.7654671194217	0.756415331534129\\
79.8582189928627	0.736082561501377\\
79.9556084599757	0.71563605725251\\
79.9556084599757	0.970242113818713\\
79.99303842984	0.958325846623268\\
79.99303842984	1.21293190318947\\
80.0631251002686	1.18317268873926\\
80.133211770697	1.15434671090841\\
80.2032984411256	1.1264247037837\\
80.2797566270476	1.09696202043838\\
80.3562148129696	1.06850581833721\\
80.4326729988916	1.04102171485175\\
80.5091311848136	1.01447650190609\\
80.5855893707356	0.988838105852793\\
80.6301899791901	0.974288784750811\\
80.6301899791901	1.22889484131701\\
80.6999718253276	1.19876456662196\\
80.7271092099367	1.18730295608826\\
80.7271092099367	1.44190901265445\\
80.7878769618058	1.40981321744434\\
80.8573258210849	1.37420175631568\\
80.9267746803639	1.33969705254881\\
80.9962235396429	1.30626470958099\\
81.065672398922	1.27387139984934\\
81.135121258201	1.24248483156784\\
81.2045701174801	1.21207371653666\\
81.2740189767591	1.1826077389521\\
81.3434678360381	1.15405752518572\\
81.4129166953172	1.12639461450281\\
81.4823655545962	1.09959143069089\\
81.5604955212851	1.07043225515569\\
81.5952199509247	1.05780136908908\\
81.5952199509247	1.31240742565528\\
81.6609438993236	1.28154488683523\\
81.7313624154653	1.24948531175956\\
81.801780931607	1.21843579611256\\
81.8721994477487	1.18836451726254\\
81.9426179638904	1.15924065517223\\
82.0130364800321	1.13103436081117\\
82.0646767252026	1.11091613489724\\
82.0646767252026	1.36552219146343\\
82.1280551727764	1.33423673706643\\
82.1984756700805	1.30051613467418\\
82.2688961673846	1.26785795295633\\
82.3393166646888	1.23622871867668\\
82.4097371619929	1.20559601322599\\
82.480157659297	1.1759284393944\\
82.5505781566012	1.14719558919056\\
82.6209986539053	1.11936801267477\\
82.6914191512095	1.09241718777407\\
82.768881698244	1.06375098603984\\
82.768881698244	1.31835704260602\\
82.8328841188635	1.28812057566807\\
82.9039979195518	1.25554036159721\\
82.9751117202401	1.22399658200383\\
83.0462255209284	1.19345626606629\\
83.1173393216167	1.16388749182342\\
83.1884531223049	1.13525935280825\\
83.2595669229932	1.10754192574349\\
83.3306807236815	1.08070623926442\\
83.4089059044387	1.05217194393455\\
83.480019705127	1.0270976749231\\
83.480019705127	1.28170373148929\\
83.5475477892749	1.25093518708155\\
83.617122179003	1.22020687478833\\
83.684650263151	1.19129751913802\\
83.684650263151	1.44590357570421\\
83.7504642233724	1.41106442993451\\
83.8162781835938	1.3772522122174\\
83.8820921438152	1.34443665254473\\
83.9479061040366	1.31258837315532\\
84.013720064258	1.28167886223478\\
84.0842350216381	1.24957185347867\\
84.1547499790182	1.21847776186367\\
84.1547499790182	1.47308381842987\\
84.187095720882	1.45543432522587\\
84.187095720882	1.71004038179206\\
84.2482690198965	1.67037941523378\\
84.309442318911	1.6318062149692\\
84.3706156179255	1.59429094724455\\
84.43178891694	1.55780459654514\\
84.4929622159545	1.52231894315381\\
84.5541355149689	1.48780654132484\\
84.5694288397226	1.47932736709556\\
84.5694288397226	1.73393342366175\\
84.6308777770248	1.69343801771548\\
84.692326714327	1.65405819878528\\
84.7537756516291	1.61576323414084\\
84.8152245889313	1.57852323769194\\
84.8766735262335	1.54230914666481\\
84.9381224635357	1.50709269892104\\
84.9995714008379	1.47284641090125\\
85.0610203381401	1.43954355617646\\
85.1224692754422	1.40715814459024\\
85.1839182127444	1.3756649019756\\
85.2453671500466	1.34503925043046\\
85.3068160873488	1.31525728913671\\
85.368265024651	1.2862957757075\\
85.4297139619532	1.25813210804853\\
85.4911628992554	1.23074430671886\\
85.5526118365575	1.20411099777787\\
85.6140607738597	1.17821139610454\\
85.6959926902626	1.14478506156374\\
85.7779246066656	1.11258084789732\\
85.8598565230685	1.08155407238873\\
85.9417884394714	1.05166168599385\\
86.0237203558743	1.02286221361123\\
86.1056522722772	0.99511569653626\\
86.1875841886801	0.96838363701923\\
86.269516105083	0.942628944850426\\
86.3514480214859	0.917815885898221\\
86.4333799378889	0.893910032528652\\
86.5153118542918	0.870878215837791\\
86.5972437706947	0.848688479630468\\
86.6177267497954	0.843268987650447\\
86.6177267497954	1.09787504421665\\
86.6939992362672	1.0694556488512\\
86.770271722739	1.04200477743106\\
86.8465442092108	1.01548942296854\\
86.9228166956826	0.989877703343595\\
86.9990891821544	0.965138822968669\\
87.0753616686262	0.941243035760053\\
87.162530224594	0.914929110948549\\
87.2496987805617	0.889637546829618\\
87.3368673365295	0.865328622176079\\
87.4240358924973	0.841964159028109\\
87.5112044484651	0.819507462733483\\
87.5983730044328	0.797923264317518\\
87.6855415604006	0.77717766509187\\
87.7073336993925	0.772118450048126\\
87.7073336993925	1.02672450661431\\
87.7849110598406	1.00029297680651\\
87.8641046152979	0.974255300613081\\
87.8689532003259	0.972691405262637\\
87.8689532003259	1.22729746182883\\
87.9367072696219	1.19807777143741\\
88.0044613389178	1.16974436918575\\
88.0722154082138	1.14227037228841\\
88.1484387361717	1.11235695772852\\
88.2246620641297	1.0834623370896\\
88.3008853920876	1.0555518121913\\
88.3771087200456	1.02859186660717\\
88.4533320480035	1.00255012541648\\
88.5295553759614	0.977395316326536\\
88.6057787039194	0.953097232119433\\
88.6904712905393	0.927068706279329\\
88.7158790665253	0.919453569654237\\
88.7158790665253	1.17405962622043\\
88.7805904067587	1.14767628219028\\
88.8453017469921	1.12205778246816\\
88.9100130872255	1.09718195447371\\
88.9747244274589	1.07302726840226\\
89.0394357676923	1.04957281859095\\
89.1041471079257	1.02679830542509\\
89.1688584481591	1.00468401776907\\
89.2335697883925	0.983210815906418\\
89.2982811286259	0.9623601149747\\
89.3629924688593	0.942113868880384\\
89.4277038090927	0.922454554680158\\
89.4924151493261	0.903365157414967\\
89.5571264895595	0.884829155383727\\
89.6218378297929	0.866830505843922\\
89.6865491700263	0.849353631126789\\
89.7512605102597	0.832383405154943\\
89.8159718504931	0.815905140350921\\
89.8806831907265	0.799904574925236\\
90.0101058711932	0.769281550287744\\
90.13952855166	0.740408292497449\\
90.2689512321268	0.713184821749749\\
90.3983739125936	0.687516870979081\\
90.5277965930604	0.663315559439042\\
90.6572192735272	0.640497084933997\\
90.786641953994	0.618982433636006\\
90.9160646344608	0.598697106482703\\
91.0454873149276	0.57957086120841\\
91.1749099953944	0.561537469115308\\
91.3043326758612	0.54453448574246\\
91.433755356328	0.528503034638604\\
91.5631780367948	0.513387603489861\\
91.6926007172616	0.499135851896568\\
91.8220233977284	0.485698430133468\\
91.9514460781952	0.473028808265738\\
92.0808687586619	0.461083115029268\\
92.2102914391288	0.449819985917003\\
92.3397141195955	0.439200419945536\\
92.5338481402957	0.424397889875635\\
92.7279821609959	0.410845761438338\\
92.9221161816961	0.398438410511602\\
93.1162502023963	0.387079135270696\\
93.3103842230965	0.37667940250256\\
93.5045182437967	0.367158157585521\\
93.6986522644969	0.358441192756587\\
93.8927862851971	0.350460568742506\\
94.1516316461307	0.34085841459104\\
94.4104770070643	0.332322224395853\\
94.6693223679978	0.324733662298357\\
94.9281677289314	0.317987529258787\\
95.187013089865	0.311990304698625\\
95.187013089865	0.566596361264814\\
95.3201456611161	0.548823487631154\\
95.4532782323673	0.532094375075232\\
95.5864108036184	0.516347725845776\\
95.7195433748695	0.501525842071217\\
95.8526759461206	0.487574414346795\\
95.9858085173717	0.474442322737502\\
96.1189410886229	0.462081449467661\\
96.2853568026868	0.44764613978252\\
96.4517725167507	0.434262625459709\\
96.6181882308146	0.421854269869428\\
96.7846039448785	0.410350020332189\\
96.9510196589424	0.399684001257214\\
97.1174353730063	0.389795136925869\\
97.317134229883	0.378874909101171\\
97.5168330867596	0.368902396949252\\
97.7165319436363	0.359795352644241\\
97.916230800513	0.35147866626572\\
98.1492128002024	0.342683617676087\\
98.3821947998919	0.334772461996408\\
98.515327371143	0.330614086948316\\
98.515327371143	0.585220143514505\\
98.6680887410421	0.563667213453897\\
98.8208501109412	0.543560263401872\\
98.9736114808402	0.524802282966846\\
99.1263728507393	0.507302770157068\\
99.2791342206384	0.490977294733952\\
99.4318955905374	0.475747090859798\\
99.5846569604365	0.461538677074842\\
99.7374183303355	0.448283501769708\\
99.8901797002346	0.43591761244322\\
100.042941070134	0.424381347149492\\
};\addlegendentry{Hawkes};
\addplot [color=red, dashed, line width=1.0pt]
  table[row sep=crcr]{%
-0.100224851653294	0.19049327058849\\
1.88131698571365	0.190150453516424\\
2.08990033701544	0.190140412489072\\
2.08990033701544	0.621480165315617\\
2.23340130644104	0.585523939681252\\
2.35081119051652	0.556954119691682\\
2.46822107459202	0.52932700131143\\
2.57258541599245	0.505675928530565\\
2.67694975739289	0.482964229546155\\
2.78131409879333	0.461257690322881\\
2.87263289751871	0.44312813668914\\
2.9639516962441	0.425829040927184\\
3.05527049496948	0.409374425337035\\
3.14658929369486	0.393770028046916\\
3.23790809242024	0.379014032504784\\
3.32922689114562	0.365097869901007\\
3.39445460452089	0.355664125531121\\
3.39445460452089	0.890719439764311\\
3.50001033921747	0.866653166967239\\
3.60556607391403	0.841725869887199\\
3.72620119928155	0.812318134726766\\
3.86191571532	0.778279913684386\\
4.02778901270031	0.735718081613825\\
4.51032951417035	0.611229643649253\\
4.6460440302088	0.577473860022707\\
4.76667915557631	0.548386398618121\\
4.87223489027288	0.523785736010439\\
4.90239367161476	0.516917966747243\\
4.90239367161476	0.987200277266069\\
4.98951030959857	0.971349519672899\\
5.09114638724637	0.95188836330577\\
5.19278246489417	0.931405517230473\\
5.29441854254195	0.90993689058179\\
5.39605462018974	0.887532985782045\\
5.49769069783754	0.864259238172068\\
5.61384621514929	0.836699190706327\\
5.73000173246106	0.808250860200673\\
5.87519612910076	0.77169392768883\\
6.04942940506841	0.726846558469489\\
6.35433763801178	0.647778998588919\\
6.35433763801178	1.03018899927349\\
6.44754899220986	1.01568079267399\\
6.54076034640795	1.00029357395105\\
6.63397170060603	0.984020835309664\\
6.72718305480412	0.966863742227716\\
6.82039440900219	0.948831994716542\\
6.91360576320028	0.9299445898003\\
7.00681711739836	0.9102304430223\\
7.10002847159645	0.889728826472179\\
7.21188209663414	0.864158349211152\\
7.32373572167184	0.837632327203153\\
7.45423161754915	0.805648072020446\\
7.60336978426609	0.768016338077189\\
7.78979249266226	0.719944024851387\\
8.14399563861498	0.628338856602568\\
8.21856472197344	0.6094439049252\\
8.21856472197344	1.01950758862129\\
8.31126185549647	1.00443411596967\\
8.40395898901949	0.988485856118359\\
8.49665612254252	0.971661858799067\\
8.58935325606554	0.953969302846872\\
8.68205038958855	0.935424268082002\\
8.77474752311159	0.916052382155982\\
8.8674446566346	0.895889301312451\\
8.96014179015764	0.874980985473698\\
9.08373796818833	0.846042744667983\\
9.20733414621903	0.816042043034187\\
9.33093032424972	0.785169428854161\\
9.48542554678809	0.745683433970399\\
10.0416083479262	0.602416933891035\\
10.1652045259569	0.571867751086003\\
10.2888007039876	0.542269838088501\\
10.4123968820183	0.513802403777945\\
10.5050940155414	0.49328433565293\\
10.5977911490644	0.473537252258268\\
10.6904882825874	0.454601609763799\\
10.7831854161104	0.436507679167406\\
10.8758825496335	0.419275935577062\\
10.9685796831565	0.402917632440619\\
11.0612768166795	0.38743552003568\\
11.1539739502025	0.372824667388969\\
11.2466710837255	0.359073348779319\\
11.3084691727409	0.350374842505559\\
11.3084691727409	0.886050518886051\\
11.4177000205194	0.86094729547014\\
11.526930868298	0.83494657160324\\
11.6529664618886	0.803988570355813\\
11.7958068012913	0.767922742763361\\
11.9806590052243	0.720256581090112\\
12.1487064633451	0.676591374116171\\
12.1487064633451	1.03742033344174\\
12.2500240268931	1.022103000013\\
12.3513415904412	1.00575313580163\\
12.4526591539892	0.988358869412309\\
12.5539767175372	0.969918598106688\\
12.6552942810852	0.950442325845557\\
12.7566118446333	0.929952855832454\\
12.8579294081813	0.908486762776036\\
12.9592469717293	0.886095068737703\\
13.0605645352774	0.862843550483078\\
13.182145611535	0.83392097437509\\
13.3037266877926	0.804042204353806\\
13.4455712767599	0.768231988228365\\
13.6279428911463	0.72121480467257\\
13.9926861199192	0.626900860788965\\
14.1345307088864	0.591211475845469\\
14.1750577343057	0.581199650252728\\
14.1750577343057	1.01073629354015\\
14.2731125696284	0.994220457156217\\
14.3711674049511	0.976724197526707\\
14.4692222402738	0.958252798640558\\
14.5672770755966	0.938822414305903\\
14.6653319109193	0.918460972933019\\
14.763386746242	0.897208863296257\\
14.8614415815647	0.875119341973445\\
14.9594964168875	0.852258608954372\\
15.0820649610409	0.822719441848278\\
15.2046335051943	0.792279265657498\\
15.3517157581784	0.75485251771164\\
15.5968528464852	0.691330781585691\\
15.841989934792	0.628077067517893\\
15.9890721877761	0.591057520299302\\
16.1116407319295	0.561083653578152\\
16.2342092760829	0.532112131971331\\
16.3322641114056	0.509768128851476\\
16.4303189467283	0.48824176526503\\
16.528373782051	0.467590446614636\\
16.6264286173738	0.447858647910806\\
16.6264286173738	0.954386790311773\\
16.7210910789308	0.935459314900228\\
16.8157535404878	0.915669534010632\\
16.918304540508	0.893301940640043\\
17.0208555405281	0.870030453451875\\
17.1312950790113	0.844048588749942\\
17.2496231559576	0.815283187179872\\
17.38372830983	0.781731703042396\\
17.4152824636824	0.77371843247613\\
17.4152824636824	1.05782941780517\\
17.5146840494737	1.0442408786642\\
17.614085635265	1.02969029623108\\
17.7044507132571	1.01560809130798\\
17.7948157912492	1.00069965952535\\
17.8851808692413	0.984958996499742\\
17.9755459472333	0.968386856095563\\
18.0659110252254	0.950991491123901\\
18.1653126110167	0.930925610829874\\
18.264714196808	0.909917714321196\\
18.3189332436033	0.898078213187802\\
18.3189332436033	1.07751623590829\\
18.424859189323	1.06456664993424\\
18.5307851350427	1.05057779062979\\
18.6367110807624	1.03551098912455\\
18.7426370264821	1.01933491559844\\
18.8485629722018	1.00202732880206\\
18.9544889179215	0.983576862555566\\
19.0604148636412	0.963984778501128\\
19.1663408093609	0.943266599962783\\
19.2722667550806	0.921453530309336\\
19.3781927008003	0.898593552691352\\
19.48411864652	0.874752108378502\\
19.5900445922397	0.850012259788883\\
19.6959705379594	0.82447426264315\\
19.8372051322523	0.789385307626972\\
20.0137483751185	0.744304917291004\\
20.543378103717	0.60774024099068\\
20.6846126980099	0.572737994235439\\
20.7905386437296	0.547280708124077\\
20.8964645894493	0.522633177129094\\
21.002390535169	0.498893843393674\\
21.1083164808887	0.476143879502061\\
21.2142424266084	0.454446827190964\\
21.3201683723281	0.433848819965291\\
21.4260943180478	0.414379311609324\\
21.5320202637675	0.39605221528349\\
21.6379462094872	0.378867350010339\\
21.7438721552069	0.362812091826044\\
21.8497981009266	0.347863134026966\\
21.8497981009266	0.883783680303779\\
21.9579202357981	0.858853774979835\\
22.0660423706696	0.833053428394535\\
22.1861780760824	0.803509636252414\\
22.3303409225777	0.767094057698742\\
22.5225580512381	0.717502018822046\\
22.8709515969352	0.627422745735601\\
23.0151144434305	0.591144672855776\\
23.0511551550544	0.582237100742077\\
23.0511551550544	1.01107353025117\\
23.1510337246186	0.994262237993652\\
23.2509122941829	0.976433744699037\\
23.3507908637472	0.957593714946057\\
23.4506694333114	0.937759530829879\\
23.5505480028757	0.916961278268545\\
23.6504265724399	0.895242486343449\\
23.7503051420042	0.872660552442838\\
23.8501837115684	0.849286792985154\\
23.9833551376541	0.817038585624445\\
24.1165265637398	0.783770799806959\\
24.2829908463469	0.741166413694742\\
24.7823836941682	0.612294685364944\\
24.9155551202539	0.579132778835131\\
25.0487265463395	0.547019926845991\\
25.1486051159038	0.523764381128316\\
25.248483685468	0.501312686772891\\
25.3483622550323	0.479734003216592\\
25.4482408245966	0.459083552026826\\
25.5481193941608	0.439402729521987\\
25.6479979637251	0.420719585110604\\
25.7478765332893	0.403049603665707\\
25.8477551028536	0.386396724100308\\
25.9476336724179	0.370754525297485\\
26.0475122419821	0.356107513807842\\
26.1473908115464	0.342432454192547\\
26.2472693811106	0.329699691449392\\
26.3471479506749	0.317874424579017\\
26.3804408071963	0.314127728875263\\
26.3804408071963	0.849823973216701\\
26.4948540074573	0.822202648705911\\
26.621525764889	0.790716015704803\\
26.7727146366624	0.752199106000802\\
26.7890593795568	0.747990514883426\\
26.7890593795568	1.05293931164736\\
26.8847011852565	1.03954464456011\\
26.9803429909561	1.02525153851664\\
26.988313141431	1.02401926251169\\
26.988313141431	1.09258014567989\\
27.0897482146599	1.08140507224914\\
27.1911832878888	1.06933135422483\\
27.2926183611177	1.05631865715132\\
27.386250736406	1.04344227326723\\
27.4798831116942	1.02971090502032\\
27.5735154869824	1.01510539567141\\
27.6671478622706	0.999612536154856\\
27.7607802375588	0.983226029869385\\
27.7685829354995	0.981820137799687\\
27.7685829354995	1.08796318616308\\
27.8695669546391	1.07646674496092\\
27.9314603857247	1.06897434445266\\
27.9314603857247	1.09709762393192\\
28.028902520299	1.08673555555714\\
28.1263446548733	1.07556262204018\\
28.2237867894476	1.06354158862489\\
28.321228924022	1.05063835720118\\
28.4186710585963	1.0368229829914\\
28.5161131931706	1.02207076992441\\
28.6135553277449	1.00636342229222\\
28.7109974623192	0.989690222365908\\
28.8084395968935	0.972049195585143\\
28.9058817314679	0.953448217335662\\
29.0033238660422	0.933906008939047\\
29.1007660006165	0.913452966146622\\
29.1982081351908	0.892131762021862\\
29.2956502697651	0.869997668403215\\
29.3930924043395	0.847118546749485\\
29.5230152504385	0.815594185398169\\
29.6529380965376	0.783109925587894\\
29.8153416541615	0.741540666098246\\
30.3350330385579	0.607546786745388\\
30.464955884657	0.575311719340391\\
30.5948787307561	0.544102932324137\\
30.6923208653304	0.521498186542104\\
30.7897629999047	0.499665728203993\\
30.887205134479	0.478668657732655\\
30.9846472690533	0.458557440785327\\
31.0820894036276	0.439370029940989\\
31.179531538202	0.421132299374747\\
31.179531538202	0.938799422026477\\
31.2748345428439	0.919020747848379\\
31.3701375474858	0.898399454780829\\
31.4760297748658	0.874557920952171\\
31.5819220022457	0.849819287054004\\
31.6984034523636	0.821690825154008\\
31.8254741252195	0.790089748439129\\
31.9843124662894	0.749589913754164\\
32.2384538120012	0.683675982941963\\
32.2384538120012	1.0391050691489\\
32.3592743962575	1.02086073717041\\
32.4800949805138	1.00114674972963\\
32.6009155647701	0.979945970197306\\
32.7217361490265	0.957262767365577\\
32.8425567332828	0.933126118362793\\
32.9633773175391	0.907592193717591\\
33.0841979017954	0.880746165550278\\
33.2050184860517	0.85270298892118\\
33.325839070308	0.823606944517451\\
33.4466596545644	0.793629799979968\\
33.6278905309488	0.747446257464304\\
34.1715831601022	0.607266975763991\\
34.2924037443586	0.577266679687284\\
34.4132243286149	0.548142022961869\\
34.5340449128712	0.520065542339992\\
34.6548654971275	0.493182363670286\\
34.7756860813838	0.467608321197801\\
34.8965066656401	0.443429461083383\\
35.0173272498965	0.420702788939892\\
35.1381478341528	0.399458051165794\\
35.2589684184091	0.379700300796841\\
35.3797890026654	0.361412988747489\\
35.5006095869217	0.344561335516431\\
35.621430171178	0.32909576973131\\
35.7422507554344	0.314955261047487\\
35.8630713396907	0.302070419436021\\
35.983891923947	0.290366275779519\\
36.1047125082033	0.279764696574603\\
36.2255330924596	0.270186416595664\\
36.3463536767159	0.261552697044564\\
36.4671742609722	0.253786633328303\\
36.5879948452286	0.246814147054948\\
36.7088154294849	0.240564702261381\\
36.8296360137412	0.234971787477377\\
37.0108668901257	0.227678564101026\\
37.1920977665101	0.22153247223865\\
37.3733286428946	0.216364660762693\\
37.5545595192791	0.212027585930144\\
37.7962006877917	0.207318807496137\\
38.0378418563044	0.203607424405163\\
38.279483024817	0.200687462756534\\
38.279483024817	0.651884046521388\\
38.4453483251553	0.609581491929674\\
38.5743546698629	0.577514816638484\\
38.6849315367551	0.550813703620463\\
38.7955084036473	0.52497834407913\\
38.9060852705396	0.50012298136518\\
38.9982326596164	0.480227108473912\\
39.0903800486933	0.461120513250165\\
39.1825274377701	0.442836362504337\\
39.274674826847	0.425398101834958\\
39.3668222159238	0.408819954322837\\
39.4589696050007	0.393107572511184\\
39.5511169940775	0.378258804288691\\
39.6432643831544	0.364264534509118\\
39.7354117722312	0.351109567108523\\
39.8275591613081	0.338773516620407\\
39.9197065503849	0.327231682856265\\
40.0118539394618	0.316455887681158\\
40.122430806354	0.304492488256216\\
40.122430806354	0.838743140660213\\
40.2405462846732	0.809868514062472\\
40.3586617629924	0.780235540977515\\
40.5358349804713	0.734788616099252\\
40.9492391545886	0.627845147838457\\
41.0673546329078	0.598040116121425\\
41.185470111227	0.568943581901621\\
41.3035855895463	0.540733077641093\\
41.4217010678655	0.513563126505687\\
41.5398165461847	0.487562632365311\\
41.6579320245039	0.462833515917893\\
41.7760475028232	0.439450537910488\\
41.8941629811424	0.417462173693778\\
42.0122784594616	0.396892350404883\\
42.1303939377809	0.377742830439104\\
42.2485094161001	0.359996020509541\\
42.3666248944193	0.343618000029963\\
42.4847403727386	0.32856159011952\\
42.6028558510578	0.314769319453148\\
42.720971329377	0.302176180413213\\
42.8390868076962	0.290712104635304\\
42.9572022860155	0.280304118479449\\
43.0753177643347	0.270878164791171\\
43.1934332426539	0.262360597112746\\
43.3115487209731	0.25467936653105\\
43.4296641992924	0.247764930302935\\
43.5477796776116	0.241550916191159\\
43.6658951559308	0.235974578029115\\
43.8430683734097	0.228678109338716\\
44.0202415908885	0.222503500883363\\
44.1974148083674	0.21728973195772\\
44.3745880258462	0.212895447566012\\
44.6108189824847	0.208100978850609\\
44.8470499391231	0.204300460377894\\
45.0832808957616	0.201293286535346\\
45.3785695915597	0.198405978885404\\
45.7329160265173	0.195900731340103\\
46.0282047223154	0.194398261004068\\
46.0282047223154	0.634151316828422\\
46.1978207485548	0.59137103968439\\
46.3108980993811	0.563676142807694\\
46.4239754502075	0.536821208638941\\
46.5370528010337	0.510938306881741\\
46.65013015186	0.486137747195386\\
46.7632075026863	0.462507102053081\\
46.8762848535126	0.440111136730266\\
46.9893622043389	0.418992542235543\\
47.1024395551652	0.399173330620314\\
47.2155169059915	0.380656732885171\\
47.3285942568178	0.36342943627433\\
47.4416716076441	0.347464007224872\\
47.5547489584704	0.332721364952675\\
47.6678263092967	0.319153194841491\\
47.780903660123	0.306704217076955\\
47.8939810109493	0.295314251646019\\
48.0070583617756	0.284920044018037\\
48.1201357126019	0.275456835424308\\
48.2332130634282	0.266859677196138\\
48.3462904142545	0.25906450014223\\
48.4593677650808	0.252008957803852\\
48.5724451159071	0.245633067167603\\
48.7420611421465	0.237219403271851\\
48.911677168386	0.230027642170839\\
49.0812931946254	0.223895364385854\\
49.2509092208649	0.218677396822642\\
49.4205252471043	0.214245302115103\\
49.6466799487569	0.209365672066411\\
49.8728346504095	0.205456897266629\\
50.1555280274753	0.201653752101322\\
50.438221404541	0.198784194721213\\
50.7774534570199	0.196259258973768\\
51.1732241849119	0.19422142813761\\
51.6820722636303	0.192556142192842\\
51.6820722636303	0.628738035840811\\
51.8318435466722	0.591033769167822\\
51.9602189321366	0.559664061874045\\
52.0778963688124	0.531877702768412\\
52.1848758566994	0.507548524845461\\
52.2811573957978	0.486488508186028\\
52.3774389348962	0.466276253491841\\
52.4737204739945	0.446952964203945\\
52.5700020130929	0.428548135862712\\
52.6662835521912	0.411080120579541\\
52.7518671425009	0.39634612771728\\
52.7518671425009	0.92246480460517\\
52.8419061297332	0.903137186331534\\
52.9319451169656	0.8830898960627\\
53.0519970999421	0.855325146367392\\
53.1720490829185	0.826506598680737\\
53.292101065895	0.796800321509551\\
53.4421660446156	0.758710587232571\\
53.6522570148244	0.704348363694479\\
53.9223739765215	0.634482237635922\\
54.0724389552421	0.596556383326245\\
54.1924909382185	0.567031028095059\\
54.312542921195	0.538432360393756\\
54.4325949041715	0.510920680522645\\
54.5226338914038	0.491081221182782\\
54.6126728786362	0.471973869574754\\
54.7027118658686	0.453634799775557\\
54.7927508531009	0.436091138902469\\
54.8827898403333	0.419361315794092\\
54.9728288275656	0.403455563294372\\
55.062867814798	0.388376540873921\\
55.1529068020303	0.374120044260735\\
55.2429457892627	0.360675770325201\\
55.332984776495	0.348028108287266\\
55.4230237637274	0.336156931990189\\
55.5130627509598	0.325038372139559\\
55.6031017381921	0.31464555171371\\
55.6931407254245	0.304949271948885\\
55.7531667169127	0.298856849076159\\
55.7531667169127	0.831930804530543\\
55.8666232208283	0.804020261436861\\
56.0368079767016	0.760959402081454\\
56.2637209845327	0.7022549422081\\
56.5473622443216	0.628973035967761\\
56.717547000195	0.586207778234026\\
56.8310035041106	0.558565898184867\\
56.9444600080261	0.531796167745114\\
57.0579165119417	0.506027945041822\\
57.1713730158572	0.481368272331636\\
57.2848295197728	0.457901066043576\\
57.3982860236884	0.435687215324066\\
57.5117425276039	0.414765473775788\\
57.6251990315195	0.395153995217385\\
57.7386555354351	0.376852347985022\\
57.8521120393506	0.359843841757268\\
57.9655685432662	0.344098012904894\\
58.0790250471817	0.32957313508345\\
58.1924815510973	0.316218647351718\\
58.3059380550129	0.303977419156467\\
58.4193945589284	0.292787797468137\\
58.532851062844	0.282585404420018\\
58.6463075667596	0.273304673005057\\
58.7597640706751	0.264880123376656\\
58.8732205745907	0.257247393208473\\
58.9866770785062	0.250344042823116\\
59.1001335824218	0.244110159993127\\
59.2703183382952	0.235890882866968\\
59.4405030941685	0.228872156707226\\
59.6106878500419	0.222892978544834\\
59.7808726059152	0.217809777252086\\
59.9510573617885	0.213495792581099\\
60.1779703696197	0.208750616457451\\
60.4048833774508	0.204953437532311\\
60.6885246372397	0.201262892160273\\
60.9721658970286	0.198481545680494\\
61.3125354087753	0.196037215082185\\
61.4259919126909	0.195391666546683\\
61.4259919126909	0.6370281908941\\
61.5779075751655	0.598577245663549\\
61.6918443220215	0.570481975160732\\
61.8057810688775	0.543202937590181\\
61.9197178157335	0.516880413191785\\
62.0336545625895	0.491632645051254\\
62.1475913094455	0.467554590680479\\
62.2615280563015	0.444717640728783\\
62.3754648031575	0.423170206354001\\
62.4894015500135	0.402939034055834\\
62.6033382968695	0.384031082429686\\
62.7172750437255	0.366435788327294\\
62.8312117905814	0.350127557477208\\
62.9451485374374	0.335068332885314\\
63.0590852842934	0.321210119212864\\
63.1730220311494	0.308497369064952\\
63.2869587780054	0.296869164669971\\
63.4008955248614	0.286261153604897\\
63.5148322717174	0.276607218691197\\
63.6287690185734	0.267840879353429\\
63.7427057654294	0.259896434564212\\
63.8566425122854	0.252709866342443\\
63.9705792591414	0.246219528196605\\
64.122494921616	0.238547640957549\\
64.2744105840907	0.231879042279104\\
64.4263262465653	0.226094295012786\\
64.57824190904	0.221085093480184\\
64.7681364871333	0.215766891443039\\
64.9580310652266	0.211341825044173\\
65.1859045589386	0.207009764418601\\
65.2238834745573	0.206377534592363\\
65.2238834745573	0.666996249290051\\
65.4096946515706	0.619322659603142\\
65.5490530343307	0.584447326210054\\
65.665185019964	0.556215496997794\\
65.7813170055973	0.528909947395704\\
65.8974489912307	0.502667110310242\\
65.9903545797374	0.482513973489475\\
66.083260168244	0.46315853711593\\
66.1761657567507	0.444635942066142\\
66.2690713452574	0.426971239869076\\
66.3619769337641	0.410179893060629\\
66.4548825222707	0.39426844068673\\
66.5477881107774	0.379235287249571\\
66.6406936992841	0.365071574491665\\
66.7335992877908	0.351762098403\\
66.8265048762974	0.339286238173599\\
66.9194104648041	0.327618868970788\\
67.0123160533108	0.316731235923243\\
67.1052216418175	0.306591772154775\\
67.2213536274508	0.294918183131315\\
67.3374856130841	0.284292398141417\\
67.4536175987175	0.274644235093447\\
67.5465231872242	0.267582314826583\\
67.5465231872242	0.788911546447721\\
67.7045710590869	0.748589142536886\\
67.977562837759	0.677773250074637\\
68.1787146746753	0.62598615994348\\
68.3223945581869	0.589865199034037\\
68.4517064533474	0.558307770020718\\
68.5666503601567	0.531202530701535\\
68.6672262786148	0.508326870131583\\
68.767802197073	0.486315765401343\\
68.8683781155311	0.465230064030365\\
68.9689540339893	0.445116320331522\\
68.9833220223404	0.442324344270901\\
68.9833220223404	0.951313710346838\\
69.0801664139852	0.931791449525321\\
69.17701080563	0.911373347392285\\
69.2738551972747	0.890102553056352\\
69.3706995889195	0.86803452301092\\
69.4675439805643	0.845236979335326\\
69.5966698360906	0.81384463191047\\
69.725795691617	0.781516932836354\\
69.8872030110249	0.740172909235824\\
70.3714249692488	0.615154944007003\\
70.5005508247751	0.58291158533352\\
70.6296766803015	0.551627324216881\\
70.7265210719462	0.52892442845345\\
70.823365463591	0.506960951262585\\
70.9202098552358	0.485802964406602\\
71.0170542468805	0.465504248019286\\
71.1138986385253	0.446106295002977\\
71.2107430301701	0.427638632561013\\
71.3075874218148	0.41011941345154\\
71.4044318134596	0.393556223383072\\
71.5012762051044	0.37794704886764\\
71.5981205967491	0.363281351245291\\
71.6949649883939	0.349541196747836\\
71.7918093800387	0.336702398563716\\
71.8886537716835	0.324735634102765\\
71.9854981633282	0.313607508336233\\
72.082342554973	0.303281541632003\\
72.1791869466177	0.293719067494052\\
72.2114684104993	0.29069434422594\\
72.2114684104993	0.821595665051873\\
72.3380175236165	0.790123367622925\\
72.4882945954431	0.751828185129725\\
72.7334835021075	0.688260744467712\\
72.9628537696323	0.629084994980943\\
73.0024003674814	0.619031314589947\\
73.0024003674814	1.02230301212974\\
73.101625829935	1.00631416352179\\
73.2008512923885	0.989323793564324\\
73.3000767548421	0.971329942663985\\
73.3993022172956	0.952341265856433\\
73.4985276797492	0.932378118194919\\
73.5977531422027	0.911473450810618\\
73.6969786046563	0.889673451731881\\
73.8072291184936	0.864474278153565\\
73.9174796323308	0.838345331858775\\
74.0387551975519	0.808674831806016\\
74.1049055058542	0.792144434882189\\
74.1049055058542	1.06113643528107\\
74.1999448376261	1.04839381266132\\
74.2949841693979	1.03477915358832\\
74.3900235011698	1.02027038600033\\
74.4850628329416	1.00485138081666\\
74.5801021647135	0.988512992340475\\
74.6751414964854	0.97125408370627\\
74.7701808282572	0.953082498119102\\
74.8652201600291	0.934015931515731\\
74.9602594918009	0.914082658858689\\
75.0552988235728	0.893322065232709\\
75.0552988235728	1.07686411846176\\
75.1592938867504	1.06410745895671\\
75.2502895670309	1.05212381942724\\
75.3412852473113	1.03934739297749\\
75.4322809275918	1.0257573770439\\
75.5232766078722	1.01133767805032\\
75.6142722881527	0.996077746615157\\
75.7052679684331	0.97997341137949\\
75.7962636487136	0.963027684203098\\
75.887259328994	0.945251505492635\\
75.9782550092745	0.926664395391342\\
76.0822500724521	0.904466153113958\\
76.1862451356298	0.881304300823516\\
76.2902401988074	0.857253091388927\\
76.3552371132935	0.841808972441271\\
76.3552371132935	1.06932902404094\\
76.4533767731214	1.05675405218985\\
76.5487124426686	1.0436656308563\\
76.6356361413734	1.03096046649883\\
76.6356361413734	1.09330337721526\\
76.7387786633999	1.08199278252648\\
76.8361910453139	1.07046017545936\\
76.9336034272279	1.0580647781718\\
77.0310158091419	1.04477419130123\\
77.1284281910559	1.03056062893502\\
77.2086501526321	1.0181465222345\\
77.2086501526321	1.09196054045483\\
77.2999781102377	1.08189316033497\\
77.3913060678432	1.07109869628924\\
77.4826340254488	1.05954744526358\\
77.5739619830543	1.04721241320705\\
77.6652899406598	1.03407007203006\\
77.7566178982654	1.02010116580453\\
77.8479458558709	1.00529155057316\\
77.9392738134765	0.989633047357771\\
78.030601771082	0.973124283161596\\
78.1219297286875	0.955771490283084\\
78.2132576862931	0.937589230497892\\
78.3045856438986	0.918601008069587\\
78.3959136015042	0.898839734574295\\
78.5100735485111	0.873116867469975\\
78.624233495518	0.846357972562672\\
78.738393442525	0.81869073974751\\
78.8753853789333	0.784502405585172\\
79.035209304743	0.743627848546552\\
79.4918490927707	0.625544481834282\\
79.4918490927707	1.02415319262757\\
79.5846009662117	1.0093495890321\\
79.6773528396527	0.993672048979647\\
79.7701047130937	0.977117196643064\\
79.8628565865347	0.959689537746456\\
79.9556084599757	0.941402265145811\\
79.9556084599757	1.08315303237245\\
79.99303842984	1.0788550766963\\
79.99303842984	1.09804005896989\\
80.094982677736	1.08725839398907\\
80.1969269256321	1.07559127614964\\
80.2988711735281	1.06299600245407\\
80.3944439059306	1.05031027908468\\
80.4900166383331	1.03674641156184\\
80.5855893707356	1.0222811751063\\
80.6301899791901	1.01521714593505\\
80.6301899791901	1.09164879608225\\
80.7271092099367	1.08091751210337\\
80.7271092099367	1.09823460276266\\
80.8312824988552	1.08722404905704\\
80.9354557877738	1.07528876652407\\
81.0309479692825	1.06349680390134\\
81.1264401507911	1.05085747372551\\
81.2219323322998	1.03734255980609\\
81.3174245138085	1.02292866954583\\
81.4129166953172	1.00759827408726\\
81.5084088768259	0.991340772629286\\
81.5952199509247	0.975754342070388\\
81.5952199509247	1.08726670714414\\
81.6985004412658	1.07544127009156\\
81.7970863638642	1.06326478599054\\
81.8956722864626	1.05018454927709\\
81.9895636413182	1.0368586540195\\
82.0646767252026	1.02557256763879\\
82.0646767252026	1.09274284095444\\
82.1703074711588	1.08110032437261\\
82.2688961673846	1.06935461561893\\
82.3674848636104	1.05672193458665\\
82.4660735598362	1.04316911726836\\
82.564662256062	1.0286679598869\\
82.6562089025574	1.0143340661832\\
82.7477555490528	0.999151413969514\\
82.768881698244	0.995526458200047\\
82.768881698244	1.08950569912639\\
82.8684410192076	1.07829996545212\\
82.9680003401712	1.06621788897324\\
83.0675596611349	1.05322225363473\\
83.1671189820985	1.03928012244839\\
83.2595669229932	1.0254622587116\\
83.352014863888	1.01078774166325\\
83.4444628047828	0.995245694240012\\
83.480019705127	0.989035885563808\\
83.480019705127	1.08878057752445\\
83.582334984139	1.07719317906383\\
83.6826039575707	1.06493608907381\\
83.684650263151	1.06467637937253\\
83.684650263151	1.09668221993914\\
83.7880722006417	1.08562320622472\\
83.8867931409739	1.07421128029446\\
83.985514081306	1.06192460786312\\
84.0842350216381	1.04872820520477\\
84.1547499790182	1.03872813807064\\
84.1547499790182	1.09410126098604\\
84.187095720882	1.09067176649198\\
84.187095720882	1.09914472586578\\
84.290325662969	1.08831494856004\\
84.3935556050559	1.07658154404439\\
84.4929622159545	1.06438698254958\\
84.5694288397226	1.05438511760312\\
84.5694288397226	1.09567379303489\\
84.6718437352262	1.0846427831588\\
84.7742586307299	1.07270789573813\\
84.8766735262335	1.05982661445179\\
84.9790884217371	1.04596054541247\\
85.0815033172408	1.03107675015528\\
85.1839182127444	1.01514917659117\\
85.2863331082481	0.99816015262833\\
85.3887480037517	0.980101895238434\\
85.4911628992554	0.9609779759258\\
85.593577794759	0.940804672941013\\
85.6959926902626	0.919612132477695\\
85.7984075857663	0.897445256924129\\
85.9008224812699	0.874364239381833\\
86.0032373767736	0.850444671228075\\
86.1261352513779	0.820762892225247\\
86.2490331259823	0.790187982210256\\
86.4128969587881	0.748395815633415\\
86.6177267497954	0.695286315951464\\
86.6177267497954	1.04179179501114\\
86.7157913752592	1.0272766431782\\
86.8138560007229	1.01179971927594\\
86.9119206261866	0.99534732058585\\
87.0099852516504	0.977914311771926\\
87.1080498771141	0.959505293328462\\
87.2061145025779	0.940135673643596\\
87.3041791280416	0.919832586595305\\
87.4022437535053	0.898635594016\\
87.5003083789691	0.876597113462353\\
87.6092690739288	0.851202925089737\\
87.7073336993925	0.827618052751234\\
87.7073336993925	1.06708844782405\\
87.8043053999526	1.0545054572664\\
87.8689532003259	1.04562119271415\\
87.8689532003259	1.09479937785646\\
87.9705843042699	1.08378406165308\\
88.0722154082138	1.07187540940799\\
88.1738465121577	1.05903211595722\\
88.2670083574396	1.04640615776933\\
88.3601702027216	1.03293875161856\\
88.4533320480035	1.01860982944065\\
88.5464938932854	1.00340493506046\\
88.6396557385674	0.987316166133141\\
88.7158790665253	0.973494645650291\\
88.7158790665253	1.08700502823359\\
88.8453017469921	1.07200983476893\\
88.9747244274589	1.05549998142726\\
89.1041471079257	1.03740004770003\\
89.2335697883925	1.01764969232561\\
89.3629924688593	0.996208356314028\\
89.4924151493261	0.973060107623809\\
89.6218378297929	0.948218341338659\\
89.7512605102597	0.921729980088244\\
89.8806831907265	0.893678770982845\\
90.0101058711932	0.864187261864529\\
90.13952855166	0.8334170741755\\
90.2689512321268	0.801567180243907\\
90.3983739125936	0.768870038871412\\
90.5925079332938	0.718810088548324\\
90.9160646344608	0.635048639416212\\
91.0454873149276	0.602267869886703\\
91.1749099953944	0.570304841979905\\
91.3043326758612	0.539395626439472\\
91.433755356328	0.509743407467496\\
91.5631780367948	0.481514363423372\\
91.6926007172616	0.454835694590912\\
91.8220233977284	0.429795672482214\\
91.9514460781952	0.406445433000599\\
92.0808687586619	0.384802138480353\\
92.2102914391288	0.364853092772719\\
92.3397141195955	0.34656040194578\\
92.4691368000623	0.329865818244571\\
92.5985594805291	0.314695472344184\\
92.7279821609959	0.300964275283761\\
92.8574048414627	0.288579846232579\\
92.9868275219295	0.277445888298487\\
93.1162502023963	0.267464988142095\\
93.2456728828631	0.258540855082799\\
93.3750955633299	0.250580042423181\\
93.5045182437967	0.243493209719276\\
93.6339409242635	0.237195991991641\\
93.7633636047303	0.231609542735683\\
93.8927862851971	0.226660814131094\\
94.0869203058973	0.220288092082669\\
94.2810543265975	0.214997977553651\\
94.4751883472976	0.21061561577622\\
94.6693223679978	0.206991448676618\\
94.9281677289314	0.203122157209506\\
95.187013089865	0.200130229467035\\
95.187013089865	0.65035789799002\\
95.3534288039289	0.607951974173915\\
95.48656137518	0.574921020713703\\
95.6196939464312	0.542970485474115\\
95.7195433748695	0.519854166366045\\
95.8193928033078	0.497554068042007\\
95.9192422317462	0.476136912343236\\
96.0190916601845	0.455655490457133\\
96.1189410886229	0.436148841789461\\
96.2187905170612	0.417642788066686\\
96.3186399454995	0.400150759670822\\
96.4184893739379	0.383674845995642\\
96.5183388023762	0.368207001398048\\
96.6181882308146	0.35373034219171\\
96.7180376592529	0.340220477013517\\
96.8178870876912	0.327646821680318\\
96.9177365161296	0.315973859339394\\
97.0175859445679	0.305162316455778\\
97.1174353730063	0.295170234339579\\
97.2172848014446	0.285953924062028\\
97.317134229883	0.277468799499118\\
97.4502668011341	0.267215365605495\\
97.5833993723852	0.258077501218352\\
97.7165319436363	0.249953659679406\\
97.8496645148874	0.242746952269783\\
97.9827970861385	0.236366121712805\\
98.1492128002024	0.229422550045626\\
98.3156285142664	0.223485281903891\\
98.4820442283303	0.218418538393323\\
98.515327371143	0.217498801522368\\
98.515327371143	0.694250086758814\\
98.7444694259916	0.635028002900754\\
98.8972307958907	0.596416196985047\\
99.0499921657897	0.559004923109796\\
99.2027535356888	0.523168127165562\\
99.2791342206384	0.50593895272533\\
99.3555149055879	0.489212826933539\\
99.4318955905374	0.473016487255933\\
99.5082762754869	0.457371899760005\\
99.5846569604365	0.442296333563107\\
99.661037645386	0.427802504886387\\
99.7374183303355	0.413898780916313\\
99.8137990152851	0.400589433018609\\
99.8901797002346	0.387874928660523\\
99.9665603851841	0.375752251616348\\
100.042941070134	0.364215240588436\\
};\addlegendentry{Gamma};

==> fig7b_part1b_220211_0.tex <==

\addplot [color=blue, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-0.0105293600245062	0.281303191839456\\
0.581537315664846	0.277211735636271\\
1.17360399135418	0.274085768090458\\
1.76567066704354	0.271697456298227\\
2.65377068057755	0.26912882981344\\
3.54187069411158	0.267413448031306\\
4.72600404549027	0.265977887355419\\
6.20617073471364	0.26499194196677\\
8.57443743747102	0.264314795503054\\
13.0149375051411	0.264011296328775\\
21.8959376404813	0.263965627297978\\
21.8959376404813	0.518571683864167\\
22.0144172051296	0.505220941665868\\
22.1328967697779	0.492570268214592\\
22.2513763344262	0.480582954221589\\
22.3698558990745	0.469224215311726\\
22.5179553548849	0.455859678157054\\
22.6660548106953	0.443365312337562\\
22.8141542665057	0.431684460586084\\
22.9622537223161	0.420764154616847\\
23.1103531781264	0.410554874934277\\
23.2584526339368	0.401010326280542\\
23.4361719809093	0.390373573772621\\
23.6138913278817	0.380562390057761\\
23.7916106748542	0.371512698827743\\
23.9693300218267	0.363165397040433\\
24.1766692599612	0.354242129057809\\
24.3840084980957	0.346121524763859\\
24.5913477362303	0.33873138314452\\
24.8283068655269	0.33109593807616\\
24.857926756689	0.330198050524388\\
24.857926756689	0.584804107090577\\
24.9556507114568	0.570862508842126\\
25.0533746662247	0.557526722168774\\
25.1510986209926	0.544770422422673\\
25.2488225757605	0.53256842885466\\
25.3465465305283	0.520896654907915\\
25.4931324626802	0.504333030930979\\
25.639718394832	0.488837214006878\\
25.7863043269838	0.474340365824389\\
25.9328902591356	0.460778085871311\\
26.0794761912874	0.448090125342915\\
26.2260621234392	0.436220119493839\\
26.372648055591	0.425115337244378\\
26.5192339877429	0.414726446929123\\
26.6658199198947	0.405007297146796\\
26.8124058520465	0.395914711738257\\
26.9589917841983	0.387408297981608\\
27.154439693734	0.376913275651106\\
27.3498876032698	0.367310527938542\\
27.5453355128055	0.358524194691483\\
27.7407834223413	0.350484865299592\\
27.936231331877	0.343129030362093\\
28.1316792414128	0.336398579973732\\
28.3759891283325	0.328784399687876\\
28.6202990152522	0.321970615944636\\
28.8646089021719	0.315873091699515\\
29.1577807664755	0.309396080001022\\
29.4509526307791	0.303727256837675\\
29.7441244950827	0.298765778064265\\
29.7441244950827	0.553371834630454\\
29.8786570130238	0.536202294156695\\
30.0131895309649	0.520051364469737\\
30.147722048906	0.50485861483547\\
30.2822545668471	0.490567199670934\\
30.4167870847882	0.477123645849431\\
30.5513196027293	0.464477652624055\\
30.6858521206704	0.452581903421162\\
30.8203846386115	0.44139188879943\\
30.9549171565526	0.430865739912221\\
31.0894496744937	0.420964071850022\\
31.2239821924348	0.411649836276823\\
31.3585147103759	0.402888182809122\\
31.493047228317	0.394646328618876\\
31.6948460052287	0.383191216268287\\
31.8966447821403	0.372740221388781\\
32.0984435590519	0.363205326345508\\
32.3002423359636	0.354506228840023\\
32.5020411128752	0.346569665609238\\
32.7038398897869	0.339328795406715\\
32.9056386666985	0.332722636069832\\
33.1747037025807	0.324806300348413\\
33.4437687384629	0.31780140078105\\
33.7128337743451	0.311603000450972\\
33.9818988102273	0.306118244205337\\
34.3182301050801	0.300141605379437\\
34.6545613999328	0.295012352058862\\
34.9908926947855	0.290610339423836\\
35.3944902486088	0.28614375621774\\
35.7980878024321	0.282425905116099\\
36.268951615226	0.278868487158149\\
36.4707503921376	0.277562079579297\\
36.4707503921376	0.532168136145501\\
36.6036522819746	0.516443630949453\\
36.7365541718116	0.501641038484635\\
36.8694560616486	0.487706307887535\\
37.0023579514856	0.474588557245198\\
37.1352598413226	0.462239887802639\\
37.2681617311596	0.450615209063187\\
37.4010636209966	0.439672074142919\\
37.5339655108336	0.42937052477825\\
37.6668674006706	0.419672945420402\\
37.8440699204532	0.407621447118714\\
38.0212724402359	0.396502710667662\\
38.1984749600186	0.386244542166679\\
38.3756774798012	0.376780335378626\\
38.5528799995839	0.368048639255846\\
38.7300825193665	0.359992758938759\\
38.9072850391492	0.352560387636473\\
39.1287881888775	0.344073574342616\\
39.3502913386059	0.336399736136201\\
39.5717944883342	0.329460995907198\\
39.7932976380625	0.323186936607215\\
40.0591014177365	0.316446230818627\\
40.3249051974105	0.310472757057312\\
40.5907089770845	0.30517918841683\\
40.9008133867041	0.299759939351347\\
40.9008133867041	0.554365995917536\\
41.0214808444336	0.538864758819088\\
41.142148302163	0.524190957560378\\
41.2628157598925	0.51030042469435\\
41.3834832176219	0.497151350374736\\
41.5041506753514	0.484704156510347\\
41.6248181330808	0.472921377636993\\
41.7696190823561	0.459609269634754\\
41.9144200316315	0.447145243216923\\
42.0592209809068	0.435475269196388\\
42.2040219301821	0.424548760452382\\
42.3488228794575	0.414318352644926\\
42.5177573202787	0.403203666473175\\
42.6866917610999	0.392910618715078\\
42.8556262019211	0.383378470842104\\
43.0245606427423	0.374550974340835\\
43.2176285751095	0.365258602505222\\
43.314162541293	0.360909460674989\\
43.314162541293	0.615515517241178\\
43.4246238633183	0.59829783397025\\
43.5350851853435	0.581923410600709\\
43.6455465073687	0.566350947310156\\
43.756007829394	0.551541166992223\\
43.8664691514193	0.537456716191272\\
43.9769304734445	0.524062070888917\\
44.1058020158073	0.509261843305367\\
44.2346735581701	0.495303788120239\\
44.3635451005329	0.482139983479343\\
44.4924166428956	0.469725234409694\\
44.6212881852585	0.458016917652714\\
44.7685699479588	0.445449543413645\\
44.9158517106591	0.433696068568722\\
45.0631334733594	0.422703782646309\\
45.1551845750471	0.416198105435427\\
45.1551845750471	0.67080416200163\\
45.2499517783219	0.653649003215165\\
45.3447189815966	0.637217224478817\\
45.4394861848713	0.621478323090585\\
45.5447830773987	0.604767795364012\\
45.6500799699262	0.588838333875117\\
45.7553768624537	0.573653430832053\\
45.8606737549811	0.559178284852536\\
45.9765003367613	0.544035846302506\\
46.0923269185415	0.529670111604005\\
46.2081535003217	0.51604124114526\\
46.2081535003217	0.770647297711463\\
46.2893609908326	0.752282956599785\\
46.3705684813435	0.734584217774881\\
46.4653105536063	0.714744801067866\\
46.560052625869	0.695741734171961\\
46.6547946981317	0.6775397599515\\
46.7495367703944	0.660105107569464\\
46.8442788426571	0.643405429831191\\
46.9390209149199	0.627409743169267\\
47.0337629871826	0.612088370158602\\
47.1420396411971	0.595367509781624\\
47.2503162952116	0.579449775654524\\
47.3585929492262	0.564296592503155\\
47.4668696032407	0.549871237877582\\
47.5616116755034	0.537818575596276\\
47.5616116755034	0.792424632162479\\
47.6438777559787	0.773025947026781\\
47.7312854664836	0.753194477327739\\
47.8186931769885	0.734135581214716\\
47.9061008874935	0.715819161576675\\
47.9986502280281	0.69720245270085\\
48.0757746784737	0.682275805112198\\
48.0757746784737	0.936881861678401\\
48.1460000714367	0.91573835719754\\
48.2162254643998	0.895259195786366\\
48.2864508573629	0.87542350334077\\
48.356676250326	0.856211061634923\\
48.4269016432891	0.837602287713253\\
48.5205355005732	0.813696930543614\\
48.6141693578573	0.790787788092615\\
48.7078032151414	0.768833344822184\\
48.8014370724255	0.747793815283018\\
48.8950709297096	0.727631072016123\\
48.9887047869938	0.70830857645889\\
49.0823386442779	0.689791312730577\\
49.175972501562	0.672045724177181\\
49.2696063588461	0.655039652560589\\
49.3632402161302	0.638742279782107\\
49.4568740734143	0.623124072034372\\
49.5505079306984	0.608156726280725\\
49.6441417879825	0.593813118964988\\
49.7611841095877	0.576721246731125\\
49.8782264311928	0.560515030375726\\
49.995268752798	0.545148577539877\\
50.1123110744031	0.53057837388603\\
50.2293533960082	0.516763159875211\\
50.3463957176134	0.503663813929251\\
50.4166211105765	0.49613231061646\\
50.4166211105765	0.750738367182649\\
50.5036737618372	0.731850669968196\\
50.5925029978175	0.713332772753674\\
50.5942795825371	0.712969988955848\\
50.5942795825371	0.967576045522051\\
50.673535919161	0.942675918267071\\
50.7527922557849	0.91865698264661\\
50.8320485924089	0.895488054133452\\
50.9113049290328	0.873139051790858\\
50.9905612656567	0.851580959217614\\
51.0698176022807	0.830785786875182\\
51.1490739389046	0.810726535747889\\
51.2283302755285	0.791377162289379\\
51.3075866121524	0.772712544609448\\
51.3868429487764	0.754708449857489\\
51.4660992854003	0.737341502760245\\
51.5453556220242	0.72058915527299\\
51.6246119586482	0.704429657304672\\
51.7038682952721	0.688842028479101\\
51.783124631896	0.673806030895534\\
51.8623809685199	0.659302142853065\\
51.9416373051439	0.645311533505151\\
52.0208936417678	0.63181603841079\\
52.1001499783917	0.618798135951167\\
52.1794063150157	0.60624092458076\\
52.2586626516396	0.594128100883523\\
52.3379189882635	0.582443938405689\\
52.4171753248875	0.571173267237626\\
52.4964316615114	0.56030145431825\\
52.6549443347593	0.539698441905003\\
52.8134570080071	0.520527868322375\\
52.971969681255	0.502690142260022\\
53.1304823545028	0.486092596563012\\
53.2889950277507	0.470649006825084\\
53.4475077009986	0.456279143452079\\
53.6060203742464	0.442908354868393\\
53.7645330474943	0.430467179701395\\
53.9230457207421	0.418890985928869\\
54.08155839399	0.408119635115142\\
54.2400710672378	0.398097169991246\\
54.3985837404857	0.388771523756461\\
54.5570964137336	0.380094249590741\\
54.7156090869814	0.372020268973046\\
54.8741217602293	0.364507637498022\\
55.0326344334772	0.357517326974374\\
55.2704034433489	0.347932469765354\\
55.5081724532207	0.339329622317067\\
55.7459414630925	0.331608173514567\\
55.9837104729643	0.324677820283526\\
56.2214794828361	0.318457511487125\\
56.4592484927079	0.312874500025416\\
56.7762738392036	0.306309959669349\\
57.0932991856993	0.300626495996752\\
57.4103245321951	0.295705853032331\\
57.7273498786908	0.291445646830951\\
58.1236315618104	0.286915243947789\\
58.5199132449301	0.283131708716368\\
58.5199132449301	0.537737765282571\\
58.6334550018987	0.523964999942777\\
58.7551068843652	0.509976407309281\\
58.8767587668316	0.496740432286103\\
59.0065207747958	0.483406028547833\\
59.1362827827599	0.470835477652244\\
59.2660447907241	0.458985022774769\\
59.3309257947062	0.453316846712269\\
59.3309257947062	0.707922903278472\\
59.4203393266414	0.690238770799127\\
59.5097528585766	0.673259048362524\\
59.5991663905118	0.656955677283349\\
59.7034821777696	0.638754028553848\\
59.8077979650273	0.621395401994974\\
59.9121137522851	0.604840752441618\\
60.0164295395428	0.589052843132933\\
60.1207453268006	0.573996161954909\\
60.2250611140583	0.559636841562025\\
60.3442791566386	0.544038737131473\\
60.4634971992189	0.529263506809443\\
60.5827152417991	0.515267740077604\\
60.7019332843794	0.502010316528683\\
60.8211513269597	0.489452285052224\\
60.8211513269597	0.744058341618427\\
60.9094366277476	0.725171322820259\\
60.9977219285355	0.707027324815712\\
61.0860072293234	0.689597116951447\\
61.1831210601901	0.671214834782106\\
61.2802348910568	0.653626449809678\\
61.3773487219235	0.636797675064059\\
61.4744625527902	0.620695704366753\\
61.5804049137357	0.603921987414537\\
61.6863472746812	0.587936981455684\\
61.7040043348388	0.585346864061378\\
61.7040043348388	0.839952920627582\\
61.7756160867604	0.821503490447611\\
61.847227838682	0.803645012521571\\
61.9188395906037	0.786358558104084\\
61.9904513425253	0.769625804754924\\
62.0620630944469	0.753429016918489\\
62.1336748463685	0.737751027125427\\
62.241092474251	0.715170583826236\\
62.3485101021334	0.693666314543862\\
62.4559277300159	0.673186929297017\\
62.5633453578983	0.653683582562408\\
62.6707629857808	0.635109756772934\\
62.7781806136632	0.617421151368319\\
62.8855982415457	0.600575577133554\\
62.9930158694281	0.584532855573102\\
63.1004334973106	0.569254723080888\\
63.207851125193	0.554704739677518\\
63.3152687530754	0.540848202096996\\
63.4226863809579	0.527652061015772\\
63.5301040088403	0.515084842226543\\
63.6375216367228	0.50311657156891\\
63.780745140566	0.488041433584101\\
63.9239686444093	0.473916569939561\\
64.0671921482526	0.460682079271677\\
64.2104156520958	0.448281836151025\\
64.3536391559391	0.436663253063102\\
64.4968626597823	0.425777057392779\\
64.6400861636256	0.415577082466768\\
64.7833096674689	0.406020071767898\\
64.9623390472729	0.394916477814846\\
65.141368427077	0.384680784104077\\
65.2845919309203	0.377071348251462\\
65.2845919309203	0.631677404817651\\
65.3941409880584	0.613813230158968\\
65.5036900451965	0.596816930950183\\
65.6132391023346	0.580646344157699\\
65.7227881594727	0.565261355107978\\
65.8323372166108	0.550623797974268\\
65.9418862737489	0.536697361098049\\
66.051435330887	0.523447496909938\\
66.1609843880251	0.510841336226932\\
66.2705334451632	0.498847606713198\\
66.3800825023013	0.487436555302253\\
66.5261479118187	0.473079480900978\\
66.6722133213362	0.459644785220789\\
66.8182787308537	0.44707320949621\\
66.9643441403712	0.435309302076107\\
67.1104095498886	0.424301173833427\\
67.2564749594061	0.414000269288707\\
67.4025403689236	0.404361152437957\\
67.548605778441	0.395341306340057\\
67.7311875403379	0.384876983383677\\
67.9137693022347	0.375246158469324\\
68.0963510641315	0.366382442305579\\
68.2789328260284	0.358224733601503\\
68.4615145879252	0.350716797869893\\
68.6806127022014	0.342492397815079\\
68.8997108164776	0.335047700400096\\
68.936227168857	0.333877425404737\\
68.936227168857	0.588483481970925\\
69.0431861362423	0.573081511513962\\
69.1541065468642	0.557880744518215\\
69.265026957486	0.543427472930887\\
69.3323714925064	0.53500130091156\\
69.3323714925064	0.789607357477763\\
69.3734724142791	0.779877056512021\\
69.3734724142791	1.03448311307821\\
69.4429244815295	1.01053532904093\\
69.5123765487799	0.987331844465203\\
69.5818286160303	0.964849526451218\\
69.6512806832806	0.94306596107198\\
69.720732750531	0.921959431027474\\
69.8040752312315	0.897495700296062\\
69.887417711932	0.873941512134564\\
69.9707601926324	0.851263050454364\\
70.0541026733329	0.829427756422845\\
70.1374451540334	0.808404281719547\\
70.2207876347338	0.788162443530339\\
70.3041301154343	0.768673181214723\\
70.3874725961348	0.749908514584348\\
70.4708150768352	0.731841503732554\\
70.5541575575357	0.714446210357593\\
70.6513904516863	0.694967411761894\\
70.7486233458368	0.676330875670132\\
70.7625137592869	0.673735125914845\\
70.7625137592869	0.928341182481034\\
70.8387388681282	0.90571326907461\\
70.9149639769696	0.883856036992881\\
70.9911890858109	0.862743237695241\\
71.0716489229212	0.841237120176103\\
71.1521087600315	0.8205034304317\\
71.1859865861832	0.8119978088816\\
71.1859865861832	1.06660386544779\\
71.2554991336251	1.04163638318619\\
71.3123730360775	1.02178722106703\\
71.3123730360775	1.27639327763322\\
71.3753164647303	1.24783373636126\\
71.4010257524899	1.23640160909277\\
71.4010257524899	1.49100766565896\\
71.4501728495122	1.46389637293812\\
71.4993199465346	1.43738409938585\\
71.5484670435569	1.4114576097807\\
71.5976141405792	1.38610396133097\\
71.6713347861127	1.34911995565932\\
71.7450554316461	1.31335488675705\\
71.8187760771796	1.27876858031583\\
71.8924967227131	1.24532218611157\\
71.9662173682466	1.21297813436477\\
72.03993801378	1.18170009353886\\
72.1136586593135	1.1514529295297\\
72.187379304847	1.12220266619991\\
72.2610999503805	1.09391644721413\\
72.3348205959139	1.06656249913199\\
72.4085412414474	1.04011009571759\\
72.4822618869809	1.01452952342518\\
72.5559825325144	0.989792048022423\\
72.6297031780478	0.965869882313754\\
72.7034238235813	0.942736154927417\\
72.7771444691148	0.920364880131373\\
72.8508651146483	0.898730928643928\\
72.9245857601818	0.877809999406381\\
72.9983064057152	0.85757859228616\\
73.0720270512487	0.838013981679367\\
73.1457476967822	0.81909419098362\\
73.2194683423157	0.800797967912004\\
73.2931889878491	0.783104760620802\\
73.3914831818938	0.760417585914269\\
73.4897773759384	0.738721873900218\\
73.588071569983	0.717974296209988\\
73.6863657640277	0.698133417987862\\
73.7846599580723	0.679159615141955\\
73.8583806036058	0.665475423587822\\
73.8583806036058	0.92008148015401\\
73.928781255771	0.899415224084549\\
73.9991819079361	0.87939991038165\\
74.0695825601013	0.860015035768669\\
74.1399832122665	0.841240742777913\\
74.2103838644317	0.8230577994089\\
74.2807845165968	0.805447579427593\\
74.351185168762	0.788392043286038\\
74.4215858209272	0.77187371964304\\
74.4919864730924	0.75587568746684\\
74.5623871252575	0.740381558701586\\
74.6327877774227	0.725375461479729\\
74.7031884295879	0.71084202386325\\
74.7735890817531	0.696766358096895\\
74.8439897339182	0.683134045357519\\
74.9143903860834	0.669931120983705\\
74.9847910382486	0.65714406017068\\
75.0551916904138	0.644759764115761\\
75.1255923425789	0.632765546600226\\
75.2663936469093	0.609898587668454\\
75.4071949512396	0.588449461606032\\
75.54799625557	0.568330257726984\\
75.6887975599003	0.549458516120893\\
75.8295988642307	0.531756889685369\\
75.970400168561	0.515152827113752\\
76.1112014728914	0.499578275538724\\
76.2520027772217	0.484969401613014\\
76.3928040815521	0.471266329884159\\
76.5336053858825	0.458412897390943\\
76.6744066902128	0.446356423475692\\
76.8152079945432	0.435047493869078\\
76.9560092988735	0.424439758162421\\
77.0968106032038	0.414489739837364\\
77.2376119075342	0.405156658074546\\
77.3784132118646	0.396402260610543\\
77.5192145161949	0.388190666958479\\
77.7304164726904	0.376817985830471\\
77.941618429186	0.366486455684424\\
78.1528203856815	0.357100760793543\\
78.364022342177	0.348574311435158\\
78.5752242986725	0.340828445038895\\
78.7864262551681	0.333791700468325\\
78.9976282116636	0.327399158741116\\
79.2792308203243	0.319776717080757\\
79.560833428985	0.313070208433118\\
79.8424360376457	0.307169571833342\\
80.1240386463064	0.301977971536985\\
80.4760419071323	0.296356750056816\\
80.8280451679582	0.291566770367368\\
80.8984458201233	0.29069736822359\\
80.8984458201233	0.545303424789793\\
81.0380860287081	0.527998760022527\\
81.1777262372928	0.511758476054112\\
81.3173664458776	0.496517104613403\\
81.4570066544623	0.482213204272398\\
81.596646863047	0.468789112761925\\
81.7362870716318	0.456190714521895\\
81.8759272802165	0.444367222549232\\
82.0155674888013	0.433270973663923\\
82.155207697386	0.422857236367918\\
82.2948479059708	0.413084030522313\\
82.4344881145555	0.40391195811587\\
82.6206750593351	0.392554048103065\\
82.8068620041148	0.382117929772789\\
82.9930489488945	0.372528791834526\\
83.1792358936741	0.363717894574705\\
83.3654228384538	0.355622077096371\\
83.5516097832334	0.348183304550275\\
83.784343464208	0.339727988473626\\
84.0170771451826	0.332121563935857\\
84.2498108261571	0.325278804454825\\
84.4825445071317	0.319123040063445\\
84.7618249243012	0.312546338599702\\
85.0411053414707	0.306753799350204\\
85.3203857586402	0.301651924019254\\
85.5531194396147	0.297868236403048\\
85.5531194396147	0.552474292969251\\
85.666815481076	0.537940956414857\\
85.7829305872492	0.52385375745726\\
85.7950259108089	0.522428651804091\\
85.7950259108089	0.77703470837028\\
85.8942111227276	0.754414101146011\\
85.9933963346464	0.73279080806914\\
86.0925815465651	0.712120858812099\\
86.1917667584839	0.69236222164389\\
86.2909519704026	0.673474717959635\\
86.3901371823214	0.655419940578724\\
86.4893223942401	0.638161175644839\\
86.5885076061589	0.621663327969472\\
86.6876928180776	0.605892849666844\\
86.7868780299964	0.590817671935355\\
86.8860632419151	0.576407139846523\\
86.9852484538339	0.562631950009148\\
87.0844336657526	0.549464090981758\\
87.1836188776714	0.536876786312106\\
87.2828040895901	0.524844440088103\\
87.3819893015089	0.513342584889202\\
87.530767119387	0.497033593239323\\
87.6795449372652	0.481791189041317\\
87.8283227551433	0.467545618823209\\
87.9771005730214	0.454231690901921\\
88.1258783908995	0.441788477048135\\
88.2746562087777	0.430159033661738\\
88.4234340266558	0.419290141182145\\
88.5722118445339	0.409132060540799\\
88.7209896624121	0.399638305541416\\
88.8697674802902	0.390765430126194\\
89.0185452981683	0.382472829554629\\
89.2169157220058	0.372253447908037\\
89.4152861458433	0.36291532104083\\
89.6136565696808	0.35438245511962\\
89.8120269935183	0.34658540953815\\
90.0103974173558	0.339460731808416\\
90.2583604471527	0.331412554275573\\
90.5063234769496	0.324222345723143\\
90.7542865067465	0.317798643112653\\
90.7542865067465	0.572404699678856\\
90.8638776191211	0.557414494941668\\
90.9734687314957	0.543152815416121\\
91.0830598438704	0.52958425471563\\
91.192650956245	0.516675127206952\\
91.3205072540154	0.502405259950464\\
91.4483635517858	0.488941173444772\\
91.5762198495562	0.476237367433498\\
91.7040761473266	0.464250910936542\\
91.831932445097	0.452941297169914\\
91.9780539282632	0.440795883260051\\
92.1241754114294	0.429431048346757\\
92.2702968945955	0.418796625052082\\
92.4164183777617	0.408845670227564\\
92.5808050463237	0.398413222373662\\
92.5808050463237	0.653019278939851\\
92.6472804161133	0.641437888474002\\
92.6472804161133	0.896043945040191\\
92.7264051948105	0.873711736313879\\
92.8055299735077	0.85216855465174\\
92.8846547522049	0.831386522663109\\
92.9637795309021	0.811338747903065\\
93.0429043095993	0.7919992880731\\
93.1299415661662	0.771514144356829\\
93.2169788227331	0.751823723576564\\
93.3040160793	0.732897194386709\\
93.3910533358669	0.714704921546456\\
93.4385282030853	0.705081110992097\\
93.4385282030853	0.9596871675583\\
93.5123027567643	0.936740725178097\\
93.5860773104433	0.914551106565241\\
93.6639504504378	0.891922222578515\\
93.7418235904323	0.87008042308905\\
93.8196967304268	0.84899833149241\\
93.8483868346353	0.841417462535574\\
93.8483868346353	1.09602351910176\\
93.9129515643126	1.07195626655775\\
93.9775162939899	1.04858515797162\\
94.0420810236672	1.02589005741764\\
94.11955869928	0.999520776037059\\
94.1970363748928	0.974064102553626\\
94.2745140505056	0.94948845274773\\
94.3519917261184	0.92576333549016\\
94.4294694017312	0.902859314911609\\
94.506947077344	0.880747973881455\\
94.5844247529568	0.859401878750475\\
94.6619024285695	0.838794545313789\\
94.7393801041823	0.818900405951737\\
94.8168577797951	0.799694777908087\\
94.9072484013434	0.77812667002938\\
94.9976390228916	0.757426878845223\\
95.0880296444399	0.737560446542588\\
95.1396814281817	0.726569392759686\\
95.1396814281817	0.981175449325889\\
95.2134068487205	0.957535768081613\\
95.2871322692592	0.934675264524316\\
95.360857689798	0.912568256502794\\
95.4386789670333	0.890023101070327\\
95.5165002442686	0.868261604796473\\
95.5492670978414	0.859326705985794\\
95.5492670978414	1.113932762552\\
95.6177369175482	1.08788350263376\\
95.686206737255	1.06263258333283\\
95.7162666581019	1.05179268564886\\
95.7162666581019	1.30639874221507\\
95.784835833279	1.27440527110114\\
95.8534050084562	1.24339371563615\\
95.9219741836333	1.2133339397233\\
95.9905433588105	1.18419673217656\\
96.0591125339876	1.15595377833409\\
96.1276817091648	1.12857763254291\\
96.196250884342	1.10204169148798\\
96.2648200595191	1.07632016834\\
96.3333892346963	1.05138806769649\\
96.4019584098734	1.02722116129199\\
96.4705275850506	1.00379596445379\\
96.5390967602278	0.981089713280255\\
96.6076659354049	0.959080342519471\\
96.6762351105821	0.937746464127002\\
96.7448042857592	0.917067346481531\\
96.8133734609364	0.89702289423856\\
96.8819426361135	0.87759362880233\\
96.9505118112907	0.858760669397142\\
97.0190809864679	0.840505714719541\\
97.087650161645	0.822811025153655\\
97.1562193368222	0.805659405532452\\
97.2247885119993	0.789034188427877\\
97.2933576871765	0.772919217954055\\
97.3619268623537	0.757298834067399\\
97.4304960375308	0.74215785734873\\
97.499065212708	0.727481574252295\\
97.5676343878851	0.713255722807659\\
97.6362035630623	0.699466478760286\\
97.7047727382395	0.686100442137601\\
97.7733419134166	0.673144624227277\\
97.8419110885938	0.66058643495515\\
97.9790494389481	0.636614502187598\\
98.1161877893024	0.614091440384627\\
98.2533261396567	0.592929679341012\\
98.390464490011	0.573046941621584\\
98.5276028403653	0.554365922664559\\
98.6647411907197	0.536813990219585\\
98.801879541074	0.520322901951772\\
98.9390178914283	0.504828540113863\\
99.0761562417826	0.490270662254929\\
99.2132945921369	0.476592666996197\\
99.3504329424913	0.463741373963629\\
99.4875712928456	0.451666817021234\\
99.6247096431999	0.440322050001654\\
99.7618479935542	0.429662964178249\\
99.8989863439085	0.419648116769338\\
100.036124694263	0.41023856980766\\
};
\addplot [color=red, dashed, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-0.0105293600245062	0.192088660951427\\
0.877570653509508	0.190903717837188\\
2.06170400488821	0.190339011652412\\
4.72600404549027	0.190113972213254\\
21.8959376404813	0.190098048641119\\
21.8959376404813	0.621351240655457\\
22.0144172051296	0.591592914857571\\
22.1328967697779	0.562588423238765\\
22.2513763344262	0.534512104764048\\
22.3402360079125	0.514155400393363\\
22.4290956813987	0.494459673238822\\
22.5179553548849	0.475470022241538\\
22.6068150283711	0.457222800691341\\
22.6956747018574	0.439745735874126\\
22.7845343753436	0.42305822453072\\
22.8733940488298	0.407171776207804\\
22.9622537223161	0.39209057437894\\
23.0511133958023	0.377812124807861\\
23.1399730692885	0.364327961741367\\
23.2288327427748	0.351624384828355\\
23.317692416261	0.339683202811656\\
23.4065520897472	0.328482463698236\\
23.4954117632334	0.317997154979267\\
23.5842714367197	0.308199861300324\\
23.6731311102059	0.299061370583033\\
23.7619907836921	0.290551222842666\\
23.8508504571784	0.282638198752565\\
23.9693300218267	0.272961825413518\\
24.087809586475	0.264216377335387\\
24.2062891511233	0.256328679499674\\
24.3247687157716	0.249227908184523\\
24.4432482804199	0.242846318394413\\
24.5617278450682	0.237119750527825\\
24.7098273008786	0.230791261586319\\
24.857926756689	0.225283695022554\\
24.857926756689	0.711726758614361\\
25.1510986209926	0.635845909428014\\
25.2976845531444	0.598754733502645\\
25.3954085079123	0.574607136067627\\
25.4931324626802	0.551043700804996\\
25.590856417448	0.528155878763187\\
25.6885803722159	0.506023469271767\\
25.7863043269838	0.484713872234096\\
25.8840282817517	0.464281737170808\\
25.9817522365195	0.44476898459672\\
26.0794761912874	0.42620515976661\\
26.1772001460553	0.408608067804039\\
26.2749241008232	0.391984632879314\\
26.372648055591	0.37633192212509\\
26.4703720103589	0.361638276743946\\
26.5680959651268	0.347884497443715\\
26.6658199198947	0.335045038039155\\
26.7635438746625	0.3230891689186\\
26.8612678294304	0.311982080335028\\
26.9589917841983	0.301685903535301\\
27.0567157389662	0.292160635147312\\
27.154439693734	0.283364956717634\\
27.2521636485019	0.275256946687804\\
27.3498876032698	0.267794686382828\\
27.4476115580377	0.260936764808378\\
27.5453355128055	0.254642689317933\\
27.6430594675734	0.248873210650544\\
27.7896453997252	0.241120471743983\\
27.936231331877	0.234343276922104\\
28.0828172640289	0.228430662814645\\
28.2294031961807	0.223281292340516\\
28.3759891283325	0.218803425628238\\
28.5714370378682	0.213736283975891\\
28.766884947404	0.209546054484392\\
28.9623328569397	0.206086683856398\\
29.2066427438594	0.202603861618144\\
29.4509526307791	0.199872319199045\\
29.7441244950827	0.197364409502541\\
29.7441244950827	0.642655338532137\\
29.8786570130238	0.608436924992304\\
30.0131895309649	0.575049984645347\\
30.147722048906	0.542765246370706\\
30.2822545668471	0.51181601393246\\
30.3495208258177	0.496903517169883\\
30.4167870847882	0.482392828889814\\
30.4840533437588	0.468300654350728\\
30.5513196027293	0.454640840233495\\
30.6185858616999	0.441424428047455\\
30.6858521206704	0.42865973872135\\
30.753118379641	0.416352484256876\\
30.8203846386115	0.404505902118359\\
30.8876508975821	0.393120907973838\\
30.9549171565526	0.382196262476455\\
31.0221834155232	0.371728747958599\\
31.0894496744937	0.361713351183894\\
31.1567159334643	0.352143448642011\\
31.2239821924348	0.343010991257444\\
31.2912484514054	0.334306685795227\\
31.3585147103759	0.326020170668798\\
31.4257809693465	0.318140184271115\\
31.493047228317	0.31065472434976\\
31.6275797462581	0.296816556747302\\
31.7621122641992	0.284400236679858\\
31.8966447821403	0.273296882337434\\
32.0311773000814	0.263397322000074\\
32.1657098180225	0.254594564632129\\
32.3002423359636	0.246785645647307\\
32.4347748539047	0.239872929857384\\
32.5693073718458	0.233764959372081\\
32.7038398897869	0.228376932304201\\
32.838372407728	0.223630891366227\\
32.9729049256691	0.219455692033804\\
33.1747037025807	0.214123809631459\\
33.3765024794924	0.209741088972279\\
33.578301256404	0.206144969845937\\
33.7801000333157	0.203198581248202\\
34.0491650691979	0.200085672599641\\
34.3182301050801	0.197706853217255\\
34.6545613999328	0.195509313235362\\
35.0581589537561	0.193689959701032\\
35.5290227665499	0.19232323274386\\
36.2016853562554	0.19121985415228\\
36.4707503921376	0.190950882844461\\
36.4707503921376	0.623935630140025\\
36.6036522819746	0.590538800575047\\
36.7365541718116	0.558098282958838\\
36.8251554317029	0.537124009504012\\
36.9137566915943	0.516746084695029\\
37.0023579514856	0.497018885190712\\
37.0909592113769	0.4779882476127\\
37.1795604712683	0.459691362708384\\
37.2681617311596	0.442156868299506\\
37.3567629910509	0.425405118433673\\
37.4453642509422	0.40944860181969\\
37.5339655108336	0.394292480220187\\
37.6225667707249	0.379935216845041\\
37.7111680306162	0.366369265686231\\
37.7997692905076	0.35358179484038\\
37.8883705503989	0.341555419843459\\
37.9769718102902	0.330268926560848\\
38.0655730701816	0.319697966939273\\
38.1541743300729	0.309815714687787\\
38.2427755899642	0.300593471519122\\
38.3313768498556	0.292001217815169\\
38.4199781097469	0.284008104396989\\
38.5085793696382	0.276582884439406\\
38.5971806295295	0.269694286470227\\
38.7300825193665	0.260299933442653\\
38.8629844092035	0.251941419031837\\
38.9958862990405	0.244521066270224\\
39.1287881888775	0.237946582641484\\
39.2616900787145	0.232131737599545\\
39.3945919685515	0.226996720916631\\
39.5274938583885	0.222468252005015\\
39.7046963781712	0.217259208283593\\
39.8818988979538	0.2128690782029\\
40.0591014177365	0.209174899418002\\
40.2806045674648	0.205375459343159\\
40.5021077171932	0.202323490112121\\
40.7679114968671	0.199447352190035\\
40.9008133867041	0.198271822175272\\
40.9008133867041	0.645206087314023\\
41.0456143359795	0.608351941320578\\
41.1662817937089	0.578361431851889\\
41.2869492514384	0.549237500044043\\
41.3834832176219	0.526679341760527\\
41.4800171838055	0.504863028391341\\
41.576551149989	0.483852802438406\\
41.6730851161726	0.463700756787617\\
41.7696190823561	0.444446870764494\\
41.8661530485397	0.426119353280313\\
41.9626870147232	0.408735245966113\\
42.0592209809068	0.392301233558712\\
42.1557549470904	0.376814607078259\\
42.2522889132739	0.362264326958041\\
42.3488228794575	0.348632137521605\\
42.445356845641	0.335893690257578\\
42.5418908118246	0.324019640452192\\
42.6384247780081	0.312976689229998\\
42.7349587441917	0.302728550381914\\
42.8314927103752	0.293236828125742\\
42.9280266765588	0.284461797888852\\
43.0245606427423	0.276363087187747\\
43.1210946089259	0.26890025766879\\
43.2417620666553	0.260405038635042\\
43.314162541293	0.255722994695844\\
43.314162541293	0.769847052155669\\
43.4798545243309	0.727183193509859\\
43.8848793717568	0.622507536213305\\
44.0137509141196	0.590144582565699\\
44.1242122361448	0.563114294005572\\
44.2346735581701	0.536888418847099\\
44.3267246598578	0.515737293673055\\
44.4187757615455	0.495291205497679\\
44.5108268632332	0.475600879742217\\
44.6028779649209	0.456706972319793\\
44.6949290666086	0.438640206307255\\
44.7869801682963	0.42142172601659\\
44.879031269984	0.405063632733359\\
44.9710823716717	0.38956966353679\\
45.0631334733594	0.374935974210686\\
45.1551845750471	0.361151988903359\\
45.1551845750471	0.895419093955383\\
45.2499517783219	0.874018988535312\\
45.3447189815966	0.851901784478414\\
45.450015874124	0.82657344111918\\
45.5658424559042	0.797927501715279\\
45.7027284161899	0.763241204236948\\
45.8817331334866	0.717020946872978\\
46.2081535003217	0.632555478256378\\
46.2081535003217	1.02610220955921\\
46.2893609908326	1.01329216764147\\
46.3705684813435	0.999813683700424\\
46.4517759718544	0.985662890730808\\
46.5329834623653	0.970840359435186\\
46.6141909528762	0.955351532842641\\
46.6953984433871	0.939207119575414\\
46.7901405156499	0.919565465508626\\
46.8848825879126	0.899089938941628\\
46.9796246601753	0.877827759555501\\
47.074366732438	0.855837438319469\\
47.1826433864526	0.829903792170811\\
47.2909200404671	0.803230957960636\\
47.4262658579853	0.769060178215724\\
47.5616116755034	0.734245613775371\\
47.5616116755034	1.0501863709687\\
47.6490193860084	1.03780853887214\\
47.7364270965133	1.0246780181529\\
47.8238348070182	1.01078098002802\\
47.9112425175232	0.99610837079031\\
47.9986502280281	0.980656593367428\\
48.0757746784737	0.966377466098763\\
48.0757746784737	1.0861728425394\\
48.1694085357578	1.07541063373446\\
48.2630423930419	1.06386486939583\\
48.356676250326	1.05150526575449\\
48.4503101076101	1.03830505586146\\
48.5439439648942	1.0242418847066\\
48.6375778221783	1.00929875009963\\
48.7312116794625	0.993464966894336\\
48.8248455367466	0.976737126257134\\
48.9184793940307	0.959120016063679\\
49.0121132513148	0.940627463642002\\
49.1057471085989	0.921283058528857\\
49.199380965883	0.901120711254023\\
49.2930148231671	0.880185004970372\\
49.3866486804512	0.858531300451133\\
49.4802825377354	0.836225561840294\\
49.5973248593405	0.807543289827649\\
49.7143671809456	0.778130637171074\\
49.8782264311928	0.736087023063646\\
50.3463957176134	0.615217960478375\\
50.4166211105765	0.59757671074648\\
50.4166211105765	1.01592321450649\\
50.5018971771176	1.00189349702295\\
50.5871732436586	0.987122800261076\\
50.5942795825371	0.985858420898253\\
50.5942795825371	1.0884221124776\\
50.673535919161	1.07950329607033\\
50.7527922557849	1.07003163094527\\
50.8320485924089	1.05998794359483\\
50.9113049290328	1.04935463509896\\
50.9905612656567	1.03811605478586\\
51.0698176022807	1.02625889525441\\
51.1490739389046	1.01377260314959\\
51.2283302755285	1.00064979854817\\
51.3075866121524	0.986886694253911\\
51.3868429487764	0.972483504791114\\
51.4660992854003	0.9574448335174\\
51.5453556220242	0.941780025152468\\
51.6246119586482	0.92550347024978\\
51.7038682952721	0.908634847836694\\
51.783124631896	0.89119929271439\\
51.8623809685199	0.873227474829434\\
51.9416373051439	0.854755579754368\\
52.0208936417678	0.835825181659644\\
52.1794063150157	0.796780560246205\\
52.3379189882635	0.756521995332136\\
52.5756879981353	0.694935444851879\\
52.8134570080071	0.63349631956369\\
52.971969681255	0.593492862281849\\
53.0512260178789	0.573960789957198\\
53.1304823545028	0.554814877524308\\
53.2097386911268	0.536104336290961\\
53.2889950277507	0.517873395343543\\
53.3682513643746	0.500161002912307\\
53.4475077009986	0.483000642322978\\
53.5267640376225	0.466420258717676\\
53.6060203742464	0.450442289385805\\
53.6852767108703	0.435083787845812\\
53.7645330474943	0.420356629825719\\
53.8437893841182	0.40626778801645\\
53.9230457207421	0.392819661881276\\
54.0023020573661	0.380010448830262\\
54.08155839399	0.367834543613441\\
54.1608147306139	0.356282953744667\\
54.2400710672378	0.345343720025667\\
54.3193274038618	0.335002332689953\\
54.3985837404857	0.325242135230596\\
54.4778400771096	0.316044709530246\\
54.5570964137336	0.30739023741117\\
54.6363527503575	0.299257835113934\\
54.7156090869814	0.291625858463988\\
54.7948654236054	0.284472177574258\\
54.8741217602293	0.277774420850221\\
54.9533780968532	0.271510188814034\\
55.0326344334772	0.265657238854828\\
55.191147106725	0.25509791675006\\
55.3496597799729	0.245927000619645\\
55.5081724532207	0.237985125133804\\
55.6666851264686	0.231124928129574\\
55.8251977997164	0.225212001519452\\
55.9837104729643	0.220125121403029\\
56.1422231462122	0.215755964333127\\
56.30073581946	0.212008478035685\\
56.5385048293318	0.207370655590793\\
56.7762738392036	0.203701147574293\\
57.0140428490754	0.20080289020251\\
57.3310681955711	0.197868252427824\\
57.6480935420668	0.195733626712794\\
58.0443752251865	0.19386704569871\\
58.5199132449301	0.19242201327674\\
58.5199132449301	0.628339834269397\\
58.657785378392	0.593601500234115\\
58.7713271353607	0.565733798605606\\
58.8767587668316	0.540602200881168\\
58.9740802728047	0.518138237406276\\
59.0714017787779	0.49645499720495\\
59.1606131592532	0.477316836100201\\
59.2498245397286	0.458923752077325\\
59.3309257947062	0.442873798992352\\
59.3309257947062	0.951622244869128\\
59.4203393266414	0.933643801316691\\
59.5097528585766	0.914898700354527\\
59.5991663905118	0.89541963620286\\
59.6885799224471	0.875248232733284\\
59.7928957097048	0.850907848973534\\
59.8972114969625	0.825789617620018\\
60.0164295395428	0.796273023792295\\
60.1505498374456	0.762258651691113\\
60.3293769013161	0.716070476968738\\
60.6572265184118	0.631255997645042\\
60.7913468163146	0.597383629600046\\
60.8211513269597	0.589971541870867\\
60.8211513269597	1.01355032879862\\
60.9094366277476	0.998879610438152\\
60.9977219285355	0.983414237512804\\
61.0860072293234	0.967155624631459\\
61.1742925301113	0.95011208005991\\
61.2625778308992	0.93229938671702\\
61.3508631316871	0.913741281912664\\
61.4391484324751	0.894469806682125\\
61.5362622633418	0.872495875084084\\
61.6333760942084	0.849773819530981\\
61.7040043348388	0.832822839351081\\
61.7040043348388	1.06791908818722\\
61.8114219627212	1.05399464764656\\
61.9188395906037	1.03897052996382\\
61.9904513425253	1.02832608205763\\
62.0620630944469	1.01716927050828\\
62.1336748463685	1.00549410556152\\
62.2052865982902	0.99329691790966\\
62.2768983502118	0.98057660792341\\
62.3485101021334	0.967334885378193\\
62.4201218540551	0.953576493630692\\
62.5275394819375	0.931988533678236\\
62.63495710982	0.909298277815182\\
62.7423747377024	0.885565363635394\\
62.8497923655848	0.860868054449782\\
62.9572099934673	0.835303077197977\\
63.0646276213497	0.808984785019518\\
63.207851125193	0.772949395083558\\
63.3868805049971	0.726880719262837\\
63.780745140566	0.625047797592586\\
63.9239686444093	0.589064517806534\\
64.0313862722917	0.562797164338093\\
64.1388039001742	0.537292071236465\\
64.2462215280566	0.512662344269216\\
64.3536391559391	0.489003377808473\\
64.4610567838215	0.466392068434175\\
64.568474411704	0.444886700032427\\
64.6400861636256	0.431184749271537\\
64.7116979155472	0.41800014370817\\
64.7833096674689	0.405337283031017\\
64.8549214193905	0.393197557023001\\
64.9265331713121	0.381579571756248\\
64.9981449232338	0.370479390649436\\
65.0697566751554	0.359890784398118\\
65.1771743030378	0.344948494674668\\
65.2845919309203	0.331103038151653\\
65.2845919309203	0.86777713483373\\
65.3941409880584	0.841929904824354\\
65.5036900451965	0.815267081533591\\
65.6132391023346	0.78792299986587\\
65.759304511852	0.750665531103706\\
66.0149189785076	0.684378396049723\\
66.1975007404045	0.637222354821617\\
66.3435661499219	0.600228594211842\\
66.45311520706	0.573160327137728\\
66.5626642641981	0.546833226869737\\
66.6722133213362	0.521374158358796\\
66.7817623784743	0.496891351881601\\
66.8913114356124	0.473473250731317\\
66.9643441403712	0.458487228077786\\
67.0373768451299	0.444020463424366\\
67.1104095498886	0.430084440106512\\
67.1834422546473	0.416686983541837\\
67.2564749594061	0.403832458811578\\
67.3295076641648	0.391521999118908\\
67.4025403689236	0.379753757451297\\
67.4755730736823	0.368523174120426\\
67.548605778441	0.357823253386613\\
67.6216384831997	0.34764484304317\\
67.6946711879585	0.33797691159441\\
67.8042202450966	0.324404135233038\\
67.9137693022347	0.311903082689213\\
68.0233183593728	0.300420644643239\\
68.1328674165109	0.289900343901834\\
68.242416473649	0.28028377310676\\
68.3519655307871	0.271511819489007\\
68.4615145879252	0.263525681523731\\
68.5710636450633	0.256267689779349\\
68.6806127022014	0.249681949128558\\
68.7901617593395	0.24371482223097\\
68.936227168857	0.236633139443867\\
68.936227168857	0.73514541429607\\
69.3323714925064	0.632600406276396\\
69.3323714925064	1.02611455998348\\
69.3734724142791	1.01971458659814\\
69.3734724142791	1.0921266779492\\
69.4707053084296	1.08139665962229\\
69.5679382025802	1.06984086396469\\
69.6512806832806	1.05925156734615\\
69.7346231639811	1.04800899785285\\
69.8179656446816	1.03609520684259\\
69.901308125382	1.02349517190873\\
69.9846506060825	1.01019732710469\\
70.067993086783	0.996194102856251\\
70.1513355674835	0.981482462754457\\
70.2346780481839	0.966064422205321\\
70.3180205288844	0.949947531957363\\
70.4013630095849	0.933145308009003\\
70.4847054902853	0.915677588500202\\
70.5819383844359	0.894493097263208\\
70.6791712785864	0.872492597692641\\
70.7625137592869	0.853035293698952\\
70.7625137592869	1.07104871180299\\
70.8514430529351	1.0598073998521\\
70.9403723465833	1.04782344837368\\
71.0293016402316	1.03507500597381\\
71.1182309338798	1.02154402605345\\
71.1859865861832	1.01070093291597\\
71.1859865861832	1.09116463988745\\
71.279512559105	1.08078646568882\\
71.3123730360775	1.07695993340619\\
71.3123730360775	1.09786063846211\\
71.4010257524899	1.08852098214754\\
71.4010257524899	1.09894544817779\\
71.4993199465346	1.08863763192166\\
71.5976141405792	1.07751171432012\\
71.6959083346238	1.06552901783475\\
71.7942025286684	1.05265394418329\\
71.8924967227131	1.03885502095673\\
71.9907909167577	1.02410603415822\\
72.0890851108024	1.00838722411348\\
72.187379304847	0.991686513785922\\
72.2856734988916	0.97400072987503\\
72.3839676929363	0.955336768822846\\
72.4822618869809	0.935712652797449\\
72.5805560810255	0.915158415775792\\
72.6788502750702	0.893716757963361\\
72.7771444691148	0.871443408837237\\
72.8754386631594	0.848407145753598\\
72.9737328572041	0.824689426635487\\
73.0966005997599	0.794227249209555\\
73.2440418908268	0.756751541150294\\
73.4406302789161	0.705874393244159\\
73.7109393125388	0.635934646542253\\
73.8583806036058	0.598627722378055\\
73.8583806036058	1.01624639840763\\
73.928781255771	1.0047317067649\\
73.9991819079361	0.992712348591695\\
74.0695825601013	0.980187420004157\\
74.1399832122665	0.96715865150712\\
74.2103838644317	0.953630613221435\\
74.2807845165968	0.939610900058142\\
74.351185168762	0.925110290865589\\
74.4215858209272	0.910142875530084\\
74.4919864730924	0.894726144172196\\
74.5623871252575	0.878881032972004\\
74.7031884295879	0.846006579659701\\
74.8439897339182	0.811754511051433\\
74.9847910382486	0.776409192708655\\
75.1255923425789	0.74029640956087\\
75.54799625557	0.63098179068129\\
75.6887975599003	0.595450476325553\\
75.8295988642307	0.560948336405019\\
75.970400168561	0.527769036016068\\
76.0408008207262	0.511754256927972\\
76.1112014728914	0.496158224161022\\
76.1816021250566	0.481003296484403\\
76.2520027772217	0.466308381500156\\
76.3224034293869	0.452088962141275\\
76.3928040815521	0.438357168623043\\
76.4632047337173	0.425121890613255\\
76.5336053858825	0.41238892389535\\
76.6040060380476	0.400161145545582\\
76.6744066902128	0.38843871160806\\
76.744807342378	0.377219271404314\\
76.8152079945432	0.366498192923501\\
76.8856086467083	0.356268794170489\\
76.9560092988735	0.34652257586977\\
77.0264099510387	0.337249451498579\\
77.0968106032038	0.328437971225199\\
77.167211255369	0.320075536933402\\
77.2376119075342	0.312148606099072\\
77.3080125596994	0.304642882836376\\
77.3784132118646	0.297543494935425\\
77.4488138640297	0.290835156164178\\
77.5896151683601	0.27852927929257\\
77.7304164726904	0.267599902412812\\
77.8712177770208	0.257922939830436\\
78.0120190813511	0.249378240340775\\
78.1528203856815	0.24185149554603\\
78.2936216900118	0.23523550473432\\
78.4344229943422	0.229430916127043\\
78.5752242986725	0.224346556679336\\
78.7160256030029	0.219899450009009\\
78.8568269073332	0.216014607253612\\
79.0680288638288	0.211096191004643\\
79.2792308203243	0.207095223493766\\
79.4904327768198	0.20384610356588\\
79.7720353854805	0.200449107044378\\
80.0536379941412	0.197884975129298\\
80.4056412549671	0.195548931466249\\
80.8280451679582	0.19364781180758\\
80.8984458201233	0.193402687520475\\
80.8984458201233	0.631238513744279\\
81.0380860287081	0.595990294501632\\
81.1777262372928	0.561749625362978\\
81.2708197096826	0.53962598369435\\
81.3639131820725	0.518152745160506\\
81.4570066544623	0.497393908168263\\
81.5501001268521	0.477403086147802\\
81.643193599242	0.458223359642673\\
81.7362870716318	0.439887396152798\\
81.8293805440216	0.422417805843665\\
81.9224740164114	0.405827694884763\\
82.0155674888013	0.39012137482294\\
82.1086609611911	0.375295185773069\\
82.2017544335809	0.361338392889593\\
82.2948479059708	0.348234119042203\\
82.3879413783606	0.335960281302178\\
82.4810348507504	0.324490504226461\\
82.5741283231402	0.313794988542128\\
82.6672217955301	0.303841319313904\\
82.7603152679199	0.294595202746024\\
82.8534087403097	0.286021125246137\\
82.9465022126995	0.278082932166328\\
83.0395956850894	0.270744326702001\\
83.1326891574792	0.263969291798347\\
83.225782629869	0.257722439638997\\
83.3654228384538	0.249267393585626\\
83.5050630470385	0.241812063967416\\
83.6447032556233	0.235251950489726\\
83.784343464208	0.229490149955453\\
83.9239836727927	0.224437671855881\\
84.0636238813775	0.220013457031499\\
84.2498108261571	0.214966137924463\\
84.4359977709368	0.210752632301563\\
84.6221847157165	0.207240738104105\\
84.854918396691	0.203667037725012\\
85.0876520776656	0.200830364766389\\
85.3669324948351	0.198191536905085\\
85.5531194396147	0.196801074677353\\
85.5531194396147	0.641059962805912\\
85.6982633223312	0.604209279260786\\
85.7950259108089	0.580181097385207\\
85.7950259108089	1.01040402643976\\
85.8942111227276	0.993671544531963\\
85.9933963346464	0.975935935523452\\
86.0925815465651	0.957203079810554\\
86.1917667584839	0.93749028231565\\
86.2909519704026	0.916827220353596\\
86.3901371823214	0.8952566533018\\
86.4893223942401	0.87283483009125\\
86.5885076061589	0.849631537231062\\
86.6876928180776	0.825729742098247\\
86.7868780299964	0.801224803438743\\
86.9356558478745	0.763572171364075\\
87.134026271712	0.712325953029747\\
87.4315819074683	0.63531427999834\\
87.5803597253464	0.597688820926848\\
87.6795449372652	0.573208186867589\\
87.7787301491839	0.549335124814391\\
87.8779153611027	0.526164472440428\\
87.9771005730214	0.503778632160859\\
88.0762857849402	0.482246800927925\\
88.1754709968589	0.461624632009674\\
88.2746562087777	0.441954299842465\\
88.3738414206964	0.423264922049157\\
88.4730266326152	0.405573280931534\\
88.5722118445339	0.388884780277991\\
88.6713970564527	0.373194571770711\\
88.7705822683714	0.358488787858064\\
88.8697674802902	0.344745823700094\\
88.9689526922089	0.331937618657363\\
89.0681379041277	0.320030896795473\\
89.1673231160464	0.308988335174277\\
89.2665083279652	0.298769637620452\\
89.3656935398839	0.289332499776577\\
89.4648787518027	0.280633458192824\\
89.5640639637215	0.272628621948428\\
89.6632491756402	0.265274289751147\\
89.762434387559	0.258527458741426\\
89.8616195994777	0.252346233457615\\
89.9608048113965	0.246690144760123\\
90.1095826292746	0.239106258704297\\
90.2583604471527	0.232493953242795\\
90.4071382650309	0.226740122351302\\
90.555916082909	0.221741900661854\\
90.7046939007871	0.217406531995422\\
90.7542865067465	0.216094087153365\\
90.7542865067465	0.690962471722187\\
90.9734687314957	0.634340706437087\\
91.1195902146619	0.597401800648541\\
91.2291813270365	0.570393494333999\\
91.3387724394112	0.544140904485275\\
91.43009836639	0.522931875424348\\
91.5214242933689	0.502397389498896\\
91.6127502203477	0.482590389987266\\
91.7040761473266	0.463554072744344\\
91.7954020743055	0.445321936002799\\
91.8867280012843	0.427918048619162\\
91.9780539282632	0.411357504550324\\
92.069379855242	0.395647027758343\\
92.1607057822209	0.380785690537238\\
92.2520317091998	0.366765709116478\\
92.3433576361786	0.353573282905444\\
92.4346835631575	0.341189447444009\\
92.5260094901363	0.329590915570378\\
92.5808050463237	0.322997715891049\\
92.5808050463237	0.859440316175167\\
92.6472804161133	0.843685656545205\\
92.6472804161133	1.06961968696915\\
92.7343176726802	1.05853148202023\\
92.8213549292471	1.04672944191968\\
92.9083921858141	1.03419339977938\\
92.995429442381	1.02090673826156\\
93.0824666989479	1.00685705037773\\
93.1695039555148	0.992036810414916\\
93.2565412120817	0.976444037096442\\
93.3435784686486	0.960082928009996\\
93.4306157252155	0.942964441703438\\
93.4385282030853	0.941371230409302\\
93.4385282030853	1.08314918021006\\
93.5286971020263	1.07258482196015\\
93.6188660009673	1.0612864914816\\
93.7090348999083	1.04922779953854\\
93.7951052125338	1.03698656796965\\
93.8483868346353	1.02904333642766\\
93.8483868346353	1.09310459909116\\
93.9387774561835	1.08322723210595\\
94.0291680777318	1.07264152264122\\
94.11955869928	1.06131837262812\\
94.2099493208283	1.04923118685345\\
94.3003399423765	1.03635658420754\\
94.3907305639248	1.02267515705921\\
94.481121185473	1.00817226488313\\
94.5715118070213	0.992838843891121\\
94.6619024285695	0.976672209985225\\
94.7522930501178	0.95967682814593\\
94.8426836716661	0.941865017748356\\
94.9330742932143	0.923257560655742\\
95.0234649147626	0.903884177691282\\
95.1138555363108	0.883783839623646\\
95.1396814281817	0.877913894272183\\
95.1396814281817	1.07470297404144\\
95.2297902755069	1.06355769693107\\
95.319899122832	1.0516580027856\\
95.4100079701571	1.0389800521698\\
95.4960209607857	1.02613389447795\\
95.5492670978414	1.01781084678314\\
95.5492670978414	1.09192490888886\\
95.6427868515873	1.08160443534915\\
95.7162666581019	1.07296165648684\\
95.7162666581019	1.09748002704946\\
95.784835833279	1.09029234008692\\
95.8534050084562	1.0827095256075\\
95.9219741836333	1.07471817926469\\
95.9905433588105	1.06630551810731\\
96.0591125339876	1.05745954374291\\
96.1276817091648	1.04816921688142\\
96.196250884342	1.03842464202665\\
96.2648200595191	1.02821726065086\\
96.3333892346963	1.01754005072358\\
96.4019584098734	1.00638772998136\\
96.4705275850506	0.994756959833168\\
96.5390967602278	0.982646546316545\\
96.6076659354049	0.970057634070074\\
96.6762351105821	0.956993888895809\\
96.7448042857592	0.94346166417246\\
96.8133734609364	0.929470146176897\\
96.8819426361135	0.915031473300346\\
96.9505118112907	0.900160824233581\\
97.0190809864679	0.884876470459602\\
97.1562193368222	0.853155230794883\\
97.2933576871765	0.820075153636338\\
97.4304960375308	0.785889215045586\\
97.5676343878851	0.750889686898461\\
98.1161877893024	0.609407451277647\\
98.2533261396567	0.575355511813228\\
98.390464490011	0.542446313221575\\
98.5276028403653	0.510926935914711\\
98.5961720155425	0.495753108934423\\
98.6647411907197	0.480998263519581\\
98.7333103658968	0.46667982703174\\
98.801879541074	0.452812144532814\\
98.8704487162511	0.43940654142385\\
98.9390178914283	0.426471420545468\\
99.0075870666055	0.414012388988297\\
99.0761562417826	0.402032409646552\\
99.1447254169598	0.390531972506352\\
99.2132945921369	0.379509280768971\\
99.2818637673141	0.368960447145682\\
99.3504329424913	0.358879695997317\\
99.4190021176684	0.349259567401958\\
99.4875712928456	0.340091119694122\\
99.5561404680227	0.331364127503548\\
99.6247096431999	0.323067272813546\\
99.693278818377	0.315188327038555\\
99.7618479935542	0.307714322577553\\
99.8304171687314	0.300631712721923\\
99.9675555190857	0.287584466800354\\
100.036124694263	0.281591105427083\\
};

==> fig7b_part2a_220214.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
name = plot2a,
width=0.2\textwidth,
height=0.2\textwidth,
at=(plot1b.right of north east), anchor=left of north west,
scale only axis,
xlabel = $\CIntensity_\infty$,
xmin=0,
xmax=2.5,
ymin=0,
ymax=1.2,
axis background/.style={fill=white}
]
\addplot [color=blue,line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0.188581545388456	0\\
0.256404352405221	0\\
0.266093324836188	0.0133966106827925\\
0.275782297267154	0.0670435038932102\\
0.285471269698121	0.0964568921036815\\
0.295160242129087	0.120904632077888\\
0.304849214560054	0.142713093220437\\
0.31453818699102	0.16283715934695\\
0.324227159421987	0.181784691768771\\
0.333916131852953	0.199865413061552\\
0.353294076714886	0.234190169825635\\
0.372672021576819	0.266860201255988\\
0.392049966438752	0.298478807103836\\
0.421116883731651	0.344752425692332\\
0.518006608041316	0.497070953454974\\
0.527695580472283	0.511829350252236\\
0.537384552903249	0.525802727468372\\
0.556762497765182	0.55221501132592\\
0.576140442627115	0.577093119964564\\
0.595518387489048	0.60071354568969\\
0.614896332350981	0.623233257139533\\
0.634274277212914	0.644742901349209\\
0.653652222074847	0.665299917941859\\
0.67303016693678	0.684939619993894\\
0.692408111798713	0.703681270120634\\
0.711786056660646	0.721531732522882\\
0.731164001522579	0.738487808018292\\
0.750541946384512	0.754537791080409\\
0.769919891246444	0.769663390896764\\
0.789297836108378	0.783873505944475\\
0.80867578097031	0.797251022199986\\
0.828053725832243	0.809868071200299\\
0.847431670694176	0.821772800722457\\
0.866809615556109	0.833003526000899\\
0.886187560418042	0.843592997381511\\
0.905565505279975	0.853570515459814\\
0.924943450141908	0.862963241144275\\
0.944321395003841	0.871797115192479\\
0.963699339865774	0.880095268509905\\
0.983077284727707	0.88788215429571\\
1.00245522958964	0.895187744849642\\
1.02183317445157	0.902039094351857\\
1.04121111931351	0.908464295654033\\
1.07027803660641	0.917361158798948\\
1.0993449538993	0.925437878646377\\
1.1284118711922	0.932763797103154\\
1.1574787884851	0.939402364074557\\
1.186545705778	0.945412562066822\\
1.2156126230709	0.950849572941266\\
1.2446795403638	0.955765008968704\\
1.2737464576567	0.960206827205633\\
1.31250234738057	0.965467890356943\\
1.35125823710443	0.97005689205059\\
1.3900141268283	0.974053632096008\\
1.42877001655216	0.9775338801364\\
1.477214878707	0.981255104785734\\
1.52565974086183	0.984378610373891\\
1.58379357544763	0.987467919062482\\
1.64192741003343	0.989964464748939\\
1.70975021705019	0.992274428996009\\
1.78726199649792	0.994289552341005\\
1.87446274837662	0.995955134574747\\
1.98104144511725	0.997368340917848\\
2.10699808671982	0.998440018152424\\
2.27171061804625	0.999238808974657\\
2.50424595638944	0.999752962914633\\
2.91118279849003	0.99998778169372\\
3.0952732746784	0.99999998817224\\
};
\addplot [color=red, dashed,line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0.188581545388456	0\\
0.198270517819422	0.201292661198258\\
0.207959490250389	0.234170709120197\\
0.217648462681356	0.254771679094473\\
0.227337435112322	0.270405959894726\\
0.237026407543288	0.283301729518167\\
0.246715379974255	0.294428871459112\\
0.256404352405221	0.304317067557908\\
0.266093324836188	0.313285348484976\\
0.275782297267154	0.321543788271159\\
0.285471269698121	0.329249810921029\\
0.295160242129087	0.336509196517611\\
0.31453818699102	0.34998786142978\\
0.333916131852953	0.362424517790696\\
0.353294076714886	0.374120271199538\\
0.372672021576819	0.385273544100146\\
0.401738938869718	0.401301525172502\\
0.440494828593584	0.42189908821803\\
0.537384552903249	0.472942835587004\\
0.566451470196148	0.488871050273046\\
0.595518387489048	0.505382962810845\\
0.624585304781947	0.522421977863696\\
0.653652222074847	0.536462366671926\\
0.692408111798713	0.55509350793041\\
0.721475029091612	0.569620853451465\\
0.750541946384512	0.584925128915878\\
0.769919891246444	0.595686794597888\\
0.789297836108378	0.606993649639112\\
0.80867578097031	0.618935948073715\\
0.828053725832243	0.63162570548577\\
0.847431670694176	0.645181972129504\\
0.866809615556109	0.659750879439529\\
0.886187560418042	0.675509729820689\\
0.905565505279975	0.692657709451984\\
0.915254477710941	0.701831549740113\\
0.924943450141908	0.711455302308082\\
0.934632422572875	0.721563775934909\\
0.944321395003841	0.732199785423684\\
0.954010367434808	0.743411915893936\\
0.963699339865774	0.755256279520395\\
0.97338831229674	0.767794437915299\\
0.983077284727707	0.781080950302714\\
0.992766257158674	0.795180427477689\\
1.00245522958964	0.810155790764592\\
1.01214420202061	0.826075552302847\\
1.02183317445157	0.843005779805188\\
1.03152214688254	0.861021600856501\\
1.04121111931351	0.880308789529174\\
1.05090009174447	0.900938605684429\\
1.06058906417544	0.922863624810088\\
1.07996700903737	0.96887306410133\\
1.08965598146834	0.98944570982094\\
1.0993449538993	0.999815733697957\\
1.11872289876124	1\\
3.0952732746784	1\\
};
\end{axis}

==> fig7b_part2b_220214.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{axis}[%
name = plot2b,
yticklabel = \empty,
width=0.2\textwidth,
height=0.2\textwidth,
at=(plot2a.right of north east), anchor=left of north west,
scale only axis,
xmin=3.5,
xmax=5.5,
xtick = {4,5},
xlabel = $\CIntensity_\infty$,
ymin=0,
ymax=1.2,
axis background/.style={fill=white}
]
\addplot [color=blue,line width=1.0pt, forget plot]
  table[row sep=crcr]{%
3.60237347709409	0\\
4.00941026519596	0.000270503689050017\\
4.05463657498506	0.00107845548477226\\
4.07724972987961	0.00199294498367841\\
4.09986288477416	0.00351627651215747\\
4.12247603966871	0.00594356823915554\\
4.13378261711598	0.00761139465145355\\
4.14508919456325	0.00965406369176591\\
4.15639577201053	0.0121319195776541\\
4.1677023494578	0.0151098373904421\\
4.17900892690508	0.0186565754030159\\
4.19031550435235	0.0228439345178657\\
4.20162208179963	0.0277457306733897\\
4.2129286592469	0.0334365939487844\\
4.22423523669417	0.0399906159621599\\
4.23554181414145	0.0474798746202119\\
4.24684839158872	0.0559728719504822\\
4.258154969036	0.0655329262715814\\
4.26946154648327	0.0762165640213164\\
4.28076812393055	0.0880719589315584\\
4.29207470137782	0.101137466752857\\
4.30338127882509	0.1154403023335\\
4.31468785627237	0.130995402575538\\
4.32599443371964	0.147804513757879\\
4.33730101116692	0.165855535139468\\
4.34860758861419	0.185122142927513\\
4.35991416606147	0.205563709948022\\
4.37122074350874	0.227125527076859\\
4.38252732095601	0.249739323060062\\
4.39383389840329	0.273324070174215\\
4.41644705329784	0.323025182749999\\
4.43906020819239	0.375371799921322\\
4.47297994053421	0.456709902363535\\
4.50689967287603	0.538345487635409\\
4.52951282777058	0.591283629119215\\
4.55212598266513	0.642010078142865\\
4.57473913755968	0.689801845381263\\
4.58604571500695	0.71241548063794\\
4.59735229245422	0.734098791378886\\
4.6086588699015	0.754808703653587\\
4.61996544734877	0.774512786859521\\
4.63127202479605	0.793188904736926\\
4.64257860224332	0.810824728128734\\
4.6538851796906	0.827417131393664\\
4.66519175713787	0.842971494996297\\
4.67649833458514	0.857500936739473\\
4.68780491203242	0.871025493444638\\
4.69911148947969	0.88357127373231\\
4.71041806692697	0.895169600959314\\
4.72172464437424	0.905856163490165\\
4.73303122182152	0.915670187345325\\
4.74433779926879	0.924653644039026\\
4.75564437671606	0.93285050410557\\
4.76695095416334	0.940306044559986\\
4.77825753161061	0.947066216335714\\
4.78956410905789	0.953177075712475\\
4.80087068650516	0.958684281856036\\
4.81217726395244	0.963632660940783\\
4.82348384139971	0.968065835857349\\
4.83479041884698	0.972025919305082\\
4.84609699629426	0.975553267055665\\
4.85740357374153	0.978686287419698\\
4.88001672863608	0.983912455357355\\
4.90262988353063	0.987968590129417\\
4.92524303842518	0.991083219194238\\
4.94785619331973	0.99345012649045\\
4.97046934821427	0.99523065285708\\
5.0043890805561	0.997083767522295\\
5.03830881289792	0.998250102381411\\
5.08353512268702	0.999139144444319\\
5.15137458737066	0.999719853892767\\
5.28705351673795	0.999975646207347\\
6.16896655762534	0.9999999999999\\
6.99434671127636	0.999999999999921\\
};
\addplot [color=red, dashed,line width=1.0pt, forget plot]
  table[row sep=crcr]{%
3.60237347709409	0\\
4.12247603966871	0.000188652173763515\\
4.13378261711598	0.000641249467941307\\
4.14508919456325	0.00160513120077344\\
4.15639577201053	0.00331680942601587\\
4.1677023494578	0.00598925242269299\\
4.17900892690508	0.00978459415909771\\
4.19031550435235	0.0148263992930273\\
4.20162208179963	0.0212180425410393\\
4.2129286592469	0.0289784152501626\\
4.22423523669417	0.0381083027462745\\
4.23554181414145	0.0485849817791948\\
4.24684839158872	0.0603821701488823\\
4.258154969036	0.073412691877528\\
4.26946154648327	0.0875949160568297\\
4.28076812393055	0.102869646512956\\
4.29207470137782	0.119153723272014\\
4.30338127882509	0.13635987604648\\
4.31468785627237	0.154401617009587\\
4.32599443371964	0.173212559034606\\
4.34860758861419	0.21280701195674\\
4.37122074350874	0.25455374315558\\
4.39383389840329	0.297930933063019\\
4.42775363074511	0.364975092723666\\
4.54081940521785	0.591313465487933\\
4.5634325601124	0.634802297798553\\
4.58604571500695	0.67707336109028\\
4.6086588699015	0.717873742376454\\
4.63127202479605	0.756934655124874\\
4.6538851796906	0.793986272664012\\
4.67649833458514	0.828702045545324\\
4.68780491203242	0.845105159758616\\
4.69911148947969	0.860813702978487\\
4.71041806692697	0.8758013797383\\
4.72172464437424	0.890039184884539\\
4.73303122182152	0.903483075075469\\
4.74433779926879	0.916088991269096\\
4.75564437671606	0.927841493604736\\
4.76695095416334	0.938705003620351\\
4.77825753161061	0.948655320743858\\
4.78956410905789	0.957661192327414\\
4.80087068650516	0.965722422957095\\
4.81217726395244	0.97282116738588\\
4.82348384139971	0.97896929818766\\
4.83479041884698	0.984187895914719\\
4.84609699629426	0.98851896833872\\
4.85740357374153	0.992005590021554\\
4.86871015118881	0.994700765700225\\
4.88001672863608	0.996702666965031\\
4.89132330608335	0.99810591588957\\
4.90262988353063	0.999017142991888\\
4.92524303842518	0.999831481624489\\
4.97046934821427	0.999999961528556\\
6.99434671127636	1\\
};
\end{axis}

==> fig7b_part2c_220214.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0, 0}%
\definecolor{mycolor2}{rgb}{0, 0, 0}%
%

\begin{axis}[%
name = plot2c,
width=0.4\textwidth,
height=0.2\textwidth,
at=(plot1d.right of south east), anchor = left of south west,
scale only axis,
ytick = {0,0.1},
xmin=0,
xmax=4,
xlabel = leakage,
ymin=0,
ymax=0.14,
axis background/.style={fill=white}
]
\addplot [color=mycolor1, line width=1.0pt,]
  table[row sep=crcr]{%
0.0999999999999996	0.136851038399232\\
0.2	0.113031599497694\\
0.3	0.0969259914777201\\
0.4	0.0851487846547085\\
0.5	0.0761343974390805\\
0.7	0.0627274097262447\\
0.9	0.0532279636847237\\
1.1	0.0462310927792569\\
1.3	0.0407747213284706\\
1.5	0.0364071475534251\\
2	0.0282874230297665\\
2.5	0.0231428167232917\\
3	0.0192881731035737\\
3.5	0.016028134985782\\
4	0.0142101898934719\\
};\addlegendentry{Wasserstein}
\addplot [color=mycolor2, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0.0999999999999996	0.119045898654783\\
0.2	0.0977968955344473\\
0.3	0.0848785672788681\\
0.4	0.0786599223742774\\
0.5	0.067478626822739\\
0.7	0.0602194177309876\\
0.9	0.0514624000176989\\
1.1	0.0452271355395633\\
1.3	0.040748836926495\\
1.5	0.0347202974077412\\
2	0.0286286480117344\\
2.5	0.0241596156153925\\
3	0.0202815624807666\\
3.5	0.0176651182104806\\
4	0.0157307249302354\\
};
\addlegendentry{path-average distance}
\addplot[only marks, mark=*, mark options={}, mark size=1.5000pt, color=black, fill=black, forget plot] table[row sep=crcr]{%
x	y\\
0.1	0.136851038399232\\
};
\addplot[only marks, mark=*, mark options={}, mark size=1.5000pt, color=black, fill=black, forget plot] table[row sep=crcr]{%
x	y\\
4	0.0142101898934722\\
};
\end{axis}

==> fig7b_part3_extra_220211.tex <==

\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-0.168974128730547	0\\
0.242531426972192	0\\
0.242531426972192	1\\
0.323000895240845	1\\
0.323000895240845	2\\
0.331094201820818	2\\
0.331094201820818	3\\
0.485430962500246	3\\
0.485430962500246	4\\
0.511328499145407	4\\
0.511328499145407	5\\
0.747941414141366	5\\
0.747941414141366	6\\
0.87267232050722	6\\
0.87267232050722	7\\
1.0590270310149	7\\
1.0590270310149	8\\
1.24048602411626	8\\
1.24048602411626	9\\
1.29562320801925	9\\
1.29562320801925	10\\
1.43099737287712	10\\
1.43099737287712	11\\
1.44119725122376	11\\
1.44119725122376	12\\
1.57136637592622	12\\
1.57136637592622	13\\
2.11063752001272	13\\
2.11063752001272	14\\
2.32939129584391	14\\
2.32939129584391	15\\
2.3644355933836	15\\
2.3644355933836	16\\
2.5590150236136	16\\
2.5590150236136	17\\
3.34994397391924	17\\
3.34994397391924	18\\
3.66180098947807	18\\
3.66180098947807	19\\
4.27103254440738	19\\
4.27103254440738	20\\
4.27242731587892	21\\
4.279107549682	21\\
4.279107549682	22\\
4.32847829566025	22\\
4.32847829566025	23\\
4.44023072013263	23\\
4.44023072013263	24\\
4.49881586847421	24\\
4.49881586847421	25\\
4.88768377543516	25\\
4.88768377543516	26\\
5.15804246827994	26\\
5.15804246827994	27\\
5.30030143011857	27\\
5.30030143011857	28\\
5.52700493319151	28\\
5.52700493319151	29\\
6.21384214531732	29\\
6.21384214531732	30\\
6.21764424718249	30\\
6.21764424718249	31\\
6.39950975806866	31\\
6.39950975806866	32\\
6.55144928472836	32\\
6.55144928472836	33\\
6.80146194010178	33\\
6.80146194010178	34\\
7.10094935027323	34\\
7.10094935027323	35\\
7.31224967775398	35\\
7.31224967775398	36\\
7.35297367832771	36\\
7.35297367832771	37\\
7.42007848673764	37\\
7.42007848673764	38\\
7.63232166549208	38\\
7.63232166549208	39\\
8.60076185318474	39\\
8.60076185318474	40\\
8.65191545544558	40\\
8.65191545544558	41\\
8.9473885463811	41\\
8.9473885463811	42\\
9.06888618985343	42\\
9.06888618985343	43\\
9.90282417891225	43\\
9.90282417891225	44\\
9.99739200224326	44\\
9.99739200224326	45\\
10.2139119522388	45\\
};

==> fig7b_part3b_220211.tex <==

\addplot [color=blue, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-0.000256850892421667	4.42585953499815\\
0.0738141491340709	4.41088754529585\\
0.147885149160564	4.39618964643962\\
0.221956149187056	4.38176082067341\\
0.242531426972192	4.37779989973666\\
0.242531426972192	4.42724372552159\\
0.315758643096668	4.41241568286627\\
0.323000895240847	4.41096383786725\\
0.323000895240847	4.46040766365218\\
0.331094201820816	4.45868859131946\\
0.331094201820816	4.50813241710439\\
0.402089111733352	4.49233254317329\\
0.473084021645889	4.47681001003645\\
0.485430962500242	4.47413838841466\\
0.485430962500242	4.52358221419959\\
0.511328499145403	4.51768680635938\\
0.511328499145403	4.56713063214431\\
0.579946244494232	4.55085404325481\\
0.648563989843062	4.53485367819798\\
0.71718173519189	4.51912484928363\\
0.747941414141366	4.51216091562024\\
0.747941414141366	4.56160474140516\\
0.816543412642586	4.54542561236921\\
0.872672320507222	4.53239253323551\\
0.872672320507222	4.58183635902044\\
0.939760016289986	4.56567563268786\\
1.00871125917783	4.54934542552072\\
1.0590270310149	4.53760480610591\\
1.0590270310149	4.58704863189084\\
1.1261668584624	4.57078888621897\\
1.19512127584092	4.55437073646116\\
1.24048602411626	4.54372231156637\\
1.24048602411626	4.5931661373513\\
1.29562320801925	4.57970964477423\\
1.29562320801925	4.62915347055916\\
1.36195654879961	4.61239647311823\\
1.42828988957997	4.59591446306322\\
1.43099737287712	4.59524750354249\\
1.43099737287712	4.64469132932742\\
1.44119725122376	4.6420570996749\\
1.44119725122376	4.69150092545983\\
1.50628181357499	4.674052802935\\
1.57136637592622	4.65688566263473\\
1.57136637592622	4.70632948841966\\
1.6360789132166	4.68874285380815\\
1.70079145050698	4.67143782618039\\
1.76550398779736	4.65440989628859\\
1.83021652508774	4.63765462708955\\
1.89492906237812	4.62116765258846\\
1.9596415996685	4.60494467670125\\
2.02435413695888	4.58898147213517\\
2.09445938569013	4.57197632247083\\
2.11063752001272	4.56809410827886\\
2.11063752001272	4.61753793406379\\
2.17626365276208	4.60114673060969\\
2.24407732326974	4.58448869818058\\
2.31189099377741	4.56811007816311\\
2.3293912958439	4.56392812034803\\
2.3293912958439	4.61337194613296\\
2.3644355933836	4.60462193732828\\
2.3644355933836	4.65406576311321\\
2.4305925996618	4.63694520398296\\
2.49674960594	4.62010485768004\\
2.5590150236136	4.60450698458293\\
2.5590150236136	4.65395081036786\\
2.62228933963805	4.63757218105462\\
2.68556365566251	4.62145003260112\\
2.74883797168696	4.60558034864984\\
2.81211228771141	4.5899591757373\\
2.88329589323891	4.57267756149826\\
2.95447949876642	4.5557000966973\\
3.02566310429393	4.53902142842703\\
3.09684670982143	4.52263629798905\\
3.16803031534894	4.50653953923594\\
3.23921392087645	4.49072607694241\\
3.31039752640396	4.47519092520506\\
3.34994397391924	4.46667873652242\\
3.34994397391924	4.51612256230735\\
3.41855251734218	4.50071366111352\\
3.49027963092071	4.48488384420596\\
3.56200674449924	4.46933473389849\\
3.63373385807777	4.45406135248381\\
3.66180098947806	4.44815880477501\\
3.66180098947806	4.49760263055994\\
3.73490877606958	4.48152709522465\\
3.8080165626611	4.46574206106702\\
3.88112434925262	4.45024227843703\\
3.95423213584413	4.43502259255115\\
4.02733992243565	4.42007794177802\\
4.10044770902717	4.40540335595504\\
4.17355549561868	4.39099395473552\\
4.2466632822102	4.37684494596552\\
4.27103254440737	4.37218565892745\\
4.27103254440737	4.42162948471238\\
4.27242731587892	4.42134646762397\\
4.27242731587892	4.4707902934089\\
4.27910754968199	4.46935383053\\
4.27910754968199	4.51879765631493\\
4.32847829566025	4.50765008867055\\
4.32847829566025	4.55709391445548\\
4.3966472745884	4.54109209827055\\
4.44023072013262	4.53100310645646\\
4.44023072013262	4.58044693224139\\
4.49881586847421	4.56633960343969\\
4.49881586847421	4.61578342922462\\
4.56492341265757	4.5993016687637\\
4.63103095684093	4.58308946586341\\
4.69713850102429	4.56714241193652\\
4.76713472427727	4.55054148108531\\
4.83713094753024	4.53422788879045\\
4.88768377543516	4.52262173962599\\
4.88768377543516	4.57206556541092\\
4.95527344864636	4.55594828738545\\
5.02286312185755	4.54010046599499\\
5.09315638199719	4.52389972963413\\
5.15804246827993	4.50919524879655\\
5.15804246827993	4.55863907458148\\
5.22632676996248	4.5425843217286\\
5.2960336612634	4.52647474046969\\
5.30030143011856	4.52549750986039\\
5.30030143011856	4.57494133564532\\
5.36831248104045	4.55867605100616\\
5.43632353196234	4.542684378424\\
5.50433458288422	4.52696171523991\\
5.52700493319151	4.52177982303372\\
5.52700493319151	4.57122364881865\\
5.5956886544041	4.55486201643819\\
5.66437237561668	4.53877831582732\\
5.73305609682926	4.52296782581478\\
5.80173981804184	4.5074259054269\\
5.87042353925442	4.4921479925253\\
5.939107260467	4.47712960246772\\
6.00779098167958	4.46236632679165\\
6.08334307501342	4.44641621073781\\
6.15889516834726	4.43076387581662\\
6.21384214531732	4.41956421710135\\
6.21384214531732	4.46900804288628\\
6.21764424718249	4.46819186601082\\
6.21764424718249	4.51763569179575\\
6.2885717964281	4.50168401924221\\
6.3594993456737	4.48601208872944\\
6.39950975806866	4.47729306942102\\
6.39950975806866	4.52673689520595\\
6.46940194033212	4.5108587568511\\
6.53929412259558	4.49525504159179\\
6.55144928472836	4.49256901283161\\
6.55144928472836	4.54201283861654\\
6.62145282823291	4.52584518909046\\
6.69145637173747	4.5099574076468\\
6.76145991524203	4.49434464966399\\
6.80146194010178	4.4855447180511\\
6.80146194010178	4.53498854383603\\
6.87034404444121	4.51919733912267\\
6.93922614878065	4.50367514458018\\
7.01110312722179	4.48775992478882\\
7.08298010566294	4.47212751042313\\
7.10094935027323	4.46826300430158\\
7.10094935027323	4.51770683008651\\
7.17067845834188	4.50202112407654\\
7.24040756641052	4.48660588829307\\
7.31224967775398	4.47100148616201\\
7.31224967775398	4.52044531194694\\
7.35297367832771	4.51122356272989\\
7.35297367832771	4.56066738851482\\
7.42007848673764	4.54485397000366\\
7.42007848673764	4.59429779578859\\
7.48799630393906	4.57772945152675\\
7.55591412114048	4.56143943849764\\
7.6238319383419	4.54542308102131\\
7.63232166549208	4.54344004793732\\
7.63232166549208	4.59288387372225\\
7.70011247863057	4.57636995889832\\
7.76790329176905	4.56013294656169\\
7.83569410490754	4.54416819365901\\
7.90348491804602	4.52847113499086\\
7.97127573118451	4.51303728190629\\
8.039066544323	4.49786222101929\\
8.10685735746148	4.48294161294674\\
8.17464817059997	4.46827119106754\\
8.24243898373846	4.4538467603026\\
8.31991419875387	4.43765762215081\\
8.39738941376928	4.42177834684905\\
8.47486462878469	4.40620300356981\\
8.55233984380011	4.39092577500262\\
8.60076185318474	4.38152635358596\\
8.60076185318474	4.43097017937089\\
8.65191545544558	4.42053617262686\\
8.65191545544558	4.46997999841179\\
8.72282899727011	4.45486701537068\\
8.79669727000399	4.43940602939277\\
8.87056554273786	4.42422731871711\\
8.94443381547174	4.40932572976901\\
8.9473885463811	4.40873535846585\\
8.9473885463811	4.45817918425078\\
9.0202871324645	4.44285963404573\\
9.06888618985343	4.43280027325353\\
9.06888618985343	4.48224409903846\\
9.14394060886872	4.46602938173209\\
9.21899502788402	4.45011541007253\\
9.29404944689931	4.43449660592094\\
9.36910386591461	4.41916749460014\\
9.4441582849299	4.40412270297558\\
9.5192127039452	4.38935695757197\\
9.59426712296049	4.37486508272484\\
9.66932154197578	4.36064199876638\\
9.74437596099108	4.3466827202449\\
9.81943038000637	4.33298235417737\\
9.89448479902167	4.31953609833432\\
9.90282417891225	4.31805755014125\\
9.90282417891225	4.36750137592618\\
9.97942411581037	4.35312756520415\\
9.99739200224326	4.34979551223782\\
9.99739200224326	4.39923933802275\\
10.0017224012432	4.39838513852327\\
};
\addplot [color=red, dashed, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
-0.000256850892421667	4.40557287079745\\
0.0573539269059609	4.39291726276832\\
0.110849649147317	4.3814325226981\\
0.164345371388672	4.37021318256241\\
0.217841093630028	4.35926625617403\\
0.242531426972192	4.35430737841036\\
0.242531426972192	4.40684699955622\\
0.298860054760251	4.39444145341616\\
0.323000895240847	4.38921110859816\\
0.323000895240847	4.44337250928273\\
0.331094201820816	4.44146921943178\\
0.331094201820816	4.49698556673579\\
0.402089111733352	4.47941645192779\\
0.468453918825505	4.46326201410789\\
0.485430962500242	4.45917499695566\\
0.485430962500242	4.51486541486839\\
0.511328499145403	4.50833453676567\\
0.511328499145403	4.5637719790093\\
0.620170440043546	4.5357551590508\\
0.707717218592052	4.51349432645893\\
0.747941414141366	4.5033736777413\\
0.747941414141366	4.55888508678428\\
0.851468066425026	4.53228110905928\\
0.872672320507222	4.52687321856076\\
0.872672320507222	4.581939445974\\
1.00684771207275	4.54723583648184\\
1.0590270310149	4.53385448266238\\
1.0590270310149	4.5887424096912\\
1.20782340535801	4.55021265432127\\
1.24048602411626	4.54181576813662\\
1.24048602411626	4.5964748415576\\
1.29562320801925	4.5821464188936\\
1.29562320801925	4.63523332263372\\
1.43099737287712	4.60009227556062\\
1.43099737287712	4.65226112826996\\
1.44119725122376	4.64963564220672\\
1.44119725122376	4.69858768750577\\
1.51799703479821	4.67922952561804\\
1.57136637592622	4.66563438297565\\
1.57136637592622	4.71333748890019\\
1.64147162465746	4.69587937442373\\
1.72236229627044	4.67544451538726\\
1.81403839076515	4.65198537040748\\
1.92728533102331	4.62270738340735\\
2.11063752001272	4.57507073408779\\
2.11063752001272	4.62848288858473\\
2.3293912958439	4.5716658049381\\
2.3293912958439	4.62522702810058\\
2.3644355933836	4.61613073948603\\
2.3644355933836	4.66736708106607\\
2.4597795141963	4.64287232730873\\
2.5590150236136	4.61716606282304\\
2.5590150236136	4.66833860253847\\
2.65392649765028	4.64396581181209\\
2.78047512969918	4.61117082431917\\
3.00984452528782	4.55168197484904\\
3.10475599932449	4.52735711483592\\
3.18384889435506	4.50733621856997\\
3.25503249988256	4.48956473150097\\
3.32621610541007	4.47207035407958\\
3.34994397391924	4.46630721363429\\
3.34994397391924	4.522027696853\\
3.43102679796453	4.50158004408375\\
3.50275391154306	4.4837595252802\\
3.571362454966	4.46698892031081\\
3.63685242823336	4.4512630041879\\
3.66180098947806	4.44535056630665\\
3.66180098947806	4.5009172613766\\
3.73490877606958	4.48276684766127\\
3.8019242471118	4.46639882450175\\
3.86893971815403	4.45032118555539\\
3.92986287364696	4.43598144727428\\
3.99078602913989	4.42192536379261\\
4.04561686908353	4.4095322975277\\
4.10044770902717	4.39739534389802\\
4.15527854897081	4.38552501728001\\
4.21010938891444	4.37393056095987\\
4.26494022885808	4.36261995218852\\
4.27103254440737	4.36138104347149\\
4.27103254440737	4.4142965724268\\
4.27242731587892	4.41398211310496\\
4.27242731587892	4.46894403114578\\
4.27910754968199	4.46732333299233\\
4.27910754968199	4.52304623838287\\
4.32847829566025	4.51055231903495\\
4.32847829566025	4.56595321694904\\
4.4391131958879	4.53745396474161\\
4.44023072013262	4.53716780023305\\
4.44023072013262	4.59196377992176\\
4.49881586847421	4.57674711494955\\
4.49881586847421	4.63008409735558\\
4.88379509636555	4.53046047676204\\
4.88768377543516	4.52946849441427\\
4.88768377543516	4.58447088777327\\
5.025566708786	4.5487897482392\\
5.12019225128167	4.52457140971461\\
5.15804246827993	4.51497429228176\\
5.15804246827993	4.57029592966022\\
5.27469481698761	4.54020897226037\\
5.30030143011856	4.53365320536377\\
5.30030143011856	4.58854656630155\\
5.44765870711598	4.55038918592599\\
5.52700493319151	4.53004563666491\\
5.52700493319151	4.58503344025375\\
5.66437237561668	4.54947989510473\\
5.76052958531429	4.52486374561185\\
5.84295005076939	4.50404093428411\\
5.91850214410323	4.48523869953445\\
5.9871858653158	4.46842491123545\\
6.04900121440713	4.45354898536579\\
6.11081656349845	4.43893989663074\\
6.17263191258978	4.4246187416645\\
6.21384214531732	4.41524080891185\\
6.21384214531732	4.47023574351111\\
6.21764424718249	4.46931167678649\\
6.21764424718249	4.52503798204999\\
6.29948372708127	4.50435846637466\\
6.3740485865446	4.48579499971217\\
6.39950975806866	4.47952576149934\\
6.39950975806866	4.53524166064718\\
6.48611528826469	4.51322520302337\\
6.55144928472836	4.49682933896644\\
6.55144928472836	4.55242183048983\\
6.64895422032399	4.52742780799421\\
6.73145839659722	4.50654857930725\\
6.80146194010178	4.4890807024879\\
6.80146194010178	4.54474483185037\\
6.89430303725493	4.52102897760829\\
6.97516463800122	4.50065092362165\\
7.04704161644237	4.48280775714354\\
7.10094935027323	4.46961876030141\\
7.10094935027323	4.52534543267147\\
7.18335647799072	4.50451923940619\\
7.25731159260899	4.48610389137806\\
7.31224967775398	4.47262055896581\\
7.31224967775398	4.52834859646029\\
7.35297367832771	4.51800111069803\\
7.35297367832771	4.57326359379535\\
7.42007848673764	4.55590223623093\\
7.42007848673764	4.61009017249109\\
7.63232166549208	4.55502543971335\\
7.63232166549208	4.60924515906576\\
7.85506290866139	4.55148068634548\\
7.95190692743066	4.52666599045686\\
8.02938214244607	4.50706067346802\\
8.10685735746148	4.48773552930982\\
8.17464817059997	4.47109755603675\\
8.24243898373846	4.45474772865513\\
8.30054539500001	4.44098617903724\\
8.35865180626157	4.42747653398239\\
8.41675821752314	4.41423498371152\\
8.47486462878469	4.40127616116565\\
8.53297104004625	4.3886131111471\\
8.59107745130781	4.37625727653338\\
8.60076185318474	4.37422855336855\\
8.60076185318474	4.42776520339839\\
8.65191545544558	4.41608825638219\\
8.65191545544558	4.47110500540932\\
8.7169195354514	4.45542107138932\\
8.77896888454785	4.44072203220613\\
8.83806350273496	4.42699003847581\\
8.89715812092206	4.41353591041019\\
8.9473885463811	4.40232986231384\\
8.9473885463811	4.45695106329717\\
9.01056732098671	4.44195809657312\\
9.06888618985343	4.42838097496766\\
9.06888618985343	4.48367674031342\\
9.13560122897814	4.46736642555727\\
9.20231626810284	4.45134211836912\\
9.26069192733696	4.43757801008572\\
9.31906758657108	4.42407238320937\\
9.3774432458052	4.4108412587786\\
9.43581890503931	4.39789906180511\\
9.49419456427343	4.38525859425813\\
9.55257022350755	4.37293102539954\\
9.60260650285108	4.36262085722174\\
9.65264278219461	4.35255268172348\\
9.70267906153814	4.34273071942507\\
9.75271534088166	4.33315836212006\\
9.80275162022519	4.32383819855225\\
9.85278789956872	4.31477204402001\\
9.90282417891225	4.30596097335332\\
9.90282417891225	4.35527606409662\\
9.95578215997762	4.3448167281878\\
9.99739200224326	4.33679412863279\\
9.99739200224326	4.38829849728072\\
10.0017224012432	4.38736752629412\\
};

==> fig7b_part3c_220211.tex <==
\pgfplotsset{my plot options/.style={color=red, line width=0.5pt, opacity = 0.07, forget plot}}
\addplot [my plot options]
  table[row sep=crcr]{%
0.500663657537274	0\\
0.794677584869618	0\\
0.794677584869618	1\\
0.851372207863825	1\\
0.851372207863825	2\\
1.02806436473831	2\\
1.02806436473831	3\\
1.22551298426886	3\\
1.22551298426886	4\\
1.34053134015642	4\\
1.34053134015642	5\\
1.44685605164505	5\\
1.44685605164505	6\\
1.49497097011808	6\\
1.49497097011808	7\\
1.59036962395925	7\\
1.59036962395925	8\\
2.28296527467228	8\\
2.28296527467228	9\\
2.46043857579349	9\\
2.46043857579349	10\\
2.56885090612003	10\\
2.56885090612003	11\\
2.64036477404227	11\\
2.64036477404227	12\\
3.04721602244755	12\\
3.04721602244755	13\\
3.6161944894076	13\\
3.6161944894076	14\\
3.84701515731771	14\\
3.84701515731771	15\\
4.31037644416697	15\\
4.31037644416697	16\\
4.40424177368809	16\\
4.40424177368809	17\\
4.81997426299543	17\\
4.81997426299543	18\\
4.90151374209999	18\\
4.90151374209999	19\\
5.02876254383653	19\\
5.02876254383653	20\\
5.28614432081147	20\\
5.28614432081147	21\\
5.3108422541117	21\\
5.3108422541117	22\\
5.48917898814597	22\\
5.48917898814597	23\\
5.68877485156774	23\\
5.68877485156774	24\\
5.82802742831344	24\\
5.82802742831344	25\\
6.22759815247927	25\\
6.22759815247927	26\\
6.94633474957813	26\\
6.94633474957813	27\\
7.21508163680079	27\\
7.21508163680079	28\\
7.37339645646138	28\\
7.37339645646138	29\\
7.74769998309512	29\\
7.74769998309512	30\\
7.79738512297157	30\\
7.79738512297157	31\\
7.8877823279659	31\\
7.8877823279659	32\\
8.07232724823967	32\\
8.07232724823967	33\\
8.74985720443699	33\\
8.74985720443699	34\\
8.93369589177697	34\\
8.93369589177697	35\\
8.97797496761849	35\\
8.97797496761849	36\\
9.32121848107948	36\\
9.32121848107948	37\\
9.65665212872476	37\\
9.65665212872476	38\\
9.75096022947866	38\\
9.75096022947866	39\\
9.75646565175339	39\\
9.75646565175339	40\\
10.116787404338	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0836367265701483	0\\
0.731431614080023	0\\
0.731431614080023	1\\
1.324577114944	1\\
1.324577114944	2\\
2.32938091026734	2\\
2.32938091026734	3\\
2.72726810030266	3\\
2.72726810030266	4\\
2.83523369451578	4\\
2.83523369451578	5\\
3.03653190764589	5\\
3.03653190764589	6\\
3.46419866530456	6\\
3.46419866530456	7\\
3.69681855774284	7\\
3.69681855774284	8\\
3.92096512687644	8\\
3.92096512687644	9\\
4.37631391603574	9\\
4.37631391603574	10\\
4.45212701158868	10\\
4.45212701158868	11\\
4.46704504410171	11\\
4.46704504410171	12\\
4.8542944215037	12\\
4.8542944215037	13\\
4.89664052975714	13\\
4.89664052975714	14\\
5.44730970220692	14\\
5.44730970220692	15\\
5.96100673624885	15\\
5.96100673624885	16\\
6.06862600215089	16\\
6.06862600215089	17\\
6.29585550719763	17\\
6.29585550719763	18\\
6.52154913001269	18\\
6.52154913001269	19\\
6.88728411249201	19\\
6.88728411249201	20\\
7.04233048968348	20\\
7.04233048968348	21\\
7.17599436817368	21\\
7.17599436817368	22\\
7.42461447683228	22\\
7.42461447683228	23\\
7.65531604834367	23\\
7.65531604834367	24\\
7.73492597416946	24\\
7.73492597416946	25\\
7.86982526666436	25\\
7.86982526666436	26\\
7.93661435776057	26\\
7.93661435776057	27\\
7.98942396350292	27\\
7.98942396350292	28\\
8.21061254330208	28\\
8.21061254330208	29\\
8.4250009183166	29\\
8.4250009183166	30\\
8.43978325617134	30\\
8.43978325617134	31\\
8.56399372757276	31\\
8.56399372757276	32\\
8.65321953516652	32\\
8.65321953516652	33\\
9.45882247949649	33\\
9.45882247949649	34\\
10.6207493842132	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0582365602499095	0\\
0.218489162745463	0\\
0.218489162745463	1\\
0.375820883570768	1\\
0.375820883570768	2\\
0.381954180493821	2\\
0.381954180493821	3\\
0.884309684147354	3\\
0.884309684147354	4\\
1.11475175472515	4\\
1.11475175472515	5\\
1.16275967600069	5\\
1.16275967600069	6\\
1.26775301173072	6\\
1.26775301173072	7\\
1.98147000739208	7\\
1.98147000739208	8\\
2.57412187199603	8\\
2.57412187199603	9\\
2.91364805547912	9\\
2.91364805547912	10\\
2.92272811683148	10\\
2.92272811683148	11\\
3.5539676679367	11\\
3.5539676679367	12\\
3.96127288797544	12\\
3.96127288797544	13\\
4.009494432885	13\\
4.009494432885	14\\
4.0097003329326	15\\
4.17535384134842	15\\
4.17535384134842	16\\
4.28132912894682	16\\
4.28132912894682	17\\
4.540316980006	17\\
4.540316980006	18\\
4.58144689228883	18\\
4.58144689228883	19\\
4.62966594273531	19\\
4.62966594273531	20\\
4.72405838077265	20\\
4.72405838077265	21\\
5.29006289486003	21\\
5.29006289486003	22\\
5.47967282055244	22\\
5.47967282055244	23\\
5.5110667218968	23\\
5.5110667218968	24\\
5.7571879228878	24\\
5.7571879228878	25\\
5.8375389040441	25\\
5.8375389040441	26\\
5.86363830797256	26\\
5.86363830797256	27\\
5.90951074468267	27\\
5.90951074468267	28\\
6.00220360004064	28\\
6.00220360004064	29\\
6.60905899952951	29\\
6.60905899952951	30\\
6.65418864578685	30\\
6.65418864578685	31\\
7.08260032746464	31\\
7.08260032746464	32\\
7.55246610652899	32\\
7.55246610652899	33\\
7.59634412681662	33\\
7.59634412681662	34\\
7.80252695924247	34\\
7.80252695924247	35\\
7.8928584722877	35\\
7.8928584722877	36\\
8.33296954733197	36\\
8.33296954733197	37\\
8.55471751910858	37\\
8.55471751910858	38\\
8.67952732062125	38\\
8.67952732062125	39\\
8.80760476113763	39\\
8.80760476113763	40\\
8.99831344949843	40\\
8.99831344949843	41\\
9.32949290289334	41\\
9.32949290289334	42\\
9.59025570523578	42\\
9.59025570523578	43\\
10.3663572888037	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0240967662602358	0\\
0.0695320659678131	0\\
0.0695320659678131	1\\
0.532896040528968	1\\
0.532896040528968	2\\
0.697213928813781	2\\
0.697213928813781	3\\
0.727089361998551	3\\
0.727089361998551	4\\
1.1415552190166	4\\
1.1415552190166	5\\
1.18988909944272	5\\
1.18988909944272	6\\
1.22729833310183	6\\
1.22729833310183	7\\
1.7275027485076	7\\
1.7275027485076	8\\
2.0513975311959	8\\
2.0513975311959	9\\
2.3468705817739	9\\
2.3468705817739	10\\
3.03302829261244	10\\
3.03302829261244	11\\
3.20007303604434	11\\
3.20007303604434	12\\
3.27535356922975	12\\
3.27535356922975	13\\
3.38687518369547	13\\
3.38687518369547	14\\
3.70121401962682	14\\
3.70121401962682	15\\
3.75378279600696	15\\
3.75378279600696	16\\
3.90591269374157	16\\
3.90591269374157	17\\
4.08739815965998	17\\
4.08739815965998	18\\
4.14223310656532	18\\
4.14223310656532	19\\
4.33777093111969	19\\
4.33777093111969	20\\
4.9249982922239	20\\
4.9249982922239	21\\
5.06314813655846	21\\
5.06314813655846	22\\
5.57462314349822	22\\
5.57462314349822	23\\
5.76827991442926	23\\
5.76827991442926	24\\
6.39827123099444	24\\
6.39827123099444	25\\
6.4246315360247	25\\
6.4246315360247	26\\
6.46516578303586	26\\
6.46516578303586	27\\
6.48383455734135	27\\
6.48383455734135	28\\
6.97834640756738	28\\
6.97834640756738	29\\
7.00928028429233	29\\
7.00928028429233	30\\
7.05266297500515	30\\
7.05266297500515	31\\
7.48798718484532	31\\
7.48798718484532	32\\
7.49270678489049	32\\
7.49270678489049	33\\
7.50099789701526	33\\
7.50099789701526	34\\
7.79817870262721	34\\
7.79817870262721	35\\
7.84705559203424	35\\
7.84705559203424	36\\
8.23554788187485	36\\
8.23554788187485	37\\
8.33872388331858	37\\
8.33872388331858	38\\
9.0128904871321	38\\
9.0128904871321	39\\
9.07867641072615	39\\
9.07867641072615	40\\
9.21349061979657	40\\
9.21349061979657	41\\
9.28488789423233	41\\
9.28488789423233	42\\
9.44218576516808	42\\
9.44218576516808	43\\
9.46237076314264	43\\
9.46237076314264	44\\
9.55341299560821	44\\
9.55341299560821	45\\
9.83745867793778	45\\
9.83745867793778	46\\
10.1108808058966	46\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.618612680705532	0\\
0.762404619540597	0\\
0.762404619540597	1\\
1.11856610975376	1\\
1.11856610975376	2\\
1.17616757978426	2\\
1.17616757978426	3\\
1.29548994413064	3\\
1.29548994413064	4\\
2.91240217082824	4\\
2.91240217082824	5\\
2.94881158436198	5\\
2.94881158436198	6\\
3.14957904486791	6\\
3.14957904486791	7\\
3.23245156300303	7\\
3.23245156300303	8\\
3.49093915554597	8\\
3.49093915554597	9\\
3.57236944789308	9\\
3.57236944789308	10\\
3.66736250706847	10\\
3.66736250706847	11\\
3.94154873829925	11\\
3.94154873829925	12\\
3.97979990819454	12\\
3.97979990819454	13\\
4.31829914533068	13\\
4.31829914533068	14\\
4.56184535759177	14\\
4.56184535759177	15\\
4.72492262125702	15\\
4.72492262125702	16\\
4.96270709624892	16\\
4.96270709624892	17\\
5.01270212822885	17\\
5.01270212822885	18\\
5.1027892198583	18\\
5.1027892198583	19\\
5.19437688614231	19\\
5.19437688614231	20\\
5.46211757505064	20\\
5.46211757505064	21\\
5.67680532889682	21\\
5.67680532889682	22\\
5.90959499660521	22\\
5.90959499660521	23\\
6.13134865107925	23\\
6.13134865107925	24\\
6.24928288836004	24\\
6.24928288836004	25\\
6.29478960585404	25\\
6.29478960585404	26\\
6.34098132866433	26\\
6.34098132866433	27\\
6.41820223965815	27\\
6.41820223965815	28\\
6.62902371264084	28\\
6.62902371264084	29\\
7.45007432342067	29\\
7.45007432342067	30\\
7.63266802468758	30\\
7.63266802468758	31\\
7.91408580888352	31\\
7.91408580888352	32\\
8.08808431901817	32\\
8.08808431901817	33\\
8.42536335892698	33\\
8.42536335892698	34\\
8.52905566454906	34\\
8.52905566454906	35\\
9.39331529939935	35\\
9.39331529939935	36\\
9.51589746935235	36\\
9.51589746935235	37\\
9.83482394345685	37\\
9.83482394345685	38\\
10.0378766289596	38\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0287729285034004	0\\
0.135481341778757	0\\
0.135481341778757	1\\
0.470136778096602	1\\
0.470136778096602	2\\
0.505534189382196	2\\
0.505534189382196	3\\
0.884874114643495	3\\
0.884874114643495	4\\
1.05668762603661	4\\
1.05668762603661	5\\
1.08831186049743	5\\
1.08831186049743	6\\
1.13585466494091	6\\
1.13585466494091	7\\
1.36580291787437	7\\
1.36580291787437	8\\
1.51941423225934	8\\
1.51941423225934	9\\
1.89058585998757	9\\
1.89058585998757	10\\
2.0406742552149	10\\
2.0406742552149	11\\
2.29224645409618	11\\
2.29224645409618	12\\
2.62188605543475	12\\
2.62188605543475	13\\
3.05843222597017	13\\
3.05843222597017	14\\
3.06107788844539	14\\
3.06107788844539	15\\
3.17187543979627	15\\
3.17187543979627	16\\
3.51447257612254	16\\
3.51447257612254	17\\
3.64165651062896	17\\
3.64165651062896	18\\
3.66690348647354	18\\
3.66690348647354	19\\
4.08191492957263	19\\
4.08191492957263	20\\
4.0936439877153	20\\
4.0936439877153	21\\
4.17575366579975	21\\
4.17575366579975	22\\
4.61679031242843	22\\
4.61679031242843	23\\
4.65490209785003	23\\
4.65490209785003	24\\
4.89075705704664	24\\
4.89075705704664	25\\
5.31395311563771	25\\
5.31395311563771	26\\
6.11924972745682	26\\
6.11924972745682	27\\
6.49089123789868	27\\
6.49089123789868	28\\
6.70173329705893	28\\
6.70173329705893	29\\
6.78697909935579	29\\
6.78697909935579	30\\
6.87449009211857	30\\
6.87449009211857	31\\
7.30339370416232	31\\
7.30339370416232	32\\
7.34224888846858	32\\
7.34224888846858	33\\
7.49279675377714	33\\
7.49279675377714	34\\
7.55063345231638	34\\
7.55063345231638	35\\
7.85421399888014	35\\
7.85421399888014	36\\
8.06089526329662	36\\
8.06089526329662	37\\
8.20388686086916	37\\
8.20388686086916	38\\
8.27322814078613	38\\
8.27322814078613	39\\
8.67597406897223	39\\
8.67597406897223	40\\
9.13520134391362	40\\
9.13520134391362	41\\
9.25454398388534	41\\
9.25454398388534	42\\
9.42447539975546	42\\
9.42447539975546	43\\
9.79445062959483	43\\
9.79445062959483	44\\
10.0197321789806	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
1.1563370269905	0\\
1.19604626376493	0\\
1.19604626376493	1\\
1.21341224911902	1\\
1.21341224911902	2\\
1.90020928888073	2\\
1.90020928888073	3\\
1.91910238810318	3\\
1.91910238810318	4\\
2.04134260729652	4\\
2.04134260729652	5\\
2.16269197625949	5\\
2.16269197625949	6\\
2.35610601545191	6\\
2.35610601545191	7\\
2.41884474156683	7\\
2.41884474156683	8\\
2.66715472665717	8\\
2.66715472665717	9\\
3.14264096238836	9\\
3.14264096238836	10\\
3.17326079428836	10\\
3.17326079428836	11\\
3.52964759403902	11\\
3.52964759403902	12\\
3.55657945735064	12\\
3.55657945735064	13\\
3.56104628057821	13\\
3.56104628057821	14\\
3.62943418801155	14\\
3.62943418801155	15\\
3.94172159795541	15\\
3.94172159795541	16\\
4.08052019724569	16\\
4.08052019724569	17\\
4.14668408417915	17\\
4.14668408417915	18\\
4.20499228248259	18\\
4.20499228248259	19\\
4.5921663932053	19\\
4.5921663932053	20\\
4.64009630795798	20\\
4.64009630795798	21\\
4.65226149962434	21\\
4.65226149962434	22\\
5.2675652611434	22\\
5.2675652611434	23\\
5.84590970455439	23\\
5.84590970455439	24\\
5.93718073124656	24\\
5.93718073124656	25\\
5.98536743090915	25\\
5.98536743090915	26\\
6.03382539185341	26\\
6.03382539185341	27\\
6.24071459075023	27\\
6.24071459075023	28\\
6.86532677629359	28\\
6.86532677629359	29\\
6.87198056673277	29\\
6.87198056673277	30\\
7.06601719692804	30\\
7.06601719692804	31\\
7.13721653756701	31\\
7.13721653756701	32\\
7.57429102614811	32\\
7.57429102614811	33\\
7.93700551047975	33\\
7.93700551047975	34\\
8.30472252100562	34\\
8.30472252100562	35\\
8.63695694608349	35\\
8.63695694608349	36\\
8.66839743621161	36\\
8.66839743621161	37\\
8.73038138355348	37\\
8.73038138355348	38\\
8.75447374132327	38\\
8.75447374132327	39\\
8.75730100320646	39\\
8.75730100320646	40\\
9.32890039336888	40\\
9.32890039336888	41\\
9.34318561735899	41\\
9.34318561735899	42\\
9.47572041018853	42\\
9.47572041018853	43\\
9.58065760919186	43\\
9.58065760919186	44\\
9.92663393471344	44\\
9.92663393471344	45\\
10.1592351367488	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.344145880444863	0\\
1.0892885289859	0\\
1.0892885289859	1\\
1.46450842698792	1\\
1.46450842698792	2\\
1.97613102810629	2\\
1.97613102810629	3\\
2.53876017202896	3\\
2.53876017202896	4\\
2.63487985705933	4\\
2.63487985705933	5\\
2.73095295631954	5\\
2.73095295631954	6\\
2.74551989053425	6\\
2.74551989053425	7\\
3.84189484207314	7\\
3.84189484207314	8\\
3.84493161813582	8\\
3.84493161813582	9\\
3.89720668631752	9\\
3.89720668631752	10\\
4.00745765785403	10\\
4.00745765785403	11\\
4.02603872877669	11\\
4.02603872877669	12\\
4.4480343805913	12\\
4.4480343805913	13\\
4.77071257314096	13\\
4.77071257314096	14\\
5.53050554327231	14\\
5.53050554327231	15\\
5.66084165571478	15\\
5.66084165571478	16\\
5.81640772620455	16\\
5.81640772620455	17\\
6.00076776839175	17\\
6.00076776839175	18\\
6.20939029941437	18\\
6.20939029941437	19\\
6.70664955832568	19\\
6.70664955832568	20\\
6.72441847026748	20\\
6.72441847026748	21\\
7.02265908613326	21\\
7.02265908613326	22\\
7.2208224433778	22\\
7.2208224433778	23\\
7.22600687995722	23\\
7.22600687995722	24\\
7.53831996349596	24\\
7.53831996349596	25\\
7.76255062265259	25\\
7.76255062265259	26\\
7.782213999702	26\\
7.782213999702	27\\
7.85432239110766	27\\
7.85432239110766	28\\
8.1758802009459	28\\
8.1758802009459	29\\
8.50823402332078	29\\
8.50823402332078	30\\
8.67302526320548	30\\
8.67302526320548	31\\
8.80081604001529	31\\
8.80081604001529	32\\
9.20487204702189	32\\
9.20487204702189	33\\
9.25970966737096	33\\
9.25970966737096	34\\
9.57515767141777	34\\
9.57515767141777	35\\
9.6860592781659	35\\
9.6860592781659	36\\
9.72630357959749	36\\
9.72630357959749	37\\
9.84380412309475	37\\
9.84380412309475	38\\
9.88087465874694	38\\
9.88087465874694	39\\
9.93076992093694	39\\
9.93076992093694	40\\
10.1677611760543	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.208477313076394	0\\
0.343200600311022	0\\
0.343200600311022	1\\
0.534912777159839	1\\
0.534912777159839	2\\
0.866180225661331	2\\
0.866180225661331	3\\
0.995885190959505	3\\
0.995885190959505	4\\
1.05861584209093	4\\
1.05861584209093	5\\
1.57470341478608	5\\
1.57470341478608	6\\
1.69265786273172	6\\
1.69265786273172	7\\
1.70781930067557	7\\
1.70781930067557	8\\
2.23655101479404	8\\
2.23655101479404	9\\
2.26999826312732	9\\
2.26999826312732	10\\
2.8094180231579	10\\
2.8094180231579	11\\
3.13217522602816	11\\
3.13217522602816	12\\
3.19011268631028	12\\
3.19011268631028	13\\
3.23627949051792	13\\
3.23627949051792	14\\
3.23878801697273	14\\
3.23878801697273	15\\
3.38325094777861	15\\
3.38325094777861	16\\
3.99628688003232	16\\
3.99628688003232	17\\
4.06474907859307	17\\
4.06474907859307	18\\
4.25134574882396	18\\
4.25134574882396	19\\
4.45978520040376	19\\
4.45978520040376	20\\
4.73171825142197	20\\
4.73171825142197	21\\
5.04171251821172	21\\
5.04171251821172	22\\
5.09949572178064	22\\
5.09949572178064	23\\
5.39577215850144	23\\
5.39577215850144	24\\
5.66541743492323	24\\
5.66541743492323	25\\
5.91011927411004	25\\
5.91011927411004	26\\
6.03263844937339	26\\
6.03263844937339	27\\
6.47377606369626	27\\
6.47377606369626	28\\
6.86150236113785	28\\
6.86150236113785	29\\
6.94938205087262	29\\
6.94938205087262	30\\
6.99540719126648	30\\
6.99540719126648	31\\
7.06908050780381	31\\
7.06908050780381	32\\
7.29577306196083	32\\
7.29577306196083	33\\
7.53956983433535	33\\
7.53956983433535	34\\
8.22621636446936	34\\
8.22621636446936	35\\
8.68055369193659	35\\
8.68055369193659	36\\
8.98356301603584	36\\
8.98356301603584	37\\
9.43948214954236	37\\
9.43948214954236	38\\
9.52724315599077	38\\
9.52724315599077	39\\
9.9845182708675	39\\
9.9845182708675	40\\
10.0847267690279	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.456893150541561	0\\
0.475970979446288	0\\
0.475970979446288	1\\
0.835140277567447	1\\
0.835140277567447	2\\
0.837763290169384	2\\
0.837763290169384	3\\
0.926662493738441	3\\
0.926662493738441	4\\
0.969046742829157	4\\
0.969046742829157	5\\
1.20539583604283	5\\
1.20539583604283	6\\
1.68377857172592	6\\
1.68377857172592	7\\
1.71791170673517	7\\
1.71791170673517	8\\
1.78035956664667	8\\
1.78035956664667	9\\
2.16419859776845	9\\
2.16419859776845	10\\
2.21155998428154	10\\
2.21155998428154	11\\
2.30359738443375	11\\
2.30359738443375	12\\
2.43691033364114	12\\
2.43691033364114	13\\
2.88774485473959	13\\
2.88774485473959	14\\
2.92391552271085	14\\
2.92391552271085	15\\
3.1680915640918	15\\
3.1680915640918	16\\
3.27192841995735	16\\
3.27192841995735	17\\
3.27590286537045	17\\
3.27590286537045	18\\
3.9755582938426	18\\
3.9755582938426	19\\
4.18410759937411	19\\
4.18410759937411	20\\
4.19396595829849	20\\
4.19396595829849	21\\
4.5272711849582	21\\
4.5272711849582	22\\
4.82424021420511	22\\
4.82424021420511	23\\
5.06812024656739	23\\
5.06812024656739	24\\
5.50323340756173	24\\
5.50323340756173	25\\
6.01330618536307	25\\
6.01330618536307	26\\
6.08796571498874	26\\
6.08796571498874	27\\
7.15174462650307	27\\
7.15174462650307	28\\
7.25735495830065	28\\
7.25735495830065	29\\
7.49443256253181	29\\
7.49443256253181	30\\
7.50617838412492	30\\
7.50617838412492	31\\
7.56665616735646	31\\
7.56665616735646	32\\
7.7582323324995	32\\
7.7582323324995	33\\
7.90999009149446	33\\
7.90999009149446	34\\
8.07721690816585	34\\
8.07721690816585	35\\
8.37716636523304	35\\
8.37716636523304	36\\
8.51092113890743	36\\
8.51092113890743	37\\
9.10916433347091	37\\
9.10916433347091	38\\
9.72694862454751	38\\
9.72694862454751	39\\
9.95210121865754	39\\
9.95210121865754	40\\
10.2483762573738	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
1.03718713187889	0\\
1.30378796438387	0\\
1.30378796438387	1\\
1.63797507225137	1\\
1.63797507225137	2\\
1.77195135980843	2\\
1.77195135980843	3\\
1.80327345998484	3\\
1.80327345998484	4\\
1.91183639544881	4\\
1.91183639544881	5\\
2.07687554628946	5\\
2.07687554628946	6\\
2.0806483040329	6\\
2.0806483040329	7\\
2.18051588977613	7\\
2.18051588977613	8\\
2.47997991445759	8\\
2.47997991445759	9\\
2.98562007203626	9\\
2.98562007203626	10\\
3.05721443615855	10\\
3.05721443615855	11\\
3.32538490952525	11\\
3.32538490952525	12\\
3.79029523301901	12\\
3.79029523301901	13\\
3.92740643617423	13\\
3.92740643617423	14\\
4.07430340890165	14\\
4.07430340890165	15\\
4.32401440192747	15\\
4.32401440192747	16\\
4.45504183783425	16\\
4.45504183783425	17\\
5.01842423379297	17\\
5.01842423379297	18\\
5.05404043542254	18\\
5.05404043542254	19\\
5.56955354601064	19\\
5.56955354601064	20\\
5.61577124203709	20\\
5.61577124203709	21\\
6.06092239346719	21\\
6.06092239346719	22\\
6.12515065047222	22\\
6.12515065047222	23\\
6.24313089579825	23\\
6.24313089579825	24\\
6.35765411478096	24\\
6.35765411478096	25\\
6.44988477197178	25\\
6.44988477197178	26\\
6.50274710929281	26\\
6.50274710929281	27\\
6.65989545250508	27\\
6.65989545250508	28\\
6.68701937394641	28\\
6.68701937394641	29\\
6.82597352719899	29\\
6.82597352719899	30\\
7.07548534389205	30\\
7.07548534389205	31\\
7.2864063631894	31\\
7.2864063631894	32\\
8.01688392079992	32\\
8.01688392079992	33\\
8.25270227516221	33\\
8.25270227516221	34\\
8.55639758687494	34\\
8.55639758687494	35\\
8.59166698655762	35\\
8.59166698655762	36\\
8.82835615557691	36\\
8.82835615557691	37\\
8.84409087776326	37\\
8.84409087776326	38\\
9.34562701112514	38\\
9.34562701112514	39\\
9.39034043306326	39\\
9.39034043306326	40\\
9.59179001462228	40\\
9.59179001462228	41\\
9.73968244915048	41\\
9.73968244915048	42\\
9.82324193613873	42\\
9.82324193613873	43\\
10.1844452556427	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0788779540326701	0\\
0.320693502823268	0\\
0.320693502823268	1\\
0.453626025476289	1\\
0.453626025476289	2\\
0.529679422456297	2\\
0.529679422456297	3\\
0.650628216263677	3\\
0.650628216263677	4\\
0.933048187472508	4\\
0.933048187472508	5\\
0.933457462455316	6\\
1.12647459347161	6\\
1.12647459347161	7\\
1.34036412441725	7\\
1.34036412441725	8\\
1.65970162659345	8\\
1.65970162659345	9\\
1.74792793353168	9\\
1.74792793353168	10\\
1.85527683809291	10\\
1.85527683809291	11\\
2.07631125181612	11\\
2.07631125181612	12\\
2.24378140108603	12\\
2.24378140108603	13\\
2.27809934823136	13\\
2.27809934823136	14\\
2.47386052501884	14\\
2.47386052501884	15\\
2.52220005889367	15\\
2.52220005889367	16\\
2.59835618388423	16\\
2.59835618388423	17\\
3.09174825871542	17\\
3.09174825871542	18\\
3.20001948794517	18\\
3.20001948794517	19\\
3.56152424349557	19\\
3.56152424349557	20\\
3.68786389052259	20\\
3.68786389052259	21\\
3.74454084541205	21\\
3.74454084541205	22\\
3.81479278726639	22\\
3.81479278726639	23\\
3.84110568862135	23\\
3.84110568862135	24\\
3.88431982942859	24\\
3.88431982942859	25\\
4.1953014567834	25\\
4.1953014567834	26\\
4.45409813399404	26\\
4.45409813399404	27\\
4.59690883498691	27\\
4.59690883498691	28\\
5.06456446216073	28\\
5.06456446216073	29\\
5.08156375594312	29\\
5.08156375594312	30\\
5.24414573028362	30\\
5.24414573028362	31\\
5.31320204007503	31\\
5.31320204007503	32\\
5.6192120000369	32\\
5.6192120000369	33\\
5.65467418107666	33\\
5.65467418107666	34\\
5.73091386177653	34\\
5.73091386177653	35\\
5.76946134654649	35\\
5.76946134654649	36\\
5.78207854142948	36\\
5.78207854142948	37\\
5.84255700449285	37\\
5.84255700449285	38\\
6.00952150054518	38\\
6.00952150054518	39\\
6.11449335180138	39\\
6.11449335180138	40\\
6.12268531813567	40\\
6.12268531813567	41\\
6.1326562818888	41\\
6.1326562818888	42\\
6.28652971319805	42\\
6.28652971319805	43\\
6.35847983234868	43\\
6.35847983234868	44\\
6.36904611307969	44\\
6.36904611307969	45\\
6.37625572872251	45\\
6.37625572872251	46\\
6.42303493576733	46\\
6.42303493576733	47\\
6.48467970902177	47\\
6.48467970902177	48\\
6.96990844017419	48\\
6.96990844017419	49\\
7.22064436827979	49\\
7.22064436827979	50\\
7.43340586815891	50\\
7.43340586815891	51\\
8.05818759281539	51\\
8.05818759281539	52\\
8.37306385171607	52\\
8.37306385171607	53\\
8.48587942690818	53\\
8.48587942690818	54\\
8.85331467030223	54\\
8.85331467030223	55\\
9.50261059414091	55\\
9.50261059414091	56\\
9.52213430331575	56\\
9.52213430331575	57\\
9.60050646846486	57\\
9.60050646846486	58\\
10.1845751127041	58\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.297475249746824	0\\
0.3110371678492	0\\
0.3110371678492	1\\
0.43011684646789	1\\
0.43011684646789	2\\
0.613092869358255	2\\
0.613092869358255	3\\
0.740056775479324	3\\
0.740056775479324	4\\
1.08884076242846	4\\
1.08884076242846	5\\
1.27982513945462	5\\
1.27982513945462	6\\
1.34979860011619	6\\
1.34979860011619	7\\
1.86784318762578	7\\
1.86784318762578	8\\
1.88396532440084	8\\
1.88396532440084	9\\
2.16927431413023	9\\
2.16927431413023	10\\
2.5069294610439	10\\
2.5069294610439	11\\
2.62875904541572	11\\
2.62875904541572	12\\
2.83891082315725	12\\
2.83891082315725	13\\
3.22495653372391	13\\
3.22495653372391	14\\
3.29943567514295	14\\
3.29943567514295	15\\
3.4901991906118	15\\
3.4901991906118	16\\
4.50304422879479	16\\
4.50304422879479	17\\
4.59881577920447	17\\
4.59881577920447	18\\
4.69486588431771	18\\
4.69486588431771	19\\
4.74115803852545	19\\
4.74115803852545	20\\
5.01493268903843	20\\
5.01493268903843	21\\
5.41029290226689	21\\
5.41029290226689	22\\
5.4788458310478	22\\
5.4788458310478	23\\
5.68397923287088	23\\
5.68397923287088	24\\
6.10874961469814	24\\
6.10874961469814	25\\
6.29901747683972	25\\
6.29901747683972	26\\
6.94884579894056	26\\
6.94884579894056	27\\
7.24686912269537	27\\
7.24686912269537	28\\
7.98925159965934	28\\
7.98925159965934	29\\
8.25988723005364	29\\
8.25988723005364	30\\
8.29209324458268	30\\
8.29209324458268	31\\
8.5377702813183	31\\
8.5377702813183	32\\
8.59810213529055	32\\
8.59810213529055	33\\
8.98370602693568	33\\
8.98370602693568	34\\
9.29425128400828	34\\
9.29425128400828	35\\
9.42444684628603	35\\
9.42444684628603	36\\
9.62551224556123	36\\
9.62551224556123	37\\
9.98162303526819	37\\
9.98162303526819	38\\
10.1384800724751	38\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.330331390983211	0\\
0.509252586136085	0\\
0.509252586136085	1\\
0.739542539994517	1\\
0.739542539994517	2\\
0.976307550954481	2\\
0.976307550954481	3\\
1.38978313182502	3\\
1.38978313182502	4\\
1.54420463583926	4\\
1.54420463583926	5\\
1.60870813870105	5\\
1.60870813870105	6\\
1.69840705856821	6\\
1.69840705856821	7\\
2.39000813409874	7\\
2.39000813409874	8\\
3.20143758634936	8\\
3.20143758634936	9\\
3.26165553365485	9\\
3.26165553365485	10\\
3.26520062594972	10\\
3.26520062594972	11\\
3.65746813341834	11\\
3.65746813341834	12\\
3.94096511429809	12\\
3.94096511429809	13\\
4.13281089414241	13\\
4.13281089414241	14\\
4.3053841545121	14\\
4.3053841545121	15\\
4.63279329115256	15\\
4.63279329115256	16\\
5.44783205919829	16\\
5.44783205919829	17\\
6.47546841381212	17\\
6.47546841381212	18\\
6.58927588690445	18\\
6.58927588690445	19\\
6.95293199354762	19\\
6.95293199354762	20\\
6.95632634166611	20\\
6.95632634166611	21\\
7.06409233480516	21\\
7.06409233480516	22\\
7.17470553882185	22\\
7.17470553882185	23\\
7.30382272119214	23\\
7.30382272119214	24\\
7.35462505788103	24\\
7.35462505788103	25\\
7.38393642560789	25\\
7.38393642560789	26\\
7.88936405300554	26\\
7.88936405300554	27\\
8.14729045204121	27\\
8.14729045204121	28\\
8.28112181442815	28\\
8.28112181442815	29\\
8.38565096507256	29\\
8.38565096507256	30\\
8.78002346361548	30\\
8.78002346361548	31\\
9.0962330823525	31\\
9.0962330823525	32\\
9.29830211650663	32\\
9.29830211650663	33\\
9.95884115235395	33\\
9.95884115235395	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.215572966844803	0\\
0.255338861145546	0\\
0.255338861145546	1\\
0.550069188573524	1\\
0.550069188573524	2\\
0.566922520842951	2\\
0.566922520842951	3\\
0.577952168102804	3\\
0.577952168102804	4\\
0.727054450697075	4\\
0.727054450697075	5\\
0.818152630080505	5\\
0.818152630080505	6\\
0.93839766110321	6\\
0.93839766110321	7\\
0.969241930250497	7\\
0.969241930250497	8\\
1.10680495970384	8\\
1.10680495970384	9\\
1.31342838943307	9\\
1.31342838943307	10\\
1.77790364265842	10\\
1.77790364265842	11\\
2.06178228078942	11\\
2.06178228078942	12\\
2.12791535358413	12\\
2.12791535358413	13\\
2.34539881163746	13\\
2.34539881163746	14\\
2.46359039083037	14\\
2.46359039083037	15\\
2.57639404692123	15\\
2.57639404692123	16\\
2.61230612468822	16\\
2.61230612468822	17\\
2.86170761432383	17\\
2.86170761432383	18\\
3.14277746200044	18\\
3.14277746200044	19\\
3.15953856081889	19\\
3.15953856081889	20\\
3.21178735516607	20\\
3.21178735516607	21\\
3.2866464569063	21\\
3.2866464569063	22\\
3.40198766827121	22\\
3.40198766827121	23\\
3.5563265970377	23\\
3.5563265970377	24\\
3.64283762347993	24\\
3.64283762347993	25\\
3.67130863904923	25\\
3.67130863904923	26\\
3.6943399220539	26\\
3.6943399220539	27\\
3.69894751281262	27\\
3.69894751281262	28\\
4.24715213637617	28\\
4.24715213637617	29\\
4.29403804558002	29\\
4.29403804558002	30\\
4.59826445033332	30\\
4.59826445033332	31\\
5.04262519120661	31\\
5.04262519120661	32\\
5.13659256726211	32\\
5.13659256726211	33\\
5.19464106451571	33\\
5.19464106451571	34\\
5.55818512774591	34\\
5.55818512774591	35\\
5.68852498038314	35\\
5.68852498038314	36\\
5.81672289759422	36\\
5.81672289759422	37\\
6.15635921442526	37\\
6.15635921442526	38\\
6.31562777403384	38\\
6.31562777403384	39\\
6.37302842831303	39\\
6.37302842831303	40\\
6.98062032771362	40\\
6.98062032771362	41\\
7.65475592362841	41\\
7.65475592362841	42\\
8.40863635415221	42\\
8.40863635415221	43\\
8.86093765205473	43\\
8.86093765205473	44\\
9.092737756586	44\\
9.092737756586	45\\
9.45494327238327	45\\
9.45494327238327	46\\
10.0051500539724	46\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.205019139573906	0\\
0.233591070333475	0\\
0.233591070333475	1\\
0.736302981122755	1\\
0.736302981122755	2\\
0.852490390448452	2\\
0.852490390448452	3\\
0.870412059260588	3\\
0.870412059260588	4\\
1.02858430842185	4\\
1.02858430842185	5\\
1.25206369589502	5\\
1.25206369589502	6\\
1.35887542740544	6\\
1.35887542740544	7\\
2.11178793269104	7\\
2.11178793269104	8\\
2.63957591784115	8\\
2.63957591784115	9\\
2.71263288776904	9\\
2.71263288776904	10\\
2.91132081067222	10\\
2.91132081067222	11\\
2.97808389994739	11\\
2.97808389994739	12\\
3.02475919340927	12\\
3.02475919340927	13\\
3.40943044745934	13\\
3.40943044745934	14\\
3.50332557993453	14\\
3.50332557993453	15\\
3.64077302420448	15\\
3.64077302420448	16\\
3.65910895352999	16\\
3.65910895352999	17\\
3.96587156928007	17\\
3.96587156928007	18\\
4.53629411524788	18\\
4.53629411524788	19\\
4.77471782087269	19\\
4.77471782087269	20\\
5.07135927958495	20\\
5.07135927958495	21\\
5.32088145186646	21\\
5.32088145186646	22\\
5.51621479718744	22\\
5.51621479718744	23\\
6.08220552603312	23\\
6.08220552603312	24\\
6.19239186389749	24\\
6.19239186389749	25\\
6.38725097974458	25\\
6.38725097974458	26\\
6.95220911372118	26\\
6.95220911372118	27\\
7.55572684109485	27\\
7.55572684109485	28\\
7.65353419864373	28\\
7.65353419864373	29\\
8.27369593947183	29\\
8.27369593947183	30\\
8.27530718220562	31\\
8.68692197042269	31\\
8.68692197042269	32\\
8.85065389798089	32\\
8.85065389798089	33\\
9.04992088241507	33\\
9.04992088241507	34\\
9.23849411569199	34\\
9.23849411569199	35\\
9.27718428083928	35\\
9.27718428083928	36\\
9.3051840189325	36\\
9.3051840189325	37\\
9.31923595458869	37\\
9.31923595458869	38\\
9.96939132187907	38\\
9.96939132187907	39\\
10.0312936542715	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0579691450273359	0\\
0.0870318540538335	0\\
0.0870318540538335	1\\
0.155516648732238	1\\
0.155516648732238	2\\
1.30792600385961	2\\
1.30792600385961	3\\
1.74510578986678	3\\
1.74510578986678	4\\
1.97924614962412	4\\
1.97924614962412	5\\
2.23830036845629	5\\
2.23830036845629	6\\
2.80067150649548	6\\
2.80067150649548	7\\
3.49516994760062	7\\
3.49516994760062	8\\
3.65007632979604	8\\
3.65007632979604	9\\
3.85322905139427	9\\
3.85322905139427	10\\
4.01097878906694	10\\
4.01097878906694	11\\
4.34657061115865	11\\
4.34657061115865	12\\
4.44565427709404	12\\
4.44565427709404	13\\
4.45089395852835	13\\
4.45089395852835	14\\
4.46742208430992	14\\
4.46742208430992	15\\
4.81973066929254	15\\
4.81973066929254	16\\
5.11198670028429	16\\
5.11198670028429	17\\
5.29171350865017	17\\
5.29171350865017	18\\
5.43627300126854	18\\
5.43627300126854	19\\
5.49529912410708	19\\
5.49529912410708	20\\
5.55379448641455	20\\
5.55379448641455	21\\
5.7274973277918	21\\
5.7274973277918	22\\
5.75300116586	22\\
5.75300116586	23\\
6.09560482212953	23\\
6.09560482212953	24\\
6.34716710586449	24\\
6.34716710586449	25\\
6.76894479712206	25\\
6.76894479712206	26\\
7.23648840325856	26\\
7.23648840325856	27\\
7.74972705804182	27\\
7.74972705804182	28\\
7.77718189539105	28\\
7.77718189539105	29\\
8.12866816048304	29\\
8.12866816048304	30\\
8.25381298466682	30\\
8.25381298466682	31\\
8.44002085752922	31\\
8.44002085752922	32\\
8.6520612443859	32\\
8.6520612443859	33\\
8.81828120727904	33\\
8.81828120727904	34\\
9.03953573069232	34\\
9.03953573069232	35\\
9.12385775165928	35\\
9.12385775165928	36\\
9.173078093717	36\\
9.173078093717	37\\
9.27886484845196	37\\
9.27886484845196	38\\
10.5181364924155	38\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.490443118450926	0\\
1.00597614067259	0\\
1.00597614067259	1\\
1.05903846690718	1\\
1.05903846690718	2\\
1.55157464564933	2\\
1.55157464564933	3\\
1.75882890918795	3\\
1.75882890918795	4\\
1.95082761212123	4\\
1.95082761212123	5\\
1.97000046596792	5\\
1.97000046596792	6\\
1.99820624571242	6\\
1.99820624571242	7\\
2.35235590378414	7\\
2.35235590378414	8\\
2.68747352960519	8\\
2.68747352960519	9\\
2.76782249426248	9\\
2.76782249426248	10\\
3.63484335748613	10\\
3.63484335748613	11\\
3.83957233129977	11\\
3.83957233129977	12\\
4.16810421611441	12\\
4.16810421611441	13\\
4.24280669121246	13\\
4.24280669121246	14\\
4.47724538416378	14\\
4.47724538416378	15\\
5.09883151351152	15\\
5.09883151351152	16\\
5.31002191422709	16\\
5.31002191422709	17\\
5.31716390788137	17\\
5.31716390788137	18\\
5.32871312166004	18\\
5.32871312166004	19\\
5.41282121562643	19\\
5.41282121562643	20\\
5.44101085498411	20\\
5.44101085498411	21\\
5.5201277933462	21\\
5.5201277933462	22\\
5.55716180770582	22\\
5.55716180770582	23\\
5.97789263204176	23\\
5.97789263204176	24\\
6.65457061581981	24\\
6.65457061581981	25\\
6.82177941512839	25\\
6.82177941512839	26\\
7.20806087729825	26\\
7.20806087729825	27\\
7.69005081779633	27\\
7.69005081779633	28\\
7.94815058304157	28\\
7.94815058304157	29\\
7.98075764318082	29\\
7.98075764318082	30\\
8.19592538999309	30\\
8.19592538999309	31\\
8.45511853925241	31\\
8.45511853925241	32\\
8.65949272999404	32\\
8.65949272999404	33\\
9.53147639264517	33\\
9.53147639264517	34\\
9.98333112435379	34\\
9.98333112435379	35\\
10.2504905636471	35\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0426985377636342	0\\
0.0982812088092473	0\\
0.0982812088092473	1\\
0.298835315664221	1\\
0.298835315664221	2\\
0.334226385255967	2\\
0.334226385255967	3\\
0.564499433051672	3\\
0.564499433051672	4\\
1.02577798316629	4\\
1.02577798316629	5\\
1.21321197695234	5\\
1.21321197695234	6\\
1.41632193076167	6\\
1.41632193076167	7\\
1.54062136018435	7\\
1.54062136018435	8\\
1.55158353762514	8\\
1.55158353762514	9\\
2.0999222865698	9\\
2.0999222865698	10\\
2.20450213369314	10\\
2.20450213369314	11\\
2.32176003436626	11\\
2.32176003436626	12\\
2.36327807369176	12\\
2.36327807369176	13\\
2.80725267836739	13\\
2.80725267836739	14\\
2.93830184132764	14\\
2.93830184132764	15\\
3.31940781528219	15\\
3.31940781528219	16\\
3.7717268286274	16\\
3.7717268286274	17\\
3.93820868366191	17\\
3.93820868366191	18\\
3.98988378650002	18\\
3.98988378650002	19\\
4.06013461754323	19\\
4.06013461754323	20\\
4.06832990303329	20\\
4.06832990303329	21\\
4.22890496182214	21\\
4.22890496182214	22\\
4.41675447053291	22\\
4.41675447053291	23\\
4.7490622760614	23\\
4.7490622760614	24\\
4.83732281319096	24\\
4.83732281319096	25\\
5.42403909227632	25\\
5.42403909227632	26\\
5.55183489591468	26\\
5.55183489591468	27\\
5.62852708501175	27\\
5.62852708501175	28\\
5.83225959354703	28\\
5.83225959354703	29\\
6.21407796206273	29\\
6.21407796206273	30\\
6.30014796105652	30\\
6.30014796105652	31\\
6.84090344834905	31\\
6.84090344834905	32\\
7.18760441919687	32\\
7.18760441919687	33\\
7.24585019712695	33\\
7.24585019712695	34\\
7.24861953072661	34\\
7.24861953072661	35\\
7.35447531696997	35\\
7.35447531696997	36\\
7.54586581085808	36\\
7.54586581085808	37\\
7.68707860554018	37\\
7.68707860554018	38\\
7.89514020135292	38\\
7.89514020135292	39\\
7.89781524415817	39\\
7.89781524415817	40\\
8.22133525191494	40\\
8.22133525191494	41\\
8.81500060526846	41\\
8.81500060526846	42\\
8.96711981088548	42\\
8.96711981088548	43\\
8.99920681014835	43\\
8.99920681014835	44\\
9.02042322313105	44\\
9.02042322313105	45\\
9.6276230127848	45\\
9.6276230127848	46\\
9.68247728717473	46\\
9.68247728717473	47\\
10.2201269456819	47\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.114444880228639	0\\
0.898770394879193	0\\
0.898770394879193	1\\
0.903376803938322	1\\
0.903376803938322	2\\
0.947937808311536	2\\
0.947937808311536	3\\
1.01349730559068	3\\
1.01349730559068	4\\
1.03927299407676	4\\
1.03927299407676	5\\
1.57795778430472	5\\
1.57795778430472	6\\
1.66401468843158	6\\
1.66401468843158	7\\
1.66877475480477	7\\
1.66877475480477	8\\
1.74799931751838	8\\
1.74799931751838	9\\
2.00174519954761	9\\
2.00174519954761	10\\
2.30162890857549	10\\
2.30162890857549	11\\
2.36460464021301	11\\
2.36460464021301	12\\
2.68459194990737	12\\
2.68459194990737	13\\
3.58480729373242	13\\
3.58480729373242	14\\
3.63152640551094	14\\
3.63152640551094	15\\
3.70093158216115	15\\
3.70093158216115	16\\
3.81759702420554	16\\
3.81759702420554	17\\
4.44861362058847	17\\
4.44861362058847	18\\
4.48795794009062	18\\
4.48795794009062	19\\
5.06669801275751	19\\
5.06669801275751	20\\
5.68505696013779	20\\
5.68505696013779	21\\
5.8548242136605	21\\
5.8548242136605	22\\
5.90315785287132	22\\
5.90315785287132	23\\
6.13058808112275	23\\
6.13058808112275	24\\
6.49142283013546	24\\
6.49142283013546	25\\
6.5152971456046	25\\
6.5152971456046	26\\
6.87990031445233	26\\
6.87990031445233	27\\
7.23485729788762	27\\
7.23485729788762	28\\
7.23719724862167	28\\
7.23719724862167	29\\
7.46840891189697	29\\
7.46840891189697	30\\
7.69826905297596	30\\
7.69826905297596	31\\
7.74793745945202	31\\
7.74793745945202	32\\
7.90620640755114	32\\
7.90620640755114	33\\
7.90801003006176	34\\
8.39745568561963	34\\
8.39745568561963	35\\
9.05066801216785	35\\
9.05066801216785	36\\
9.18535639631771	36\\
9.18535639631771	37\\
9.24061585279928	37\\
9.24061585279928	38\\
9.33199381842837	38\\
9.33199381842837	39\\
10.1230279956374	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.451660278869412	0\\
0.977131326721882	0\\
0.977131326721882	1\\
1.13074020872848	1\\
1.13074020872848	2\\
1.31829868339994	2\\
1.31829868339994	3\\
1.7530069134776	3\\
1.7530069134776	4\\
1.81285364168355	4\\
1.81285364168355	5\\
1.95878215826469	5\\
1.95878215826469	6\\
2.28889768262033	6\\
2.28889768262033	7\\
2.43495050122801	7\\
2.43495050122801	8\\
2.75201771609442	8\\
2.75201771609442	9\\
2.99087916948182	9\\
2.99087916948182	10\\
3.13393496908675	10\\
3.13393496908675	11\\
3.34809007701595	11\\
3.34809007701595	12\\
3.6325910048572	12\\
3.6325910048572	13\\
3.72321660987522	13\\
3.72321660987522	14\\
3.77978593268465	14\\
3.77978593268465	15\\
4.19972615177247	15\\
4.19972615177247	16\\
4.23909162876301	16\\
4.23909162876301	17\\
5.13753200091985	17\\
5.13753200091985	18\\
5.38376618293521	18\\
5.38376618293521	19\\
5.56971059979777	19\\
5.56971059979777	20\\
5.59386827074354	20\\
5.59386827074354	21\\
5.67586834522533	21\\
5.67586834522533	22\\
5.97423884823976	22\\
5.97423884823976	23\\
6.05908850184073	23\\
6.05908850184073	24\\
6.34061945222589	24\\
6.34061945222589	25\\
6.89046514056736	25\\
6.89046514056736	26\\
6.98917828505224	26\\
6.98917828505224	27\\
7.04251706348462	27\\
7.04251706348462	28\\
7.04703781384691	28\\
7.04703781384691	29\\
7.70300970518434	29\\
7.70300970518434	30\\
8.20311374404103	30\\
8.20311374404103	31\\
8.5631371628937	31\\
8.5631371628937	32\\
8.61276957039068	32\\
8.61276957039068	33\\
8.76303634523853	33\\
8.76303634523853	34\\
9.0425945753404	34\\
9.0425945753404	35\\
9.09371127973789	35\\
9.09371127973789	36\\
9.15479432756198	36\\
9.15479432756198	37\\
9.31118792926519	37\\
9.31118792926519	38\\
9.37292478211924	38\\
9.37292478211924	39\\
9.70482133553559	39\\
9.70482133553559	40\\
10.1477892757467	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.225608134030026	0\\
0.518901839902682	0\\
0.518901839902682	1\\
0.545847908327573	1\\
0.545847908327573	2\\
1.25544642809854	2\\
1.25544642809854	3\\
1.31043898190003	3\\
1.31043898190003	4\\
1.50057536493946	4\\
1.50057536493946	5\\
1.59453646918079	5\\
1.59453646918079	6\\
2.15802659265206	6\\
2.15802659265206	7\\
2.85486582589208	7\\
2.85486582589208	8\\
3.48560182616578	8\\
3.48560182616578	9\\
3.7062838426621	9\\
3.7062838426621	10\\
3.76474431517473	10\\
3.76474431517473	11\\
4.05133504732363	11\\
4.05133504732363	12\\
4.57524167042511	12\\
4.57524167042511	13\\
4.63165143865227	13\\
4.63165143865227	14\\
4.86685984176057	14\\
4.86685984176057	15\\
4.94805061250495	15\\
4.94805061250495	16\\
5.16460158088854	16\\
5.16460158088854	17\\
5.56910556214123	17\\
5.56910556214123	18\\
5.59436450208315	18\\
5.59436450208315	19\\
5.78339375994971	19\\
5.78339375994971	20\\
5.83198237626766	20\\
5.83198237626766	21\\
6.39045808122439	21\\
6.39045808122439	22\\
6.82760076620506	22\\
6.82760076620506	23\\
6.83612232904643	23\\
6.83612232904643	24\\
7.16760680050675	24\\
7.16760680050675	25\\
7.18240587804308	25\\
7.18240587804308	26\\
7.34655345027801	26\\
7.34655345027801	27\\
7.46716312199434	27\\
7.46716312199434	28\\
7.54821133284356	28\\
7.54821133284356	29\\
7.69111363600461	29\\
7.69111363600461	30\\
7.83999499354874	30\\
7.83999499354874	31\\
8.03136885160727	31\\
8.03136885160727	32\\
8.24163848788023	32\\
8.24163848788023	33\\
8.59017834651257	33\\
8.59017834651257	34\\
8.91545211819751	34\\
8.91545211819751	35\\
9.13636611075131	35\\
9.13636611075131	36\\
9.96671144617537	36\\
9.96671144617537	37\\
10.3047136257304	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.309812684510639	0\\
0.376415671885972	0\\
0.376415671885972	1\\
0.497012938550732	1\\
0.497012938550732	2\\
0.814640736329096	2\\
0.814640736329096	3\\
1.04506380680817	3\\
1.04506380680817	4\\
1.41621652776325	4\\
1.41621652776325	5\\
1.57248239876389	5\\
1.57248239876389	6\\
1.64179656741548	6\\
1.64179656741548	7\\
1.69148926529569	7\\
1.69148926529569	8\\
1.84789492964971	8\\
1.84789492964971	9\\
2.57872166939702	9\\
2.57872166939702	10\\
2.61719250488326	10\\
2.61719250488326	11\\
3.09792033627088	11\\
3.09792033627088	12\\
3.30508456804101	12\\
3.30508456804101	13\\
3.35367829939074	13\\
3.35367829939074	14\\
3.41922980184624	14\\
3.41922980184624	15\\
3.46176267394069	15\\
3.46176267394069	16\\
3.81399807183849	16\\
3.81399807183849	17\\
3.85152629128923	17\\
3.85152629128923	18\\
4.30531338131439	18\\
4.30531338131439	19\\
4.41979418908038	19\\
4.41979418908038	20\\
4.45977317368229	20\\
4.45977317368229	21\\
4.80188010099378	21\\
4.80188010099378	22\\
4.81165653500126	22\\
4.81165653500126	23\\
4.95588236428007	23\\
4.95588236428007	24\\
4.9577526359924	25\\
4.99896897694988	25\\
4.99896897694988	26\\
5.04388104319028	26\\
5.04388104319028	27\\
5.08684546302749	27\\
5.08684546302749	28\\
5.15031220504177	28\\
5.15031220504177	29\\
5.35217798440378	29\\
5.35217798440378	30\\
5.55195014795469	30\\
5.55195014795469	31\\
5.67830787730917	31\\
5.67830787730917	32\\
5.75304507783384	32\\
5.75304507783384	33\\
5.88746942271865	33\\
5.88746942271865	34\\
5.91894797555367	34\\
5.91894797555367	35\\
6.23647262038612	35\\
6.23647262038612	36\\
6.31386798545502	36\\
6.31386798545502	37\\
6.56621874155101	37\\
6.56621874155101	38\\
6.70264166917375	38\\
6.70264166917375	39\\
6.79751653884448	39\\
6.79751653884448	40\\
6.903347868015	40\\
6.903347868015	41\\
6.96875585718578	41\\
6.96875585718578	42\\
7.11689842320708	42\\
7.11689842320708	43\\
8.08026685837282	43\\
8.08026685837282	44\\
8.08233377790258	45\\
8.40130291240266	45\\
8.40130291240266	46\\
8.55377050459246	46\\
8.55377050459246	47\\
9.1038213110164	47\\
9.1038213110164	48\\
9.22413429733207	48\\
9.22413429733207	49\\
9.43045535715697	49\\
9.43045535715697	50\\
9.67715282944147	50\\
9.67715282944147	51\\
9.74782788557528	51\\
9.74782788557528	52\\
10.1823695673455	52\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0310609777654349	0\\
0.443042440150741	0\\
0.443042440150741	1\\
0.470288349249699	1\\
0.470288349249699	2\\
1.04005518267738	2\\
1.04005518267738	3\\
1.13548702901232	3\\
1.13548702901232	4\\
1.40572533862121	4\\
1.40572533862121	5\\
1.41501336310257	5\\
1.41501336310257	6\\
1.66975324640549	6\\
1.66975324640549	7\\
1.67461016262858	7\\
1.67461016262858	8\\
2.25477521782984	8\\
2.25477521782984	9\\
2.77426373692651	9\\
2.77426373692651	10\\
3.56403513086503	10\\
3.56403513086503	11\\
3.58024641028945	11\\
3.58024641028945	12\\
3.59260221318069	12\\
3.59260221318069	13\\
3.70366935672416	13\\
3.70366935672416	14\\
3.71238368361963	14\\
3.71238368361963	15\\
4.0429083150859	15\\
4.0429083150859	16\\
4.11710879652939	16\\
4.11710879652939	17\\
4.1700850654257	17\\
4.1700850654257	18\\
4.42886373784442	18\\
4.42886373784442	19\\
4.92152162177867	19\\
4.92152162177867	20\\
5.49628949333846	20\\
5.49628949333846	21\\
5.49900317877444	21\\
5.49900317877444	22\\
5.80078899159	22\\
5.80078899159	23\\
5.88249182433558	23\\
5.88249182433558	24\\
5.97794636948428	24\\
5.97794636948428	25\\
6.39476933694718	25\\
6.39476933694718	26\\
6.45490653103236	26\\
6.45490653103236	27\\
6.80645209031079	27\\
6.80645209031079	28\\
6.86886113656774	28\\
6.86886113656774	29\\
7.10825224425852	29\\
7.10825224425852	30\\
7.2352526115632	30\\
7.2352526115632	31\\
7.55843923034244	31\\
7.55843923034244	32\\
7.58181315323409	32\\
7.58181315323409	33\\
7.66431078519376	33\\
7.66431078519376	34\\
7.84553747191082	34\\
7.84553747191082	35\\
8.15198343829362	35\\
8.15198343829362	36\\
8.28526708226362	36\\
8.28526708226362	37\\
8.34458534179196	37\\
8.34458534179196	38\\
8.68255787278716	38\\
8.68255787278716	39\\
9.33781557814664	39\\
9.33781557814664	40\\
9.50927631057114	40\\
9.50927631057114	41\\
9.65486208831334	41\\
9.65486208831334	42\\
9.69408339507752	42\\
9.69408339507752	43\\
10.0945210138484	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0146550316246916	0\\
0.297561235130999	0\\
0.297561235130999	1\\
0.326617283268924	1\\
0.326617283268924	2\\
0.844411133716413	2\\
0.844411133716413	3\\
0.853565104230164	3\\
0.853565104230164	4\\
0.878311760211432	4\\
0.878311760211432	5\\
2.01185022971523	5\\
2.01185022971523	6\\
2.31449582547764	6\\
2.31449582547764	7\\
2.40165388492073	7\\
2.40165388492073	8\\
2.71737521545417	8\\
2.71737521545417	9\\
2.87498400292471	9\\
2.87498400292471	10\\
2.92555931163655	10\\
2.92555931163655	11\\
3.02706228614624	11\\
3.02706228614624	12\\
3.13044065191666	12\\
3.13044065191666	13\\
3.56519785427037	13\\
3.56519785427037	14\\
3.69017962894866	14\\
3.69017962894866	15\\
4.22254042201872	15\\
4.22254042201872	16\\
4.45687810882911	16\\
4.45687810882911	17\\
4.63224731594144	17\\
4.63224731594144	18\\
4.65655832986722	18\\
4.65655832986722	19\\
4.74980092023218	19\\
4.74980092023218	20\\
4.75351501074407	20\\
4.75351501074407	21\\
4.80201851694428	21\\
4.80201851694428	22\\
4.80443938392188	22\\
4.80443938392188	23\\
4.95733909087895	23\\
4.95733909087895	24\\
5.03254444241909	24\\
5.03254444241909	25\\
5.33423579852469	25\\
5.33423579852469	26\\
5.48600928238211	26\\
5.48600928238211	27\\
5.54668473030488	27\\
5.54668473030488	28\\
5.99783650612101	28\\
5.99783650612101	29\\
6.19728799350809	29\\
6.19728799350809	30\\
6.33092115994286	30\\
6.33092115994286	31\\
6.49848033620461	31\\
6.49848033620461	32\\
6.59856987129369	32\\
6.59856987129369	33\\
7.32889169672742	33\\
7.32889169672742	34\\
8.35573337803873	34\\
8.35573337803873	35\\
8.7348651101953	35\\
8.7348651101953	36\\
9.18880513737828	36\\
9.18880513737828	37\\
9.68377143840796	37\\
9.68377143840796	38\\
9.74717138819125	38\\
9.74717138819125	39\\
9.87483997932214	39\\
9.87483997932214	40\\
10.1441603323098	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0477376789729718	0\\
0.211565313831883	0\\
0.211565313831883	1\\
0.247284496534974	1\\
0.247284496534974	2\\
0.290015880664114	2\\
0.290015880664114	3\\
0.60180689581729	3\\
0.60180689581729	4\\
0.610355922219647	4\\
0.610355922219647	5\\
0.656502926105219	5\\
0.656502926105219	6\\
1.42143064618298	6\\
1.42143064618298	7\\
1.43485151633769	7\\
1.43485151633769	8\\
1.77241716872773	8\\
1.77241716872773	9\\
1.89127316763947	9\\
1.89127316763947	10\\
1.94034990023553	10\\
1.94034990023553	11\\
1.9619919640117	11\\
1.9619919640117	12\\
3.00907139914941	12\\
3.00907139914941	13\\
3.16561782568144	13\\
3.16561782568144	14\\
3.69516231008969	14\\
3.69516231008969	15\\
3.75498420040631	15\\
3.75498420040631	16\\
4.18136283720591	16\\
4.18136283720591	17\\
4.25351742488198	17\\
4.25351742488198	18\\
4.69405769497912	18\\
4.69405769497912	19\\
4.81834220396546	19\\
4.81834220396546	20\\
4.83681008836631	20\\
4.83681008836631	21\\
5.21709874485978	21\\
5.21709874485978	22\\
5.22250093012153	22\\
5.22250093012153	23\\
5.49569702424355	23\\
5.49569702424355	24\\
5.80899855924279	24\\
5.80899855924279	25\\
6.3544810512587	25\\
6.3544810512587	26\\
6.49055900274332	26\\
6.49055900274332	27\\
6.79678413907777	27\\
6.79678413907777	28\\
6.84812314989792	28\\
6.84812314989792	29\\
6.93331849745913	29\\
6.93331849745913	30\\
7.24741858413409	30\\
7.24741858413409	31\\
7.39288359020289	31\\
7.39288359020289	32\\
7.79391761317294	32\\
7.79391761317294	33\\
7.86302656754987	33\\
7.86302656754987	34\\
7.91389855547277	34\\
7.91389855547277	35\\
7.94661821724521	35\\
7.94661821724521	36\\
8.13611758196094	36\\
8.13611758196094	37\\
8.15018281379664	37\\
8.15018281379664	38\\
8.19053935825367	38\\
8.19053935825367	39\\
8.30336217711501	39\\
8.30336217711501	40\\
8.48047991995642	40\\
8.48047991995642	41\\
8.90426538745608	41\\
8.90426538745608	42\\
10.2599483529975	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0553637272657141	0\\
0.111996947491242	0\\
0.111996947491242	1\\
0.706281886251865	1\\
0.706281886251865	2\\
0.98993368251142	2\\
0.98993368251142	3\\
1.00299359869621	3\\
1.00299359869621	4\\
1.0282867512726	4\\
1.0282867512726	5\\
1.11588607490655	5\\
1.11588607490655	6\\
1.35233003154989	6\\
1.35233003154989	7\\
1.71089143821129	7\\
1.71089143821129	8\\
1.73293657508232	8\\
1.73293657508232	9\\
1.79622195775937	9\\
1.79622195775937	10\\
2.54375482244661	10\\
2.54375482244661	11\\
2.55580541026939	11\\
2.55580541026939	12\\
2.831902764158	12\\
2.831902764158	13\\
2.8948400576376	13\\
2.8948400576376	14\\
2.90204083683969	14\\
2.90204083683969	15\\
2.92878284594349	15\\
2.92878284594349	16\\
2.99803372645717	16\\
2.99803372645717	17\\
3.33147733896151	17\\
3.33147733896151	18\\
3.60982540185282	18\\
3.60982540185282	19\\
3.8325945872045	19\\
3.8325945872045	20\\
3.9016483261349	20\\
3.9016483261349	21\\
4.05583601841038	21\\
4.05583601841038	22\\
4.15646520984212	22\\
4.15646520984212	23\\
4.17872389614917	23\\
4.17872389614917	24\\
4.27931773705194	24\\
4.27931773705194	25\\
4.50697015218869	25\\
4.50697015218869	26\\
4.83279587870571	26\\
4.83279587870571	27\\
5.08256384397738	27\\
5.08256384397738	28\\
5.09684229676676	28\\
5.09684229676676	29\\
5.24677474349656	29\\
5.24677474349656	30\\
5.37148815442588	30\\
5.37148815442588	31\\
5.3794670031552	31\\
5.3794670031552	32\\
5.64368829043963	32\\
5.64368829043963	33\\
5.77856938907055	33\\
5.77856938907055	34\\
6.10664666091785	34\\
6.10664666091785	35\\
6.16203705909535	35\\
6.16203705909535	36\\
6.39285123359485	36\\
6.39285123359485	37\\
6.66678268211383	37\\
6.66678268211383	38\\
6.74098631849891	38\\
6.74098631849891	39\\
6.94131443101003	39\\
6.94131443101003	40\\
7.04979297775925	40\\
7.04979297775925	41\\
7.24229740119811	41\\
7.24229740119811	42\\
7.51129008271646	42\\
7.51129008271646	43\\
7.62119662301119	43\\
7.62119662301119	44\\
7.62880593199776	44\\
7.62880593199776	45\\
7.63062148122593	46\\
7.91236655496323	46\\
7.91236655496323	47\\
7.95141818999059	47\\
7.95141818999059	48\\
8.01782664201285	48\\
8.01782664201285	49\\
8.48814476265743	49\\
8.48814476265743	50\\
8.70142511413277	50\\
8.70142511413277	51\\
8.74137871101468	51\\
8.74137871101468	52\\
8.98009127524142	52\\
8.98009127524142	53\\
9.13331344598215	53\\
9.13331344598215	54\\
9.22393092658491	54\\
9.22393092658491	55\\
9.84336077363698	55\\
9.84336077363698	56\\
10.0097121579008	56\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.16523504590743	0\\
0.33114453454003	0\\
0.33114453454003	1\\
0.503124835649793	1\\
0.503124835649793	2\\
0.88072984365165	2\\
0.88072984365165	3\\
0.959655221494494	3\\
0.959655221494494	4\\
1.08690034950284	4\\
1.08690034950284	5\\
1.15573172436326	5\\
1.15573172436326	6\\
1.16282525881951	6\\
1.16282525881951	7\\
1.18938978459278	7\\
1.18938978459278	8\\
1.65227679131687	8\\
1.65227679131687	9\\
1.79302472248735	9\\
1.79302472248735	10\\
1.84912061532486	10\\
1.84912061532486	11\\
2.01022070657541	11\\
2.01022070657541	12\\
2.09773572177935	12\\
2.09773572177935	13\\
2.16644526232623	13\\
2.16644526232623	14\\
2.17460009186768	14\\
2.17460009186768	15\\
2.19404798589853	15\\
2.19404798589853	16\\
2.44401801629061	16\\
2.44401801629061	17\\
3.21040066447686	17\\
3.21040066447686	18\\
3.29227299903566	18\\
3.29227299903566	19\\
3.64703162258473	19\\
3.64703162258473	20\\
3.85703089044245	20\\
3.85703089044245	21\\
4.04020750526845	21\\
4.04020750526845	22\\
4.40640784686774	22\\
4.40640784686774	23\\
4.765128772362	23\\
4.765128772362	24\\
5.11063907907025	24\\
5.11063907907025	25\\
5.14374819076577	25\\
5.14374819076577	26\\
5.62779756828002	26\\
5.62779756828002	27\\
5.84103706632689	27\\
5.84103706632689	28\\
5.94094376582234	28\\
5.94094376582234	29\\
6.46101351629265	29\\
6.46101351629265	30\\
6.90105423462172	30\\
6.90105423462172	31\\
7.47395021051371	31\\
7.47395021051371	32\\
7.49326477939867	32\\
7.49326477939867	33\\
7.50317069924695	33\\
7.50317069924695	34\\
8.35031130230898	34\\
8.35031130230898	35\\
8.52779086229405	35\\
8.52779086229405	36\\
8.54069806453608	36\\
8.54069806453608	37\\
8.60857890075926	37\\
8.60857890075926	38\\
8.94828548186713	38\\
8.94828548186713	39\\
9.22617292022013	39\\
9.22617292022013	40\\
9.26552649325172	40\\
9.26552649325172	41\\
9.28929531876666	41\\
9.28929531876666	42\\
9.41034635232513	42\\
9.41034635232513	43\\
9.56737734070483	43\\
9.56737734070483	44\\
9.66056522749457	44\\
9.66056522749457	45\\
11	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0976357384772299	0\\
0.671966658567399	0\\
0.671966658567399	1\\
1.42040016016331	1\\
1.42040016016331	2\\
1.60097512409472	2\\
1.60097512409472	3\\
2.06919630103909	3\\
2.06919630103909	4\\
2.14453709016636	4\\
2.14453709016636	5\\
2.32060458807323	5\\
2.32060458807323	6\\
2.57168228698452	6\\
2.57168228698452	7\\
3.07629660425405	7\\
3.07629660425405	8\\
3.21918035089049	8\\
3.21918035089049	9\\
3.25275942867065	9\\
3.25275942867065	10\\
3.38347321870428	10\\
3.38347321870428	11\\
3.42788223966572	11\\
3.42788223966572	12\\
3.54924413941109	12\\
3.54924413941109	13\\
3.56339499706288	13\\
3.56339499706288	14\\
3.79854151515044	14\\
3.79854151515044	15\\
4.02817424255018	15\\
4.02817424255018	16\\
4.11647949591232	16\\
4.11647949591232	17\\
4.20021055478214	17\\
4.20021055478214	18\\
4.22284632448577	18\\
4.22284632448577	19\\
4.30425572885511	19\\
4.30425572885511	20\\
4.50550933423001	20\\
4.50550933423001	21\\
4.75186821720701	21\\
4.75186821720701	22\\
5.31135687250919	22\\
5.31135687250919	23\\
5.50398737356704	23\\
5.50398737356704	24\\
5.5157666022244	24\\
5.5157666022244	25\\
5.68684548790632	25\\
5.68684548790632	26\\
6.08550059811372	26\\
6.08550059811372	27\\
6.27680799100773	27\\
6.27680799100773	28\\
6.3356282244923	28\\
6.3356282244923	29\\
6.52206258287701	29\\
6.52206258287701	30\\
7.50766761296237	30\\
7.50766761296237	31\\
7.88990967771432	31\\
7.88990967771432	32\\
8.55002472083407	32\\
8.55002472083407	33\\
8.8074018246217	33\\
8.8074018246217	34\\
8.82381221855615	34\\
8.82381221855615	35\\
9.2906142299837	35\\
9.2906142299837	36\\
9.73132065117053	36\\
9.73132065117053	37\\
9.76655911610403	37\\
9.76655911610403	38\\
9.96068557570698	38\\
9.96068557570698	39\\
9.96940695910072	39\\
9.96940695910072	40\\
10.0003147255601	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.212681633207119	0\\
0.395076765616309	0\\
0.395076765616309	1\\
0.934987617629048	1\\
0.934987617629048	2\\
0.978292301029718	2\\
0.978292301029718	3\\
1.2484811030361	3\\
1.2484811030361	4\\
1.50958318670254	4\\
1.50958318670254	5\\
1.61457383904068	5\\
1.61457383904068	6\\
1.76027471356216	6\\
1.76027471356216	7\\
1.85097746493074	7\\
1.85097746493074	8\\
1.98492149604055	8\\
1.98492149604055	9\\
2.14192496134042	9\\
2.14192496134042	10\\
2.46172139217175	10\\
2.46172139217175	11\\
2.59687155740311	11\\
2.59687155740311	12\\
2.74527964724071	12\\
2.74527964724071	13\\
2.84269403497793	13\\
2.84269403497793	14\\
2.914232735334	14\\
2.914232735334	15\\
2.93930748322348	15\\
2.93930748322348	16\\
3.05475721665962	16\\
3.05475721665962	17\\
3.06742075846753	17\\
3.06742075846753	18\\
3.26429111153636	18\\
3.26429111153636	19\\
3.31127237561746	19\\
3.31127237561746	20\\
3.42783141872313	20\\
3.42783141872313	21\\
3.83678389581602	21\\
3.83678389581602	22\\
3.90299335050722	22\\
3.90299335050722	23\\
3.93041488228734	23\\
3.93041488228734	24\\
4.0532026795567	24\\
4.0532026795567	25\\
4.31865291337768	25\\
4.31865291337768	26\\
4.34912435735342	26\\
4.34912435735342	27\\
4.86215689650092	27\\
4.86215689650092	28\\
5.25920089968854	28\\
5.25920089968854	29\\
5.87472730160617	29\\
5.87472730160617	30\\
5.90253459549343	30\\
5.90253459549343	31\\
6.47110710848068	31\\
6.47110710848068	32\\
6.79310968758666	32\\
6.79310968758666	33\\
6.80616854723579	33\\
6.80616854723579	34\\
6.99746777160064	34\\
6.99746777160064	35\\
7.1056451462008	35\\
7.1056451462008	36\\
7.1611148185047	36\\
7.1611148185047	37\\
7.1904262178633	37\\
7.1904262178633	38\\
7.2509495030246	38\\
7.2509495030246	39\\
7.76271893568367	39\\
7.76271893568367	40\\
7.89235818614917	40\\
7.89235818614917	41\\
8.32614316264772	41\\
8.32614316264772	42\\
8.55067359455638	42\\
8.55067359455638	43\\
8.81628603929624	43\\
8.81628603929624	44\\
8.8569610541148	44\\
8.8569610541148	45\\
9.00958011875745	45\\
9.00958011875745	46\\
9.34498062080925	46\\
9.34498062080925	47\\
9.48314328642562	47\\
9.48314328642562	48\\
9.85990372808022	48\\
9.85990372808022	49\\
9.87175779708672	49\\
9.87175779708672	50\\
10.22333033541	50\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.895540176291924	0\\
0.913275898609186	0\\
0.913275898609186	1\\
1.13093082697529	1\\
1.13093082697529	2\\
1.14914336253831	2\\
1.14914336253831	3\\
1.23618896855085	3\\
1.23618896855085	4\\
1.45017760562512	4\\
1.45017760562512	5\\
1.7141203743187	5\\
1.7141203743187	6\\
2.13364444080862	6\\
2.13364444080862	7\\
2.16617171252535	7\\
2.16617171252535	8\\
2.19942177481163	8\\
2.19942177481163	9\\
2.2055855834853	9\\
2.2055855834853	10\\
2.27612463620039	10\\
2.27612463620039	11\\
2.31266801707767	11\\
2.31266801707767	12\\
2.70146287956543	12\\
2.70146287956543	13\\
3.32572092869024	13\\
3.32572092869024	14\\
3.67315427778276	14\\
3.67315427778276	15\\
3.78504532775417	15\\
3.78504532775417	16\\
3.86216139114534	16\\
3.86216139114534	17\\
4.16829851666011	17\\
4.16829851666011	18\\
4.43507476512507	18\\
4.43507476512507	19\\
5.02995860006099	19\\
5.02995860006099	20\\
5.11785723524354	20\\
5.11785723524354	21\\
5.13724730341998	21\\
5.13724730341998	22\\
5.7218510674973	22\\
5.7218510674973	23\\
5.99154675766729	23\\
5.99154675766729	24\\
6.26787093989043	24\\
6.26787093989043	25\\
6.42581925525489	25\\
6.42581925525489	26\\
6.45843452503738	26\\
6.45843452503738	27\\
6.71615693848064	27\\
6.71615693848064	28\\
6.83485395115593	28\\
6.83485395115593	29\\
6.83859619047549	29\\
6.83859619047549	30\\
7.14929392540308	30\\
7.14929392540308	31\\
7.32805676419286	31\\
7.32805676419286	32\\
8.07934163746815	32\\
8.07934163746815	33\\
8.51858058051742	33\\
8.51858058051742	34\\
8.53946717795854	34\\
8.53946717795854	35\\
8.78794326013369	35\\
8.78794326013369	36\\
8.80719921318701	36\\
8.80719921318701	37\\
8.87333598023727	37\\
8.87333598023727	38\\
9.10415043272702	38\\
9.10415043272702	39\\
9.21496244288715	39\\
9.21496244288715	40\\
9.52529772302225	40\\
9.52529772302225	41\\
9.70528333100451	41\\
9.70528333100451	42\\
10.2309102545204	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0474766134665714	0\\
0.313762748536234	0\\
0.313762748536234	1\\
0.432388826088385	1\\
0.432388826088385	2\\
1.06892037370084	2\\
1.06892037370084	3\\
1.48873934460171	3\\
1.48873934460171	4\\
2.00443203567326	4\\
2.00443203567326	5\\
2.7293394450132	5\\
2.7293394450132	6\\
2.76468684662599	6\\
2.76468684662599	7\\
2.79857950876836	7\\
2.79857950876836	8\\
2.82524631519583	8\\
2.82524631519583	9\\
3.02009748099651	9\\
3.02009748099651	10\\
3.73187416765099	10\\
3.73187416765099	11\\
3.85334809527275	11\\
3.85334809527275	12\\
3.85923324587623	12\\
3.85923324587623	13\\
4.54644239398849	13\\
4.54644239398849	14\\
4.74847358710291	14\\
4.74847358710291	15\\
4.79748939378631	15\\
4.79748939378631	16\\
5.14647069890843	16\\
5.14647069890843	17\\
5.20209584695844	17\\
5.20209584695844	18\\
5.36422211231832	18\\
5.36422211231832	19\\
5.38894381120442	19\\
5.38894381120442	20\\
5.66237234330356	20\\
5.66237234330356	21\\
5.69358986789933	21\\
5.69358986789933	22\\
5.99267947345774	22\\
5.99267947345774	23\\
6.71472530584056	23\\
6.71472530584056	24\\
6.75610323942265	24\\
6.75610323942265	25\\
7.3769362526814	25\\
7.3769362526814	26\\
7.40057976840415	26\\
7.40057976840415	27\\
7.46792032281744	27\\
7.46792032281744	28\\
8.15165492327905	28\\
8.15165492327905	29\\
8.16448832668348	29\\
8.16448832668348	30\\
8.87362908034032	30\\
8.87362908034032	31\\
9.35856887673088	31\\
9.35856887673088	32\\
9.48906635187365	32\\
9.48906635187365	33\\
9.84780975291343	33\\
9.84780975291343	34\\
10.0644863565192	34\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.673232963765102	0\\
1.45772391279759	0\\
1.45772391279759	1\\
1.69336423012163	1\\
1.69336423012163	2\\
1.73669171092316	2\\
1.73669171092316	3\\
1.91097255564731	3\\
1.91097255564731	4\\
3.25450492233955	4\\
3.25450492233955	5\\
3.47291433141724	5\\
3.47291433141724	6\\
3.78052193868788	6\\
3.78052193868788	7\\
3.9299762798982	7\\
3.9299762798982	8\\
4.09090636680076	8\\
4.09090636680076	9\\
4.21344811311949	9\\
4.21344811311949	10\\
4.80690952251711	10\\
4.80690952251711	11\\
5.84795350454824	11\\
5.84795350454824	12\\
6.10429539714616	12\\
6.10429539714616	13\\
6.58465639842771	13\\
6.58465639842771	14\\
7.04331576688252	14\\
7.04331576688252	15\\
8.06107836847457	15\\
8.06107836847457	16\\
8.57885832490319	16\\
8.57885832490319	17\\
9.02736766919387	17\\
9.02736766919387	18\\
9.39858145541448	18\\
9.39858145541448	19\\
9.47412772902695	19\\
9.47412772902695	20\\
10.0702656149899	20\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.32754492991014	0\\
0.567798663598722	0\\
0.567798663598722	1\\
0.593004802576473	1\\
0.593004802576473	2\\
0.864848398788915	2\\
0.864848398788915	3\\
0.932533974013317	3\\
0.932533974013317	4\\
1.49908240386356	4\\
1.49908240386356	5\\
1.82301781158073	5\\
1.82301781158073	6\\
1.96950478445613	6\\
1.96950478445613	7\\
2.05982994901855	7\\
2.05982994901855	8\\
2.07646724997931	8\\
2.07646724997931	9\\
2.56304435384634	9\\
2.56304435384634	10\\
2.67621514343283	10\\
2.67621514343283	11\\
3.06198696229653	11\\
3.06198696229653	12\\
3.11118956928301	12\\
3.11118956928301	13\\
3.32664135044077	13\\
3.32664135044077	14\\
3.60412829606565	14\\
3.60412829606565	15\\
3.99059989473656	15\\
3.99059989473656	16\\
4.04030517590634	16\\
4.04030517590634	17\\
4.16065929817087	17\\
4.16065929817087	18\\
4.51655353426763	18\\
4.51655353426763	19\\
4.95354560798497	19\\
4.95354560798497	20\\
4.96393183133176	20\\
4.96393183133176	21\\
5.30548318117002	21\\
5.30548318117002	22\\
5.37277075648893	22\\
5.37277075648893	23\\
5.56982001143162	23\\
5.56982001143162	24\\
5.6032611199385	24\\
5.6032611199385	25\\
5.92750274203716	25\\
5.92750274203716	26\\
5.99642973957789	26\\
5.99642973957789	27\\
6.21109162634614	27\\
6.21109162634614	28\\
7.23659334255672	28\\
7.23659334255672	29\\
7.34168195686504	29\\
7.34168195686504	30\\
7.40450477282189	30\\
7.40450477282189	31\\
7.81988440034971	31\\
7.81988440034971	32\\
7.90770032074761	32\\
7.90770032074761	33\\
8.66619737678439	33\\
8.66619737678439	34\\
8.92428344083471	34\\
8.92428344083471	35\\
9.02462394604517	35\\
9.02462394604517	36\\
9.94699739321148	36\\
9.94699739321148	37\\
10.0073971849904	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.180325498589738	0\\
0.314912778617838	0\\
0.314912778617838	1\\
0.441223439314598	1\\
0.441223439314598	2\\
0.617226185733877	2\\
0.617226185733877	3\\
0.839145544666216	3\\
0.839145544666216	4\\
0.892686259657729	4\\
0.892686259657729	5\\
0.92825853482924	5\\
0.92825853482924	6\\
1.36934051383219	6\\
1.36934051383219	7\\
1.73697452951319	7\\
1.73697452951319	8\\
1.88529323323486	8\\
1.88529323323486	9\\
1.90329506710089	9\\
1.90329506710089	10\\
2.17768544359492	10\\
2.17768544359492	11\\
2.33341111322431	11\\
2.33341111322431	12\\
2.7432240609591	12\\
2.7432240609591	13\\
2.75860166437054	13\\
2.75860166437054	14\\
2.98665692769161	14\\
2.98665692769161	15\\
3.1173158939701	15\\
3.1173158939701	16\\
3.31765473826372	16\\
3.31765473826372	17\\
3.68077210467801	17\\
3.68077210467801	18\\
4.89993878129813	18\\
4.89993878129813	19\\
5.26068360723282	19\\
5.26068360723282	20\\
5.29029873923017	20\\
5.29029873923017	21\\
5.44765879988737	21\\
5.44765879988737	22\\
5.52377842366921	22\\
5.52377842366921	23\\
5.6763937406997	23\\
5.6763937406997	24\\
5.71885301334317	24\\
5.71885301334317	25\\
6.09638337011283	25\\
6.09638337011283	26\\
6.55141500489258	26\\
6.55141500489258	27\\
7.15605168738981	27\\
7.15605168738981	28\\
7.32685580546682	28\\
7.32685580546682	29\\
7.71372280326857	29\\
7.71372280326857	30\\
7.74694670515111	30\\
7.74694670515111	31\\
8.32616313983323	31\\
8.32616313983323	32\\
8.47238342057535	32\\
8.47238342057535	33\\
8.73773411661859	33\\
8.73773411661859	34\\
8.81356455191462	34\\
8.81356455191462	35\\
8.84943408841178	35\\
8.84943408841178	36\\
9.1093057074156	36\\
9.1093057074156	37\\
9.12315869410557	37\\
9.12315869410557	38\\
9.17805667805805	38\\
9.17805667805805	39\\
9.32042998308244	39\\
9.32042998308244	40\\
9.36050593143132	40\\
9.36050593143132	41\\
9.77731971628843	41\\
9.77731971628843	42\\
10.6714843318333	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.445480516166185	0\\
0.689107335315406	0\\
0.689107335315406	1\\
0.733725672797512	1\\
0.733725672797512	2\\
1.11998734392154	2\\
1.11998734392154	3\\
1.19164782068123	3\\
1.19164782068123	4\\
1.35054868665373	4\\
1.35054868665373	5\\
1.58225701647683	5\\
1.58225701647683	6\\
1.61413492682925	6\\
1.61413492682925	7\\
1.86306481749551	7\\
1.86306481749551	8\\
2.06234518222208	8\\
2.06234518222208	9\\
2.17709678816207	9\\
2.17709678816207	10\\
2.33163634210882	10\\
2.33163634210882	11\\
3.34922867554631	11\\
3.34922867554631	12\\
3.43301595818092	12\\
3.43301595818092	13\\
3.43338425045688	14\\
3.59546870725072	14\\
3.59546870725072	15\\
3.63940222279727	15\\
3.63940222279727	16\\
3.67424743109804	16\\
3.67424743109804	17\\
3.71791416936738	17\\
3.71791416936738	18\\
3.81276326401161	18\\
3.81276326401161	19\\
4.03585796723057	19\\
4.03585796723057	20\\
4.09090235100659	20\\
4.09090235100659	21\\
4.11026508802328	21\\
4.11026508802328	22\\
4.20308745742	22\\
4.20308745742	23\\
4.3194156191517	23\\
4.3194156191517	24\\
4.67556459683554	24\\
4.67556459683554	25\\
4.67897541281091	25\\
4.67897541281091	26\\
4.69705675346336	26\\
4.69705675346336	27\\
4.80494422332164	27\\
4.80494422332164	28\\
5.0085710047148	28\\
5.0085710047148	29\\
5.08927786304827	29\\
5.08927786304827	30\\
5.40193011690957	30\\
5.40193011690957	31\\
5.63887546234717	31\\
5.63887546234717	32\\
5.64411253387607	32\\
5.64411253387607	33\\
5.70422272523675	33\\
5.70422272523675	34\\
5.75924115132756	34\\
5.75924115132756	35\\
5.92158700837425	35\\
5.92158700837425	36\\
6.25410588498976	36\\
6.25410588498976	37\\
6.47831412649336	37\\
6.47831412649336	38\\
6.58037484254024	38\\
6.58037484254024	39\\
6.58970264123538	39\\
6.58970264123538	40\\
7.33891001075225	40\\
7.33891001075225	41\\
7.4264442117561	41\\
7.4264442117561	42\\
8.22982875715373	42\\
8.22982875715373	43\\
8.31894080582219	43\\
8.31894080582219	44\\
8.34894301181301	44\\
8.34894301181301	45\\
8.37136161879989	45\\
8.37136161879989	46\\
8.38362699819184	46\\
8.38362699819184	47\\
8.38409617579128	48\\
8.85468089929658	48\\
8.85468089929658	49\\
9.1145954525979	49\\
9.1145954525979	50\\
9.28629975121794	50\\
9.28629975121794	51\\
9.58276743486724	51\\
9.58276743486724	52\\
10.1672238478818	52\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.546343488845494	0\\
0.577353446349036	0\\
0.577353446349036	1\\
0.942298430899001	1\\
0.942298430899001	2\\
0.949605208705812	2\\
0.949605208705812	3\\
0.980970664973782	3\\
0.980970664973782	4\\
1.05161848438455	4\\
1.05161848438455	5\\
1.2161775114159	5\\
1.2161775114159	6\\
1.34174756610769	6\\
1.34174756610769	7\\
1.35739553076176	7\\
1.35739553076176	8\\
1.37056460722643	8\\
1.37056460722643	9\\
1.40511687898879	9\\
1.40511687898879	10\\
1.50031873247502	10\\
1.50031873247502	11\\
1.52684135350572	11\\
1.52684135350572	12\\
1.68118054582807	12\\
1.68118054582807	13\\
1.9963591996458	13\\
1.9963591996458	14\\
2.04093182361155	14\\
2.04093182361155	15\\
2.09599490755566	15\\
2.09599490755566	16\\
2.71401146926915	16\\
2.71401146926915	17\\
2.83375051651471	17\\
2.83375051651471	18\\
2.90717141819604	18\\
2.90717141819604	19\\
3.02388413255189	19\\
3.02388413255189	20\\
3.61498695286203	20\\
3.61498695286203	21\\
4.33600911592886	21\\
4.33600911592886	22\\
4.50103809551296	22\\
4.50103809551296	23\\
4.98399619450151	23\\
4.98399619450151	24\\
5.22748222379395	24\\
5.22748222379395	25\\
6.00446568927452	25\\
6.00446568927452	26\\
6.02774678994908	26\\
6.02774678994908	27\\
6.63922598422334	27\\
6.63922598422334	28\\
6.95638670774417	28\\
6.95638670774417	29\\
7.00637581514539	29\\
7.00637581514539	30\\
7.16347347688689	30\\
7.16347347688689	31\\
7.45640370005119	31\\
7.45640370005119	32\\
7.75704625245759	32\\
7.75704625245759	33\\
8.03027196916604	33\\
8.03027196916604	34\\
8.26830701798705	34\\
8.26830701798705	35\\
8.46308985466616	35\\
8.46308985466616	36\\
8.71952868613481	36\\
8.71952868613481	37\\
8.92592225282484	37\\
8.92592225282484	38\\
8.94837806391485	38\\
8.94837806391485	39\\
9.02371359167976	39\\
9.02371359167976	40\\
9.16517939009653	40\\
9.16517939009653	41\\
9.53015321182664	41\\
9.53015321182664	42\\
9.53964419829038	42\\
9.53964419829038	43\\
9.5602173089263	43\\
9.5602173089263	44\\
10.381427366799	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.092439453378276	0\\
0.116999553306471	0\\
0.116999553306471	1\\
0.248120768530214	1\\
0.248120768530214	2\\
0.285859028349989	2\\
0.285859028349989	3\\
0.36010306480668	3\\
0.36010306480668	4\\
0.458045642658355	4\\
0.458045642658355	5\\
0.458551288621564	6\\
0.995661116579278	6\\
0.995661116579278	7\\
1.3393479259295	7\\
1.3393479259295	8\\
1.6797685728231	8\\
1.6797685728231	9\\
1.70379082469198	9\\
1.70379082469198	10\\
1.71990030881444	10\\
1.71990030881444	11\\
1.88843139669806	11\\
1.88843139669806	12\\
1.9375450710302	12\\
1.9375450710302	13\\
2.06653158485057	13\\
2.06653158485057	14\\
2.19357327024318	14\\
2.19357327024318	15\\
2.3235058736307	15\\
2.3235058736307	16\\
2.36669640112995	16\\
2.36669640112995	17\\
2.4174041580204	17\\
2.4174041580204	18\\
2.44869477148608	18\\
2.44869477148608	19\\
2.46106106681744	19\\
2.46106106681744	20\\
2.50895705611557	20\\
2.50895705611557	21\\
2.79203901020488	21\\
2.79203901020488	22\\
3.38502465534727	22\\
3.38502465534727	23\\
4.01452021184528	23\\
4.01452021184528	24\\
4.06346828988089	24\\
4.06346828988089	25\\
4.12273080414865	25\\
4.12273080414865	26\\
4.3111015451772	26\\
4.3111015451772	27\\
4.49058482473691	27\\
4.49058482473691	28\\
4.70919072242869	28\\
4.70919072242869	29\\
4.94413456973719	29\\
4.94413456973719	30\\
4.99202949786113	30\\
4.99202949786113	31\\
5.02691573602085	31\\
5.02691573602085	32\\
5.50153489807077	32\\
5.50153489807077	33\\
5.67800544086836	33\\
5.67800544086836	34\\
5.81831537913497	34\\
5.81831537913497	35\\
5.92111274543072	35\\
5.92111274543072	36\\
6.05922483397824	36\\
6.05922483397824	37\\
6.37190238191076	37\\
6.37190238191076	38\\
6.79813969602098	38\\
6.79813969602098	39\\
7.41505313087331	39\\
7.41505313087331	40\\
7.42985536396774	40\\
7.42985536396774	41\\
7.59100966741951	41\\
7.59100966741951	42\\
7.65541373851838	42\\
7.65541373851838	43\\
7.88483216241294	43\\
7.88483216241294	44\\
8.0889164653894	44\\
8.0889164653894	45\\
8.13708426998289	45\\
8.13708426998289	46\\
8.40200973462072	46\\
8.40200973462072	47\\
8.40827939456352	47\\
8.40827939456352	48\\
8.58587907897067	48\\
8.58587907897067	49\\
8.59063049007607	49\\
8.59063049007607	50\\
8.73771605266526	50\\
8.73771605266526	51\\
8.74251156342542	51\\
8.74251156342542	52\\
8.89033616489831	52\\
8.89033616489831	53\\
8.98467441521278	53\\
8.98467441521278	54\\
9.20343817442906	54\\
9.20343817442906	55\\
9.24924740796286	55\\
9.24924740796286	56\\
9.33274893526134	56\\
9.33274893526134	57\\
9.56073085758914	57\\
9.56073085758914	58\\
9.57527610702319	58\\
9.57527610702319	59\\
9.58513308226705	59\\
9.58513308226705	60\\
9.84065645160793	60\\
9.84065645160793	61\\
9.95799127084464	61\\
9.95799127084464	62\\
10.1251034791321	62\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.12854102693548	0\\
0.139286778192698	0\\
0.139286778192698	1\\
0.211264403084776	1\\
0.211264403084776	2\\
0.431624463670687	2\\
0.431624463670687	3\\
0.524358563658154	3\\
0.524358563658154	4\\
0.705239862300694	4\\
0.705239862300694	5\\
0.826614216597228	5\\
0.826614216597228	6\\
0.850729857155429	6\\
0.850729857155429	7\\
1.19418436573005	7\\
1.19418436573005	8\\
1.23308608653154	8\\
1.23308608653154	9\\
1.39721784660863	9\\
1.39721784660863	10\\
1.51327576559327	10\\
1.51327576559327	11\\
1.70337113423885	11\\
1.70337113423885	12\\
1.74158353844007	12\\
1.74158353844007	13\\
2.26438351389704	13\\
2.26438351389704	14\\
2.28552723502926	14\\
2.28552723502926	15\\
2.57553883670106	15\\
2.57553883670106	16\\
2.61242157618286	16\\
2.61242157618286	17\\
2.87038721685229	17\\
2.87038721685229	18\\
3.0223055598745	18\\
3.0223055598745	19\\
3.10494499797786	19\\
3.10494499797786	20\\
3.58490455675023	20\\
3.58490455675023	21\\
3.75877479581555	21\\
3.75877479581555	22\\
3.94105040200975	22\\
3.94105040200975	23\\
4.0119607244771	23\\
4.0119607244771	24\\
4.11940500833265	24\\
4.11940500833265	25\\
4.15891619841062	25\\
4.15891619841062	26\\
4.5744690937101	26\\
4.5744690937101	27\\
4.67900447073831	27\\
4.67900447073831	28\\
5.46023448782896	28\\
5.46023448782896	29\\
5.51157897287776	29\\
5.51157897287776	30\\
5.82507719725478	30\\
5.82507719725478	31\\
5.87572100954992	31\\
5.87572100954992	32\\
5.99669425145506	32\\
5.99669425145506	33\\
6.32093058297103	33\\
6.32093058297103	34\\
6.91166730556348	34\\
6.91166730556348	35\\
7.16706783239177	35\\
7.16706783239177	36\\
7.24848593011078	36\\
7.24848593011078	37\\
7.83006686041593	37\\
7.83006686041593	38\\
7.89077773105427	38\\
7.89077773105427	39\\
8.31743807042377	39\\
8.31743807042377	40\\
8.32290756753902	40\\
8.32290756753902	41\\
8.3832244923227	41\\
8.3832244923227	42\\
8.44978531696989	42\\
8.44978531696989	43\\
8.45215773310462	43\\
8.45215773310462	44\\
8.49730541669896	44\\
8.49730541669896	45\\
8.68192869677364	45\\
8.68192869677364	46\\
8.84420508741986	46\\
8.84420508741986	47\\
9.55242210645172	47\\
9.55242210645172	48\\
9.60065677637672	48\\
9.60065677637672	49\\
9.65160935438293	49\\
9.65160935438293	50\\
9.66988988837417	50\\
9.66988988837417	51\\
10.2105396796135	51\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.624276138544062	0\\
1.13622950381428	0\\
1.13622950381428	1\\
1.45252492692468	1\\
1.45252492692468	2\\
1.48739032295597	2\\
1.48739032295597	3\\
1.77331547885114	3\\
1.77331547885114	4\\
1.77798325125762	4\\
1.77798325125762	5\\
2.10646279288932	5\\
2.10646279288932	6\\
2.29665996274141	6\\
2.29665996274141	7\\
2.64712748400116	7\\
2.64712748400116	8\\
2.76221706303802	8\\
2.76221706303802	9\\
2.89422615049752	9\\
2.89422615049752	10\\
3.87526665250383	10\\
3.87526665250383	11\\
3.890074252902	11\\
3.890074252902	12\\
3.90497004194938	12\\
3.90497004194938	13\\
3.97736245875105	13\\
3.97736245875105	14\\
4.21508615619989	14\\
4.21508615619989	15\\
4.51834902738642	15\\
4.51834902738642	16\\
4.56814151054024	16\\
4.56814151054024	17\\
4.86213214763477	17\\
4.86213214763477	18\\
5.14239060412542	18\\
5.14239060412542	19\\
5.32589518760599	19\\
5.32589518760599	20\\
5.69313233479195	20\\
5.69313233479195	21\\
5.72378306268356	21\\
5.72378306268356	22\\
5.83309857051408	22\\
5.83309857051408	23\\
5.90007695258267	23\\
5.90007695258267	24\\
6.11217761326682	24\\
6.11217761326682	25\\
6.2608113814611	25\\
6.2608113814611	26\\
6.63109148185934	26\\
6.63109148185934	27\\
6.8581600336957	27\\
6.8581600336957	28\\
6.88350337584349	28\\
6.88350337584349	29\\
7.0745800217461	29\\
7.0745800217461	30\\
7.17758072274435	30\\
7.17758072274435	31\\
7.3219766726837	31\\
7.3219766726837	32\\
7.50919542477122	32\\
7.50919542477122	33\\
7.61632876617899	33\\
7.61632876617899	34\\
7.88318895424471	34\\
7.88318895424471	35\\
8.06474003050872	35\\
8.06474003050872	36\\
8.11196727163401	36\\
8.11196727163401	37\\
8.15925571085618	37\\
8.15925571085618	38\\
8.19475682321212	38\\
8.19475682321212	39\\
8.4073932762897	39\\
8.4073932762897	40\\
8.54932753261864	40\\
8.54932753261864	41\\
8.96628717423339	41\\
8.96628717423339	42\\
9.00843988492154	42\\
9.00843988492154	43\\
9.18008848459716	43\\
9.18008848459716	44\\
9.28901723385675	44\\
9.28901723385675	45\\
9.39619727600659	45\\
9.39619727600659	46\\
9.54895240122219	46\\
9.54895240122219	47\\
9.66266098808167	47\\
9.66266098808167	48\\
9.67056671762271	48\\
9.67056671762271	49\\
10.531083531271	49\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.105493123266484	0\\
0.973331354013645	0\\
0.973331354013645	1\\
1.61248015963653	1\\
1.61248015963653	2\\
1.74013653808331	2\\
1.74013653808331	3\\
1.74564087516777	3\\
1.74564087516777	4\\
2.1015173800786	4\\
2.1015173800786	5\\
2.52780212395454	5\\
2.52780212395454	6\\
2.55632329046538	6\\
2.55632329046538	7\\
2.55721509842094	8\\
2.77886349529133	8\\
2.77886349529133	9\\
2.99366897304088	9\\
2.99366897304088	10\\
4.18065513677269	10\\
4.18065513677269	11\\
4.24450155154255	11\\
4.24450155154255	12\\
4.24681814455104	12\\
4.24681814455104	13\\
4.60238948906282	13\\
4.60238948906282	14\\
4.64808264092217	14\\
4.64808264092217	15\\
4.72439816203087	15\\
4.72439816203087	16\\
4.84368532677787	16\\
4.84368532677787	17\\
5.21079339058618	17\\
5.21079339058618	18\\
5.28205339646719	18\\
5.28205339646719	19\\
5.36583306070379	19\\
5.36583306070379	20\\
5.39890295515991	20\\
5.39890295515991	21\\
6.07683737542446	21\\
6.07683737542446	22\\
6.12431799294527	22\\
6.12431799294527	23\\
6.1665959308113	23\\
6.1665959308113	24\\
6.68190620008923	24\\
6.68190620008923	25\\
6.79330314380937	25\\
6.79330314380937	26\\
6.88394706014029	26\\
6.88394706014029	27\\
7.47988924920153	27\\
7.47988924920153	28\\
7.60225742409897	28\\
7.60225742409897	29\\
7.90419953109735	29\\
7.90419953109735	30\\
8.00082855965481	30\\
8.00082855965481	31\\
8.18750228251949	31\\
8.18750228251949	32\\
8.31500852404005	32\\
8.31500852404005	33\\
8.48790969603824	33\\
8.48790969603824	34\\
8.76944611044926	34\\
8.76944611044926	35\\
9.42956208428705	35\\
9.42956208428705	36\\
10.0259061704796	36\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.344299077933599	0\\
0.598506465519328	0\\
0.598506465519328	1\\
0.95418052511247	1\\
0.95418052511247	2\\
1.14291999662159	2\\
1.14291999662159	3\\
1.43830343813508	3\\
1.43830343813508	4\\
1.53317741362443	4\\
1.53317741362443	5\\
1.61958477807251	5\\
1.61958477807251	6\\
1.94194470544176	6\\
1.94194470544176	7\\
2.27766903023409	7\\
2.27766903023409	8\\
2.33192200591438	8\\
2.33192200591438	9\\
2.34468671283427	9\\
2.34468671283427	10\\
2.53014570938906	10\\
2.53014570938906	11\\
2.77104257538043	11\\
2.77104257538043	12\\
2.83298931571075	12\\
2.83298931571075	13\\
2.84719030518996	13\\
2.84719030518996	14\\
3.05839366660583	14\\
3.05839366660583	15\\
3.93432544978448	15\\
3.93432544978448	16\\
4.08999858571898	16\\
4.08999858571898	17\\
4.46159109558462	17\\
4.46159109558462	18\\
4.56709848529702	18\\
4.56709848529702	19\\
4.90637213503286	19\\
4.90637213503286	20\\
4.95621914518124	20\\
4.95621914518124	21\\
5.09154626310934	21\\
5.09154626310934	22\\
5.15423227941006	22\\
5.15423227941006	23\\
5.19758167887245	23\\
5.19758167887245	24\\
5.20650700399004	24\\
5.20650700399004	25\\
5.63058503389399	25\\
5.63058503389399	26\\
5.73759435501334	26\\
5.73759435501334	27\\
6.30959669431186	27\\
6.30959669431186	28\\
6.35654841256189	28\\
6.35654841256189	29\\
6.48052058109587	29\\
6.48052058109587	30\\
6.58700040144111	30\\
6.58700040144111	31\\
6.86049177280497	31\\
6.86049177280497	32\\
6.95584193522775	32\\
6.95584193522775	33\\
7.04704839126014	33\\
7.04704839126014	34\\
7.21950419115194	34\\
7.21950419115194	35\\
7.3274285627822	35\\
7.3274285627822	36\\
7.37413774599693	36\\
7.37413774599693	37\\
7.40871295137236	37\\
7.40871295137236	38\\
7.53216527632713	38\\
7.53216527632713	39\\
8.21904286724171	39\\
8.21904286724171	40\\
8.2280313749601	40\\
8.2280313749601	41\\
8.61545000863929	41\\
8.61545000863929	42\\
8.63275459569345	42\\
8.63275459569345	43\\
8.88560653145205	43\\
8.88560653145205	44\\
8.91928446906164	44\\
8.91928446906164	45\\
9.08021260065849	45\\
9.08021260065849	46\\
9.47842804248989	46\\
9.47842804248989	47\\
9.87246432874801	47\\
9.87246432874801	48\\
9.88586177661076	48\\
9.88586177661076	49\\
10.4483518573336	49\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.00880511788478344	0\\
0.55581435994376	0\\
0.55581435994376	1\\
0.699231112730196	1\\
0.699231112730196	2\\
1.53336383516976	2\\
1.53336383516976	3\\
1.56435063433651	3\\
1.56435063433651	4\\
1.66313322812014	4\\
1.66313322812014	5\\
1.89904204344221	5\\
1.89904204344221	6\\
1.90677232084829	6\\
1.90677232084829	7\\
2.02058062129947	7\\
2.02058062129947	8\\
2.40025659511784	8\\
2.40025659511784	9\\
2.45108581030513	9\\
2.45108581030513	10\\
2.5163738840242	10\\
2.5163738840242	11\\
2.57316175640661	11\\
2.57316175640661	12\\
2.59927928998834	12\\
2.59927928998834	13\\
2.82388066128107	13\\
2.82388066128107	14\\
2.9858124469045	14\\
2.9858124469045	15\\
3.08664014684312	15\\
3.08664014684312	16\\
3.1112908568311	16\\
3.1112908568311	17\\
3.66393166151785	17\\
3.66393166151785	18\\
3.80865752815205	18\\
3.80865752815205	19\\
3.83363009255812	19\\
3.83363009255812	20\\
3.8792322273972	20\\
3.8792322273972	21\\
4.04488749681371	21\\
4.04488749681371	22\\
4.30390163396346	22\\
4.30390163396346	23\\
4.49241661967575	23\\
4.49241661967575	24\\
4.74248708242028	24\\
4.74248708242028	25\\
5.99983923915664	25\\
5.99983923915664	26\\
6.12365006246685	26\\
6.12365006246685	27\\
6.15625628234006	27\\
6.15625628234006	28\\
6.54916713248327	28\\
6.54916713248327	29\\
6.92768514965088	29\\
6.92768514965088	30\\
7.08868447805064	30\\
7.08868447805064	31\\
7.38036124311608	31\\
7.38036124311608	32\\
7.65705498393277	32\\
7.65705498393277	33\\
7.97309584413831	33\\
7.97309584413831	34\\
8.46587916625126	34\\
8.46587916625126	35\\
8.84282393457534	35\\
8.84282393457534	36\\
9.04815676548295	36\\
9.04815676548295	37\\
10.103328542019	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.200087342004856	0\\
0.227671087179878	0\\
0.227671087179878	1\\
0.627765864303122	1\\
0.627765864303122	2\\
0.701958994496202	2\\
0.701958994496202	3\\
0.993513990699775	3\\
0.993513990699775	4\\
1.00936167728242	4\\
1.00936167728242	5\\
1.06735362822518	5\\
1.06735362822518	6\\
1.23952112987747	6\\
1.23952112987747	7\\
1.28990947351323	7\\
1.28990947351323	8\\
1.6749337956679	8\\
1.6749337956679	9\\
1.74591909526924	9\\
1.74591909526924	10\\
2.2610430351186	10\\
2.2610430351186	11\\
2.57310319549397	11\\
2.57310319549397	12\\
2.9637041196091	12\\
2.9637041196091	13\\
2.9977616304398	13\\
2.9977616304398	14\\
3.03462810460843	14\\
3.03462810460843	15\\
3.03476899598432	16\\
3.09623244217508	16\\
3.09623244217508	17\\
3.1109771325342	17\\
3.1109771325342	18\\
3.36969137060196	18\\
3.36969137060196	19\\
4.02584116923554	19\\
4.02584116923554	20\\
4.04908031490439	20\\
4.04908031490439	21\\
4.12969626452147	21\\
4.12969626452147	22\\
4.30404650440658	22\\
4.30404650440658	23\\
4.84594520828241	23\\
4.84594520828241	24\\
5.45084263265992	24\\
5.45084263265992	25\\
5.76230887353143	25\\
5.76230887353143	26\\
6.03679919899027	26\\
6.03679919899027	27\\
6.11421714321681	27\\
6.11421714321681	28\\
6.27584220430993	28\\
6.27584220430993	29\\
6.61950186574502	29\\
6.61950186574502	30\\
7.57009306638137	30\\
7.57009306638137	31\\
8.26616131255366	31\\
8.26616131255366	32\\
8.35379687657296	32\\
8.35379687657296	33\\
8.48606701517163	33\\
8.48606701517163	34\\
8.77300532393129	34\\
8.77300532393129	35\\
9.04758151065346	35\\
9.04758151065346	36\\
9.75110441236804	36\\
9.75110441236804	37\\
9.75224428819909	38\\
9.86314884824522	38\\
9.86314884824522	39\\
9.91308285705118	39\\
9.91308285705118	40\\
10.8089987135175	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.140326100316088	0\\
0.239621033445246	0\\
0.239621033445246	1\\
0.239677883332789	2\\
1.14480080756857	2\\
1.14480080756857	3\\
1.18900477081501	3\\
1.18900477081501	4\\
1.52323993876492	4\\
1.52323993876492	5\\
1.62342596230584	5\\
1.62342596230584	6\\
2.00782481413955	6\\
2.00782481413955	7\\
2.29896128595365	7\\
2.29896128595365	8\\
2.36442270764343	8\\
2.36442270764343	9\\
2.67047664751512	9\\
2.67047664751512	10\\
2.81002389276088	10\\
2.81002389276088	11\\
3.36403267782093	11\\
3.36403267782093	12\\
3.56866118226969	12\\
3.56866118226969	13\\
3.77019756302317	13\\
3.77019756302317	14\\
4.05021512470585	14\\
4.05021512470585	15\\
4.15918149515898	15\\
4.15918149515898	16\\
4.26730408802067	16\\
4.26730408802067	17\\
4.52844604739957	17\\
4.52844604739957	18\\
4.73893630630554	18\\
4.73893630630554	19\\
4.91114385700214	19\\
4.91114385700214	20\\
5.36009090264326	20\\
5.36009090264326	21\\
5.87067674028712	21\\
5.87067674028712	22\\
6.16509421563345	22\\
6.16509421563345	23\\
6.50163360285515	23\\
6.50163360285515	24\\
6.50689951715602	24\\
6.50689951715602	25\\
6.61562114594089	25\\
6.61562114594089	26\\
6.78328541950746	26\\
6.78328541950746	27\\
6.82143383593161	27\\
6.82143383593161	28\\
7.85102369129748	28\\
7.85102369129748	29\\
7.86886748284125	29\\
7.86886748284125	30\\
7.975793269339	30\\
7.975793269339	31\\
8.18322650174677	31\\
8.18322650174677	32\\
8.22915890104971	32\\
8.22915890104971	33\\
8.24981724348405	33\\
8.24981724348405	34\\
8.49126438685855	34\\
8.49126438685855	35\\
8.59676607381812	35\\
8.59676607381812	36\\
8.68851937070073	36\\
8.68851937070073	37\\
8.85466547239668	37\\
8.85466547239668	38\\
8.86146817386385	38\\
8.86146817386385	39\\
9.00562840338227	39\\
9.00562840338227	40\\
9.04645516825824	40\\
9.04645516825824	41\\
9.25880962813209	41\\
9.25880962813209	42\\
9.27560876354929	42\\
9.27560876354929	43\\
9.2880492614761	43\\
9.2880492614761	44\\
9.42132823220788	44\\
9.42132823220788	45\\
9.55578874963575	45\\
9.55578874963575	46\\
9.64480255513809	46\\
9.64480255513809	47\\
9.98835354657681	47\\
9.98835354657681	48\\
10.0046157582888	48\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.230685903795631	0\\
0.512710248106877	0\\
0.512710248106877	1\\
0.57045029182536	1\\
0.57045029182536	2\\
0.594284991821247	2\\
0.594284991821247	3\\
0.608182798017509	3\\
0.608182798017509	4\\
0.917044908594541	4\\
0.917044908594541	5\\
0.994285979121095	5\\
0.994285979121095	6\\
1.02974599167554	6\\
1.02974599167554	7\\
1.06623034194421	7\\
1.06623034194421	8\\
1.29748889458494	8\\
1.29748889458494	9\\
1.40610019608653	9\\
1.40610019608653	10\\
1.95325445300388	10\\
1.95325445300388	11\\
2.01384225093074	11\\
2.01384225093074	12\\
2.35952799006385	12\\
2.35952799006385	13\\
2.40483888932754	13\\
2.40483888932754	14\\
2.47776574835673	14\\
2.47776574835673	15\\
2.93515092329209	15\\
2.93515092329209	16\\
2.99654538079781	16\\
2.99654538079781	17\\
3.06977630229702	17\\
3.06977630229702	18\\
3.37923624285456	18\\
3.37923624285456	19\\
3.86210996095655	19\\
3.86210996095655	20\\
4.38411235964008	20\\
4.38411235964008	21\\
4.62798089647685	21\\
4.62798089647685	22\\
4.67334160524769	22\\
4.67334160524769	23\\
4.92501211199721	23\\
4.92501211199721	24\\
5.11904603514364	24\\
5.11904603514364	25\\
5.21916944989277	25\\
5.21916944989277	26\\
5.26543607887115	26\\
5.26543607887115	27\\
5.28834468174698	27\\
5.28834468174698	28\\
5.3145961763859	28\\
5.3145961763859	29\\
5.4159510582842	29\\
5.4159510582842	30\\
6.1803728824759	30\\
6.1803728824759	31\\
6.30561741184557	31\\
6.30561741184557	32\\
6.76229233008082	32\\
6.76229233008082	33\\
6.78500250332695	33\\
6.78500250332695	34\\
6.93206417114158	34\\
6.93206417114158	35\\
8.42609420646853	35\\
8.42609420646853	36\\
8.71200374189555	36\\
8.71200374189555	37\\
8.81987506584314	37\\
8.81987506584314	38\\
8.86757054828059	38\\
8.86757054828059	39\\
8.86913971972511	40\\
9.50080768691337	40\\
9.50080768691337	41\\
9.72696590881895	41\\
9.72696590881895	42\\
10.0529663151411	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.361942215703138	0\\
0.580985744748183	0\\
0.580985744748183	1\\
0.633336837658248	1\\
0.633336837658248	2\\
1.14872274683466	2\\
1.14872274683466	3\\
1.34467770766138	3\\
1.34467770766138	4\\
1.76725789903944	4\\
1.76725789903944	5\\
2.02301013181633	5\\
2.02301013181633	6\\
2.85074453935789	6\\
2.85074453935789	7\\
3.12928121089906	7\\
3.12928121089906	8\\
3.15912463686649	8\\
3.15912463686649	9\\
3.22116135727585	9\\
3.22116135727585	10\\
3.37692966487938	10\\
3.37692966487938	11\\
3.64722222103931	11\\
3.64722222103931	12\\
3.64901356631065	13\\
4.02510733980705	13\\
4.02510733980705	14\\
4.1350237796983	14\\
4.1350237796983	15\\
4.16158119636452	15\\
4.16158119636452	16\\
4.62941098833497	16\\
4.62941098833497	17\\
4.71173725155941	17\\
4.71173725155941	18\\
4.86835583011345	18\\
4.86835583011345	19\\
4.89831087261389	19\\
4.89831087261389	20\\
4.95442206076036	20\\
4.95442206076036	21\\
5.21986122170257	21\\
5.21986122170257	22\\
5.76912688255972	22\\
5.76912688255972	23\\
5.79858847738416	23\\
5.79858847738416	24\\
6.21229885645673	24\\
6.21229885645673	25\\
6.27593484365629	25\\
6.27593484365629	26\\
6.62357623662105	26\\
6.62357623662105	27\\
6.67297363923417	27\\
6.67297363923417	28\\
6.85699511238279	28\\
6.85699511238279	29\\
6.87177548685253	29\\
6.87177548685253	30\\
7.18475872615964	30\\
7.18475872615964	31\\
7.34340303645326	31\\
7.34340303645326	32\\
7.83924932365883	32\\
7.83924932365883	33\\
7.90539998955112	33\\
7.90539998955112	34\\
7.92999711765456	34\\
7.92999711765456	35\\
8.13328294634833	35\\
8.13328294634833	36\\
8.15546047544075	36\\
8.15546047544075	37\\
8.2426200294015	37\\
8.2426200294015	38\\
8.75527424487385	38\\
8.75527424487385	39\\
9.07982727492201	39\\
9.07982727492201	40\\
9.30429022198901	40\\
9.30429022198901	41\\
9.36450390401298	41\\
9.36450390401298	42\\
9.50538978989993	42\\
9.50538978989993	43\\
9.60647618750429	43\\
9.60647618750429	44\\
11	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0547098025732069	0\\
0.120126942515171	0\\
0.120126942515171	1\\
0.301088738424319	1\\
0.301088738424319	2\\
0.692940000017529	2\\
0.692940000017529	3\\
0.888548768372878	3\\
0.888548768372878	4\\
1.11361181733929	4\\
1.11361181733929	5\\
1.20884618113607	5\\
1.20884618113607	6\\
1.30031394726129	6\\
1.30031394726129	7\\
2.00771277750905	7\\
2.00771277750905	8\\
2.22762522371231	8\\
2.22762522371231	9\\
2.33027699279288	9\\
2.33027699279288	10\\
2.34103774039923	10\\
2.34103774039923	11\\
2.62458449809542	11\\
2.62458449809542	12\\
2.85485041302344	12\\
2.85485041302344	13\\
2.91712062262186	13\\
2.91712062262186	14\\
3.06113785548113	14\\
3.06113785548113	15\\
3.2023069124898	15\\
3.2023069124898	16\\
3.23666815043069	16\\
3.23666815043069	17\\
3.55506991557024	17\\
3.55506991557024	18\\
3.56919084033244	18\\
3.56919084033244	19\\
3.68552726134045	19\\
3.68552726134045	20\\
3.73225858281098	20\\
3.73225858281098	21\\
4.07506507708564	21\\
4.07506507708564	22\\
4.08217203854395	22\\
4.08217203854395	23\\
4.21306068235172	23\\
4.21306068235172	24\\
4.22782322252457	24\\
4.22782322252457	25\\
4.71057268790634	25\\
4.71057268790634	26\\
4.97737015912467	26\\
4.97737015912467	27\\
5.10794837808618	27\\
5.10794837808618	28\\
5.13053617629257	28\\
5.13053617629257	29\\
5.23723887996644	29\\
5.23723887996644	30\\
5.57551529174084	30\\
5.57551529174084	31\\
5.70025640669522	31\\
5.70025640669522	32\\
5.98084810671628	32\\
5.98084810671628	33\\
6.09372623845264	33\\
6.09372623845264	34\\
6.2315768365904	34\\
6.2315768365904	35\\
6.42102208735005	35\\
6.42102208735005	36\\
6.70746620443105	36\\
6.70746620443105	37\\
6.88647151881528	37\\
6.88647151881528	38\\
6.94844165682333	38\\
6.94844165682333	39\\
7.48753343570912	39\\
7.48753343570912	40\\
8.3026146664861	40\\
8.3026146664861	41\\
8.42431084488933	41\\
8.42431084488933	42\\
8.43471313963565	42\\
8.43471313963565	43\\
8.49963220909098	43\\
8.49963220909098	44\\
8.52338016803645	44\\
8.52338016803645	45\\
9.27355285904424	45\\
9.27355285904424	46\\
9.4350182763715	46\\
9.4350182763715	47\\
9.90662713832246	47\\
9.90662713832246	48\\
9.97623808420683	48\\
9.97623808420683	49\\
9.98809087562125	49\\
9.98809087562125	50\\
10.2759757041115	50\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0183047580969742	0\\
0.0569514429622657	0\\
0.0569514429622657	1\\
0.225578948322969	1\\
0.225578948322969	2\\
0.271712274693776	2\\
0.271712274693776	3\\
0.609384407710429	3\\
0.609384407710429	4\\
1.27490535671186	4\\
1.27490535671186	5\\
1.48283145557478	5\\
1.48283145557478	6\\
1.98407767729235	6\\
1.98407767729235	7\\
2.05803410737411	7\\
2.05803410737411	8\\
2.36318289035953	8\\
2.36318289035953	9\\
2.51306783765704	9\\
2.51306783765704	10\\
2.88788736579983	10\\
2.88788736579983	11\\
2.96269586831081	11\\
2.96269586831081	12\\
3.13405027810711	12\\
3.13405027810711	13\\
3.49561847276181	13\\
3.49561847276181	14\\
3.78077615078403	14\\
3.78077615078403	15\\
4.00463900130703	15\\
4.00463900130703	16\\
4.68999235809744	16\\
4.68999235809744	17\\
4.71279403453413	17\\
4.71279403453413	18\\
4.76869885723998	18\\
4.76869885723998	19\\
4.78700322871675	19\\
4.78700322871675	20\\
4.83541744110912	20\\
4.83541744110912	21\\
4.91681947420005	21\\
4.91681947420005	22\\
4.91744803510051	23\\
5.32077466180683	23\\
5.32077466180683	24\\
5.54118087493631	24\\
5.54118087493631	25\\
5.62859733463576	25\\
5.62859733463576	26\\
5.74730046489442	26\\
5.74730046489442	27\\
5.95606104794667	27\\
5.95606104794667	28\\
6.24211100810668	28\\
6.24211100810668	29\\
6.46508792646279	29\\
6.46508792646279	30\\
6.50083523057701	30\\
6.50083523057701	31\\
6.68479396297013	31\\
6.68479396297013	32\\
6.71287185413104	32\\
6.71287185413104	33\\
7.69013746988065	33\\
7.69013746988065	34\\
8.42842484574338	34\\
8.42842484574338	35\\
8.73435977340773	35\\
8.73435977340773	36\\
9.9775011346111	36\\
9.9775011346111	37\\
10.1076439458706	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0516087331001103	0\\
0.0986368155389457	0\\
0.0986368155389457	1\\
0.5093320060069	1\\
0.5093320060069	2\\
0.516273820807555	2\\
0.516273820807555	3\\
0.621270011462215	3\\
0.621270011462215	4\\
1.6083172617584	4\\
1.6083172617584	5\\
1.66907229229975	5\\
1.66907229229975	6\\
1.81047658670166	6\\
1.81047658670166	7\\
2.13839377714505	7\\
2.13839377714505	8\\
2.22201428563645	8\\
2.22201428563645	9\\
2.23035357383877	9\\
2.23035357383877	10\\
2.30488862312745	10\\
2.30488862312745	11\\
2.57401732967719	11\\
2.57401732967719	12\\
2.59027070224582	12\\
2.59027070224582	13\\
2.66114772751725	13\\
2.66114772751725	14\\
2.93733661063514	14\\
2.93733661063514	15\\
3.05602275570164	15\\
3.05602275570164	16\\
3.43888145913305	16\\
3.43888145913305	17\\
3.54697200530899	17\\
3.54697200530899	18\\
3.56149847209956	18\\
3.56149847209956	19\\
4.45495056197232	19\\
4.45495056197232	20\\
4.82768477877062	20\\
4.82768477877062	21\\
4.99110095027973	21\\
4.99110095027973	22\\
5.10140244149712	22\\
5.10140244149712	23\\
5.10937411500007	23\\
5.10937411500007	24\\
5.18735502433336	24\\
5.18735502433336	25\\
5.33963941218332	25\\
5.33963941218332	26\\
5.4001985316894	26\\
5.4001985316894	27\\
5.57183971528243	27\\
5.57183971528243	28\\
5.84082769860579	28\\
5.84082769860579	29\\
6.91197565970706	29\\
6.91197565970706	30\\
7.03841907696811	30\\
7.03841907696811	31\\
7.12434565929959	31\\
7.12434565929959	32\\
7.71002036838665	32\\
7.71002036838665	33\\
8.3179362519224	33\\
8.3179362519224	34\\
8.82833323873428	34\\
8.82833323873428	35\\
9.27773190041375	35\\
9.27773190041375	36\\
9.45521716001181	36\\
9.45521716001181	37\\
9.49738955679309	37\\
9.49738955679309	38\\
9.72463474909167	38\\
9.72463474909167	39\\
9.82090099222956	39\\
9.82090099222956	40\\
10.2716946416951	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
1.22314878994354	0\\
1.78267661935785	0\\
1.78267661935785	1\\
2.01571616031794	1\\
2.01571616031794	2\\
2.08079883159823	2\\
2.08079883159823	3\\
2.16928414966262	3\\
2.16928414966262	4\\
2.67274499614232	4\\
2.67274499614232	5\\
2.91594918944202	5\\
2.91594918944202	6\\
3.119024561708	6\\
3.119024561708	7\\
3.19881052659722	7\\
3.19881052659722	8\\
3.66218278882375	8\\
3.66218278882375	9\\
4.04364884426997	9\\
4.04364884426997	10\\
4.04389914103593	11\\
4.21579380202656	11\\
4.21579380202656	12\\
4.54127768021636	12\\
4.54127768021636	13\\
4.7059618963852	13\\
4.7059618963852	14\\
4.86178686528459	14\\
4.86178686528459	15\\
5.03145599399334	15\\
5.03145599399334	16\\
5.32643826102265	16\\
5.32643826102265	17\\
5.37538995978343	17\\
5.37538995978343	18\\
5.73014268384269	18\\
5.73014268384269	19\\
5.89875088337086	19\\
5.89875088337086	20\\
6.03818469069174	20\\
6.03818469069174	21\\
6.37074822107561	21\\
6.37074822107561	22\\
6.64366319611378	22\\
6.64366319611378	23\\
6.65582403281228	23\\
6.65582403281228	24\\
6.70984425338885	24\\
6.70984425338885	25\\
7.02827673706081	25\\
7.02827673706081	26\\
7.03700371924337	26\\
7.03700371924337	27\\
7.0442675847826	27\\
7.0442675847826	28\\
7.17075539296799	28\\
7.17075539296799	29\\
7.21040029032907	29\\
7.21040029032907	30\\
7.37714344415469	30\\
7.37714344415469	31\\
7.38509950713861	31\\
7.38509950713861	32\\
7.54467819991046	32\\
7.54467819991046	33\\
7.80299214570501	33\\
7.80299214570501	34\\
7.91417302909083	34\\
7.91417302909083	35\\
7.98275261758727	35\\
7.98275261758727	36\\
8.07798332631367	36\\
8.07798332631367	37\\
8.19461268161894	37\\
8.19461268161894	38\\
8.24224898533927	38\\
8.24224898533927	39\\
8.46028615504267	39\\
8.46028615504267	40\\
8.52688546661909	40\\
8.52688546661909	41\\
8.70876691959437	41\\
8.70876691959437	42\\
8.74875502259179	42\\
8.74875502259179	43\\
8.93734636673096	43\\
8.93734636673096	44\\
9.09428050116905	44\\
9.09428050116905	45\\
9.23587039194371	45\\
9.23587039194371	46\\
9.61163203117401	46\\
9.61163203117401	47\\
9.71046798190546	47\\
9.71046798190546	48\\
10.0725708031991	48\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.00494139399663851	0\\
0.210320440652943	0\\
0.210320440652943	1\\
0.237072801379306	1\\
0.237072801379306	2\\
1.00480394538162	2\\
1.00480394538162	3\\
1.20461352159396	3\\
1.20461352159396	4\\
1.36194785233638	4\\
1.36194785233638	5\\
1.47253106435454	5\\
1.47253106435454	6\\
1.76507750360276	6\\
1.76507750360276	7\\
2.26112785334971	7\\
2.26112785334971	8\\
2.40389303530157	8\\
2.40389303530157	9\\
2.47643042288963	9\\
2.47643042288963	10\\
2.5607072156993	10\\
2.5607072156993	11\\
2.71440899287396	11\\
2.71440899287396	12\\
3.0682496476215	12\\
3.0682496476215	13\\
3.20033374521842	13\\
3.20033374521842	14\\
3.26172104746578	14\\
3.26172104746578	15\\
3.53402851320934	15\\
3.53402851320934	16\\
3.54761634461912	16\\
3.54761634461912	17\\
3.68171359951947	17\\
3.68171359951947	18\\
3.73892006777251	18\\
3.73892006777251	19\\
3.9837398743899	19\\
3.9837398743899	20\\
4.41666398106673	20\\
4.41666398106673	21\\
4.59075818522746	21\\
4.59075818522746	22\\
4.72492723284475	22\\
4.72492723284475	23\\
5.07152937415374	23\\
5.07152937415374	24\\
5.1605209208662	24\\
5.1605209208662	25\\
5.18267508016224	25\\
5.18267508016224	26\\
5.55842566730434	26\\
5.55842566730434	27\\
6.74902908749905	27\\
6.74902908749905	28\\
7.40639507185169	28\\
7.40639507185169	29\\
7.94281900862589	29\\
7.94281900862589	30\\
8.22147464066744	30\\
8.22147464066744	31\\
8.42409086733913	31\\
8.42409086733913	32\\
8.85574605471835	32\\
8.85574605471835	33\\
9.31341358051871	33\\
9.31341358051871	34\\
9.83918709388158	34\\
9.83918709388158	35\\
10.1691248360495	35\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0919035416267704	0\\
0.303781766848324	0\\
0.303781766848324	1\\
0.346429805377092	1\\
0.346429805377092	2\\
1.24437477475082	2\\
1.24437477475082	3\\
1.70162712146309	3\\
1.70162712146309	4\\
2.37806022231867	4\\
2.37806022231867	5\\
2.42191469362257	5\\
2.42191469362257	6\\
2.48590440255573	6\\
2.48590440255573	7\\
2.65606563791331	7\\
2.65606563791331	8\\
2.83603434259143	8\\
2.83603434259143	9\\
2.98514957076946	9\\
2.98514957076946	10\\
3.39027614430468	10\\
3.39027614430468	11\\
3.39710008850076	11\\
3.39710008850076	12\\
3.72181944812016	12\\
3.72181944812016	13\\
3.76471256603528	13\\
3.76471256603528	14\\
4.06804401337872	14\\
4.06804401337872	15\\
4.08182195041163	15\\
4.08182195041163	16\\
4.23573196236211	16\\
4.23573196236211	17\\
4.63073783865273	17\\
4.63073783865273	18\\
5.2492698080837	18\\
5.2492698080837	19\\
5.42381107689525	19\\
5.42381107689525	20\\
5.54120665351334	20\\
5.54120665351334	21\\
5.55400710405173	21\\
5.55400710405173	22\\
5.64487112684443	22\\
5.64487112684443	23\\
5.75902251067627	23\\
5.75902251067627	24\\
5.79574218151373	24\\
5.79574218151373	25\\
6.0009962999831	25\\
6.0009962999831	26\\
6.87171854363531	26\\
6.87171854363531	27\\
7.25721024085389	27\\
7.25721024085389	28\\
7.4951518125971	28\\
7.4951518125971	29\\
8.80593685619587	29\\
8.80593685619587	30\\
9.00826160563879	30\\
9.00826160563879	31\\
9.02569441504627	31\\
9.02569441504627	32\\
9.20955803040097	32\\
9.20955803040097	33\\
9.38256579241479	33\\
9.38256579241479	34\\
9.44570676662287	34\\
9.44570676662287	35\\
9.60704502922403	35\\
9.60704502922403	36\\
9.65615992637721	36\\
9.65615992637721	37\\
10.0242821939387	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
1.06014913288853	0\\
1.37412455960322	0\\
1.37412455960322	1\\
1.49694625961437	1\\
1.49694625961437	2\\
1.69874027702116	2\\
1.69874027702116	3\\
1.8275597902067	3\\
1.8275597902067	4\\
1.87737111980191	4\\
1.87737111980191	5\\
1.99568494417795	5\\
1.99568494417795	6\\
2.07360187522234	6\\
2.07360187522234	7\\
2.18898185978694	7\\
2.18898185978694	8\\
2.68143531863076	8\\
2.68143531863076	9\\
2.6948231111402	9\\
2.6948231111402	10\\
2.70621068178134	10\\
2.70621068178134	11\\
2.90880042435788	11\\
2.90880042435788	12\\
3.19819518272286	12\\
3.19819518272286	13\\
3.70708451708836	13\\
3.70708451708836	14\\
3.95193639048959	14\\
3.95193639048959	15\\
4.38533597043281	15\\
4.38533597043281	16\\
4.90483954442962	16\\
4.90483954442962	17\\
4.95074534950355	17\\
4.95074534950355	18\\
5.010079993308	18\\
5.010079993308	19\\
5.51870047136669	19\\
5.51870047136669	20\\
5.75577862719845	20\\
5.75577862719845	21\\
5.94741304498508	21\\
5.94741304498508	22\\
6.15450867469951	22\\
6.15450867469951	23\\
6.30816194722847	23\\
6.30816194722847	24\\
6.45018059211014	24\\
6.45018059211014	25\\
6.49551646942365	25\\
6.49551646942365	26\\
6.56727748482201	26\\
6.56727748482201	27\\
6.6074345850019	27\\
6.6074345850019	28\\
6.88023465083148	28\\
6.88023465083148	29\\
6.9444214273536	29\\
6.9444214273536	30\\
7.1888663662527	30\\
7.1888663662527	31\\
7.49928020068752	31\\
7.49928020068752	32\\
7.81720067005256	32\\
7.81720067005256	33\\
7.91115717609514	33\\
7.91115717609514	34\\
8.11043924533264	34\\
8.11043924533264	35\\
8.41456342937427	35\\
8.41456342937427	36\\
8.67502570613865	36\\
8.67502570613865	37\\
8.92734323790437	37\\
8.92734323790437	38\\
9.02942384114235	38\\
9.02942384114235	39\\
9.12431623124928	39\\
9.12431623124928	40\\
9.36207449399932	40\\
9.36207449399932	41\\
9.41764400382728	41\\
9.41764400382728	42\\
10.4141756781602	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.160074915963062	0\\
0.21995428244028	0\\
0.21995428244028	1\\
0.254291824320759	1\\
0.254291824320759	2\\
0.566766373964853	2\\
0.566766373964853	3\\
0.65333279455179	3\\
0.65333279455179	4\\
1.05696451282316	4\\
1.05696451282316	5\\
1.27677953853329	5\\
1.27677953853329	6\\
1.87485302675285	6\\
1.87485302675285	7\\
1.9589955854398	7\\
1.9589955854398	8\\
1.96854695117958	8\\
1.96854695117958	9\\
2.07883892589594	9\\
2.07883892589594	10\\
2.1957887746926	10\\
2.1957887746926	11\\
2.37618045750264	11\\
2.37618045750264	12\\
2.58900143025706	12\\
2.58900143025706	13\\
2.81771077418016	13\\
2.81771077418016	14\\
2.96156029660474	14\\
2.96156029660474	15\\
3.14714095454523	15\\
3.14714095454523	16\\
4.32633212363388	16\\
4.32633212363388	17\\
4.42959421584804	17\\
4.42959421584804	18\\
4.7548726621032	18\\
4.7548726621032	19\\
5.48738359123497	19\\
5.48738359123497	20\\
5.6119272343003	20\\
5.6119272343003	21\\
5.69941029740551	21\\
5.69941029740551	22\\
6.19448934242238	22\\
6.19448934242238	23\\
6.33468751159426	23\\
6.33468751159426	24\\
7.05325626821704	24\\
7.05325626821704	25\\
7.864716834833	25\\
7.864716834833	26\\
8.80536352776413	26\\
8.80536352776413	27\\
8.82773963573239	27\\
8.82773963573239	28\\
8.9723796037359	28\\
8.9723796037359	29\\
9.31404789494325	29\\
9.31404789494325	30\\
9.92409154869912	30\\
9.92409154869912	31\\
10.0489527786708	31\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0487456254659975	0\\
0.217927126997282	0\\
0.217927126997282	1\\
0.232444016701301	1\\
0.232444016701301	2\\
0.317117256390802	2\\
0.317117256390802	3\\
0.476061386343339	3\\
0.476061386343339	4\\
0.599260784690578	4\\
0.599260784690578	5\\
1.11560116228541	5\\
1.11560116228541	6\\
1.22242860008794	6\\
1.22242860008794	7\\
1.58681799233296	7\\
1.58681799233296	8\\
1.77924682424685	8\\
1.77924682424685	9\\
1.96849484233242	9\\
1.96849484233242	10\\
2.0689661400679	10\\
2.0689661400679	11\\
2.1390203183911	11\\
2.1390203183911	12\\
2.15301617601452	12\\
2.15301617601452	13\\
2.56094346681412	13\\
2.56094346681412	14\\
2.82124087968688	14\\
2.82124087968688	15\\
2.8821750546081	15\\
2.8821750546081	16\\
2.90278542699486	16\\
2.90278542699486	17\\
3.16159668103219	17\\
3.16159668103219	18\\
3.31404032535006	18\\
3.31404032535006	19\\
3.36216631832052	19\\
3.36216631832052	20\\
3.60094501045263	20\\
3.60094501045263	21\\
3.60379865729158	21\\
3.60379865729158	22\\
3.7841229591524	22\\
3.7841229591524	23\\
4.01589532795641	23\\
4.01589532795641	24\\
4.12001300341561	24\\
4.12001300341561	25\\
4.52259549619007	25\\
4.52259549619007	26\\
4.64962615567791	26\\
4.64962615567791	27\\
4.80306010135995	27\\
4.80306010135995	28\\
5.3998781814788	28\\
5.3998781814788	29\\
5.61392850007256	29\\
5.61392850007256	30\\
5.81935482551005	30\\
5.81935482551005	31\\
5.90219908978163	31\\
5.90219908978163	32\\
5.91965628156107	32\\
5.91965628156107	33\\
6.0023745040922	33\\
6.0023745040922	34\\
6.44340824728074	34\\
6.44340824728074	35\\
6.45809520071621	35\\
6.45809520071621	36\\
6.6035958471348	36\\
6.6035958471348	37\\
6.83876817066348	37\\
6.83876817066348	38\\
6.94203997472952	38\\
6.94203997472952	39\\
7.08966572940393	39\\
7.08966572940393	40\\
7.12265394430405	40\\
7.12265394430405	41\\
7.13258167864904	41\\
7.13258167864904	42\\
7.29133776180357	42\\
7.29133776180357	43\\
7.34870265820755	43\\
7.34870265820755	44\\
7.41164760355569	44\\
7.41164760355569	45\\
7.61173405000356	45\\
7.61173405000356	46\\
7.62715055548502	46\\
7.62715055548502	47\\
7.77157253734112	47\\
7.77157253734112	48\\
7.86071730419714	48\\
7.86071730419714	49\\
8.13497154831316	49\\
8.13497154831316	50\\
8.37715259290055	50\\
8.37715259290055	51\\
8.40833808767407	51\\
8.40833808767407	52\\
8.50473706123898	52\\
8.50473706123898	53\\
8.66584970569502	53\\
8.66584970569502	54\\
8.74879122001406	54\\
8.74879122001406	55\\
8.82055624408858	55\\
8.82055624408858	56\\
9.29575382173554	56\\
9.29575382173554	57\\
10.3666393178074	57\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.459317242144508	0\\
0.702115209452447	0\\
0.702115209452447	1\\
0.896366508513182	1\\
0.896366508513182	2\\
0.905581849095103	2\\
0.905581849095103	3\\
1.20120616481232	3\\
1.20120616481232	4\\
1.43729306642718	4\\
1.43729306642718	5\\
1.49864162573208	5\\
1.49864162573208	6\\
1.68823189010533	6\\
1.68823189010533	7\\
2.11814864207329	7\\
2.11814864207329	8\\
2.31455040356438	8\\
2.31455040356438	9\\
2.89281014768072	9\\
2.89281014768072	10\\
3.00618687435385	10\\
3.00618687435385	11\\
3.03824898215451	11\\
3.03824898215451	12\\
3.8843184632641	12\\
3.8843184632641	13\\
4.70766695032606	13\\
4.70766695032606	14\\
4.97637833179248	14\\
4.97637833179248	15\\
5.24633839017637	15\\
5.24633839017637	16\\
5.51470005021012	16\\
5.51470005021012	17\\
6.36644738061808	17\\
6.36644738061808	18\\
6.47188235340856	18\\
6.47188235340856	19\\
6.57867385593464	19\\
6.57867385593464	20\\
6.65716277047182	20\\
6.65716277047182	21\\
7.19282745150334	21\\
7.19282745150334	22\\
7.43105000187114	22\\
7.43105000187114	23\\
7.84837824989827	23\\
7.84837824989827	24\\
8.50904224787526	24\\
8.50904224787526	25\\
8.9056213214167	25\\
8.9056213214167	26\\
9.00863299857043	26\\
9.00863299857043	27\\
9.03645833306391	27\\
9.03645833306391	28\\
9.06623014230776	28\\
9.06623014230776	29\\
9.18327794886183	29\\
9.18327794886183	30\\
10.1366602024629	30\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0817464194769926	0\\
0.244956783036152	0\\
0.244956783036152	1\\
0.367994656613917	1\\
0.367994656613917	2\\
0.501930766379537	2\\
0.501930766379537	3\\
0.553279759005669	3\\
0.553279759005669	4\\
0.655900340431941	4\\
0.655900340431941	5\\
0.731378734640877	5\\
0.731378734640877	6\\
0.78181900183408	6\\
0.78181900183408	7\\
0.832040130342953	7\\
0.832040130342953	8\\
0.953375784345319	8\\
0.953375784345319	9\\
0.977675702182765	9\\
0.977675702182765	10\\
1.14723407889014	10\\
1.14723407889014	11\\
1.66963085983275	11\\
1.66963085983275	12\\
1.74856185069608	12\\
1.74856185069608	13\\
2.20578619391187	13\\
2.20578619391187	14\\
2.28099242145404	14\\
2.28099242145404	15\\
2.58085986255475	15\\
2.58085986255475	16\\
2.68081714636091	16\\
2.68081714636091	17\\
2.86626865446994	17\\
2.86626865446994	18\\
3.15936581784603	18\\
3.15936581784603	19\\
3.38820454204273	19\\
3.38820454204273	20\\
4.54831956991887	20\\
4.54831956991887	21\\
4.93770518436153	21\\
4.93770518436153	22\\
5.25785382311424	22\\
5.25785382311424	23\\
5.33931817512887	23\\
5.33931817512887	24\\
5.46604744788212	24\\
5.46604744788212	25\\
5.5000883430804	25\\
5.5000883430804	26\\
5.62151735965212	26\\
5.62151735965212	27\\
5.87231081436484	27\\
5.87231081436484	28\\
5.94964039747877	28\\
5.94964039747877	29\\
6.47627618114309	29\\
6.47627618114309	30\\
6.61913907231197	30\\
6.61913907231197	31\\
6.63884739007505	31\\
6.63884739007505	32\\
6.69254864846515	32\\
6.69254864846515	33\\
6.82825055265466	33\\
6.82825055265466	34\\
6.8744492212786	34\\
6.8744492212786	35\\
6.94283594633561	35\\
6.94283594633561	36\\
7.48985548979893	36\\
7.48985548979893	37\\
7.81834399995639	37\\
7.81834399995639	38\\
7.89919615360392	38\\
7.89919615360392	39\\
8.34332615907159	39\\
8.34332615907159	40\\
8.70917578405404	40\\
8.70917578405404	41\\
8.73923382192608	41\\
8.73923382192608	42\\
9.08074967248713	42\\
9.08074967248713	43\\
9.45036408947669	43\\
9.45036408947669	44\\
9.51311168601222	44\\
9.51311168601222	45\\
10.268343682484	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0406705259186779	0\\
0.519969706978543	0\\
0.519969706978543	1\\
0.771612395617126	1\\
0.771612395617126	2\\
0.941746163234193	2\\
0.941746163234193	3\\
1.48951131210683	3\\
1.48951131210683	4\\
1.69700744230597	4\\
1.69700744230597	5\\
1.8116652987395	5\\
1.8116652987395	6\\
1.86982886200364	6\\
1.86982886200364	7\\
2.4732886935659	7\\
2.4732886935659	8\\
2.52367483872608	8\\
2.52367483872608	9\\
2.64626908916343	9\\
2.64626908916343	10\\
2.72918200894313	10\\
2.72918200894313	11\\
2.82660205583316	11\\
2.82660205583316	12\\
2.82782196634113	13\\
3.04403952725298	13\\
3.04403952725298	14\\
3.38477783219346	14\\
3.38477783219346	15\\
3.51139260286725	15\\
3.51139260286725	16\\
3.98317993842007	16\\
3.98317993842007	17\\
4.05514575654011	17\\
4.05514575654011	18\\
4.13242811279851	18\\
4.13242811279851	19\\
5.19699570803579	19\\
5.19699570803579	20\\
5.5359731413668	20\\
5.5359731413668	21\\
5.73238851371624	21\\
5.73238851371624	22\\
5.80896423067128	22\\
5.80896423067128	23\\
6.03722224439662	23\\
6.03722224439662	24\\
6.1539169816434	24\\
6.1539169816434	25\\
6.23881847162252	25\\
6.23881847162252	26\\
6.31456381737929	26\\
6.31456381737929	27\\
6.56080371763399	27\\
6.56080371763399	28\\
6.88108286553873	28\\
6.88108286553873	29\\
7.01968101692151	29\\
7.01968101692151	30\\
7.09025871375379	30\\
7.09025871375379	31\\
7.21039731599649	31\\
7.21039731599649	32\\
7.42395627212891	32\\
7.42395627212891	33\\
7.80867499588557	33\\
7.80867499588557	34\\
7.96553358146982	34\\
7.96553358146982	35\\
7.98720933258712	35\\
7.98720933258712	36\\
8.41868832112942	36\\
8.41868832112942	37\\
8.89356808763098	37\\
8.89356808763098	38\\
8.96807477224914	38\\
8.96807477224914	39\\
9.0391401603443	39\\
9.0391401603443	40\\
9.06258707646181	40\\
9.06258707646181	41\\
10.2332422099419	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.00136876836749167	0\\
0.293951355905314	0\\
0.293951355905314	1\\
0.336587029198839	1\\
0.336587029198839	2\\
0.710560865155529	2\\
0.710560865155529	3\\
0.711993186509254	4\\
1.03317046776702	4\\
1.03317046776702	5\\
1.40366788221804	5\\
1.40366788221804	6\\
1.91922112044959	6\\
1.91922112044959	7\\
1.94831390220378	7\\
1.94831390220378	8\\
2.28138462723469	8\\
2.28138462723469	9\\
2.51092594651618	9\\
2.51092594651618	10\\
2.60252685611378	10\\
2.60252685611378	11\\
2.74854390730107	11\\
2.74854390730107	12\\
3.07757608909239	12\\
3.07757608909239	13\\
3.22875670776084	13\\
3.22875670776084	14\\
3.27399666651651	14\\
3.27399666651651	15\\
3.30888523937807	15\\
3.30888523937807	16\\
3.57735766912753	16\\
3.57735766912753	17\\
4.2638829473561	17\\
4.2638829473561	18\\
4.58787771950075	18\\
4.58787771950075	19\\
4.69741898457941	19\\
4.69741898457941	20\\
5.0718323981941	20\\
5.0718323981941	21\\
5.60983643379608	21\\
5.60983643379608	22\\
5.90892356803914	22\\
5.90892356803914	23\\
6.22667117958605	23\\
6.22667117958605	24\\
7.19216848753666	24\\
7.19216848753666	25\\
7.51858553754967	25\\
7.51858553754967	26\\
7.59449375337618	26\\
7.59449375337618	27\\
7.69072903269252	27\\
7.69072903269252	28\\
7.72728060263166	28\\
7.72728060263166	29\\
8.13971055734611	29\\
8.13971055734611	30\\
8.35462426380101	30\\
8.35462426380101	31\\
8.60642928104446	31\\
8.60642928104446	32\\
8.62038463704558	32\\
8.62038463704558	33\\
8.98561728195189	33\\
8.98561728195189	34\\
9.18099169208141	34\\
9.18099169208141	35\\
9.68405048554391	35\\
9.68405048554391	36\\
9.72648426265295	36\\
9.72648426265295	37\\
9.77830755339787	37\\
9.77830755339787	38\\
10.0179725263152	38\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.555148339706555	0\\
0.644743071968882	0\\
0.644743071968882	1\\
0.659215526084246	1\\
0.659215526084246	2\\
0.670404216017118	2\\
0.670404216017118	3\\
0.817724411733323	3\\
0.817724411733323	4\\
1.41696798324782	4\\
1.41696798324782	5\\
1.5062586796211	5\\
1.5062586796211	6\\
1.94867224445203	6\\
1.94867224445203	7\\
2.64714263299867	7\\
2.64714263299867	8\\
2.84397950178519	8\\
2.84397950178519	9\\
2.84728474922697	9\\
2.84728474922697	10\\
3.08881601501472	10\\
3.08881601501472	11\\
3.33703585880428	11\\
3.33703585880428	12\\
3.42795307334761	12\\
3.42795307334761	13\\
3.71799385547254	13\\
3.71799385547254	14\\
3.95937236346909	14\\
3.95937236346909	15\\
3.97524208777494	15\\
3.97524208777494	16\\
4.04180813497164	16\\
4.04180813497164	17\\
4.05614439161039	17\\
4.05614439161039	18\\
4.56830637222095	18\\
4.56830637222095	19\\
4.63579496621744	19\\
4.63579496621744	20\\
4.8737995433663	20\\
4.8737995433663	21\\
4.91315567580482	21\\
4.91315567580482	22\\
4.9510174293478	22\\
4.9510174293478	23\\
5.16072354575046	23\\
5.16072354575046	24\\
5.4887072452728	24\\
5.4887072452728	25\\
5.93083020038522	25\\
5.93083020038522	26\\
5.97778625774941	26\\
5.97778625774941	27\\
6.04238974888391	27\\
6.04238974888391	28\\
6.29099027296326	28\\
6.29099027296326	29\\
6.34373644630321	29\\
6.34373644630321	30\\
6.42156826299119	30\\
6.42156826299119	31\\
6.99136796332876	31\\
6.99136796332876	32\\
7.05435162102633	32\\
7.05435162102633	33\\
7.33363348858888	33\\
7.33363348858888	34\\
7.38069721757098	34\\
7.38069721757098	35\\
7.98105812198546	35\\
7.98105812198546	36\\
8.14795145514523	36\\
8.14795145514523	37\\
8.24620957595691	37\\
8.24620957595691	38\\
8.33837352521588	38\\
8.33837352521588	39\\
8.55653912220374	39\\
8.55653912220374	40\\
8.88089522904998	40\\
8.88089522904998	41\\
9.02598235393265	41\\
9.02598235393265	42\\
9.48680336932658	42\\
9.48680336932658	43\\
9.89194169538552	43\\
9.89194169538552	44\\
10.1755224165111	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0775422395141092	0\\
0.115985900245832	0\\
0.115985900245832	1\\
0.148668063914165	1\\
0.148668063914165	2\\
0.154926793009714	2\\
0.154926793009714	3\\
0.192039598330872	3\\
0.192039598330872	4\\
0.195438570687898	4\\
0.195438570687898	5\\
0.389740716795799	5\\
0.389740716795799	6\\
1.00720505188608	6\\
1.00720505188608	7\\
1.00828537564867	8\\
1.31842063688102	8\\
1.31842063688102	9\\
1.69497918356371	9\\
1.69497918356371	10\\
2.00996771404249	10\\
2.00996771404249	11\\
2.04246363436459	11\\
2.04246363436459	12\\
2.49569385488226	12\\
2.49569385488226	13\\
2.63825429999309	13\\
2.63825429999309	14\\
2.82459382216953	14\\
2.82459382216953	15\\
3.62363791973249	15\\
3.62363791973249	16\\
3.71400936603057	16\\
3.71400936603057	17\\
3.80693762768685	17\\
3.80693762768685	18\\
3.89118535408238	18\\
3.89118535408238	19\\
4.23617003564308	19\\
4.23617003564308	20\\
4.73057175033711	20\\
4.73057175033711	21\\
4.98293512751623	21\\
4.98293512751623	22\\
5.03165514203162	22\\
5.03165514203162	23\\
5.19858981240232	23\\
5.19858981240232	24\\
5.34055157223496	24\\
5.34055157223496	25\\
5.51606504914515	25\\
5.51606504914515	26\\
5.60842944817085	26\\
5.60842944817085	27\\
5.93492020549226	27\\
5.93492020549226	28\\
6.30654855372137	28\\
6.30654855372137	29\\
6.69757666667426	29\\
6.69757666667426	30\\
7.19933952099353	30\\
7.19933952099353	31\\
7.68571196731364	31\\
7.68571196731364	32\\
7.91176708954179	32\\
7.91176708954179	33\\
7.95934174647673	33\\
7.95934174647673	34\\
7.96101018650145	35\\
8.5303319728006	35\\
8.5303319728006	36\\
9.21641246128359	36\\
9.21641246128359	37\\
9.67697656999167	37\\
9.67697656999167	38\\
9.78356168119127	38\\
9.78356168119127	39\\
10.4932731943862	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.153605938423503	0\\
0.229182038670587	0\\
0.229182038670587	1\\
0.381295283891014	1\\
0.381295283891014	2\\
0.421833965117386	2\\
0.421833965117386	3\\
0.489710836171554	3\\
0.489710836171554	4\\
0.491020369625424	5\\
0.869114480220404	5\\
0.869114480220404	6\\
0.87623526067199	6\\
0.87623526067199	7\\
1.12487561552559	7\\
1.12487561552559	8\\
1.41168183214056	8\\
1.41168183214056	9\\
1.43634120663348	9\\
1.43634120663348	10\\
2.2733184925032	10\\
2.2733184925032	11\\
2.34370211564173	11\\
2.34370211564173	12\\
2.48472398216906	12\\
2.48472398216906	13\\
2.55429904811029	13\\
2.55429904811029	14\\
2.87419193615045	14\\
2.87419193615045	15\\
3.05641724624404	15\\
3.05641724624404	16\\
3.15554504674766	16\\
3.15554504674766	17\\
3.58052072726858	17\\
3.58052072726858	18\\
3.59021518804703	18\\
3.59021518804703	19\\
3.75210337037225	19\\
3.75210337037225	20\\
4.0851105276073	20\\
4.0851105276073	21\\
4.11356981438526	21\\
4.11356981438526	22\\
4.35811335881924	22\\
4.35811335881924	23\\
4.53177285678696	23\\
4.53177285678696	24\\
4.54564615207727	24\\
4.54564615207727	25\\
4.97543720219844	25\\
4.97543720219844	26\\
4.98257289193062	26\\
4.98257289193062	27\\
5.03907801437948	27\\
5.03907801437948	28\\
5.11118465769652	28\\
5.11118465769652	29\\
5.16476099081324	29\\
5.16476099081324	30\\
5.19565331866721	30\\
5.19565331866721	31\\
5.78571140162821	31\\
5.78571140162821	32\\
5.81246683658237	32\\
5.81246683658237	33\\
5.88201681610055	33\\
5.88201681610055	34\\
5.93715057713741	34\\
5.93715057713741	35\\
5.98089172142689	35\\
5.98089172142689	36\\
6.01523462822504	36\\
6.01523462822504	37\\
6.18477068981721	37\\
6.18477068981721	38\\
6.22446243717507	38\\
6.22446243717507	39\\
6.35124508196273	39\\
6.35124508196273	40\\
6.54874837407702	40\\
6.54874837407702	41\\
6.73693222460364	41\\
6.73693222460364	42\\
6.83823402056593	42\\
6.83823402056593	43\\
6.95066777597147	43\\
6.95066777597147	44\\
7.21879939491502	44\\
7.21879939491502	45\\
7.29785234669519	45\\
7.29785234669519	46\\
7.35692526730891	46\\
7.35692526730891	47\\
8.16385444846045	47\\
8.16385444846045	48\\
8.65499761948707	48\\
8.65499761948707	49\\
8.66153023054944	49\\
8.66153023054944	50\\
8.81789978567284	50\\
8.81789978567284	51\\
8.82154695121977	51\\
8.82154695121977	52\\
8.8670628107951	52\\
8.8670628107951	53\\
8.92618389419873	53\\
8.92618389419873	54\\
9.47818466492453	54\\
9.47818466492453	55\\
9.71079410636043	55\\
9.71079410636043	56\\
9.76583411771765	56\\
9.76583411771765	57\\
9.81218053709518	57\\
9.81218053709518	58\\
9.97403671110582	58\\
9.97403671110582	59\\
9.99940568658714	59\\
9.99940568658714	60\\
10.2430306295352	60\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.18705192019118	0\\
0.500897054115043	0\\
0.500897054115043	1\\
0.627236457613094	1\\
0.627236457613094	2\\
0.683146210356334	2\\
0.683146210356334	3\\
0.713433882844321	3\\
0.713433882844321	4\\
0.985910209293145	4\\
0.985910209293145	5\\
0.987311497040629	6\\
1.5752156583715	6\\
1.5752156583715	7\\
1.7214829310618	7\\
1.7214829310618	8\\
2.05872636379395	8\\
2.05872636379395	9\\
2.53038677126064	9\\
2.53038677126064	10\\
2.68546100163942	10\\
2.68546100163942	11\\
3.07275052264166	11\\
3.07275052264166	12\\
3.08939509523655	12\\
3.08939509523655	13\\
3.16731036622492	13\\
3.16731036622492	14\\
3.26055531283498	14\\
3.26055531283498	15\\
3.59853657847518	15\\
3.59853657847518	16\\
3.98524385096968	16\\
3.98524385096968	17\\
4.59693337560388	17\\
4.59693337560388	18\\
4.96906831811231	18\\
4.96906831811231	19\\
5.09238709644641	19\\
5.09238709644641	20\\
5.70501278142311	20\\
5.70501278142311	21\\
5.75623448483921	21\\
5.75623448483921	22\\
7.02854719498588	22\\
7.02854719498588	23\\
7.10313076047697	23\\
7.10313076047697	24\\
7.45236068948968	24\\
7.45236068948968	25\\
7.57987512638388	25\\
7.57987512638388	26\\
7.71927241163075	26\\
7.71927241163075	27\\
8.07952257036764	27\\
8.07952257036764	28\\
8.70583275839105	28\\
8.70583275839105	29\\
8.78942073119709	29\\
8.78942073119709	30\\
8.81755907250187	30\\
8.81755907250187	31\\
8.8692117282821	31\\
8.8692117282821	32\\
8.90430747489967	32\\
8.90430747489967	33\\
9.17410603058114	33\\
9.17410603058114	34\\
9.29782007387696	34\\
9.29782007387696	35\\
9.36369693009524	35\\
9.36369693009524	36\\
9.45085635040589	36\\
9.45085635040589	37\\
9.78629151852675	37\\
9.78629151852675	38\\
9.86137100799327	38\\
9.86137100799327	39\\
9.89148696816195	39\\
9.89148696816195	40\\
9.92784757369103	40\\
9.92784757369103	41\\
10.2626875631897	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.201883884259843	0\\
0.590155994043613	0\\
0.590155994043613	1\\
0.793235190355475	1\\
0.793235190355475	2\\
0.826913287646214	2\\
0.826913287646214	3\\
1.33118010290808	3\\
1.33118010290808	4\\
1.87449757437254	4\\
1.87449757437254	5\\
2.17444883323862	5\\
2.17444883323862	6\\
2.56618547411002	6\\
2.56618547411002	7\\
2.58579578936065	7\\
2.58579578936065	8\\
2.59654802540707	8\\
2.59654802540707	9\\
3.05287312269532	9\\
3.05287312269532	10\\
3.10106060906825	10\\
3.10106060906825	11\\
3.44821617410332	11\\
3.44821617410332	12\\
3.65050708778265	12\\
3.65050708778265	13\\
3.97466739683939	13\\
3.97466739683939	14\\
4.19607638843677	14\\
4.19607638843677	15\\
4.65081202794359	15\\
4.65081202794359	16\\
4.70217119684659	16\\
4.70217119684659	17\\
4.91410321658835	17\\
4.91410321658835	18\\
4.94757586422254	18\\
4.94757586422254	19\\
4.99449506530844	19\\
4.99449506530844	20\\
5.21543980165136	20\\
5.21543980165136	21\\
5.57935079156778	21\\
5.57935079156778	22\\
6.42185349732207	22\\
6.42185349732207	23\\
6.46114058637874	23\\
6.46114058637874	24\\
6.59729929672896	24\\
6.59729929672896	25\\
6.65203163459026	25\\
6.65203163459026	26\\
6.94812916444381	26\\
6.94812916444381	27\\
7.32736007588924	27\\
7.32736007588924	28\\
7.34405497464181	28\\
7.34405497464181	29\\
7.49378928049352	29\\
7.49378928049352	30\\
7.68646772718963	30\\
7.68646772718963	31\\
7.72845142263083	31\\
7.72845142263083	32\\
7.84458904849794	32\\
7.84458904849794	33\\
8.19066798635578	33\\
8.19066798635578	34\\
9.57910308751395	34\\
9.57910308751395	35\\
9.59749234911747	35\\
9.59749234911747	36\\
9.83680163532239	36\\
9.83680163532239	37\\
10.4493959747994	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.342441312075877	0\\
0.347759234215516	0\\
0.347759234215516	1\\
0.445161009344751	1\\
0.445161009344751	2\\
0.565585147698748	2\\
0.565585147698748	3\\
0.65015985052225	3\\
0.65015985052225	4\\
0.750938053573726	4\\
0.750938053573726	5\\
0.920922705946687	5\\
0.920922705946687	6\\
1.16152725149948	6\\
1.16152725149948	7\\
1.2121931764951	7\\
1.2121931764951	8\\
1.45906924172315	8\\
1.45906924172315	9\\
1.74941809972179	9\\
1.74941809972179	10\\
2.13616311942801	10\\
2.13616311942801	11\\
2.1365508593821	12\\
2.1608228941762	12\\
2.1608228941762	13\\
2.1839554819358	13\\
2.1839554819358	14\\
2.2467980279608	14\\
2.2467980279608	15\\
2.48976851239836	15\\
2.48976851239836	16\\
2.56209207599385	16\\
2.56209207599385	17\\
3.10381573869608	17\\
3.10381573869608	18\\
3.66156949952586	18\\
3.66156949952586	19\\
3.68848065738878	19\\
3.68848065738878	20\\
3.69241463973849	20\\
3.69241463973849	21\\
3.7090264014933	21\\
3.7090264014933	22\\
3.76044802016526	22\\
3.76044802016526	23\\
3.85382931131369	23\\
3.85382931131369	24\\
4.69044405299325	24\\
4.69044405299325	25\\
4.8240588736727	25\\
4.8240588736727	26\\
5.1476862403379	26\\
5.1476862403379	27\\
5.29962142680812	27\\
5.29962142680812	28\\
6.10748226358915	28\\
6.10748226358915	29\\
6.43847250318723	29\\
6.43847250318723	30\\
6.45617928690274	30\\
6.45617928690274	31\\
6.70110218995042	31\\
6.70110218995042	32\\
6.81650511068433	32\\
6.81650511068433	33\\
7.28506867055008	33\\
7.28506867055008	34\\
7.32653366096614	34\\
7.32653366096614	35\\
7.49777165229056	35\\
7.49777165229056	36\\
7.55286976765464	36\\
7.55286976765464	37\\
7.87674805502912	37\\
7.87674805502912	38\\
8.38454173853	38\\
8.38454173853	39\\
8.9634785737023	39\\
8.9634785737023	40\\
9.15091499099044	40\\
9.15091499099044	41\\
9.210464135777	41\\
9.210464135777	42\\
9.50048784837498	42\\
9.50048784837498	43\\
9.62554982382963	43\\
9.62554982382963	44\\
9.78741408243643	44\\
9.78741408243643	45\\
9.82579008461889	45\\
9.82579008461889	46\\
10.6974708958359	46\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.00529474862464241	0\\
0.171863471243149	0\\
0.171863471243149	1\\
0.514476847551357	1\\
0.514476847551357	2\\
1.03256980527151	2\\
1.03256980527151	3\\
1.11800181815971	3\\
1.11800181815971	4\\
1.35099292863358	4\\
1.35099292863358	5\\
1.51970057659662	5\\
1.51970057659662	6\\
1.770643128836	6\\
1.770643128836	7\\
2.40182607789082	7\\
2.40182607789082	8\\
2.88243018708959	8\\
2.88243018708959	9\\
2.97593598804438	9\\
2.97593598804438	10\\
3.09749659108033	10\\
3.09749659108033	11\\
3.2768451450513	11\\
3.2768451450513	12\\
3.29589516425838	12\\
3.29589516425838	13\\
3.46681341911509	13\\
3.46681341911509	14\\
3.4823290353159	14\\
3.4823290353159	15\\
3.49748931730792	15\\
3.49748931730792	16\\
3.66292079039771	16\\
3.66292079039771	17\\
3.72337498036823	17\\
3.72337498036823	18\\
4.10233870801647	18\\
4.10233870801647	19\\
4.68252820795781	19\\
4.68252820795781	20\\
4.79811245544324	20\\
4.79811245544324	21\\
4.80316039415686	21\\
4.80316039415686	22\\
4.89996159385154	22\\
4.89996159385154	23\\
4.92187704176034	23\\
4.92187704176034	24\\
5.03456274743659	24\\
5.03456274743659	25\\
5.03640441114609	26\\
5.88752336828674	26\\
5.88752336828674	27\\
6.09507985500552	27\\
6.09507985500552	28\\
6.40409875831902	28\\
6.40409875831902	29\\
6.46483564883321	29\\
6.46483564883321	30\\
6.5508727559913	30\\
6.5508727559913	31\\
6.57829692187634	31\\
6.57829692187634	32\\
6.70747410218254	32\\
6.70747410218254	33\\
6.93743862641923	33\\
6.93743862641923	34\\
7.00255754021714	34\\
7.00255754021714	35\\
7.24437947699447	35\\
7.24437947699447	36\\
7.81019092368103	36\\
7.81019092368103	37\\
7.90895926994622	37\\
7.90895926994622	38\\
8.14513725413486	38\\
8.14513725413486	39\\
8.39111129615193	39\\
8.39111129615193	40\\
8.58510380582711	40\\
8.58510380582711	41\\
8.96602905931402	41\\
8.96602905931402	42\\
9.80459708464809	42\\
9.80459708464809	43\\
10.004257553139	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.07955650828535	0\\
0.105008668081268	0\\
0.105008668081268	1\\
0.788153747798766	1\\
0.788153747798766	2\\
1.06466046600206	2\\
1.06466046600206	3\\
1.181036246457	3\\
1.181036246457	4\\
1.22492777764686	4\\
1.22492777764686	5\\
1.30486256581411	5\\
1.30486256581411	6\\
1.8844949990042	6\\
1.8844949990042	7\\
1.9077318616155	7\\
1.9077318616155	8\\
2.11365091439274	8\\
2.11365091439274	9\\
2.21944198224882	9\\
2.21944198224882	10\\
2.54328769374938	10\\
2.54328769374938	11\\
2.60154570562437	11\\
2.60154570562437	12\\
2.72233496439532	12\\
2.72233496439532	13\\
3.47697721301142	13\\
3.47697721301142	14\\
3.74777483052554	14\\
3.74777483052554	15\\
3.7846734380124	15\\
3.7846734380124	16\\
3.80690732343272	16\\
3.80690732343272	17\\
3.96369275656337	17\\
3.96369275656337	18\\
4.05933906179061	18\\
4.05933906179061	19\\
4.49125995215736	19\\
4.49125995215736	20\\
4.51006570715136	20\\
4.51006570715136	21\\
4.58357648720759	21\\
4.58357648720759	22\\
4.78393728978113	22\\
4.78393728978113	23\\
5.01238467313219	23\\
5.01238467313219	24\\
5.09850792432375	24\\
5.09850792432375	25\\
5.63033329334542	25\\
5.63033329334542	26\\
5.66289799679083	26\\
5.66289799679083	27\\
6.0449926976731	27\\
6.0449926976731	28\\
6.38796345821716	28\\
6.38796345821716	29\\
6.41497045921814	29\\
6.41497045921814	30\\
6.70578385565158	30\\
6.70578385565158	31\\
6.81709694490175	31\\
6.81709694490175	32\\
7.0039606128081	32\\
7.0039606128081	33\\
7.87910603549106	33\\
7.87910603549106	34\\
7.95103492418592	34\\
7.95103492418592	35\\
8.04192832793707	35\\
8.04192832793707	36\\
8.19944467247465	36\\
8.19944467247465	37\\
8.27331026045407	37\\
8.27331026045407	38\\
8.5500088921799	38\\
8.5500088921799	39\\
8.56064329210243	39\\
8.56064329210243	40\\
9.15480258015377	40\\
9.15480258015377	41\\
9.3045918267607	41\\
9.3045918267607	42\\
9.43759841461177	42\\
9.43759841461177	43\\
9.62472448250249	43\\
9.62472448250249	44\\
9.68016871097772	44\\
9.68016871097772	45\\
9.72132572717427	45\\
9.72132572717427	46\\
9.87247987958474	46\\
9.87247987958474	47\\
9.99662165611071	47\\
9.99662165611071	48\\
10.0310007193996	48\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.59920316197173	0\\
0.73954106729073	0\\
0.73954106729073	1\\
0.770717681898176	1\\
0.770717681898176	2\\
0.949283999772092	2\\
0.949283999772092	3\\
1.14457329542126	3\\
1.14457329542126	4\\
1.3510734109932	4\\
1.3510734109932	5\\
1.43355702197241	5\\
1.43355702197241	6\\
1.62956482688543	6\\
1.62956482688543	7\\
1.64451345481559	7\\
1.64451345481559	8\\
1.91968913471192	8\\
1.91968913471192	9\\
2.09355772802687	9\\
2.09355772802687	10\\
2.10556651027446	10\\
2.10556651027446	11\\
2.5538232534368	11\\
2.5538232534368	12\\
2.55507512965689	13\\
2.66868939331012	13\\
2.66868939331012	14\\
2.69375779830385	14\\
2.69375779830385	15\\
2.95106879882585	15\\
2.95106879882585	16\\
2.99530242410521	16\\
2.99530242410521	17\\
3.0728239073835	17\\
3.0728239073835	18\\
3.2703114242596	18\\
3.2703114242596	19\\
4.40599119567738	19\\
4.40599119567738	20\\
4.56424614069462	20\\
4.56424614069462	21\\
4.59091344824312	21\\
4.59091344824312	22\\
4.91474553752464	22\\
4.91474553752464	23\\
5.04702788959655	23\\
5.04702788959655	24\\
5.429722421782	24\\
5.429722421782	25\\
5.43761041767479	25\\
5.43761041767479	26\\
5.66558529637854	26\\
5.66558529637854	27\\
5.73480900927895	27\\
5.73480900927895	28\\
5.73925464209353	28\\
5.73925464209353	29\\
5.98744536828758	29\\
5.98744536828758	30\\
6.07380609905689	30\\
6.07380609905689	31\\
6.10992992470302	31\\
6.10992992470302	32\\
7.43505795450383	32\\
7.43505795450383	33\\
7.85528778352214	33\\
7.85528778352214	34\\
7.94749950533797	34\\
7.94749950533797	35\\
7.95859464648043	35\\
7.95859464648043	36\\
8.02295036137911	36\\
8.02295036137911	37\\
8.09431571065315	37\\
8.09431571065315	38\\
8.10936227008859	38\\
8.10936227008859	39\\
8.25406127760159	39\\
8.25406127760159	40\\
8.44845071464604	40\\
8.44845071464604	41\\
8.7698375167694	41\\
8.7698375167694	42\\
8.97296951153811	42\\
8.97296951153811	43\\
9.28011880238994	43\\
9.28011880238994	44\\
9.32425588041911	44\\
9.32425588041911	45\\
9.50452888856934	45\\
9.50452888856934	46\\
9.66430618756881	46\\
9.66430618756881	47\\
9.98388622032518	47\\
9.98388622032518	48\\
10.3016319682821	48\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.13805632267443	0\\
0.520362635237554	0\\
0.520362635237554	1\\
0.751277689550278	1\\
0.751277689550278	2\\
0.944168569706754	2\\
0.944168569706754	3\\
1.01065462141904	3\\
1.01065462141904	4\\
1.0742229258338	4\\
1.0742229258338	5\\
1.1127499917374	5\\
1.1127499917374	6\\
1.13208698070823	6\\
1.13208698070823	7\\
1.26917411329175	7\\
1.26917411329175	8\\
1.53987679385564	8\\
1.53987679385564	9\\
1.80782261359723	9\\
1.80782261359723	10\\
2.05162665013131	10\\
2.05162665013131	11\\
2.13168678952879	11\\
2.13168678952879	12\\
2.64911271438323	12\\
2.64911271438323	13\\
2.79501976912344	13\\
2.79501976912344	14\\
3.16035302023854	14\\
3.16035302023854	15\\
3.16281306220482	15\\
3.16281306220482	16\\
3.31462742090495	16\\
3.31462742090495	17\\
3.73592018854163	17\\
3.73592018854163	18\\
3.76683542610316	18\\
3.76683542610316	19\\
3.89895610572754	19\\
3.89895610572754	20\\
4.01342467345392	20\\
4.01342467345392	21\\
4.21148853111927	21\\
4.21148853111927	22\\
4.37456828456886	22\\
4.37456828456886	23\\
5.13768435417731	23\\
5.13768435417731	24\\
5.37942158128146	24\\
5.37942158128146	25\\
5.41368253278581	25\\
5.41368253278581	26\\
5.49759920959367	26\\
5.49759920959367	27\\
5.78674837842244	27\\
5.78674837842244	28\\
6.0882821689753	28\\
6.0882821689753	29\\
6.30256445048543	29\\
6.30256445048543	30\\
6.56240278024153	30\\
6.56240278024153	31\\
6.66430267201174	31\\
6.66430267201174	32\\
6.7720579585485	32\\
6.7720579585485	33\\
7.12402671813674	33\\
7.12402671813674	34\\
7.25240953592431	34\\
7.25240953592431	35\\
7.59198682001177	35\\
7.59198682001177	36\\
7.74424639630284	36\\
7.74424639630284	37\\
7.80458037872103	37\\
7.80458037872103	38\\
7.86648473723669	38\\
7.86648473723669	39\\
7.87559247054052	39\\
7.87559247054052	40\\
7.89981497126804	40\\
7.89981497126804	41\\
7.97352713984744	41\\
7.97352713984744	42\\
8.07470670704364	42\\
8.07470670704364	43\\
8.16219350829638	43\\
8.16219350829638	44\\
8.18958136778277	44\\
8.18958136778277	45\\
8.28729147295439	45\\
8.28729147295439	46\\
8.44810872291107	46\\
8.44810872291107	47\\
8.45596298844124	47\\
8.45596298844124	48\\
8.94220380640373	48\\
8.94220380640373	49\\
9.56158581600588	49\\
9.56158581600588	50\\
9.59006677607266	50\\
9.59006677607266	51\\
9.5910391589915	52\\
9.63827155850837	52\\
9.63827155850837	53\\
9.77022047773352	53\\
9.77022047773352	54\\
9.77834073594828	54\\
9.77834073594828	55\\
10.0086556784203	55\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.14052592909006	0\\
0.144229619755393	0\\
0.144229619755393	1\\
0.152104214729903	1\\
0.152104214729903	2\\
0.756386966291025	2\\
0.756386966291025	3\\
0.829478888770595	3\\
0.829478888770595	4\\
0.858408721314987	4\\
0.858408721314987	5\\
0.906689126367347	5\\
0.906689126367347	6\\
0.967844154852102	6\\
0.967844154852102	7\\
1.50148065364557	7\\
1.50148065364557	8\\
1.54834503230125	8\\
1.54834503230125	9\\
2.39551750158186	9\\
2.39551750158186	10\\
2.43480908363124	10\\
2.43480908363124	11\\
2.7178704121719	11\\
2.7178704121719	12\\
2.72474051919755	12\\
2.72474051919755	13\\
2.79451328461347	13\\
2.79451328461347	14\\
2.91383730073265	14\\
2.91383730073265	15\\
2.99557100567871	15\\
2.99557100567871	16\\
3.00838113548333	16\\
3.00838113548333	17\\
3.15323360888394	17\\
3.15323360888394	18\\
3.59219928225665	18\\
3.59219928225665	19\\
3.91432266697457	19\\
3.91432266697457	20\\
4.07244256479534	20\\
4.07244256479534	21\\
4.10369800819056	21\\
4.10369800819056	22\\
4.20179420567377	22\\
4.20179420567377	23\\
4.40706096315415	23\\
4.40706096315415	24\\
4.42821901450993	24\\
4.42821901450993	25\\
4.56078986998703	25\\
4.56078986998703	26\\
5.2085591262429	26\\
5.2085591262429	27\\
5.50331594477414	27\\
5.50331594477414	28\\
5.5312252164088	28\\
5.5312252164088	29\\
6.47911326095082	29\\
6.47911326095082	30\\
6.68633702685349	30\\
6.68633702685349	31\\
6.89379772447711	31\\
6.89379772447711	32\\
7.01043534589026	32\\
7.01043534589026	33\\
7.2588921690914	33\\
7.2588921690914	34\\
7.45074191321916	34\\
7.45074191321916	35\\
7.50997352553995	35\\
7.50997352553995	36\\
7.56861738145378	36\\
7.56861738145378	37\\
7.6003025204721	37\\
7.6003025204721	38\\
7.69265254646012	38\\
7.69265254646012	39\\
7.70121077163265	39\\
7.70121077163265	40\\
7.70473815948578	40\\
7.70473815948578	41\\
8.02254219885403	41\\
8.02254219885403	42\\
8.13844009673493	42\\
8.13844009673493	43\\
8.23016359020529	43\\
8.23016359020529	44\\
8.5301137974561	44\\
8.5301137974561	45\\
8.79695870179098	45\\
8.79695870179098	46\\
9.06623644016691	46\\
9.06623644016691	47\\
9.21990977540801	47\\
9.21990977540801	48\\
9.36935843104224	48\\
9.36935843104224	49\\
9.50100670793404	49\\
9.50100670793404	50\\
9.77005007897976	50\\
9.77005007897976	51\\
9.82710556639132	51\\
9.82710556639132	52\\
9.99147072548028	52\\
9.99147072548028	53\\
10.0823792556217	53\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.120474602666889	0\\
0.27032413819574	0\\
0.27032413819574	1\\
0.392474376632045	1\\
0.392474376632045	2\\
1.25050151126839	2\\
1.25050151126839	3\\
1.54370176211395	3\\
1.54370176211395	4\\
1.60849927559373	4\\
1.60849927559373	5\\
2.33472695451048	5\\
2.33472695451048	6\\
2.52691606697923	6\\
2.52691606697923	7\\
2.63371661817153	7\\
2.63371661817153	8\\
2.90838808405397	8\\
2.90838808405397	9\\
3.1240274990407	9\\
3.1240274990407	10\\
3.43312933706155	10\\
3.43312933706155	11\\
3.84992726610695	11\\
3.84992726610695	12\\
3.85747024128256	12\\
3.85747024128256	13\\
4.01866083234339	13\\
4.01866083234339	14\\
4.01881133905506	15\\
4.48158689183538	15\\
4.48158689183538	16\\
4.63515583957482	16\\
4.63515583957482	17\\
4.96883357910345	17\\
4.96883357910345	18\\
5.13314877158598	18\\
5.13314877158598	19\\
5.49678041695378	19\\
5.49678041695378	20\\
5.57764215595439	20\\
5.57764215595439	21\\
5.77969551085368	21\\
5.77969551085368	22\\
6.14655339505642	22\\
6.14655339505642	23\\
6.3340535864475	23\\
6.3340535864475	24\\
6.36960754347774	24\\
6.36960754347774	25\\
6.84980507543736	25\\
6.84980507543736	26\\
7.21747590496266	26\\
7.21747590496266	27\\
7.23448181808285	27\\
7.23448181808285	28\\
7.24364239339083	28\\
7.24364239339083	29\\
7.54896183133213	29\\
7.54896183133213	30\\
7.8081897852757	30\\
7.8081897852757	31\\
7.95312634410624	31\\
7.95312634410624	32\\
8.35786979705467	32\\
8.35786979705467	33\\
8.5163314464632	33\\
8.5163314464632	34\\
8.58282176158222	34\\
8.58282176158222	35\\
8.85708783723831	35\\
8.85708783723831	36\\
9.0514195408867	36\\
9.0514195408867	37\\
9.16905043550737	37\\
9.16905043550737	38\\
9.228496404489	38\\
9.228496404489	39\\
9.40849209320744	39\\
9.40849209320744	40\\
9.41679603835383	40\\
9.41679603835383	41\\
9.6114790403818	41\\
9.6114790403818	42\\
9.76725358537082	42\\
9.76725358537082	43\\
9.99133809450434	43\\
9.99133809450434	44\\
10.1868176428923	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.040168924325144	0\\
0.137155209773532	0\\
0.137155209773532	1\\
0.376122072219296	1\\
0.376122072219296	2\\
0.406150832963192	2\\
0.406150832963192	3\\
0.548160592792222	3\\
0.548160592792222	4\\
0.77170222366918	4\\
0.77170222366918	5\\
0.938541005099118	5\\
0.938541005099118	6\\
1.00377883610233	6\\
1.00377883610233	7\\
1.08479698697663	7\\
1.08479698697663	8\\
1.41328454609886	8\\
1.41328454609886	9\\
1.61895505214255	9\\
1.61895505214255	10\\
1.78764274140232	10\\
1.78764274140232	11\\
2.32132589425921	11\\
2.32132589425921	12\\
2.854119399174	12\\
2.854119399174	13\\
3.398445012945	13\\
3.398445012945	14\\
3.81745543263683	14\\
3.81745543263683	15\\
3.89656358276676	15\\
3.89656358276676	16\\
4.19827935950908	16\\
4.19827935950908	17\\
4.59002236942374	17\\
4.59002236942374	18\\
4.89147171919898	18\\
4.89147171919898	19\\
5.12531924925946	19\\
5.12531924925946	20\\
5.31561200676207	20\\
5.31561200676207	21\\
5.32932263059761	21\\
5.32932263059761	22\\
5.46938510430606	22\\
5.46938510430606	23\\
5.83062414168191	23\\
5.83062414168191	24\\
6.07220823380397	24\\
6.07220823380397	25\\
6.09381218564712	25\\
6.09381218564712	26\\
6.15820040431586	26\\
6.15820040431586	27\\
6.40276610287071	27\\
6.40276610287071	28\\
7.0361383418095	28\\
7.0361383418095	29\\
7.59594855022009	29\\
7.59594855022009	30\\
7.82458573604257	30\\
7.82458573604257	31\\
7.98110814896924	31\\
7.98110814896924	32\\
8.24632946750358	32\\
8.24632946750358	33\\
8.64370241008827	33\\
8.64370241008827	34\\
8.69598945416754	34\\
8.69598945416754	35\\
9.46136359112677	35\\
9.46136359112677	36\\
10.1683608402325	36\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.504269948147325	0\\
0.69498739769714	0\\
0.69498739769714	1\\
0.777834480509739	1\\
0.777834480509739	2\\
0.925952851836996	2\\
0.925952851836996	3\\
0.986557005628868	3\\
0.986557005628868	4\\
1.25866860473281	4\\
1.25866860473281	5\\
1.43562304011326	5\\
1.43562304011326	6\\
1.44890298390256	6\\
1.44890298390256	7\\
1.54007076081302	7\\
1.54007076081302	8\\
1.89237353745125	8\\
1.89237353745125	9\\
1.98137323492733	9\\
1.98137323492733	10\\
2.03196032697188	10\\
2.03196032697188	11\\
2.12835282020858	11\\
2.12835282020858	12\\
2.38675826758222	12\\
2.38675826758222	13\\
2.50638623628191	13\\
2.50638623628191	14\\
2.6383231525196	14\\
2.6383231525196	15\\
2.6407874322122	15\\
2.6407874322122	16\\
2.7540603944873	16\\
2.7540603944873	17\\
2.7582782167859	17\\
2.7582782167859	18\\
2.83249908729832	18\\
2.83249908729832	19\\
2.85995899878059	19\\
2.85995899878059	20\\
3.06631840212076	20\\
3.06631840212076	21\\
4.05380067763544	21\\
4.05380067763544	22\\
4.0975445244163	22\\
4.0975445244163	23\\
4.36755955618316	23\\
4.36755955618316	24\\
4.45073581566389	24\\
4.45073581566389	25\\
4.82425348605526	25\\
4.82425348605526	26\\
4.91686541299179	26\\
4.91686541299179	27\\
5.32918121195424	27\\
5.32918121195424	28\\
5.35095667923697	28\\
5.35095667923697	29\\
5.40277118469996	29\\
5.40277118469996	30\\
5.42511717841037	30\\
5.42511717841037	31\\
5.51713545710001	31\\
5.51713545710001	32\\
5.8893573995331	32\\
5.8893573995331	33\\
5.96330862169014	33\\
5.96330862169014	34\\
6.20343538380943	34\\
6.20343538380943	35\\
6.34348354446482	35\\
6.34348354446482	36\\
6.42847227698495	36\\
6.42847227698495	37\\
6.49296298007382	37\\
6.49296298007382	38\\
6.58377760073838	38\\
6.58377760073838	39\\
6.67276492963677	39\\
6.67276492963677	40\\
7.28056402707666	40\\
7.28056402707666	41\\
7.34384940283502	41\\
7.34384940283502	42\\
7.38956867495892	42\\
7.38956867495892	43\\
7.54165324454791	43\\
7.54165324454791	44\\
7.9775654882887	44\\
7.9775654882887	45\\
8.1194665487236	45\\
8.1194665487236	46\\
8.25174895607437	46\\
8.25174895607437	47\\
9.00294724187471	47\\
9.00294724187471	48\\
9.13405082865185	48\\
9.13405082865185	49\\
9.22756900062886	49\\
9.22756900062886	50\\
9.35110820378184	50\\
9.35110820378184	51\\
9.36247673237965	51\\
9.36247673237965	52\\
9.37085924442199	52\\
9.37085924442199	53\\
9.47269260485346	53\\
9.47269260485346	54\\
9.98317185251822	54\\
9.98317185251822	55\\
10.4190549181429	55\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.20479366885067	0\\
0.209937586396236	0\\
0.209937586396236	1\\
0.267151306895556	1\\
0.267151306895556	2\\
0.350319627367789	2\\
0.350319627367789	3\\
2.04848653833476	3\\
2.04848653833476	4\\
2.38467493039079	4\\
2.38467493039079	5\\
2.59734145514298	5\\
2.59734145514298	6\\
2.83496766508182	6\\
2.83496766508182	7\\
3.3652882700669	7\\
3.3652882700669	8\\
3.72893129440143	8\\
3.72893129440143	9\\
4.16346847460233	9\\
4.16346847460233	10\\
4.30012886876928	10\\
4.30012886876928	11\\
4.66175553798793	11\\
4.66175553798793	12\\
4.84103659340398	12\\
4.84103659340398	13\\
5.07470797314058	13\\
5.07470797314058	14\\
5.08723145009006	14\\
5.08723145009006	15\\
5.35083370950191	15\\
5.35083370950191	16\\
5.74456449860049	16\\
5.74456449860049	17\\
5.79675567632172	17\\
5.79675567632172	18\\
6.07174886636791	18\\
6.07174886636791	19\\
6.55224643381894	19\\
6.55224643381894	20\\
6.66763808193088	20\\
6.66763808193088	21\\
6.86369731184396	21\\
6.86369731184396	22\\
7.67623450697862	22\\
7.67623450697862	23\\
8.00772037677102	23\\
8.00772037677102	24\\
8.04640633345387	24\\
8.04640633345387	25\\
8.07270349009342	25\\
8.07270349009342	26\\
8.36801878235382	26\\
8.36801878235382	27\\
8.43104117976417	27\\
8.43104117976417	28\\
8.55167445494543	28\\
8.55167445494543	29\\
9.00378536566111	29\\
9.00378536566111	30\\
9.47808040764984	30\\
9.47808040764984	31\\
9.92045612807307	31\\
9.92045612807307	32\\
10.0969435807843	32\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0655002917338479	0\\
0.092014947744282	0\\
0.092014947744282	1\\
0.206506480433966	1\\
0.206506480433966	2\\
0.704830220636069	2\\
0.704830220636069	3\\
0.899943672030595	3\\
0.899943672030595	4\\
0.951766735745053	4\\
0.951766735745053	5\\
1.15565197054836	5\\
1.15565197054836	6\\
1.17414712842253	6\\
1.17414712842253	7\\
1.69316559588552	7\\
1.69316559588552	8\\
1.72740124741343	8\\
1.72740124741343	9\\
1.75291072262009	9\\
1.75291072262009	10\\
1.75930961055327	10\\
1.75930961055327	11\\
1.84162732115205	11\\
1.84162732115205	12\\
2.05337737985901	12\\
2.05337737985901	13\\
2.2933340585804	13\\
2.2933340585804	14\\
2.34511820441296	14\\
2.34511820441296	15\\
2.47022222248169	15\\
2.47022222248169	16\\
2.51499257921659	16\\
2.51499257921659	17\\
2.84295014693895	17\\
2.84295014693895	18\\
2.94061681934345	18\\
2.94061681934345	19\\
3.01107809880224	19\\
3.01107809880224	20\\
3.367169671497	20\\
3.367169671497	21\\
3.46567787481808	21\\
3.46567787481808	22\\
3.52630774112358	22\\
3.52630774112358	23\\
3.87130960737885	23\\
3.87130960737885	24\\
4.48751881076237	24\\
4.48751881076237	25\\
4.63301656791545	25\\
4.63301656791545	26\\
4.73769987943052	26\\
4.73769987943052	27\\
4.85837092537212	27\\
4.85837092537212	28\\
5.03025763441779	28\\
5.03025763441779	29\\
5.2529602057548	29\\
5.2529602057548	30\\
5.25322879661593	31\\
5.27653834103655	31\\
5.27653834103655	32\\
5.45313075378886	32\\
5.45313075378886	33\\
5.56401103762509	33\\
5.56401103762509	34\\
5.66234212602663	34\\
5.66234212602663	35\\
6.10583697398404	35\\
6.10583697398404	36\\
6.16113529085315	36\\
6.16113529085315	37\\
6.2583291482277	37\\
6.2583291482277	38\\
6.27957024689713	38\\
6.27957024689713	39\\
6.44869928930898	39\\
6.44869928930898	40\\
6.59834639846711	40\\
6.59834639846711	41\\
6.99249396437198	41\\
6.99249396437198	42\\
7.36315130300554	42\\
7.36315130300554	43\\
7.37174680902358	43\\
7.37174680902358	44\\
7.48684263860157	44\\
7.48684263860157	45\\
7.55072764097936	45\\
7.55072764097936	46\\
7.80102624722547	46\\
7.80102624722547	47\\
7.99875835622207	47\\
7.99875835622207	48\\
8.27789418398486	48\\
8.27789418398486	49\\
8.53252603052876	49\\
8.53252603052876	50\\
9.04982697329496	50\\
9.04982697329496	51\\
9.11745598850565	51\\
9.11745598850565	52\\
9.16769672091857	52\\
9.16769672091857	53\\
9.23331216428539	53\\
9.23331216428539	54\\
10.3884282232264	54\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0831856729841292	0\\
0.278162981771402	0\\
0.278162981771402	1\\
0.2978134905876	1\\
0.2978134905876	2\\
0.51699590076155	2\\
0.51699590076155	3\\
0.704417675171804	3\\
0.704417675171804	4\\
0.71186973617921	4\\
0.71186973617921	5\\
0.752673696928007	5\\
0.752673696928007	6\\
0.986826409037945	6\\
0.986826409037945	7\\
2.0510274834716	7\\
2.0510274834716	8\\
2.11353635029967	8\\
2.11353635029967	9\\
2.19395762873795	9\\
2.19395762873795	10\\
2.85740498105815	10\\
2.85740498105815	11\\
3.35974355508836	11\\
3.35974355508836	12\\
3.46879239116834	12\\
3.46879239116834	13\\
3.51658551939677	13\\
3.51658551939677	14\\
3.69094287436651	14\\
3.69094287436651	15\\
3.97226954206477	15\\
3.97226954206477	16\\
4.01847594012518	16\\
4.01847594012518	17\\
4.39074542956769	17\\
4.39074542956769	18\\
4.4343040128237	18\\
4.4343040128237	19\\
4.82559307313383	19\\
4.82559307313383	20\\
5.0680782281919	20\\
5.0680782281919	21\\
5.07725909261757	21\\
5.07725909261757	22\\
5.15369452789178	22\\
5.15369452789178	23\\
5.45875476209869	23\\
5.45875476209869	24\\
5.51010224240064	24\\
5.51010224240064	25\\
5.66232085729237	25\\
5.66232085729237	26\\
5.67992881518978	26\\
5.67992881518978	27\\
5.92663790061675	27\\
5.92663790061675	28\\
5.9587981021632	28\\
5.9587981021632	29\\
6.59321429186159	29\\
6.59321429186159	30\\
7.41497760829105	30\\
7.41497760829105	31\\
7.53252007468147	31\\
7.53252007468147	32\\
7.90248050527385	32\\
7.90248050527385	33\\
8.07668867787891	33\\
8.07668867787891	34\\
8.17501610807168	34\\
8.17501610807168	35\\
8.62168564855171	35\\
8.62168564855171	36\\
9.05168950181474	36\\
9.05168950181474	37\\
9.06165370817519	37\\
9.06165370817519	38\\
9.08539470461252	38\\
9.08539470461252	39\\
10.0753799008139	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0969748821689933	0\\
0.369392490420175	0\\
0.369392490420175	1\\
0.386037710260112	1\\
0.386037710260112	2\\
0.526213624076021	2\\
0.526213624076021	3\\
0.539916579309981	3\\
0.539916579309981	4\\
0.656727184402776	4\\
0.656727184402776	5\\
0.775185814840015	5\\
0.775185814840015	6\\
1.10142783413853	6\\
1.10142783413853	7\\
1.26430473637944	7\\
1.26430473637944	8\\
1.44981945376518	8\\
1.44981945376518	9\\
1.47654093897632	9\\
1.47654093897632	10\\
1.66056160761828	10\\
1.66056160761828	11\\
1.68298093555345	11\\
1.68298093555345	12\\
2.06565278254752	12\\
2.06565278254752	13\\
2.19370694119738	13\\
2.19370694119738	14\\
2.20933790047525	14\\
2.20933790047525	15\\
2.30857505010696	15\\
2.30857505010696	16\\
2.32657742542813	16\\
2.32657742542813	17\\
2.49205577392831	17\\
2.49205577392831	18\\
2.53859778607618	18\\
2.53859778607618	19\\
2.56333594296056	19\\
2.56333594296056	20\\
2.5994160331845	20\\
2.5994160331845	21\\
2.79308997672305	21\\
2.79308997672305	22\\
3.38878451159501	22\\
3.38878451159501	23\\
3.44534204507819	23\\
3.44534204507819	24\\
3.60888940066888	24\\
3.60888940066888	25\\
4.0016385110082	25\\
4.0016385110082	26\\
4.43746818863696	26\\
4.43746818863696	27\\
4.45103101634547	27\\
4.45103101634547	28\\
4.49168572167035	28\\
4.49168572167035	29\\
4.53475632805744	29\\
4.53475632805744	30\\
4.57409372641611	30\\
4.57409372641611	31\\
4.75178598292072	31\\
4.75178598292072	32\\
4.79826359295846	32\\
4.79826359295846	33\\
5.41891428010004	33\\
5.41891428010004	34\\
5.48945989136836	34\\
5.48945989136836	35\\
5.82661695141879	35\\
5.82661695141879	36\\
5.90537452657689	36\\
5.90537452657689	37\\
5.91316316057273	37\\
5.91316316057273	38\\
6.75553664493274	38\\
6.75553664493274	39\\
7.25408611320197	39\\
7.25408611320197	40\\
7.37013345133875	40\\
7.37013345133875	41\\
7.38479003674701	41\\
7.38479003674701	42\\
8.41509342866556	42\\
8.41509342866556	43\\
8.53814024154163	43\\
8.53814024154163	44\\
8.74345187962302	44\\
8.74345187962302	45\\
8.82459288586571	45\\
8.82459288586571	46\\
9.47557002576083	46\\
9.47557002576083	47\\
9.53083393719077	47\\
9.53083393719077	48\\
9.59723273312155	48\\
9.59723273312155	49\\
9.75335877562606	49\\
9.75335877562606	50\\
9.99755872523293	50\\
9.99755872523293	51\\
10.019993718716	51\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.708781963294516	0\\
1.8785607818619	0\\
1.8785607818619	1\\
1.97331546421244	1\\
1.97331546421244	2\\
2.17713082850634	2\\
2.17713082850634	3\\
2.28650278259587	3\\
2.28650278259587	4\\
2.30653969585182	4\\
2.30653969585182	5\\
2.88940057479498	5\\
2.88940057479498	6\\
3.32417139171332	6\\
3.32417139171332	7\\
3.58087837935292	7\\
3.58087837935292	8\\
3.64597534680668	8\\
3.64597534680668	9\\
3.71141754630045	9\\
3.71141754630045	10\\
4.33830289045655	10\\
4.33830289045655	11\\
4.36870018432222	11\\
4.36870018432222	12\\
5.84845247727618	12\\
5.84845247727618	13\\
5.91646497281126	13\\
5.91646497281126	14\\
6.04457117906088	14\\
6.04457117906088	15\\
6.64820802077807	15\\
6.64820802077807	16\\
6.8351209976841	16\\
6.8351209976841	17\\
7.43444447197292	17\\
7.43444447197292	18\\
7.89860165496689	18\\
7.89860165496689	19\\
7.91461831990938	19\\
7.91461831990938	20\\
8.09029488027475	20\\
8.09029488027475	21\\
8.71524242606886	21\\
8.71524242606886	22\\
9.09614629382353	22\\
9.09614629382353	23\\
9.1153316826415	23\\
9.1153316826415	24\\
9.53706268658082	24\\
9.53706268658082	25\\
10.0553106185875	25\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.28850086551563	0\\
0.549308869894332	0\\
0.549308869894332	1\\
0.913116567024801	1\\
0.913116567024801	2\\
1.05528799289145	2\\
1.05528799289145	3\\
1.46136074860464	3\\
1.46136074860464	4\\
1.79838459409826	4\\
1.79838459409826	5\\
1.82435456425569	5\\
1.82435456425569	6\\
1.89309253529226	6\\
1.89309253529226	7\\
2.18075292632514	7\\
2.18075292632514	8\\
2.2089759738474	8\\
2.2089759738474	9\\
2.24218639666318	9\\
2.24218639666318	10\\
2.24967071486604	10\\
2.24967071486604	11\\
2.32247629062812	11\\
2.32247629062812	12\\
2.33174317941237	12\\
2.33174317941237	13\\
2.38085223525153	13\\
2.38085223525153	14\\
2.41278285783145	14\\
2.41278285783145	15\\
3.05846630546373	15\\
3.05846630546373	16\\
3.45101303266273	16\\
3.45101303266273	17\\
3.53670215461165	17\\
3.53670215461165	18\\
4.02959103607292	18\\
4.02959103607292	19\\
4.69973435417527	19\\
4.69973435417527	20\\
4.77966014232418	20\\
4.77966014232418	21\\
4.82192190846889	21\\
4.82192190846889	22\\
4.88250509957621	22\\
4.88250509957621	23\\
4.94401517854049	23\\
4.94401517854049	24\\
5.27535085343395	24\\
5.27535085343395	25\\
5.65210081370849	25\\
5.65210081370849	26\\
5.84175153696143	26\\
5.84175153696143	27\\
5.88424611690447	27\\
5.88424611690447	28\\
6.20658290772123	28\\
6.20658290772123	29\\
6.21774038405247	29\\
6.21774038405247	30\\
7.91087464779191	30\\
7.91087464779191	31\\
8.16571574565147	31\\
8.16571574565147	32\\
8.55082151674518	32\\
8.55082151674518	33\\
8.78434477247291	33\\
8.78434477247291	34\\
9.48623818795654	34\\
9.48623818795654	35\\
10.0236938590236	35\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.205215726250962	0\\
0.3680410776686	0\\
0.3680410776686	1\\
0.541382296746832	1\\
0.541382296746832	2\\
0.604849540802213	2\\
0.604849540802213	3\\
0.666194245885869	3\\
0.666194245885869	4\\
1.02962894274854	4\\
1.02962894274854	5\\
1.26873241197004	5\\
1.26873241197004	6\\
1.60633732579772	6\\
1.60633732579772	7\\
1.67026832226379	7\\
1.67026832226379	8\\
1.76507124554581	8\\
1.76507124554581	9\\
1.84645183177438	9\\
1.84645183177438	10\\
2.08829314836641	10\\
2.08829314836641	11\\
2.6152109249062	11\\
2.6152109249062	12\\
2.78877462375291	12\\
2.78877462375291	13\\
3.18861082897261	13\\
3.18861082897261	14\\
3.43040105590287	14\\
3.43040105590287	15\\
3.49455804795366	15\\
3.49455804795366	16\\
3.79780813833153	16\\
3.79780813833153	17\\
3.88327339386736	17\\
3.88327339386736	18\\
3.88960631638323	18\\
3.88960631638323	19\\
4.36804860252859	19\\
4.36804860252859	20\\
4.44781507807699	20\\
4.44781507807699	21\\
4.61332297997089	21\\
4.61332297997089	22\\
4.68643048247908	22\\
4.68643048247908	23\\
5.00684202712176	23\\
5.00684202712176	24\\
5.37438389626064	24\\
5.37438389626064	25\\
6.30552599529103	25\\
6.30552599529103	26\\
6.3319006674025	26\\
6.3319006674025	27\\
7.26715473994144	27\\
7.26715473994144	28\\
7.27201359519768	28\\
7.27201359519768	29\\
7.68215539103914	29\\
7.68215539103914	30\\
8.12286157681921	30\\
8.12286157681921	31\\
8.2178603651985	31\\
8.2178603651985	32\\
9.08790069308878	32\\
9.08790069308878	33\\
9.14452204512521	33\\
9.14452204512521	34\\
9.21362935620016	34\\
9.21362935620016	35\\
9.22261386826943	35\\
9.22261386826943	36\\
9.54675189293431	36\\
9.54675189293431	37\\
9.71734642747212	37\\
9.71734642747212	38\\
9.72404152289141	38\\
9.72404152289141	39\\
9.83000431889167	39\\
9.83000431889167	40\\
9.92148911936336	40\\
9.92148911936336	41\\
10.0501035498839	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.067018118005727	0\\
0.25258996175377	0\\
0.25258996175377	1\\
0.303443993962802	1\\
0.303443993962802	2\\
0.375529326695833	2\\
0.375529326695833	3\\
0.837685374260765	3\\
0.837685374260765	4\\
1.07902555279712	4\\
1.07902555279712	5\\
1.22383028300555	5\\
1.22383028300555	6\\
1.34545267135	6\\
1.34545267135	7\\
1.5025301958435	7\\
1.5025301958435	8\\
1.81080281162973	8\\
1.81080281162973	9\\
2.00716693474745	9\\
2.00716693474745	10\\
2.07724400441491	10\\
2.07724400441491	11\\
2.53397932697405	11\\
2.53397932697405	12\\
2.55616108171347	12\\
2.55616108171347	13\\
2.95660720995473	13\\
2.95660720995473	14\\
3.29884699614281	14\\
3.29884699614281	15\\
3.36944727846542	15\\
3.36944727846542	16\\
3.64786994133457	16\\
3.64786994133457	17\\
3.87812752014226	17\\
3.87812752014226	18\\
4.17703708729682	18\\
4.17703708729682	19\\
4.5034353114158	19\\
4.5034353114158	20\\
4.55562828811976	20\\
4.55562828811976	21\\
4.57176330490231	21\\
4.57176330490231	22\\
5.13833441877278	22\\
5.13833441877278	23\\
5.38480385056734	23\\
5.38480385056734	24\\
5.59862771730484	24\\
5.59862771730484	25\\
5.7536785701845	25\\
5.7536785701845	26\\
5.85398228736059	26\\
5.85398228736059	27\\
6.05284634381461	27\\
6.05284634381461	28\\
6.23275729478943	28\\
6.23275729478943	29\\
6.39212757152072	29\\
6.39212757152072	30\\
6.65027327138867	30\\
6.65027327138867	31\\
7.5319348979111	31\\
7.5319348979111	32\\
7.69193426425387	32\\
7.69193426425387	33\\
7.70863847539719	33\\
7.70863847539719	34\\
8.33806249545058	34\\
8.33806249545058	35\\
8.51297650915122	35\\
8.51297650915122	36\\
8.74072858269685	36\\
8.74072858269685	37\\
9.41627982769086	37\\
9.41627982769086	38\\
9.69702728412872	38\\
9.69702728412872	39\\
9.95800566104561	39\\
9.95800566104561	40\\
10.3209071914515	40\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.132858119841302	0\\
0.215754219721369	0\\
0.215754219721369	1\\
0.52440836768519	1\\
0.52440836768519	2\\
0.986730219542792	2\\
0.986730219542792	3\\
1.49804755796496	3\\
1.49804755796496	4\\
1.91949334488846	4\\
1.91949334488846	5\\
2.1142875799547	5\\
2.1142875799547	6\\
2.50478054920622	6\\
2.50478054920622	7\\
2.72435909072642	7\\
2.72435909072642	8\\
2.76021448227682	8\\
2.76021448227682	9\\
3.00874378377593	9\\
3.00874378377593	10\\
3.0820056264782	10\\
3.0820056264782	11\\
3.10696899000001	11\\
3.10696899000001	12\\
3.15481741466387	12\\
3.15481741466387	13\\
3.33125419105868	13\\
3.33125419105868	14\\
3.42550973229407	14\\
3.42550973229407	15\\
3.81380416155538	15\\
3.81380416155538	16\\
3.97042527109184	16\\
3.97042527109184	17\\
4.36152625972495	17\\
4.36152625972495	18\\
4.44881998718357	18\\
4.44881998718357	19\\
4.57004283098489	19\\
4.57004283098489	20\\
4.80390266719365	20\\
4.80390266719365	21\\
5.03035158362061	21\\
5.03035158362061	22\\
5.39662643870373	22\\
5.39662643870373	23\\
5.47670497035718	23\\
5.47670497035718	24\\
5.73887361945113	24\\
5.73887361945113	25\\
5.77372333640133	25\\
5.77372333640133	26\\
5.81647684334089	26\\
5.81647684334089	27\\
6.15106888097686	27\\
6.15106888097686	28\\
6.27656620861844	28\\
6.27656620861844	29\\
6.47947406229554	29\\
6.47947406229554	30\\
6.77146716811323	30\\
6.77146716811323	31\\
6.83879668745816	31\\
6.83879668745816	32\\
6.91900310224009	32\\
6.91900310224009	33\\
7.30804377710832	33\\
7.30804377710832	34\\
7.4133629586028	34\\
7.4133629586028	35\\
7.8082780884576	35\\
7.8082780884576	36\\
8.2297514015949	36\\
8.2297514015949	37\\
8.62274293456237	37\\
8.62274293456237	38\\
8.66093670222055	38\\
8.66093670222055	39\\
8.7574091239789	39\\
8.7574091239789	40\\
8.8168273390468	40\\
8.8168273390468	41\\
9.47127638408642	41\\
9.47127638408642	42\\
9.58745666731504	42\\
9.58745666731504	43\\
9.89839279852329	43\\
9.89839279852329	44\\
10.0749370112598	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.160136117354291	0\\
0.663101126569302	0\\
0.663101126569302	1\\
1.02998445916212	1\\
1.02998445916212	2\\
1.11933750949983	2\\
1.11933750949983	3\\
1.1194780427367	4\\
1.26976508847	4\\
1.26976508847	5\\
1.50106323148491	5\\
1.50106323148491	6\\
1.5120944389813	6\\
1.5120944389813	7\\
1.71034468491479	7\\
1.71034468491479	8\\
1.7411365372262	8\\
1.7411365372262	9\\
1.77447563443833	9\\
1.77447563443833	10\\
1.94827236386801	10\\
1.94827236386801	11\\
2.49707463014278	11\\
2.49707463014278	12\\
2.56913307357537	12\\
2.56913307357537	13\\
2.62264195883241	13\\
2.62264195883241	14\\
2.79246267644076	14\\
2.79246267644076	15\\
2.92470779267794	15\\
2.92470779267794	16\\
2.98589619526474	16\\
2.98589619526474	17\\
3.19161580887615	17\\
3.19161580887615	18\\
3.24611570374011	18\\
3.24611570374011	19\\
3.25107065918115	19\\
3.25107065918115	20\\
3.29246778532539	20\\
3.29246778532539	21\\
3.44859066668577	21\\
3.44859066668577	22\\
3.57221281102321	22\\
3.57221281102321	23\\
3.62051452812653	23\\
3.62051452812653	24\\
3.72262132198365	24\\
3.72262132198365	25\\
4.03710567174836	25\\
4.03710567174836	26\\
4.30243117527322	26\\
4.30243117527322	27\\
4.66919613762323	27\\
4.66919613762323	28\\
4.82207417264608	28\\
4.82207417264608	29\\
4.97231437594144	29\\
4.97231437594144	30\\
5.2670325219209	30\\
5.2670325219209	31\\
5.38909940961479	31\\
5.38909940961479	32\\
5.53132978246416	32\\
5.53132978246416	33\\
5.54675229878434	33\\
5.54675229878434	34\\
5.68418433667216	34\\
5.68418433667216	35\\
5.81947172792285	35\\
5.81947172792285	36\\
5.94634644673283	36\\
5.94634644673283	37\\
6.32654019753932	37\\
6.32654019753932	38\\
6.54536849081932	38\\
6.54536849081932	39\\
6.55551820701253	39\\
6.55551820701253	40\\
6.99170929955099	40\\
6.99170929955099	41\\
7.01297299851027	41\\
7.01297299851027	42\\
7.60355563838517	42\\
7.60355563838517	43\\
8.0524393826093	43\\
8.0524393826093	44\\
8.35246041809359	44\\
8.35246041809359	45\\
8.65451322828628	45\\
8.65451322828628	46\\
8.66669641491215	46\\
8.66669641491215	47\\
8.80719808047306	47\\
8.80719808047306	48\\
8.81080303484578	48\\
8.81080303484578	49\\
8.93479528153136	49\\
8.93479528153136	50\\
9.06207477682258	50\\
9.06207477682258	51\\
9.210457539869	51\\
9.210457539869	52\\
9.49692961068277	52\\
9.49692961068277	53\\
9.82678337947006	53\\
9.82678337947006	54\\
9.92752330375141	54\\
9.92752330375141	55\\
10.3812651257258	55\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.363260719703518	0\\
0.539281211842329	0\\
0.539281211842329	1\\
0.55685804986652	1\\
0.55685804986652	2\\
0.578014094418386	2\\
0.578014094418386	3\\
0.765623858940153	3\\
0.765623858940153	4\\
1.00765216876867	4\\
1.00765216876867	5\\
1.36494838528157	5\\
1.36494838528157	6\\
1.61307841729003	6\\
1.61307841729003	7\\
1.88309752828228	7\\
1.88309752828228	8\\
2.4773458328213	8\\
2.4773458328213	9\\
2.72970866571437	9\\
2.72970866571437	10\\
2.85554884306652	10\\
2.85554884306652	11\\
2.94327448101846	11\\
2.94327448101846	12\\
3.23851475458696	12\\
3.23851475458696	13\\
3.50921517404216	13\\
3.50921517404216	14\\
3.52881886176593	14\\
3.52881886176593	15\\
3.63467993787006	15\\
3.63467993787006	16\\
3.75672877269631	16\\
3.75672877269631	17\\
3.83922903325342	17\\
3.83922903325342	18\\
4.0842119891684	18\\
4.0842119891684	19\\
4.12992532565286	19\\
4.12992532565286	20\\
4.39073663774628	20\\
4.39073663774628	21\\
4.64065292731379	21\\
4.64065292731379	22\\
4.71387325137459	22\\
4.71387325137459	23\\
4.78372599289631	23\\
4.78372599289631	24\\
5.22992116523369	24\\
5.22992116523369	25\\
5.24679463424206	25\\
5.24679463424206	26\\
5.27495625822795	26\\
5.27495625822795	27\\
5.39680176686207	27\\
5.39680176686207	28\\
5.94935509171206	28\\
5.94935509171206	29\\
6.08299386287457	29\\
6.08299386287457	30\\
6.368920116403	30\\
6.368920116403	31\\
6.86335402567442	31\\
6.86335402567442	32\\
6.97010377373726	32\\
6.97010377373726	33\\
7.04501842749129	33\\
7.04501842749129	34\\
7.24568721996897	34\\
7.24568721996897	35\\
7.27274778265965	35\\
7.27274778265965	36\\
7.42092242868213	36\\
7.42092242868213	37\\
7.51688309036806	37\\
7.51688309036806	38\\
7.77591174243179	38\\
7.77591174243179	39\\
8.0027552555222	39\\
8.0027552555222	40\\
8.09175056879717	40\\
8.09175056879717	41\\
8.26941466195881	41\\
8.26941466195881	42\\
8.87359270106901	42\\
8.87359270106901	43\\
8.8862194928908	43\\
8.8862194928908	44\\
8.91951847400848	44\\
8.91951847400848	45\\
9.66811647833174	45\\
9.66811647833174	46\\
10.130188045236	46\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
1.27063676837648	0\\
1.48129026629721	0\\
1.48129026629721	1\\
1.57496919686388	1\\
1.57496919686388	2\\
1.66574285218366	2\\
1.66574285218366	3\\
1.8866285477496	3\\
1.8866285477496	4\\
2.07964227694972	4\\
2.07964227694972	5\\
2.3062736236074	5\\
2.3062736236074	6\\
2.58952924101457	6\\
2.58952924101457	7\\
2.69009109119145	7\\
2.69009109119145	8\\
2.75786886409785	8\\
2.75786886409785	9\\
3.29278338180396	9\\
3.29278338180396	10\\
3.60470987585235	10\\
3.60470987585235	11\\
3.64984751071734	11\\
3.64984751071734	12\\
3.66963892907415	12\\
3.66963892907415	13\\
4.00814210081027	13\\
4.00814210081027	14\\
4.03711602711363	14\\
4.03711602711363	15\\
4.60864556712725	15\\
4.60864556712725	16\\
4.61290300222215	16\\
4.61290300222215	17\\
4.67724821325913	17\\
4.67724821325913	18\\
4.95036284705661	18\\
4.95036284705661	19\\
5.59236975921619	19\\
5.59236975921619	20\\
5.63564535551215	20\\
5.63564535551215	21\\
5.64253950066511	21\\
5.64253950066511	22\\
6.197122496208	22\\
6.197122496208	23\\
6.88640305632018	23\\
6.88640305632018	24\\
6.99781031278667	24\\
6.99781031278667	25\\
6.9993849327809	26\\
7.09859025634168	26\\
7.09859025634168	27\\
7.20933923009035	27\\
7.20933923009035	28\\
7.79882649227667	28\\
7.79882649227667	29\\
7.89758179093378	29\\
7.89758179093378	30\\
8.0436302651044	30\\
8.0436302651044	31\\
8.05139986949063	31\\
8.05139986949063	32\\
8.06188604543056	32\\
8.06188604543056	33\\
8.07166353837657	33\\
8.07166353837657	34\\
8.73332214657637	34\\
8.73332214657637	35\\
9.23193525528909	35\\
9.23193525528909	36\\
9.29897700966962	36\\
9.29897700966962	37\\
9.88890540632564	37\\
9.88890540632564	38\\
9.89442696358766	38\\
9.89442696358766	39\\
9.9266872608241	39\\
9.9266872608241	40\\
9.96159472096032	40\\
9.96159472096032	41\\
10.051823669702	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.194894567713902	0\\
1.14026651699124	0\\
1.14026651699124	1\\
1.2650916333568	1\\
1.2650916333568	2\\
1.32743302721991	2\\
1.32743302721991	3\\
1.33505592865671	3\\
1.33505592865671	4\\
1.3714066928103	4\\
1.3714066928103	5\\
1.75232788278091	5\\
1.75232788278091	6\\
1.81059115802736	6\\
1.81059115802736	7\\
1.88563278059129	7\\
1.88563278059129	8\\
1.91095578434771	8\\
1.91095578434771	9\\
2.7441980338449	9\\
2.7441980338449	10\\
2.96619436760439	10\\
2.96619436760439	11\\
3.08008697426124	11\\
3.08008697426124	12\\
3.17677942536663	12\\
3.17677942536663	13\\
3.35629244045229	13\\
3.35629244045229	14\\
4.37819913360453	14\\
4.37819913360453	15\\
4.50157990432659	15\\
4.50157990432659	16\\
4.55197996086637	16\\
4.55197996086637	17\\
4.60421480177964	17\\
4.60421480177964	18\\
4.75754390763458	18\\
4.75754390763458	19\\
5.53415167236909	19\\
5.53415167236909	20\\
6.1795768084376	20\\
6.1795768084376	21\\
6.26838722299846	21\\
6.26838722299846	22\\
6.46137574931881	22\\
6.46137574931881	23\\
6.93460563560674	23\\
6.93460563560674	24\\
7.2279199594342	24\\
7.2279199594342	25\\
7.98868125646544	25\\
7.98868125646544	26\\
8.34733589820529	26\\
8.34733589820529	27\\
8.37428810830227	27\\
8.37428810830227	28\\
8.64274808930968	28\\
8.64274808930968	29\\
8.65199593615581	29\\
8.65199593615581	30\\
8.7916516770664	30\\
8.7916516770664	31\\
8.82143679213717	31\\
8.82143679213717	32\\
8.83149852986849	32\\
8.83149852986849	33\\
8.91085477157317	33\\
8.91085477157317	34\\
8.94902681774188	34\\
8.94902681774188	35\\
9.02655883967448	35\\
9.02655883967448	36\\
9.17340485573812	36\\
9.17340485573812	37\\
9.58320946203366	37\\
9.58320946203366	38\\
9.76456006247004	38\\
9.76456006247004	39\\
10.482211881755	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.188190642375289	0\\
0.299971037462207	0\\
0.299971037462207	1\\
0.356609351002867	1\\
0.356609351002867	2\\
0.603254683973354	2\\
0.603254683973354	3\\
0.808292727556761	3\\
0.808292727556761	4\\
0.94252970880099	4\\
0.94252970880099	5\\
1.03026622331997	5\\
1.03026622331997	6\\
1.0959664558297	6\\
1.0959664558297	7\\
1.35411510058155	7\\
1.35411510058155	8\\
1.52385215253576	8\\
1.52385215253576	9\\
1.61796826139585	9\\
1.61796826139585	10\\
1.92593390264859	10\\
1.92593390264859	11\\
2.41846337550481	11\\
2.41846337550481	12\\
2.56552908958326	12\\
2.56552908958326	13\\
2.58370649237697	13\\
2.58370649237697	14\\
2.70811316221113	14\\
2.70811316221113	15\\
3.56424753736104	15\\
3.56424753736104	16\\
3.79685449591096	16\\
3.79685449591096	17\\
4.39647104622301	17\\
4.39647104622301	18\\
4.42033110496848	18\\
4.42033110496848	19\\
4.57883239022441	19\\
4.57883239022441	20\\
4.84737270952456	20\\
4.84737270952456	21\\
5.3951370729294	21\\
5.3951370729294	22\\
5.70178929308349	22\\
5.70178929308349	23\\
5.83684036931822	23\\
5.83684036931822	24\\
5.99644177932423	24\\
5.99644177932423	25\\
6.20257106149733	25\\
6.20257106149733	26\\
7.18174220399962	26\\
7.18174220399962	27\\
7.20530793700424	27\\
7.20530793700424	28\\
7.23273532147739	28\\
7.23273532147739	29\\
7.43116036658549	29\\
7.43116036658549	30\\
7.44466858861252	30\\
7.44466858861252	31\\
7.49120112459416	31\\
7.49120112459416	32\\
7.66869229268289	32\\
7.66869229268289	33\\
7.8195312102569	33\\
7.8195312102569	34\\
7.98350366961866	34\\
7.98350366961866	35\\
8.13296692729512	35\\
8.13296692729512	36\\
8.65781924857442	36\\
8.65781924857442	37\\
8.89826914423872	37\\
8.89826914423872	38\\
8.94561435901682	38\\
8.94561435901682	39\\
9.30394562653483	39\\
9.30394562653483	40\\
9.91055391823441	40\\
9.91055391823441	41\\
10.0040580214411	41\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.215501317222984	0\\
0.353510947696819	0\\
0.353510947696819	1\\
0.72304793963708	1\\
0.72304793963708	2\\
1.10988210582781	2\\
1.10988210582781	3\\
1.17037843332509	3\\
1.17037843332509	4\\
1.1900229196438	4\\
1.1900229196438	5\\
1.22407687696295	5\\
1.22407687696295	6\\
1.23874904697761	6\\
1.23874904697761	7\\
1.51803949788216	7\\
1.51803949788216	8\\
1.63903585074316	8\\
1.63903585074316	9\\
2.1164476054547	9\\
2.1164476054547	10\\
2.13047776363117	10\\
2.13047776363117	11\\
2.60281383615959	11\\
2.60281383615959	12\\
3.13842583468158	12\\
3.13842583468158	13\\
4.18652661225741	13\\
4.18652661225741	14\\
4.7258277318029	14\\
4.7258277318029	15\\
5.38242650420687	15\\
5.38242650420687	16\\
5.49240042813662	16\\
5.49240042813662	17\\
5.51753605284485	17\\
5.51753605284485	18\\
5.95324175286731	18\\
5.95324175286731	19\\
6.02609184585426	19\\
6.02609184585426	20\\
6.05044338952496	20\\
6.05044338952496	21\\
6.11615085863821	21\\
6.11615085863821	22\\
6.43597757550255	22\\
6.43597757550255	23\\
6.90093112490305	23\\
6.90093112490305	24\\
6.97732892231262	24\\
6.97732892231262	25\\
7.0063178005086	25\\
7.0063178005086	26\\
7.19745635167954	26\\
7.19745635167954	27\\
7.86133530947168	27\\
7.86133530947168	28\\
8.03399178452387	28\\
8.03399178452387	29\\
9.42816444609268	29\\
9.42816444609268	30\\
10.2935389941999	30\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.387340876544911	0\\
0.655761064131163	0\\
0.655761064131163	1\\
0.689907123171338	1\\
0.689907123171338	2\\
0.791957706304032	2\\
0.791957706304032	3\\
0.829650799709825	3\\
0.829650799709825	4\\
0.927602936361794	4\\
0.927602936361794	5\\
1.11896473294514	5\\
1.11896473294514	6\\
1.92552383199757	6\\
1.92552383199757	7\\
2.07132974133338	7\\
2.07132974133338	8\\
2.12177624754463	8\\
2.12177624754463	9\\
2.29232978506273	9\\
2.29232978506273	10\\
2.33453271282514	10\\
2.33453271282514	11\\
2.41123670795395	11\\
2.41123670795395	12\\
3.09793623793489	12\\
3.09793623793489	13\\
3.33831729551694	13\\
3.33831729551694	14\\
3.49878852643104	14\\
3.49878852643104	15\\
3.68639000836931	15\\
3.68639000836931	16\\
4.38994529839979	16\\
4.38994529839979	17\\
4.48516764487146	17\\
4.48516764487146	18\\
4.82445344281833	18\\
4.82445344281833	19\\
4.95851107916287	19\\
4.95851107916287	20\\
5.0764615767088	20\\
5.0764615767088	21\\
5.35517445544232	21\\
5.35517445544232	22\\
5.82083750671119	22\\
5.82083750671119	23\\
6.16094911450658	23\\
6.16094911450658	24\\
6.24789818005183	24\\
6.24789818005183	25\\
6.79811350321386	25\\
6.79811350321386	26\\
7.03261177575052	26\\
7.03261177575052	27\\
7.17890126934732	27\\
7.17890126934732	28\\
7.290652454009	28\\
7.290652454009	29\\
7.73323200626309	29\\
7.73323200626309	30\\
8.1319970851502	30\\
8.1319970851502	31\\
8.17190347326699	31\\
8.17190347326699	32\\
8.52888242673083	32\\
8.52888242673083	33\\
8.67508598381814	33\\
8.67508598381814	34\\
8.7952029558993	34\\
8.7952029558993	35\\
9.13941988559587	35\\
9.13941988559587	36\\
9.15889768692541	36\\
9.15889768692541	37\\
9.37066146640795	37\\
9.37066146640795	38\\
10.2970229712559	38\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.178665822321392	0\\
0.59394660804162	0\\
0.59394660804162	1\\
0.934636003522378	1\\
0.934636003522378	2\\
1.48852975764736	2\\
1.48852975764736	3\\
1.87400541214997	3\\
1.87400541214997	4\\
2.37545187006728	4\\
2.37545187006728	5\\
2.42141129718458	5\\
2.42141129718458	6\\
3.02889055634834	6\\
3.02889055634834	7\\
3.23216676559865	7\\
3.23216676559865	8\\
3.2430737387513	8\\
3.2430737387513	9\\
3.3764359683039	9\\
3.3764359683039	10\\
3.43535207237461	10\\
3.43535207237461	11\\
3.72993705437246	11\\
3.72993705437246	12\\
3.78638882059619	12\\
3.78638882059619	13\\
3.95774618192814	13\\
3.95774618192814	14\\
4.20669073057373	14\\
4.20669073057373	15\\
4.20798041954771	16\\
4.65724409338213	16\\
4.65724409338213	17\\
4.812641785785	17\\
4.812641785785	18\\
4.85352536777016	18\\
4.85352536777016	19\\
4.99713289234774	19\\
4.99713289234774	20\\
5.20701634122851	20\\
5.20701634122851	21\\
5.52103614187128	21\\
5.52103614187128	22\\
5.96487946423081	22\\
5.96487946423081	23\\
6.26296861584555	23\\
6.26296861584555	24\\
6.39340502555249	24\\
6.39340502555249	25\\
6.41556851733452	25\\
6.41556851733452	26\\
6.94576052434686	26\\
6.94576052434686	27\\
6.95226648530072	27\\
6.95226648530072	28\\
7.21904892557703	28\\
7.21904892557703	29\\
7.76620082581624	29\\
7.76620082581624	30\\
7.78646697394424	30\\
7.78646697394424	31\\
7.96674924074806	31\\
7.96674924074806	32\\
7.99547489880867	32\\
7.99547489880867	33\\
8.21860546166189	33\\
8.21860546166189	34\\
8.78039882120607	34\\
8.78039882120607	35\\
8.84740757527804	35\\
8.84740757527804	36\\
9.33416910723038	36\\
9.33416910723038	37\\
9.42384313774841	37\\
9.42384313774841	38\\
9.9417155357185	38\\
9.9417155357185	39\\
10.173339275194	39\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.212950366976827	0\\
0.26307615085021	0\\
0.26307615085021	1\\
0.288099987232926	1\\
0.288099987232926	2\\
0.540504516575723	2\\
0.540504516575723	3\\
0.659936092785372	3\\
0.659936092785372	4\\
1.06628932955479	4\\
1.06628932955479	5\\
1.16643130520561	5\\
1.16643130520561	6\\
1.35530204773843	6\\
1.35530204773843	7\\
1.50373490527544	7\\
1.50373490527544	8\\
1.5475865360109	8\\
1.5475865360109	9\\
1.66232910782013	9\\
1.66232910782013	10\\
2.05435890484775	10\\
2.05435890484775	11\\
2.15410722477265	11\\
2.15410722477265	12\\
2.89225813143493	12\\
2.89225813143493	13\\
3.36387884441599	13\\
3.36387884441599	14\\
3.57228509398365	14\\
3.57228509398365	15\\
4.33749169563554	15\\
4.33749169563554	16\\
4.75372083272274	16\\
4.75372083272274	17\\
4.90788792460304	17\\
4.90788792460304	18\\
5.10234967688367	18\\
5.10234967688367	19\\
5.17715494031169	19\\
5.17715494031169	20\\
5.30252505827033	20\\
5.30252505827033	21\\
5.74402761657313	21\\
5.74402761657313	22\\
5.98944821640278	22\\
5.98944821640278	23\\
6.17162368832361	23\\
6.17162368832361	24\\
6.19698390403348	24\\
6.19698390403348	25\\
6.24499114411516	25\\
6.24499114411516	26\\
6.27556510588749	26\\
6.27556510588749	27\\
6.46331355894721	27\\
6.46331355894721	28\\
6.73548876213989	28\\
6.73548876213989	29\\
7.62504884720689	29\\
7.62504884720689	30\\
7.74294542639996	30\\
7.74294542639996	31\\
7.81665337033262	31\\
7.81665337033262	32\\
8.10257558652894	32\\
8.10257558652894	33\\
8.19651291770981	33\\
8.19651291770981	34\\
8.35384682373537	34\\
8.35384682373537	35\\
8.57750219981213	35\\
8.57750219981213	36\\
8.87174413942576	36\\
8.87174413942576	37\\
8.91291749050547	37\\
8.91291749050547	38\\
8.92120514162247	38\\
8.92120514162247	39\\
9.4903548344608	39\\
9.4903548344608	40\\
9.55730036763691	40\\
9.55730036763691	41\\
9.66750064807843	41\\
9.66750064807843	42\\
9.77129518177722	42\\
9.77129518177722	43\\
9.84080557991255	43\\
9.84080557991255	44\\
10.3902574350091	44\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.475933550547445	0\\
1.07332274020529	0\\
1.07332274020529	1\\
1.09743628468656	1\\
1.09743628468656	2\\
1.19868429168073	2\\
1.19868429168073	3\\
1.66492138349425	3\\
1.66492138349425	4\\
2.56067025484047	4\\
2.56067025484047	5\\
2.75321499866288	5\\
2.75321499866288	6\\
2.80021577671882	6\\
2.80021577671882	7\\
2.91039472501429	7\\
2.91039472501429	8\\
2.9263765921469	8\\
2.9263765921469	9\\
2.96954228973269	9\\
2.96954228973269	10\\
3.02397654794427	10\\
3.02397654794427	11\\
3.03545776671136	11\\
3.03545776671136	12\\
3.36448943200126	12\\
3.36448943200126	13\\
3.56431960459034	13\\
3.56431960459034	14\\
4.09253873142806	14\\
4.09253873142806	15\\
4.30413255088674	15\\
4.30413255088674	16\\
4.32348191402952	16\\
4.32348191402952	17\\
4.63398188354969	17\\
4.63398188354969	18\\
4.65238337698856	18\\
4.65238337698856	19\\
4.88724065009063	19\\
4.88724065009063	20\\
4.95226710797118	20\\
4.95226710797118	21\\
5.02272173101277	21\\
5.02272173101277	22\\
5.20080908195887	22\\
5.20080908195887	23\\
5.69926661561099	23\\
5.69926661561099	24\\
5.83653773844402	24\\
5.83653773844402	25\\
6.08334473095675	25\\
6.08334473095675	26\\
6.3310071484928	26\\
6.3310071484928	27\\
6.62419545845288	27\\
6.62419545845288	28\\
7.308403879303	28\\
7.308403879303	29\\
7.32292942778304	29\\
7.32292942778304	30\\
7.64041084664868	30\\
7.64041084664868	31\\
8.1153296658718	31\\
8.1153296658718	32\\
8.48883284424167	32\\
8.48883284424167	33\\
8.7858634017325	33\\
8.7858634017325	34\\
9.37385961313348	34\\
9.37385961313348	35\\
9.5470839663467	35\\
9.5470839663467	36\\
9.65507797913597	36\\
9.65507797913597	37\\
10.1470786159944	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.141546169266825	0\\
0.28041167970536	0\\
0.28041167970536	1\\
0.789815833941127	1\\
0.789815833941127	2\\
1.01212845443649	2\\
1.01212845443649	3\\
1.11597772256016	3\\
1.11597772256016	4\\
1.51343607075314	4\\
1.51343607075314	5\\
1.62376704041606	5\\
1.62376704041606	6\\
1.63942129446326	6\\
1.63942129446326	7\\
1.65365741713906	7\\
1.65365741713906	8\\
1.72725789549352	8\\
1.72725789549352	9\\
2.35139579998981	9\\
2.35139579998981	10\\
2.86296803486243	10\\
2.86296803486243	11\\
2.91059130577009	11\\
2.91059130577009	12\\
3.14794506222757	12\\
3.14794506222757	13\\
3.30616853655847	13\\
3.30616853655847	14\\
3.37305441092188	14\\
3.37305441092188	15\\
4.19283470956267	15\\
4.19283470956267	16\\
4.25979340013203	16\\
4.25979340013203	17\\
4.47929961476056	17\\
4.47929961476056	18\\
4.88641306815861	18\\
4.88641306815861	19\\
5.11631568878669	19\\
5.11631568878669	20\\
5.69775763860634	20\\
5.69775763860634	21\\
5.73345772491734	21\\
5.73345772491734	22\\
5.82829036918072	22\\
5.82829036918072	23\\
5.8315250047734	23\\
5.8315250047734	24\\
5.99820342735676	24\\
5.99820342735676	25\\
6.16670136412092	25\\
6.16670136412092	26\\
6.68490240629453	26\\
6.68490240629453	27\\
6.79686872969031	27\\
6.79686872969031	28\\
6.82764069600364	28\\
6.82764069600364	29\\
7.04519087207238	29\\
7.04519087207238	30\\
7.09374476995043	30\\
7.09374476995043	31\\
7.18990306327333	31\\
7.18990306327333	32\\
7.87774726439072	32\\
7.87774726439072	33\\
8.043534817127	33\\
8.043534817127	34\\
8.13960074681284	34\\
8.13960074681284	35\\
8.25623541884141	35\\
8.25623541884141	36\\
8.25779165932651	37\\
8.30374043391125	37\\
8.30374043391125	38\\
8.34020810473864	38\\
8.34020810473864	39\\
8.44933367342608	39\\
8.44933367342608	40\\
8.55376295314118	40\\
8.55376295314118	41\\
9.03596930642374	41\\
9.03596930642374	42\\
10.2404404215156	42\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0560092067036635	0\\
0.308805670674396	0\\
0.308805670674396	1\\
0.375843669733833	1\\
0.375843669733833	2\\
1.14166169759449	2\\
1.14166169759449	3\\
1.86437091641852	3\\
1.86437091641852	4\\
1.89661732395096	4\\
1.89661732395096	5\\
2.08264125219223	5\\
2.08264125219223	6\\
2.0893148871185	6\\
2.0893148871185	7\\
2.13061365990764	7\\
2.13061365990764	8\\
2.14185838366845	8\\
2.14185838366845	9\\
2.2660442453882	9\\
2.2660442453882	10\\
2.30466333968146	10\\
2.30466333968146	11\\
2.98528474862843	11\\
2.98528474862843	12\\
3.25540625810145	12\\
3.25540625810145	13\\
3.34996521284522	13\\
3.34996521284522	14\\
3.36611465955652	14\\
3.36611465955652	15\\
3.50557652738348	15\\
3.50557652738348	16\\
3.54170037375685	16\\
3.54170037375685	17\\
4.25770964951864	17\\
4.25770964951864	18\\
4.67786000614609	18\\
4.67786000614609	19\\
4.67827550030073	20\\
4.9364630938934	20\\
4.9364630938934	21\\
5.44610358702915	21\\
5.44610358702915	22\\
5.71449457427926	22\\
5.71449457427926	23\\
5.83840405292852	23\\
5.83840405292852	24\\
5.88449477647144	24\\
5.88449477647144	25\\
6.03599201344659	25\\
6.03599201344659	26\\
6.29129983398411	26\\
6.29129983398411	27\\
6.33025707340297	27\\
6.33025707340297	28\\
6.91214613938241	28\\
6.91214613938241	29\\
7.00841535415793	29\\
7.00841535415793	30\\
7.34944853985496	30\\
7.34944853985496	31\\
7.71128735589954	31\\
7.71128735589954	32\\
7.7936368316348	32\\
7.7936368316348	33\\
8.2720074982077	33\\
8.2720074982077	34\\
8.47939805977719	34\\
8.47939805977719	35\\
8.53772025954175	35\\
8.53772025954175	36\\
8.79670331379966	36\\
8.79670331379966	37\\
8.87445311757278	37\\
8.87445311757278	38\\
9.51564406966089	38\\
9.51564406966089	39\\
9.55404084583215	39\\
9.55404084583215	40\\
9.63654836870889	40\\
9.63654836870889	41\\
9.71025983465201	41\\
9.71025983465201	42\\
9.92298594595482	42\\
9.92298594595482	43\\
9.95705194734862	43\\
9.95705194734862	44\\
9.97478435709819	44\\
9.97478435709819	45\\
10.0903158726348	45\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.357520920847072	0\\
0.403066465744992	0\\
0.403066465744992	1\\
0.55904742534225	1\\
0.55904742534225	2\\
0.713478871576747	2\\
0.713478871576747	3\\
0.806127599282924	3\\
0.806127599282924	4\\
0.834392838483083	4\\
0.834392838483083	5\\
0.92640511125775	5\\
0.92640511125775	6\\
1.36182051268612	6\\
1.36182051268612	7\\
1.47290046356327	7\\
1.47290046356327	8\\
1.80172395088501	8\\
1.80172395088501	9\\
2.4787174350822	9\\
2.4787174350822	10\\
2.67681477524533	10\\
2.67681477524533	11\\
2.70335809902524	11\\
2.70335809902524	12\\
2.75501897553885	12\\
2.75501897553885	13\\
3.12645248839555	13\\
3.12645248839555	14\\
3.56146035127671	14\\
3.56146035127671	15\\
3.65207046123945	15\\
3.65207046123945	16\\
3.65292321362965	17\\
3.86284586229347	17\\
3.86284586229347	18\\
3.98005910283012	18\\
3.98005910283012	19\\
4.15447909123534	19\\
4.15447909123534	20\\
4.24591417910758	20\\
4.24591417910758	21\\
4.25992863568048	21\\
4.25992863568048	22\\
4.60064926947954	22\\
4.60064926947954	23\\
4.64079714564596	23\\
4.64079714564596	24\\
4.71211496297836	24\\
4.71211496297836	25\\
4.98307627481632	25\\
4.98307627481632	26\\
5.37506248623844	26\\
5.37506248623844	27\\
5.86313344460658	27\\
5.86313344460658	28\\
6.02052850281478	28\\
6.02052850281478	29\\
6.12027995357592	29\\
6.12027995357592	30\\
6.2599259359831	30\\
6.2599259359831	31\\
6.56493015204567	31\\
6.56493015204567	32\\
6.63572856517923	32\\
6.63572856517923	33\\
6.71777943979416	33\\
6.71777943979416	34\\
7.16073121691605	34\\
7.16073121691605	35\\
7.40548358065551	35\\
7.40548358065551	36\\
7.5080817485193	36\\
7.5080817485193	37\\
8.01630235622052	37\\
8.01630235622052	38\\
8.06740230397904	38\\
8.06740230397904	39\\
8.13217251578358	39\\
8.13217251578358	40\\
8.57956333748712	40\\
8.57956333748712	41\\
9.18923919266087	41\\
9.18923919266087	42\\
9.91592907807443	42\\
9.91592907807443	43\\
10.356032412586	43\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.323587726619749	0\\
0.408462743063168	0\\
0.408462743063168	1\\
0.89901617460805	1\\
0.89901617460805	2\\
1.09975387783103	2\\
1.09975387783103	3\\
1.37244585259695	3\\
1.37244585259695	4\\
1.8369144044993	4\\
1.8369144044993	5\\
2.00601266084184	5\\
2.00601266084184	6\\
2.26693177264081	6\\
2.26693177264081	7\\
2.38092160067055	7\\
2.38092160067055	8\\
2.46269409133512	8\\
2.46269409133512	9\\
2.48759718908745	9\\
2.48759718908745	10\\
2.54908584614923	10\\
2.54908584614923	11\\
2.71413167168919	11\\
2.71413167168919	12\\
2.78984624822179	12\\
2.78984624822179	13\\
2.83544065080449	13\\
2.83544065080449	14\\
3.01083627409425	14\\
3.01083627409425	15\\
3.28958278877469	15\\
3.28958278877469	16\\
3.51341701859469	16\\
3.51341701859469	17\\
3.55707135044679	17\\
3.55707135044679	18\\
3.62989761186601	18\\
3.62989761186601	19\\
3.82035258879432	19\\
3.82035258879432	20\\
4.13894540618253	20\\
4.13894540618253	21\\
4.16931144639304	21\\
4.16931144639304	22\\
5.01921187698957	22\\
5.01921187698957	23\\
5.02518090693078	23\\
5.02518090693078	24\\
5.31462671814187	24\\
5.31462671814187	25\\
5.46265998453483	25\\
5.46265998453483	26\\
5.59278284287861	26\\
5.59278284287861	27\\
5.65083410914178	27\\
5.65083410914178	28\\
5.75989716197853	28\\
5.75989716197853	29\\
6.04575213245032	29\\
6.04575213245032	30\\
6.41597352465478	30\\
6.41597352465478	31\\
6.44953734585877	31\\
6.44953734585877	32\\
6.55364539933623	32\\
6.55364539933623	33\\
6.61047949542329	33\\
6.61047949542329	34\\
7.43928784728212	34\\
7.43928784728212	35\\
7.80460549655	35\\
7.80460549655	36\\
7.82700564192314	36\\
7.82700564192314	37\\
8.19984135697882	37\\
8.19984135697882	38\\
8.28742166668896	38\\
8.28742166668896	39\\
8.30386527373835	39\\
8.30386527373835	40\\
8.60439902280297	40\\
8.60439902280297	41\\
8.84391010248427	41\\
8.84391010248427	42\\
9.18471356957316	42\\
9.18471356957316	43\\
9.54224239425196	43\\
9.54224239425196	44\\
9.90755934425965	44\\
9.90755934425965	45\\
9.92614413380132	45\\
9.92614413380132	46\\
10.037824215442	46\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.154434217693883	0\\
0.333324444887708	0\\
0.333324444887708	1\\
0.40096815548771	1\\
0.40096815548771	2\\
0.642582540936573	2\\
0.642582540936573	3\\
0.799962649225812	3\\
0.799962649225812	4\\
0.823090374451013	4\\
0.823090374451013	5\\
1.01149370338476	5\\
1.01149370338476	6\\
1.13774853509963	6\\
1.13774853509963	7\\
1.17446536960562	7\\
1.17446536960562	8\\
1.27496396886629	8\\
1.27496396886629	9\\
1.36391767581163	9\\
1.36391767581163	10\\
1.95429834697384	10\\
1.95429834697384	11\\
2.10550174582233	11\\
2.10550174582233	12\\
2.25292062576281	12\\
2.25292062576281	13\\
2.79688279270103	13\\
2.79688279270103	14\\
3.06945170908591	14\\
3.06945170908591	15\\
3.10638738629265	15\\
3.10638738629265	16\\
3.19979529696172	16\\
3.19979529696172	17\\
3.23608270274337	17\\
3.23608270274337	18\\
3.30947178623997	18\\
3.30947178623997	19\\
3.36400026042543	19\\
3.36400026042543	20\\
3.50384457975716	20\\
3.50384457975716	21\\
3.61312833141875	21\\
3.61312833141875	22\\
3.76249315550003	22\\
3.76249315550003	23\\
4.08859982408828	23\\
4.08859982408828	24\\
4.20990807645695	24\\
4.20990807645695	25\\
4.26725776537203	25\\
4.26725776537203	26\\
4.8499143954304	26\\
4.8499143954304	27\\
4.85941376974257	27\\
4.85941376974257	28\\
5.04506918153879	28\\
5.04506918153879	29\\
5.07977716754427	29\\
5.07977716754427	30\\
5.12381990696147	30\\
5.12381990696147	31\\
5.56793976785688	31\\
5.56793976785688	32\\
5.98720401691883	32\\
5.98720401691883	33\\
6.21510728078535	33\\
6.21510728078535	34\\
6.50158685532585	34\\
6.50158685532585	35\\
6.51484880829704	35\\
6.51484880829704	36\\
6.59546357443018	36\\
6.59546357443018	37\\
6.89314962268917	37\\
6.89314962268917	38\\
6.97331553417123	38\\
6.97331553417123	39\\
6.98188386016125	39\\
6.98188386016125	40\\
7.12143628595356	40\\
7.12143628595356	41\\
7.18733127911347	41\\
7.18733127911347	42\\
7.42405267942366	42\\
7.42405267942366	43\\
7.43049828186886	43\\
7.43049828186886	44\\
7.45376448099888	44\\
7.45376448099888	45\\
7.48432211025185	45\\
7.48432211025185	46\\
7.48964825042191	46\\
7.48964825042191	47\\
7.8782398473069	47\\
7.8782398473069	48\\
7.97800937652352	48\\
7.97800937652352	49\\
8.05447965070125	49\\
8.05447965070125	50\\
8.33713231577799	50\\
8.33713231577799	51\\
8.37540206494825	51\\
8.37540206494825	52\\
9.18395712654954	52\\
9.18395712654954	53\\
10.1014189385411	53\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.0341609132252643	0\\
0.284949231770021	0\\
0.284949231770021	1\\
0.561850966474985	1\\
0.561850966474985	2\\
1.08091496166181	2\\
1.08091496166181	3\\
1.59210815231993	3\\
1.59210815231993	4\\
2.28366611254686	4\\
2.28366611254686	5\\
2.75491914791608	5\\
2.75491914791608	6\\
2.96935873496816	6\\
2.96935873496816	7\\
3.18454898432789	7\\
3.18454898432789	8\\
3.85493390561729	8\\
3.85493390561729	9\\
4.41530298272188	9\\
4.41530298272188	10\\
4.44764652581372	10\\
4.44764652581372	11\\
4.51507292673878	11\\
4.51507292673878	12\\
4.63087734674107	12\\
4.63087734674107	13\\
5.138027021123	13\\
5.138027021123	14\\
5.22721136498995	14\\
5.22721136498995	15\\
5.24109904634334	15\\
5.24109904634334	16\\
6.01981518358108	16\\
6.01981518358108	17\\
6.06816348230581	17\\
6.06816348230581	18\\
6.16556910779353	18\\
6.16556910779353	19\\
6.46331551293674	19\\
6.46331551293674	20\\
6.97070473160666	20\\
6.97070473160666	21\\
7.06743468416838	21\\
7.06743468416838	22\\
7.17712390892639	22\\
7.17712390892639	23\\
7.27652201075087	23\\
7.27652201075087	24\\
7.34996627860079	24\\
7.34996627860079	25\\
7.64754331948401	25\\
7.64754331948401	26\\
8.19777871424142	26\\
8.19777871424142	27\\
8.29133987682879	27\\
8.29133987682879	28\\
8.78926700183521	28\\
8.78926700183521	29\\
8.89686840540046	29\\
8.89686840540046	30\\
8.95428264285557	30\\
8.95428264285557	31\\
9.00299860690738	31\\
9.00299860690738	32\\
9.01816128729062	32\\
9.01816128729062	33\\
9.17818060777513	33\\
9.17818060777513	34\\
9.57509238370397	34\\
9.57509238370397	35\\
9.80652104794834	35\\
9.80652104794834	36\\
9.84870672979115	36\\
9.84870672979115	37\\
10.3465445067014	37\\
};
\addplot [my plot options]
  table[row sep=crcr]{%
0.258852573154947	0\\
0.328581247858374	0\\
0.328581247858374	1\\
0.494925515857197	1\\
0.494925515857197	2\\
0.601088493703699	2\\
0.601088493703699	3\\
0.603332383500806	3\\
0.603332383500806	4\\
0.990222682550517	4\\
0.990222682550517	5\\
1.03097924348453	5\\
1.03097924348453	6\\
1.26733450984914	6\\
1.26733450984914	7\\
1.35742691222038	7\\
1.35742691222038	8\\
1.398590752087	8\\
1.398590752087	9\\
1.5642403798596	9\\
1.5642403798596	10\\
1.86340189401871	10\\
1.86340189401871	11\\
2.00549618400664	11\\
2.00549618400664	12\\
2.05163979077624	12\\
2.05163979077624	13\\
2.12482862124565	13\\
2.12482862124565	14\\
2.28429582488671	14\\
2.28429582488671	15\\
2.4400772534571	15\\
2.4400772534571	16\\
2.45803436447366	16\\
2.45803436447366	17\\
3.28497125420875	17\\
3.28497125420875	18\\
3.48937332219403	18\\
3.48937332219403	19\\
3.73198917054229	19\\
3.73198917054229	20\\
3.80974442724594	20\\
3.80974442724594	21\\
3.81509511606723	21\\
3.81509511606723	22\\
3.83152922344555	22\\
3.83152922344555	23\\
3.84307414936831	23\\
3.84307414936831	24\\
3.86042894208711	24\\
3.86042894208711	25\\
3.90333841708034	25\\
3.90333841708034	26\\
4.05303748820982	26\\
4.05303748820982	27\\
4.22269439485346	27\\
4.22269439485346	28\\
4.3604954253105	28\\
4.3604954253105	29\\
4.5398865396987	29\\
4.5398865396987	30\\
4.55945668979671	30\\
4.55945668979671	31\\
4.77578320278079	31\\
4.77578320278079	32\\
5.01515267883941	32\\
5.01515267883941	33\\
5.22617577549212	33\\
5.22617577549212	34\\
6.08651611035371	34\\
6.08651611035371	35\\
6.16750970868372	35\\
6.16750970868372	36\\
6.21097242279222	36\\
6.21097242279222	37\\
6.47644957467011	37\\
6.47644957467011	38\\
6.55523840359884	38\\
6.55523840359884	39\\
6.61580083474573	39\\
6.61580083474573	40\\
6.96210421151296	40\\
6.96210421151296	41\\
7.25080476535613	41\\
7.25080476535613	42\\
7.40789483055156	42\\
7.40789483055156	43\\
7.43498122383898	43\\
7.43498122383898	44\\
7.63226872570026	44\\
7.63226872570026	45\\
7.70375729767505	45\\
7.70375729767505	46\\
7.7832320848703	46\\
7.7832320848703	47\\
7.78782252134468	47\\
7.78782252134468	48\\
7.96140197698121	48\\
7.96140197698121	49\\
8.20549113621472	49\\
8.20549113621472	50\\
8.37162618106113	50\\
8.37162618106113	51\\
8.400295285835	51\\
8.400295285835	52\\
8.46715484866457	52\\
8.46715484866457	53\\
8.59385690718631	53\\
8.59385690718631	54\\
8.9516322255179	54\\
8.9516322255179	55\\
9.26027281868451	55\\
9.26027281868451	56\\
9.51050676355079	56\\
9.51050676355079	57\\
9.78893049065511	57\\
9.78893049065511	58\\
9.91883286940031	58\\
9.91883286940031	59\\
10.0343180073027	59\\
};

==> fig9_part1a_220222.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\begin{axis}[%
width=0.7\linewidth,
height=0.7\linewidth,
name = mb,
%at={(1.011in,0.642in)},
scale only axis,
colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.2444,0.1534,0.6728); rgb(2pt)=(0.2464,0.1569,0.6847); rgb(3pt)=(0.2484,0.1607,0.6961); rgb(4pt)=(0.2503,0.1648,0.7071); rgb(5pt)=(0.2522,0.1689,0.7179); rgb(6pt)=(0.254,0.1732,0.7286); rgb(7pt)=(0.2558,0.1773,0.7393); rgb(8pt)=(0.2576,0.1814,0.7501); rgb(9pt)=(0.2594,0.1854,0.761); rgb(11pt)=(0.2628,0.1932,0.7828); rgb(12pt)=(0.2645,0.1972,0.7937); rgb(13pt)=(0.2661,0.2011,0.8043); rgb(14pt)=(0.2676,0.2052,0.8148); rgb(15pt)=(0.2691,0.2094,0.8249); rgb(16pt)=(0.2704,0.2138,0.8346); rgb(17pt)=(0.2717,0.2184,0.8439); rgb(18pt)=(0.2729,0.2231,0.8528); rgb(19pt)=(0.274,0.228,0.8612); rgb(20pt)=(0.2749,0.233,0.8692); rgb(21pt)=(0.2758,0.2382,0.8767); rgb(22pt)=(0.2766,0.2435,0.884); rgb(23pt)=(0.2774,0.2489,0.8908); rgb(24pt)=(0.2781,0.2543,0.8973); rgb(25pt)=(0.2788,0.2598,0.9035); rgb(26pt)=(0.2794,0.2653,0.9094); rgb(27pt)=(0.2798,0.2708,0.915); rgb(28pt)=(0.2802,0.2764,0.9204); rgb(29pt)=(0.2806,0.2819,0.9255); rgb(30pt)=(0.2809,0.2875,0.9305); rgb(31pt)=(0.2811,0.293,0.9352); rgb(32pt)=(0.2813,0.2985,0.9397); rgb(33pt)=(0.2814,0.304,0.9441); rgb(34pt)=(0.2814,0.3095,0.9483); rgb(35pt)=(0.2813,0.315,0.9524); rgb(36pt)=(0.2811,0.3204,0.9563); rgb(37pt)=(0.2809,0.3259,0.96); rgb(38pt)=(0.2807,0.3313,0.9636); rgb(39pt)=(0.2803,0.3367,0.967); rgb(40pt)=(0.2798,0.3421,0.9702); rgb(41pt)=(0.2791,0.3475,0.9733); rgb(42pt)=(0.2784,0.3529,0.9763); rgb(43pt)=(0.2776,0.3583,0.9791); rgb(44pt)=(0.2766,0.3638,0.9817); rgb(45pt)=(0.2754,0.3693,0.984); rgb(46pt)=(0.2741,0.3748,0.9862); rgb(47pt)=(0.2726,0.3804,0.9881); rgb(48pt)=(0.271,0.386,0.9898); rgb(49pt)=(0.2691,0.3916,0.9912); rgb(50pt)=(0.267,0.3973,0.9924); rgb(51pt)=(0.2647,0.403,0.9935); rgb(52pt)=(0.2621,0.4088,0.9946); rgb(53pt)=(0.2591,0.4145,0.9955); rgb(54pt)=(0.2556,0.4203,0.9965); rgb(55pt)=(0.2517,0.4261,0.9974); rgb(56pt)=(0.2473,0.4319,0.9983); rgb(57pt)=(0.2424,0.4378,0.9991); rgb(58pt)=(0.2369,0.4437,0.9996); rgb(59pt)=(0.2311,0.4497,0.9995); rgb(60pt)=(0.225,0.4559,0.9985); rgb(61pt)=(0.2189,0.462,0.9968); rgb(62pt)=(0.2128,0.4682,0.9948); rgb(63pt)=(0.2066,0.4743,0.9926); rgb(64pt)=(0.2006,0.4803,0.9906); rgb(65pt)=(0.195,0.4861,0.9887); rgb(66pt)=(0.1903,0.4919,0.9867); rgb(67pt)=(0.1869,0.4975,0.9844); rgb(68pt)=(0.1847,0.503,0.9819); rgb(69pt)=(0.1831,0.5084,0.9793); rgb(70pt)=(0.1818,0.5138,0.9766); rgb(71pt)=(0.1806,0.5191,0.9738); rgb(72pt)=(0.1795,0.5244,0.9709); rgb(73pt)=(0.1785,0.5296,0.9677); rgb(74pt)=(0.1778,0.5349,0.9641); rgb(75pt)=(0.1773,0.5401,0.9602); rgb(76pt)=(0.1768,0.5452,0.956); rgb(77pt)=(0.1764,0.5504,0.9516); rgb(78pt)=(0.1755,0.5554,0.9473); rgb(79pt)=(0.174,0.5605,0.9432); rgb(80pt)=(0.1716,0.5655,0.9393); rgb(81pt)=(0.1686,0.5705,0.9357); rgb(82pt)=(0.1649,0.5755,0.9323); rgb(83pt)=(0.161,0.5805,0.9289); rgb(84pt)=(0.1573,0.5854,0.9254); rgb(85pt)=(0.154,0.5902,0.9218); rgb(86pt)=(0.1513,0.595,0.9182); rgb(87pt)=(0.1492,0.5997,0.9147); rgb(88pt)=(0.1475,0.6043,0.9113); rgb(89pt)=(0.1461,0.6089,0.908); rgb(90pt)=(0.1446,0.6135,0.905); rgb(91pt)=(0.1429,0.618,0.9022); rgb(92pt)=(0.1408,0.6226,0.8998); rgb(93pt)=(0.1383,0.6272,0.8975); rgb(94pt)=(0.1354,0.6317,0.8953); rgb(95pt)=(0.1321,0.6363,0.8932); rgb(96pt)=(0.1288,0.6408,0.891); rgb(97pt)=(0.1253,0.6453,0.8887); rgb(98pt)=(0.1219,0.6497,0.8862); rgb(99pt)=(0.1185,0.6541,0.8834); rgb(100pt)=(0.1152,0.6584,0.8804); rgb(101pt)=(0.1119,0.6627,0.877); rgb(102pt)=(0.1085,0.6669,0.8734); rgb(103pt)=(0.1048,0.671,0.8695); rgb(104pt)=(0.1009,0.675,0.8653); rgb(105pt)=(0.0964,0.6789,0.8609); rgb(106pt)=(0.0914,0.6828,0.8562); rgb(107pt)=(0.0855,0.6865,0.8513); rgb(108pt)=(0.0789,0.6902,0.8462); rgb(109pt)=(0.0713,0.6938,0.8409); rgb(110pt)=(0.0628,0.6972,0.8355); rgb(111pt)=(0.0535,0.7006,0.8299); rgb(112pt)=(0.0433,0.7039,0.8242); rgb(113pt)=(0.0328,0.7071,0.8183); rgb(114pt)=(0.0234,0.7103,0.8124); rgb(115pt)=(0.0155,0.7133,0.8064); rgb(116pt)=(0.0091,0.7163,0.8003); rgb(117pt)=(0.0046,0.7192,0.7941); rgb(118pt)=(0.0019,0.722,0.7878); rgb(119pt)=(0.0009,0.7248,0.7815); rgb(120pt)=(0.0018,0.7275,0.7752); rgb(121pt)=(0.0046,0.7301,0.7688); rgb(122pt)=(0.0094,0.7327,0.7623); rgb(123pt)=(0.0162,0.7352,0.7558); rgb(124pt)=(0.0253,0.7376,0.7492); rgb(125pt)=(0.0369,0.74,0.7426); rgb(126pt)=(0.0504,0.7423,0.7359); rgb(127pt)=(0.0638,0.7446,0.7292); rgb(128pt)=(0.077,0.7468,0.7224); rgb(129pt)=(0.0899,0.7489,0.7156); rgb(130pt)=(0.1023,0.751,0.7088); rgb(131pt)=(0.1141,0.7531,0.7019); rgb(132pt)=(0.1252,0.7552,0.695); rgb(133pt)=(0.1354,0.7572,0.6881); rgb(134pt)=(0.1448,0.7593,0.6812); rgb(135pt)=(0.1532,0.7614,0.6741); rgb(136pt)=(0.1609,0.7635,0.6671); rgb(137pt)=(0.1678,0.7656,0.6599); rgb(138pt)=(0.1741,0.7678,0.6527); rgb(139pt)=(0.1799,0.7699,0.6454); rgb(140pt)=(0.1853,0.7721,0.6379); rgb(141pt)=(0.1905,0.7743,0.6303); rgb(142pt)=(0.1954,0.7765,0.6225); rgb(143pt)=(0.2003,0.7787,0.6146); rgb(144pt)=(0.2061,0.7808,0.6065); rgb(145pt)=(0.2118,0.7828,0.5983); rgb(146pt)=(0.2178,0.7849,0.5899); rgb(147pt)=(0.2244,0.7869,0.5813); rgb(148pt)=(0.2318,0.7887,0.5725); rgb(149pt)=(0.2401,0.7905,0.5636); rgb(150pt)=(0.2491,0.7922,0.5546); rgb(151pt)=(0.2589,0.7937,0.5454); rgb(152pt)=(0.2695,0.7951,0.536); rgb(153pt)=(0.2809,0.7964,0.5266); rgb(154pt)=(0.2929,0.7975,0.517); rgb(155pt)=(0.3052,0.7985,0.5074); rgb(156pt)=(0.3176,0.7994,0.4975); rgb(157pt)=(0.3301,0.8002,0.4876); rgb(158pt)=(0.3424,0.8009,0.4774); rgb(159pt)=(0.3548,0.8016,0.4669); rgb(160pt)=(0.3671,0.8021,0.4563); rgb(161pt)=(0.3795,0.8026,0.4454); rgb(162pt)=(0.3921,0.8029,0.4344); rgb(163pt)=(0.405,0.8031,0.4233); rgb(164pt)=(0.4184,0.803,0.4122); rgb(165pt)=(0.4322,0.8028,0.4013); rgb(166pt)=(0.4463,0.8024,0.3904); rgb(167pt)=(0.4608,0.8018,0.3797); rgb(168pt)=(0.4753,0.8011,0.3691); rgb(169pt)=(0.4899,0.8002,0.3586); rgb(170pt)=(0.5044,0.7993,0.348); rgb(171pt)=(0.5187,0.7982,0.3374); rgb(172pt)=(0.5329,0.797,0.3267); rgb(173pt)=(0.547,0.7957,0.3159); rgb(175pt)=(0.5748,0.7929,0.2941); rgb(176pt)=(0.5886,0.7913,0.2833); rgb(177pt)=(0.6024,0.7896,0.2726); rgb(178pt)=(0.6161,0.7878,0.2622); rgb(179pt)=(0.6297,0.7859,0.2521); rgb(180pt)=(0.6433,0.7839,0.2423); rgb(181pt)=(0.6567,0.7818,0.2329); rgb(182pt)=(0.6701,0.7796,0.2239); rgb(183pt)=(0.6833,0.7773,0.2155); rgb(184pt)=(0.6963,0.775,0.2075); rgb(185pt)=(0.7091,0.7727,0.1998); rgb(186pt)=(0.7218,0.7703,0.1924); rgb(187pt)=(0.7344,0.7679,0.1852); rgb(188pt)=(0.7468,0.7654,0.1782); rgb(189pt)=(0.759,0.7629,0.1717); rgb(190pt)=(0.771,0.7604,0.1658); rgb(191pt)=(0.7829,0.7579,0.1608); rgb(192pt)=(0.7945,0.7554,0.157); rgb(193pt)=(0.806,0.7529,0.1546); rgb(194pt)=(0.8172,0.7505,0.1535); rgb(195pt)=(0.8281,0.7481,0.1536); rgb(196pt)=(0.8389,0.7457,0.1546); rgb(197pt)=(0.8495,0.7435,0.1564); rgb(198pt)=(0.86,0.7413,0.1587); rgb(199pt)=(0.8703,0.7392,0.1615); rgb(200pt)=(0.8804,0.7372,0.165); rgb(201pt)=(0.8903,0.7353,0.1695); rgb(202pt)=(0.9,0.7336,0.1749); rgb(203pt)=(0.9093,0.7321,0.1815); rgb(204pt)=(0.9184,0.7308,0.189); rgb(205pt)=(0.9272,0.7298,0.1973); rgb(206pt)=(0.9357,0.729,0.2061); rgb(207pt)=(0.944,0.7285,0.2151); rgb(208pt)=(0.9523,0.7284,0.2237); rgb(209pt)=(0.9606,0.7285,0.2312); rgb(210pt)=(0.9689,0.7292,0.2373); rgb(211pt)=(0.977,0.7304,0.2418); rgb(212pt)=(0.9842,0.733,0.2446); rgb(213pt)=(0.99,0.7365,0.2429); rgb(214pt)=(0.9946,0.7407,0.2394); rgb(215pt)=(0.9966,0.7458,0.2351); rgb(216pt)=(0.9971,0.7513,0.2309); rgb(217pt)=(0.9972,0.7569,0.2267); rgb(218pt)=(0.9971,0.7626,0.2224); rgb(219pt)=(0.9969,0.7683,0.2181); rgb(220pt)=(0.9966,0.774,0.2138); rgb(221pt)=(0.9962,0.7798,0.2095); rgb(222pt)=(0.9957,0.7856,0.2053); rgb(223pt)=(0.9949,0.7915,0.2012); rgb(224pt)=(0.9938,0.7974,0.1974); rgb(225pt)=(0.9923,0.8034,0.1939); rgb(226pt)=(0.9906,0.8095,0.1906); rgb(227pt)=(0.9885,0.8156,0.1875); rgb(228pt)=(0.9861,0.8218,0.1846); rgb(229pt)=(0.9835,0.828,0.1817); rgb(230pt)=(0.9807,0.8342,0.1787); rgb(231pt)=(0.9778,0.8404,0.1757); rgb(232pt)=(0.9748,0.8467,0.1726); rgb(233pt)=(0.972,0.8529,0.1695); rgb(234pt)=(0.9694,0.8591,0.1665); rgb(235pt)=(0.9671,0.8654,0.1636); rgb(236pt)=(0.9651,0.8716,0.1608); rgb(237pt)=(0.9634,0.8778,0.1582); rgb(238pt)=(0.9619,0.884,0.1557); rgb(239pt)=(0.9608,0.8902,0.1532); rgb(240pt)=(0.9601,0.8963,0.1507); rgb(241pt)=(0.9596,0.9023,0.148); rgb(242pt)=(0.9595,0.9084,0.145); rgb(243pt)=(0.9597,0.9143,0.1418); rgb(244pt)=(0.9601,0.9203,0.1382); rgb(245pt)=(0.9608,0.9262,0.1344); rgb(246pt)=(0.9618,0.932,0.1304); rgb(247pt)=(0.9629,0.9379,0.1261); rgb(248pt)=(0.9642,0.9437,0.1216); rgb(249pt)=(0.9657,0.9494,0.1168); rgb(250pt)=(0.9674,0.9552,0.1116); rgb(251pt)=(0.9692,0.9609,0.1061); rgb(252pt)=(0.9711,0.9667,0.1001); rgb(253pt)=(0.973,0.9724,0.0938); rgb(254pt)=(0.9749,0.9782,0.0872); rgb(255pt)=(0.9769,0.9839,0.0805)},
xmin=1.76918334463198,
xmax=3.33041309291151,
ymin=0.0883129677735573,
ymax=0.112575806912646,
xlabel=m,
ylabel = $\beta$,
axis background/.style={fill=white}
]
\addplot[contour prepared, contour prepared format=matlab, contour/labels=false] table[row sep=crcr] {%
%
-6.90775527898214	7\\
1.87157698333989	0.0883129677735573\\
1.87957332683357	0.0885686721990915\\
1.89226085793077	0.0888081277559877\\
1.89534332429094	0.0888887080957357\\
1.90242868486034	0.0888081277559877\\
1.9111133217483	0.0888081277559877\\
1.92688331920567	0.0883129677735573\\
-6.90775527898214	150\\
1.95968866020694	0.0883129677735573\\
1.97419331157778	0.0887730833314097\\
1.97901894154959	0.0888081277559877\\
1.98996330903515	0.0889794059051731\\
2.00467018878387	0.0888081277559877\\
2.00573330649252	0.088790395263885\\
2.02150330394989	0.0885860196288027\\
2.03727330140726	0.0886407848635398\\
2.04671278600041	0.0888081277559877\\
2.05304329886463	0.0889281766858201\\
2.06881329632199	0.0892115352456779\\
2.08458329377936	0.0892985001393151\\
2.10035329123673	0.0892576066566807\\
2.11141487295501	0.0893032877384181\\
2.1161232886941	0.0893310786420738\\
2.13189328615147	0.089522239384975\\
2.14766328360884	0.0897164383172031\\
2.15691460490434	0.0897984477208485\\
2.16343328106621	0.0898684457859836\\
2.17920327852358	0.0900158817952382\\
2.19497327598095	0.0901713197677579\\
2.20686246426726	0.0902936077032789\\
2.21074327343832	0.0903370600676151\\
2.22651327089568	0.0905070198943466\\
2.24228326835305	0.0906740749558112\\
2.25280294408644	0.0907887676857093\\
2.25805326581042	0.0908542844351215\\
2.27382326326779	0.091050140177458\\
2.28959326072516	0.0912367566706018\\
2.29367221890532	0.0912839276681397\\
2.30536325818253	0.0914380474398947\\
2.3211332556399	0.0916423709743313\\
2.33186479809941	0.0917790876505701\\
2.33690325309727	0.0918507287911036\\
2.35267325055464	0.092070975503182\\
2.36769685592339	0.0922742476330004\\
2.368443248012	0.0922855005165239\\
2.38421324546937	0.0925210998644247\\
2.39998324292674	0.0927518870750339\\
2.40119285593397	0.0927694076154308\\
2.41575324038411	0.0930038810975653\\
2.43152323784148	0.0932475240260507\\
2.43263667913586	0.0932645675978612\\
2.44729323529885	0.0935163724588523\\
2.46190691612386	0.0937597275802916\\
2.46306323275622	0.0937819086922788\\
2.47883323021359	0.0940507243806814\\
2.48989042130431	0.094254887562722\\
2.49460322767096	0.0943588811356599\\
2.51037322512833	0.0946665006198456\\
2.51476738571706	0.0947500475451524\\
2.52614322258569	0.0949894358736701\\
2.53867763585286	0.0952452075275828\\
2.54191322004306	0.0953220437867318\\
2.55768321750043	0.0956841224380851\\
2.56023166869232	0.0957403675100132\\
2.5734532149578	0.0960728851242835\\
2.58008520954523	0.0962355274924436\\
2.58922321241517	0.0964981689671494\\
2.59771333050175	0.096730687474874\\
2.60499320987254	0.0969678444248867\\
2.61316334799768	0.0972258474573043\\
2.62076320732991	0.0975190398576587\\
2.62626756119639	0.0977210074397347\\
2.63653320478728	0.0982112684016493\\
2.63663965922411	0.0982161674221651\\
2.64387979497486	0.0987113274045955\\
2.64721038944497	0.0992064873870259\\
2.64575744817271	0.0997016473694563\\
2.63726796936541	0.100196807351887\\
2.63653320478728	0.10021947811208\\
2.62076320732991	0.100620064544881\\
2.61725018612489	0.100691967334317\\
2.60499320987254	0.100856103944548\\
2.58922321241517	0.101017036825475\\
2.5734532149578	0.101137047881259\\
2.56401818649686	0.101187127316747\\
2.55768321750043	0.101211704677968\\
2.54191322004306	0.101250677042184\\
2.52614322258569	0.101272917861195\\
2.51037322512833	0.101268762561141\\
2.49460322767096	0.101254232443672\\
2.47883323021359	0.101234198105372\\
2.46411685850313	0.101187127316747\\
2.46306323275622	0.101183282151684\\
2.44729323529885	0.101118906021728\\
2.43152323784148	0.10105453786799\\
2.41575324038411	0.100964879497766\\
2.39998324292674	0.100866791163252\\
2.38421324546937	0.100765309843491\\
2.3751171658268	0.100691967334317\\
2.368443248012	0.100633208745036\\
2.35267325055464	0.100501210512996\\
2.33690325309727	0.100351949801216\\
2.3211332556399	0.10020848897545\\
2.32001970959039	0.100196807351887\\
2.30536325818253	0.100026499457734\\
2.28959326072516	0.0998439729008163\\
2.27700762899124	0.0997016473694563\\
2.27382326326779	0.0996615432157942\\
2.25805326581042	0.0994400823322696\\
2.24228326835305	0.0992334003335129\\
2.24041676061361	0.0992064873870259\\
2.22651327089568	0.0989853096064723\\
2.21074327343832	0.0987528822656459\\
2.20816581638791	0.0987113274045955\\
2.19497327598095	0.0984753915452536\\
2.17920327852358	0.0982242466093614\\
2.17875590680828	0.0982161674221651\\
2.16343328106621	0.09791059907795\\
2.15288104467162	0.0977210074397347\\
2.14766328360884	0.0976177475583456\\
2.13189328615147	0.0972994988544008\\
2.12832630915157	0.0972258474573043\\
2.1161232886941	0.0969525350166648\\
2.10544040045408	0.096730687474874\\
2.10035329123673	0.0966159474963173\\
2.08458329377936	0.0962648995065713\\
2.08337689501277	0.0962355274924436\\
2.06881329632199	0.0958628049816586\\
2.06388074384633	0.0957403675100132\\
2.05304329886463	0.0954593378400147\\
2.04461970231707	0.0952452075275828\\
2.03727330140726	0.095051505428009\\
2.02574609403663	0.0947500475451524\\
2.02150330394989	0.0946361341074809\\
2.00738417525501	0.094254887562722\\
2.00573330649252	0.094209634072928\\
1.98996330903515	0.0937612714108473\\
1.98993178987012	0.0937597275802916\\
1.97419331157778	0.0932699229524321\\
1.97419331157778	0.0932645675978612\\
1.95842331412041	0.0927694076154308\\
1.95842331412041	0.0927694076154308\\
1.94344347459782	0.0922742476330004\\
1.94265331666304	0.092250180979511\\
1.93123797677365	0.0917790876505701\\
1.92688331920567	0.0916430043355028\\
1.9211883724799	0.0912839276681397\\
1.9111133217483	0.0909647235394064\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.86648527356964	0.0893032877384181\\
1.8638033293762	0.0892079132798894\\
1.8638033293762	0.0888081277559877\\
1.84803333191883	0.0883129677735573\\
1.84803333191883	0.0883129677735573\\
-6.14022691465079	8\\
1.86989859765359	0.0883129677735573\\
1.87957332683357	0.0886223430610399\\
1.88941711214842	0.0888081277559877\\
1.89534332429094	0.0889630479179834\\
1.90896532204675	0.0888081277559877\\
1.9111133217483	0.0888081277559877\\
1.92688331920567	0.088369612159585\\
1.93016125920101	0.0883129677735573\\
-6.14022691465079	143\\
1.95509419210627	0.0883129677735573\\
1.95842331412041	0.0883547447330463\\
1.97236900612924	0.0888081277559877\\
1.97419331157778	0.0888491384902246\\
1.98996330903515	0.0890920677187475\\
2.00573330649252	0.0889618066738842\\
2.01709244567025	0.0888081277559877\\
2.02150330394989	0.0887510778352357\\
2.03727330140726	0.0888056782606608\\
2.03741147263796	0.0888081277559877\\
2.05304329886463	0.0891045625078141\\
2.06634580705954	0.0893032877384181\\
2.06881329632199	0.0893444452568499\\
2.08458329377936	0.0894899819804013\\
2.10035329123673	0.0895164392753496\\
2.1161232886941	0.0896209622301354\\
2.13189328615147	0.089777300683846\\
2.13379155625254	0.0897984477208485\\
2.14766328360884	0.0899599864217507\\
2.16343328106621	0.0901204964795992\\
2.17920327852358	0.0902758748118135\\
2.18094127888557	0.0902936077032789\\
2.19497327598095	0.090459100431554\\
2.21074327343832	0.0906333201292392\\
2.22566279435502	0.0907887676857093\\
2.22651327089568	0.0907989481731149\\
2.24228326835305	0.0909900357109361\\
2.25805326581042	0.0911812654014957\\
2.26666046134443	0.0912839276681397\\
2.27382326326779	0.0913799170825222\\
2.28959326072516	0.0915871057546017\\
2.3045737702078	0.0917790876505701\\
2.30536325818253	0.0917904404135458\\
2.3211332556399	0.0920160160239966\\
2.33690325309727	0.092235392260178\\
2.33974660957772	0.0922742476330004\\
2.35267325055464	0.0924715524585939\\
2.368443248012	0.0927043456739062\\
2.37290481666467	0.0927694076154308\\
2.38421324546937	0.0929556881276837\\
2.39998324292674	0.0932086054225998\\
2.40356022979635	0.0932645675978612\\
2.41575324038411	0.0934777125134544\\
2.43152323784148	0.0937449655692941\\
2.43240049140615	0.0937597275802916\\
2.44729323529885	0.094043388177938\\
2.45836811752815	0.094254887562722\\
2.46306323275622	0.094350465490558\\
2.47883323021359	0.0946455516716959\\
2.48380517558123	0.0947500475451524\\
2.49460322767096	0.0949909613506637\\
2.50655513687833	0.0952452075275828\\
2.51037322512833	0.0953378349924582\\
2.52614322258569	0.0957128478332299\\
2.52731804969441	0.0957403675100132\\
2.54191322004306	0.0961309940379876\\
2.54601745630729	0.0962355274924436\\
2.55768321750043	0.0965939266925428\\
2.56227518956554	0.096730687474874\\
2.5734532149578	0.0971303196101304\\
2.57626025092739	0.0972258474573043\\
2.58740323590263	0.0977210074397347\\
2.58922321241517	0.0978356511811569\\
2.59554770916667	0.0982161674221651\\
2.59963440111986	0.0987113274045955\\
2.5988338753042	0.0992064873870259\\
2.59104725252908	0.0997016473694563\\
2.58922321241517	0.0997581248871449\\
2.5734532149578	0.100150031800093\\
2.57109122502099	0.100196807351887\\
2.55768321750043	0.100364915490366\\
2.54191322004306	0.100511149006685\\
2.52614322258569	0.100607767915276\\
2.51037322512833	0.100678501635651\\
2.50232196796273	0.100691967334317\\
2.49460322767096	0.100701463349673\\
2.47883323021359	0.100704670782477\\
2.46306323275622	0.100697745827797\\
2.45808994371412	0.100691967334317\\
2.44729323529885	0.100677466600993\\
2.43152323784148	0.100613792136645\\
2.41575324038411	0.100555189805453\\
2.39998324292674	0.100483263908855\\
2.38421324546937	0.100396817541106\\
2.368443248012	0.100298126176387\\
2.35378367832193	0.100196807351887\\
2.35267325055464	0.100188064521045\\
2.33690325309727	0.100051044796915\\
2.3211332556399	0.0999035035926607\\
2.30536325818253	0.0997618775331253\\
2.29936813468904	0.0997016473694563\\
2.28959326072516	0.0995907664740065\\
2.27382326326779	0.099409505278343\\
2.25805326581042	0.099229703702054\\
2.25622680956043	0.0992064873870259\\
2.24228326835305	0.0990087510319119\\
2.22651327089568	0.0987968190000378\\
2.22040551560679	0.0987113274045955\\
2.21074327343832	0.0985592234326536\\
2.19497327598095	0.0983122145000495\\
2.18887175523815	0.0982161674221651\\
2.17920327852358	0.0980466536135323\\
2.16343328106621	0.0977780211296336\\
2.16026002965489	0.0977210074397347\\
2.14766328360884	0.0974717168940479\\
2.13396467827345	0.0972258474573043\\
2.13189328615147	0.0971846436205788\\
2.1161232886941	0.096845358681881\\
2.11060138983096	0.096730687474874\\
2.10035329123673	0.0964995411474195\\
2.08774184110753	0.0962355274924436\\
2.08458329377936	0.0961637082101763\\
2.06881329632199	0.0957913297973831\\
2.06676021442351	0.0957403675100132\\
2.05304329886463	0.0953846692564658\\
2.04755706328876	0.0952452075275828\\
2.03727330140726	0.0949740562124806\\
2.02870761277228	0.0947500475451524\\
2.02150330394989	0.094556621151853\\
2.01032886726298	0.094254887562722\\
2.00573330649252	0.0941289143980771\\
1.9926063490601	0.0937597275802916\\
1.98996330903515	0.0936855547023112\\
1.97573929250152	0.0932645675978612\\
1.97419331157778	0.0932200806624811\\
1.95996110685693	0.0927694076154308\\
1.95842331412041	0.0927239008759376\\
1.94554024392147	0.0922742476330004\\
1.94265331666304	0.0921863175181208\\
1.93278548991701	0.0917790876505701\\
1.92688331920567	0.0915946444552205\\
1.92195535893963	0.0912839276681397\\
1.9111133217483	0.0909404233893475\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.86813773255776	0.0893032877384181\\
1.8638033293762	0.0891491490514544\\
1.8638033293762	0.0888081277559877\\
1.84803333191883	0.0883129677735573\\
1.84803333191883	0.0883129677735573\\
-5.37269855031944	138\\
1.86822021196728	0.0883129677735573\\
1.87957332683357	0.0886760139229884\\
1.88657336636606	0.0888081277559877\\
1.89534332429094	0.089037387740231\\
1.9111133217483	0.0889057547641656\\
1.91849561607138	0.0888081277559877\\
1.92688331920567	0.0886183689428721\\
1.94265331666304	0.0883380633671264\\
1.95842331412041	0.0885346496954574\\
1.96683527621503	0.0888081277559877\\
1.97419331157778	0.0889735377935497\\
1.98996330903515	0.0892047295323219\\
2.00573330649252	0.0891344596438362\\
2.02150330394989	0.0889947250743809\\
2.03727330140726	0.0890801078875562\\
2.05304329886463	0.0892809483298081\\
2.05453868103226	0.0893032877384181\\
2.06881329632199	0.0895413871501696\\
2.08458329377936	0.0896831830843449\\
2.10035329123673	0.0897915542859662\\
2.10131053358247	0.0897984477208485\\
2.1161232886941	0.0899182613900325\\
2.13189328615147	0.0900721121219986\\
2.14766328360884	0.0902266103303812\\
2.15468349157943	0.0902936077032789\\
2.16343328106621	0.0903946207232593\\
2.17920327852358	0.0905810161638161\\
2.19497327598095	0.0907596329142881\\
2.19764486989872	0.0907887676857093\\
2.21074327343832	0.0909514834577368\\
2.22651327089568	0.0911393174243039\\
2.23867580693993	0.0912839276681397\\
2.24228326835305	0.0913327065421891\\
2.25805326581042	0.0915433547143329\\
2.27382326326779	0.0917472955465549\\
2.27630306412711	0.0917790876505701\\
2.28959326072516	0.0919714695071377\\
2.30536325818253	0.0921921819019666\\
2.31125558292295	0.0922742476330004\\
2.3211332556399	0.0924307271176282\\
2.33690325309727	0.0926712264800501\\
2.34353031136337	0.0927694076154308\\
2.35267325055464	0.092922151429871\\
2.368443248012	0.0931790173620959\\
2.37375688028512	0.0932645675978612\\
2.38421324546937	0.0934548021588126\\
2.39998324292674	0.0937288361926404\\
2.40179405049348	0.0937597275802916\\
2.41575324038411	0.0940316776531394\\
2.42764987273666	0.094254887562722\\
2.43152323784148	0.0943384677258475\\
2.44729323529885	0.0946646483493509\\
2.451689900557	0.0947500475451524\\
2.46306323275622	0.0950123559942165\\
2.47323866959124	0.0952452075275828\\
2.47883323021359	0.0953909307625088\\
2.4930723832932	0.0957403675100132\\
2.49460322767096	0.0957860494798298\\
2.5101467828547	0.0962355274924436\\
2.51037322512833	0.0962434330507443\\
2.52499677648976	0.096730687474874\\
2.52614322258569	0.096780438679248\\
2.53690370830092	0.0972258474573043\\
2.54191322004306	0.0975085868070997\\
2.54585396231996	0.0977210074397347\\
2.55058636054734	0.0982161674221651\\
2.55027576633237	0.0987113274045955\\
2.54209386280028	0.0992064873870259\\
2.54191322004306	0.0992118728641497\\
2.52614322258569	0.0996078396243688\\
2.52089392159553	0.0997016473694563\\
2.51037322512833	0.0998217572266993\\
2.49460322767096	0.0999543999428422\\
2.47883323021359	0.100042135700943\\
2.46306323275622	0.100088658235815\\
2.44729323529885	0.100100982969172\\
2.43152323784148	0.100097762012964\\
2.41575324038411	0.100076799682735\\
2.39998324292674	0.100019716234855\\
2.38421324546937	0.0999675513908743\\
2.368443248012	0.099885742201914\\
2.35267325055464	0.0998063447291492\\
2.33690325309727	0.0997125609570451\\
2.33555696423334	0.0997016473694563\\
2.3211332556399	0.0995730948401787\\
2.30536325818253	0.0994409482335636\\
2.28959326072516	0.0992919837570393\\
2.28020466629243	0.0992064873870259\\
2.27382326326779	0.0991415661671655\\
2.25805326581042	0.0989546676183383\\
2.24228326835305	0.0987740413263016\\
2.23710442435801	0.0987113274045955\\
2.22651327089568	0.0985676869190485\\
2.21074327343832	0.0983472357852832\\
2.20127396733894	0.0982161674221651\\
2.19497327598095	0.0981189548000021\\
2.17920327852358	0.0978649096369203\\
2.17003383789683	0.0977210074397347\\
2.16343328106621	0.0976055724972079\\
2.14766328360884	0.0973256862297501\\
2.14210077059779	0.0972258474573043\\
2.13189328615147	0.0970228016322085\\
2.1161232886941	0.0967381823470972\\
2.11576237920785	0.096730687474874\\
2.10035329123673	0.0963831347985218\\
2.09330235980108	0.0962355274924436\\
2.08458329377936	0.0960372727257234\\
2.07053072455147	0.0957403675100132\\
2.06881329632199	0.0957008553117738\\
2.05304329886463	0.0953100006729169\\
2.05049442426045	0.0952452075275828\\
2.03727330140726	0.0948966069969522\\
2.03166913150792	0.0947500475451524\\
2.02150330394989	0.0944771081962251\\
2.01327355927096	0.094254887562722\\
2.00573330649252	0.0940481947232261\\
1.99547645082073	0.0937597275802916\\
1.98996330903515	0.0936050096838203\\
1.97846069100187	0.0932645675978612\\
1.97419331157778	0.0931417700718592\\
1.96243414660234	0.0927694076154308\\
1.95842331412041	0.092650718077776\\
1.94763701324512	0.0922742476330004\\
1.94265331666304	0.0921224540567305\\
1.93433300306036	0.0917790876505701\\
1.92688331920567	0.0915462845749383\\
1.92272234539936	0.0912839276681397\\
1.9111133217483	0.0909161232392886\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.86979019154588	0.0893032877384181\\
1.8638033293762	0.0890903848230194\\
1.8638033293762	0.0888081277559877\\
1.84803333191883	0.0883129677735573\\
1.84803333191883	0.0883129677735573\\
-4.60517018598809	132\\
1.86654182628098	0.0883129677735573\\
1.87957332683357	0.0887296847849369\\
1.88372962058371	0.0888081277559877\\
1.89534332429094	0.0891117275624786\\
1.9111133217483	0.0890511648907152\\
1.92688331920567	0.0888587948309003\\
1.92906599526834	0.0888081277559877\\
1.94265331666304	0.0885278803069716\\
1.95842331412041	0.0887145546578686\\
1.96130154630082	0.0888081277559877\\
1.97419331157778	0.0890979370968747\\
1.98885167735938	0.0893032877384181\\
1.98996330903515	0.089324662645591\\
2.00573330649252	0.0893093221791381\\
2.00908513904204	0.0893032877384181\\
2.02150330394989	0.0892798830000436\\
2.02623250665079	0.0893032877384181\\
2.03727330140726	0.0893687340473407\\
2.05304329886463	0.0895507600995799\\
2.06881329632199	0.0897383290434893\\
2.07560638253609	0.0897984477208485\\
2.08458329377936	0.0899105671424335\\
2.10035329123673	0.0900755783003845\\
2.1161232886941	0.0902272703247138\\
2.12328962254991	0.0902936077032789\\
2.13189328615147	0.0903806648573049\\
2.14766328360884	0.0905442571130534\\
2.16343328106621	0.090717151413812\\
2.16981729323749	0.0907887676857093\\
2.17920327852358	0.0909087649462363\\
2.19497327598095	0.0911060397495743\\
2.20989133843416	0.0912839276681397\\
2.21074327343832	0.0912957512965418\\
2.22651327089568	0.0915118339937705\\
2.24228326835305	0.0917197907720149\\
2.24684293718864	0.0917790876505701\\
2.25805326581042	0.0919447110025226\\
2.27382326326779	0.0921699953582446\\
2.28130214604571	0.0922742476330004\\
2.28959326072516	0.0924049572054392\\
2.30536325818253	0.0926495678590107\\
2.31317510732312	0.0927694076154308\\
2.3211332556399	0.0929080323700568\\
2.33690325309727	0.0931705210836835\\
2.34271591024693	0.0932645675978612\\
2.35267325055464	0.0934503326090803\\
2.368443248012	0.0937349065286593\\
2.36985062790671	0.0937597275802916\\
2.38421324546937	0.0940478571134386\\
2.39490692616818	0.094254887562722\\
2.39998324292674	0.0943682421039025\\
2.41575324038411	0.0947083032033487\\
2.41772002176544	0.0947500475451524\\
2.43152323784148	0.0950848348130737\\
2.4384857894014	0.0952452075275828\\
2.44729323529885	0.0954946386066088\\
2.4564544941377	0.0957403675100132\\
2.46306323275622	0.0959535349898991\\
2.47217998400298	0.0962355274924436\\
2.47883323021359	0.096499918440181\\
2.48491721022426	0.096730687474874\\
2.4945856428326	0.0972258474573043\\
2.49460322767096	0.0972276244515154\\
2.49975292690593	0.0977210074397347\\
2.49966549511705	0.0982161674221651\\
2.49460322767096	0.0985485008023565\\
2.49147796628468	0.0987113274045955\\
2.47883323021359	0.0989999422855451\\
2.46606356356453	0.0992064873870259\\
2.46306323275622	0.0992364140840141\\
2.44729323529885	0.099350148343669\\
2.43152323784148	0.0994200266817221\\
2.41575324038411	0.0994503544837664\\
2.39998324292674	0.0994600202357036\\
2.38421324546937	0.0994382863286936\\
2.368443248012	0.0993998869147847\\
2.35267325055464	0.099347012267832\\
2.33690325309727	0.0992684881281075\\
2.32266299469791	0.0992064873870259\\
2.3211332556399	0.0991989589088676\\
2.30536325818253	0.0990729953260446\\
2.28959326072516	0.0989425356044992\\
2.27382326326779	0.0988077719005162\\
2.26320816636923	0.0987113274045955\\
2.25805326581042	0.0986596054134151\\
2.24228326835305	0.0984773144808742\\
2.22651327089568	0.0983048214607451\\
2.21911582899228	0.0982161674221651\\
2.21074327343832	0.0981030008620087\\
2.19497327598095	0.0978826539484682\\
2.18288320623497	0.0977210074397347\\
2.17920327852358	0.0976653850541787\\
2.16343328106621	0.0974030411925313\\
2.15185087482002	0.0972258474573043\\
2.14766328360884	0.0971533289918167\\
2.13189328615147	0.0968609596438383\\
2.12457698494127	0.096730687474874\\
2.1161232886941	0.0965633004832238\\
2.10035329123673	0.0962667284496241\\
2.09886287849463	0.0962355274924436\\
2.08458329377936	0.0959108372412704\\
2.07651493535048	0.0957403675100132\\
2.06881329632199	0.0955631789190494\\
2.05389745571473	0.0952452075275828\\
2.05304329886463	0.0952252997621157\\
2.03727330140726	0.0948191577814238\\
2.03463065024357	0.0947500475451524\\
2.02150330394989	0.0943975952405972\\
2.01621825127894	0.094254887562722\\
2.00573330649252	0.0939674750483752\\
1.99834655258136	0.0937597275802916\\
1.98996330903515	0.0935244646653294\\
1.98118208950222	0.0932645675978612\\
1.97419331157778	0.0930634594812372\\
1.96490718634776	0.0927694076154308\\
1.95842331412041	0.0925775352796144\\
1.94973378256877	0.0922742476330004\\
1.94265331666304	0.0920585905953403\\
1.93588051620371	0.0917790876505701\\
1.92688331920567	0.091497924694656\\
1.92348933185909	0.0912839276681397\\
1.9111133217483	0.0908918230892298\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.87144265053401	0.0893032877384181\\
1.8638033293762	0.0890316205945844\\
1.8638033293762	0.0888081277559877\\
1.84803333191883	0.0883129677735573\\
1.84803333191883	0.0883129677735573\\
-3.83764182165674	119\\
1.86486344059467	0.0883129677735573\\
1.87957332683357	0.0887833556468853\\
1.88088587480135	0.0888081277559877\\
1.89534332429094	0.0891860673847262\\
1.9111133217483	0.0891965750172648\\
1.92688331920567	0.0890724255462819\\
1.93826894707714	0.0888081277559877\\
1.94265331666304	0.0887176972468168\\
1.95050973845196	0.0888081277559877\\
1.95842331412041	0.0889242721395697\\
1.97419331157778	0.0892223364001998\\
1.97997179036507	0.0893032877384181\\
1.98996330903515	0.0894954087338387\\
2.00573330649252	0.0895817138289251\\
2.02150330394989	0.0896329359684725\\
2.03727330140726	0.0897102841391131\\
2.04787349415605	0.0897984477208485\\
2.05304329886463	0.0898425326790426\\
2.06881329632199	0.0900133694291639\\
2.08458329377936	0.0901885062989707\\
2.09434137212414	0.0902936077032789\\
2.10035329123673	0.0903721231099647\\
2.1161232886941	0.0905538515176551\\
2.13189328615147	0.0907184424311919\\
2.13876475891183	0.0907887676857093\\
2.14766328360884	0.0908961083924837\\
2.16343328106621	0.0910888187002785\\
2.17920327852358	0.0912763387104494\\
2.17983632403484	0.0912839276681397\\
2.19497327598095	0.0914938957620092\\
2.21074327343832	0.0917046609360087\\
2.2163982240205	0.0917790876505701\\
2.22651327089568	0.0919306324938557\\
2.24228326835305	0.0921633063674534\\
2.25007077449292	0.0922742476330004\\
2.25805326581042	0.0924046033664311\\
2.27382326326779	0.0926531998091421\\
2.28146088553312	0.0927694076154308\\
2.28959326072516	0.0929135407447657\\
2.30536325818253	0.0931870316959367\\
2.30998262149135	0.0932645675978612\\
2.3211332556399	0.0934778094320289\\
2.33650499994186	0.0937597275802916\\
2.33690325309727	0.093768286822151\\
2.35267325055464	0.0940992949322591\\
2.36047724439015	0.094254887562722\\
2.368443248012	0.0944440444086038\\
2.38213084511664	0.0947500475451524\\
2.38421324546937	0.0948061107979349\\
2.39998324292674	0.0952176114339128\\
2.40108955891242	0.0952452075275828\\
2.41575324038411	0.0956844238567825\\
2.41770069329583	0.0957403675100132\\
2.43115800090699	0.0962355274924436\\
2.43152323784148	0.0962550165786739\\
2.44107851671714	0.096730687474874\\
2.44667069763393	0.0972258474573043\\
2.44660669093887	0.0977210074397347\\
2.43603162597601	0.0982161674221651\\
2.43152323784148	0.0983096765925975\\
2.41575324038411	0.0985527245383118\\
2.39998324292674	0.0986981248355595\\
2.39770810511249	0.0987113274045955\\
2.38421324546937	0.0987608789769193\\
2.368443248012	0.0987781922014984\\
2.35267325055464	0.0987703313403522\\
2.33690325309727	0.098750938582982\\
2.32626852206415	0.0987113274045955\\
2.3211332556399	0.098688919054531\\
2.30536325818253	0.0986159735104116\\
2.28959326072516	0.0985194523315553\\
2.27382326326779	0.0984102357955984\\
2.25805326581042	0.09829098419335\\
2.24974380588784	0.0982161674221651\\
2.24228326835305	0.0981411592568608\\
2.22651327089568	0.0979767814190895\\
2.21074327343832	0.0978065336716444\\
2.2032163082189	0.0977210074397347\\
2.19497327598095	0.0976133243286204\\
2.17920327852358	0.0973982455672717\\
2.16599397809077	0.0972258474573043\\
2.16343328106621	0.0971877351043545\\
2.14766328360884	0.0969240697156873\\
2.13485521635252	0.096730687474874\\
2.13189328615147	0.0966801247961088\\
2.1161232886941	0.0963833279608037\\
2.10778508186977	0.0962355274924436\\
2.10035329123673	0.096087694577252\\
2.08458329377936	0.0957844017568175\\
2.0824991461495	0.0957403675100132\\
2.06881329632199	0.0954255025263251\\
2.060355769841	0.0952452075275828\\
2.05304329886463	0.0950747763507274\\
2.03802295229731	0.0947500475451524\\
2.03727330140726	0.0947323059518573\\
2.02150330394989	0.0943180822849693\\
2.01916294328692	0.094254887562722\\
2.00573330649252	0.0938867553735243\\
2.00121665434198	0.0937597275802916\\
1.98996330903515	0.0934439196468385\\
1.98390348800256	0.0932645675978612\\
1.97419331157778	0.0929851488906153\\
1.96738022609317	0.0927694076154308\\
1.95842331412041	0.0925043524814528\\
1.95183055189242	0.0922742476330004\\
1.94265331666304	0.0919947271339501\\
1.93742802934707	0.0917790876505701\\
1.92688331920567	0.0914495648143737\\
1.92425631831882	0.0912839276681397\\
1.9111133217483	0.0908675229391709\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.87309510952213	0.0893032877384181\\
1.8638033293762	0.0889728563661494\\
1.8638033293762	0.0888081277559877\\
1.85371201223332	0.0883129677735573\\
-3.07011345732539	5\\
1.8638033293762	0.0888081277559877\\
1.8638033293762	0.0883969636344844\\
1.87594714983831	0.0888081277559877\\
1.8638033293762	0.0889140921377144\\
1.8638033293762	0.0888081277559877\\
-3.07011345732539	107\\
1.87474756851025	0.0893032877384181\\
1.87957332683357	0.0888852112506863\\
1.89534332429094	0.0892604072069738\\
1.90613457264183	0.0893032877384181\\
1.9111133217483	0.0893642301363012\\
1.92321532348816	0.0893032877384181\\
1.92688331920567	0.0892860562616636\\
1.9378851427877	0.0893032877384181\\
1.94265331666304	0.0893175040645307\\
1.94357069088093	0.0893032877384181\\
1.95842331412041	0.0891663027169693\\
1.96817539689378	0.0893032877384181\\
1.97419331157778	0.0894015275346107\\
1.98996330903515	0.0896661548220864\\
2.00244231871838	0.0897984477208485\\
2.00573330649252	0.0898539345566655\\
2.02150330394989	0.0899767453715854\\
2.03727330140726	0.0900770041808248\\
2.05304329886463	0.0901927158239618\\
2.06493000487026	0.0902936077032789\\
2.06881329632199	0.0903331272509812\\
2.08458329377936	0.0905263194401358\\
2.10035329123673	0.0907091365903289\\
2.10741863588577	0.0907887676857093\\
2.1161232886941	0.0909071624192901\\
2.13189328615147	0.0911042571575628\\
2.14680740782996	0.0912839276681397\\
2.14766328360884	0.0912960235102196\\
2.16343328106621	0.0915108297900264\\
2.17920327852358	0.0917196242326057\\
2.18375465519322	0.0917790876505701\\
2.19497327598095	0.0919490846580719\\
2.21074327343832	0.0921761062007732\\
2.2176154619539	0.0922742476330004\\
2.22651327089568	0.0924259627295974\\
2.24228326835305	0.0926856291591663\\
2.24764590322951	0.0927694076154308\\
2.25805326581042	0.0929580327847811\\
2.27382326326779	0.0932325516765719\\
2.27567729157545	0.0932645675978612\\
2.28959326072516	0.0935453424840014\\
2.30092277308956	0.0937597275802916\\
2.30536325818253	0.0938611248501547\\
2.3211332556399	0.0942049845898614\\
2.3235296379463	0.094254887562722\\
2.33690325309727	0.0945886276903655\\
2.3436078656834	0.0947500475451524\\
2.35267325055464	0.0950166415953039\\
2.3609221591128	0.0952452075275828\\
2.368443248012	0.0955185258146633\\
2.37496067198949	0.0957403675100132\\
2.38421324546937	0.0961894552478372\\
2.38522785253683	0.0962355274924436\\
2.39056890290326	0.096730687474874\\
2.38905641370144	0.0972258474573043\\
2.38421324546937	0.0974233022655061\\
2.37365598165749	0.0977210074397347\\
2.368443248012	0.0977898755194026\\
2.35267325055464	0.0979321869684691\\
2.33690325309727	0.0979969602145996\\
2.3211332556399	0.0980203309994716\\
2.30536325818253	0.0980080587717556\\
2.28959326072516	0.0979625738856238\\
2.27382326326779	0.0979046447252565\\
2.25805326581042	0.097813571197611\\
2.24228326835305	0.0977295429316456\\
2.241237244196	0.0977210074397347\\
2.22651327089568	0.0975801906874042\\
2.21074327343832	0.0974313282117983\\
2.19497327598095	0.0972724786403774\\
2.19058331486379	0.0972258474573043\\
2.17920327852358	0.0970878541836202\\
2.16343328106621	0.0968830908651903\\
2.15142093052891	0.096730687474874\\
2.14766328360884	0.0966754932671083\\
2.13189328615147	0.0964209163298371\\
2.11927669665908	0.0962355274924436\\
2.1161232886941	0.0961820722695619\\
2.10035329123673	0.0958857274298974\\
2.0920773614619	0.0957403675100132\\
2.08458329377936	0.0955907723802825\\
2.06881329632199	0.0952878261336007\\
2.06681408396728	0.0952452075275828\\
2.05304329886463	0.0949242529393392\\
2.04498541995256	0.0947500475451524\\
2.03727330140726	0.0945675288921488\\
2.02304256723074	0.094254887562722\\
2.02150330394989	0.0942176397450356\\
2.00573330649252	0.0938060356986734\\
2.00408675610261	0.0937597275802916\\
1.98996330903515	0.0933633746283476\\
1.98662488650291	0.0932645675978612\\
1.97419331157778	0.0929068382999933\\
1.96985326583859	0.0927694076154308\\
1.95842331412041	0.0924311696832913\\
1.95392732121607	0.0922742476330004\\
1.94265331666304	0.0919308636725599\\
1.93897554249042	0.0917790876505701\\
1.92688331920567	0.0914012049340914\\
1.92502330477855	0.0912839276681397\\
1.9111133217483	0.0908432227891121\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.87957332683357	0.0897984477208485\\
1.87957332683357	0.0897984477208485\\
1.87474756851025	0.0893032877384181\\
-2.30258509299405	5\\
1.8638033293762	0.0888081277559877\\
1.8638033293762	0.0886249812189461\\
1.8692126016054	0.0888081277559877\\
1.8638033293762	0.0888553279092794\\
1.8638033293762	0.0888081277559877\\
-2.30258509299405	91\\
1.87640002749838	0.0893032877384181\\
1.87957332683357	0.0890283709788762\\
1.89249566428137	0.0893032877384181\\
1.89534332429094	0.0893757682578415\\
1.9111133217483	0.0895932284812205\\
1.92688331920567	0.0897557478795126\\
1.94265331666304	0.0897241731567748\\
1.95842331412041	0.0896448932812427\\
1.97419331157778	0.0896828056606432\\
1.98438213321012	0.0897984477208485\\
1.98996330903515	0.0898819369790816\\
2.00573330649252	0.0901254897060248\\
2.02050376936246	0.0902936077032789\\
2.02150330394989	0.0903089175074653\\
2.03727330140726	0.0904641588638923\\
2.05304329886463	0.0906019317293746\\
2.06881329632199	0.0907529950099763\\
2.07231332500535	0.0907887676857093\\
2.08458329377936	0.0909333594852781\\
2.10035329123673	0.0911266037953236\\
2.11341889497768	0.0912839276681397\\
2.1161232886941	0.0913231928939824\\
2.13189328615147	0.0915519806712816\\
2.14766328360884	0.0917634524171458\\
2.14883744414244	0.0917790876505701\\
2.16343328106621	0.0920109842766832\\
2.17920327852358	0.0922427733893045\\
2.18136683760807	0.0922742476330004\\
2.19497327598095	0.0925054115227332\\
2.21074327343832	0.0927568998661363\\
2.2115050165551	0.0927694076154308\\
2.22651327089568	0.0930598870411097\\
2.23807657651892	0.0932645675978612\\
2.24228326835305	0.0933543097560168\\
2.25805326581042	0.0936820788026141\\
2.2619284596103	0.0937597275802916\\
2.27382326326779	0.0940451725482061\\
2.28315901519044	0.094254887562722\\
2.28959326072516	0.0944417418078108\\
2.30112500949747	0.0947500475451524\\
2.30536325818253	0.0949018879585842\\
2.31542838557219	0.0952452075275828\\
2.3211332556399	0.0955275859720588\\
2.32579585504279	0.0957403675100132\\
2.32980277246308	0.0962355274924436\\
2.32442987665431	0.096730687474874\\
2.3211332556399	0.0968136161413401\\
2.30536325818253	0.0970587521813708\\
2.28959326072516	0.0971669476751603\\
2.27382326326779	0.0971851297913238\\
2.25805326581042	0.0971866301577618\\
2.24228326835305	0.0971186158956729\\
2.22651327089568	0.0970469235903414\\
2.21074327343832	0.0969359759838677\\
2.19497327598095	0.0968277805159709\\
2.18362593552684	0.096730687474874\\
2.17920327852358	0.096685003963481\\
2.16343328106621	0.0965049463699814\\
2.14766328360884	0.0963227945558733\\
2.14033181884628	0.0962355274924436\\
2.13189328615147	0.0961176103784955\\
2.1161232886941	0.0958830403432628\\
2.10618908966283	0.0957403675100132\\
2.10035329123673	0.0956421859756807\\
2.08458329377936	0.0953612353825502\\
2.07791775308113	0.0952452075275828\\
2.06881329632199	0.0950634819515778\\
2.05304329886463	0.0947737295279509\\
2.05194788760782	0.0947500475451524\\
2.03727330140726	0.0944027518324404\\
2.0305428505087	0.094254887562722\\
2.02150330394989	0.0940361443585029\\
2.00918217480352	0.0937597275802916\\
2.00573330649252	0.093674191557767\\
1.98996330903515	0.0932828296098567\\
1.98934628500326	0.0932645675978612\\
1.97419331157778	0.0928285277093714\\
1.972326305584	0.0927694076154308\\
1.95842331412041	0.0923579868851297\\
1.95602409053972	0.0922742476330004\\
1.94265331666304	0.0918670002111696\\
1.94052305563377	0.0917790876505701\\
1.92688331920567	0.0913528450538092\\
1.92579029123828	0.0912839276681397\\
1.9111133217483	0.0908189226390532\\
1.9111133217483	0.0907887676857093\\
1.89534332429094	0.0902936077032789\\
1.89534332429094	0.0902936077032789\\
1.8822030340888	0.0897984477208485\\
1.87957332683357	0.0896971529586672\\
1.87640002749838	0.0893032877384181\\
-1.5350567286627	5\\
1.8780524864865	0.0893032877384181\\
1.87957332683357	0.089171530707066\\
1.88576650626391	0.0893032877384181\\
1.87957332683357	0.0894920521930091\\
1.8780524864865	0.0893032877384181\\
-1.5350567286627	75\\
1.88752764278416	0.0897984477208485\\
1.89534332429094	0.0895470432228124\\
1.91007141139381	0.0897984477208485\\
1.9111133217483	0.089825744030105\\
1.92688331920567	0.0900598942606372\\
1.94265331666304	0.0901553031434075\\
1.95842331412041	0.0902213995571563\\
1.97419331157778	0.0901952224727285\\
1.98996330903515	0.090252659523679\\
1.99350830667948	0.0902936077032789\\
2.00573330649252	0.0904692750138461\\
2.02150330394989	0.0906743521785867\\
2.03122732946841	0.0907887676857093\\
2.03727330140726	0.0908834729711719\\
2.05304329886463	0.0910761444343045\\
2.06881329632199	0.0912543460340481\\
2.07155801929514	0.0912839276681397\\
2.08458329377936	0.0914540574888625\\
2.10035329123673	0.0916604297797153\\
2.10954608730529	0.0917790876505701\\
2.1161232886941	0.0918820297367407\\
2.13189328615147	0.0920999476350886\\
2.14282177465693	0.0922742476330004\\
2.14766328360884	0.092376058230168\\
2.16343328106621	0.0926467452126279\\
2.1709121544269	0.0927694076154308\\
2.17920327852358	0.0929412330174611\\
2.19497327598095	0.0932413167098616\\
2.19621361748031	0.0932645675978612\\
2.21074327343832	0.0936010349368353\\
2.21825867452525	0.0937597275802916\\
2.22651327089568	0.0939917914267204\\
2.23665927484864	0.094254887562722\\
2.24228326835305	0.0944614645926916\\
2.25088635630958	0.0947500475451524\\
2.25805326581042	0.0951561405241957\\
2.2598062767906	0.0952452075275828\\
2.25979748873951	0.0957403675100132\\
2.25805326581042	0.0958040279189143\\
2.24228326835305	0.0961118429001238\\
2.22651327089568	0.0961870383156681\\
2.21074327343832	0.0962242937147312\\
2.19497327598095	0.0961581575440054\\
2.17920327852358	0.0960768349305989\\
2.16343328106621	0.0959588930062459\\
2.14766328360884	0.0958399494419949\\
2.13692985343905	0.0957403675100132\\
2.13189328615147	0.0956826238565608\\
2.1161232886941	0.0954810878244948\\
2.10035329123673	0.0952918871658262\\
2.09700579728528	0.0952452075275828\\
2.08458329377936	0.0950375733602431\\
2.06881329632199	0.0948002807700967\\
2.06590114259452	0.0947500475451524\\
2.05304329886463	0.094490275860981\\
2.03914194120019	0.094254887562722\\
2.03727330140726	0.0942165788986265\\
2.02150330394989	0.0938546489719702\\
2.01727223399388	0.0937597275802916\\
2.00573330649252	0.0934735484996004\\
1.99668266620872	0.0932645675978612\\
1.98996330903515	0.0930924524282596\\
1.97647137324229	0.0927694076154308\\
1.97419331157778	0.092708521698264\\
1.95842331412041	0.0922848040869681\\
1.95812085986337	0.0922742476330004\\
1.94265331666304	0.0918031367497794\\
1.94207056877713	0.0917790876505701\\
1.92688331920567	0.0913044851735269\\
1.92655727769801	0.0912839276681397\\
1.9111133217483	0.0907946224889944\\
1.9111133217483	0.0907887676857093\\
1.89750321716123	0.0902936077032789\\
1.89534332429094	0.0902137009981467\\
1.88752764278416	0.0897984477208485\\
-0.767528364331349	5\\
1.89285225147952	0.0897984477208485\\
1.89534332429094	0.0897183181877832\\
1.90003757101968	0.0897984477208485\\
1.89534332429094	0.0899308003695627\\
1.89285225147952	0.0897984477208485\\
-0.767528364331349	55\\
1.90515007294974	0.0902936077032789\\
1.9111133217483	0.0900886138717403\\
1.92387760912293	0.0902936077032789\\
1.92688331920567	0.0903734693679379\\
1.94265331666304	0.0906149429111481\\
1.95842331412041	0.0907881252224988\\
1.95852352031476	0.0907887676857093\\
1.97419331157778	0.0909360154209259\\
1.98996330903515	0.0910010605285708\\
2.00573330649252	0.0910690116434394\\
2.02150330394989	0.0912034493918823\\
2.02828120530121	0.0912839276681397\\
2.03727330140726	0.0914247610730931\\
2.05304329886463	0.0916548712967428\\
2.06229904758068	0.0917790876505701\\
2.06881329632199	0.0918987564429446\\
2.08458329377936	0.0921562723739706\\
2.09272729986482	0.0922742476330004\\
2.10035329123673	0.0924156232680511\\
2.1161232886941	0.0926944057637284\\
2.12053002356513	0.0927694076154308\\
2.13189328615147	0.0930241820897468\\
2.14405595713322	0.0932645675978612\\
2.14766328360884	0.0933705188186489\\
2.16229790634541	0.0937597275802916\\
2.16343328106621	0.0938119525253198\\
2.1747688258479	0.094254887562722\\
2.17448001000919	0.0947500475451524\\
2.16343328106621	0.0948966892196034\\
2.14766328360884	0.0949204096519657\\
2.13189328615147	0.0948868364139619\\
2.1161232886941	0.0948057398640851\\
2.10693492392263	0.0947500475451524\\
2.10035329123673	0.094694644233908\\
2.08458329377936	0.0945030587748658\\
2.06881329632199	0.0943266263719937\\
2.06302530907226	0.094254887562722\\
2.05304329886463	0.0940937642401152\\
2.03727330140726	0.0938433472180622\\
2.03223348304562	0.0937597275802916\\
2.02150330394989	0.0935355373387725\\
2.00573330649252	0.0932729054414339\\
2.00537220735719	0.0932645675978612\\
1.98996330903515	0.0928698713375545\\
1.98576745126379	0.0927694076154308\\
1.97419331157778	0.0924600647555875\\
1.9668386924275	0.0922742476330004\\
1.95842331412041	0.0920366883902747\\
1.94899057934615	0.0917790876505701\\
1.94265331666304	0.0915889362932314\\
1.93264002087349	0.0912839276681397\\
1.92688331920567	0.0910978488711447\\
1.91809725324275	0.0907887676857093\\
1.9111133217483	0.0905445287410985\\
1.90515007294974	0.0902936077032789\\
0	3\\
1.94265331666304	0.0912839276681397\\
1.94265331666304	0.0912839276681397\\
1.94265331666304	0.0912839276681397\\
0	3\\
1.94265331666304	0.0912839276681397\\
1.94265331666304	0.0912839276681397\\
1.94265331666304	0.0912839276681397\\
};
\end{axis}


==> fig9_part1b_220222.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%

\begin{axis}[%
width=0.7\linewidth,
height=0.7\linewidth,
name = mv,
at={(mb.below south west)},
anchor = above north west,
scale only axis,
colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.2444,0.1534,0.6728); rgb(2pt)=(0.2464,0.1569,0.6847); rgb(3pt)=(0.2484,0.1607,0.6961); rgb(4pt)=(0.2503,0.1648,0.7071); rgb(5pt)=(0.2522,0.1689,0.7179); rgb(6pt)=(0.254,0.1732,0.7286); rgb(7pt)=(0.2558,0.1773,0.7393); rgb(8pt)=(0.2576,0.1814,0.7501); rgb(9pt)=(0.2594,0.1854,0.761); rgb(11pt)=(0.2628,0.1932,0.7828); rgb(12pt)=(0.2645,0.1972,0.7937); rgb(13pt)=(0.2661,0.2011,0.8043); rgb(14pt)=(0.2676,0.2052,0.8148); rgb(15pt)=(0.2691,0.2094,0.8249); rgb(16pt)=(0.2704,0.2138,0.8346); rgb(17pt)=(0.2717,0.2184,0.8439); rgb(18pt)=(0.2729,0.2231,0.8528); rgb(19pt)=(0.274,0.228,0.8612); rgb(20pt)=(0.2749,0.233,0.8692); rgb(21pt)=(0.2758,0.2382,0.8767); rgb(22pt)=(0.2766,0.2435,0.884); rgb(23pt)=(0.2774,0.2489,0.8908); rgb(24pt)=(0.2781,0.2543,0.8973); rgb(25pt)=(0.2788,0.2598,0.9035); rgb(26pt)=(0.2794,0.2653,0.9094); rgb(27pt)=(0.2798,0.2708,0.915); rgb(28pt)=(0.2802,0.2764,0.9204); rgb(29pt)=(0.2806,0.2819,0.9255); rgb(30pt)=(0.2809,0.2875,0.9305); rgb(31pt)=(0.2811,0.293,0.9352); rgb(32pt)=(0.2813,0.2985,0.9397); rgb(33pt)=(0.2814,0.304,0.9441); rgb(34pt)=(0.2814,0.3095,0.9483); rgb(35pt)=(0.2813,0.315,0.9524); rgb(36pt)=(0.2811,0.3204,0.9563); rgb(37pt)=(0.2809,0.3259,0.96); rgb(38pt)=(0.2807,0.3313,0.9636); rgb(39pt)=(0.2803,0.3367,0.967); rgb(40pt)=(0.2798,0.3421,0.9702); rgb(41pt)=(0.2791,0.3475,0.9733); rgb(42pt)=(0.2784,0.3529,0.9763); rgb(43pt)=(0.2776,0.3583,0.9791); rgb(44pt)=(0.2766,0.3638,0.9817); rgb(45pt)=(0.2754,0.3693,0.984); rgb(46pt)=(0.2741,0.3748,0.9862); rgb(47pt)=(0.2726,0.3804,0.9881); rgb(48pt)=(0.271,0.386,0.9898); rgb(49pt)=(0.2691,0.3916,0.9912); rgb(50pt)=(0.267,0.3973,0.9924); rgb(51pt)=(0.2647,0.403,0.9935); rgb(52pt)=(0.2621,0.4088,0.9946); rgb(53pt)=(0.2591,0.4145,0.9955); rgb(54pt)=(0.2556,0.4203,0.9965); rgb(55pt)=(0.2517,0.4261,0.9974); rgb(56pt)=(0.2473,0.4319,0.9983); rgb(57pt)=(0.2424,0.4378,0.9991); rgb(58pt)=(0.2369,0.4437,0.9996); rgb(59pt)=(0.2311,0.4497,0.9995); rgb(60pt)=(0.225,0.4559,0.9985); rgb(61pt)=(0.2189,0.462,0.9968); rgb(62pt)=(0.2128,0.4682,0.9948); rgb(63pt)=(0.2066,0.4743,0.9926); rgb(64pt)=(0.2006,0.4803,0.9906); rgb(65pt)=(0.195,0.4861,0.9887); rgb(66pt)=(0.1903,0.4919,0.9867); rgb(67pt)=(0.1869,0.4975,0.9844); rgb(68pt)=(0.1847,0.503,0.9819); rgb(69pt)=(0.1831,0.5084,0.9793); rgb(70pt)=(0.1818,0.5138,0.9766); rgb(71pt)=(0.1806,0.5191,0.9738); rgb(72pt)=(0.1795,0.5244,0.9709); rgb(73pt)=(0.1785,0.5296,0.9677); rgb(74pt)=(0.1778,0.5349,0.9641); rgb(75pt)=(0.1773,0.5401,0.9602); rgb(76pt)=(0.1768,0.5452,0.956); rgb(77pt)=(0.1764,0.5504,0.9516); rgb(78pt)=(0.1755,0.5554,0.9473); rgb(79pt)=(0.174,0.5605,0.9432); rgb(80pt)=(0.1716,0.5655,0.9393); rgb(81pt)=(0.1686,0.5705,0.9357); rgb(82pt)=(0.1649,0.5755,0.9323); rgb(83pt)=(0.161,0.5805,0.9289); rgb(84pt)=(0.1573,0.5854,0.9254); rgb(85pt)=(0.154,0.5902,0.9218); rgb(86pt)=(0.1513,0.595,0.9182); rgb(87pt)=(0.1492,0.5997,0.9147); rgb(88pt)=(0.1475,0.6043,0.9113); rgb(89pt)=(0.1461,0.6089,0.908); rgb(90pt)=(0.1446,0.6135,0.905); rgb(91pt)=(0.1429,0.618,0.9022); rgb(92pt)=(0.1408,0.6226,0.8998); rgb(93pt)=(0.1383,0.6272,0.8975); rgb(94pt)=(0.1354,0.6317,0.8953); rgb(95pt)=(0.1321,0.6363,0.8932); rgb(96pt)=(0.1288,0.6408,0.891); rgb(97pt)=(0.1253,0.6453,0.8887); rgb(98pt)=(0.1219,0.6497,0.8862); rgb(99pt)=(0.1185,0.6541,0.8834); rgb(100pt)=(0.1152,0.6584,0.8804); rgb(101pt)=(0.1119,0.6627,0.877); rgb(102pt)=(0.1085,0.6669,0.8734); rgb(103pt)=(0.1048,0.671,0.8695); rgb(104pt)=(0.1009,0.675,0.8653); rgb(105pt)=(0.0964,0.6789,0.8609); rgb(106pt)=(0.0914,0.6828,0.8562); rgb(107pt)=(0.0855,0.6865,0.8513); rgb(108pt)=(0.0789,0.6902,0.8462); rgb(109pt)=(0.0713,0.6938,0.8409); rgb(110pt)=(0.0628,0.6972,0.8355); rgb(111pt)=(0.0535,0.7006,0.8299); rgb(112pt)=(0.0433,0.7039,0.8242); rgb(113pt)=(0.0328,0.7071,0.8183); rgb(114pt)=(0.0234,0.7103,0.8124); rgb(115pt)=(0.0155,0.7133,0.8064); rgb(116pt)=(0.0091,0.7163,0.8003); rgb(117pt)=(0.0046,0.7192,0.7941); rgb(118pt)=(0.0019,0.722,0.7878); rgb(119pt)=(0.0009,0.7248,0.7815); rgb(120pt)=(0.0018,0.7275,0.7752); rgb(121pt)=(0.0046,0.7301,0.7688); rgb(122pt)=(0.0094,0.7327,0.7623); rgb(123pt)=(0.0162,0.7352,0.7558); rgb(124pt)=(0.0253,0.7376,0.7492); rgb(125pt)=(0.0369,0.74,0.7426); rgb(126pt)=(0.0504,0.7423,0.7359); rgb(127pt)=(0.0638,0.7446,0.7292); rgb(128pt)=(0.077,0.7468,0.7224); rgb(129pt)=(0.0899,0.7489,0.7156); rgb(130pt)=(0.1023,0.751,0.7088); rgb(131pt)=(0.1141,0.7531,0.7019); rgb(132pt)=(0.1252,0.7552,0.695); rgb(133pt)=(0.1354,0.7572,0.6881); rgb(134pt)=(0.1448,0.7593,0.6812); rgb(135pt)=(0.1532,0.7614,0.6741); rgb(136pt)=(0.1609,0.7635,0.6671); rgb(137pt)=(0.1678,0.7656,0.6599); rgb(138pt)=(0.1741,0.7678,0.6527); rgb(139pt)=(0.1799,0.7699,0.6454); rgb(140pt)=(0.1853,0.7721,0.6379); rgb(141pt)=(0.1905,0.7743,0.6303); rgb(142pt)=(0.1954,0.7765,0.6225); rgb(143pt)=(0.2003,0.7787,0.6146); rgb(144pt)=(0.2061,0.7808,0.6065); rgb(145pt)=(0.2118,0.7828,0.5983); rgb(146pt)=(0.2178,0.7849,0.5899); rgb(147pt)=(0.2244,0.7869,0.5813); rgb(148pt)=(0.2318,0.7887,0.5725); rgb(149pt)=(0.2401,0.7905,0.5636); rgb(150pt)=(0.2491,0.7922,0.5546); rgb(151pt)=(0.2589,0.7937,0.5454); rgb(152pt)=(0.2695,0.7951,0.536); rgb(153pt)=(0.2809,0.7964,0.5266); rgb(154pt)=(0.2929,0.7975,0.517); rgb(155pt)=(0.3052,0.7985,0.5074); rgb(156pt)=(0.3176,0.7994,0.4975); rgb(157pt)=(0.3301,0.8002,0.4876); rgb(158pt)=(0.3424,0.8009,0.4774); rgb(159pt)=(0.3548,0.8016,0.4669); rgb(160pt)=(0.3671,0.8021,0.4563); rgb(161pt)=(0.3795,0.8026,0.4454); rgb(162pt)=(0.3921,0.8029,0.4344); rgb(163pt)=(0.405,0.8031,0.4233); rgb(164pt)=(0.4184,0.803,0.4122); rgb(165pt)=(0.4322,0.8028,0.4013); rgb(166pt)=(0.4463,0.8024,0.3904); rgb(167pt)=(0.4608,0.8018,0.3797); rgb(168pt)=(0.4753,0.8011,0.3691); rgb(169pt)=(0.4899,0.8002,0.3586); rgb(170pt)=(0.5044,0.7993,0.348); rgb(171pt)=(0.5187,0.7982,0.3374); rgb(172pt)=(0.5329,0.797,0.3267); rgb(173pt)=(0.547,0.7957,0.3159); rgb(175pt)=(0.5748,0.7929,0.2941); rgb(176pt)=(0.5886,0.7913,0.2833); rgb(177pt)=(0.6024,0.7896,0.2726); rgb(178pt)=(0.6161,0.7878,0.2622); rgb(179pt)=(0.6297,0.7859,0.2521); rgb(180pt)=(0.6433,0.7839,0.2423); rgb(181pt)=(0.6567,0.7818,0.2329); rgb(182pt)=(0.6701,0.7796,0.2239); rgb(183pt)=(0.6833,0.7773,0.2155); rgb(184pt)=(0.6963,0.775,0.2075); rgb(185pt)=(0.7091,0.7727,0.1998); rgb(186pt)=(0.7218,0.7703,0.1924); rgb(187pt)=(0.7344,0.7679,0.1852); rgb(188pt)=(0.7468,0.7654,0.1782); rgb(189pt)=(0.759,0.7629,0.1717); rgb(190pt)=(0.771,0.7604,0.1658); rgb(191pt)=(0.7829,0.7579,0.1608); rgb(192pt)=(0.7945,0.7554,0.157); rgb(193pt)=(0.806,0.7529,0.1546); rgb(194pt)=(0.8172,0.7505,0.1535); rgb(195pt)=(0.8281,0.7481,0.1536); rgb(196pt)=(0.8389,0.7457,0.1546); rgb(197pt)=(0.8495,0.7435,0.1564); rgb(198pt)=(0.86,0.7413,0.1587); rgb(199pt)=(0.8703,0.7392,0.1615); rgb(200pt)=(0.8804,0.7372,0.165); rgb(201pt)=(0.8903,0.7353,0.1695); rgb(202pt)=(0.9,0.7336,0.1749); rgb(203pt)=(0.9093,0.7321,0.1815); rgb(204pt)=(0.9184,0.7308,0.189); rgb(205pt)=(0.9272,0.7298,0.1973); rgb(206pt)=(0.9357,0.729,0.2061); rgb(207pt)=(0.944,0.7285,0.2151); rgb(208pt)=(0.9523,0.7284,0.2237); rgb(209pt)=(0.9606,0.7285,0.2312); rgb(210pt)=(0.9689,0.7292,0.2373); rgb(211pt)=(0.977,0.7304,0.2418); rgb(212pt)=(0.9842,0.733,0.2446); rgb(213pt)=(0.99,0.7365,0.2429); rgb(214pt)=(0.9946,0.7407,0.2394); rgb(215pt)=(0.9966,0.7458,0.2351); rgb(216pt)=(0.9971,0.7513,0.2309); rgb(217pt)=(0.9972,0.7569,0.2267); rgb(218pt)=(0.9971,0.7626,0.2224); rgb(219pt)=(0.9969,0.7683,0.2181); rgb(220pt)=(0.9966,0.774,0.2138); rgb(221pt)=(0.9962,0.7798,0.2095); rgb(222pt)=(0.9957,0.7856,0.2053); rgb(223pt)=(0.9949,0.7915,0.2012); rgb(224pt)=(0.9938,0.7974,0.1974); rgb(225pt)=(0.9923,0.8034,0.1939); rgb(226pt)=(0.9906,0.8095,0.1906); rgb(227pt)=(0.9885,0.8156,0.1875); rgb(228pt)=(0.9861,0.8218,0.1846); rgb(229pt)=(0.9835,0.828,0.1817); rgb(230pt)=(0.9807,0.8342,0.1787); rgb(231pt)=(0.9778,0.8404,0.1757); rgb(232pt)=(0.9748,0.8467,0.1726); rgb(233pt)=(0.972,0.8529,0.1695); rgb(234pt)=(0.9694,0.8591,0.1665); rgb(235pt)=(0.9671,0.8654,0.1636); rgb(236pt)=(0.9651,0.8716,0.1608); rgb(237pt)=(0.9634,0.8778,0.1582); rgb(238pt)=(0.9619,0.884,0.1557); rgb(239pt)=(0.9608,0.8902,0.1532); rgb(240pt)=(0.9601,0.8963,0.1507); rgb(241pt)=(0.9596,0.9023,0.148); rgb(242pt)=(0.9595,0.9084,0.145); rgb(243pt)=(0.9597,0.9143,0.1418); rgb(244pt)=(0.9601,0.9203,0.1382); rgb(245pt)=(0.9608,0.9262,0.1344); rgb(246pt)=(0.9618,0.932,0.1304); rgb(247pt)=(0.9629,0.9379,0.1261); rgb(248pt)=(0.9642,0.9437,0.1216); rgb(249pt)=(0.9657,0.9494,0.1168); rgb(250pt)=(0.9674,0.9552,0.1116); rgb(251pt)=(0.9692,0.9609,0.1061); rgb(252pt)=(0.9711,0.9667,0.1001); rgb(253pt)=(0.973,0.9724,0.0938); rgb(254pt)=(0.9749,0.9782,0.0872); rgb(255pt)=(0.9769,0.9839,0.0805)},
xmin=1.76918334463198,
xmax=3.33041309291151,
ymin=0.157324708585984,
ymax=0.374422810439933,
xlabel = m,
ylabel = v,
axis background/.style={fill=white}
]
\addplot[contour prepared, contour prepared format=matlab, contour/labels=false] table[row sep=crcr] {%
%
-6.90775527898214	5\\
1.84803333191883	0.161755282093207\\
1.84803333191883	0.161755282093207\\
1.85081405811951	0.161755282093207\\
1.84803333191883	0.1643490524781\\
1.84803333191883	0.161755282093207\\
-6.90775527898214	147\\
1.85142333869075	0.16618585560043\\
1.8638033293762	0.164607027079521\\
1.87957332683357	0.16618585560043\\
1.89291318323343	0.16618585560043\\
1.89534332429094	0.166770708739558\\
1.9111133217483	0.170616429107654\\
1.92688331920567	0.167131025894254\\
1.94265331666304	0.168223700857689\\
1.95842331412041	0.169847331758262\\
1.97419331157778	0.170616429107654\\
1.97602984018968	0.170616429107654\\
1.98996330903515	0.173286061676318\\
2.00573330649252	0.173533880389846\\
2.02150330394989	0.174590929935866\\
2.03463836776162	0.175047002614877\\
2.03727330140726	0.17520308933539\\
2.05304329886463	0.177053796229388\\
2.06881329632199	0.17871548690505\\
2.07977456466891	0.179477576122101\\
2.08458329377936	0.180033745069131\\
2.10035329123673	0.181787262783968\\
2.1161232886941	0.183053984701747\\
2.12519656001405	0.183908149629324\\
2.13189328615147	0.184717345312121\\
2.14766328360884	0.186405040786818\\
2.16343328106621	0.187924903947915\\
2.16792223546936	0.188338723136548\\
2.17920327852358	0.189707704012049\\
2.19497327598095	0.191415944465396\\
2.20859887437887	0.192769296643771\\
2.21074327343832	0.193049930444195\\
2.22651327089568	0.195010477114869\\
2.24228326835305	0.196730708490644\\
2.246854930257	0.197199870150995\\
2.25805326581042	0.198721230969574\\
2.27382326326779	0.200630047183446\\
2.2828111374795	0.201630443658218\\
2.28959326072516	0.202661112801988\\
2.30536325818253	0.204824525735123\\
2.31558681194529	0.206061017165442\\
2.3211332556399	0.206884125420127\\
2.33690325309727	0.209250822448116\\
2.34628073961166	0.210491590672665\\
2.35267325055464	0.211388059579642\\
2.368443248012	0.213846202453704\\
2.37523617468612	0.214922164179889\\
2.38421324546937	0.216185691636085\\
2.39998324292674	0.218558631029591\\
2.40478592517125	0.219352737687112\\
2.41575324038411	0.221078818742747\\
2.43152323784148	0.22327329751286\\
2.43473098220307	0.223783311194335\\
2.44729323529885	0.225728119370047\\
2.46306323275622	0.228078894788097\\
2.46394374938981	0.228213884701559\\
2.47883323021359	0.230584268825854\\
2.49258385094748	0.232644458208782\\
2.49460322767096	0.23298732621964\\
2.51037322512833	0.23548564200267\\
2.52099256783758	0.237075031716006\\
2.52614322258569	0.238001068664826\\
2.54191322004306	0.240557961073588\\
2.54810978838268	0.241505605223229\\
2.55768321750043	0.243297655822109\\
2.5734532149578	0.245814665239705\\
2.57423386263974	0.245936178730453\\
2.58922321241517	0.248892643808947\\
2.59817660993654	0.250366752237676\\
2.60499320987254	0.252041274487898\\
2.6197790070476	0.2547973257449\\
2.62076320732991	0.255177183661657\\
2.63559151241761	0.259227899252123\\
2.63653320478728	0.261640261358474\\
2.63782738225677	0.263658472759347\\
2.63653320478728	0.263787675529053\\
2.62076320732991	0.264144656202457\\
2.60499320987254	0.263794805731867\\
2.60232044291311	0.263658472759347\\
2.58922321241517	0.262637447530704\\
2.5734532149578	0.261415891777318\\
2.55768321750043	0.26028294200291\\
2.54235059480421	0.259227899252123\\
2.54191322004306	0.259184699073275\\
2.52614322258569	0.257413104560417\\
2.51037322512833	0.255960600422994\\
2.49632731118751	0.2547973257449\\
2.49460322767096	0.254600070852478\\
2.47883323021359	0.252677933383712\\
2.46306323275622	0.251147656465892\\
2.45488321674664	0.250366752237676\\
2.44729323529885	0.249398710485481\\
2.43152323784148	0.247541053102202\\
2.41575324038411	0.246041634077822\\
2.41478209656204	0.245936178730453\\
2.39998324292674	0.243893574311754\\
2.38421324546937	0.242199549772687\\
2.37759139242063	0.241505605223229\\
2.368443248012	0.240219402987597\\
2.35267325055464	0.238281472797498\\
2.34081614965576	0.237075031716006\\
2.33690325309727	0.236515277232669\\
2.3211332556399	0.234303189662913\\
2.30536325818253	0.232719610581084\\
2.30482006585671	0.232644458208782\\
2.28959326072516	0.230268103493475\\
2.27382326326779	0.228622574509884\\
2.27079643908593	0.228213884701559\\
2.25805326581042	0.226168891748209\\
2.24228326835305	0.224451607565737\\
2.23731868228737	0.223783311194335\\
2.22651327089568	0.221999334185325\\
2.21074327343832	0.220226377265038\\
2.20435154928965	0.219352737687112\\
2.19497327598095	0.217757623323617\\
2.17920327852358	0.215958176098478\\
2.17195878986729	0.214922164179889\\
2.16343328106621	0.213414482404836\\
2.14766328360884	0.21165066139633\\
2.14013410432578	0.210491590672665\\
2.13189328615147	0.208979781549905\\
2.1161232886941	0.207308838543676\\
2.1080598891171	0.206061017165442\\
2.10035329123673	0.204622189146972\\
2.08458329377936	0.202985307649651\\
2.0762260390161	0.201630443658218\\
2.06881329632199	0.200175190943971\\
2.05304329886463	0.198536024517639\\
2.03727330140726	0.197252797380452\\
2.03689825930068	0.197199870150995\\
2.02150330394989	0.194010173747785\\
2.00573330649252	0.192855908288938\\
2.00479495332097	0.192769296643771\\
1.98996330903515	0.189377228052524\\
1.97419331157778	0.188338723136548\\
1.9735789161225	0.188338723136548\\
1.95842331412041	0.184498086910803\\
1.9431612687362	0.183908149629324\\
1.94265331666304	0.183871789655444\\
1.92688331920567	0.179493576990181\\
1.92598397016355	0.179477576122101\\
1.9111133217483	0.178909417334573\\
1.89706358834176	0.175047002614877\\
1.89534332429094	0.174600555116199\\
1.87957332683357	0.17357126408106\\
1.86901352749556	0.170616429107654\\
1.8638033293762	0.169194251600785\\
1.85142333869075	0.16618585560043\\
-6.14022691465079	5\\
1.84803333191883	0.161755282093207\\
1.84803333191883	0.161755282093207\\
1.84953774964522	0.161755282093207\\
1.84803333191883	0.163158553707745\\
1.84803333191883	0.161755282093207\\
-6.14022691465079	137\\
1.85362052511993	0.16618585560043\\
1.8638033293762	0.164887235739469\\
1.87957332683357	0.16618585560043\\
1.89077767748032	0.16618585560043\\
1.89534332429094	0.167284653080141\\
1.9111133217483	0.170616429107654\\
1.92688331920567	0.167898690775837\\
1.94265331666304	0.168863444835975\\
1.95842331412041	0.170077635644345\\
1.97346968310796	0.170616429107654\\
1.97419331157778	0.170728441314162\\
1.98996330903515	0.173682548016239\\
2.00573330649252	0.174099729045624\\
2.01946021554274	0.175047002614877\\
2.02150330394989	0.175285529165801\\
2.03727330140726	0.176239387620853\\
2.05304329886463	0.177975397106186\\
2.06881329632199	0.179350815881424\\
2.07063651200684	0.179477576122101\\
2.08458329377936	0.181090635779804\\
2.10035329123673	0.182680017591846\\
2.11557384653487	0.183908149629324\\
2.1161232886941	0.183973249093315\\
2.13189328615147	0.1858709998617\\
2.14766328360884	0.187443141638108\\
2.15719458267742	0.188338723136548\\
2.16343328106621	0.189126886323956\\
2.17920327852358	0.190959089898814\\
2.19497327598095	0.192555718019056\\
2.19712359325478	0.192769296643771\\
2.21074327343832	0.19455168066116\\
2.22651327089568	0.196360668978647\\
2.23444213467328	0.197199870150995\\
2.24228326835305	0.198390386112082\\
2.25805326581042	0.200333043089417\\
2.26945914757754	0.201630443658218\\
2.27382326326779	0.202272856316873\\
2.28959326072516	0.204634871048949\\
2.30075841091005	0.206061017165442\\
2.30536325818253	0.206689418586178\\
2.3211332556399	0.209045395375938\\
2.33102228228799	0.210491590672665\\
2.33690325309727	0.211302920964759\\
2.35267325055464	0.213572336290238\\
2.36111688758451	0.214922164179889\\
2.368443248012	0.215993378413039\\
2.38421324546937	0.218247172405608\\
2.39137396289433	0.219352737687112\\
2.39998324292674	0.22070013689659\\
2.41575324038411	0.223206733774212\\
2.4199167490229	0.223783311194335\\
2.43152323784148	0.225401824935178\\
2.44729323529885	0.227757918034862\\
2.45035525642586	0.228213884701559\\
2.46306323275622	0.230300870753907\\
2.47876158922593	0.232644458208782\\
2.47883323021359	0.232657468404788\\
2.49460322767096	0.235333238774012\\
2.50632041017598	0.237075031716006\\
2.51037322512833	0.237861947424269\\
2.52614322258569	0.240570078999142\\
2.53219975043949	0.241505605223229\\
2.54191322004306	0.243497075643028\\
2.55658001633924	0.245936178730453\\
2.55768321750043	0.246240060391218\\
2.5734532149578	0.2496528751785\\
2.5775517648276	0.250366752237676\\
2.58922321241517	0.254125228761135\\
2.59220810793359	0.2547973257449\\
2.58922321241517	0.256786106713119\\
2.5734532149578	0.258008486531485\\
2.55768321750043	0.25735969745039\\
2.54191322004306	0.256436968116571\\
2.52614322258569	0.255466809134969\\
2.51609086796852	0.2547973257449\\
2.51037322512833	0.254233351788938\\
2.49460322767096	0.25260216728753\\
2.47883323021359	0.251238696593916\\
2.46804527682937	0.250366752237676\\
2.46306323275622	0.249791752757011\\
2.44729323529885	0.247950120102414\\
2.43152323784148	0.246487450100931\\
2.42560200224452	0.245936178730453\\
2.41575324038411	0.244662512302261\\
2.39998324292674	0.242860279391777\\
2.38520152051974	0.241505605223229\\
2.38421324546937	0.241375893478755\\
2.368443248012	0.239198944344502\\
2.35267325055464	0.237563387044252\\
2.34787361426046	0.237075031716006\\
2.33690325309727	0.235505680532521\\
2.3211332556399	0.2336209312624\\
2.31132271486634	0.232644458208782\\
2.30536325818253	0.231775492713589\\
2.28959326072516	0.229618947235244\\
2.27522499787318	0.228213884701559\\
2.27382326326779	0.228005230928187\\
2.25805326581042	0.225553131706702\\
2.24228326835305	0.223978784295115\\
2.24083115358201	0.223783311194335\\
2.22651327089568	0.221419424008165\\
2.21074327343832	0.219789795398387\\
2.20754567067615	0.219352737687112\\
2.19497327598095	0.217214347527035\\
2.17920327852358	0.2155526189942\\
2.17479471654796	0.214922164179889\\
2.16343328106621	0.212912966885751\\
2.14766328360884	0.211270674820911\\
2.14260244986594	0.210491590672665\\
2.13189328615147	0.208526954266642\\
2.1161232886941	0.206949300226082\\
2.11038321933773	0.206061017165442\\
2.10035329123673	0.204188421527395\\
2.08458329377936	0.202647667868028\\
2.07830871424481	0.201630443658218\\
2.06881329632199	0.199766324900111\\
2.05304329886463	0.198209819794314\\
2.04036382163542	0.197199870150995\\
2.03727330140726	0.196742664301062\\
2.02150330394989	0.19369347462431\\
2.00725821322587	0.192769296643771\\
2.00573330649252	0.192572785826513\\
1.98996330903515	0.189065127322133\\
1.97702061809753	0.188338723136548\\
1.97419331157778	0.188027950998852\\
1.95842331412041	0.184181353900221\\
1.95135534924942	0.183908149629324\\
1.94265331666304	0.18328524503997\\
1.92887628059086	0.179477576122101\\
1.92688331920567	0.178974147267329\\
1.9111133217483	0.17834540709196\\
1.89911520478442	0.175047002614877\\
1.89534332429094	0.174068114164108\\
1.87957332683357	0.173023921053712\\
1.87096958683216	0.170616429107654\\
1.8638033293762	0.168660324957904\\
1.85362052511993	0.16618585560043\\
-5.37269855031944	5\\
1.84803333191883	0.161755282093207\\
1.84803333191883	0.161755282093207\\
1.84826144117093	0.161755282093207\\
1.84803333191883	0.16196805493739\\
1.84803333191883	0.161755282093207\\
-5.37269855031944	129\\
1.85581771154911	0.16618585560043\\
1.8638033293762	0.165167444399418\\
1.87957332683357	0.16618585560043\\
1.88864217172722	0.16618585560043\\
1.89534332429094	0.167798597420725\\
1.9111133217483	0.170616429107654\\
1.92688331920567	0.16866635565742\\
1.94265331666304	0.169503188814261\\
1.95842331412041	0.170307939530428\\
1.9670382070689	0.170616429107654\\
1.97419331157778	0.171723985094269\\
1.98996330903515	0.17407903435616\\
2.00573330649252	0.174665577701402\\
2.01126052193134	0.175047002614877\\
2.02150330394989	0.176242827258684\\
2.03727330140726	0.177275685906317\\
2.05304329886463	0.178896997982984\\
2.05998838068964	0.179477576122101\\
2.06881329632199	0.180427944017999\\
2.08458329377936	0.182147526490476\\
2.10035329123673	0.183572772399723\\
2.10450970725155	0.183908149629324\\
2.1161232886941	0.185284159668289\\
2.13189328615147	0.18702465441128\\
2.14596699215937	0.188338723136548\\
2.14766328360884	0.188558255957096\\
2.16343328106621	0.190522639701337\\
2.17920327852358	0.192210475785579\\
2.18479604896912	0.192769296643771\\
2.19497327598095	0.194169831026281\\
2.21074327343832	0.196053430878126\\
2.22128646600077	0.197199870150995\\
2.22651327089568	0.19796331119021\\
2.24228326835305	0.200327239401527\\
2.25450889316976	0.201630443658218\\
2.25805326581042	0.202037936891298\\
2.27382326326779	0.204358725335447\\
2.28559223983337	0.206061017165442\\
2.28959326072516	0.206615189145123\\
2.30536325818253	0.208798126514091\\
2.31653191984929	0.210491590672665\\
2.3211332556399	0.211152590124456\\
2.33690325309727	0.213341766320206\\
2.34746697730794	0.214922164179889\\
2.35267325055464	0.215712597282407\\
2.368443248012	0.21799115476506\\
2.37782810337355	0.219352737687112\\
2.38421324546937	0.220377275904577\\
2.39998324292674	0.222789822188054\\
2.40620795317823	0.223783311194335\\
2.41575324038411	0.225349174929546\\
2.43152323784148	0.227544575683318\\
2.43605188209791	0.228213884701559\\
2.44729323529885	0.230162337572894\\
2.46306323275622	0.23253944343721\\
2.46376666685052	0.232644458208782\\
2.47883323021359	0.235380586630474\\
2.48998711599615	0.237075031716006\\
2.49460322767096	0.23808953549071\\
2.51037322512833	0.240926096760372\\
2.51398852900541	0.241505605223229\\
2.52614322258569	0.244443973650919\\
2.5345241844157	0.245936178730453\\
2.54191322004306	0.249106800400112\\
2.54657774576946	0.250366752237676\\
2.54191322004306	0.251337364382748\\
2.52614322258569	0.251843279219608\\
2.51037322512833	0.251350788960839\\
2.49460322767096	0.250604263722581\\
2.49094905970111	0.250366752237676\\
2.47883323021359	0.249171372849487\\
2.46306323275622	0.247736607943565\\
2.44729323529885	0.246501529719348\\
2.44019485621514	0.245936178730453\\
2.43152323784148	0.244926302855578\\
2.41575324038411	0.243198994643422\\
2.39998324292674	0.2418269844718\\
2.39647646694323	0.241505605223229\\
2.38421324546937	0.239896049412152\\
2.368443248012	0.238178485701407\\
2.35627370714983	0.237075031716006\\
2.35267325055464	0.236594797089134\\
2.33690325309727	0.234496083832374\\
2.3211332556399	0.232938672861887\\
2.31817730632847	0.232644458208782\\
2.30536325818253	0.230776005045454\\
2.28959326072516	0.228969790977013\\
2.28186331291372	0.228213884701559\\
2.27382326326779	0.227017091321223\\
2.25805326581042	0.224937371665195\\
2.24604239545236	0.223783311194335\\
2.24228326835305	0.223210107742054\\
2.22651327089568	0.220839513831004\\
2.21074327343832	0.219353213531735\\
2.21073979206265	0.219352737687112\\
2.19497327598095	0.216671071730454\\
2.17920327852358	0.215147061889922\\
2.17763064322863	0.214922164179889\\
2.16343328106621	0.212411451366666\\
2.14766328360884	0.210890688245491\\
2.1450707954061	0.210491590672665\\
2.13189328615147	0.208074126983379\\
2.1161232886941	0.206589761908488\\
2.11270654955836	0.206061017165442\\
2.10035329123673	0.203754653907818\\
2.08458329377936	0.202310028086405\\
2.08039138947353	0.201630443658218\\
2.06881329632199	0.199357458856252\\
2.05304329886463	0.19788361507099\\
2.04445917964541	0.197199870150995\\
2.03727330140726	0.196136804607062\\
2.02150330394989	0.193376775500834\\
2.012139748862	0.192769296643771\\
2.00573330649252	0.191943714856891\\
1.98996330903515	0.188753026591741\\
1.98258146614194	0.188338723136548\\
1.97419331157778	0.1874167131928\\
1.95879205374973	0.183908149629324\\
1.95842331412041	0.183820000213968\\
1.94265331666304	0.182698700424495\\
1.93099853609669	0.179477576122101\\
1.92688331920567	0.178438058275954\\
1.9111133217483	0.177781396849346\\
1.90116682122707	0.175047002614877\\
1.89534332429094	0.173535673212018\\
1.87957332683357	0.172476578026365\\
1.87292564616876	0.170616429107654\\
1.8638033293762	0.168126398315023\\
1.85581771154911	0.16618585560043\\
-4.60517018598809	121\\
1.85801489797829	0.16618585560043\\
1.8638033293762	0.165447653059367\\
1.87957332683357	0.16618585560043\\
1.88650666597412	0.16618585560043\\
1.89534332429094	0.168312541761308\\
1.9111133217483	0.170616429107654\\
1.92688331920567	0.169434020539003\\
1.94265331666304	0.170142932792547\\
1.95842331412041	0.170538243416511\\
1.96060673102984	0.170616429107654\\
1.97419331157778	0.172719528874376\\
1.98996330903515	0.174475520696081\\
2.00282499904743	0.175047002614877\\
2.00573330649252	0.175441836960629\\
2.02150330394989	0.177200125351567\\
2.03727330140726	0.17831198419178\\
2.04913948049459	0.179477576122101\\
2.05304329886463	0.179963239565844\\
2.06881329632199	0.181615190146395\\
2.08458329377936	0.183204417201149\\
2.0927220257765	0.183908149629324\\
2.10035329123673	0.184823037776728\\
2.1161232886941	0.186595070243263\\
2.13189328615147	0.188178308960859\\
2.13361132563048	0.188338723136548\\
2.14766328360884	0.190157317441309\\
2.16343328106621	0.191918393078718\\
2.1716992776963	0.192769296643771\\
2.17920327852358	0.193785606191493\\
2.19497327598095	0.195893325725171\\
2.20699215606282	0.197199870150995\\
2.21074327343832	0.197679625652858\\
2.22651327089568	0.199980553180936\\
2.23777759226658	0.201630443658218\\
2.24228326835305	0.202240182537641\\
2.25805326581042	0.20412692671898\\
2.27121004909597	0.206061017165442\\
2.27382326326779	0.206432570596794\\
2.28959326072516	0.208612591054746\\
2.30263356836376	0.210491590672665\\
2.30536325818253	0.210904937143425\\
2.3211332556399	0.213150421033181\\
2.33371352757228	0.214922164179889\\
2.33690325309727	0.215431950521009\\
2.35267325055464	0.217781657210082\\
2.36378366382276	0.219352737687112\\
2.368443248012	0.220140810470634\\
2.38421324546937	0.222586745109142\\
2.39222388402531	0.223783311194335\\
2.39998324292674	0.225147615603633\\
2.41575324038411	0.227497014932275\\
2.42090638896849	0.228213884701559\\
2.43152323784148	0.2302791163899\\
2.44705131941071	0.232644458208782\\
2.44729323529885	0.232702320096163\\
2.46306323275622	0.23587002578286\\
2.4707150452136	0.237075031716006\\
2.47883323021359	0.239323572067101\\
2.49040791184043	0.241505605223229\\
2.49460322767096	0.245486101956046\\
2.49553930683744	0.245936178730453\\
2.49460322767096	0.246010456519713\\
2.47883323021359	0.246138661867495\\
2.47331216114562	0.245936178730453\\
2.46306323275622	0.245250334636456\\
2.44729323529885	0.243972856486384\\
2.43152323784148	0.242808163786775\\
2.41575324038411	0.241735476984582\\
2.41282554285524	0.241505605223229\\
2.39998324292674	0.239992018149768\\
2.38421324546937	0.238416205345549\\
2.368443248012	0.237158027058312\\
2.36752792646445	0.237075031716006\\
2.35267325055464	0.235093691418123\\
2.33690325309727	0.233486487132226\\
2.32752723428152	0.232644458208782\\
2.3211332556399	0.231776483673889\\
2.30536325818253	0.22977651737732\\
2.28959326072516	0.228320634718783\\
2.28850162795427	0.228213884701559\\
2.27382326326779	0.22602895171426\\
2.25805326581042	0.224321611623688\\
2.25245091061856	0.223783311194335\\
2.24228326835305	0.222232917314537\\
2.22651327089568	0.220259603653843\\
2.21689019721723	0.219352737687112\\
2.21074327343832	0.218386640869063\\
2.19497327598095	0.216127795933872\\
2.18183961084742	0.214922164179889\\
2.17920327852358	0.214493873835752\\
2.16343328106621	0.211909935847581\\
2.14766328360884	0.210510701670072\\
2.14753914094626	0.210491590672665\\
2.13189328615147	0.207621299700116\\
2.1161232886941	0.206230223590894\\
2.115029879779	0.206061017165442\\
2.10035329123673	0.203320886288241\\
2.08458329377936	0.201972388304782\\
2.08247406470225	0.201630443658218\\
2.06881329632199	0.198948592812392\\
2.05304329886463	0.197557410347665\\
2.0485545376554	0.197199870150995\\
2.03727330140726	0.195530944913062\\
2.02150330394989	0.193060076377359\\
2.01702128449812	0.192769296643771\\
2.00573330649252	0.19131464388727\\
1.98996330903515	0.18844092586135\\
1.98814231418635	0.188338723136548\\
1.97419331157778	0.186805475386748\\
1.961475154932	0.183908149629324\\
1.95842331412041	0.183178588817537\\
1.94265331666304	0.182112155809021\\
1.93312079160253	0.179477576122101\\
1.92688331920567	0.177901969284579\\
1.9111133217483	0.177217386606732\\
1.90321843766973	0.175047002614877\\
1.89534332429094	0.173003232259927\\
1.87957332683357	0.171929234999018\\
1.87488170550536	0.170616429107654\\
1.8638033293762	0.167592471672142\\
1.85801489797829	0.16618585560043\\
-3.83764182165674	109\\
1.86021208440747	0.16618585560043\\
1.8638033293762	0.165727861719315\\
1.87957332683357	0.16618585560043\\
1.88437116022101	0.16618585560043\\
1.89534332429094	0.168826486101892\\
1.9111133217483	0.170616429107654\\
1.92688331920567	0.170201685420587\\
1.93753155877119	0.170616429107654\\
1.94265331666304	0.170883496661697\\
1.95842331412041	0.171552012042803\\
1.97419331157778	0.173715072654483\\
1.98996330903515	0.174872007036002\\
1.99390173440783	0.175047002614877\\
2.00573330649252	0.176653267121458\\
2.02150330394989	0.17815742344445\\
2.03727330140726	0.179348282477244\\
2.03858956098732	0.179477576122101\\
2.05304329886463	0.181275726406537\\
2.06881329632199	0.18280243627479\\
2.08041922834853	0.183908149629324\\
2.08458329377936	0.184441733442867\\
2.10035329123673	0.186288419277704\\
2.1161232886941	0.187905980818236\\
2.12049402366562	0.188338723136548\\
2.13189328615147	0.189820410851111\\
2.14766328360884	0.191756378925522\\
2.15742041726093	0.192769296643771\\
2.16343328106621	0.193519086094855\\
2.17920327852358	0.19562196143921\\
2.19150872776088	0.197199870150995\\
2.19497327598095	0.197671510708223\\
2.21074327343832	0.199707350779211\\
2.22397298286372	0.201630443658218\\
2.22651327089568	0.201989999134856\\
2.24228326835305	0.204103950480569\\
2.25701311167833	0.206061017165442\\
2.25805326581042	0.206221144320915\\
2.27382326326779	0.208453055167512\\
2.28871813838193	0.210491590672665\\
2.28959326072516	0.210631232631168\\
2.30536325818253	0.213004010131938\\
2.31939549737239	0.214922164179889\\
2.3211332556399	0.21521954206622\\
2.33690325309727	0.217699114205985\\
2.34876059280645	0.219352737687112\\
2.35267325055464	0.220067317295853\\
2.368443248012	0.22261551878485\\
2.37644227292473	0.223783311194335\\
2.38421324546937	0.225303618272135\\
2.39998324292674	0.227748396956136\\
2.40332263866195	0.228213884701559\\
2.41575324038411	0.230915013851707\\
2.42628055459789	0.232644458208782\\
2.43152323784148	0.234494531573524\\
2.44418417592485	0.237075031716006\\
2.43152323784148	0.239001798930835\\
2.41575324038411	0.238598984693095\\
2.39998324292674	0.237795154255958\\
2.38771915013982	0.237075031716006\\
2.38421324546937	0.23672068450269\\
2.368443248012	0.234972734488395\\
2.35267325055464	0.233592585747112\\
2.34018490191962	0.232644458208782\\
2.33690325309727	0.232243954394631\\
2.3211332556399	0.23025041110651\\
2.30536325818253	0.228777029709186\\
2.29901199671291	0.228213884701559\\
2.28959326072516	0.226909990667745\\
2.27382326326779	0.225040812107296\\
2.25947188974069	0.223783311194335\\
2.25805326581042	0.223580661899997\\
2.24228326835305	0.22125572688702\\
2.22651327089568	0.219679693476683\\
2.22304382803636	0.219352737687112\\
2.21074327343832	0.217419489922079\\
2.19497327598095	0.21558452013729\\
2.18775783783827	0.214922164179889\\
2.17920327852358	0.213532417098422\\
2.16343328106621	0.211408420328497\\
2.15305486397464	0.210491590672665\\
2.14766328360884	0.209588027741079\\
2.13189328615147	0.207168472416854\\
2.11892941644899	0.206061017165442\\
2.1161232886941	0.205558726956191\\
2.10035329123673	0.202887118668665\\
2.08458329377936	0.201634748523159\\
2.08455673993096	0.201630443658218\\
2.06881329632199	0.198539726768533\\
2.05304329886463	0.19723120562434\\
2.05264989566539	0.197199870150995\\
2.03727330140726	0.194925085219063\\
2.02185787186915	0.192769296643771\\
2.02150330394989	0.192696886459295\\
2.00573330649252	0.190685572917648\\
1.99237197989597	0.188338723136548\\
1.98996330903515	0.187808222634984\\
1.97419331157778	0.186194237580696\\
1.96415825611428	0.183908149629324\\
1.95842331412041	0.182537177421106\\
1.94265331666304	0.181525611193546\\
1.93524304710836	0.179477576122101\\
1.92688331920567	0.177365880293204\\
1.9111133217483	0.176653376364118\\
1.90527005411238	0.175047002614877\\
1.89534332429094	0.172470791307836\\
1.87957332683357	0.171381891971671\\
1.87683776484196	0.170616429107654\\
1.8638033293762	0.167058545029261\\
1.86021208440747	0.16618585560043\\
-3.07011345732539	101\\
1.86240927083665	0.16618585560043\\
1.8638033293762	0.166008070379264\\
1.87957332683357	0.16618585560043\\
1.88223565446791	0.16618585560043\\
1.89534332429094	0.169340430442476\\
1.9111133217483	0.170616429107654\\
1.92424802746745	0.170616429107654\\
1.92688331920567	0.171154535377665\\
1.94265331666304	0.171911209510272\\
1.95842331412041	0.172968465779992\\
1.97419331157778	0.17471061643459\\
1.98013687020485	0.175047002614877\\
1.98996330903515	0.175865148970803\\
2.00573330649252	0.177864697282287\\
2.02150330394989	0.179114721537333\\
2.02626897571676	0.179477576122101\\
2.03727330140726	0.18082278105224\\
2.05304329886463	0.182588213247229\\
2.06780525719622	0.183908149629324\\
2.06881329632199	0.184028176745403\\
2.08458329377936	0.186038580533389\\
2.10035329123673	0.187753800778681\\
2.10624145933399	0.188338723136548\\
2.1161232886941	0.189567005124404\\
2.13189328615147	0.191541399866354\\
2.14231109336015	0.192769296643771\\
2.14766328360884	0.193472718723863\\
2.16343328106621	0.195439837713001\\
2.17710364026825	0.197199870150995\\
2.17920327852358	0.197492716459336\\
2.19497327598095	0.19962107172946\\
2.20999139354227	0.201630443658218\\
2.21074327343832	0.201744358647898\\
2.22651327089568	0.20396443065052\\
2.24228326835305	0.205967718423498\\
2.24298548042477	0.206061017165442\\
2.25805326581042	0.208380636478234\\
2.27382326326779	0.210473539738229\\
2.27395515521347	0.210491590672665\\
2.28959326072516	0.212986939691936\\
2.30386582193111	0.214922164179889\\
2.30536325818253	0.215211364922454\\
2.3211332556399	0.217847330176383\\
2.3318437653076	0.219352737687112\\
2.33690325309727	0.220430112262364\\
2.35267325055464	0.223036331442245\\
2.35776187197539	0.223783311194335\\
2.368443248012	0.226335208170046\\
2.38043651773865	0.228213884701559\\
2.38421324546937	0.230920971258684\\
2.39010077575854	0.232644458208782\\
2.38421324546937	0.232939210727465\\
2.368443248012	0.232684317038382\\
2.36773127959339	0.232644458208782\\
2.35267325055464	0.231070643032279\\
2.33690325309727	0.229830916893526\\
2.3211332556399	0.228724338539132\\
2.31429212933837	0.228213884701559\\
2.30536325818253	0.227085552997982\\
2.28959326072516	0.225349479545032\\
2.27382326326779	0.224052672500332\\
2.2707491464411	0.223783311194335\\
2.25805326581042	0.221969714795795\\
2.24228326835305	0.220278536459504\\
2.23148492748246	0.219352737687112\\
2.22651327089568	0.218619680048677\\
2.21074327343832	0.216452338975096\\
2.19497327598095	0.215041244340708\\
2.19367606482913	0.214922164179889\\
2.17920327852358	0.212570960361093\\
2.16343328106621	0.210906904809412\\
2.15873196789667	0.210491590672665\\
2.14766328360884	0.208636614553352\\
2.13189328615147	0.206715645133591\\
2.12423021202557	0.206061017165442\\
2.1161232886941	0.204609897126645\\
2.10035329123673	0.202453351049088\\
2.08998099037516	0.201630443658218\\
2.08458329377936	0.200652633434046\\
2.06881329632199	0.198130860724673\\
2.05752470829853	0.197199870150995\\
2.05304329886463	0.196341466451176\\
2.03727330140726	0.194319225525063\\
2.02619020182482	0.192769296643771\\
2.02150330394989	0.191812134076848\\
2.00573330649252	0.190056501948027\\
1.99595347145338	0.188338723136548\\
1.98996330903515	0.187019412881667\\
1.97419331157778	0.185582999774644\\
1.96684135729656	0.183908149629324\\
1.95842331412041	0.181895766024675\\
1.94265331666304	0.180939066578072\\
1.93736530261419	0.179477576122101\\
1.92688331920567	0.176829791301829\\
1.9111133217483	0.176089366121505\\
1.90732167055504	0.175047002614877\\
1.89534332429094	0.171938350355746\\
1.87957332683357	0.170834548944324\\
1.87879382417856	0.170616429107654\\
1.8638033293762	0.16652461838638\\
1.86240927083665	0.16618585560043\\
-2.30258509299405	5\\
1.87321876440813	0.16618585560043\\
1.87957332683357	0.16618585560043\\
1.88010014871481	0.16618585560043\\
1.87957332683357	0.167474490574209\\
1.87321876440813	0.16618585560043\\
-2.30258509299405	83\\
1.884124387963	0.170616429107654\\
1.89534332429094	0.169854374783059\\
1.9111133217483	0.170616429107654\\
1.91851581032777	0.170616429107654\\
1.92688331920567	0.17232500995518\\
1.94265331666304	0.172938922358846\\
1.95842331412041	0.174384919517182\\
1.96494926086479	0.175047002614877\\
1.97419331157778	0.175953867767554\\
1.98996330903515	0.177329696984679\\
2.00573330649252	0.179076127443116\\
2.01122074333392	0.179477576122101\\
2.02150330394989	0.180501824991254\\
2.03727330140726	0.182359745142928\\
2.05304329886463	0.183900700087922\\
2.05312661334953	0.183908149629324\\
2.06881329632199	0.185775961373823\\
2.08458329377936	0.187635427623911\\
2.09125357249517	0.188338723136548\\
2.10035329123673	0.189474112800211\\
2.1161232886941	0.191400557902833\\
2.12751931170867	0.192769296643771\\
2.13189328615147	0.193363988555157\\
2.14766328360884	0.195391727712335\\
2.16214704078806	0.197199870150995\\
2.16343328106621	0.19739855111135\\
2.17920327852358	0.1995734944166\\
2.19497327598095	0.201570632750698\\
2.19542030483993	0.201630443658218\\
2.21074327343832	0.20395197907756\\
2.22651327089568	0.205938862166184\\
2.22747754866582	0.206061017165442\\
2.24228326835305	0.208467228556879\\
2.25762188082239	0.210491590672665\\
2.25805326581042	0.210581493710023\\
2.27382326326779	0.213321854967857\\
2.28578357127613	0.214922164179889\\
2.28959326072516	0.215852104828674\\
2.30536325818253	0.218566754165242\\
2.31094874384061	0.219352737687112\\
2.3211332556399	0.222366791833091\\
2.32996426785278	0.223783311194335\\
2.3211332556399	0.224810003216982\\
2.30536325818253	0.224500993372346\\
2.28959326072516	0.22378896842232\\
2.28951505604823	0.223783311194335\\
2.27382326326779	0.221711662149737\\
2.25805326581042	0.220358767691593\\
2.24350816769914	0.219352737687112\\
2.24228326835305	0.21918349000875\\
2.22651327089568	0.216939109930781\\
2.21074327343832	0.215485188028112\\
2.20400758818382	0.214922164179889\\
2.19497327598095	0.21353332650055\\
2.17920327852358	0.211609503623764\\
2.16546426775586	0.210491590672665\\
2.16343328106621	0.210166618670556\\
2.14766328360884	0.207685201365625\\
2.13189328615147	0.206262817850328\\
2.12953100760215	0.206061017165442\\
2.1161232886941	0.203661067297099\\
2.10035329123673	0.202019583429511\\
2.09544839570433	0.201630443658218\\
2.08458329377936	0.199662195246999\\
2.06881329632199	0.197721994680814\\
2.06248235282943	0.197199870150995\\
2.05304329886463	0.195391841010681\\
2.03727330140726	0.193713365831063\\
2.03052253178049	0.192769296643771\\
2.02150330394989	0.190927381694402\\
2.00573330649252	0.189427430978405\\
1.99953496301079	0.188338723136548\\
1.98996330903515	0.186230603128349\\
1.97419331157778	0.184971761968593\\
1.96952445847884	0.183908149629324\\
1.95842331412041	0.181254354628244\\
1.94265331666304	0.180352521962597\\
1.93948755812003	0.179477576122101\\
1.92688331920567	0.176293702310454\\
1.9111133217483	0.175525355878891\\
1.90937328699769	0.175047002614877\\
1.89534332429094	0.171405909403655\\
1.884124387963	0.170616429107654\\
-1.5350567286627	7\\
1.89169065803984	0.170616429107654\\
1.89534332429094	0.170368319123643\\
1.9111133217483	0.170616429107654\\
1.91278359318808	0.170616429107654\\
1.9111133217483	0.173528964789161\\
1.89534332429094	0.170873468451564\\
1.89169065803984	0.170616429107654\\
-1.5350567286627	65\\
1.91273440064155	0.175047002614877\\
1.92688331920567	0.173495484532695\\
1.94265331666304	0.17396663520742\\
1.95312045038673	0.175047002614877\\
1.95842331412041	0.176071728957741\\
1.97419331157778	0.177323531050492\\
1.98996330903515	0.178794244998554\\
1.99644499205898	0.179477576122101\\
2.00573330649252	0.18063981789866\\
2.02150330394989	0.182151286169134\\
2.03727330140726	0.183896709233616\\
2.03739047829686	0.183908149629324\\
2.05304329886463	0.185748858781071\\
2.06881329632199	0.187523746002243\\
2.07598131907223	0.188338723136548\\
2.08458329377936	0.189523548482413\\
2.10035329123673	0.191363784822533\\
2.11211466147038	0.192769296643771\\
2.1161232886941	0.193411300766867\\
2.13189328615147	0.195439580439266\\
2.14665752794778	0.197199870150995\\
2.14766328360884	0.197383776480418\\
2.16343328106621	0.199772983184326\\
2.1789757504004	0.201630443658218\\
2.17920327852358	0.201676198540795\\
2.19497327598095	0.204263024079959\\
2.20974675876199	0.206061017165442\\
2.21074327343832	0.206311039551157\\
2.22651327089568	0.209135599977341\\
2.23713035635347	0.210491590672665\\
2.24228326835305	0.21218640158303\\
2.25805326581042	0.214581350575527\\
2.26061353157294	0.214922164179889\\
2.25805326581042	0.215741579999553\\
2.24228326835305	0.215965317510281\\
2.22651327089568	0.215258539812885\\
2.22140581268443	0.214922164179889\\
2.21074327343832	0.213332391268972\\
2.19497327598095	0.211754614432449\\
2.17920327852358	0.210648046886435\\
2.17728045116609	0.210491590672665\\
2.16343328106621	0.208275947106991\\
2.14766328360884	0.206733788177898\\
2.13882335732575	0.206061017165442\\
2.13189328615147	0.204864556220045\\
2.1161232886941	0.202712237467553\\
2.10165856828144	0.201630443658218\\
2.10035329123673	0.201388199898892\\
2.08458329377936	0.198671757059953\\
2.06881329632199	0.197313128636954\\
2.06743999736032	0.197199870150995\\
2.05304329886463	0.194442215570185\\
2.03727330140726	0.193107506137063\\
2.03485486173617	0.192769296643771\\
2.02150330394989	0.190042629311955\\
2.00573330649252	0.188798360008783\\
2.0031164545682	0.188338723136548\\
1.98996330903515	0.185441793375031\\
1.97419331157778	0.184360524162541\\
1.97220755966112	0.183908149629324\\
1.95842331412041	0.180612943231813\\
1.94265331666304	0.179765977347123\\
1.94160981362586	0.179477576122101\\
1.92688331920567	0.175757613319078\\
1.91273440064155	0.175047002614877\\
-0.767528364331349	7\\
1.92340842994796	0.175047002614877\\
1.92688331920567	0.17466595911021\\
1.94265331666304	0.174994348055994\\
1.94316346006906	0.175047002614877\\
1.94265331666304	0.175452691826785\\
1.92688331920567	0.175221524327703\\
1.92340842994796	0.175047002614877\\
-0.767528364331349	39\\
1.94892356662775	0.179477576122101\\
1.95842331412041	0.177995819559836\\
1.97419331157778	0.17869319433343\\
1.98235820787703	0.179477576122101\\
1.98996330903515	0.181076953030382\\
2.00573330649252	0.182378098061675\\
2.02150330394989	0.183800747347014\\
2.02247415549737	0.183908149629324\\
2.03727330140726	0.186115160837418\\
2.05304329886463	0.187600075248619\\
2.05978955460452	0.188338723136548\\
2.06881329632199	0.189927019108804\\
2.08458329377936	0.191640924751613\\
2.09523306847705	0.192769296643771\\
2.10035329123673	0.193866025566212\\
2.1161232886941	0.195943815598001\\
2.12819567251978	0.197199870150995\\
2.13189328615147	0.198234745345945\\
2.14766328360884	0.200567044109846\\
2.15721070939432	0.201630443658218\\
2.14766328360884	0.203991267175805\\
2.13189328615147	0.202706258402451\\
2.1161232886941	0.201763407638007\\
2.11434542051257	0.201630443658218\\
2.10035329123673	0.199033672336381\\
2.08458329377936	0.197681318872906\\
2.07824320220912	0.197199870150995\\
2.06881329632199	0.195290967628394\\
2.05304329886463	0.19349259012969\\
2.04306233257738	0.192769296643771\\
2.03727330140726	0.191411734587928\\
2.02150330394989	0.189157876929509\\
2.00928710981833	0.188338723136548\\
2.00573330649252	0.187300637505288\\
1.98996330903515	0.184652983621713\\
1.97759710065903	0.183908149629324\\
1.97419331157778	0.18252508037002\\
1.95842331412041	0.179971531835381\\
1.94892356662775	0.179477576122101\\
-0.767528364331349	7\\
2.15760907464273	0.206061017165442\\
2.16343328106621	0.204108790440908\\
2.17920327852358	0.205671619549475\\
2.18273297482284	0.206061017165442\\
2.17920327852358	0.206522975981252\\
2.16343328106621	0.206385275543427\\
2.15760907464273	0.206061017165442\\
0	3\\
2.03727330140726	0.188338723136548\\
2.03727330140726	0.188338723136548\\
2.03727330140726	0.188338723136548\\
0	3\\
2.03727330140726	0.188338723136548\\
2.03727330140726	0.188338723136548\\
2.03727330140726	0.188338723136548\\
};
\end{axis}

==> fig9_part2_220222.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.447000,0.44700,0.4474100}%
%
\begin{axis}[%
width=0.7\linewidth,
height=0.5\linewidth,
at={(mv.below south west)},
anchor = above north west,
scale only axis,
xmin=1.7085,
xmax=3.4,
ymin=0,
ymax=4,
xlabel = $\CIntensity_\infty$,
ylabel = ACID,
axis background/.style={fill=white}
]
\addplot[ybar interval, fill=mycolor3, fill opacity=0.6, draw=black, area legend] table[row sep=crcr] {%
x	y\\
1.76	0.0475728155339807\\
1.7703	0.183495145631068\\
1.7806	0.346601941747574\\
1.7909	0.582524271844662\\
1.8012	0.804854368932023\\
1.8115	0.990291262135925\\
1.8218	1.24174757281554\\
1.8321	1.57087378640777\\
1.8424	1.80679611650486\\
1.8527	2.12718446601942\\
1.863	2.46990291262136\\
1.8733	2.71941747572816\\
1.8836	2.89417475728156\\
1.8939	3.10097087378642\\
1.9042	3.10873786407761\\
1.9145	3.45728155339807\\
1.9248	3.53786407766991\\
1.9351	3.48058252427185\\
1.9454	3.58349514563108\\
1.9557	3.62038834951457\\
1.966	3.52135922330098\\
1.9763	3.51262135922331\\
1.9866	3.47378640776692\\
1.9969	3.40776699029127\\
2.0072	3.29611650485438\\
2.0175	3.11553398058253\\
2.0278	3.07864077669904\\
2.0381	2.77281553398059\\
2.0484	2.57961165048544\\
2.0587	2.46699029126214\\
2.069	2.29708737864078\\
2.0793	2.16407766990292\\
2.0896	1.98058252427185\\
2.0999	1.85145631067962\\
2.1102	1.66407766990292\\
2.1205	1.53786407766991\\
2.1308	1.36407766990292\\
2.1411	1.23398058252422\\
2.1514	1.16699029126214\\
2.1617	1.01844660194175\\
2.172	0.942718446601944\\
2.1823	0.804854368932041\\
2.1926	0.727184466019419\\
2.2029	0.679611650485438\\
2.2132	0.556310679611652\\
2.2235	0.574757281553399\\
2.2338	0.484466019417477\\
2.2441	0.400970873786409\\
2.2544	0.340776699029127\\
2.2647	0.350485436893205\\
2.275	0.256310679611651\\
2.2853	0.244660194174758\\
2.2956	0.2135922330097\\
2.3059	0.183495145631068\\
2.3162	0.173786407766991\\
2.3265	0.133980582524272\\
2.3368	0.118446601941748\\
2.3471	0.0873786407766992\\
2.3574	0.0922330097087381\\
2.3677	0.0844660194174759\\
2.378	0.0660194174757283\\
2.3883	0.0737864077669905\\
2.3986	0.0485436893203885\\
2.4089	0.0436893203883496\\
2.4192	0.037864077669903\\
2.4295	0.0300970873786408\\
2.4398	0.0242718446601942\\
2.4501	0.0213592233009709\\
2.4604	0.0194174757281554\\
2.4707	0.0145631067961165\\
2.481	0.0165048543689321\\
2.4913	0.00970873786407769\\
2.5016	0.00388349514563108\\
2.5119	0.012621359223301\\
2.5222	0.00485436893203885\\
2.5325	0.00582524271844636\\
2.5428	0.000970873786407769\\
2.5531	0.00291262135922331\\
2.5634	0.00582524271844662\\
2.5737	0.00194174757281554\\
2.584	0.00194174757281554\\
2.5943	0.00388349514563108\\
2.6046	0.000970873786407769\\
2.6149	0\\
2.6252	0.000970873786407769\\
2.6355	0.00194174757281554\\
2.6458	0.000970873786407769\\
2.6561	0.000970873786407769\\
2.6664	0\\
2.6767	0\\
2.687	0.000970873786407769\\
2.6973	0\\
2.7076	0\\
2.7179	0\\
2.7282	0\\
2.7385	0\\
2.7488	0\\
2.7591	0\\
2.7694	0\\
2.7797	0.000970873786407769\\
2.79	0.000970873786407769\\
};\addlegendentry{Monte Carlo samples};
\addplot [color=mycolor1, line width = 1pt]
  table[row sep=crcr]{%
1.76918334463198	0.10285114710848\\
1.78495334208935	0.363502447734539\\
1.80072333954672	0.674122138631273\\
1.81649333700409	1.02626556022878\\
1.83226333446146	1.41825139384779\\
1.8638033293762	2.27980997175717\\
1.87957332683357	2.67028058815216\\
1.89534332429094	3.00126185896589\\
1.9111133217483	3.26538184638407\\
1.92688331920567	3.45589895132093\\
1.94265331666304	3.56695120942892\\
1.95842331412041	3.59843360378473\\
1.97419331157778	3.55772486985581\\
1.98996330903515	3.45505066776132\\
2.00573330649252	3.3012446864634\\
2.02150330394989	3.10740781959115\\
2.03727330140726	2.88487636433801\\
2.05304329886463	2.64461055221179\\
2.08458329377936	2.14790987877696\\
2.10035329123673	1.9059414454516\\
2.1161232886941	1.67535917316819\\
2.13189328615147	1.45930039628248\\
2.14766328360884	1.26044254801997\\
2.16343328106621	1.08049950443098\\
2.17920327852358	0.919427595633987\\
2.19497327598095	0.77691546229736\\
2.21074327343832	0.652153244685043\\
2.22651327089568	0.544012477883776\\
2.24228326835305	0.451137112787313\\
2.25805326581042	0.372019035394927\\
2.27382326326779	0.305130951099371\\
2.28959326072516	0.248990407105708\\
2.30536325818253	0.202190533858719\\
2.3211332556399	0.163425285478479\\
2.33690325309727	0.131506202997301\\
2.35267325055464	0.105371498871939\\
2.368443248012	0.0840869695119633\\
2.38421324546937	0.0668403751088475\\
2.39998324292674	0.0529329312680655\\
2.41575324038411	0.0417691848437967\\
2.43152323784148	0.0328467375806496\\
2.44729323529885	0.0257451921626255\\
2.46306323275622	0.0201152744975124\\
2.47883323021359	0.0156675590307973\\
2.49460322767096	0.0121670721760565\\
2.51037322512833	0.00942289774319427\\
2.52614322258569	0.0072779858729608\\
2.54191322004306	0.00560678375063128\\
2.5734532149578	0.00329985226649665\\
2.60499320987254	0.0019247881326967\\
2.65230320224465	0.000843336962702779\\
2.71538319207412	0.000272992493113744\\
2.85731316919044	1.95605422907974e-05\\
3.33041309291151	9.02756536191873e-10\\
};\addlegendentry{parametrization $(M, \beta)$};
\addplot [color=mycolor2, line width = 1pt]
  table[row sep=crcr]{%
1.76918334463198	1.80024737841622\\
1.80072333954672	2.39280999514266\\
1.81649333700409	2.6167611481036\\
1.83226333446146	2.80107456903665\\
1.84803333191883	2.95907701887951\\
1.8638033293762	3.08779334400984\\
1.87957332683357	3.17817996612899\\
1.89534332429094	3.22828904205434\\
1.9111133217483	3.23898097030234\\
1.92688331920567	3.20966004968485\\
1.94265331666304	3.14084825364146\\
1.95842331412041	3.03447046149277\\
1.97419331157778	2.8958797711882\\
1.98996330903515	2.73129987570912\\
2.00573330649252	2.5470282935976\\
2.02150330394989	2.34928628640369\\
2.06881329632199	1.73408456572153\\
2.08458329377936	1.53795092854427\\
2.10035329123673	1.35228883653967\\
2.1161232886941	1.17925431110886\\
2.13189328615147	1.02029649650224\\
2.14766328360884	0.876228464910356\\
2.16343328106621	0.747161536277427\\
2.17920327852358	0.632791979761479\\
2.19497327598095	0.532477563295538\\
2.21074327343832	0.445296932440173\\
2.22651327089568	0.370199470356184\\
2.24228326835305	0.30603717131623\\
2.25805326581042	0.251626820528162\\
2.27382326326779	0.205824582223903\\
2.28959326072516	0.167534012181186\\
2.30536325818253	0.135721951456278\\
2.3211332556399	0.109450318415525\\
2.33690325309727	0.0878817628489728\\
2.35267325055464	0.0702692036391843\\
2.368443248012	0.0559618481444386\\
2.38421324546937	0.0443973147005754\\
2.39998324292674	0.0350919486534829\\
2.41575324038411	0.0276385477334302\\
2.43152323784148	0.0216940508817656\\
2.44729323529885	0.0169717593318648\\
2.46306323275622	0.0132355256476964\\
2.47883323021359	0.0102902635101643\\
2.49460322767096	0.00797669563750114\\
2.51037322512833	0.00616575087290849\\
2.54191322004306	0.00365414266356678\\
2.5734532149578	0.00214363032634335\\
2.62076320732991	0.00094628576415845\\
2.68384319715938	0.000308745775965402\\
2.81000317681834	3.01326922031997e-05\\
3.33041309291151	5.06983788284288e-10\\
};\addlegendentry{parametrization $(M,V)$};

\end{axis}
